Cartesian institutions with evidence: Data and system modelling with diagrammatic constraints and generalized sketches

Data constraints are fundamental for practical data modelling, and a verifiable conformance of a data instance to a safety-critical constraint (satisfaction relation) is a corner-stone of safety assurance. Diagrammatic constraints are important as both a theoretical concepts and a practically convenient device. The paper shows that basic formal constraint management can well be developed within a finitely complete category (hence the reference to Cartesianity in the title). In the data modelling context, objects of such a category can be thought of as graphs, while their morphisms play two roles: of data instances and (when being additionally labelled) of constraints. Specifically, a generalized sketch $S$ consists of a graph $G_S$ and a set of constraints $C_S$ declared over $G_S$, and appears as a pattern for typical data schemas (in databases, XML, and UML class diagrams). Interoperability of data modelling frameworks (and tools based on them) very much depends on the laws regulating the transformation of satisfaction relations between data instances and schemas when the schema graph changes: then constraints are translated co- whereas instances contra-variantly. Investigation of this transformation pattern is the main mathematical subject of the paper

==> ShortLongTricks.tex <==
% Definitions to control different outputs
\newtoggle{long}
\NewEnviron{includeLong}
{\iftoggle{long}{\BODY}{}}
\NewEnviron{includeShort}
{\iftoggle{long}{}{\BODY}}

% Set the desired output version TRUE = long journal version, FALSE = short ACT version

% comment this and uncomment the other line below to produce the short ACT version
\toggletrue{long}

\newcommand{\shortlong}[2]{#1}   % produces the short version (going first)
\renewcommand{\shortlong}[2]{#2}   % produces the long version (going second)


% comment this and uncomment the other line above to produce the long journal/onlune version
%\togglefalse{long}
\input{lstlistinglibrary}

%== Traceability commands
\newcommand{\traceLong}[1]{\mynoteColored{Tracing incLong}{#1}{blue}}
%  trace includeLong
\renewenvironment{includeLong}{\par \traceLong{includeLong Starts here}}{\par\traceLong{includeLong Ends here}}
%--- do nothing
\renewenvironment{includeLong}{}{}


==> abstract4theTalk.tex <==
%\clearpage

Constraints are fundamental for data modelling: they keep data integrity and ensure safety. If $D$ is a data instance over schema $S$, then adding a {\em constraint} $c$ to $S$ classifies $S$-instances into {\em valid} (and then we write $D\vDash c$) or (otherwise) invalid. Many constraint specification languages were developed, % in string-based logics, 
\eg, FOL and its fragments, database dependencies, or the OCL (Object Constraint Language) widely used in the UML/EML software development ecosystem, %and in diagrammatic logics, \eg, injectivity \cite{adamek-injLogic-2007} or lifting constraints \cite{spivak-lifting14}  popular within the ACT community. This diversity does
which does contribute to the problems of software interoperability and model management (cf. \cite{spivak-algMMt-arxiv16}) and calls for a unifying abstract \fwk.

%--- this piece is for a longer manner 
%A {\em constraint} $c$ declared over schema $S$  is a device that classifies all instances over $S$ into {\em valid} (we then write $D\vDash c$) and (otherwise) {\em invalid}. Such a classification plays at least two important roles. i) Applications usually assume that data do satisfy some constraints $c', c'',...$ so that it makes sense to include them into schema $S^+= (S, c', c'')$ and disallow instances that violate constraints upfront (this is often called data integrity). ii) In safety-critical applications, there are constraints whose violation can compromise safety and thus instances violating such are to be prohibited.
%
%Moreover, there are constraints that cannot de decomposed ... no syntax???
% 

Developing such a \fwk\ can be traced back to so called {\em abstract model theory} \cite{barwise-axioms4amt-AML74} and, more recently, Goguen \& Burstall's {\em institutions}  \cite{GoguenBurstall-jofacm92}. 
%Studying binary \satty\ relation $\vDash$ is a classical subject of mathematical logic. %, in which constraints are logical sentences. 
%
% Attempts to develop such a theory %for purely mathematical reasons can be traced back to {\em abstract model theory} \cite{barwise-axioms4amt-AML74} and, more recently, Goguen and Burstall's {\em institutions} \cite{Goguen-Burstall-92}. 
%
The latter are practically a bare-bone \fwk\ for describing translation of a binary satisfaction relation (further called {\em Sat}),  $\satrelsig\subset \Modsetsig \timm \Sensetsig$,  between  sets   \Modsetsig\ of {\em \Sigmaa-models} and \Sensetsig\ of {\em \Sigmaa-sentences} (\ie, constraints),  when the logical signature \Sigmaa\ (of, say, relation and function symbols) 
changes. 
%({\em \satrelsymbol-interoperability} in the technological speak). 
If such changes are specified by a signature \mor\ \frar{f}{\Sigmaa}{\Sigmaa'}, then the main and, in fact, the only substantial postulate of the institution theory states that Sat is preserved in a twisted way: for models with a function  \frar{f^*}{\ModsetsigPrim}{\Modsetsig} in the direction opposite to $f$, for sentences with \frar{f_*}{\Sensetsig}{\SensetsigPrim} in the same direction, and for all $m'\in\ModsetsigPrim$ and all $\phi\in\Sensetsig$, the {\em twisted Sat  
condition} \fbox{$f^*(m')\satrelsig \phi \text{~iff~} m'\satrelsigPrim f_*(\phi)$}
holds. 
%%
%%\input{diagrams/satAxiom-Rel}
%%
%%\input{sections/piece--aboutInstit4briefExpo}
%%%specified in \cref{eqdiag:satisfyAxiom} holds. 
%Logicians refers to the Sat-axiom above as to `{The invariance of truth under language translations}'; it may also be termed technologically as `{The main law of Sat-interoperability}'. 

There is a major deficiency of the  \instfwk\ wrt. its application to software interoperability, where models become many-sorted data instances, and sentences are sort-spanning constraints. To wit: institutions ignore the {\em local} nature of Sat  appearing in practice: %(and logic with finitary signatures): 
to find if a model $m$ satisfies a constraint $c$, normally a small part of $m$ is to be examined and fixed if the constraint is violated. For industrial instances/models comprising thousands of elements over dozens of sorts, locality of constraints is their crucial feature (\eg, see \cite{me-ecmfa17} for how it can be used to make inter-model consistency checking more effective) and needs to be included into a principled \fwk.  It is here where the {\em generalized sketches} (further just {\em sketches}) come on the stage and place the constraints' locality at the very centre, but otherwise strive to keep the \fwk\ as abstract as possible. 

\begin{wrapfigure}{r}[5mm]{0.425\textwidth}
	\vspace{-4ex}
\includegraphics[width=0.42\textwidth]{pdfs/VehOntology-Small}
	\vspace{-2.5ex}
\end{wrapfigure}
The inset figure shows a small example of a data schema $S=(G_S, C_S)$ consisting of a graph $G_S$ (six nodes and six arrows, arrow \hasDr\ shows the set of {\em driving} wheels of a vehicle) and a set $C_S$ of four {\em constraint declarations} (or juts constraints) (dog-eared notes), each one having a scope shown with red dotted lines.%
\footnote{Actually each of the four other arrows has an attached default multiplicity constraint [1] (each vehicle has exactly one type, one load \etc). } 
% (except the two multiplicities, whose obvious scope is not shown but is stored in the tool used to build the schema). 
In detail, a constraint declaration is a pair $(c,\bmpa)$ of a constraint name/symbol $c$ (\eg, $\subseteq$) and a binding map \frar{\bmap}{G_c}{G_S}, where $G_c$ is the {\em arity} graph of the constraint (\eg, the arity graph of $\subseteq$ consists of two parallel arrows, and \bmap\ sends arrows $sub$ and $sup$ in $G_\subseteq$ to arrows \hasDr\ and \has\ in $G_S$ resp.). Each constraint name $c$ has its predefined semantics: a class \semm{c} of data instances over $G_c$ considered {\em valid}, \ie, \semm{c} is a class of graph \mor s into $G_c$. E.g., for constraint $\subseteq$, data instance \frar{t_D}{G_D}{G_\subseteq} is {\em valid} if $\semmD{sub}\subseteq\semmD{sup}$, where \frar{\semmD{\cdot}}{G_c}{\carr{\spancat}} is the copresheaf-like graph \mor\ into the big graph underlying the \caty\ $\spancat=\spanfunX{(\setcat)}$ equivalent to map $t_D$. Now we say that a data instance \frar{t_D}{G_D}{G_S} over $S$ {\em satisfies} a constraint declaration  $(c,\bmap)$ (and we  write $D\modelsd (c,\bmap)$  iff pulling $t_D$ \ back along \bmap\ results in ${\tmap_\bmap}\in \Ob\semm{c}$. %; then we say that instance \tmap\ (a logician's  {\em model}) satisfies a constraint declaration ({\em sentence}) $(c,\bmap)$ if  is considered valid, if it satisfies all constraint declarations in $C_S$ such that all constraints in $C_S$ are satisfied. Semantics of the three upper constraints is clear, \eg, 
Semantics of the two multiplicity constraints can be specified in a similar way by logical means, but constraint $c!$ is essentially different. It is a very special customized constraint with a complex arity graph \Gcbang\ actually iso\moric\ to graph $G_S$, and the following semantics. An instance \frar{\semmD{\cdot}}{\Gcbang}{\carr{\spancat}} is considered {\em valid}, if for each vehicle $v\in\semmD{\Vehicle}$, the collection of its parameters,  $\left( v.\semmD{type},...., (w.\semmD{code})_{w\in v.\semmD{\has}},...\right)$ satisfies some predefined conditions specified in a corresponding normative document. Moreover, it is not excluded that the final decision whether a vehicle $v$ satisfies the condition is delegated to an expert, say $e$, so that we should write $D\modelsd^e \cbang$ to assert the validity of an instance $D$. 

%The second goal is to present several simple but interesting mathematical results about what we will call Cartesian \sation\ relation. 
Let \GG\ be a finitely complete \caty\ (FCC) (of  {\em graphs}). A {\em constraint} over \GG\ is a triple $(c, G_c, \semm{c})$ of a {\em constraint name} $c$, its {\em arity} graph $G_c\in \Ob\GG$, and a \caty\ $\semm{c} \hookrightarrow\GG/G_c$ of {\em valid} instances and their \mor s (typically, a full sub\caty\ but it's not a must); we require \semm{c} to be closed under iso\mor s. Then any graph  $G$ determines a {\em Cartesian Sat} $\models_G \subset \GG/G\times\GG(G_c,G)$ by setting $\tmap\models_G (c,\bmap)$ iff pulling \tmap\ back along \bmap\ results in ${\tmap_\bmap}\in \Ob\semm{c}$. %




; then we say that instance \tmap\ (a logician's  {\em model}) satisfies a constraint declaration ({\em sentence}) $(c,\bmap)$.\footnote{Although this definition and much of further work only need pullbacks, having \tcat\ and  elements will  also be useful.} % hence, the FCC requirement for the base \caty\ \GG.} 
%
(Below term `constraint' will refer to both constraints $c$ and constraint declarations $(c,\bmap)$ but the context will resolve the ambiguity.)  
%
If $G$ changes by a \GG-\mor\ \frar{f}{G}{G'}, then instances/models change contravariantly via the pullback functor \frar{f^*}{\GG/G'}{\GG/G}, while  constraints change covariantly via post-composition \frar{f_*}{\GG(G_c,G)}{\GG(G_c, G')}. Now the \pblemma\ allows us to prove that the Sat-axiom holds for Cartesian $\vDash_G$ with  $G$ ranging over $\Ob\GG$.  
%for any $\tmap'\in\GG/G'$ and $\bmap\in\GG(G_c,G)$, the following {\em (twisted) satisfaction axiom} of the abstract model theory \cite{barwise-axioms4amt-AML74} %(in which constraints and instances are sentences and models )
%\fbox{$f^*(\tmap')\models_G (c,\bmap)$ iff $\tmap'\models_{G'} f_*(c, \bmap))$} (where $f_*(c,\bmap):=(c,f_*(\bmap))$holds  due to the \pblemma. 
% ---- Older version in the indexed setting \models_G
%A major result \cite[Th.1]{myTR-sketchesNew-arxiv23} states that a collection \predsig\ of constraints with their arities and valid instances as described above gives rise to an institution
%$\vDash_G^\predsig \subset \GG/G \times\LDiagcat_G^\predsig$ where $\LDiagcat_G^\predsig$ is the collection of \predsig-labelled diagrams into $G$, \ie, $\LDiagcat_G^\predsig=\predsig\timm_{(\arfun,\dom_G)}\GG/G$ where \frar{\arfun}{\predsig}{\GG} is the arity mapping and \frar{\dom_G}{\GG/G}{\GG}. Now the main theorem \cite[Th.4.19]{me-entcs08} is an easy corollary of the above.%
%\footnote{Note that including constraints' semantics into the signature means an essential departure from Makkai's generalized sketches \cite{makkai-ske}, whose semantics is defined via injectivity. In a sense, it is a return to classical Ehresmann's sketches, whose signatures consist of universal properties which do have a predefined semantics in \setcat.}
%%, and it makes sense to call them somehow differently from Makkai's sketches, \eg {\em Ehresmann's generalized sketches}}
%%
%
A major result \cite[Th.1]{myTR-sketchesNew-arxiv23} states that a collection \predsig\ of constraints with their arities and valid instances as described above gives rise to an institution (and the main theorem \cite[Th.4.19]{me-entcs08} becomes an easy corollary). 
%
In a bit more detail, the inset figure shows a commutative digram of \caties\ and functors specifying the main constructs (where \twocat\ is the interval \caty, and \arrowcatGG\ is the arrow category over \GG).

\begin{wrapfigure}{r}[5mm]{0.45\textwidth}
	\vspace{-2ex}
	\input{diagrams/mainTh-brief}
\end{wrapfigure}
%(where \arrowcatGG\ is the arrows category over \GG). 
The leftmost square defines the notion of a constraint signature: objects of the carrier \caty\ are constraint names, arrows are dependencies between them, and functor \arfun\ provides arities. \InstcatSig\ is the global \caty\ of all (indexes of) valid instances: for any $i\in\Ob\InstcatSig$, arrow $\tmap_i\in\GG/G_{\labfun(i)}$ is a valid instance of constraint $\labfun(i)$. The middle PB-square defines the \caty\ of all labelled diagrams that can be built with \predsig-constraints. Finally, a non-trivial diagram chasing involving comma-categories allows inferring a ternary span \modelsReverseSig, whose subspan $(\constrleg, \instleg)$ specifies the global Sat; fibres over $G$ ranging over $\GG$ give us the institutions' setting, and the Sat axiom can be proved (see \cite{myTR-sketchesNew-arxiv23} for details). 

Thus, Cartesian Sat is a well-defined logical \fwk, which is much more concrete than institutions but much more abstract than constraint specification languages mentioned above. % used in practice as illustrated by the figure below. 
%%The place of sketches in a general landscape of constraint \specifin\ formalisms is illustrated by diagram in \cref{fig:bigPicture}. 
%%%Diagram in \cref{fig:bigPicture} presents a methodological view of the story described in the paper. 
%%The sketch \fwk\ in the upper row takes its place between extremely abstract \instin s and concrete logical formalisms including string-based logics (such as FOL and its fragments) and diagrammatic logics (injectivity, lifting constraints).
%\begin{figure}[ht]\label{fig:bigPicture}
%	\centering
%	\includegraphics[width=0.95\linewidth]{pdfs/bigPicture}
%%	\caption{A big picture of constraint specification \fwk s
%%			\zd{the right [PBC] is nonsense!!}
%%		}
%%	\label{fig:bigPicture}
%	\vspace{-2ex}
%\end{figure}
This fine tuning allowed for several successful applications of sketches in diagrammatic domain and data modelling   \cite{%Diskin-kluwer99,
	Diskin-diagrams00, me-dke03}  and software engineering  \cite{me-clafer16,rutleRLW-jlamp12}; see also applications of sketches to an important Model-Driven Engineering (MDE) problem of model consistency \cite{me-ecmfa17,patrick-faoc21}

%Note that including constraints' semantics into the signature means an essential departure from Makkai's generalized sketches \cite{makkai-ske}, whose semantics is defined via injectivity. In a sense, it is a return to classical Ehresmann's sketches, whose signatures consist of universal properties which do have a predefined semantics in \setcat.
An important novel feature of sketches above %in \cite{myTR-sketchesNew-arxiv23} 
is that Sat spans are ternary rather than binary, which implies 
%the third leg are formed by arrows \frar{\verif_G}{\cdot}{\semm{c}} 
that  \sation\ $\tmap\modelsDsig{G} (c,\bmap)$ takes place only if it has a witnessing index  $w\in\InstcatSig$ such that $\tmap_\bmap = \tmap_w\in\semm{c}\subset \GG/G_c$. This component of \sation\ is crucial for applications in safety assurance, in which any fact of conformance of a product (instance) to a requirement (modelled by a constraint) is to be evidenced by an explicit reference to a verification procedure. 

%The place of sketches in a general landscape of constraint \specifin\ formalisms is illustrated by diagram in \cref{fig:bigPicture}. 
%%Diagram in \cref{fig:bigPicture} presents a methodological view of the story described in the paper. 
%The sketch \fwk\ in the upper row takes its place between extremely abstract \instin s and concrete logical formalisms including string-based logics (such as FOL and its fragments) and diagrammatic logics (injectivity, lifting constraints).
%\begin{figure}[ht]\label{fig:bigPicture}
%	\centering
%	\includegraphics[width=0.8\linewidth]{pdfs/bigPicture}
%	\caption{A big picture of constraint specification \fwk s
%		\zd{the right [PBC] is nonsense!!}
%	}
%	\label{fig:bigPicture}
%	\vspace{-2ex}
%\end{figure}
%These are ``classical'' generalized sketches of the 90s.
%{\em \Sketchesplus} in the lower row  refer to an enriched \fwk\ considered in this paper: it includes a) dependencies between constraints and models as typing mappings 
%introduced in \cite{me-entcs08}, and novel features:
%b) indexing, and c) verification (plus the fibred rather than (co)presheaveal form of main definitions used so far).%
%\footnote{Remarkably, constraint indexing was introduced into the (generalized) sketch \fwk\ by Makkai \cite{makkai-ske} by purely mathematical reasons: sketches with indexed constraints behave mathematically better. 
%	%(To wit: a remarkable fact discovered by Makkai is that if sketches are built over graphical objects specifiable as functors \frarxy{\II}{\setcat}, \ie, the \caty\ of graphs underlying sketches is a copresheaf topos, then the \caty\ of sketches with indexed constraints is a copresheaf topos as well. In other words, sketches, \ie, schemas with constraints are graphs!) 
%	Similarly, instance indexing added to the sketch \fwk\ in the paper  directly leads to the third verification leg for the \sation\ relation, and hence feature c).}
%%
%Ordinary sketches can be seen as \sketchesplus\ with trivial extra structure (discrete \caties, bijective indexing). We will also see that it is possible to suitably enrich \instin s to \instinsplus\ so that \sketchesplus\ specialize  \instinsplus\ as shown in the lower row. We can consider the left square as something like a pullback completion (PBC), and hopefully with a suitable categorical arrangement it can indeed be formalized as PBC. 
%
%The right upper cell of the figure shows multiple constraint \specifin\ languages, %: regular logic as a sublogic of FOL,  %Ehresmann's sketches, relational data dependencies, and 
%%Spivak's lifting constraints popular within the ACT community, injectivity, and industrially usable \OCLTM \cite{oclBook-99}, which supersets FOL. %B \cite{B-book}.
%which can be used for specifying semantics of constraints. 
%%seen as different implementations of non-plus sketches.%
%\footnote{Note the  iso\mor\ of the lifting constraint \fwk\ to the classical injectivity logic, which we will prove in the paper.}
%% Now PBC-like procedures can enrich these logics for being capable to  implement \sketchesplus. 
%We thus have a template for enriching existing logics with verification and indexing. (\OCLTMplus\ may especially be attractive for practitioners). 

The proposed talk aims at two goals. One is expository: discussions at the last NIST workshop\footnote{ https://www.nist.gov/news-events/events/2022/11/compositional-structures-systems-engineering-and-design-0}
showed an interest within the ACT community towards generalized sketches and their accurate presentation. % explaining Why, What and How with an emphasis on Why. 
Paper \cite{myTR-sketchesNew-arxiv23} and the talk presenting it take on this duty and go further by presenting sketches with several novel features, specifically, verification aspects just mentioned. %crucial for modelling safety assurance. Moreover, sketches of this paper essentially depart from Makkai's sketches and their version described in \cite{me-entcs08} in that semantics is built-in it into the very notion of a constraint signature. In this sense, it is a return to classical Ehresmann's sketches, whose signatures consist of universal properties which do have a predefined semantics in \setcat, and it makes sense to call them somehow differently from Makkai's sketches, \eg {\em Ehresmann's generalized sketches}. %The paper also shows that semantic universe better aligned with data modelling needs is \spancat\ rather than \setcat\ or even \relcat\ (it is discussed in detail in Sect. 2.1  ).  
%
The second goal is to show some interesting mathematics that unexpectedly appeared in a first seemingly routine diagram chasing heavily employing the \pblemma. Specifically, element-free formalization of the twisted Sat-axiom requires a comma \caty\ generated by a span of functors, one of which is a fibration an the other is an opfibration. Also, rewriting main constructs of the sketch \fwk\ from their usual representation as indexed-\caties\ into an equivalent fibrational form turned out to be, although generally clear, not entirely routine exercise.  


\endinput

\clearpage
\bibliographystyle{eptcs}\label{sect:bib}
\bibliography{../library,../refsGrand17-21}

%\endinput
\end{document}



% --- another shortcoming -- verification 
%Another institutions' shortcoming is that for safety-critical constraints, satisfaction instance $m\satrelsymbol c$ is to be verified by a suitably certified procedure (a model checking procedure, simulation, or an expert review), and safety assurance norms demand those procedures to be explicitly referenced. This makes \sation\ a ternary rather than binary relation (where the third leg can be refined into a separate structure if needed). 
%








\clearpage
\endinput
The sketch \fwk\ in the upper row takes its place between extremely abstract \instin s and concrete logical formalisms including string-based logics (such as FOL and its fragments) and diagrammatic logics (injectivity, lifting constraints).

\clearpage 
The sketch \fwk\ in the upper row takes its place between extremely abstract \instin s and concrete logical formalisms including string-based logics (such as FOL and its fragments) and diagrammatic logics (injectivity, lifting constraints).

==> diagrams/arrowDef4arrowCatDelta.tex <==
%\begin{wrapfigure}{r}{0.185\textwidth}
%	\vspace{-10mm}
\begin{equation}\label{eqdiag:deltaarrowcatMorphisms}
	% https://q.uiver.app/#q=WzAsNixbMCwwLCJcXGJ1bGxldCJdLFswLDEsIlxcYnVsbGV0Il0sWzIsMCwiXFxidWxsZXQiXSxbMiwxLCJcXGJ1bGxldCJdLFsxLDAsIlxcY2lyYyIsWzEyMCw2MCwzOSwxXV0sWzEsMSwiXFxidWxsZXQiXSxbMCwxLCJhIiwyXSxbMiwzLCJiIl0sWzQsMCwicF8wIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM5XX0sWzEyMCw2MCwzOSwxXV0sWzQsMiwicV8wIiwwLHsiY29sb3VyIjpbMTIwLDYwLDM5XX0sWzEyMCw2MCwzOSwxXV0sWzUsMywicV8xIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM5XX0sWzEyMCw2MCwzOSwxXV0sWzUsMSwiXFxtYXRoc2Z7aWR9IiwwLHsibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw1LCJyIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM5XX0sWzEyMCw2MCwzOSwxXV1d
	\begin{tikzcd}[ampersand replacement=\&,column sep=small]
		\bullet \& \textcolor{rgb,255:red,40;green,159;blue,40}{\circ} \& \bullet \\
		\bullet \& \bullet \& \bullet
		\arrow["a"', from=1-1, to=2-1]
		\arrow["b", from=1-3, to=2-3]
		\arrow["{p_0}"', color={rgb,255:red,40;green,159;blue,40}, from=1-2, to=1-1]
		\arrow["{q_0}", color={rgb,255:red,40;green,159;blue,40}, from=1-2, to=1-3]
		\arrow["{q_1}"', color={rgb,255:red,40;green,159;blue,40}, from=2-2, to=2-3]
		\arrow["{\mathsf{id}}", Rightarrow, no head, from=2-2, to=2-1]
		\arrow["r"', color={rgb,255:red,40;green,159;blue,40}, from=1-2, to=2-2]
	\end{tikzcd}
\end{equation}
%	\vspace{-5mm}≠
%\caption{Arrows in \deltaarrowcatGG \label{figdiag:arrows-in-deltaarrowCat}}
%\end{wrapfigure}

==> diagrams/backup4today.tex <==
\newcommand{\mainThProofChasingNew}{
	% https://q.uiver.app/#q=WzAsMjMsWzAsMCwiXFxhcnJvd2NhdGRlbHRhR0ciXSxbMiwwLCJcXEdHIl0sWzQsMCwiXFxHRy9HIixbMTEsNTYsNTUsMV1dLFs1LDAsIlxcX3tcXHRpbWVzfVxcXyIsWzExLDU2LDU1LDFdXSxbNiwwLCJcXHZlcnRYe0d9IixbMTEsNTYsNTUsMV1dLFswLDIsIlxcT0tvYmoiXSxbMiwyLCJcXGNhcnJvcHtcXHByZWRzaWd9Il0sWzMsMSwiXFxMRHh7R30iLFsxMSw1Niw1NSwxXV0sWzUsMiwiXFxRb2JqRExSe0d9e0d9e0d9IixbMTEsNTYsNTUsMV1dLFsxLDEsIlxcb2tUYXJnZXRYe1xcY3NpZ30iLFsyMjIsNzMsNDgsMV1dLFs0LDMsIlxcdkRhc2hfe0cnfSIsWzExLDU2LDU1LDFdXSxbNywxXSxbNSw0LCJcXFFvYmpETFJ7Zn17R317Ryd9Il0sWzYsOCwiXFx2ZXJ0WHtHJ30iLFsxMjAsNjAsMzUsMV1dLFs1LDYsIlxcUW9iakRMUntHJ317Ryd9e0cnfSIsWzEyMCw2MCwzNSwxXV0sWzMsNywiXFxMRHh7Ryd9IixbMTIwLDYwLDM1LDFdXSxbMSw3LCJcXG9rVGFyZ2V0WHtcXGNzaWd9Il0sWzUsOCwiXFxfe1xcdGltZXN9XFxfIixbMTIwLDYwLDM1LDFdXSxbNCw4LCJcXEdHL0cnIl0sWzAsNiwiXFxPS29iaiJdLFs0LDUsIlxcdkRhc2hfe0cnfSIsWzEyMCw2MCwzNSwxXV0sWzAsOCwiXFxhcnJvd2NhdGRlbHRhR0ciXSxbNiw0LCJcXF97XFx0aW1lc31cXF8iXSxbNSwwLCJcXHRtYXBmdW5zaWciXSxbMCwxLCJcXGNvZCJdLFs2LDEsIlxcYXJmdW4iLDEseyJsYWJlbF9wb3NpdGlvbiI6NjB9XSxbNSw2LCJcXGxhYmZ1bnNpZyJdLFs1LDksIlxcb2tfXFxjc2lnIl0sWzksMCwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzksNiwiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzksMSwiXFx0ZXh0e1twYl19X1xcY3NpZyIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsMSwiXFxkb21fe0d9IiwyLHsiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs3LDYsIlxcZWxsWHtHfSIsMCx7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTEsNTYsNTUsMV1dLFs3LDIsIlxcYm1hcGZ1blh7R30iLDAseyJsYWJlbF9wb3NpdGlvbiI6MCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzMsMiwiaF8wIiwyLHsiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzgsNCwidiIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs4LDMsIihcXGJtYXBmdW5eRyxcXCwgMSkiLDAseyJsYWJlbF9wb3NpdGlvbiI6NzAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFszLDAsIlxccGJmdW52WHtHfSIsMix7ImN1cnZlIjo0LCJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzgsOSwiXFwjX3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs3LDEsIlxcdGV4dHtbcGJdfV97R30iLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTEsNTYsNTUsMV1dLFsxMCw1LCJcXGxpZnRlZFh7XFwjX0d9IiwwLHsiY3VydmUiOi0xLCJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMyw0LCJ2XzAiLDAseyJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMTAsOSwiXFx0ZXh0e1twYl19J197R30iLDEseyJsYWJlbF9wb3NpdGlvbiI6MTAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTEsNTYsNTUsMV1dLFs4LDcsImgiLDEseyJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzEwLDgsIlxcbGlmdGVkWHtcXG9rX1xcY3NpZ30iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFsxMiwxMywiXFx0d2l4RHt2fSIsMCx7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxMyw0LCJmXipfXFxEZWx0YSIsMix7ImN1cnZlIjo1fV0sWzEyLDgsIigxLGZeKl9cXERlbHRhKSIsMl0sWzE0LDE1LCJoJyIsMSx7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxNCwxMywidiciLDEseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTIsMTQsIihmXypeXFxjc2lnLCAxKSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFs3LDE1LCJmXypeXFxjc2lnIiwyXSxbMTQsMTYsIlxcI197Ryd9IiwyLHsibGFiZWxfcG9zaXRpb24iOjMwLCJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTcsMTMsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxNCwxNywiKFxcYm1hcGZ1bl57Ryd9LCAxKSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxNywxOCwiIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzE1LDE4XSxbOSwxNiwiIiwyLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE5LDE2LCJcXG9rX1xcY3NpZyJdLFsyMCwxOSwiXFxsaWZ0ZWRYe1xcI197Ryd9fSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCwzNSwxXV0sWzIwLDE0LCIiLDIseyJjb2xvdXIiOlsxMjAsNjAsMzVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNSwxOSwiIiwyLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEyLDcsIiIsMCx7ImN1cnZlIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMTksMjEsIlxcdG1hcGZ1bnNpZyIsMl0sWzE4LDIxLCJcXHBiZnVudlh7Ryd9IiwwLHsiY3VydmUiOi0yLCJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMjIsMTNdLFsxMiwyMiwiKC4sMSkiLDJdLFsyMiwyLCIiLDIseyJjdXJ2ZSI6NSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzIyLDMsIigxLGZeKl9cXERlbHRhKSIsMSx7ImN1cnZlIjo1LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XV0=
	\begin{tikzcd}[ampersand replacement=\&,sep=small]
		\arrowcatdeltaGG \&\& \GG \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\GG/G} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\_{\times}\_} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\vertX{G}} \\
		\& \textcolor{rgb,255:red,33;green,87;blue,212}{\okTargetX{\csig}} \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\LDx{G}} \&\&\&\& {} \\
		\OKobj \&\& {\carrop{\predsig}} \&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\QobjDLR{G}{G}{G}} \\
		\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\vDash_{G'}} \\
		\&\&\&\&\& {\QobjDLR{f}{G}{G'}} \& {\_{\times}\_} \\
		\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\vDash_{G'}} \\
		\OKobj \&\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\QobjDLR{G'}{G'}{G'}} \\
		\& {\okTargetX{\csig}} \&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\LDx{G'}} \\
		\arrowcatdeltaGG \&\&\&\& {\GG/G'} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\_{\times}\_} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\vertX{G'}}
		\arrow["\tmapfunsig", from=3-1, to=1-1]
		\arrow["\cod", from=1-1, to=1-3]
		\arrow["\arfun"{description, pos=0.6}, from=3-3, to=1-3]
		\arrow["\labfunsig", from=3-1, to=3-3]
		\arrow["{\ok_\csig}", from=3-1, to=2-2]
		\arrow[dotted, from=2-2, to=1-1]
		\arrow[dotted, from=2-2, to=3-3]
		\arrow["{\text{[pb]}_\csig}"{description, pos=0.4}, draw=none, from=2-2, to=1-3]
		\arrow["{\dom_{G}}"', color={rgb,255:red,205;green,100;blue,76}, from=1-5, to=1-3]
		\arrow["{\ellX{G}}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=2-4, to=3-3]
		\arrow["{\bmapfunX{G}}"{pos=0}, color={rgb,255:red,205;green,100;blue,76}, dotted, from=2-4, to=1-5]
		\arrow["{h_0}"', color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-5]
		\arrow["v"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=1-7]
		\arrow["{(\bmapfun^G,\, 1)}"{pos=0.7}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=3-6, to=1-6]
		\arrow["{\pbfunvX{G}}"', color={rgb,255:red,205;green,100;blue,76}, curve={height=24pt}, from=1-6, to=1-1]
		\arrow["{\#_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-2]
		\arrow["{\text{[pb]}_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=2-4, to=1-3]
		\arrow["{\liftedX{\#_G}}", color={rgb,255:red,205;green,100;blue,76}, curve={height=-6pt}, dashed, from=4-5, to=3-1]
		\arrow["{v_0}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-7]
		\arrow["{\text{[pb]}'_{G}}"{description, pos=0.1}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=4-5, to=2-2]
		\arrow["h"{description}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-4]
		\arrow["{\liftedX{\ok_\csig}}"{pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=4-5, to=3-6]
		\arrow["{\twixD{v}}", color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=9-7]
		\arrow["{f^*_\Delta}"', curve={height=30pt}, from=9-7, to=1-7]
		\arrow["{(1,f^*_\Delta)}"', from=5-6, to=3-6]
		\arrow["{h'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-4]
		\arrow["{v'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-7]
		\arrow["{(f_*^\csig, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=7-6]
		\arrow["{f_*^\csig}"', from=2-4, to=8-4]
		\arrow["{\#_{G'}}"'{pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-2]
		\arrow[dotted, from=9-6, to=9-7]
		\arrow["{(\bmapfun^{G'}, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-6]
		\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=9-6, to=9-5]
		\arrow[from=8-4, to=9-5]
		\arrow[Rightarrow, dotted, no head, from=2-2, to=8-2]
		\arrow["{\ok_\csig}", from=7-1, to=8-2]
		\arrow["{\liftedX{\#_{G'}}}"', color={rgb,255:red,36;green,143;blue,36}, dotted, from=6-5, to=7-1]
		\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=6-5, to=7-6]
		\arrow[Rightarrow, dotted, no head, from=3-1, to=7-1]
		\arrow[curve={height=12pt}, dotted, from=5-6, to=2-4]
		\arrow["\tmapfunsig"', from=7-1, to=9-1]
		\arrow["{\pbfunvX{G'}}", color={rgb,255:red,36;green,143;blue,36}, curve={height=-12pt}, from=9-5, to=9-1]
		\arrow[from=5-7, to=9-7]
		\arrow["{(.,1)}"', from=5-6, to=5-7]
		\arrow[curve={height=30pt}, dotted, from=5-7, to=1-5]
		\arrow["{(1,f^*_\Delta)}"{description}, curve={height=30pt}, dotted, from=5-7, to=1-6]
	\end{tikzcd}
}


\newcommand{\mainThProofChasingNewest}{
	% https://q.uiver.app/#q=WzAsMjAsWzAsMCwiXFxhcnJvd2NhdGRlbHRhR0ciXSxbMiwwLCJcXEdHIl0sWzQsMCwiXFxHRy9HIixbMTEsNTYsNTUsMV1dLFs1LDAsIlxcX3tcXHRpbWVzfVxcXyIsWzExLDU2LDU1LDFdXSxbNiwwLCJcXHZlcnRYe0d9IixbMTEsNTYsNTUsMV1dLFswLDQsIlxcT0tvYmoiXSxbMyw0LCJcXGNhcnJvcHtcXGNzaWd9Il0sWzQsMSwiXFxMRHh7R30iLFsxMSw1Niw1NSwxXV0sWzUsMiwiXFxRb2JqRExSe0d9e0d9e0d9IixbMTEsNTYsNTUsMV1dLFsxLDQsIlxcb2tUYXJnZXRYe1xcY3NpZ30iLFsyMjIsNzMsNDgsMV1dLFs3LDFdLFs1LDQsIlxcUW9iakRMUntmfXtHfXtHJ30iXSxbNiw4LCJcXHZlcnRYe0cnfSIsWzEyMCw2MCwzNSwxXV0sWzUsNiwiXFxRb2JqRExSe0cnfXtHJ317Ryd9IixbMTIwLDYwLDM1LDFdXSxbNCw3LCJcXExEeHtHJ30iLFsxMjAsNjAsMzUsMV1dLFs1LDgsIlxcX3tcXHRpbWVzfVxcXyIsWzEyMCw2MCwzNSwxXV0sWzQsOCwiXFxHRy9HJyJdLFswLDgsIlxcYXJyb3djYXRkZWx0YUdHIl0sWzYsNCwiXFxfe1xcdGltZXN9XFxfIl0sWzIsOCwiXFxHRyJdLFs1LDAsIlxcdG1hcGZ1bnNpZyIsMV0sWzAsMSwiXFxjb2QiXSxbNSw2LCJcXGxhYmZ1bnNpZyIsMCx7ImN1cnZlIjo1fV0sWzUsOSwiXFxva19cXGNzaWciXSxbOSwwLCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSw2LCIiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSwxLCJcXHRleHR7W3BiXX1fXFxjc2lnIiwxLHsibGFiZWxfcG9zaXRpb24iOjMwLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxLCJcXGRvbV97R30iLDIseyJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzcsMiwiXFxibWFwZnVuWHtHfSIsMCx7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFszLDIsImhfMCIsMix7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTEsNTYsNTUsMV1dLFs4LDQsInYiLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsImNvbG91ciI6WzExLDU2LDU1XX0sWzExLDU2LDU1LDFdXSxbOCwzLCIoXFxibWFwZnVuXkcsXFwsIDEpIiwwLHsibGFiZWxfcG9zaXRpb24iOjcwLCJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMywwLCJcXHBiZnVudlh7R30iLDIseyJjdXJ2ZSI6NCwiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs4LDksIlxcI197R30iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsImxldmVsIjoyLCJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzcsMSwiXFx0ZXh0e1twYl19X3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMSw1Niw1NSwxXV0sWzMsNCwidl8wIiwwLHsiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzgsNywiaCIsMSx7ImNvbG91ciI6WzExLDU2LDU1XX0sWzExLDU2LDU1LDFdXSxbMTEsMTIsIlxcdHdpeER7dn0iLDAseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTIsNCwiZl4qX1xcRGVsdGEiLDIseyJjdXJ2ZSI6NX1dLFsxMSw4LCIoMSxmXipfXFxEZWx0YSkiLDIseyJsZXZlbCI6Mn1dLFsxMywxNCwiaCciLDEseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTMsMTIsInYnIiwxLHsiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzExLDEzLCIoZl8qXlxcY3NpZywgMSkiLDIseyJsZXZlbCI6MiwiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzcsMTQsImZfKl5cXGNzaWciLDIseyJjdXJ2ZSI6LTN9XSxbMTUsMTIsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxMywxNSwiKFxcYm1hcGZ1bl57Ryd9LCAxKSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxNSwxNiwiIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzE0LDE2LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTEsNywiIiwwLHsiY3VydmUiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxOCwxMl0sWzExLDE4LCIoLiwxKSIsMl0sWzE4LDIsIiIsMix7ImN1cnZlIjo1LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMTgsMywiKDEsZl4qX1xcRGVsdGEpIiwxLHsiY3VydmUiOjUsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs1LDE3LCJcXHRtYXBmdW5zaWciLDFdLFsxMyw5LCJcXCNfe0cnfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMCwibGV2ZWwiOjIsImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFs3LDYsIlxcZWxsWHtHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMSw1Niw1NSwxXV0sWzE0LDYsIlxcZWxsWHtHJ30iLDEseyJsYWJlbF9wb3NpdGlvbiI6MzAsImNvbG91ciI6WzEyMCw2MCwzNV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCwzNSwxXV0sWzYsMSwiXFxhcmZ1biIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo2MH1dLFsxNSwxNywiXFxwYmZ1bnZYe0cnfSIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzAsMTcsIlxcbWF0aHNme0lEfSIsMSx7ImN1cnZlIjo1LCJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTcsMTksIlxcY29kIiwxXSxbNiwxOSwiXFxhcmZ1biIsMV0sWzksMTksIlxcdGV4dHtbcGJdfV9cXGNzaWciLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDE3LCIiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XV0=
	\begin{tikzcd}[ampersand replacement=\&,sep=small]
		\arrowcatdeltaGG \&\& \GG \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\GG/G} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\_{\times}\_} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\vertX{G}} \\
		\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\LDx{G}} \&\&\& {} \\
		\&\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\QobjDLR{G}{G}{G}} \\
		\\
		\OKobj \& \textcolor{rgb,255:red,33;green,87;blue,212}{\okTargetX{\csig}} \&\& {\carrop{\csig}} \&\& {\QobjDLR{f}{G}{G'}} \& {\_{\times}\_} \\
		\\
		\&\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\QobjDLR{G'}{G'}{G'}} \\
		\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\LDx{G'}} \\
		\arrowcatdeltaGG \&\& \GG \&\& {\GG/G'} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\_{\times}\_} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\vertX{G'}}
		\arrow["\tmapfunsig"{description}, from=5-1, to=1-1]
		\arrow["\cod", from=1-1, to=1-3]
		\arrow["\labfunsig", curve={height=30pt}, from=5-1, to=5-4]
		\arrow["{\ok_\csig}", from=5-1, to=5-2]
		\arrow[dashed, from=5-2, to=1-1]
		\arrow[dashed, from=5-2, to=5-4]
		\arrow["{\text{[pb]}_\csig}"{description, pos=0.3}, draw=none, from=5-2, to=1-3]
		\arrow["{\dom_{G}}"', color={rgb,255:red,205;green,100;blue,76}, from=1-5, to=1-3]
		\arrow["{\bmapfunX{G}}", color={rgb,255:red,205;green,100;blue,76}, dashed, from=2-5, to=1-5]
		\arrow["{h_0}"', color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-5]
		\arrow["v"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=1-7]
		\arrow["{(\bmapfun^G,\, 1)}"{pos=0.7}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=3-6, to=1-6]
		\arrow["{\pbfunvX{G}}"', color={rgb,255:red,205;green,100;blue,76}, curve={height=24pt}, from=1-6, to=1-1]
		\arrow["{\#_{G}}"{pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, Rightarrow, from=3-6, to=5-2]
		\arrow["{\text{[pb]}_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=2-5, to=1-3]
		\arrow["{v_0}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-7]
		\arrow["h"{description}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-5]
		\arrow["{\twixD{v}}", color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=9-7]
		\arrow["{f^*_\Delta}"', curve={height=30pt}, from=9-7, to=1-7]
		\arrow["{(1,f^*_\Delta)}"', Rightarrow, from=5-6, to=3-6]
		\arrow["{h'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-5]
		\arrow["{v'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-7]
		\arrow["{(f_*^\csig, 1)}"', color={rgb,255:red,36;green,143;blue,36}, Rightarrow, from=5-6, to=7-6]
		\arrow["{f_*^\csig}"', curve={height=-18pt}, from=2-5, to=8-5]
		\arrow[dotted, from=9-6, to=9-7]
		\arrow["{(\bmapfun^{G'}, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-6]
		\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=9-6, to=9-5]
		\arrow[dashed, from=8-5, to=9-5]
		\arrow[curve={height=12pt}, dotted, from=5-6, to=2-5]
		\arrow[from=5-7, to=9-7]
		\arrow["{(.,1)}"', from=5-6, to=5-7]
		\arrow[curve={height=30pt}, dotted, from=5-7, to=1-5]
		\arrow["{(1,f^*_\Delta)}"{description}, curve={height=30pt}, dotted, from=5-7, to=1-6]
		\arrow["\tmapfunsig"{description}, from=5-1, to=9-1]
		\arrow["{\#_{G'}}"'{pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, Rightarrow, from=7-6, to=5-2]
		\arrow["{\ellX{G}}"{description, pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=2-5, to=5-4]
		\arrow["{\ellX{G'}}"{description, pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, dashed, from=8-5, to=5-4]
		\arrow["\arfun"{description, pos=0.6}, from=5-4, to=1-3]
		\arrow["{\pbfunvX{G'}}", color={rgb,255:red,36;green,143;blue,36}, curve={height=-18pt}, from=9-6, to=9-1]
		\arrow["{\mathsf{ID}}"{description}, curve={height=30pt}, Rightarrow, dotted, no head, from=1-1, to=9-1]
		\arrow["\cod"{description}, from=9-1, to=9-3]
		\arrow["\arfun"{description}, from=5-4, to=9-3]
		\arrow["{\text{[pb]}_\csig}"{description, pos=0.4}, draw=none, from=5-2, to=9-3]
		\arrow[dashed, from=5-2, to=9-1]
	\end{tikzcd}
}


==> diagrams/cattyOkayed--full.tex <==
\newcommand{\horzX}[1]{\slicecatcsigXY{\GG}{#1}}
\newcommand{\vertX}[1]{\slicecatdeltaXY{\GG}{#1}}

\renewcommand{\LDx}[1]{\horzX{#1}}
\newcommand{\PsubobjX}[1]{\enma{\vDash_{#1}^{}}}
\newcommand{\PsubobjtwiX}[1]{\enma{\vDash_{\twixSymbol#1}}}

\renewcommand{\PobjX}[1]{\PreinstcatX{#1}}
\renewcommand{\PobjtwiX}[1]{\PreinstcatX{\twixSymbol#1}}

\newcommand{\QobjDLR}[3]{\enma{  % 3 arguments : Down index, Left slice and Right slice
		\begin{array}{c}
			\PobjX{#1}=
			\\
			\horzX{#2}\timm\vertX{#3}.
		\end{array}
}}

\newcommand{\okTargetX}[1]{\PreinstcatX{#1}}

\newcommand{\OKobj}{\InstcatXdn{\csig}}
\newcommand{\okArrow}{\ok}

\newcommand{\mainThProofChasingNew}{
% https://q.uiver.app/#q=WzAsMjMsWzAsMCwiXFxhcnJvd2NhdGRlbHRhR0ciXSxbMiwwLCJcXEdHIl0sWzQsMCwiXFxHRy9HIixbMTEsNTYsNTUsMV1dLFs1LDAsIlxcX3tcXHRpbWVzfVxcXyIsWzExLDU2LDU1LDFdXSxbNiwwLCJcXHZlcnRYe0d9IixbMTEsNTYsNTUsMV1dLFswLDIsIlxcT0tvYmoiXSxbMiwyLCJcXGNhcnJvcHtcXHByZWRzaWd9Il0sWzMsMSwiXFxMRHh7R30iLFsxMSw1Niw1NSwxXV0sWzUsMiwiXFxRb2JqRExSe0d9e0d9e0d9IixbMTEsNTYsNTUsMV1dLFsxLDEsIlxcb2tUYXJnZXRYe1xcY3NpZ30iLFsyMjIsNzMsNDgsMV1dLFs0LDMsIlxcdkRhc2hfe0cnfSIsWzExLDU2LDU1LDFdXSxbNywxXSxbNSw0LCJcXFFvYmpETFJ7Zn17R317Ryd9Il0sWzYsOCwiXFx2ZXJ0WHtHJ30iLFsxMjAsNjAsMzUsMV1dLFs1LDYsIlxcUW9iakRMUntHJ317Ryd9e0cnfSIsWzEyMCw2MCwzNSwxXV0sWzMsNywiXFxMRHh7Ryd9IixbMTIwLDYwLDM1LDFdXSxbMSw3LCJcXG9rVGFyZ2V0WHtcXGNzaWd9Il0sWzUsOCwiXFxfe1xcdGltZXN9XFxfIixbMTIwLDYwLDM1LDFdXSxbNCw4LCJcXEdHL0cnIl0sWzAsNiwiXFxPS29iaiJdLFs0LDUsIlxcdkRhc2hfe0cnfSIsWzEyMCw2MCwzNSwxXV0sWzAsOCwiXFxhcnJvd2NhdGRlbHRhR0ciXSxbNiw0LCJcXF97XFx0aW1lc31cXF8iXSxbNSwwLCJcXHRtYXBmdW5zaWciXSxbMCwxLCJcXGNvZCJdLFs2LDEsIlxcYXJmdW4iLDEseyJsYWJlbF9wb3NpdGlvbiI6NjB9XSxbNSw2LCJcXGxhYmZ1bnNpZyJdLFs1LDksIlxcb2tfXFxjc2lnIl0sWzksMCwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzksNiwiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzksMSwiXFx0ZXh0e1twYl19X1xcY3NpZyIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsMSwiXFxkb21fe0d9IiwyLHsiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs3LDYsIlxcZWxsWHtHfSIsMCx7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTEsNTYsNTUsMV1dLFs3LDIsIlxcYm1hcGZ1blh7R30iLDAseyJsYWJlbF9wb3NpdGlvbiI6MCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzMsMiwiaF8wIiwyLHsiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzgsNCwidiIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs4LDMsIihcXGJtYXBmdW5eRyxcXCwgMSkiLDAseyJsYWJlbF9wb3NpdGlvbiI6NzAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFszLDAsIlxccGJmdW52WHtHfSIsMix7ImN1cnZlIjo0LCJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzgsOSwiXFwjX3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs3LDEsIlxcdGV4dHtbcGJdfV97R30iLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTEsNTYsNTUsMV1dLFsxMCw1LCJcXGxpZnRlZFh7XFwjX0d9IiwwLHsiY3VydmUiOi0xLCJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMyw0LCJ2XzAiLDAseyJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMTAsOSwiXFx0ZXh0e1twYl19J197R30iLDEseyJsYWJlbF9wb3NpdGlvbiI6MTAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTEsNTYsNTUsMV1dLFs4LDcsImgiLDEseyJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzEwLDgsIlxcbGlmdGVkWHtcXG9rX1xcY3NpZ30iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFsxMiwxMywiXFx0d2l4RHt2fSIsMCx7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxMyw0LCJmXipfXFxEZWx0YSIsMix7ImN1cnZlIjo1fV0sWzEyLDgsIigxLGZeKl9cXERlbHRhKSIsMl0sWzE0LDE1LCJoJyIsMSx7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxNCwxMywidiciLDEseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTIsMTQsIihmXypeXFxjc2lnLCAxKSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFs3LDE1LCJmXypeXFxjc2lnIiwyXSxbMTQsMTYsIlxcI197Ryd9IiwyLHsibGFiZWxfcG9zaXRpb24iOjMwLCJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTcsMTMsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxNCwxNywiKFxcYm1hcGZ1bl57Ryd9LCAxKSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxNywxOCwiIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzE1LDE4XSxbOSwxNiwiIiwyLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE5LDE2LCJcXG9rX1xcY3NpZyJdLFsyMCwxOSwiXFxsaWZ0ZWRYe1xcI197Ryd9fSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCwzNSwxXV0sWzIwLDE0LCIiLDIseyJjb2xvdXIiOlsxMjAsNjAsMzVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNSwxOSwiIiwyLHsibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEyLDcsIiIsMCx7ImN1cnZlIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMTksMjEsIlxcdG1hcGZ1bnNpZyIsMl0sWzE4LDIxLCJcXHBiZnVudlh7Ryd9IiwwLHsiY3VydmUiOi0yLCJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMjIsMTNdLFsxMiwyMiwiKC4sMSkiLDJdLFsyMiwyLCIiLDIseyJjdXJ2ZSI6NSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzIyLDMsIigxLGZeKl9cXERlbHRhKSIsMSx7ImN1cnZlIjo1LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\arrowcatdeltaGG \&\& \GG \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\GG/G} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\_{\times}\_} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\vertX{G}} \\
	\& \textcolor{rgb,255:red,33;green,87;blue,212}{\okTargetX{\csig}} \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\LDx{G}} \&\&\&\& {} \\
	\OKobj \&\& {\carrop{\predsig}} \&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\QobjDLR{G}{G}{G}} \\
	\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\vDash_{G'}} \\
	\&\&\&\&\& {\QobjDLR{f}{G}{G'}} \& {\_{\times}\_} \\
	\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\vDash_{G'}} \\
	\OKobj \&\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\QobjDLR{G'}{G'}{G'}} \\
	\& {\okTargetX{\csig}} \&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\LDx{G'}} \\
	\arrowcatdeltaGG \&\&\&\& {\GG/G'} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\_{\times}\_} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\vertX{G'}}
	\arrow["\tmapfunsig", from=3-1, to=1-1]
	\arrow["\cod", from=1-1, to=1-3]
	\arrow["\arfun"{description, pos=0.6}, from=3-3, to=1-3]
	\arrow["\labfunsig", from=3-1, to=3-3]
	\arrow["{\ok_\csig}", from=3-1, to=2-2]
	\arrow[dotted, from=2-2, to=1-1]
	\arrow[dotted, from=2-2, to=3-3]
	\arrow["{\text{[pb]}_\csig}"{description, pos=0.4}, draw=none, from=2-2, to=1-3]
	\arrow["{\dom_{G}}"', color={rgb,255:red,205;green,100;blue,76}, from=1-5, to=1-3]
	\arrow["{\ellX{G}}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=2-4, to=3-3]
	\arrow["{\bmapfunX{G}}"{pos=0}, color={rgb,255:red,205;green,100;blue,76}, dotted, from=2-4, to=1-5]
	\arrow["{h_0}"', color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-5]
	\arrow["v"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=1-7]
	\arrow["{(\bmapfun^G,\, 1)}"{pos=0.7}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=3-6, to=1-6]
	\arrow["{\pbfunvX{G}}"', color={rgb,255:red,205;green,100;blue,76}, curve={height=24pt}, from=1-6, to=1-1]
	\arrow["{\#_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-2]
	\arrow["{\text{[pb]}_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=2-4, to=1-3]
	\arrow["{\liftedX{\#_G}}", color={rgb,255:red,205;green,100;blue,76}, curve={height=-6pt}, dashed, from=4-5, to=3-1]
	\arrow["{v_0}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-7]
	\arrow["{\text{[pb]}'_{G}}"{description, pos=0.1}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=4-5, to=2-2]
	\arrow["h"{description}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-4]
	\arrow["{\liftedX{\ok_\csig}}"{pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=4-5, to=3-6]
	\arrow["{\twixD{v}}", color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=9-7]
	\arrow["{f^*_\Delta}"', curve={height=30pt}, from=9-7, to=1-7]
	\arrow["{(1,f^*_\Delta)}"', from=5-6, to=3-6]
	\arrow["{h'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-4]
	\arrow["{v'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-7]
	\arrow["{(f_*^\csig, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=7-6]
	\arrow["{f_*^\csig}"', from=2-4, to=8-4]
	\arrow["{\#_{G'}}"'{pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-2]
	\arrow[dotted, from=9-6, to=9-7]
	\arrow["{(\bmapfun^{G'}, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-6]
	\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=9-6, to=9-5]
	\arrow[from=8-4, to=9-5]
	\arrow[Rightarrow, dotted, no head, from=2-2, to=8-2]
	\arrow["{\ok_\csig}", from=7-1, to=8-2]
	\arrow["{\liftedX{\#_{G'}}}"', color={rgb,255:red,36;green,143;blue,36}, dotted, from=6-5, to=7-1]
	\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=6-5, to=7-6]
	\arrow[Rightarrow, dotted, no head, from=3-1, to=7-1]
	\arrow[curve={height=12pt}, dotted, from=5-6, to=2-4]
	\arrow["\tmapfunsig"', from=7-1, to=9-1]
	\arrow["{\pbfunvX{G'}}", color={rgb,255:red,36;green,143;blue,36}, curve={height=-12pt}, from=9-5, to=9-1]
	\arrow[from=5-7, to=9-7]
	\arrow["{(.,1)}"', from=5-6, to=5-7]
	\arrow[curve={height=30pt}, dotted, from=5-7, to=1-5]
	\arrow["{(1,f^*_\Delta)}"{description}, curve={height=30pt}, dotted, from=5-7, to=1-6]
\end{tikzcd}
}


\newcommand{\mainThProofChasingNewest}{
% https://q.uiver.app/#q=WzAsMjAsWzAsMCwiXFxhcnJvd2NhdGRlbHRhR0ciXSxbMiwwLCJcXEdHIl0sWzQsMCwiXFxHRy9HIixbMTEsNTYsNTUsMV1dLFs1LDAsIlxcX3tcXHRpbWVzfVxcXyIsWzExLDU2LDU1LDFdXSxbNiwwLCJcXHZlcnRYe0d9IixbMTEsNTYsNTUsMV1dLFswLDQsIlxcT0tvYmoiXSxbMyw0LCJcXGNhcnJvcHtcXGNzaWd9Il0sWzQsMSwiXFxMRHh7R30iLFsxMSw1Niw1NSwxXV0sWzUsMiwiXFxRb2JqRExSe0d9e0d9e0d9IixbMTEsNTYsNTUsMV1dLFsxLDQsIlxcb2tUYXJnZXRYe1xcY3NpZ30iLFsyMjIsNzMsNDgsMV1dLFs3LDFdLFs1LDQsIlxcUW9iakRMUntmfXtHfXtHJ30iXSxbNiw4LCJcXHZlcnRYe0cnfSIsWzEyMCw2MCwzNSwxXV0sWzUsNiwiXFxRb2JqRExSe0cnfXtHJ317Ryd9IixbMTIwLDYwLDM1LDFdXSxbNCw3LCJcXExEeHtHJ30iLFsxMjAsNjAsMzUsMV1dLFs1LDgsIlxcX3tcXHRpbWVzfVxcXyIsWzEyMCw2MCwzNSwxXV0sWzQsOCwiXFxHRy9HJyJdLFswLDgsIlxcYXJyb3djYXRkZWx0YUdHIl0sWzYsNCwiXFxfe1xcdGltZXN9XFxfIl0sWzIsOCwiXFxHRyJdLFs1LDAsIlxcdG1hcGZ1bnNpZyIsMV0sWzAsMSwiXFxjb2QiXSxbNSw2LCJcXGxhYmZ1bnNpZyIsMCx7ImN1cnZlIjo1fV0sWzUsOSwiXFxva19cXGNzaWciXSxbOSwwLCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSw2LCIiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSwxLCJcXHRleHR7W3BiXX1fXFxjc2lnIiwxLHsibGFiZWxfcG9zaXRpb24iOjMwLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxLCJcXGRvbV97R30iLDIseyJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzcsMiwiXFxibWFwZnVuWHtHfSIsMCx7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFszLDIsImhfMCIsMix7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTEsNTYsNTUsMV1dLFs4LDQsInYiLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsImNvbG91ciI6WzExLDU2LDU1XX0sWzExLDU2LDU1LDFdXSxbOCwzLCIoXFxibWFwZnVuXkcsXFwsIDEpIiwwLHsibGFiZWxfcG9zaXRpb24iOjcwLCJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMywwLCJcXHBiZnVudlh7R30iLDIseyJjdXJ2ZSI6NCwiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFs4LDksIlxcI197R30iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsImxldmVsIjoyLCJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzcsMSwiXFx0ZXh0e1twYl19X3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMSw1Niw1NSwxXV0sWzMsNCwidl8wIiwwLHsiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzgsNywiaCIsMSx7ImNvbG91ciI6WzExLDU2LDU1XX0sWzExLDU2LDU1LDFdXSxbMTEsMTIsIlxcdHdpeER7dn0iLDAseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTIsNCwiZl4qX1xcRGVsdGEiLDIseyJjdXJ2ZSI6NX1dLFsxMSw4LCIoMSxmXipfXFxEZWx0YSkiLDIseyJsZXZlbCI6Mn1dLFsxMywxNCwiaCciLDEseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTMsMTIsInYnIiwxLHsiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzExLDEzLCIoZl8qXlxcY3NpZywgMSkiLDIseyJsZXZlbCI6MiwiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzcsMTQsImZfKl5cXGNzaWciLDIseyJjdXJ2ZSI6LTN9XSxbMTUsMTIsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxMywxNSwiKFxcYm1hcGZ1bl57Ryd9LCAxKSIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFsxNSwxNiwiIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzE0LDE2LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTEsNywiIiwwLHsiY3VydmUiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxOCwxMl0sWzExLDE4LCIoLiwxKSIsMl0sWzE4LDIsIiIsMix7ImN1cnZlIjo1LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMTgsMywiKDEsZl4qX1xcRGVsdGEpIiwxLHsiY3VydmUiOjUsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs1LDE3LCJcXHRtYXBmdW5zaWciLDFdLFsxMyw5LCJcXCNfe0cnfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMCwibGV2ZWwiOjIsImNvbG91ciI6WzEyMCw2MCwzNV19LFsxMjAsNjAsMzUsMV1dLFs3LDYsIlxcZWxsWHtHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMSw1Niw1NSwxXV0sWzE0LDYsIlxcZWxsWHtHJ30iLDEseyJsYWJlbF9wb3NpdGlvbiI6MzAsImNvbG91ciI6WzEyMCw2MCwzNV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCwzNSwxXV0sWzYsMSwiXFxhcmZ1biIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo2MH1dLFsxNSwxNywiXFxwYmZ1bnZYe0cnfSIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzAsMTcsIlxcbWF0aHNme0lEfSIsMSx7ImN1cnZlIjo1LCJsZXZlbCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTcsMTksIlxcY29kIiwxXSxbNiwxOSwiXFxhcmZ1biIsMV0sWzksMTksIlxcdGV4dHtbcGJdfV9cXGNzaWciLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs5LDE3LCIiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\arrowcatdeltaGG \&\& \GG \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\GG/G} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\_{\times}\_} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\vertX{G}} \\
	\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\LDx{G}} \&\&\& {} \\
	\&\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\QobjDLR{G}{G}{G}} \\
	\\
	\OKobj \& \textcolor{rgb,255:red,33;green,87;blue,212}{\okTargetX{\csig}} \&\& {\carrop{\csig}} \&\& {\QobjDLR{f}{G}{G'}} \& {\_{\times}\_} \\
	\\
	\&\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\QobjDLR{G'}{G'}{G'}} \\
	\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\LDx{G'}} \\
	\arrowcatdeltaGG \&\& \GG \&\& {\GG/G'} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\_{\times}\_} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\vertX{G'}}
	\arrow["\tmapfunsig"{description}, from=5-1, to=1-1]
	\arrow["\cod", from=1-1, to=1-3]
	\arrow["\labfunsig", curve={height=30pt}, from=5-1, to=5-4]
	\arrow["{\ok_\csig}", from=5-1, to=5-2]
	\arrow[dashed, from=5-2, to=1-1]
	\arrow[dashed, from=5-2, to=5-4]
	\arrow["{\text{[pb]}_\csig}"{description, pos=0.3}, draw=none, from=5-2, to=1-3]
	\arrow["{\dom_{G}}"', color={rgb,255:red,205;green,100;blue,76}, from=1-5, to=1-3]
	\arrow["{\bmapfunX{G}}", color={rgb,255:red,205;green,100;blue,76}, dashed, from=2-5, to=1-5]
	\arrow["{h_0}"', color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-5]
	\arrow["v"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=1-7]
	\arrow["{(\bmapfun^G,\, 1)}"{pos=0.7}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=3-6, to=1-6]
	\arrow["{\pbfunvX{G}}"', color={rgb,255:red,205;green,100;blue,76}, curve={height=24pt}, from=1-6, to=1-1]
	\arrow["{\#_{G}}"{pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, Rightarrow, from=3-6, to=5-2]
	\arrow["{\text{[pb]}_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=2-5, to=1-3]
	\arrow["{v_0}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-7]
	\arrow["h"{description}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-5]
	\arrow["{\twixD{v}}", color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=9-7]
	\arrow["{f^*_\Delta}"', curve={height=30pt}, from=9-7, to=1-7]
	\arrow["{(1,f^*_\Delta)}"', Rightarrow, from=5-6, to=3-6]
	\arrow["{h'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-5]
	\arrow["{v'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-7]
	\arrow["{(f_*^\csig, 1)}"', color={rgb,255:red,36;green,143;blue,36}, Rightarrow, from=5-6, to=7-6]
	\arrow["{f_*^\csig}"', curve={height=-18pt}, from=2-5, to=8-5]
	\arrow[dotted, from=9-6, to=9-7]
	\arrow["{(\bmapfun^{G'}, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-6]
	\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=9-6, to=9-5]
	\arrow[dashed, from=8-5, to=9-5]
	\arrow[curve={height=12pt}, dotted, from=5-6, to=2-5]
	\arrow[from=5-7, to=9-7]
	\arrow["{(.,1)}"', from=5-6, to=5-7]
	\arrow[curve={height=30pt}, dotted, from=5-7, to=1-5]
	\arrow["{(1,f^*_\Delta)}"{description}, curve={height=30pt}, dotted, from=5-7, to=1-6]
	\arrow["\tmapfunsig"{description}, from=5-1, to=9-1]
	\arrow["{\#_{G'}}"'{pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, Rightarrow, from=7-6, to=5-2]
	\arrow["{\ellX{G}}"{description, pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=2-5, to=5-4]
	\arrow["{\ellX{G'}}"{description, pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, dashed, from=8-5, to=5-4]
	\arrow["\arfun"{description, pos=0.6}, from=5-4, to=1-3]
	\arrow["{\pbfunvX{G'}}", color={rgb,255:red,36;green,143;blue,36}, curve={height=-18pt}, from=9-6, to=9-1]
	\arrow["{\mathsf{ID}}"{description}, curve={height=30pt}, Rightarrow, dotted, no head, from=1-1, to=9-1]
	\arrow["\cod"{description}, from=9-1, to=9-3]
	\arrow["\arfun"{description}, from=5-4, to=9-3]
	\arrow["{\text{[pb]}_\csig}"{description, pos=0.4}, draw=none, from=5-2, to=9-3]
	\arrow[dashed, from=5-2, to=9-1]
\end{tikzcd}
}



%\newcommand{\horzX}[1]{\slicecatcsigXY{\GG}{#1}}
%\newcommand{\vertX}[1]{\slicecatdeltaXY{\GG}{#1}}
%
%\newcommand{\PsubobjX}[1]{\enma{\vDash_{#1}^{}}}
%\newcommand{\PsubobjtwiX}[1]{\enma{\vDash_{\twixSymbol#1}}}
%
%\renewcommand{\PobjX}[1]{\PreinstcatX{#1}}
%\renewcommand{\PobjtwiX}[1]{\PreinstcatX{\twixSymbol#1}}
%\newcommand{\focusObjX}[1]{\PreinstcatX{#1}}
%
%\newcommand{\OKobj}{\InstcatXdn{\csig}}
%\newcommand{\okArrow}{\ok}

\newcommand{\cattyOkayedFull}{
% https://q.uiver.app/#q=WzAsMTQsWzAsMCwiXFxob3J6WHtHfSIsWzAsNjAsNjAsMV1dLFsxLDAsIlxcdmVydFh7R30iLFswLDYwLDYwLDFdXSxbNCwwLCJcXHZlcnRYe0cnfSIsWzEyMCw2MCw0MCwxXV0sWzMsMCwiXFxob3J6WHtHJ30iLFsxMjAsNjAsNDAsMV1dLFswLDEsIlxcUG9ialh7R30iLFswLDYwLDYwLDFdXSxbMiwxLCJcXFBvYmpYe2Z9Il0sWzQsMSwiXFxQb2JqWHtHJ30iLFsxMjAsNjAsNDAsMV1dLFsyLDMsIlxcb2tUYXJnZXRYe1xcY3NpZ30iXSxbMyw0LCJcXGNhcnJvcHtcXGNzaWd9Il0sWzEsNCwiXFxHRyJdLFs3LDMsIlxcT0tvYmoiXSxbNiwxLCJcXFBzdWJvYmpYe0d9IixbMCw2MCw2MCwxXV0sWzgsMSwiXFxQc3Vib2JqWHtHJ30iLFsxMjAsNjAsNDAsMV1dLFs3LDEsIlxcUHN1Ym9ialh7Zn0iXSxbMiwxLCJmXipfXFxEZWx0YSIsMix7ImN1cnZlIjozfV0sWzAsMywiZl8qIiwwLHsiY3VydmUiOi0zfV0sWzQsMCwiaCIsMix7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzUsMiwiXFx0d2l4e3Z9IiwwLHsibGFiZWxfcG9zaXRpb24iOjIwLCJjb2xvdXIiOlsxMjAsNjAsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMjAsNjAsNDAsMV1dLFs2LDIsInYnIiwyLHsiY29sb3VyIjpbMTIwLDYwLDQwXX0sWzEyMCw2MCw0MCwxXV0sWzYsMywiaCciLDIseyJsYWJlbF9wb3NpdGlvbiI6MjAsImNvbG91ciI6WzEyMCw2MCw0MF19LFsxMjAsNjAsNDAsMV1dLFs1LDQsIigxLGZeKl9cXERlbHRhKSIsMSx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzUsNiwiKGZfKiwgMSkiLDEseyJjb2xvdXIiOlsxMjAsNjAsNDBdfSxbMTIwLDYwLDQwLDFdXSxbNCw3LCJcXCNfRyIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzYsNywiXFwjX3tHJ30iLDIseyJjb2xvdXIiOlsxMjAsNjAsNDBdfSxbMTIwLDYwLDQwLDFdXSxbNCwxLCJ2IiwwLHsibGFiZWxfcG9zaXRpb24iOjMwLCJjb2xvdXIiOlswLDYwLDYwXX0sWzAsNjAsNjAsMV1dLFs1LDAsIlxcdHdpeHtofSIsMix7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzAsNjAsNjAsMV1dLFs1LDcsInBfZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs4LDksIlxcYXJmdW4iLDEseyJjdXJ2ZSI6LTJ9XSxbNCw5LCJcXGRvbV9HIiwxLHsiY3VydmUiOjEsImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbNiw4LCJcXGVsbFh7Ryd9IiwxLHsibGFiZWxfcG9zaXRpb24iOjMwLCJjdXJ2ZSI6LTEsImNvbG91ciI6WzEyMCw2MCw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MCwxXV0sWzcsOSwiXFxjb2RePyIsMl0sWzcsOCwiXFxlbGxeP19cXGNzaWciLDAseyJsYWJlbF9wb3NpdGlvbiI6NzB9XSxbMTAsNywiXFxva0Fycm93IiwyLHsiY3VydmUiOjJ9XSxbMTEsMTAsIlxcbGlmdGVkWHtcXCNfR30iLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzEzLDEwLCJxX2YiLDJdLFsxMiwxMCwiXFxsaWZ0ZWRYe1xcI197Ryd9fSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY29sb3VyIjpbMTIwLDYwLDQwXX0sWzEyMCw2MCw0MCwxXV0sWzEzLDExLCJcXHJob19mIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19LFswLDYwLDYwLDFdXSxbMTMsMTIsIlxccmhvJ19mIiwyLHsiY29sb3VyIjpbMTIwLDYwLDQwXX0sWzEyMCw2MCw0MCwxXV0sWzEwLDgsIlxcZWxsWHtcXGNzaWd9IiwyXSxbMTIsNiwiXFxsaWZ0ZWRYe1xcb2tBcnJvd31fe0cnfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY3VydmUiOjIsImNvbG91ciI6WzEyMCw2MCw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MCwxXV0sWzEzLDUsIlxcbGlmdGVkWHtcXG9rQXJyb3d9X2YiLDIseyJsYWJlbF9wb3NpdGlvbiI6NDAsImN1cnZlIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,row sep=small]
	\textcolor{rgb,255:red,214;green,92;blue,92}{\horzX{G}} \& \textcolor{rgb,255:red,214;green,92;blue,92}{\vertX{G}} \&\& \textcolor{rgb,255:red,41;green,163;blue,41}{\horzX{G'}} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\vertX{G'}} \\
	\textcolor{rgb,255:red,214;green,92;blue,92}{\PobjX{G}} \&\& {\PobjX{f}} \&\& \textcolor{rgb,255:red,41;green,163;blue,41}{\PobjX{G'}} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{\PsubobjX{G}} \& {\PsubobjX{f}} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\PsubobjX{G'}} \\
	\\
	\&\& {\okTargetX{\csig}} \&\&\&\&\& \OKobj \\
	\& \GG \&\& {\carrop{\csig}}
	\arrow["{f^*_\Delta}"', curve={height=18pt}, from=1-5, to=1-2]
	\arrow["{f_*}", curve={height=-18pt}, from=1-1, to=1-4]
	\arrow["h"', color={rgb,255:red,214;green,92;blue,92}, from=2-1, to=1-1]
	\arrow["{\twix{v}}"{pos=0.2}, color={rgb,255:red,41;green,163;blue,41}, dotted, from=2-3, to=1-5]
	\arrow["{v'}"', color={rgb,255:red,41;green,163;blue,41}, from=2-5, to=1-5]
	\arrow["{h'}"'{pos=0.2}, color={rgb,255:red,41;green,163;blue,41}, from=2-5, to=1-4]
	\arrow["{(1,f^*_\Delta)}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=2-3, to=2-1]
	\arrow["{(f_*, 1)}"{description}, color={rgb,255:red,41;green,163;blue,41}, from=2-3, to=2-5]
	\arrow["{\#_G}", color={rgb,255:red,214;green,92;blue,92}, from=2-1, to=4-3]
	\arrow["{\#_{G'}}"', color={rgb,255:red,41;green,163;blue,41}, from=2-5, to=4-3]
	\arrow["v"{pos=0.3}, color={rgb,255:red,214;green,92;blue,92}, from=2-1, to=1-2]
	\arrow["{\twix{h}}"'{pos=0.2}, color={rgb,255:red,214;green,92;blue,92}, dotted, from=2-3, to=1-1]
	\arrow["{p_f}"', dashed, from=2-3, to=4-3]
	\arrow["\arfun"{description}, curve={height=-12pt}, from=5-4, to=5-2]
	\arrow["{\dom_G}"{description}, color={rgb,255:red,214;green,92;blue,92}, curve={height=6pt}, dashed, from=2-1, to=5-2]
	\arrow["{\ellX{G'}}"{description, pos=0.3}, color={rgb,255:red,41;green,163;blue,41}, curve={height=-6pt}, dashed, from=2-5, to=5-4]
	\arrow["{\cod^?}"', from=4-3, to=5-2]
	\arrow["{\ell^?_\csig}"{pos=0.7}, from=4-3, to=5-4]
	\arrow["\okArrow"', curve={height=12pt}, from=4-8, to=4-3]
	\arrow["{\liftedX{\#_G}}"'{pos=0.3}, color={rgb,255:red,214;green,92;blue,92}, from=2-7, to=4-8]
	\arrow["{q_f}"', from=2-8, to=4-8]
	\arrow["{\liftedX{\#_{G'}}}"{pos=0.3}, color={rgb,255:red,41;green,163;blue,41}, from=2-9, to=4-8]
	\arrow["{\rho_f}", color={rgb,255:red,214;green,92;blue,92}, from=2-8, to=2-7]
	\arrow["{\rho'_f}"', color={rgb,255:red,41;green,163;blue,41}, from=2-8, to=2-9]
	\arrow["{\ellX{\csig}}"', from=4-8, to=5-4]
	\arrow["{\liftedX{\okArrow}_{G'}}"'{pos=0.2}, color={rgb,255:red,41;green,163;blue,41}, curve={height=12pt}, dashed, from=2-9, to=2-5]
	\arrow["{\liftedX{\okArrow}_f}"'{pos=0.4}, curve={height=12pt}, dotted, from=2-8, to=2-3]
\end{tikzcd}
}
\begin{figure}
\begin{equation}\label{eqdiag:mainTHProof-chasing}
		%\mainThProofChasingNew
		\mainThProofChasingNewest
\end{equation}
%\vspace{-1ex}
\begin{equation}\label{eqdiag:mainTHProof-cattyOkayed}
	\cattyOkayedFull
\end{equation}
\end{figure}

==> diagrams/collage4jmonic.tex <==
{ %\begin{group}




\begin{figure}[h]
\[
	\xymatrix @C=3em %3.25em %6em %5em 
	{
% row 1
	& \textcolor{red}{\Node} & & 
\\  % row 2
	& \textcolor{red}{\Edge} 
	\ar@[red]@<+0.5ex>[u]^{\textcolor{red}{\so}} 
	\ar@[red]@<-0.5ex>[u]_{\textcolor{red}{\ta}} 
& & 
\\ % row 3
	\textcolor{orange}{[1]} 
%--> to coproduct	\ar@[orange]@{^{(}-->}[ddr] 
	\ar[ur]^{\ovr{01}} %
	\ar@/^2.pc/[uur]^{\ovr{0}} 
	\ar@/^0.5pc/[uur]^{\ovr{1}}
% phantom arrow  \ar@{}[r]|{p_1\!\comp\ovr{01}= \ovr{10},\;etc} %~p_2\comp\ovr{01}=\ovr{32}}
	& \textcolor{orange}{\jmpred}
		\ar@[orange]@<+0.5ex>[l]^{	\textcolor{orange}{p_1}} 
		\ar@[orange]@<-0.5ex>[l]_{	\textcolor{orange}{p_2}}
		\ar@<+0.5ex>[u]^{\ovr{10}} 
		\ar@<-0.5ex>[u]_{\ovr{20}}
		\ar@/_2.65pc/[uu]^{\ovr{0}} 
		\ar@/_3.pc/[uu]|{\ovr{1}}
		\ar@/_3.35pc/[uu]_{\ovr{2}}
%	&	& 
%	*-<1px>{\qqquad\scriptsize )\!)\!)\{\ovr{0},\ovr{1},\ovr{2},\ovr{3}\} } 
%	\ar@3{->}@/_1pc/[uull] 
%\\ % row 4
%& 	
%
%%\ar@[orange][ur]^{	\textcolor{orange}{p}} 
%\ar@2{->}[uu]|{\{\ovr{10},\ovr{20}\}} % % \ar@3{->}@/_13pc/[uuu]^{\{\ovr{0},\ovr{1},\ovr{2},\ovr{3}\}} causes arithmetic overflow
%\ar@3{-}@/_2pc/[urr]^{} 
%%--> to coproduct \ar@[orange]@{^{(}-->}[d] 
%& &
%--> the copoduct node 
%\\  % row 5
%& \textcolor{orange}{\textsf{\{\monicpred, \pbpred,\commsqpred\}}} \ar@[orange]@{-->}[r]^{\qquad\textcolor{orange}{\plabel^!}} 
%&\textcolor{orange}{\predsigpbm} 
%&
}
\]
\caption{Collage of $\predsig_\jmpred$ and $\II_\Graph$ : elements of \II\ and \PP\ are, resp., red and orange,
	binding (wavy) arrows are black
}
\label{fig:collage-pbm}
\end{figure}
} %\end{group}


==> diagrams/collage4pbmonic.tex <==
\begin{figure}[h]
\[
	\xymatrix @C=6em %5em 
	{
% row 1
	& \textcolor{red}{\Node} & & 
\\  % row 2
& \textcolor{red}{\Edge} 
\ar@[red]@<+0.5ex>[u]^{\textcolor{red}{\so}} 
\ar@[red]@<-0.5ex>[u]_{\textcolor{red}{\ta}} 
& & 
\\ % row 3
	\textcolor{orange}{\monicpred} 
%--> to coproduct	\ar@[orange]@{^{(}-->}[ddr] 
	\ar[ur]^{\ovr{01}} %
	\ar@/^3.5pc/[uur]^{\ovr{0}} 
	\ar@/^1.5pc/[uur]^{\ovr{1}}
	\ar@{}[r]|{p_1\!\comp\ovr{01}= \ovr{10},\;etc} %~p_2\comp\ovr{01}=\ovr{32}}
	& 
	& 	\textcolor{orange}{\commsqpred} \ar@3{->}[ul]|{\{\ovr{10},\ovr{30},\ovr{23},\ovr{21}\}} 
	\ar@3{->}[uul]|{\{\ovr{0},\ovr{1},\ovr{2},\ovr{3}\}} 
%--> to coproduct	\ar@[orange]@{_{(}-->}[ddl] 
	\ar@{}[l]|{p\comp\ovr{10}= \ovr{10},\;etc} 
	& 
	*-<1px>{\qqquad\scriptsize )\!)\!)\{\ovr{0},\ovr{1},\ovr{2},\ovr{3}\} } 
	\ar@3{->}@/_1pc/[uull] 
\\ % row 4
& 	\textcolor{orange}{\pbmpred}
\ar@[orange]@<+0.5ex>[ul]^{	\textcolor{orange}{p_1}} 
\ar@[orange]@<-0.5ex>[ul]_{	\textcolor{orange}{p_2}}
\ar@[orange][ur]^{	\textcolor{orange}{p}} \ar@3{->}[uu]|{\{\ovr{10},\ovr{20},\ovr{32},\ovr{31}\}} % % \ar@3{->}@/_13pc/[uuu]^{\{\ovr{0},\ovr{1},\ovr{2},\ovr{3}\}} causes arithmetic overflow
\ar@3{-}@/_2pc/[urr]^{} 
%--> to coproduct \ar@[orange]@{^{(}-->}[d] 
& &
%--> the copoduct node 
%\\  % row 5
%& \textcolor{orange}{\textsf{\{\monicpred, \pbpred,\commsqpred\}}} \ar@[orange]@{-->}[r]^{\qquad\textcolor{orange}{\plabel^!}} 
%&\textcolor{orange}{\predsigpbm} 
%&
}
\]
\caption{Collage of \predsigpbm\ and $\II_\Graph$ : elements of \II\ and \PP\ are, resp., blue and orange,
	binding (wavy) arrows are black
}
\label{fig:collage-pbm}
\end{figure}


==> diagrams/commaDiags--macros.tex <==
%		Content
%----
%==  1) commalemma-General 
%		\longOrane
%		\longGreen
%		\commalemmaGeneralDiamond
%		\commalemmaGeneralElementsFull
%
%== 2) commalemma-Special 
%		\commalemmaDiamondSpecial
%		\commalemmaSpecialElementsSmall -- Not Used
%		\commalemmaSpecialElementsFull
%		\newleft
%		\newright
%
%=== 3)  Institution Definition
%		\ModSenPB  % for the name of the PB of Mod x Sen
%		\instDefoooIndToFiboooFirst
%		\instDefoooIndToFiboooSecond

%==  1) commalemma-General 
\newcommand{\longOrange}{
	\begin{array}{c}
		\textcolor{rgb,255:red,56;green,188;blue,41}{\tau.w_*}\textcolor{rgb,255:red,220;green,115;blue,86}{.v^*}
		\textcolor{black}{=} \\ [-3.5pt]
		\textcolor{black}{(b_1{,}{(f_*)^*}\!,a_1)}
	\end{array}
}
\newcommand{\longGreen}{
	\begin{array}{c}
		\textcolor{rgb,255:red,220;green,115;blue,86}{\tau.v^*} 
		\textcolor{rgb,255:red,56;green,188;blue,41}{.w_*}	\textcolor{black}{=} \\ [-3.5pt]
		\textcolor{black}{(b_1,(f^*)_*,a_1)}
	\end{array}
}


%------



\newcommand{\commalemmaGeneralDiamond}{
	% https://q.uiver.app/?q=WzAsNCxbMiwwLCJcXGNvbW1hY2F0WVh7cX17cH0iLFsyNDAsNjAsNjAsMV1dLFswLDEsIlxcQkIiXSxbNCwxLCJcXEFBIl0sWzIsMiwiXFxYWCJdLFsxLDMsInEiLDJdLFsyLDMsInAiXSxbMCwyLCJcXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dLFswLDEsIlxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6MiwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjQwLDYwLDYwLDFdXSxbMCwzLCJcXG9kb3QiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwxLCJcXHRleHR7W29wZl19IiwwLHsibGFiZWxfcG9zaXRpb24iOjYwLCJvZmZzZXQiOjMsImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzI0MCw2MCw2MCwxXV0sWzAsMiwiXFx0ZXh0e1tmaWJdfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo2MCwib2Zmc2V0IjotMywic2hvcnRlbiI6eyJzb3VyY2UiOjEwfSwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjQwLDYwLDYwLDFdXSxbNyw2LCJcXHRleHR7W2ZpYnIuc3Bhbl19IiwxLHsibGV2ZWwiOjEsImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjQwLDYwLDYwLDFdXV0=
	\begin{tikzcd}[ampersand replacement=\&, sep=scriptsize] %,column sep=small,row sep=scriptsize]
		\&\& \textcolor{rgb,255:red,92;green,92;blue,214}{\commacatYX{q}{p}} \\
		\BB \&\&\&\& \AA \\
		\&\& \XX
		\arrow["q"', from=2-1, to=3-3]
		\arrow["p", from=2-5, to=3-3]
		\arrow[""{name=0, anchor=center, inner sep=0}, "{\liftedX{q}}", shift left=2, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-3, to=2-5]
		\arrow[""{name=1, anchor=center, inner sep=0}, "{\liftedX{p}}"', shift right=2, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-3, to=2-1]
		\arrow["\odot"{description}, draw=none, from=1-3, to=3-3]
		\arrow["{\text{[opf]}}"{pos=0.6}, shift right=3, color={rgb,255:red,92;green,92;blue,214}, draw=none, from=1-3, to=2-1]
		\arrow["{\text{[fib]}}"'{pos=0.6}, shift left=3, color={rgb,255:red,92;green,92;blue,214}, draw=none, from=1-3, to=2-5]
		\arrow["{\text{[fibr.span]}}"{description}, color={rgb,255:red,92;green,92;blue,214}, dotted, no head, from=1, to=0]
	\end{tikzcd} 
}
%
%
%--------
\newcommand{\commalemmaGeneralElementsFull}{%row sep=4ex, column sep=2ex,
	% https://q.uiver.app/?q=WzAsMTQsWzAsMywiYl8xIixbMTE2LDU2LDYwLDFdXSxbNiwzLCJhXzEiLFsxMyw2Niw2MCwxXV0sWzEsNF0sWzIsNCwiYi5xIl0sWzQsNCwiYS5wIl0sWzIsNSwiYl8xLnEiXSxbNCw1LCJhXzEucCJdLFszLDAsIlxcdGF1PShiLGYsYSkiXSxbMCwyLCJiIl0sWzIsMiwiXFx0YXUud18qez19KGJfMSxmXyosYSkiLFsxMTQsNjQsNDUsMV1dLFs2LDIsImEiXSxbNCwyLCJcXHRhdS52Xip7PX0oYixmXiosYV8xKSIsWzEzLDY2LDYwLDFdXSxbMiwzLCJcXGxvbmdPcmFuZ2UiLFsxMyw2Niw2MCwxXV0sWzQsMywiXFxsb25nR3JlZW4iLFsxMTIsNjMsNDUsMV1dLFs0LDMsImYiLDJdLFs2LDQsInYucCJdLFszLDUsIncucSIsMl0sWzgsMCwidyIsMix7ImNvbG91ciI6WzExNiw1Niw2MF19LFsxMTYsNTYsNjAsMV1dLFs3LDgsIns6fVxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6Miwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs4LDMsIns6fXEiLDIseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzAsNSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs3LDksIlxcdGlsZGUgdyIsMix7ImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNiw1Niw2MCwxXV0sWzksMCwiIiwyLHsiY29sb3VyIjpbMTEyLDYzLDQ1XSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNywxMCwiezp9XFxsaWZ0ZWRYe3F9IiwwLHsib2Zmc2V0IjotMiwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxMCw0LCJ7On1wIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxLDEwLCJ2IiwwLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxMyw2Niw2MF19LFsxMyw2Niw2MCwxXV0sWzEsNiwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxMSw3LCJcXGJhciB2IiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzExLDEsIiIsMCx7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCw1LCJmXyoiLDIseyJsYWJlbF9wb3NpdGlvbiI6ODAsImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExMiw2Myw0NSwxXV0sWzYsMywiZl4qIiwyLHsibGFiZWxfcG9zaXRpb24iOjIwLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbOSwxMCwiIiwxLHsiY3VydmUiOi00LCJjb2xvdXIiOlsxMTIsNjMsNDVdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMSw4LCIiLDIseyJjdXJ2ZSI6NCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMiw5LCJcXGJhciB2JyIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFsxMiwxLCIiLDEseyJjdXJ2ZSI6LTMsImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTEsMTMsIlxcdGlsZGUgdyciLDIseyJjb2xvdXIiOlsxMTYsNTYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTYsNTYsNjAsMV1dLFsxMywwLCIiLDEseyJjdXJ2ZSI6MywiY29sb3VyIjpbMTEyLDYzLDQ1XSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTMsOSwiIV8qIiwyLHsibGFiZWxfcG9zaXRpb24iOjcwLCJvZmZzZXQiOjEsImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExNiw1Niw2MCwxXV0sWzExLDEyLCIhXioiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6MSwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMyw2Niw2MCwxXV0sWzEzLDEyLCIhXipfKiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6ImFycm93aGVhZCJ9LCJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNiw1LCIoZl8qKV4qez19KHYucCkuZl8qIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzYsNSwiKGZeKilfKns9fWZeKi4ody5xKSIsMCx7Im9mZnNldCI6LTIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dXQ==
	\begin{tikzcd}[ampersand replacement=\&,column sep=tiny,row sep=scriptsize]
		\&\&\& {\tau=(b,f,a)} \\
		\\
		b \&\& \textcolor{rgb,255:red,56;green,188;blue,41}{\tau.w_*{=}(b_1,f_*,a)} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\tau.v^*{=}(b,f^*,a_1)} \&\& a \\
		\textcolor{rgb,255:red,103;green,210;blue,96}{b_1} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\longOrange} \&\& \textcolor{rgb,255:red,62;green,187;blue,42}{\longGreen} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{a_1} \\
		\& {} \& {b.q} \&\& {a.p} \\
		\&\& {b_1.q} \&\& {a_1.p}
		\arrow["f"', from=5-5, to=5-3]
		\arrow["{v.p}", from=6-5, to=5-5]
		\arrow["{w.q}"', from=5-3, to=6-3]
		\arrow["w"', color={rgb,255:red,103;green,210;blue,96}, from=3-1, to=4-1]
		\arrow["{{:}\liftedX{p}}"', shift right=2, maps to, from=1-4, to=3-1]
		\arrow["{{:}q}"', maps to, from=3-1, to=5-3]
		\arrow[maps to, from=4-1, to=6-3]
		\arrow["{\tilde w}"'{text={rgb,255:red,103;green,210;blue,96}}, draw={rgb,255:red,62;green,187;blue,42}, dashed, from=1-4, to=3-3]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, dashed, maps to, from=3-3, to=4-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, maps to, from=1-4, to=3-7]
		\arrow["{{:}p}", maps to, from=3-7, to=5-5]
		\arrow["v", shift right=2, color={rgb,255:red,220;green,115;blue,86}, from=4-7, to=3-7]
		\arrow[maps to, from=4-7, to=6-5]
		\arrow["{\bar v}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-5, to=1-4]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=3-5, to=4-7]
		\arrow["{f_*}"'{pos=0.8}, color={rgb,255:red,62;green,187;blue,42}, dotted, from=5-5, to=6-3]
		\arrow["{f^*}"'{pos=0.2}, color={rgb,255:red,220;green,115;blue,86}, dotted, from=6-5, to=5-3]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, curve={height=-24pt}, dashed, maps to, from=3-3, to=3-7]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, curve={height=24pt}, dashed, maps to, from=3-5, to=3-1]
		\arrow["{\bar v'}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=4-3, to=3-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, curve={height=-18pt}, dashed, maps to, from=4-3, to=4-7]
		\arrow["{\tilde w'}"', color={rgb,255:red,103;green,210;blue,96}, dashed, from=3-5, to=4-5]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, curve={height=18pt}, dashed, maps to, from=4-5, to=4-1]
		\arrow["{!_*}"'{pos=0.7, text={rgb,255:red,103;green,210;blue,96}}, shift right=1, draw={rgb,255:red,62;green,187;blue,42}, dotted, from=4-5, to=3-3]
		\arrow["{!^*}"'{pos=0.3}, shift right=1, color={rgb,255:red,220;green,115;blue,86}, dotted, from=3-5, to=4-3]
		\arrow["{!^*_*}", dotted, tail reversed, from=4-5, to=4-3]
		\arrow["{(f_*)^*{=}(v.p).f_*}"', dotted, from=6-5, to=6-3]
		\arrow["{(f^*)_*{=}f^*.(w.q)}", shift left=2, dotted, from=6-5, to=6-3]
	\end{tikzcd}
}

%== 2) commalemma-Special 
%======
\newcommand{\newLeft}{\gapnamegap{-1.5}{\commafibLegUp}{1.5}}
\newcommand{\newRight}{\gapnamegap{1.5}{\commafibLegDn}{-1.5}}


\newcommand{\commalemmaSpecialDiamond}{
% https://q.uiver.app/#q=WzAsNixbMiwwLCJcXGNvbW1hY2F0WVh7cX17cH0iXSxbMCwyLCJcXEJCIl0sWzQsMiwiXFxBQSJdLFsyLDMsIlxcWFgiXSxbMiwyLCJcXEJCXFx0aW1lc197X1xcWFh9XFxBQSIsWzIzNCw3Nyw2MCwxXV0sWzEsM10sWzEsMywicSJdLFsyLDMsInAiLDJdLFs0LDEsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDIsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDMsIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMiwiXFxsaWZ0ZWRYe3F9IiwwLHsib2Zmc2V0IjotMiwiY29sb3VyIjpbMTMsNjYsNjBdfSxbMTMsNjYsNjAsMV1dLFswLDEsIlxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6MiwiY29sb3VyIjpbMTA5LDU5LDQ1XX0sWzEwOSw1OSw0NSwxXV0sWzAsNCwiIV4qIiwyLHsib2Zmc2V0Ijo1LCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMCw0LCIhXyoiLDAseyJvZmZzZXQiOi01LCJjb2xvdXIiOlsxMDksNTksNDVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMDksNTksNDUsMV1dLFswLDEsIlxcbmV3bGVmdCIsMCx7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFswLDIsIlxcbmV3cmlnaHQiLDIseyJjb2xvdXIiOlsxMDksNTksNDVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMDksNTksNDUsMV1dLFsxLDMsIlxcdGV4dHtbZmliXX0iLDIseyJjb2xvdXIiOlsyLDgxLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMiw4MSw2MCwxXV0sWzIsMywiXFx0ZXh0e1tvcGZdfSIsMCx7ImNvbG91ciI6WzIsODEsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsyLDgxLDYwLDFdXSxbNCwwLCJpIiwxLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibW9ubyJ9fX1dLFsxOSwxMywiIiwxLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XSxbMTQsMTksIiIsMSx7ImxldmVsIjoxLCJzdHlsZSI6eyJuYW1lIjoiYWRqdW5jdGlvbiJ9fV1d
\begin{tikzcd}[ampersand replacement=\&]
	\&\& {\commacatYX{q}{p}} \\
	\\
	\BB \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\BB\times_{_\XX}\AA} \&\& \AA \\
	\& {} \& \XX
	\arrow["q", from=3-1, to=4-3]
	\arrow["p"', from=3-5, to=4-3]
	\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=3-3, to=3-1]
	\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=3-3, to=3-5]
	\arrow["{\text{[pb]}}"{description, pos=0.4}, draw=none, from=3-3, to=4-3]
	\arrow["{\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, from=1-3, to=3-5]
	\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,72;green,182;blue,47}, from=1-3, to=3-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{!^*}"', shift right=5, color={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=3-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{!_*}", shift left=5, color={rgb,255:red,72;green,182;blue,47}, dashed, from=1-3, to=3-3]
	\arrow["\newleft", color={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=3-1]
	\arrow["\newright"', color={rgb,255:red,72;green,182;blue,47}, dashed, from=1-3, to=3-5]
	\arrow["{\text{[fib]}}"', color={rgb,255:red,236;green,76;blue,70}, draw=none, from=3-1, to=4-3]
	\arrow["{\text{[opf]}}", color={rgb,255:red,236;green,76;blue,70}, draw=none, from=3-5, to=4-3]
	\arrow[""{name=2, anchor=center, inner sep=0}, "i"{description}, tail, from=3-3, to=1-3]
	\arrow["\dashv"{anchor=center, rotate=-180}, draw=none, from=2, to=0]
	\arrow["\dashv"{anchor=center, rotate=-180}, draw=none, from=1, to=2]
\end{tikzcd}
}%

%\renewcommand{\newleft}{\gapnamegap{-1.5}{\commafibLegUp}{1.5}}
%\renewcommand{\newright}{\gapnamegap{1.5}{\commafibLegDn}{-1.5}}


\newcommand{\commalemmaSpecialElementsSmall}{ %column sep=1.25ex, row sep=2ex
	% https://q.uiver.app/?q=WzAsOCxbMCwxLCJiIl0sWzYsMSwiYSJdLFszLDAsIihiLGYsYSkiXSxbMSwyXSxbMiwyLCJiLnEiXSxbNCwyLCJhLnAiXSxbNCwxLCJmXyooYSkiXSxbMiwxLCJmXiooYikiXSxbMiwwLCJ7On1cXGxpZnRlZFh7cH0iLDIseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19XSxbMiwxLCJ7On1cXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzAsNCwiezp9cSIsMix7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19XSxbMSw1LCJ7On1wIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs2LDQsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsNiwiXFxiYXIgZiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDAsIlxcdGlsZGUgZiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDUsIiIsMSx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzIsNywiezp9cF4qIiwyLHsib2Zmc2V0IjotMiwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMiw2LCJ7On1xXyoiLDAseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzUsNCwiZiIsMix7InNob3J0ZW4iOnsic291cmNlIjozMCwidGFyZ2V0IjozMH19XV0=
	\begin{tikzcd}[column sep=1.2ex, row sep=2ex, ampersand replacement=\&]
		\&\&\& {(b,f,a)} \\
		b \&\& {f^*(b)} \&\& {f_*(a)} \&\& a \\
		\& {} \& {b.q} \&\& {a.p}
		\arrow["{{:}\liftedX{p}}"', shift right=2, maps to, from=1-4, to=2-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, maps to, from=1-4, to=2-7]
		\arrow["{{:}q}"', maps to, from=2-1, to=3-3]
		\arrow["{{:}p}", maps to, from=2-7, to=3-5]
		\arrow[dashed, maps to, from=2-5, to=3-3]
		\arrow["{\bar f}", dashed, from=2-7, to=2-5]
		\arrow["{\tilde f}", dashed, from=2-3, to=2-1]
		\arrow[dashed, maps to, from=2-3, to=3-5]
		\arrow["{{:}p^*}"', shift left=2, color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=1-4, to=2-3]
		\arrow["{{:}q_*}", shift right=2, dashed, maps to, from=1-4, to=2-5]
		\arrow["f"', shorten <=18pt, shorten >=18pt, from=3-5, to=3-3]
	\end{tikzcd}
}
%



\newcommand{\newleft}{\gapnamegap{1.5}{\commafibLegUp}{-1.5}}
\newcommand{\newright}{\gapnamegap{-1.5}{\commafibLegDn}{1.5}}


%--------
\newcommand{\commalemmaSpecialElementsFull}{
% https://q.uiver.app/?q=WzAsMTUsWzAsMiwiYiJdLFs2LDIsImEiXSxbMywwLCIoYixmLGEpIl0sWzEsM10sWzIsNCwiYi5xIl0sWzQsNCwiYS5wIl0sWzQsMiwiZl8qKGEpIixbMTI1LDUwLDYwLDFdXSxbMiwyLCJmXiooYikiLFsxMyw2Niw2MCwxXV0sWzMsMSwiKGJfMSxmXzEsYV8xKSJdLFswLDMsImJfMSJdLFsyLDMsImZfMV4qKGJfMSkiLFsxMyw2Niw2MCwxXV0sWzIsNSwiYl8xLnEiXSxbNCw1LCJhXzEucCJdLFs2LDMsImFfMSJdLFs0LDMsIntmXzF9XyooYV8xKSIsWzEyNSw1MCw2MCwxXV0sWzIsMCwiezp9XFxsaWZ0ZWRYe3B9IiwyLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fSxbMTI1LDUwLDYwLDFdXSxbMiwxLCJ7On1cXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzAsNCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzEsNSwiIiwwLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs2LDQsIiIsMCx7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsNiwiXFxiYXIgZiIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyNSw1MCw2MCwxXV0sWzcsMCwiXFx0aWxkZSBmIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzcsNSwiIiwxLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsyLDcsIlxcbmV3bGVmdCIsMix7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMiw2LCJcXG5ld3JpZ2h0IiwwLHsibGFiZWxfcG9zaXRpb24iOjgwLCJvZmZzZXQiOjIsImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTI1LDUwLDYwLDFdXSxbNSw0LCJmIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjEwLCJ0YXJnZXQiOjEwfX1dLFsyLDgsIih3LHYpIiwyXSxbMCw5LCJ3IiwyXSxbMTAsOSwiXFx0aWxkZXtmXzF9IiwyLHsibGFiZWxfcG9zaXRpb24iOjIwLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMTIsMTEsImZfMSIsMix7InNob3J0ZW4iOnsic291cmNlIjoxMCwidGFyZ2V0IjoxMH19XSxbNCwxMSwidy5xIiwyLHsibGFiZWxfcG9zaXRpb24iOjMwfV0sWzUsMTIsInYucCIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMH1dLFs3LDksIiIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzUsMTEsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxMCwxMiwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDExLCJ7On1xIiwwLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fSxbMTMsNjYsNjAsMV1dLFs3LDEwLCIhX3tcXHRpbGRle2ZfMX19IiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzgsMTAsIiIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTMsMTIsIns6fXAiLDIseyJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fSxbMTI1LDUwLDYwLDFdXSxbMSwxMywidiIsMl0sWzEzLDE0LCJcXGJhciBmXzEiLDIseyJsYWJlbF9wb3NpdGlvbiI6MjAsImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyNSw1MCw2MCwxXV0sWzYsMTQsIiFfe1xcYmFye2Z9fSIsMCx7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyNSw1MCw2MCwxXV0sWzEsMTQsIiIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs4LDE0LCIiLDIseyJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxNCwxMSwiIiwwLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=scriptsize]
	\&\&\& {(b,f,a)} \\
	\&\&\& {(b_1,f_1,a_1)} \\
	b \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{f^*(b)} \&\& \textcolor{rgb,255:red,102;green,204;blue,111}{f_*(a)} \&\& a \\
	{b_1} \& {} \& \textcolor{rgb,255:red,220;green,115;blue,86}{f_1^*(b_1)} \&\& \textcolor{rgb,255:red,102;green,204;blue,111}{{f_1}_*(a_1)} \&\& {a_1} \\
	\&\& {b.q} \&\& {a.p} \\
	\&\& {b_1.q} \&\& {a_1.p}
	\arrow["{{:}\liftedX{p}}"', shift right=2, color={rgb,255:red,102;green,204;blue,111}, maps to, from=1-4, to=3-1]
	\arrow["{{:}\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, maps to, from=1-4, to=3-7]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, maps to, from=3-1, to=5-3]
	\arrow[draw={rgb,255:red,102;green,204;blue,111}, maps to, from=3-7, to=5-5]
	\arrow[draw={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=3-5, to=5-3]
	\arrow["{\bar f}"', color={rgb,255:red,102;green,204;blue,111}, dashed, from=3-7, to=3-5]
	\arrow["{\tilde f}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-3, to=3-1]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=3-3, to=5-5]
	\arrow["\newleft"'{pos=0.8}, color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=1-4, to=3-3]
	\arrow["\newright"{pos=0.8}, shift right=2, color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=1-4, to=3-5]
	\arrow["f"', shorten <=7pt, shorten >=7pt, from=5-5, to=5-3]
	\arrow["{(w,v)}"', from=1-4, to=2-4]
	\arrow["w"', from=3-1, to=4-1]
	\arrow["{\tilde{f_1}}"'{pos=0.2}, color={rgb,255:red,220;green,115;blue,86}, dashed, from=4-3, to=4-1]
	\arrow["{f_1}"', shorten <=7pt, shorten >=7pt, from=6-5, to=6-3]
	\arrow["{w.q}"'{pos=0.3}, from=5-3, to=6-3]
	\arrow["{v.p}"'{pos=0.3}, from=5-5, to=6-5]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, dotted, from=3-3, to=4-1]
	\arrow[dotted, from=5-5, to=6-3]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=4-3, to=6-5]
	\arrow["{{:}q}", color={rgb,255:red,220;green,115;blue,86}, maps to, from=4-1, to=6-3]
	\arrow["{!_{\tilde{f_1}}}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-3, to=4-3]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=2-4, to=4-3]
	\arrow["{{:}p}"', color={rgb,255:red,102;green,204;blue,111}, maps to, from=4-7, to=6-5]
	\arrow["v"', from=3-7, to=4-7]
	\arrow["{\bar f_1}"'{pos=0.2}, color={rgb,255:red,102;green,204;blue,111}, dashed, from=4-7, to=4-5]
	\arrow["{!_{\bar{f}}}", color={rgb,255:red,102;green,204;blue,111}, dashed, from=3-5, to=4-5]
	\arrow[draw={rgb,255:red,102;green,204;blue,111}, dotted, from=3-7, to=4-5]
	\arrow[draw={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=2-4, to=4-5]
	\arrow[draw={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=4-5, to=6-3]
\end{tikzcd}
}




%====== 3)  Institution Definition

\renewcommand{\newleft}{\gapnamegap{-0}{\commafibLegUp}{0}}
\renewcommand{\newright}{\gapnamegap{0}{\commafibLegDn}{-2.5}}

\newcommand{\ModSenPB}{\enma{\Modcat{\times_{_{\!(p,q)}}}\Sencat}}
%--------
\newcommand{\instDefoooIndToFiboooFirst}{
% https://q.uiver.app/#q=WzAsMTAsWzMsMl0sWzEsMywiXFxNb2RjYXQiXSxbNSwzLCJcXFNlbmNhdCJdLFszLDUsIlxcU2lnY2F0Il0sWzMsMywiXFxNb2RTZW5QQiIsWzIzNCw3Nyw2MCwxXV0sWzAsMV0sWzEsMSwiXFxjb21tYWNhdFhZe3B9e3F9IixbMjI3LDgwLDYwLDFdXSxbNSwxLCJcXG1vZGVscyJdLFsyLDAsIlxcdHdpeER7XFxtb2RlbHN9XioiLFsxMyw2Niw2MCwxXV0sWzQsMCwiXFx0d2l4VXtcXG1vZGVsc31fKiIsWzE2MCw1Niw0NCwxXV0sWzEsMywicSIsMl0sWzIsMywicCJdLFs0LDEsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDIsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDMsIlxcdGV4dHt9IiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMSwiXFxsaWZ0ZWRYe3B9IiwyLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxNjAsNTYsNDRdfSxbMTYwLDU2LDQ0LDFdXSxbNiwxLCJcXG5ld2xlZnQiLDAseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbNiwyLCJcXG5ld3JpZ2h0IiwyLHsib2Zmc2V0IjotMSwiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTYwLDU2LDQ0LDFdXSxbNiwyLCJcXGxpZnRlZFh7cX0iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6LTMsImNvbG91ciI6WzEzLDY2LDYwXX0sWzEzLDY2LDYwLDFdXSxbNiw0LCIhXioiLDEseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsidGFyZ2V0IjoxMH0sImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFs2LDQsIiFfKiIsMSx7Im9mZnNldCI6LTIsImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzE2MCw1Niw0NCwxXV0sWzcsMiwiXFxzZW5mdW4iXSxbNyw0LCIiLDIseyJvZmZzZXQiOi0xLCJzaG9ydGVuIjp7InNvdXJjZSI6MTAsInRhcmdldCI6MTB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNywxLCJcXG1vZGZ1biIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMH1dLFs4LDYsIiIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzgsNywiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSw2LCIiLDIseyJjb2xvdXIiOlsxNjAsNTYsNDRdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSw3LCIiLDIseyJjb2xvdXIiOlsxNjAsNTYsNDRdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOCw5LCJqIiwwLHsib2Zmc2V0IjotMSwiY29sb3VyIjpbMzU3LDgwLDUwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMzU3LDgwLDUwLDFdXSxbNCw4LCJcXHRleHR7W3BiXX0iLDEseyJsYWJlbF9wb3NpdGlvbiI6ODAsImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTMsNjYsNjAsMV1dLFs5LDQsIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTYwLDU2LDQ0LDFdXSxbMiwzLCJcXHRleHR7W29wZl19IiwwLHsib2Zmc2V0IjotMSwiY3VydmUiOi0xLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSwzLCJcXHRleHR7W2ZpYl19IiwyLHsib2Zmc2V0IjoxLCJjdXJ2ZSI6MSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsNiwiaSIsMSx7Im9mZnNldCI6LTEsImNvbG91ciI6WzIyNyw4MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1vbm8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjI3LDgwLDYwLDFdXSxbOSw4LCIiLDEseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlszNTcsODAsNTBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMiwxLCJwL1xcIS9xIiwwLHsiY3VydmUiOi0zLCJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9LCJsZXZlbCI6Mn1dLFsyMCwzMywiIiwxLHsib2Zmc2V0Ijo0LCJsZXZlbCI6MSwic3R5bGUiOnsibmFtZSI6ImFkanVuY3Rpb24ifX1dLFszNCwyOCwiXFxjb25nIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwiY29sb3VyIjpbMzU3LDgwLDUwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMzU3LDgwLDUwLDFdXSxbMjUsOSwiXFxvZG90IiwxLHsib2Zmc2V0IjotMSwic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMzLDE5LCIiLDEseyJvZmZzZXQiOjQsImxldmVsIjoxLCJzdHlsZSI6eyJuYW1lIjoiYWRqdW5jdGlvbiJ9fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\twixD{\models}^*} \&\& \textcolor{rgb,255:red,49;green,175;blue,133}{\twixU{\models}_*} \\
	{} \& \textcolor{rgb,255:red,71;green,107;blue,235}{\commacatXY{p}{q}} \&\&\&\& \models \\
	\&\&\& {} \\
	\& \Modcat \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\ModSenPB} \&\& \Sencat \\
	\\
	\&\&\& \Sigcat
	\arrow["q"', from=4-2, to=6-4]
	\arrow["p", from=4-6, to=6-4]
	\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-2]
	\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-6]
	\arrow["{\text{}}"{description}, draw=none, from=4-4, to=6-4]
	\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,49;green,175;blue,133}, from=2-2, to=4-2]
	\arrow["\newleft", shift left=1, color={rgb,255:red,220;green,115;blue,86}, dashed, from=2-2, to=4-2]
	\arrow["\newright"', shift left=1, color={rgb,255:red,49;green,175;blue,133}, dashed, from=2-2, to=4-6]
	\arrow["{\liftedX{q}}"{pos=0.3}, shift left=3, color={rgb,255:red,220;green,115;blue,86}, from=2-2, to=4-6]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{!^*}"{description}, shift right=5, color={rgb,255:red,220;green,115;blue,86}, shorten >=9pt, dashed, from=2-2, to=4-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{!_*}"{description}, shift left=2, color={rgb,255:red,49;green,175;blue,133}, dashed, from=2-2, to=4-4]
	\arrow["\senfun", from=2-6, to=4-6]
	\arrow[shift left=1, shorten <=8pt, shorten >=8pt, dashed, from=2-6, to=4-4]
	\arrow["\modfun"'{pos=0.3}, from=2-6, to=4-2]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-6]
	\arrow[draw={rgb,255:red,49;green,175;blue,133}, dashed, from=1-5, to=2-2]
	\arrow[draw={rgb,255:red,49;green,175;blue,133}, dashed, from=1-5, to=2-6]
	\arrow[""{name=3, anchor=center, inner sep=0}, "j", shift left=1, color={rgb,255:red,230;green,25;blue,36}, dashed, from=1-3, to=1-5]
	\arrow["{\text{[pb]}}"{description, pos=0.8}, color={rgb,255:red,220;green,115;blue,86}, draw=none, from=4-4, to=1-3]
	\arrow["{\text{[pb]}}"{description, pos=0.2}, color={rgb,255:red,49;green,175;blue,133}, draw=none, from=1-5, to=4-4]
	\arrow["{\text{[opf]}}", shift left=1, curve={height=-6pt}, draw=none, from=4-6, to=6-4]
	\arrow["{\text{[fib]}}"', shift right=1, curve={height=6pt}, draw=none, from=4-2, to=6-4]
	\arrow[""{name=4, anchor=center, inner sep=0}, "i"{description}, shift left=1, color={rgb,255:red,71;green,107;blue,235}, dashed, tail, from=4-4, to=2-2]
	\arrow[""{name=5, anchor=center, inner sep=0}, shift left=1, draw={rgb,255:red,230;green,25;blue,36}, dashed, from=1-5, to=1-3]
	\arrow["{p/\!/q}", curve={height=-18pt}, shorten <=38pt, shorten >=38pt, Rightarrow, from=4-6, to=4-2]
	\arrow["\dashv"{anchor=center, rotate=-119}, shift right=4, draw=none, from=1, to=4]
	\arrow["\cong"{description}, color={rgb,255:red,230;green,25;blue,36}, draw=none, from=5, to=3]
	\arrow["\odot"{description}, shift left=1, draw=none, from=2, to=1-5]
	\arrow["\dashv"{anchor=center, rotate=-119}, shift right=4, draw=none, from=4, to=0]
\end{tikzcd}
}
%
%------
\newcommand{\instDefoooIndToFiboooSecond}{
% https://q.uiver.app/#q=WzAsOSxbMywyXSxbMSwzLCJcXE1vZGNhdCJdLFs1LDMsIlxcU2VuY2F0Il0sWzMsNSwiXFxTaWdjYXQiXSxbMywzLCJcXE1vZFNlblBCIixbMjM0LDc3LDYwLDFdXSxbMCwxXSxbMSwxLCJcXGNvbW1hY2F0WFl7cH17cX0iLFsyMjcsODAsNjAsMV1dLFs1LDEsIlxcbW9kZWxzIl0sWzMsMCwiXFx0d2l4RHtcXG1vZGVsc30iLFsxMyw2Niw2MCwxXV0sWzEsMywicSIsMl0sWzIsMywicCJdLFs0LDEsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDIsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDMsIlxcdGV4dHt9IiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMSwiXFxsaWZ0ZWRYe3B9IiwyLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxNjAsNTYsNDRdfSxbMTYwLDU2LDQ0LDFdXSxbNiwxLCJcXG5ld2xlZnQiLDAseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbNiwyLCJcXG5ld3JpZ2h0IiwyLHsib2Zmc2V0IjotMSwiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTYwLDU2LDQ0LDFdXSxbNiwyLCJcXGxpZnRlZFh7cX0iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6LTMsImNvbG91ciI6WzEzLDY2LDYwXX0sWzEzLDY2LDYwLDFdXSxbNiw0LCIhXioiLDEseyJvZmZzZXQiOjUsInNob3J0ZW4iOnsidGFyZ2V0IjoxMH0sImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFs2LDQsIiFfKiIsMSx7Im9mZnNldCI6LTIsImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzE2MCw1Niw0NCwxXV0sWzcsMiwiXFxzZW5mdW4iXSxbNyw0LCIiLDIseyJvZmZzZXQiOi0xLCJzaG9ydGVuIjp7InNvdXJjZSI6MTAsInRhcmdldCI6MTB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNywxLCJcXG1vZGZ1biIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMH1dLFs4LDYsIiIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzgsNywiIiwyLHsiY3VydmUiOjIsImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDgsIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMyw2Niw2MCwxXV0sWzIsMywiXFx0ZXh0e1tvcGZdfSIsMCx7Im9mZnNldCI6LTMsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDMsIlxcdGV4dHtbZmliXX0iLDIseyJvZmZzZXQiOjMsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDYsImkiLDEseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlsyMjcsODAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtb25vIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzIyNyw4MCw2MCwxXV0sWzgsNywiIiwyLHsiY3VydmUiOi0zLCJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzIsMSwicC9cXCEvcSIsMix7ImN1cnZlIjotNCwic2hvcnRlbiI6eyJzb3VyY2UiOjMwLCJ0YXJnZXQiOjMwfSwibGV2ZWwiOjJ9XSxbMTksMjgsIiIsMSx7Im9mZnNldCI6NCwibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XSxbMjgsMTgsIiIsMSx7Im9mZnNldCI6NCwibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XSxbMjksMjQsIlxcc3Bhbk1vciIsMix7InNob3J0ZW4iOnsic291cmNlIjozMCwidGFyZ2V0IjozMH19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\&\&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\twixD{\models}} \\
	{} \& \textcolor{rgb,255:red,71;green,107;blue,235}{\commacatXY{p}{q}} \&\&\&\& \models \\
	\&\&\& {} \\
	\& \Modcat \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\ModSenPB} \&\& \Sencat \\
	\\
	\&\&\& \Sigcat
	\arrow["q"', from=4-2, to=6-4]
	\arrow["p", from=4-6, to=6-4]
	\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-2]
	\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-6]
	\arrow["{\text{}}"{description}, draw=none, from=4-4, to=6-4]
	\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,49;green,175;blue,133}, from=2-2, to=4-2]
	\arrow["\newleft", shift left=1, color={rgb,255:red,220;green,115;blue,86}, dashed, from=2-2, to=4-2]
	\arrow["\newright"', shift left=1, color={rgb,255:red,49;green,175;blue,133}, dashed, from=2-2, to=4-6]
	\arrow["{\liftedX{q}}"{pos=0.3}, shift left=3, color={rgb,255:red,220;green,115;blue,86}, from=2-2, to=4-6]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{!^*}"{description}, shift right=5, color={rgb,255:red,220;green,115;blue,86}, shorten >=8pt, dashed, from=2-2, to=4-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{!_*}"{description}, shift left=2, color={rgb,255:red,49;green,175;blue,133}, dashed, from=2-2, to=4-4]
	\arrow["\senfun", from=2-6, to=4-6]
	\arrow[shift left=1, shorten <=7pt, shorten >=7pt, dashed, from=2-6, to=4-4]
	\arrow["\modfun"'{pos=0.3}, from=2-6, to=4-2]
	\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-4, to=2-2]
	\arrow[""{name=2, anchor=center, inner sep=0}, draw={rgb,255:red,49;green,175;blue,133}, curve={height=12pt}, dashed, from=1-4, to=2-6]
	\arrow["{\text{[pb]}}"{description, pos=0.8}, color={rgb,255:red,220;green,115;blue,86}, draw=none, from=4-4, to=1-4]
	\arrow["{\text{[opf]}}", shift left=3, draw=none, from=4-6, to=6-4]
	\arrow["{\text{[fib]}}"', shift right=3, draw=none, from=4-2, to=6-4]
	\arrow[""{name=3, anchor=center, inner sep=0}, "i"{description}, shift left=1, color={rgb,255:red,71;green,107;blue,235}, dashed, tail, from=4-4, to=2-2]
	\arrow[""{name=4, anchor=center, inner sep=0}, draw={rgb,255:red,214;green,92;blue,92}, curve={height=-18pt}, dashed, from=1-4, to=2-6]
	\arrow["{p/\!/q}"', curve={height=-24pt}, shorten <=47pt, shorten >=47pt, Rightarrow, from=4-6, to=4-2]
	\arrow["\dashv"{anchor=center, rotate=-123}, shift right=4, draw=none, from=1, to=3]
	\arrow["\dashv"{anchor=center, rotate=-123}, shift right=4, draw=none, from=3, to=0]
	\arrow["\spanMor"', shorten <=6pt, shorten >=6pt, Rightarrow, from=4, to=2]
\end{tikzcd}
}








%----
%
\newcommand{ \instFiberedToIndexedDiamond}{
Hru
}


==> diagrams/commaDiagsMacros--RESERVED.tex <==
%		Content
%----
%==  1) commalemma-General 
%		\longOrane
%		\longGreen
%		\commalemmaGeneralDiamond
%		\commalemmaGeneralElementsFull
%
%== 2) commalemma-Special 
%		\commalemmaDiamondSpecial
%		\commalemmaSpecialElementsSmall -- Not Used
%		\commalemmaSpecialElementsFull
%
%=== 3)  Institution Definition
%		\ModSenPB  % for the name of the PB of Mod x Sen
%		\instDefDiamond

%==  1) commalemma-General 
\newcommand{\longOrange}{
	\begin{array}{c}
		\textcolor{rgb,255:red,56;green,188;blue,41}{\tau.w_*}\textcolor{rgb,255:red,220;green,115;blue,86}{.v^*}
		\textcolor{black}{=} \\ [-3.5pt]
		\textcolor{black}{(b_1{,}{(f_*)^*}\!,a_1)}
	\end{array}
}
\newcommand{\longGreen}{
	\begin{array}{c}
		\textcolor{rgb,255:red,220;green,115;blue,86}{\tau.v^*} 
		\textcolor{rgb,255:red,56;green,188;blue,41}{.w_*}	\textcolor{black}{=} \\ [-3.5pt]
		\textcolor{black}{(b_1,(f^*)_*,a_1)}
	\end{array}
}


%------



\newcommand{\commalemmaGeneralDiamond}{
	% https://q.uiver.app/?q=WzAsNCxbMiwwLCJcXGNvbW1hY2F0WVh7cX17cH0iLFsyNDAsNjAsNjAsMV1dLFswLDEsIlxcQkIiXSxbNCwxLCJcXEFBIl0sWzIsMiwiXFxYWCJdLFsxLDMsInEiLDJdLFsyLDMsInAiXSxbMCwyLCJcXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dLFswLDEsIlxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6MiwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjQwLDYwLDYwLDFdXSxbMCwzLCJcXG9kb3QiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwxLCJcXHRleHR7W29wZl19IiwwLHsibGFiZWxfcG9zaXRpb24iOjYwLCJvZmZzZXQiOjMsImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzI0MCw2MCw2MCwxXV0sWzAsMiwiXFx0ZXh0e1tmaWJdfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo2MCwib2Zmc2V0IjotMywic2hvcnRlbiI6eyJzb3VyY2UiOjEwfSwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjQwLDYwLDYwLDFdXSxbNyw2LCJcXHRleHR7W2ZpYnIuc3Bhbl19IiwxLHsibGV2ZWwiOjEsImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjQwLDYwLDYwLDFdXV0=
	\begin{tikzcd}[ampersand replacement=\&,column sep=small,row sep=scriptsize]
		\&\& \textcolor{rgb,255:red,92;green,92;blue,214}{\commacatYX{q}{p}} \\
		\BB \&\&\&\& \AA \\
		\&\& \XX
		\arrow["q"', from=2-1, to=3-3]
		\arrow["p", from=2-5, to=3-3]
		\arrow[""{name=0, anchor=center, inner sep=0}, "{\liftedX{q}}", shift left=2, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-3, to=2-5]
		\arrow[""{name=1, anchor=center, inner sep=0}, "{\liftedX{p}}"', shift right=2, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-3, to=2-1]
		\arrow["\odot"{description}, draw=none, from=1-3, to=3-3]
		\arrow["{\text{[opf]}}"{pos=0.6}, shift right=3, color={rgb,255:red,92;green,92;blue,214}, draw=none, from=1-3, to=2-1]
		\arrow["{\text{[fib]}}"'{pos=0.6}, shift left=3, color={rgb,255:red,92;green,92;blue,214}, draw=none, from=1-3, to=2-5]
		\arrow["{\text{[fibr.span]}}"{description}, color={rgb,255:red,92;green,92;blue,214}, dotted, no head, from=1, to=0]
	\end{tikzcd} 
}
%
%
%--------
\newcommand{\commalemmaGeneralElementsFull}{%row sep=4ex, column sep=2ex,
	% https://q.uiver.app/?q=WzAsMTQsWzAsMywiYl8xIixbMTE2LDU2LDYwLDFdXSxbNiwzLCJhXzEiLFsxMyw2Niw2MCwxXV0sWzEsNF0sWzIsNCwiYi5xIl0sWzQsNCwiYS5wIl0sWzIsNSwiYl8xLnEiXSxbNCw1LCJhXzEucCJdLFszLDAsIlxcdGF1PShiLGYsYSkiXSxbMCwyLCJiIl0sWzIsMiwiXFx0YXUud18qez19KGJfMSxmXyosYSkiLFsxMTQsNjQsNDUsMV1dLFs2LDIsImEiXSxbNCwyLCJcXHRhdS52Xip7PX0oYixmXiosYV8xKSIsWzEzLDY2LDYwLDFdXSxbMiwzLCJcXGxvbmdPcmFuZ2UiLFsxMyw2Niw2MCwxXV0sWzQsMywiXFxsb25nR3JlZW4iLFsxMTIsNjMsNDUsMV1dLFs0LDMsImYiLDJdLFs2LDQsInYucCJdLFszLDUsIncucSIsMl0sWzgsMCwidyIsMix7ImNvbG91ciI6WzExNiw1Niw2MF19LFsxMTYsNTYsNjAsMV1dLFs3LDgsIns6fVxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6Miwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs4LDMsIns6fXEiLDIseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzAsNSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs3LDksIlxcdGlsZGUgdyIsMix7ImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNiw1Niw2MCwxXV0sWzksMCwiIiwyLHsiY29sb3VyIjpbMTEyLDYzLDQ1XSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNywxMCwiezp9XFxsaWZ0ZWRYe3F9IiwwLHsib2Zmc2V0IjotMiwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxMCw0LCJ7On1wIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxLDEwLCJ2IiwwLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxMyw2Niw2MF19LFsxMyw2Niw2MCwxXV0sWzEsNiwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxMSw3LCJcXGJhciB2IiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzExLDEsIiIsMCx7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCw1LCJmXyoiLDIseyJsYWJlbF9wb3NpdGlvbiI6ODAsImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExMiw2Myw0NSwxXV0sWzYsMywiZl4qIiwyLHsibGFiZWxfcG9zaXRpb24iOjIwLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbOSwxMCwiIiwxLHsiY3VydmUiOi00LCJjb2xvdXIiOlsxMTIsNjMsNDVdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMSw4LCIiLDIseyJjdXJ2ZSI6NCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMiw5LCJcXGJhciB2JyIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFsxMiwxLCIiLDEseyJjdXJ2ZSI6LTMsImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTEsMTMsIlxcdGlsZGUgdyciLDIseyJjb2xvdXIiOlsxMTYsNTYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTYsNTYsNjAsMV1dLFsxMywwLCIiLDEseyJjdXJ2ZSI6MywiY29sb3VyIjpbMTEyLDYzLDQ1XSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTMsOSwiIV8qIiwyLHsibGFiZWxfcG9zaXRpb24iOjcwLCJvZmZzZXQiOjEsImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExNiw1Niw2MCwxXV0sWzExLDEyLCIhXioiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6MSwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMyw2Niw2MCwxXV0sWzEzLDEyLCIhXipfKiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6ImFycm93aGVhZCJ9LCJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNiw1LCIoZl8qKV4qez19KHYucCkuZl8qIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzYsNSwiKGZeKilfKns9fWZeKi4ody5xKSIsMCx7Im9mZnNldCI6LTIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dXQ==
	\begin{tikzcd}[ampersand replacement=\&,column sep=tiny,row sep=scriptsize]
		\&\&\& {\tau=(b,f,a)} \\
		\\
		b \&\& \textcolor{rgb,255:red,56;green,188;blue,41}{\tau.w_*{=}(b_1,f_*,a)} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\tau.v^*{=}(b,f^*,a_1)} \&\& a \\
		\textcolor{rgb,255:red,103;green,210;blue,96}{b_1} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\longOrange} \&\& \textcolor{rgb,255:red,62;green,187;blue,42}{\longGreen} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{a_1} \\
		\& {} \& {b.q} \&\& {a.p} \\
		\&\& {b_1.q} \&\& {a_1.p}
		\arrow["f"', from=5-5, to=5-3]
		\arrow["{v.p}", from=6-5, to=5-5]
		\arrow["{w.q}"', from=5-3, to=6-3]
		\arrow["w"', color={rgb,255:red,103;green,210;blue,96}, from=3-1, to=4-1]
		\arrow["{{:}\liftedX{p}}"', shift right=2, maps to, from=1-4, to=3-1]
		\arrow["{{:}q}"', maps to, from=3-1, to=5-3]
		\arrow[maps to, from=4-1, to=6-3]
		\arrow["{\tilde w}"'{text={rgb,255:red,103;green,210;blue,96}}, draw={rgb,255:red,62;green,187;blue,42}, dashed, from=1-4, to=3-3]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, dashed, maps to, from=3-3, to=4-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, maps to, from=1-4, to=3-7]
		\arrow["{{:}p}", maps to, from=3-7, to=5-5]
		\arrow["v", shift right=2, color={rgb,255:red,220;green,115;blue,86}, from=4-7, to=3-7]
		\arrow[maps to, from=4-7, to=6-5]
		\arrow["{\bar v}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-5, to=1-4]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=3-5, to=4-7]
		\arrow["{f_*}"'{pos=0.8}, color={rgb,255:red,62;green,187;blue,42}, dotted, from=5-5, to=6-3]
		\arrow["{f^*}"'{pos=0.2}, color={rgb,255:red,220;green,115;blue,86}, dotted, from=6-5, to=5-3]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, curve={height=-24pt}, dashed, maps to, from=3-3, to=3-7]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, curve={height=24pt}, dashed, maps to, from=3-5, to=3-1]
		\arrow["{\bar v'}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=4-3, to=3-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, curve={height=-18pt}, dashed, maps to, from=4-3, to=4-7]
		\arrow["{\tilde w'}"', color={rgb,255:red,103;green,210;blue,96}, dashed, from=3-5, to=4-5]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, curve={height=18pt}, dashed, maps to, from=4-5, to=4-1]
		\arrow["{!_*}"'{pos=0.7, text={rgb,255:red,103;green,210;blue,96}}, shift right=1, draw={rgb,255:red,62;green,187;blue,42}, dotted, from=4-5, to=3-3]
		\arrow["{!^*}"'{pos=0.3}, shift right=1, color={rgb,255:red,220;green,115;blue,86}, dotted, from=3-5, to=4-3]
		\arrow["{!^*_*}", dotted, tail reversed, from=4-5, to=4-3]
		\arrow["{(f_*)^*{=}(v.p).f_*}"', dotted, from=6-5, to=6-3]
		\arrow["{(f^*)_*{=}f^*.(w.q)}", shift left=2, dotted, from=6-5, to=6-3]
	\end{tikzcd}
}

%== 2) commalemma-Special 
\newcommand{\commalemmaDiamondSpecial}{
	%% https://q.uiver.app/?q=WzAsNixbMiwwLCJcXGNvbW1hY2F0WFl7cX17cH0iXSxbMCwxLCJcXEJCIl0sWzQsMSwiXFxBQSJdLFsyLDIsIlxcWFgiXSxbMiwxLCJcXGNpcmMiLFsyMzQsNzcsNjAsMV1dLFsxLDJdLFsxLDMsInEiXSxbMiwzLCJwIiwyXSxbNCwxLCIiLDEseyJjb2xvdXIiOlsyMzQsNzcsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCwyLCIiLDEseyJjb2xvdXIiOlsyMzQsNzcsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCwzLCJcXHRleHR7W3BiXX0iLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDIsIlxcbGlmdGVkWHtxfSIsMCx7Im9mZnNldCI6LTIsImNvbG91ciI6WzEzLDY2LDYwXX0sWzEzLDY2LDYwLDFdXSxbMCwxLCJcXGxpZnRlZFh7cH0iLDIseyJvZmZzZXQiOjIsImNvbG91ciI6WzEwOSw1OSw0NV19LFsxMDksNTksNDUsMV1dLFswLDQsIiEnIiwyLHsib2Zmc2V0IjoxLCJjb2xvdXIiOlsxMDksNTksNDVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMDksNTksNDUsMV1dLFswLDQsIiEiLDAseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMCwxLCJwXioiLDAseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMCwyLCJxXyoiLDIseyJjb2xvdXIiOlsxMDksNTksNDVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMDksNTksNDUsMV1dLFsxLDMsIlxcdGV4dHtbZmliXX0iLDIseyJjb2xvdXIiOlsyLDgxLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMiw4MSw2MCwxXV0sWzIsMywiXFx0ZXh0e1tvcGZdfSIsMCx7ImNvbG91ciI6WzIsODEsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsyLDgxLDYwLDFdXV0=
	\begin{tikzcd}[ampersand replacement=\&,row sep=4ex, column sep=2ex]
		\&\& {\commacatYX{q}{p}} \\
		\BB \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\circ} \&\& \AA \\
		\& {} \& \XX
		\arrow["q", from=2-1, to=3-3]
		\arrow["p"', from=2-5, to=3-3]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=2-3, to=2-1]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=2-3, to=2-5]
		\arrow["{\text{[pb]}}"{description, pos=0.4}, draw=none, from=2-3, to=3-3]
		\arrow["{\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, from=1-3, to=2-5]
		\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,72;green,182;blue,47}, from=1-3, to=2-1]
		\arrow["{!'}"', shift right=1, color={rgb,255:red,72;green,182;blue,47}, dashed, from=1-3, to=2-3]
		\arrow["{!}", shift left=1, color={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-3]
		\arrow["{p^*}", color={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-1]
		\arrow["{q_*}"', color={rgb,255:red,72;green,182;blue,47}, dashed, from=1-3, to=2-5]
		\arrow["{\text{[fib]}}"', color={rgb,255:red,236;green,76;blue,70}, draw=none, from=2-1, to=3-3]
		\arrow["{\text{[opf]}}", color={rgb,255:red,236;green,76;blue,70}, draw=none, from=2-5, to=3-3]
	\end{tikzcd}
}%
%
\newcommand{\commalemmaSpecialElementsSmall}{ %column sep=1.25ex, row sep=2ex
	% https://q.uiver.app/?q=WzAsOCxbMCwxLCJiIl0sWzYsMSwiYSJdLFszLDAsIihiLGYsYSkiXSxbMSwyXSxbMiwyLCJiLnEiXSxbNCwyLCJhLnAiXSxbNCwxLCJmXyooYSkiXSxbMiwxLCJmXiooYikiXSxbMiwwLCJ7On1cXGxpZnRlZFh7cH0iLDIseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19XSxbMiwxLCJ7On1cXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzAsNCwiezp9cSIsMix7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19XSxbMSw1LCJ7On1wIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs2LDQsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsNiwiXFxiYXIgZiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDAsIlxcdGlsZGUgZiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDUsIiIsMSx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzIsNywiezp9cF4qIiwyLHsib2Zmc2V0IjotMiwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMiw2LCJ7On1xXyoiLDAseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzUsNCwiZiIsMix7InNob3J0ZW4iOnsic291cmNlIjozMCwidGFyZ2V0IjozMH19XV0=
	\begin{tikzcd}[column sep=1.2ex, row sep=2ex, ampersand replacement=\&]
		\&\&\& {(b,f,a)} \\
		b \&\& {f^*(b)} \&\& {f_*(a)} \&\& a \\
		\& {} \& {b.q} \&\& {a.p}
		\arrow["{{:}\liftedX{p}}"', shift right=2, maps to, from=1-4, to=2-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, maps to, from=1-4, to=2-7]
		\arrow["{{:}q}"', maps to, from=2-1, to=3-3]
		\arrow["{{:}p}", maps to, from=2-7, to=3-5]
		\arrow[dashed, maps to, from=2-5, to=3-3]
		\arrow["{\bar f}", dashed, from=2-7, to=2-5]
		\arrow["{\tilde f}", dashed, from=2-3, to=2-1]
		\arrow[dashed, maps to, from=2-3, to=3-5]
		\arrow["{{:}p^*}"', shift left=2, color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=1-4, to=2-3]
		\arrow["{{:}q_*}", shift right=2, dashed, maps to, from=1-4, to=2-5]
		\arrow["f"', shorten <=18pt, shorten >=18pt, from=3-5, to=3-3]
	\end{tikzcd}
}
%
%--------
\newcommand{\commalemmaSpecialElementsFull}{
	% https://q.uiver.app/?q=WzAsMTUsWzAsMiwiYiJdLFs2LDIsImEiXSxbMywwLCIoYixmLGEpIl0sWzEsM10sWzIsNCwiYi5xIl0sWzQsNCwiYS5wIl0sWzQsMiwiZl8qKGEpIixbMTI1LDUwLDYwLDFdXSxbMiwyLCJmXiooYikiLFsxMyw2Niw2MCwxXV0sWzMsMSwiKGJfMSxmXzEsYV8xKSJdLFswLDMsImJfMSJdLFsyLDMsImZfMV4qKGJfMSkiLFsxMyw2Niw2MCwxXV0sWzIsNSwiYl8xLnEiXSxbNCw1LCJhXzEucCJdLFs2LDMsImFfMSJdLFs0LDMsIntmXzF9XyooYV8xKSIsWzEyNSw1MCw2MCwxXV0sWzIsMCwiezp9XFxsaWZ0ZWRYe3B9IiwyLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fSxbMTI1LDUwLDYwLDFdXSxbMiwxLCJ7On1cXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzAsNCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzEsNSwiIiwwLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs2LDQsIiIsMCx7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsNiwiXFxiYXIgZiIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyNSw1MCw2MCwxXV0sWzcsMCwiXFx0aWxkZSBmIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzcsNSwiIiwxLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsyLDcsIns6fXB7XFxiZXR3ZWVufV57XFwhKn1xIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMiw2LCJ7On1xe1xcYmV0d2Vlbn1fe1xcISp9cCIsMCx7Im9mZnNldCI6MiwiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMjUsNTAsNjAsMV1dLFs1LDQsImYiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MTAsInRhcmdldCI6MTB9fV0sWzIsOCwiKHcsdikiLDJdLFswLDksInciLDJdLFsxMCw5LCJcXHRpbGRle2ZfMX0iLDIseyJsYWJlbF9wb3NpdGlvbiI6MjAsImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFsxMiwxMSwiZl8xIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjEwLCJ0YXJnZXQiOjEwfX1dLFs0LDExLCJ3LnEiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzB9XSxbNSwxMiwidi5wIiwyLHsibGFiZWxfcG9zaXRpb24iOjMwfV0sWzcsOSwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNSwxMSwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzEwLDEyLCIiLDIseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksMTEsIns6fXEiLDAseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzcsMTAsIiFfe1xcdGlsZGV7Zl8xfX0iLDIseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbOCwxMCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMywxMiwiezp9cCIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMjUsNTAsNjAsMV1dLFsxLDEzLCJ2IiwyXSxbMTMsMTQsIlxcYmFyIGZfMSIsMix7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTI1LDUwLDYwLDFdXSxbNiwxNCwiIV97XFxiYXJ7Zn19IiwwLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTI1LDUwLDYwLDFdXSxbMSwxNCwiIiwyLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzgsMTQsIiIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzE0LDExLCIiLDAseyJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
	\begin{tikzcd}[column sep=2.5ex, row sep=3.5ex, ampersand replacement=\&]
		\&\&\& {(b,f,a)} \\
		\&\&\& {(b_1,f_1,a_1)} \\
		b \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{f^*(b)} \&\& \textcolor{rgb,255:red,102;green,204;blue,111}{f_*(a)} \&\& a \\
		{b_1} \& {} \& \textcolor{rgb,255:red,220;green,115;blue,86}{f_1^*(b_1)} \&\& \textcolor{rgb,255:red,102;green,204;blue,111}{{f_1}_*(a_1)} \&\& {a_1} \\
		\&\& {b.q} \&\& {a.p} \\
		\&\& {b_1.q} \&\& {a_1.p}
		\arrow["{{:}\liftedX{p}}"', shift right=2, color={rgb,255:red,102;green,204;blue,111}, maps to, from=1-4, to=3-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, maps to, from=1-4, to=3-7]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, maps to, from=3-1, to=5-3]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, maps to, from=3-7, to=5-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=3-5, to=5-3]
		\arrow["{\bar f}"', color={rgb,255:red,102;green,204;blue,111}, dashed, from=3-7, to=3-5]
		\arrow["{\tilde f}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-3, to=3-1]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=3-3, to=5-5]
		\arrow["{{:}p{\between}^{\!*}q}"', color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=1-4, to=3-3]
		\arrow["{{:}q{\between}_{\!*}p}", shift right=2, color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=1-4, to=3-5]
		\arrow["f"', shorten <=7pt, shorten >=7pt, from=5-5, to=5-3]
		\arrow["{(w,v)}"', from=1-4, to=2-4]
		\arrow["w"', from=3-1, to=4-1]
		\arrow["{\tilde{f_1}}"'{pos=0.2}, color={rgb,255:red,220;green,115;blue,86}, dashed, from=4-3, to=4-1]
		\arrow["{f_1}"', shorten <=7pt, shorten >=7pt, from=6-5, to=6-3]
		\arrow["{w.q}"'{pos=0.3}, from=5-3, to=6-3]
		\arrow["{v.p}"'{pos=0.3}, from=5-5, to=6-5]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dotted, from=3-3, to=4-1]
		\arrow[dotted, from=5-5, to=6-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=4-3, to=6-5]
		\arrow["{{:}q}", color={rgb,255:red,220;green,115;blue,86}, maps to, from=4-1, to=6-3]
		\arrow["{!_{\tilde{f_1}}}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-3, to=4-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=2-4, to=4-3]
		\arrow["{{:}p}"', color={rgb,255:red,102;green,204;blue,111}, maps to, from=4-7, to=6-5]
		\arrow["v"', from=3-7, to=4-7]
		\arrow["{\bar f_1}"'{pos=0.2}, color={rgb,255:red,102;green,204;blue,111}, dashed, from=4-7, to=4-5]
		\arrow["{!_{\bar{f}}}", color={rgb,255:red,102;green,204;blue,111}, dashed, from=3-5, to=4-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dotted, from=3-7, to=4-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=2-4, to=4-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=4-5, to=6-3]
	\end{tikzcd}
}




%====== 3)  Institution Definition

\newcommand{\ModSenPB}{\enma{\Modcat\times_{_\Sigcat}\Sencat}}
%--------
\newcommand{\instDefDiamond}{
	% https://q.uiver.app/?q=WzAsMTEsWzMsMl0sWzEsMywiXFxNb2RjYXQiXSxbNSwzLCJcXFNlbmNhdCJdLFszLDUsIlxcU2lnY2F0Il0sWzMsMywiXFxNb2RTZW5QQiIsWzIzNCw3Nyw2MCwxXV0sWzAsMV0sWzIsMl0sWzEsMSwiXFxjb21tYWNhdFlYe3F9e3B9IixbMjI3LDgwLDYwLDFdXSxbNSwxLCJcXG1vZGVscyJdLFsyLDAsIlxcdHdpeER7XFxtb2RlbHN9XioiLFsxMyw2Niw2MCwxXV0sWzQsMCwiXFx0d2l4VXtcXG1vZGVsc31fKiIsWzE2MCw1Niw0NCwxXV0sWzEsMywicSJdLFsyLDMsInAiLDJdLFs0LDEsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDIsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDMsIlxcdGV4dHtbcGJdfSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs3LDEsIlxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6MiwiY29sb3VyIjpbMTYwLDU2LDQ0XX0sWzE2MCw1Niw0NCwxXV0sWzcsMSwicF4qIiwwLHsib2Zmc2V0IjotMiwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzcsMiwicV8qIiwyLHsiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTYwLDU2LDQ0LDFdXSxbNywyLCJcXGxpZnRlZFh7cX0iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6LTMsImNvbG91ciI6WzEzLDY2LDYwXX0sWzEzLDY2LDYwLDFdXSxbNyw0LCIhXioiLDEseyJvZmZzZXQiOjMsInNob3J0ZW4iOnsidGFyZ2V0IjoxMH0sImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFs3LDQsIiFfKiIsMSx7Im9mZnNldCI6LTEsInNob3J0ZW4iOnsic291cmNlIjoxMH0sImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzE2MCw1Niw0NCwxXV0sWzgsMiwiXFxzZW5mdW4iXSxbOCw0LCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOCwxLCJcXG1vZGZ1biIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMH1dLFs5LDcsIiIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksOCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTAsNywiIiwyLHsiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEwLDgsIiIsMix7ImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDEwLCJcXGNvbmciLDEseyJjb2xvdXIiOlszNTcsODcsNDhdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifX19LFszNTcsODcsNDgsMV1dLFs0LDksIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMyw2Niw2MCwxXV0sWzEwLDQsIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTYwLDU2LDQ0LDFdXSxbMiwzLCJcXHRleHR7W29wZl19IiwwLHsib2Zmc2V0IjotMiwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMywiXFx0ZXh0e1tmaWJdfSIsMix7Im9mZnNldCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
	\begin{tikzcd}[ampersand replacement=\&,sep=scriptsize]
		\&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\twixD{\models}^*} \&\& \textcolor{rgb,255:red,49;green,175;blue,133}{\twixU{\models}_*} \\
		{} \& \textcolor{rgb,255:red,71;green,107;blue,235}{\commacatYX{q}{p}} \&\&\&\& \models \\
		\&\& {} \& {} \\
		\& \Modcat \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\ModSenPB} \&\& \Sencat \\
		\\
		\&\&\& \Sigcat
		\arrow["q", from=4-2, to=6-4]
		\arrow["p"', from=4-6, to=6-4]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-2]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-6]
		\arrow["{\text{[pb]}}"{description}, draw=none, from=4-4, to=6-4]
		\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,49;green,175;blue,133}, from=2-2, to=4-2]
		\arrow["{p^*}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, dashed, from=2-2, to=4-2]
		\arrow["{q_*}"', color={rgb,255:red,49;green,175;blue,133}, dashed, from=2-2, to=4-6]
		\arrow["{\liftedX{q}}"{pos=0.3}, shift left=3, color={rgb,255:red,220;green,115;blue,86}, from=2-2, to=4-6]
		\arrow["{!^*}"{description}, shift right=3, color={rgb,255:red,220;green,115;blue,86}, shorten >=9pt, dashed, from=2-2, to=4-4]
		\arrow["{!_*}"{description}, shift left=1, color={rgb,255:red,49;green,175;blue,133}, shorten <=9pt, dashed, from=2-2, to=4-4]
		\arrow["\senfun", from=2-6, to=4-6]
		\arrow[dashed, from=2-6, to=4-4]
		\arrow["\modfun"'{pos=0.3}, from=2-6, to=4-2]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-2]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-6]
		\arrow[draw={rgb,255:red,49;green,175;blue,133}, dashed, from=1-5, to=2-2]
		\arrow[draw={rgb,255:red,49;green,175;blue,133}, dashed, from=1-5, to=2-6]
		\arrow["\cong"{description}, color={rgb,255:red,229;green,16;blue,27}, tail reversed, from=1-3, to=1-5]
		\arrow["{\text{[pb]}}"{description, pos=0.8}, color={rgb,255:red,220;green,115;blue,86}, draw=none, from=4-4, to=1-3]
		\arrow["{\text{[pb]}}"{description, pos=0.2}, color={rgb,255:red,49;green,175;blue,133}, draw=none, from=1-5, to=4-4]
		\arrow["{\text{[opf]}}", shift left=2, draw=none, from=4-6, to=6-4]
		\arrow["{\text{[fib]}}"', shift right=2, draw=none, from=4-2, to=6-4]
	\end{tikzcd} 
}
%
%----

==> diagrams/commaDiagsMacros_copy.tex <==
%		Content
%----
%==  1) commalemma-General 
%		\longOrane
%		\longGreen
%		\commalemmaGeneralDiamond
%		\commalemmaGeneralElementsFull
%
%== 2) commalemma-Special 
%		\commalemmaDiamondSpecial
%		\commalemmaSpecialElementsSmall -- Not Used
%		\commalemmaSpecialElementsFull
%
%=== 3)  Institution Definition
%		\ModSenPB  % for the name of the PB of Mod x Sen
%		\instDefDiamond

%==  1) commalemma-General 
\newcommand{\longOrange}{
	\begin{array}{c}
		\textcolor{rgb,255:red,56;green,188;blue,41}{\tau.w_*}\textcolor{rgb,255:red,220;green,115;blue,86}{.v^*}
		\textcolor{black}{=} \\ [-3.5pt]
		\textcolor{black}{(b_1{,}{(f_*)^*}\!,a_1)}
	\end{array}
}
\newcommand{\longGreen}{
	\begin{array}{c}
		\textcolor{rgb,255:red,220;green,115;blue,86}{\tau.v^*} 
		\textcolor{rgb,255:red,56;green,188;blue,41}{.w_*}	\textcolor{black}{=} \\ [-3.5pt]
		\textcolor{black}{(b_1,(f^*)_*,a_1)}
	\end{array}
}


%------



\newcommand{\commalemmaGeneralDiamond}{
	% https://q.uiver.app/?q=WzAsNCxbMiwwLCJcXGNvbW1hY2F0WVh7cX17cH0iLFsyNDAsNjAsNjAsMV1dLFswLDEsIlxcQkIiXSxbNCwxLCJcXEFBIl0sWzIsMiwiXFxYWCJdLFsxLDMsInEiLDJdLFsyLDMsInAiXSxbMCwyLCJcXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dLFswLDEsIlxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6MiwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjQwLDYwLDYwLDFdXSxbMCwzLCJcXG9kb3QiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwxLCJcXHRleHR7W29wZl19IiwwLHsibGFiZWxfcG9zaXRpb24iOjYwLCJvZmZzZXQiOjMsImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzI0MCw2MCw2MCwxXV0sWzAsMiwiXFx0ZXh0e1tmaWJdfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo2MCwib2Zmc2V0IjotMywic2hvcnRlbiI6eyJzb3VyY2UiOjEwfSwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjQwLDYwLDYwLDFdXSxbNyw2LCJcXHRleHR7W2ZpYnIuc3Bhbl19IiwxLHsibGV2ZWwiOjEsImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjQwLDYwLDYwLDFdXV0=
	\begin{tikzcd}[ampersand replacement=\&,column sep=small,row sep=scriptsize]
		\&\& \textcolor{rgb,255:red,92;green,92;blue,214}{\commacatYX{q}{p}} \\
		\BB \&\&\&\& \AA \\
		\&\& \XX
		\arrow["q"', from=2-1, to=3-3]
		\arrow["p", from=2-5, to=3-3]
		\arrow[""{name=0, anchor=center, inner sep=0}, "{\liftedX{q}}", shift left=2, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-3, to=2-5]
		\arrow[""{name=1, anchor=center, inner sep=0}, "{\liftedX{p}}"', shift right=2, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-3, to=2-1]
		\arrow["\odot"{description}, draw=none, from=1-3, to=3-3]
		\arrow["{\text{[opf]}}"{pos=0.6}, shift right=3, color={rgb,255:red,92;green,92;blue,214}, draw=none, from=1-3, to=2-1]
		\arrow["{\text{[fib]}}"'{pos=0.6}, shift left=3, color={rgb,255:red,92;green,92;blue,214}, draw=none, from=1-3, to=2-5]
		\arrow["{\text{[fibr.span]}}"{description}, color={rgb,255:red,92;green,92;blue,214}, dotted, no head, from=1, to=0]
	\end{tikzcd} 
}
%
%
%--------
\newcommand{\commalemmaGeneralElementsFull}{%row sep=4ex, column sep=2ex,
	% https://q.uiver.app/?q=WzAsMTQsWzAsMywiYl8xIixbMTE2LDU2LDYwLDFdXSxbNiwzLCJhXzEiLFsxMyw2Niw2MCwxXV0sWzEsNF0sWzIsNCwiYi5xIl0sWzQsNCwiYS5wIl0sWzIsNSwiYl8xLnEiXSxbNCw1LCJhXzEucCJdLFszLDAsIlxcdGF1PShiLGYsYSkiXSxbMCwyLCJiIl0sWzIsMiwiXFx0YXUud18qez19KGJfMSxmXyosYSkiLFsxMTQsNjQsNDUsMV1dLFs2LDIsImEiXSxbNCwyLCJcXHRhdS52Xip7PX0oYixmXiosYV8xKSIsWzEzLDY2LDYwLDFdXSxbMiwzLCJcXGxvbmdPcmFuZ2UiLFsxMyw2Niw2MCwxXV0sWzQsMywiXFxsb25nR3JlZW4iLFsxMTIsNjMsNDUsMV1dLFs0LDMsImYiLDJdLFs2LDQsInYucCJdLFszLDUsIncucSIsMl0sWzgsMCwidyIsMix7ImNvbG91ciI6WzExNiw1Niw2MF19LFsxMTYsNTYsNjAsMV1dLFs3LDgsIns6fVxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6Miwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs4LDMsIns6fXEiLDIseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzAsNSwiIiwyLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs3LDksIlxcdGlsZGUgdyIsMix7ImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNiw1Niw2MCwxXV0sWzksMCwiIiwyLHsiY29sb3VyIjpbMTEyLDYzLDQ1XSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNywxMCwiezp9XFxsaWZ0ZWRYe3F9IiwwLHsib2Zmc2V0IjotMiwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxMCw0LCJ7On1wIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxLDEwLCJ2IiwwLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxMyw2Niw2MF19LFsxMyw2Niw2MCwxXV0sWzEsNiwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFsxMSw3LCJcXGJhciB2IiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzExLDEsIiIsMCx7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCw1LCJmXyoiLDIseyJsYWJlbF9wb3NpdGlvbiI6ODAsImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExMiw2Myw0NSwxXV0sWzYsMywiZl4qIiwyLHsibGFiZWxfcG9zaXRpb24iOjIwLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbOSwxMCwiIiwxLHsiY3VydmUiOi00LCJjb2xvdXIiOlsxMTIsNjMsNDVdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMSw4LCIiLDIseyJjdXJ2ZSI6NCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMiw5LCJcXGJhciB2JyIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFsxMiwxLCIiLDEseyJjdXJ2ZSI6LTMsImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTEsMTMsIlxcdGlsZGUgdyciLDIseyJjb2xvdXIiOlsxMTYsNTYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTYsNTYsNjAsMV1dLFsxMywwLCIiLDEseyJjdXJ2ZSI6MywiY29sb3VyIjpbMTEyLDYzLDQ1XSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTMsOSwiIV8qIiwyLHsibGFiZWxfcG9zaXRpb24iOjcwLCJvZmZzZXQiOjEsImNvbG91ciI6WzExMiw2Myw0NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExNiw1Niw2MCwxXV0sWzExLDEyLCIhXioiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6MSwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMyw2Niw2MCwxXV0sWzEzLDEyLCIhXipfKiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6ImFycm93aGVhZCJ9LCJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNiw1LCIoZl8qKV4qez19KHYucCkuZl8qIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzYsNSwiKGZeKilfKns9fWZeKi4ody5xKSIsMCx7Im9mZnNldCI6LTIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dXQ==
	\begin{tikzcd}[ampersand replacement=\&,column sep=tiny,row sep=scriptsize]
		\&\&\& {\tau=(b,f,a)} \\
		\\
		b \&\& \textcolor{rgb,255:red,56;green,188;blue,41}{\tau.w_*{=}(b_1,f_*,a)} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\tau.v^*{=}(b,f^*,a_1)} \&\& a \\
		\textcolor{rgb,255:red,103;green,210;blue,96}{b_1} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\longOrange} \&\& \textcolor{rgb,255:red,62;green,187;blue,42}{\longGreen} \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{a_1} \\
		\& {} \& {b.q} \&\& {a.p} \\
		\&\& {b_1.q} \&\& {a_1.p}
		\arrow["f"', from=5-5, to=5-3]
		\arrow["{v.p}", from=6-5, to=5-5]
		\arrow["{w.q}"', from=5-3, to=6-3]
		\arrow["w"', color={rgb,255:red,103;green,210;blue,96}, from=3-1, to=4-1]
		\arrow["{{:}\liftedX{p}}"', shift right=2, maps to, from=1-4, to=3-1]
		\arrow["{{:}q}"', maps to, from=3-1, to=5-3]
		\arrow[maps to, from=4-1, to=6-3]
		\arrow["{\tilde w}"'{text={rgb,255:red,103;green,210;blue,96}}, draw={rgb,255:red,62;green,187;blue,42}, dashed, from=1-4, to=3-3]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, dashed, maps to, from=3-3, to=4-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, maps to, from=1-4, to=3-7]
		\arrow["{{:}p}", maps to, from=3-7, to=5-5]
		\arrow["v", shift right=2, color={rgb,255:red,220;green,115;blue,86}, from=4-7, to=3-7]
		\arrow[maps to, from=4-7, to=6-5]
		\arrow["{\bar v}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-5, to=1-4]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=3-5, to=4-7]
		\arrow["{f_*}"'{pos=0.8}, color={rgb,255:red,62;green,187;blue,42}, dotted, from=5-5, to=6-3]
		\arrow["{f^*}"'{pos=0.2}, color={rgb,255:red,220;green,115;blue,86}, dotted, from=6-5, to=5-3]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, curve={height=-24pt}, dashed, maps to, from=3-3, to=3-7]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, curve={height=24pt}, dashed, maps to, from=3-5, to=3-1]
		\arrow["{\bar v'}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=4-3, to=3-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, curve={height=-18pt}, dashed, maps to, from=4-3, to=4-7]
		\arrow["{\tilde w'}"', color={rgb,255:red,103;green,210;blue,96}, dashed, from=3-5, to=4-5]
		\arrow[draw={rgb,255:red,62;green,187;blue,42}, curve={height=18pt}, dashed, maps to, from=4-5, to=4-1]
		\arrow["{!_*}"'{pos=0.7, text={rgb,255:red,103;green,210;blue,96}}, shift right=1, draw={rgb,255:red,62;green,187;blue,42}, dotted, from=4-5, to=3-3]
		\arrow["{!^*}"'{pos=0.3}, shift right=1, color={rgb,255:red,220;green,115;blue,86}, dotted, from=3-5, to=4-3]
		\arrow["{!^*_*}", dotted, tail reversed, from=4-5, to=4-3]
		\arrow["{(f_*)^*{=}(v.p).f_*}"', dotted, from=6-5, to=6-3]
		\arrow["{(f^*)_*{=}f^*.(w.q)}", shift left=2, dotted, from=6-5, to=6-3]
	\end{tikzcd}
}

%== 2) commalemma-Special 
\newcommand{\commalemmaDiamondSpecial}{
	%% https://q.uiver.app/?q=WzAsNixbMiwwLCJcXGNvbW1hY2F0WFl7cX17cH0iXSxbMCwxLCJcXEJCIl0sWzQsMSwiXFxBQSJdLFsyLDIsIlxcWFgiXSxbMiwxLCJcXGNpcmMiLFsyMzQsNzcsNjAsMV1dLFsxLDJdLFsxLDMsInEiXSxbMiwzLCJwIiwyXSxbNCwxLCIiLDEseyJjb2xvdXIiOlsyMzQsNzcsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCwyLCIiLDEseyJjb2xvdXIiOlsyMzQsNzcsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCwzLCJcXHRleHR7W3BiXX0iLDEseyJsYWJlbF9wb3NpdGlvbiI6NDAsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDIsIlxcbGlmdGVkWHtxfSIsMCx7Im9mZnNldCI6LTIsImNvbG91ciI6WzEzLDY2LDYwXX0sWzEzLDY2LDYwLDFdXSxbMCwxLCJcXGxpZnRlZFh7cH0iLDIseyJvZmZzZXQiOjIsImNvbG91ciI6WzEwOSw1OSw0NV19LFsxMDksNTksNDUsMV1dLFswLDQsIiEnIiwyLHsib2Zmc2V0IjoxLCJjb2xvdXIiOlsxMDksNTksNDVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMDksNTksNDUsMV1dLFswLDQsIiEiLDAseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMCwxLCJwXioiLDAseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMCwyLCJxXyoiLDIseyJjb2xvdXIiOlsxMDksNTksNDVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMDksNTksNDUsMV1dLFsxLDMsIlxcdGV4dHtbZmliXX0iLDIseyJjb2xvdXIiOlsyLDgxLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMiw4MSw2MCwxXV0sWzIsMywiXFx0ZXh0e1tvcGZdfSIsMCx7ImNvbG91ciI6WzIsODEsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsyLDgxLDYwLDFdXV0=
	\begin{tikzcd}[ampersand replacement=\&,row sep=4ex, column sep=2ex]
		\&\& {\commacatYX{q}{p}} \\
		\BB \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\circ} \&\& \AA \\
		\& {} \& \XX
		\arrow["q", from=2-1, to=3-3]
		\arrow["p"', from=2-5, to=3-3]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=2-3, to=2-1]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=2-3, to=2-5]
		\arrow["{\text{[pb]}}"{description, pos=0.4}, draw=none, from=2-3, to=3-3]
		\arrow["{\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, from=1-3, to=2-5]
		\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,72;green,182;blue,47}, from=1-3, to=2-1]
		\arrow["{!'}"', shift right=1, color={rgb,255:red,72;green,182;blue,47}, dashed, from=1-3, to=2-3]
		\arrow["{!}", shift left=1, color={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-3]
		\arrow["{p^*}", color={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-1]
		\arrow["{q_*}"', color={rgb,255:red,72;green,182;blue,47}, dashed, from=1-3, to=2-5]
		\arrow["{\text{[fib]}}"', color={rgb,255:red,236;green,76;blue,70}, draw=none, from=2-1, to=3-3]
		\arrow["{\text{[opf]}}", color={rgb,255:red,236;green,76;blue,70}, draw=none, from=2-5, to=3-3]
	\end{tikzcd}
}%
%
\newcommand{\commalemmaSpecialElementsSmall}{ %column sep=1.25ex, row sep=2ex
	% https://q.uiver.app/?q=WzAsOCxbMCwxLCJiIl0sWzYsMSwiYSJdLFszLDAsIihiLGYsYSkiXSxbMSwyXSxbMiwyLCJiLnEiXSxbNCwyLCJhLnAiXSxbNCwxLCJmXyooYSkiXSxbMiwxLCJmXiooYikiXSxbMiwwLCJ7On1cXGxpZnRlZFh7cH0iLDIseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19XSxbMiwxLCJ7On1cXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzAsNCwiezp9cSIsMix7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19XSxbMSw1LCJ7On1wIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs2LDQsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsNiwiXFxiYXIgZiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDAsIlxcdGlsZGUgZiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDUsIiIsMSx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzIsNywiezp9cF4qIiwyLHsib2Zmc2V0IjotMiwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMiw2LCJ7On1xXyoiLDAseyJvZmZzZXQiOjIsInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzUsNCwiZiIsMix7InNob3J0ZW4iOnsic291cmNlIjozMCwidGFyZ2V0IjozMH19XV0=
	\begin{tikzcd}[column sep=1.2ex, row sep=2ex, ampersand replacement=\&]
		\&\&\& {(b,f,a)} \\
		b \&\& {f^*(b)} \&\& {f_*(a)} \&\& a \\
		\& {} \& {b.q} \&\& {a.p}
		\arrow["{{:}\liftedX{p}}"', shift right=2, maps to, from=1-4, to=2-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, maps to, from=1-4, to=2-7]
		\arrow["{{:}q}"', maps to, from=2-1, to=3-3]
		\arrow["{{:}p}", maps to, from=2-7, to=3-5]
		\arrow[dashed, maps to, from=2-5, to=3-3]
		\arrow["{\bar f}", dashed, from=2-7, to=2-5]
		\arrow["{\tilde f}", dashed, from=2-3, to=2-1]
		\arrow[dashed, maps to, from=2-3, to=3-5]
		\arrow["{{:}p^*}"', shift left=2, color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=1-4, to=2-3]
		\arrow["{{:}q_*}", shift right=2, dashed, maps to, from=1-4, to=2-5]
		\arrow["f"', shorten <=18pt, shorten >=18pt, from=3-5, to=3-3]
	\end{tikzcd}
}
%
%--------
\newcommand{\commalemmaSpecialElementsFull}{
	% https://q.uiver.app/?q=WzAsMTUsWzAsMiwiYiJdLFs2LDIsImEiXSxbMywwLCIoYixmLGEpIl0sWzEsM10sWzIsNCwiYi5xIl0sWzQsNCwiYS5wIl0sWzQsMiwiZl8qKGEpIixbMTI1LDUwLDYwLDFdXSxbMiwyLCJmXiooYikiLFsxMyw2Niw2MCwxXV0sWzMsMSwiKGJfMSxmXzEsYV8xKSJdLFswLDMsImJfMSJdLFsyLDMsImZfMV4qKGJfMSkiLFsxMyw2Niw2MCwxXV0sWzIsNSwiYl8xLnEiXSxbNCw1LCJhXzEucCJdLFs2LDMsImFfMSJdLFs0LDMsIntmXzF9XyooYV8xKSIsWzEyNSw1MCw2MCwxXV0sWzIsMCwiezp9XFxsaWZ0ZWRYe3B9IiwyLHsib2Zmc2V0IjoyLCJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fSxbMTI1LDUwLDYwLDFdXSxbMiwxLCJ7On1cXGxpZnRlZFh7cX0iLDAseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzAsNCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzEsNSwiIiwwLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFs2LDQsIiIsMCx7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEsNiwiXFxiYXIgZiIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyNSw1MCw2MCwxXV0sWzcsMCwiXFx0aWxkZSBmIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzcsNSwiIiwxLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsyLDcsIns6fXB7XFxiZXR3ZWVufV57XFwhKn1xIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbMiw2LCJ7On1xe1xcYmV0d2Vlbn1fe1xcISp9cCIsMCx7Im9mZnNldCI6MiwiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9LCJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMjUsNTAsNjAsMV1dLFs1LDQsImYiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MTAsInRhcmdldCI6MTB9fV0sWzIsOCwiKHcsdikiLDJdLFswLDksInciLDJdLFsxMCw5LCJcXHRpbGRle2ZfMX0iLDIseyJsYWJlbF9wb3NpdGlvbiI6MjAsImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFsxMiwxMSwiZl8xIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjEwLCJ0YXJnZXQiOjEwfX1dLFs0LDExLCJ3LnEiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzB9XSxbNSwxMiwidi5wIiwyLHsibGFiZWxfcG9zaXRpb24iOjMwfV0sWzcsOSwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNSwxMSwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzEwLDEyLCIiLDIseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksMTEsIns6fXEiLDAseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMyw2Niw2MCwxXV0sWzcsMTAsIiFfe1xcdGlsZGV7Zl8xfX0iLDIseyJjb2xvdXIiOlsxMyw2Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEzLDY2LDYwLDFdXSxbOCwxMCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMywxMiwiezp9cCIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifX19LFsxMjUsNTAsNjAsMV1dLFsxLDEzLCJ2IiwyXSxbMTMsMTQsIlxcYmFyIGZfMSIsMix7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTI1LDUwLDYwLDFdXSxbNiwxNCwiIV97XFxiYXJ7Zn19IiwwLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTI1LDUwLDYwLDFdXSxbMSwxNCwiIiwyLHsiY29sb3VyIjpbMTI1LDUwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzgsMTQsIiIsMix7ImNvbG91ciI6WzEyNSw1MCw2MF0sInN0eWxlIjp7InRhaWwiOnsibmFtZSI6Im1hcHMgdG8ifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzE0LDExLCIiLDAseyJjb2xvdXIiOlsxMjUsNTAsNjBdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn0sImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
	\begin{tikzcd}[column sep=2.5ex, row sep=3.5ex, ampersand replacement=\&]
		\&\&\& {(b,f,a)} \\
		\&\&\& {(b_1,f_1,a_1)} \\
		b \&\& \textcolor{rgb,255:red,220;green,115;blue,86}{f^*(b)} \&\& \textcolor{rgb,255:red,102;green,204;blue,111}{f_*(a)} \&\& a \\
		{b_1} \& {} \& \textcolor{rgb,255:red,220;green,115;blue,86}{f_1^*(b_1)} \&\& \textcolor{rgb,255:red,102;green,204;blue,111}{{f_1}_*(a_1)} \&\& {a_1} \\
		\&\& {b.q} \&\& {a.p} \\
		\&\& {b_1.q} \&\& {a_1.p}
		\arrow["{{:}\liftedX{p}}"', shift right=2, color={rgb,255:red,102;green,204;blue,111}, maps to, from=1-4, to=3-1]
		\arrow["{{:}\liftedX{q}}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, maps to, from=1-4, to=3-7]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, maps to, from=3-1, to=5-3]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, maps to, from=3-7, to=5-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=3-5, to=5-3]
		\arrow["{\bar f}"', color={rgb,255:red,102;green,204;blue,111}, dashed, from=3-7, to=3-5]
		\arrow["{\tilde f}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-3, to=3-1]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=3-3, to=5-5]
		\arrow["{{:}p{\between}^{\!*}q}"', color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=1-4, to=3-3]
		\arrow["{{:}q{\between}_{\!*}p}", shift right=2, color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=1-4, to=3-5]
		\arrow["f"', shorten <=7pt, shorten >=7pt, from=5-5, to=5-3]
		\arrow["{(w,v)}"', from=1-4, to=2-4]
		\arrow["w"', from=3-1, to=4-1]
		\arrow["{\tilde{f_1}}"'{pos=0.2}, color={rgb,255:red,220;green,115;blue,86}, dashed, from=4-3, to=4-1]
		\arrow["{f_1}"', shorten <=7pt, shorten >=7pt, from=6-5, to=6-3]
		\arrow["{w.q}"'{pos=0.3}, from=5-3, to=6-3]
		\arrow["{v.p}"'{pos=0.3}, from=5-5, to=6-5]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dotted, from=3-3, to=4-1]
		\arrow[dotted, from=5-5, to=6-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=4-3, to=6-5]
		\arrow["{{:}q}", color={rgb,255:red,220;green,115;blue,86}, maps to, from=4-1, to=6-3]
		\arrow["{!_{\tilde{f_1}}}"', color={rgb,255:red,220;green,115;blue,86}, dashed, from=3-3, to=4-3]
		\arrow[color={rgb,255:red,220;green,115;blue,86}, dashed, maps to, from=2-4, to=4-3]
		\arrow["{{:}p}"', color={rgb,255:red,102;green,204;blue,111}, maps to, from=4-7, to=6-5]
		\arrow["v"', from=3-7, to=4-7]
		\arrow["{\bar f_1}"'{pos=0.2}, color={rgb,255:red,102;green,204;blue,111}, dashed, from=4-7, to=4-5]
		\arrow["{!_{\bar{f}}}", color={rgb,255:red,102;green,204;blue,111}, dashed, from=3-5, to=4-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dotted, from=3-7, to=4-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=2-4, to=4-5]
		\arrow[color={rgb,255:red,102;green,204;blue,111}, dashed, maps to, from=4-5, to=6-3]
	\end{tikzcd}
}




%====== 3)  Institution Definition

\newcommand{\ModSenPB}{\enma{\Modcat\times_{_\Sigcat}\Sencat}}
%--------
\newcommand{\instDefDiamond}{
	% https://q.uiver.app/?q=WzAsMTEsWzMsMl0sWzEsMywiXFxNb2RjYXQiXSxbNSwzLCJcXFNlbmNhdCJdLFszLDUsIlxcU2lnY2F0Il0sWzMsMywiXFxNb2RTZW5QQiIsWzIzNCw3Nyw2MCwxXV0sWzAsMV0sWzIsMl0sWzEsMSwiXFxjb21tYWNhdFlYe3F9e3B9IixbMjI3LDgwLDYwLDFdXSxbNSwxLCJcXG1vZGVscyJdLFsyLDAsIlxcdHdpeER7XFxtb2RlbHN9XioiLFsxMyw2Niw2MCwxXV0sWzQsMCwiXFx0d2l4VXtcXG1vZGVsc31fKiIsWzE2MCw1Niw0NCwxXV0sWzEsMywicSJdLFsyLDMsInAiLDJdLFs0LDEsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDIsIiIsMSx7ImNvbG91ciI6WzIzNCw3Nyw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDMsIlxcdGV4dHtbcGJdfSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs3LDEsIlxcbGlmdGVkWHtwfSIsMix7Im9mZnNldCI6MiwiY29sb3VyIjpbMTYwLDU2LDQ0XX0sWzE2MCw1Niw0NCwxXV0sWzcsMSwicF4qIiwwLHsib2Zmc2V0IjotMiwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMyw2Niw2MCwxXV0sWzcsMiwicV8qIiwyLHsiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTYwLDU2LDQ0LDFdXSxbNywyLCJcXGxpZnRlZFh7cX0iLDAseyJsYWJlbF9wb3NpdGlvbiI6MzAsIm9mZnNldCI6LTMsImNvbG91ciI6WzEzLDY2LDYwXX0sWzEzLDY2LDYwLDFdXSxbNyw0LCIhXioiLDEseyJvZmZzZXQiOjMsInNob3J0ZW4iOnsidGFyZ2V0IjoxMH0sImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTMsNjYsNjAsMV1dLFs3LDQsIiFfKiIsMSx7Im9mZnNldCI6LTEsInNob3J0ZW4iOnsic291cmNlIjoxMH0sImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzE2MCw1Niw0NCwxXV0sWzgsMiwiXFxzZW5mdW4iXSxbOCw0LCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOCwxLCJcXG1vZGZ1biIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMH1dLFs5LDcsIiIsMix7ImNvbG91ciI6WzEzLDY2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksOCwiIiwyLHsiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTAsNywiIiwyLHsiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEwLDgsIiIsMix7ImNvbG91ciI6WzE2MCw1Niw0NF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDEwLCJcXGNvbmciLDEseyJjb2xvdXIiOlszNTcsODcsNDhdLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifX19LFszNTcsODcsNDgsMV1dLFs0LDksIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY29sb3VyIjpbMTMsNjYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMyw2Niw2MCwxXV0sWzEwLDQsIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjoyMCwiY29sb3VyIjpbMTYwLDU2LDQ0XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTYwLDU2LDQ0LDFdXSxbMiwzLCJcXHRleHR7W29wZl19IiwwLHsib2Zmc2V0IjotMiwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMywiXFx0ZXh0e1tmaWJdfSIsMix7Im9mZnNldCI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
	\begin{tikzcd}[ampersand replacement=\&,sep=scriptsize]
		\&\& \textcolor{rgb,255:red,220;green,115;blue,86}{\twixD{\models}^*} \&\& \textcolor{rgb,255:red,49;green,175;blue,133}{\twixU{\models}_*} \\
		{} \& \textcolor{rgb,255:red,71;green,107;blue,235}{\commacatYX{q}{p}} \&\&\&\& \models \\
		\&\& {} \& {} \\
		\& \Modcat \&\& \textcolor{rgb,255:red,74;green,90;blue,232}{\ModSenPB} \&\& \Sencat \\
		\\
		\&\&\& \Sigcat
		\arrow["q", from=4-2, to=6-4]
		\arrow["p"', from=4-6, to=6-4]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-2]
		\arrow[draw={rgb,255:red,74;green,90;blue,232}, dashed, from=4-4, to=4-6]
		\arrow["{\text{[pb]}}"{description}, draw=none, from=4-4, to=6-4]
		\arrow["{\liftedX{p}}"', shift right=2, color={rgb,255:red,49;green,175;blue,133}, from=2-2, to=4-2]
		\arrow["{p^*}", shift left=2, color={rgb,255:red,220;green,115;blue,86}, dashed, from=2-2, to=4-2]
		\arrow["{q_*}"', color={rgb,255:red,49;green,175;blue,133}, dashed, from=2-2, to=4-6]
		\arrow["{\liftedX{q}}"{pos=0.3}, shift left=3, color={rgb,255:red,220;green,115;blue,86}, from=2-2, to=4-6]
		\arrow["{!^*}"{description}, shift right=3, color={rgb,255:red,220;green,115;blue,86}, shorten >=9pt, dashed, from=2-2, to=4-4]
		\arrow["{!_*}"{description}, shift left=1, color={rgb,255:red,49;green,175;blue,133}, shorten <=9pt, dashed, from=2-2, to=4-4]
		\arrow["\senfun", from=2-6, to=4-6]
		\arrow[dashed, from=2-6, to=4-4]
		\arrow["\modfun"'{pos=0.3}, from=2-6, to=4-2]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-2]
		\arrow[draw={rgb,255:red,220;green,115;blue,86}, dashed, from=1-3, to=2-6]
		\arrow[draw={rgb,255:red,49;green,175;blue,133}, dashed, from=1-5, to=2-2]
		\arrow[draw={rgb,255:red,49;green,175;blue,133}, dashed, from=1-5, to=2-6]
		\arrow["\cong"{description}, color={rgb,255:red,229;green,16;blue,27}, tail reversed, from=1-3, to=1-5]
		\arrow["{\text{[pb]}}"{description, pos=0.8}, color={rgb,255:red,220;green,115;blue,86}, draw=none, from=4-4, to=1-3]
		\arrow["{\text{[pb]}}"{description, pos=0.2}, color={rgb,255:red,49;green,175;blue,133}, draw=none, from=1-5, to=4-4]
		\arrow["{\text{[opf]}}", shift left=2, draw=none, from=4-6, to=6-4]
		\arrow["{\text{[fib]}}"', shift right=2, draw=none, from=4-2, to=6-4]
	\end{tikzcd} 
}
%
%----

==> diagrams/commalemma-GenSpec.tex <==
\begin{figure}[h]
\begin{tabular}{c@{\vspace{2ex}}c}
\begin{tabular}{c}
			\commalemmaGeneralDiamond
	\\ 	[5pt] 
	a)
	\\ [10pt]   
			\commalemmaSpecialDiamond
	\\  [5pt] 
	b)
\end{tabular}
& %\multirow{2}{*}{\commaLemmaElementsArrows}
\begin{tabular}{c}
			\commalemmaSpecialElementsFull
\\ [5pt] 
b')
\end{tabular}
\end{tabular}
\caption{Comma categories and fibred spans}
\label{figdiag:commaCats}
\end{figure}

==> diagrams/commalemma-General.tex <==

\begin{equation}\label{eqdiag:commalemma-GeneralDiamond}
\begin{tabular}{cc}
	\commalemmaGeneralDiamond
	& 	\commalemmaGeneralElementsFull
\end{tabular}
\end{equation}

\endinput 


==> diagrams/commalemma-Special.tex <==


%-------
\begin{equation}\label{eqdiag:commalemma-Special}
\begin{tabular}{l@{\;\;}l}
	\commalemmaDiamondSpecial
	& \commalemmaSpecialElementsFull
\end{tabular}
\end{equation}




\endinput



==> diagrams/esatDefnoProd--macros.tex <==
%\begin{mygroup}
%[row sep=2ex, column sep= 2ex ]
%[row sep=2ex,  ]
% modifications made: 
% [-15pt]  in \\ [-15pt] row  2 before \twix{P}
% [-15pt]  in \\ [15pt] row  3 after \twix{P}
% shorten >= -1 mm,shorten <= -2 mm for arrow f_*
% shorten >= -1.5mm fro arrow f^*
% 
% 
\newcommand{\satAxiomWithVerviaOk}{
% https://q.uiver.app/#q=WzAsMTIsWzAsMl0sWzEsMCwiTSIsWzAsNjAsNjAsMV1dLFsyLDAsIlxcUG9iaiJdLFsxLDEsIlMiLFswLDYwLDYwLDFdXSxbMiwyLCJcXHR3aXh7UH0iXSxbMSwzLCJNJyIsWzEyMCw2MCw0MCwxXV0sWzEsNCwiUyciLFsxMjAsNjAsNDAsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMjAsNjAsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFswLDYwLDYwLDFdXSxbMyw0LCJcXERhc2h2JyIsWzEyMCw2MCw0MCwxXV0sWzUsMiwiXFxWZXJPYmoiXSxbNiwyLCJcXG9rT2JqIixbMCw2MCw2MCwxXV0sWzIsMywiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19XSxbMiwxLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs3LDUsIiIsMCx7ImNvbG91ciI6WzEyMCw2MCw0MF19XSxbNyw2LCIiLDAseyJjb2xvdXIiOlsxMjAsNjAsNDBdfV0sWzgsMiwidSIsMix7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSw3LCJ1JyIsMCx7ImNvbG91ciI6WzEyMCw2MCw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MCwxXV0sWzQsNywiISciLDIseyJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dLFs0LDIsIiEiLDAseyJjb2xvdXIiOlsyNDksODAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDksODAsNjAsMV1dLFsxLDUsImZeKiIsMix7ImN1cnZlIjozLCJjb2xvdXIiOls2LDkwLDYwXX0sWzYsOTAsNjAsMV1dLFs2LDMsImZfKiIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbNiw5MCw2MF19LFs2LDkwLDYwLDFdXSxbMTEsMTBdLFs0LDVdLFs0LDNdLFs4LDExLCJcXHZlciIsMCx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSwxMSwiXFx2ZXInIiwyLHsiY29sb3VyIjpbMTIwLDYwLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTIwLDYwLDQwLDFdXSxbNCwxMCwiXFx0d2l4e1xcdmVyfSIsMCx7ImN1cnZlIjotMn1dLFsyLDEwLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs3LDEwLCIiLDAseyJjb2xvdXIiOlsxMjAsNjAsNDBdfV0sWzQsMTAsIlxcdHdpc3RlZFNhdFhkbntmfSIsMSx7ImN1cnZlIjoyLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \& \Pobj \& \textcolor{rgb,255:red,214;green,92;blue,92}{\Dashv} \\
	\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
	{} \&\& {\twix{P}} \&\&\& \VerObj \& \textcolor{rgb,255:red,214;green,92;blue,92}{\okObj} \\
	\& \textcolor{rgb,255:red,41;green,163;blue,41}{M'} \\
	\& \textcolor{rgb,255:red,41;green,163;blue,41}{S'} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\PobjPrim} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\Dashv'}
	\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=2-2]
	\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=1-2]
	\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=4-2]
	\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=5-2]
	\arrow["u"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=1-4, to=1-3]
	\arrow["{u'}", color={rgb,255:red,41;green,163;blue,41}, dashed, from=5-4, to=5-3]
	\arrow["{!'}"', color={rgb,255:red,92;green,92;blue,214}, dashed, from=3-3, to=5-3]
	\arrow["{!}", color={rgb,255:red,96;green,71;blue,235}, dashed, from=3-3, to=1-3]
	\arrow["{f^*}"', color={rgb,255:red,245;green,80;blue,61}, curve={height=18pt}, from=1-2, to=4-2]
	\arrow["{f_*}", color={rgb,255:red,245;green,80;blue,61}, curve={height=-18pt}, from=5-2, to=2-2]
	\arrow[from=3-7, to=3-6]
	\arrow[from=3-3, to=4-2]
	\arrow[from=3-3, to=2-2]
	\arrow["\ver", color={rgb,255:red,214;green,92;blue,92}, dashed, from=1-4, to=3-7]
	\arrow["{\ver'}"', color={rgb,255:red,41;green,163;blue,41}, dashed, from=5-4, to=3-7]
	\arrow["{\twix{\ver}}", curve={height=-12pt}, from=3-3, to=3-6]
	\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=3-6]
	\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=3-6]
	\arrow["{\twistedSatXdn{f}}"{description}, curve={height=12pt}, tail reversed, from=3-3, to=3-6]
\end{tikzcd}
}

\newcommand{\twistedMorphDefMain}{
% https://q.uiver.app/#q=WzAsOCxbMCwwLCJNIixbMTIsNjMsNTIsMV1dLFswLDEsIlMiLFsxMiw2Myw1MiwxXV0sWzAsMywiTSciLFsxMTUsNzMsNDAsMV1dLFswLDQsIlMnIixbMTE1LDczLDQzLDFdXSxbMSwwLCJcXHZEYXNoIixbMTIsNjMsNTIsMV1dLFsxLDIsIlxcdHdpeFV7XFx2RGFzaH1fZiJdLFsxLDQsIlxcdkRhc2gnIixbMTE1LDczLDQwLDFdXSxbMywyLCJFIl0sWzUsNCwiXFxzYXRUb1NhdFVwWHtmfSIsMix7ImN1cnZlIjotMSwiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzAsNjAsNjAsMV1dLFs1LDYsIlxcc2F0VG9TYXREblh7Zn0iLDAseyJjdXJ2ZSI6MSwiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbNCw3LCJxIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs2LDcsInEnIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzIsMCwiZl4qIiwwLHsiY3VydmUiOi0zfV0sWzEsMywiZl8qIiwyLHsiY3VydmUiOjN9XSxbNSw3LCJxX2YiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCwxLCIiLDIseyJjb2xvdXIiOlsxMiw2Myw1Ml19XSxbNCwwLCJwX00iLDIseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFswLDYwLDYwLDFdXSxbNiwyLCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzYsMywicF97Uyd9IiwwLHsiY29sb3VyIjpbMTE1LDczLDQzXX0sWzExNSw3Myw0MCwxXV0sWzUsMSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzUsMiwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTksOSwiIiwwLHsiY3VydmUiOjEsImxldmVsIjoxLCJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJzcXVpZ2dseSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIwLDgsIiIsMCx7ImN1cnZlIjotMSwibGV2ZWwiOjEsImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJzcXVpZ2dseSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\vDash} \\
	\textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
	\& {\twixU{\vDash}_f} \&\& E \\
	\textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
	\textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\vDash'}
	\arrow[""{name=0, anchor=center, inner sep=0}, "{\satToSatUpX{f}}"', color={rgb,255:red,214;green,92;blue,92}, curve={height=-6pt}, dashed, from=3-2, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\satToSatDnX{f}}", color={rgb,255:red,40;green,176;blue,28}, curve={height=6pt}, dashed, from=3-2, to=5-2]
	\arrow["q", color={rgb,255:red,210;green,86;blue,55}, from=1-2, to=3-4]
	\arrow["{q'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-2, to=3-4]
	\arrow["{f^*}", curve={height=-18pt}, from=4-1, to=1-1]
	\arrow["{f_*}"', curve={height=18pt}, from=2-1, to=5-1]
	\arrow["{q_f}", dashed, from=3-2, to=3-4]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-2, to=2-1]
	\arrow["{p_M}"'{text={rgb,255:red,214;green,92;blue,92}}, draw={rgb,255:red,210;green,86;blue,55}, from=1-2, to=1-1]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-2, to=4-1]
	\arrow["{p_{S'}}"{text={rgb,255:red,40;green,176;blue,28}}, draw={rgb,255:red,43;green,190;blue,30}, from=5-2, to=5-1]
	\arrow[""{name=2, anchor=center, inner sep=0}, draw={rgb,255:red,40;green,176;blue,28}, dashed, from=3-2, to=2-1]
	\arrow[""{name=3, anchor=center, inner sep=0}, draw={rgb,255:red,210;green,86;blue,55}, dashed, from=3-2, to=4-1]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, curve={height=6pt}, squiggly, no head, from=2, to=1]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, curve={height=-6pt}, squiggly, no head, from=3, to=0]
\end{tikzcd}
}

\newcommand{\twistedMorphDefPacked}{ % uses products !!
% https://q.uiver.app/#q=WzAsNCxbMCwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzAsMiwiXFx0d2l4VXtQfSJdLFswLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDIsIkUiXSxbMSwwLCIoZl4qLDEpIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19LFswLDYwLDYwLDFdXSxbMSwyLCIoMSxmXyopIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzAsMywiXFx2RGFzaCIsMCx7ImNvbG91ciI6WzEyLDYzLDUyXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fSxbMTIsNjMsNTIsMV1dLFsyLDMsIlxcdkRhc2gnIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzEsMywiXFx0d2lzdGVkU2F0WGRue2Z9IiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \\
	\\
	{\twixU{P}} \&\&\& E \\
	\\
	\textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim}
	\arrow["{(f^*,1)}", color={rgb,255:red,214;green,92;blue,92}, from=3-1, to=1-1]
	\arrow["{(1,f_*)}"', color={rgb,255:red,40;green,176;blue,28}, from=3-1, to=5-1]
	\arrow["\vDash", "\shortmid"{marking, text={rgb,255:red,210;green,86;blue,55}}, color={rgb,255:red,210;green,86;blue,55}, from=1-1, to=3-4]
	\arrow["{\vDash'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-1, to=3-4]
	\arrow["{\twistedSatXdn{f}}"{description}, dashed, from=3-1, to=3-4]
\end{tikzcd}
}

\newcommand{\satAxiomPacked}{
	% https://q.uiver.app/#q=WzAsNixbMCwyLCJNJyIsWzI0NywzOSw3NSwxXV0sWzEsMCwiTSIsWzAsNjAsNjAsMV1dLFsxLDMsIk0nIixbMTE1LDczLDQzLDFdXSxbMywwLCJTIixbMCw2MCw2MCwxXV0sWzMsMywiUyciLFsxMTUsNzMsNDAsMV1dLFs0LDEsIlMiLFsyNDcsMzksNzUsMV1dLFswLDEsImZeKiIsMCx7ImNvbG91ciI6WzI0NywzOSw3NV19XSxbMCwyLCIiLDIseyJsZXZlbCI6MiwiY29sb3VyIjpbMjQ3LDM5LDc1XSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDIsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFszLDEsIlxcdkRhc2hfe01TfSIsMix7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19LFswLDYwLDYwLDFdXSxbNCwyLCJcXHZEYXNoX3tNJ1MnfSIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFszLDUsIiIsMCx7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsNCwiZl8qIiwwLHsiY29sb3VyIjpbMjQ3LDM5LDc1XX1dLFszLDQsImZfeyoqfSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFszLDIsIlxcdkRhc2hfe00nU31eZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
	\begin{tikzcd}[ampersand replacement=\&,sep=small]
		\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
		\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
		\textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
		\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'}
		\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=3-1, to=1-2]
		\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=3-1, to=4-2]
		\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-2, to=4-2]
		\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-4, to=1-2]
		\arrow["{\vDash_{M'S'}}", color={rgb,255:red,40;green,176;blue,28}, from=4-4, to=4-2]
		\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-4, to=2-5]
		\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-5, to=4-4]
		\arrow["{f_{**}}", "\shortmid"{marking}, from=1-4, to=4-4]
		\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-4, to=4-2]
	\end{tikzcd}
}

%=== PREVIOUS VERSIONS 

\newcommand{\vsatDefTripleDiagram}{
% https://q.uiver.app/#q=WzAsMjUsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs1LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbMTEsMCwiUCJdLFsxMywyLCJFIl0sWzExLDQsIlAnIl0sWzgsNSwiXFx0ZXh0e2EpfSJdLFsxMSw1LCJcXHRleHR7Yil9Il0sWzExLDIsIlxcdHdpeFV7UH1fZiJdLFszLDUsIlxcdGV4dHsqKX0gIl0sWzIsMywiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzIsMSwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzcsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFs3LDYsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0M119XSxbOCwyLCJyIiwyLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs5LDQsInJfZiIsMl0sWzEwLDcsInInIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksOCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksMTAsIlxcc2F0VG9TYXRfKl5mIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMCw2MCw2MCwxXV0sWzQsMTAsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzExNSw3Myw0MCwxXV0sWzgsMTEsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzEwLDExLCJlJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzksMTEsImVfZiJdLFs0LDMsIiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfV0sWzQsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFsxMiwxMywiZl4qIiwwLHsiY29sb3VyIjpbMjQ3LDM5LDc1XX1dLFsxMiwxNCwiIiwyLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTQsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxMywiXFx2RGFzaF97TVN9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX0sWzAsNjAsNjAsMV1dLFsxNiwxNCwiXFx2RGFzaF97TSdTJ30iLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMTUsMTcsIiIsMCx7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDE2LCJmXyoiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzE1LDE2LCJmX3sqKn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTUsMTQsIlxcdkRhc2hfe00nU31eZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxOCwxOSwiXFx2RGFzaCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMCwxOSwiXFx2RGFzaCciLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMjMsMTgsIiFfKl5mIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIzLDIwLCIhXypeZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMywxOSwiXFx0d2lzdGVkU2F0WGRue2Z9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dXQ==
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \&\&\&\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \&\& P \\
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \&\&\&\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
	{} \&\& {\twixU{P}_f} \& {\twistedSatXdn{f}} \&\& E \&\&\&\&\&\& {\twixU{P}_f} \&\& E \\
	\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
	\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'} \&\&\&\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'} \&\& {P'} \\
	\&\&\& {\text{*)} } \&\&\&\&\& {\text{a)}} \&\&\& {\text{b)}}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
	\arrow[draw={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
	\arrow["r"', color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=1-3]
	\arrow["{r_f}"', from=3-4, to=3-3]
	\arrow["{r'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=5-3]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
	\arrow["{\satToSat^*_f}"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-4, to=1-4]
	\arrow["{\satToSat_*^f}", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-4, to=5-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-4]
	\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=3-6]
	\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=3-6]
	\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
	\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
	\arrow["{e_f}", from=3-4, to=3-6]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=4-7, to=1-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=4-7, to=5-8]
	\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-8, to=5-8]
	\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-10, to=1-8]
	\arrow["{\vDash_{M'S'}}", color={rgb,255:red,40;green,176;blue,28}, from=5-10, to=5-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-10, to=2-11]
	\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-11, to=5-10]
	\arrow["{f_{**}}", "\shortmid"{marking}, from=1-10, to=5-10]
	\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-10, to=5-8]
	\arrow["\vDash", "\shortmid"{marking}, from=1-12, to=3-14]
	\arrow["{\vDash'}"', "\shortmid"{marking}, from=5-12, to=3-14]
	\arrow["{!_*^f}", "\shortmid"{marking}, from=3-12, to=1-12]
	\arrow["{!_*^f}"', "\shortmid"{marking}, from=3-12, to=5-12]
	\arrow["{\twistedSatXdn{f}}", "\shortmid"{marking}, from=3-12, to=3-14]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
\end{tikzcd}
}


\newcommand{\vsatDefMainDiag}{
% https://q.uiver.app/#q=WzAsOSxbMCwyXSxbMSwwLCJNIixbMTIsNjMsNTIsMV1dLFsyLDAsIlxcUG9iaiIsWzEyLDYzLDUyLDFdXSxbMSwxLCJTIixbMTIsNjMsNTIsMV1dLFsyLDIsIlxcdHdpeFV7UH1fZiJdLFsxLDMsIk0nIixbMTE1LDczLDQwLDFdXSxbMSw0LCJTJyIsWzExNSw3Myw0MywxXV0sWzIsNCwiXFxQb2JqUHJpbSIsWzExNSw3Myw0MCwxXV0sWzUsMiwiRSJdLFsyLDMsIiIsMCx7ImNvbG91ciI6WzEyLDYzLDUyXX1dLFsyLDEsIiIsMCx7ImNvbG91ciI6WzEyLDYzLDUyXX1dLFs3LDUsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19XSxbNyw2LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDNdfV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXX0sWzAsNjAsNjAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzQsMywiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19XSxbNCw1LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMiw4LCJcXHZEYXNoIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19LFsxMiw2Myw1MiwxXV0sWzcsOCwiXFx2RGFzaCciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHR3aXN0ZWRTYXRYZG57Zn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \\
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
	{} \&\& {\twixU{P}_f} \&\&\& E \\
	\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
	\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
	\arrow[draw={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, from=3-3, to=1-3]
	\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
	\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, from=3-3, to=5-3]
	\arrow["\vDash", "\shortmid"{marking, text={rgb,255:red,210;green,86;blue,55}}, color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=3-6]
	\arrow["{\vDash'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-3, to=3-6]
	\arrow["{\twistedSatXdn{f}}", "\shortmid"{marking}, from=3-3, to=3-6]
\end{tikzcd}
}


\newcommand{\vsatDefMainDiagUnpacked}{
% https://q.uiver.app/#q=WzAsMTYsWzAsMl0sWzIsMCwiXFxQb2JqIixbMTIsNjMsNTIsMV1dLFsyLDIsIlxcdHdpeFV7UH1fZiJdLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs0LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbOCw1LCJcXHRleHR7aWkpfSJdLFszLDUsIlxcdGV4dHtpKX0gIl0sWzQsMSwicCIsMix7ImNvbG91ciI6WzEyLDYzLDUyXX0sWzEyLDYzLDUyLDFdXSxbNSwyLCJcXHR3aXhVe3B9X2YiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNiwzLCJwJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFsyLDMsIiFfKl5mIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbMiwxLCIhXipfZiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzUsNCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzUsNiwiXFxzYXRUb1NhdF8qXmYiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dLFsyLDQsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFswLDYwLDYwLDFdXSxbMiw2LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMTUsNzMsNDAsMV1dLFs0LDcsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzYsNywiZSciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNSw3LCJcXHR3aXhVe2V9X2YiXSxbOCw5LCJmXioiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzgsMTAsIiIsMix7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMTAsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMSw5LCJcXHZEYXNoX3tNU30iLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fSxbMCw2MCw2MCwxXV0sWzEyLDEwLCJcXHZEYXNoX3tNJ1MnfSIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFsxMSwxMywiIiwwLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTIsImZfKiIsMCx7ImNvbG91ciI6WzI0NywzOSw3NV19XSxbMTEsMTIsImZfeyoqfSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMSwxMCwiXFx2RGFzaF97TSdTfV5mIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\&\& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \&\&\&\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
	\&\&\&\&\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
	{} \&\& {\twixU{P}_f} \& {\twistedSatXdn{f}} \& E \\
	\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
	\&\& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'} \&\&\&\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'} \\
	\&\&\& {\text{i)} } \&\&\&\&\& {\text{ii)}}
	\arrow["p"', color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=1-3]
	\arrow["{\twixU{p}_f}"', dashed, from=3-4, to=3-3]
	\arrow["{p'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=5-3]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, from=3-3, to=1-3]
	\arrow["{\satToSat^*_f}"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-4, to=1-4]
	\arrow["{\satToSat_*^f}", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-4, to=5-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-4]
	\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=3-5]
	\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=3-5]
	\arrow["{\twixU{e}_f}", from=3-4, to=3-5]
	\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=4-7, to=1-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=4-7, to=5-8]
	\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-8, to=5-8]
	\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-10, to=1-8]
	\arrow["{\vDash_{M'S'}}", color={rgb,255:red,40;green,176;blue,28}, from=5-10, to=5-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-10, to=2-11]
	\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-11, to=5-10]
	\arrow["{f_{**}}", "\shortmid"{marking}, from=1-10, to=5-10]
	\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-10, to=5-8]
\end{tikzcd}
}

\newcommand{\satAxiomWithVer}{
	% https://q.uiver.app/#q=WzAsMTIsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFs0LDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzQsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzQsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs2LDIsIkUiXSxbMiwzLCIiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19XSxbMiwxLCIiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19XSxbNyw1LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzcsNiwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQzXX1dLFs4LDIsInAiLDIseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzksNCwiXFx0d2l4VXtwfV9mIiwyXSxbMTAsNywicCciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNCw3LCIhJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiISIsMCx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSw4LCJcXHNhdFRvU2F0IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzAsNjAsNjAsMV1dLFs5LDEwLCJcXHNhdFRvU2F0UHJpbSIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNSw3Myw0MCwxXV0sWzQsOCwiXFx0ZXh0e1twYl19IiwxLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzAsNjAsNjAsMV1dLFs0LDEwLCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMTUsNzMsNDAsMV1dLFs4LDExLCJlIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFsxMCwxMSwiZSciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNSwxLCJmXioiLDAseyJjdXJ2ZSI6LTN9XSxbMyw2LCJmXyoiLDIseyJjdXJ2ZSI6M31dLFs5LDExLCJcXHR3aXhVe2V9X2YiXSxbNCwzLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs0LDUsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19XV0=
	\begin{tikzcd}[ampersand replacement=\&,sep=small]
		\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \&\& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \\
		\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
		{} \&\& {\twixU{P}_f} \&\& {\twistedSatXdn{f}} \&\& E \\
		\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
		\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'}
		\arrow[color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
		\arrow[color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
		\arrow[color={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
		\arrow[color={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
		\arrow["p"', color={rgb,255:red,210;green,86;blue,55}, from=1-5, to=1-3]
		\arrow["{\twixU{p}_f}"', from=3-5, to=3-3]
		\arrow["{p'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-5, to=5-3]
		\arrow["{!'}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
		\arrow["{!}", color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
		\arrow["\satToSat"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-5, to=1-5]
		\arrow["\satToSatPrim", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-5, to=5-5]
		\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-5]
		\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-5]
		\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-5, to=3-7]
		\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-5, to=3-7]
		\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
		\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
		\arrow["{\twixU{e}_f}", from=3-5, to=3-7]
		\arrow[color={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
		\arrow[color={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\end{tikzcd}
}


\endinput


%
% URL s of useful quiver diags
%
%-->   \vsatDefTripleDiagram
% https://q.uiver.app/#q=WzAsMjUsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs1LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbMTEsMCwiUCJdLFsxMywyLCJFIl0sWzExLDQsIlAnIl0sWzgsNSwiXFx0ZXh0e2EpfSJdLFsxMSw1LCJcXHRleHR7Yil9Il0sWzExLDIsIlxcdHdpeFV7UH1fZiJdLFszLDUsIlxcdGV4dHsqKX0gIl0sWzIsMywiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzIsMSwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzcsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFs3LDYsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0M119XSxbOCwyLCJyIiwyLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs5LDQsInJfZiIsMl0sWzEwLDcsInInIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksOCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksMTAsIlxcc2F0VG9TYXRfKl5mIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMCw2MCw2MCwxXV0sWzQsMTAsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzExNSw3Myw0MCwxXV0sWzgsMTEsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzEwLDExLCJlJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzksMTEsImVfZiJdLFs0LDMsIiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfV0sWzQsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFsxMiwxMywiZl4qIiwwLHsiY29sb3VyIjpbMjQ3LDM5LDc1XX1dLFsxMiwxNCwiIiwyLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTQsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxMywiXFx2RGFzaF97TVN9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX0sWzAsNjAsNjAsMV1dLFsxNiwxNCwiXFx2RGFzaF97TSdTJ30iLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMTUsMTcsIiIsMCx7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDE2LCJmXyoiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzE1LDE2LCJmX3sqKn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTUsMTQsIlxcdkRhc2hfe00nU31eZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxOCwxOSwiXFx2RGFzaCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMCwxOSwiXFx2RGFzaCciLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMjMsMTgsIiFfKl5mIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIzLDIwLCIhXypeZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMywxOSwiXFx0d2lzdGVkU2F0WGRue2Z9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dXQ==

========
%-->  unknown   https://q.uiver.app/?q=WzAsMTQsWzEsMl0sWzIsMCwiTSJdLFszLDAsIlAiXSxbMiwxLCJTIl0sWzMsMiwiXFx0d2l4e1B9Il0sWzIsMywiTSciXSxbMiw0LCJTJyJdLFszLDQsIlAnIl0sWzQsMCwiXFxEYXNodiJdLFs0LDIsIlxcdHdpeHtcXERhc2h2fV5mIl0sWzQsNCwiXFxEYXNodiciXSxbNSwyLCJWIl0sWzAsMCwiXFxEYXNodl9WIl0sWzAsNCwiXFxEYXNodidfViJdLFsyLDNdLFsyLDFdLFs3LDVdLFs3LDZdLFs0LDFdLFs0LDZdLFs4LDIsInUiLDJdLFs5LDQsIlxcdHdpeHt1fSIsMix7ImNvbG91ciI6WzYsOTAsNjBdfSxbNiw5MCw2MCwxXV0sWzEwLDcsInUnIiwyXSxbNCw3LCIhJyIsMix7ImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0MCw2MCw2MCwxXV0sWzQsMiwiISIsMCx7ImNvbG91ciI6WzI0OSw4MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0OSw4MCw2MCwxXV0sWzksOCwiXFxiYXIgISIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDEwLCJcXGJhcnshJ30iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCw4LCJbcGJdIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsMTAsIltwYl0iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwxMSwidiJdLFsxMCwxMSwidiciLDJdLFsxLDUsImZeKiIsMix7ImN1cnZlIjozLCJjb2xvdXIiOls2LDkwLDYwXX0sWzYsOTAsNjAsMV1dLFs2LDMsImZfKiIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbNiw5MCw2MF19LFs2LDkwLDYwLDFdXSxbOSwxMSwiIiwyLHsiY29sb3VyIjpbNiw5MCw2MF19XSxbOSw0LCJcXGJhciB1ID0gXFxiYXJ7dSd9IiwxLHsibGFiZWxfcG9zaXRpb24iOjYwLCJvZmZzZXQiOjIsImN1cnZlIjotMiwiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzAsNjAsNjAsMV1dLFsxMywxMiwiZiIsMV1d


==> diagrams/esatDefwithProd--macros.tex <==
%\begin{mygroup}
%[row sep=2ex, column sep= 2ex ]
%[row sep=2ex,  ]
% modifications made: 
% [-15pt]  in \\ [-15pt] row  2 before \twix{P}
% [-15pt]  in \\ [15pt] row  3 after \twix{P}
% shorten >= -1 mm,shorten <= -2 mm for arrow f_*
% shorten >= -1.5mm fro arrow f^*
% 
% 
%\renewcommand{\Pobj}{\enma{P}}
%\renewcommand{\PobjPrim}{\enma{P'}}
%\renewcommand{\satToSat}{\enma{\rho}}


\newcommand{\twistedMorphDefMain}{
% https://q.uiver.app/#q=WzAsMTEsWzAsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMSwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzAsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMSwyLCJcXHR3aXhVe1B9Il0sWzAsMywiTSciLFsxMTUsNzMsNDAsMV1dLFswLDQsIlMnIixbMTE1LDczLDQzLDFdXSxbMSw0LCJcXFBvYmpQcmltIixbMTE1LDczLDQwLDFdXSxbMiwwLCJcXHZEYXNoIixbMTIsNjMsNTIsMV1dLFsyLDIsIlxcdHdpeFV7XFx2RGFzaH1fZiJdLFsyLDQsIlxcdkRhc2gnIixbMTE1LDczLDQwLDFdXSxbNCwyLCJFIl0sWzEsMiwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzEsMCwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzYsNCwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFs2LDUsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0M119XSxbNywxLCJwIiwyLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs4LDMsInBfZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDYsInAnIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzMsNiwiZl8qXFx0aW1tIDFfe00nfSIsMSx7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFszLDEsIjFfU1xcdGltbSBmXioiLDEseyJjb2xvdXIiOlswLDYwLDYwXX0sWzAsNjAsNjAsMV1dLFs4LDcsIlxcc2F0VG9TYXRfZiIsMSx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOCw5LCJcXHNhdFRvU2F0J19mIiwxLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbMyw5LCJcXHRleHR7W3BiXX0iLDEseyJsYWJlbF9wb3NpdGlvbiI6NzAsImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzExNSw3Myw0MCwxXV0sWzcsMTAsInEiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzksMTAsInEnIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzQsMCwiZl4qIiwwLHsiY3VydmUiOi0zfV0sWzIsNSwiZl8qIiwyLHsiY3VydmUiOjN9XSxbOCwxMCwicV9mIl0sWzMsMiwiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19XSxbMyw0LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzEsOCwiXFx0ZXh0e1twYl19IiwxLHsibGFiZWxfcG9zaXRpb24iOjcwLCJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMCw2MCw2MCwxXV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\vDash} \\
	\textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
	\& {\twixU{P}} \& {\twixU{\vDash}_f} \&\& E \\
	\textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
	\textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\vDash'}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-2, to=2-1]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-2, to=1-1]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-2, to=4-1]
	\arrow[draw={rgb,255:red,43;green,190;blue,30}, from=5-2, to=5-1]
	\arrow["p"', color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow["{p_f}"', dashed, from=3-3, to=3-2]
	\arrow["{p'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-3, to=5-2]
	\arrow["{f_*\timm 1_{M'}}"{description}, color={rgb,255:red,40;green,176;blue,28}, from=3-2, to=5-2]
	\arrow["{1_S\timm f^*}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=3-2, to=1-2]
	\arrow["{\satToSat_f}"{description}, color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
	\arrow["{\satToSat'_f}"{description}, color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
	\arrow["{\text{[pb]}}"{description, pos=0.7}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-2, to=5-3]
	\arrow["q", color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=3-5]
	\arrow["{q'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-3, to=3-5]
	\arrow["{f^*}", curve={height=-18pt}, from=4-1, to=1-1]
	\arrow["{f_*}"', curve={height=18pt}, from=2-1, to=5-1]
	\arrow["{q_f}", from=3-3, to=3-5]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, from=3-2, to=2-1]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=3-2, to=4-1]
	\arrow["{\text{[pb]}}"{description, pos=0.7}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=1-2, to=3-3]
\end{tikzcd}
}

\newcommand{\twistedMorphDefPacked}{
% https://q.uiver.app/#q=WzAsNCxbMCwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzAsMiwiXFx0d2l4VXtQfV9mIl0sWzAsNCwiXFxQb2JqUHJpbSIsWzExNSw3Myw0MCwxXV0sWzMsMiwiRSJdLFsxLDAsIjFfU1xcdGltbSBmXioiLDAseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fSxbMCw2MCw2MCwxXV0sWzEsMiwiZl8qXFx0aW1tMV97TSd9IiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fSxbMTE1LDczLDQwLDFdXSxbMCwzLCJcXHZEYXNoIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19LFsxMiw2Myw1MiwxXV0sWzIsMywiXFx2RGFzaCciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMSwzLCJcXHR3aXN0ZWRTYXRYZG57Zn0iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \\
	\\
	{\twixU{P}_f} \&\&\& E \\
	\\
	\textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim}
	\arrow["{1_S\timm f^*}", "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=3-1, to=1-1]
	\arrow["{f_*\timm1_{M'}}"', "\shortmid"{marking, text={rgb,255:red,40;green,176;blue,28}}, color={rgb,255:red,40;green,176;blue,28}, from=3-1, to=5-1]
	\arrow["\vDash", "\shortmid"{marking, text={rgb,255:red,210;green,86;blue,55}}, color={rgb,255:red,210;green,86;blue,55}, from=1-1, to=3-4]
	\arrow["{\vDash'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-1, to=3-4]
	\arrow["{\twistedSatXdn{f}}"{description}, dashed, from=3-1, to=3-4]
\end{tikzcd}
}

\newcommand{\satAxiomPacked}{
% https://q.uiver.app/#q=WzAsNixbMCwyLCJNJyIsWzI0NywzOSw3NSwxXV0sWzEsMCwiTSIsWzAsNjAsNjAsMV1dLFsxLDMsIk0nIixbMTE1LDczLDQzLDFdXSxbMywwLCJTIixbMCw2MCw2MCwxXV0sWzMsMywiUyciLFsxMTUsNzMsNDAsMV1dLFs0LDEsIlMiLFsyNDcsMzksNzUsMV1dLFswLDEsImZeKiIsMCx7ImNvbG91ciI6WzI0NywzOSw3NV19XSxbMCwyLCIiLDIseyJsZXZlbCI6MiwiY29sb3VyIjpbMjQ3LDM5LDc1XSwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDIsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFszLDEsIlxcdkRhc2hfe01TfSIsMix7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19LFswLDYwLDYwLDFdXSxbNCwyLCJcXHZEYXNoX3tNJ1MnfSIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX0sWzExNSw3Myw0MCwxXV0sWzMsNSwiIiwwLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSw0LCJmXyoiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzMsNCwiZl97Kip9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzMsMiwiXFx2RGFzaF97TSdTfV5mIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
	\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
	\textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
	\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'}
	\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=3-1, to=1-2]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=3-1, to=4-2]
	\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-2, to=4-2]
	\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-4, to=1-2]
	\arrow["{\vDash_{M'S'}}", "\shortmid"{marking, text={rgb,255:red,40;green,176;blue,28}}, color={rgb,255:red,40;green,176;blue,28}, from=4-4, to=4-2]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-4, to=2-5]
	\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-5, to=4-4]
	\arrow["{f_{**}}", "\shortmid"{marking}, from=1-4, to=4-4]
	\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-4, to=4-2]
\end{tikzcd}
}
	
\newcommand{\morphComposeProof}{
% https://q.uiver.app/#q=WzAsMTcsWzAsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMSwwLCJQIixbMTIsNjMsNTIsMV1dLFswLDEsIlMiLFsxMiw2Myw1MiwxXV0sWzEsMiwiXFx0d2l4VXtQfV9mIl0sWzAsNiwiUyciLFsxMTUsNzMsNDMsMV1dLFsxLDQsIlBfe2YuZ30iLFsyNDIsNzgsNjAsMV1dLFsyLDAsIlxcdkRhc2giLFsxMiw2Myw1MiwxXV0sWzIsMiwiXFx0d2l4VXtcXHZEYXNofV9mIl0sWzIsNCwiXFx2RGFzaF97Zi5nfSIsWzI0Miw3OCw2MCwxXV0sWzMsNCwiUCciLFsxMTUsNzMsNDAsMV1dLFs1LDQsIlxcdkRhc2gnIixbMTE1LDczLDQwLDFdXSxbMCw4LCJTJyciXSxbMCw3LCJNJyciXSxbMSw2LCJcXHR3aXhVe1B9X2ciXSxbMSw3LCJQJyciXSxbMiw2LCJcXHR3aXhVe1xcdkRhc2h9X2ciXSxbMCw1LCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsMiwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMSwwLCIiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs2LDEsInAiLDIseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzcsMywicF9mIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzgsNSwicF97Zmd9IiwyLHsiY29sb3VyIjpbMjQyLDc4LDYwXX0sWzI0Miw3OCw2MCwxXV0sWzMsMSwiMV9TXFx0aW1tIGZeKiIsMSx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzcsNiwiXFxzYXRUb1NhdF9mIiwxLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzAsNjAsNjAsMV1dLFs4LDcsIlxcZWxsX2YiLDEseyJsYWJlbF9wb3NpdGlvbiI6ODAsImNvbG91ciI6WzI0Miw3OCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzI0Miw3OCw2MCwxXV0sWzMsOCwiXFx0ZXh0e1twYl19IiwxLHsibGFiZWxfcG9zaXRpb24iOjgwLCJjb2xvdXIiOlsyNDIsNzgsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsyNDIsNzgsNjAsMV1dLFsyLDQsImZfKiIsMix7ImN1cnZlIjozfV0sWzMsMiwiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxLDcsIlxcdGV4dHtbcGJdfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzAsNjAsNjAsMV1dLFs3LDEwLCJcXHNhdFRvU2F0J19mIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbMyw5LCIiLDEseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzUsMiwiIiwwLHsiY3VydmUiOi0xLCJjb2xvdXIiOlsxMiw2Myw1Ml19XSxbNSwxMiwiIiwyLHsiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzQsMTEsImdfKiIsMix7ImN1cnZlIjozfV0sWzUsMywiMV9TXFx0aW1tIGdeKiIsMSx7ImNvbG91ciI6WzI0Miw3OCw2MF19LFsyNDIsNzgsNjAsMV1dLFsxMCw5LCJwJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFsxNCwxMV0sWzEzLDRdLFsxMywxMl0sWzgsOSwiXFwjIiwwLHsibGV2ZWwiOjJ9XSxbOCwxNSwiXFxlbGxfZyIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo3MCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzE1LDEwLCJcXHNhdFRvU2F0J19nIiwxLHsiY29sb3VyIjpbMjQyLDc4LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjQyLDc4LDYwLDFdXSxbMTMsOV0sWzUsMTNdLFsxNSwxMywiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzE0LDEyXSxbMTYsMCwiZl4qIiwwLHsiY3VydmUiOi0zfV0sWzMsMTYsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxMiwxNiwiZ14qIiwwLHsiY3VydmUiOi0zfV0sWzUsOSwiMV9TXFx0aW1tIGdeKiIsMSx7ImN1cnZlIjo0fV0sWzIwLDI5LCJcXHRleHR7W119IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwibGV2ZWwiOjEsImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMTE1LDczLDQwLDFdXV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{P} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\vDash} \\
	\textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
	\& {\twixU{P}_f} \& {\twixU{\vDash}_f} \\
	\\
	\& \textcolor{rgb,255:red,79;green,73;blue,233}{P_{f.g}} \& \textcolor{rgb,255:red,79;green,73;blue,233}{\vDash_{f.g}} \& \textcolor{rgb,255:red,40;green,176;blue,28}{P'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{\vDash'} \\
	\textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
	\textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& {\twixU{P}_g} \& {\twixU{\vDash}_g} \\
	{M''} \& {P''} \\
	{S''}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, dotted, from=1-2, to=2-1]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, dotted, from=1-2, to=1-1]
	\arrow["p"', color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{p_f}"', dashed, from=3-3, to=3-2]
	\arrow["{p_{fg}}"', color={rgb,255:red,79;green,73;blue,233}, from=5-3, to=5-2]
	\arrow["{1_S\timm f^*}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=3-2, to=1-2]
	\arrow["{\satToSat_f}"{description}, color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
	\arrow["{\ell_f}"{description, pos=0.8}, color={rgb,255:red,79;green,73;blue,233}, dotted, from=5-3, to=3-3]
	\arrow["{\text{[pb]}}"{description, pos=0.8}, color={rgb,255:red,79;green,73;blue,233}, draw=none, from=3-2, to=5-3]
	\arrow["{f_*}"', curve={height=18pt}, from=2-1, to=7-1]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, dotted, from=3-2, to=2-1]
	\arrow["{\text{[pb]}}"{description, pos=0.8}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=1-2, to=3-3]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{\satToSat'_f}", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-6]
	\arrow[color={rgb,255:red,40;green,176;blue,28}, from=3-2, to=5-4]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, curve={height=-6pt}, from=5-2, to=2-1]
	\arrow[color={rgb,255:red,92;green,92;blue,214}, dotted, from=5-2, to=8-1]
	\arrow["{g_*}"', curve={height=18pt}, from=7-1, to=9-1]
	\arrow["{1_S\timm g^*}"{description}, color={rgb,255:red,79;green,73;blue,233}, from=5-2, to=3-2]
	\arrow["{p'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-6, to=5-4]
	\arrow[from=8-2, to=9-1]
	\arrow[from=7-2, to=7-1]
	\arrow[from=7-2, to=8-1]
	\arrow["{\#}", Rightarrow, from=5-3, to=5-4]
	\arrow["{\ell_g}"{description, pos=0.7}, dotted, from=5-3, to=7-3]
	\arrow["{\satToSat'_g}"{description}, color={rgb,255:red,79;green,73;blue,233}, dashed, from=7-3, to=5-6]
	\arrow[from=7-2, to=5-4]
	\arrow[from=5-2, to=7-2]
	\arrow[dashed, from=7-3, to=7-2]
	\arrow[from=8-2, to=8-1]
	\arrow["{f^*}", curve={height=-18pt}, from=6-1, to=1-1]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, dotted, from=3-2, to=6-1]
	\arrow["{g^*}", curve={height=-18pt}, from=8-1, to=6-1]
	\arrow["{1_S\timm g^*}"{description}, curve={height=24pt}, from=5-2, to=5-4]
	\arrow["{\text{[]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, shorten <=16pt, shorten >=16pt, dotted, no head, from=0, to=1]
\end{tikzcd}
}

% this diag is drawn but is not used stil

\newcommand{\satAxiomWithVerviaOk}{
	% https://q.uiver.app/#q=WzAsMTIsWzAsMl0sWzEsMCwiTSIsWzAsNjAsNjAsMV1dLFsyLDAsIlxcUG9iaiJdLFsxLDEsIlMiLFswLDYwLDYwLDFdXSxbMiwyLCJcXHR3aXh7UH0iXSxbMSwzLCJNJyIsWzEyMCw2MCw0MCwxXV0sWzEsNCwiUyciLFsxMjAsNjAsNDAsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMjAsNjAsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFswLDYwLDYwLDFdXSxbMyw0LCJcXERhc2h2JyIsWzEyMCw2MCw0MCwxXV0sWzUsMiwiXFxWZXJPYmoiXSxbNiwyLCJcXG9rT2JqIixbMCw2MCw2MCwxXV0sWzIsMywiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19XSxbMiwxLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs3LDUsIiIsMCx7ImNvbG91ciI6WzEyMCw2MCw0MF19XSxbNyw2LCIiLDAseyJjb2xvdXIiOlsxMjAsNjAsNDBdfV0sWzgsMiwidSIsMix7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSw3LCJ1JyIsMCx7ImNvbG91ciI6WzEyMCw2MCw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MCwxXV0sWzQsNywiISciLDIseyJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dLFs0LDIsIiEiLDAseyJjb2xvdXIiOlsyNDksODAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDksODAsNjAsMV1dLFsxLDUsImZeKiIsMix7ImN1cnZlIjozLCJjb2xvdXIiOls2LDkwLDYwXX0sWzYsOTAsNjAsMV1dLFs2LDMsImZfKiIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbNiw5MCw2MF19LFs2LDkwLDYwLDFdXSxbMTEsMTBdLFs0LDVdLFs0LDNdLFs4LDExLCJcXHZlciIsMCx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSwxMSwiXFx2ZXInIiwyLHsiY29sb3VyIjpbMTIwLDYwLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTIwLDYwLDQwLDFdXSxbNCwxMCwiXFx0d2l4e1xcdmVyfSIsMCx7ImN1cnZlIjotMn1dLFsyLDEwLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs3LDEwLCIiLDAseyJjb2xvdXIiOlsxMjAsNjAsNDBdfV0sWzQsMTAsIlxcdHdpc3RlZFNhdFhkbntmfSIsMSx7ImN1cnZlIjoyLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifX19XV0=
	\begin{tikzcd}[ampersand replacement=\&,sep=small]
		\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \& \Pobj \& \textcolor{rgb,255:red,214;green,92;blue,92}{\Dashv} \\
		\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
		{} \&\& {\twix{P}} \&\&\& \VerObj \& \textcolor{rgb,255:red,214;green,92;blue,92}{\okObj} \\
		\& \textcolor{rgb,255:red,41;green,163;blue,41}{M'} \\
		\& \textcolor{rgb,255:red,41;green,163;blue,41}{S'} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\PobjPrim} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\Dashv'}
		\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=2-2]
		\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=1-2]
		\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=4-2]
		\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=5-2]
		\arrow["u"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=1-4, to=1-3]
		\arrow["{u'}", color={rgb,255:red,41;green,163;blue,41}, dashed, from=5-4, to=5-3]
		\arrow["{!'}"', color={rgb,255:red,92;green,92;blue,214}, dashed, from=3-3, to=5-3]
		\arrow["{!}", color={rgb,255:red,96;green,71;blue,235}, dashed, from=3-3, to=1-3]
		\arrow["{f^*}"', color={rgb,255:red,245;green,80;blue,61}, curve={height=18pt}, from=1-2, to=4-2]
		\arrow["{f_*}", color={rgb,255:red,245;green,80;blue,61}, curve={height=-18pt}, from=5-2, to=2-2]
		\arrow[from=3-7, to=3-6]
		\arrow[from=3-3, to=4-2]
		\arrow[from=3-3, to=2-2]
		\arrow["\ver", color={rgb,255:red,214;green,92;blue,92}, dashed, from=1-4, to=3-7]
		\arrow["{\ver'}"', color={rgb,255:red,41;green,163;blue,41}, dashed, from=5-4, to=3-7]
		\arrow["{\twix{\ver}}", curve={height=-12pt}, from=3-3, to=3-6]
		\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=3-6]
		\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=3-6]
		\arrow["{\twistedSatXdn{f}}"{description}, curve={height=12pt}, tail reversed, from=3-3, to=3-6]
	\end{tikzcd}
}




%=== PREVIOUS VERSIONS 

\newcommand{\vsatDefTripleDiagram}{
% https://q.uiver.app/#q=WzAsMjUsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs1LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbMTEsMCwiUCJdLFsxMywyLCJFIl0sWzExLDQsIlAnIl0sWzgsNSwiXFx0ZXh0e2EpfSJdLFsxMSw1LCJcXHRleHR7Yil9Il0sWzExLDIsIlxcdHdpeFV7UH1fZiJdLFszLDUsIlxcdGV4dHsqKX0gIl0sWzIsMywiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzIsMSwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzcsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFs3LDYsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0M119XSxbOCwyLCJyIiwyLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs5LDQsInJfZiIsMl0sWzEwLDcsInInIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksOCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksMTAsIlxcc2F0VG9TYXRfKl5mIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMCw2MCw2MCwxXV0sWzQsMTAsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzExNSw3Myw0MCwxXV0sWzgsMTEsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzEwLDExLCJlJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzksMTEsImVfZiJdLFs0LDMsIiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfV0sWzQsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFsxMiwxMywiZl4qIiwwLHsiY29sb3VyIjpbMjQ3LDM5LDc1XX1dLFsxMiwxNCwiIiwyLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTQsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxMywiXFx2RGFzaF97TVN9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX0sWzAsNjAsNjAsMV1dLFsxNiwxNCwiXFx2RGFzaF97TSdTJ30iLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMTUsMTcsIiIsMCx7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDE2LCJmXyoiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzE1LDE2LCJmX3sqKn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTUsMTQsIlxcdkRhc2hfe00nU31eZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxOCwxOSwiXFx2RGFzaCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMCwxOSwiXFx2RGFzaCciLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMjMsMTgsIiFfKl5mIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIzLDIwLCIhXypeZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMywxOSwiXFx0d2lzdGVkU2F0WGRue2Z9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dXQ==
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \&\&\&\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \&\& P \\
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \&\&\&\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
	{} \&\& {\twixU{P}_f} \& {\twistedSatXdn{f}} \&\& E \&\&\&\&\&\& {\twixU{P}_f} \&\& E \\
	\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
	\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'} \&\&\&\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'} \&\& {P'} \\
	\&\&\& {\text{*)} } \&\&\&\&\& {\text{a)}} \&\&\& {\text{b)}}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
	\arrow[draw={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
	\arrow["r"', color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=1-3]
	\arrow["{r_f}"', from=3-4, to=3-3]
	\arrow["{r'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=5-3]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
	\arrow["{\satToSat^*_f}"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-4, to=1-4]
	\arrow["{\satToSat_*^f}", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-4, to=5-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-4]
	\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=3-6]
	\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=3-6]
	\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
	\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
	\arrow["{e_f}", from=3-4, to=3-6]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=4-7, to=1-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=4-7, to=5-8]
	\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-8, to=5-8]
	\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-10, to=1-8]
	\arrow["{\vDash_{M'S'}}", color={rgb,255:red,40;green,176;blue,28}, from=5-10, to=5-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-10, to=2-11]
	\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-11, to=5-10]
	\arrow["{f_{**}}", "\shortmid"{marking}, from=1-10, to=5-10]
	\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-10, to=5-8]
	\arrow["\vDash", "\shortmid"{marking}, from=1-12, to=3-14]
	\arrow["{\vDash'}"', "\shortmid"{marking}, from=5-12, to=3-14]
	\arrow["{!_*^f}", "\shortmid"{marking}, from=3-12, to=1-12]
	\arrow["{!_*^f}"', "\shortmid"{marking}, from=3-12, to=5-12]
	\arrow["{\twistedSatXdn{f}}", "\shortmid"{marking}, from=3-12, to=3-14]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
\end{tikzcd}
}


\newcommand{\vsatDefMainDiag}{
% https://q.uiver.app/#q=WzAsOSxbMCwyXSxbMSwwLCJNIixbMTIsNjMsNTIsMV1dLFsyLDAsIlxcUG9iaiIsWzEyLDYzLDUyLDFdXSxbMSwxLCJTIixbMTIsNjMsNTIsMV1dLFsyLDIsIlxcdHdpeFV7UH1fZiJdLFsxLDMsIk0nIixbMTE1LDczLDQwLDFdXSxbMSw0LCJTJyIsWzExNSw3Myw0MywxXV0sWzIsNCwiXFxQb2JqUHJpbSIsWzExNSw3Myw0MCwxXV0sWzUsMiwiRSJdLFsyLDMsIiIsMCx7ImNvbG91ciI6WzEyLDYzLDUyXX1dLFsyLDEsIiIsMCx7ImNvbG91ciI6WzEyLDYzLDUyXX1dLFs3LDUsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19XSxbNyw2LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDNdfV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXX0sWzAsNjAsNjAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzQsMywiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19XSxbNCw1LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMiw4LCJcXHZEYXNoIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19LFsxMiw2Myw1MiwxXV0sWzcsOCwiXFx2RGFzaCciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHR3aXN0ZWRTYXRYZG57Zn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \\
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
	{} \&\& {\twixU{P}_f} \&\&\& E \\
	\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
	\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
	\arrow[draw={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, from=3-3, to=1-3]
	\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
	\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, from=3-3, to=5-3]
	\arrow["\vDash", "\shortmid"{marking, text={rgb,255:red,210;green,86;blue,55}}, color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=3-6]
	\arrow["{\vDash'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-3, to=3-6]
	\arrow["{\twistedSatXdn{f}}", "\shortmid"{marking}, from=3-3, to=3-6]
\end{tikzcd}
}


\newcommand{\vsatDefMainDiagUnpacked}{
% https://q.uiver.app/#q=WzAsMTYsWzAsMl0sWzIsMCwiXFxQb2JqIixbMTIsNjMsNTIsMV1dLFsyLDIsIlxcdHdpeFV7UH1fZiJdLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs0LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbOCw1LCJcXHRleHR7aWkpfSJdLFszLDUsIlxcdGV4dHtpKX0gIl0sWzQsMSwicCIsMix7ImNvbG91ciI6WzEyLDYzLDUyXX0sWzEyLDYzLDUyLDFdXSxbNSwyLCJcXHR3aXhVe3B9X2YiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNiwzLCJwJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFsyLDMsIiFfKl5mIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbMiwxLCIhXipfZiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzUsNCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzUsNiwiXFxzYXRUb1NhdF8qXmYiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dLFsyLDQsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFswLDYwLDYwLDFdXSxbMiw2LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMTUsNzMsNDAsMV1dLFs0LDcsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzYsNywiZSciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNSw3LCJcXHR3aXhVe2V9X2YiXSxbOCw5LCJmXioiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzgsMTAsIiIsMix7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzksMTAsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMSw5LCJcXHZEYXNoX3tNU30iLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fSxbMCw2MCw2MCwxXV0sWzEyLDEwLCJcXHZEYXNoX3tNJ1MnfSIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFsxMSwxMywiIiwwLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTIsImZfKiIsMCx7ImNvbG91ciI6WzI0NywzOSw3NV19XSxbMTEsMTIsImZfeyoqfSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxMSwxMCwiXFx2RGFzaF97TSdTfV5mIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\&\& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \&\&\&\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
	\&\&\&\&\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
	{} \&\& {\twixU{P}_f} \& {\twistedSatXdn{f}} \& E \\
	\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
	\&\& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'} \&\&\&\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'} \\
	\&\&\& {\text{i)} } \&\&\&\&\& {\text{ii)}}
	\arrow["p"', color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=1-3]
	\arrow["{\twixU{p}_f}"', dashed, from=3-4, to=3-3]
	\arrow["{p'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=5-3]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, from=3-3, to=1-3]
	\arrow["{\satToSat^*_f}"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-4, to=1-4]
	\arrow["{\satToSat_*^f}", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-4, to=5-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-4]
	\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=3-5]
	\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=3-5]
	\arrow["{\twixU{e}_f}", from=3-4, to=3-5]
	\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=4-7, to=1-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=4-7, to=5-8]
	\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-8, to=5-8]
	\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-10, to=1-8]
	\arrow["{\vDash_{M'S'}}", color={rgb,255:red,40;green,176;blue,28}, from=5-10, to=5-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-10, to=2-11]
	\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-11, to=5-10]
	\arrow["{f_{**}}", "\shortmid"{marking}, from=1-10, to=5-10]
	\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-10, to=5-8]
\end{tikzcd}
}

\newcommand{\satAxiomWithVer}{
	% https://q.uiver.app/#q=WzAsMTIsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFs0LDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzQsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzQsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs2LDIsIkUiXSxbMiwzLCIiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19XSxbMiwxLCIiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19XSxbNyw1LCIiLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfV0sWzcsNiwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQzXX1dLFs4LDIsInAiLDIseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzksNCwiXFx0d2l4VXtwfV9mIiwyXSxbMTAsNywicCciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNCw3LCIhJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiISIsMCx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSw4LCJcXHNhdFRvU2F0IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzAsNjAsNjAsMV1dLFs5LDEwLCJcXHNhdFRvU2F0UHJpbSIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExNSw3Myw0MCwxXV0sWzQsOCwiXFx0ZXh0e1twYl19IiwxLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzAsNjAsNjAsMV1dLFs0LDEwLCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMTUsNzMsNDAsMV1dLFs4LDExLCJlIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFsxMCwxMSwiZSciLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbNSwxLCJmXioiLDAseyJjdXJ2ZSI6LTN9XSxbMyw2LCJmXyoiLDIseyJjdXJ2ZSI6M31dLFs5LDExLCJcXHR3aXhVe2V9X2YiXSxbNCwzLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs0LDUsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0MF19XV0=
	\begin{tikzcd}[ampersand replacement=\&,sep=small]
		\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \&\& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \\
		\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \\
		{} \&\& {\twixU{P}_f} \&\& {\twistedSatXdn{f}} \&\& E \\
		\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \\
		\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'}
		\arrow[color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
		\arrow[color={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
		\arrow[color={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
		\arrow[color={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
		\arrow["p"', color={rgb,255:red,210;green,86;blue,55}, from=1-5, to=1-3]
		\arrow["{\twixU{p}_f}"', from=3-5, to=3-3]
		\arrow["{p'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-5, to=5-3]
		\arrow["{!'}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
		\arrow["{!}", color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
		\arrow["\satToSat"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-5, to=1-5]
		\arrow["\satToSatPrim", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-5, to=5-5]
		\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-5]
		\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-5]
		\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-5, to=3-7]
		\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-5, to=3-7]
		\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
		\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
		\arrow["{\twixU{e}_f}", from=3-5, to=3-7]
		\arrow[color={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
		\arrow[color={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\end{tikzcd}
}


\endinput

%
% URL s of useful quiver diags
%
%-->   \vsatDefTripleDiagram
% https://q.uiver.app/#q=WzAsMjUsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs1LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbMTEsMCwiUCJdLFsxMywyLCJFIl0sWzExLDQsIlAnIl0sWzgsNSwiXFx0ZXh0e2EpfSJdLFsxMSw1LCJcXHRleHR7Yil9Il0sWzExLDIsIlxcdHdpeFV7UH1fZiJdLFszLDUsIlxcdGV4dHsqKX0gIl0sWzIsMywiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzIsMSwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzcsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFs3LDYsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0M119XSxbOCwyLCJyIiwyLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs5LDQsInJfZiIsMl0sWzEwLDcsInInIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksOCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksMTAsIlxcc2F0VG9TYXRfKl5mIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMCw2MCw2MCwxXV0sWzQsMTAsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzExNSw3Myw0MCwxXV0sWzgsMTEsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzEwLDExLCJlJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzksMTEsImVfZiJdLFs0LDMsIiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfV0sWzQsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFsxMiwxMywiZl4qIiwwLHsiY29sb3VyIjpbMjQ3LDM5LDc1XX1dLFsxMiwxNCwiIiwyLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTQsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxMywiXFx2RGFzaF97TVN9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX0sWzAsNjAsNjAsMV1dLFsxNiwxNCwiXFx2RGFzaF97TSdTJ30iLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMTUsMTcsIiIsMCx7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDE2LCJmXyoiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzE1LDE2LCJmX3sqKn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTUsMTQsIlxcdkRhc2hfe00nU31eZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxOCwxOSwiXFx2RGFzaCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMCwxOSwiXFx2RGFzaCciLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMjMsMTgsIiFfKl5mIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIzLDIwLCIhXypeZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMywxOSwiXFx0d2lzdGVkU2F0WGRue2Z9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dXQ==

========
%-->  unknown   https://q.uiver.app/?q=WzAsMTQsWzEsMl0sWzIsMCwiTSJdLFszLDAsIlAiXSxbMiwxLCJTIl0sWzMsMiwiXFx0d2l4e1B9Il0sWzIsMywiTSciXSxbMiw0LCJTJyJdLFszLDQsIlAnIl0sWzQsMCwiXFxEYXNodiJdLFs0LDIsIlxcdHdpeHtcXERhc2h2fV5mIl0sWzQsNCwiXFxEYXNodiciXSxbNSwyLCJWIl0sWzAsMCwiXFxEYXNodl9WIl0sWzAsNCwiXFxEYXNodidfViJdLFsyLDNdLFsyLDFdLFs3LDVdLFs3LDZdLFs0LDFdLFs0LDZdLFs4LDIsInUiLDJdLFs5LDQsIlxcdHdpeHt1fSIsMix7ImNvbG91ciI6WzYsOTAsNjBdfSxbNiw5MCw2MCwxXV0sWzEwLDcsInUnIiwyXSxbNCw3LCIhJyIsMix7ImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0MCw2MCw2MCwxXV0sWzQsMiwiISIsMCx7ImNvbG91ciI6WzI0OSw4MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0OSw4MCw2MCwxXV0sWzksOCwiXFxiYXIgISIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDEwLCJcXGJhcnshJ30iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCw4LCJbcGJdIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsMTAsIltwYl0iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwxMSwidiJdLFsxMCwxMSwidiciLDJdLFsxLDUsImZeKiIsMix7ImN1cnZlIjozLCJjb2xvdXIiOls2LDkwLDYwXX0sWzYsOTAsNjAsMV1dLFs2LDMsImZfKiIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbNiw5MCw2MF19LFs2LDkwLDYwLDFdXSxbOSwxMSwiIiwyLHsiY29sb3VyIjpbNiw5MCw2MF19XSxbOSw0LCJcXGJhciB1ID0gXFxiYXJ7dSd9IiwxLHsibGFiZWxfcG9zaXRpb24iOjYwLCJvZmZzZXQiOjIsImN1cnZlIjotMiwiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzAsNjAsNjAsMV1dLFsxMywxMiwiZiIsMV1d


==> diagrams/groth-equivalence.tex <==
\newcommand{\sliceBicatmorCompact}{% mor and 2-mor for slice cat
\begin{tikzcd}[row sep=4ex, column sep=4ex, ampersand replacement=\& ]
	\bullet
	\ar[r,bend left=20, ""{name=Upper,above}]
	\ar[r, bend right=20, ""{name=Lower, below}]
	\ar[Rightarrow, from=Lower, to=Upper,] 
	\ar[r, bend right = 90, phantom,  "B"{name=B,below}]
	\ar[from=1-1,to=B]
		\& \bullet \ar[from=1-2, to=B]
\end{tikzcd}
}
%-----
\newcommand{\sliceCatmorCompact}{% mor and 2-mor for slice cat
	\begin{tikzcd}[row sep=10ex, column sep=4ex, ampersand replacement=\& ]
		\bullet
%		\ar[r,bend left=20, ""{name=Upper,above}]
%		\ar[r, bend right=20, ""{name=Lower, below}]
%		\ar[Rightarrow, from=Lower, to=Upper,] 
			\ar[r, "f"]
		\ar[r, bend right = 110, phantom,  "B"{name=B,below}]
		\ar[from=1-1,to=B, "t" ']
		\& \bullet \ar[from=1-2, to=B, "t' ", pos=0.3]
	\end{tikzcd}
}
%-----
\newcommand{\sliceCatmor}{% mor and 2-mor for slice cat
\begin{tikzcd}[row sep=4ex, column sep=2ex, ampersand replacement=\& ]
	\bullet
		\ar[rr, "f"] \ar[rd, "t" ', pos=0.35]
	\& \& \bullet \ar[ld, "t' ", pos=0.25]
\\
  \& B\&
\end{tikzcd}
}
%------
\newcommand{\groEq}{ % Grothendieck equivakence
\begin{tikzcd}[row sep=4ex, column sep=4ex, ampersand replacement=\& ]
	\catcat/B   \ar[r, bend left=25, "~\semmXY{}{-}"{name=Upper}]
	\ar[r,<-, bend right=25, "\int\_" '{name=Lower}]
	\ar[from=Lower, to=Upper, phantom, xshift=-1ex, "\approx"]
		\& \Laxcatstar(B,\spansetcat)
\end{tikzcd}
}
%-----
\newcommand{\relsetmorNatVert}{% morphisms go verically, presheaves go horizontally
\begin{tikzcd}[row sep=4ex, column sep=4ex, ampersand replacement=\& ]
	\semm{a} \ar[d, "f_a" ']	
	\ar[r, span,  "\semm{r}"  ]
	\ar[rd, bend left =25, span, derived, ""{name=diagU, below}]
	\ar[rd, bend right=25, span, derived, ""{name=diagL}]
	\ar[from=diagL, to=diagU, Rightarrow, "f_r~~"{above}, pos=0.3]
	\& \semm{b}  \ar[d, "f_b" ]  
	\\
	\semm{a}'  \ar[r,span, "\semm{r}' " ']
	\& \semm{b}'
\end{tikzcd}
}
%-----
\newcommand{\relsetmorSpan}{% relset morphisms as span morphisms 
\begin{tikzcd}[row sep=4ex, column sep=4ex, ampersand replacement=\& ]
		\semm{a} 
			\ar[r, "f_a"]	
			\ar[d, span,  "\semm{r}\;" ', " "{name=Left, right} ]
%		\ar[rd, bend left =25, span, derived, ""{name=diagU, below}]
%		\ar[rd, bend right=25, span, derived, ""{name=diagL}]
%		\ar[from=diagL, to=diagU, Rightarrow, "f_r~~"{above}, pos=0.3]
	\&  \semm{a}' 
			\ar[d,span, "\;\semm{r}'", " "{name=Right, left}] 
			\ar[from=Left, to=Right, "f_r" ]
		\\
		\semm{b} \ar[r, "f_b" '] 
	\& \semm{b}'
\end{tikzcd}
}
%--------
%-----
\newcommand{\relsetmorNat}{% relset morphisms as oplax nat transf
	\begin{tikzcd}[row sep=4ex, column sep=4ex, ampersand replacement=\& ]
		\semm{a} \ar[r, "f_a"]	
		\ar[d, span,  "\semm{r}" ' ]
		\ar[rd, bend left =25, span, derived, ""{name=diagU, below}]
		\ar[rd, bend right=25, span, derived, ""{name=diagL}]
		\ar[from=diagL, to=diagU, Rightarrow, "f_r~~"{above}, pos=0.3]
		\&  \semm{a}' \ar[d,span, "\semm{r}'"] 
		\\
		\semm{b} \ar[r, "f_b" '] 
		\& \semm{b}'
	\end{tikzcd}
}
%--------
%
\vspace{-0.5ex}
\begin{equation}\label{eqdiag:groth-equivalence}
	\begin{tabular}[h]{ccc@{\,}c}
   % slice cat diagram
\sliceCatmor 
%\sliceBicatmor
& %equivalence diagram
\groEq
&  %  morphisms of "spansets" as span morphisms
\relsetmorNat %\relsetmorSpan
&   % morphisms of "spansets" as oplax natural transf
\relsetmorSpan %\relsetmorNat
\\ [40pt]
 	 a)~~  \parbox{5em}{\mor s \rule{1.5mm}{0mm}in $\catcat/B$}
 & 	c)~~\parbox[c]{8.5em}{Grothendieck-type \rule{5mm}{0mm}equivalence}
 & 	\multicolumn{2}{c}{b)~~ 
 	\parbox[c]{15em}{\mor s in $\laxcatstar(B,\spansetcat)$
 		  \\  \rule{15mm}{0mm} \frar{f}{\semm{}}{\semm{}'}} }  %  b1) for \frar{r}{a}{b} in $B$ & b2) 
\end{tabular}
 \end{equation}




==> diagrams/instDef--Fib2ind.tex <==

\begin{equation}\label{eqdiag:instDef}
\begin{tabular}{ll}
	 \instFiberedToIndexedDiamond
		& 	hru-hru-hru
\end{tabular}
\end{equation}

\endinput 




\endinput


\begin{tabular}{c@{\vspace{2ex}}c}
	\begin{tabular}{c}
	\commaLemmaDiamond
	\\ 	[5pt] a1) and a2) 
	\\ [10pt]   \commalemmaWithOpfibElements
	\\  [10pt] b2)
	\end{tabular}
 & %\multirow{2}{*}{\commaLemmaElementsArrows}
	\begin{tabular}{c}
	\commalemmaElementsArrows
	\\ b1) 
	\end{tabular}
\end{tabular}

\\
cInstitution Definition \rule{0mm}{7mm}



==> diagrams/instDef--Ind2fib.tex <==
\begin{figure}\label{figdiag:instDef}
%\begin{equation}\label{eqdiag:instDef}
\begin{tabular}{cc}
	\instDefoooIndToFiboooFirst
& 	\instDefoooIndToFiboooSecond
\\
a) & b) Iso\moric\ PBs are identified 
\end{tabular}
\caption{Institution definition: from indexed to fibred}
%\end{equation}
\end{figure}

\endinput 




\endinput


\begin{tabular}{c@{\vspace{2ex}}c}
	\begin{tabular}{c}
	\commaLemmaDiamond
	\\ 	[5pt] a1) and a2) 
	\\ [10pt]   \commalemmaWithOpfibElements
	\\  [10pt] b2)
	\end{tabular}
 & %\multirow{2}{*}{\commaLemmaElementsArrows}
	\begin{tabular}{c}
	\commalemmaElementsArrows
	\\ b1) 
	\end{tabular}
\end{tabular}

\\
cInstitution Definition \rule{0mm}{7mm}



==> diagrams/instDef.tex <==

\begin{equation}\label{eqdiag:instDef}
\begin{tabular}{ll}
	 \instIndexedToFiberedDiamond
		& 	diagram to be built (see the whiteboard)
\end{tabular}
\end{equation}

\endinput 




\endinput


\begin{tabular}{c@{\vspace{2ex}}c}
	\begin{tabular}{c}
	\commaLemmaDiamond
	\\ 	[5pt] a1) and a2) 
	\\ [10pt]   \commalemmaWithOpfibElements
	\\  [10pt] b2)
	\end{tabular}
 & %\multirow{2}{*}{\commaLemmaElementsArrows}
	\begin{tabular}{c}
	\commalemmaElementsArrows
	\\ b1) 
	\end{tabular}
\end{tabular}

\\
cInstitution Definition \rule{0mm}{7mm}



==> diagrams/labelledDiagDef.tex <==
\newcommand{\labelledDiagDef}{
% https://q.uiver.app/#q=WzAsNSxbMCwwLCJcXEdHIl0sWzIsMCwiXFxHRy9HIl0sWzAsMiwiXFxjYXJyb3B7XFxjc2lnfSJdLFsyLDIsIlxcTER4e0d9IixbMjIyLDczLDQ4LDFdXSxbNSwxXSxbMSwwLCJcXGRvbV97R30iLDJdLFszLDEsIlxcYm1hcGZ1blh7R30iLDIseyJjb2xvdXIiOlsyMjIsNzMsNDhdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyMjIsNzMsNDgsMV1dLFszLDAsIlxcdGV4dHtbcGJdfV97R30iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMywyLCJcXGVsbFh7R30iLDIseyJjb2xvdXIiOlsyMjIsNzMsNDhdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyMjIsNzMsNDgsMV1dLFsyLDAsIlxcYXJmdW4iLDEseyJsYWJlbF9wb3NpdGlvbiI6NjB9XSxbMSwwLCJcXHRleHR7W2ZpYl19IiwxLHsib2Zmc2V0IjotMywiY29sb3VyIjpbMzM5LDc1LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMzM5LDc1LDYwLDFdXSxbMywyLCJcXHRleHR7W2ZpYl19IiwwLHsib2Zmc2V0IjotMSwiY29sb3VyIjpbMjIyLDczLDQ4XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMjIyLDczLDQ4LDFdXV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\GG \&\& {\GG/G} \\
	\&\&\&\&\& {} \\
	{\carrop{\csig}} \&\& \textcolor{rgb,255:red,33;green,87;blue,212}{\LDx{G}}
	\arrow["{\dom_{G}}"', from=1-3, to=1-1]
	\arrow["{\bmapfunX{G}}"', color={rgb,255:red,33;green,87;blue,212}, dashed, from=3-3, to=1-3]
	\arrow["{\text{[pb]}_{G}}"{description}, draw=none, from=3-3, to=1-1]
	\arrow["{\ellX{G}}"', color={rgb,255:red,33;green,87;blue,212}, dashed, from=3-3, to=3-1]
	\arrow["\arfun"{description, pos=0.6}, from=3-1, to=1-1]
	\arrow["{\text{[fib]}}"{description}, shift left=3, color={rgb,255:red,230;green,76;blue,130}, draw=none, from=1-3, to=1-1]
	\arrow["{\text{[fib]}}", shift left=1, color={rgb,255:red,33;green,87;blue,212}, draw=none, from=3-3, to=3-1]
\end{tikzcd}
}

\begin{equation}\label{eqdiag:twoPBsquares4sig}
	\labelledDiagDef
	%\twoPBsquaresFromCsig
\end{equation}

==> diagrams/liftingVSat.tex <==
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJcXG9wWHt7KFxcQ0NeXFx0d29jYXQpfX17XFx0aW1lc31cXENDXlxcdHdvY2F0Il0sWzAsMSwiXFxvcFh7XFxDQ317XFx0aW1lc31cXENDIl0sWzIsMSwiXFxWU2F0Y2F0WHtcXENDLFZ9Il0sWzIsMCwiXFxWU2F0Y2F0TGlmdGVkWHtcXENDXlxcdHdvY2F0LFxcaWRfVn0iXSxbMiwxLCIoXFxtb2RmdW4sIFxcc2VuZnVuKSJdLFswLDEsIlxcY29ke1xcdGltZXN9XFxjb2QiLDJdLFswLDEsIlxcdGV4dHtbZmliXX0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMywwLCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMywyLCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMywyLCJcXHRleHR7W2ZpYl19IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMywiXFx0ZXh0e1twYl19IiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\begin{equation}\label{eqdiag:lifitngVSats}
\begin{tikzcd}
	{\opX{{(\CC^\twocat)}}{\times}\CC^\twocat} && {\VSatcatLiftedX{\CC^\twocat,\id_V}} \\
	{\opX{\CC}{\times}\CC} && {\VSatcatX{\CC,V}}
	\arrow["{(\modfun, \senfun)}", from=2-3, to=2-1]
	\arrow["{\cod{\times}\cod}"', from=1-1, to=2-1]
	\arrow["{\text{[fib]}}", draw=none, from=1-1, to=2-1]
	\arrow[dashed, from=1-3, to=1-1]
	\arrow[dashed, from=1-3, to=2-3]
	\arrow["{\text{[fib]}}", draw=none, from=1-3, to=2-3]
	\arrow["{\text{[pb]}}"{description}, draw=none, from=2-1, to=1-3]
\end{tikzcd}
\end{equation}
\endinput
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJcXG9wWHt7KFxcQ0NeXFx0d29jYXQpfX17XFx0aW1lc31cXENDXlxcdHdvY2F0Il0sWzAsMSwiXFxvcFh7XFxDQ317XFx0aW1lc31cXENDIl0sWzIsMSwiXFxWU2F0Y2F0WHtcXENDLFZ9Il0sWzIsMCwiXFxWU2F0Y2F0TGlmdGVkWHtcXENDXlxcdHdvY2F0LFZ9Il0sWzIsMSwiKFxcbW9kZnVuLCBcXHNlbmZ1bikiXSxbMCwxLCJcXGNvZHtcXHRpbWVzfVxcY29kIiwyXSxbMCwxLCJcXHRleHR7W2ZpYl19IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMCwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzMsMiwiIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzMsMiwiXFx0ZXh0e1tmaWJdfSIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDMsIlxcdGV4dHtbcGJdfSIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==

	\begin{tikzcd}
	{\opX{{(\CC^\twocat)}}{\times}\CC^\twocat} && {\VSatcatLiftedX{\CC^\twocat,V}} \\
	{\opX{\CC}{\times}\CC} && {\VSatcatX{\CC,V}}
	\arrow["{(\modfun, \senfun)}", from=2-3, to=2-1]
	\arrow["{\cod{\times}\cod}"', from=1-1, to=2-1]
	\arrow["{\text{[fib]}}", draw=none, from=1-1, to=2-1]
	\arrow[dashed, from=1-3, to=1-1]
	\arrow[dashed, from=1-3, to=2-3]
	\arrow["{\text{[fib]}}", draw=none, from=1-3, to=2-3]
	\arrow["{\text{[pb]}}"{description}, draw=none, from=2-1, to=1-3]
\end{tikzcd}
\end{equation}
\endinput
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJcXG9wWHtcXENDXlxcdHdvY2F0fXtcXHRpbWVzfVxcQ0NeXFx0d29jYXQiXSxbMCwxLCJcXG9wWHtcXENDfXtcXHRpbWVzfVxcQ0MiXSxbMiwxLCJcXFZTYXRjYXRYe1xcQ0MsVn0iXSxbMiwwLCJcXFZTYXRjYXRYe1xcQ0NeXFx0d29jYXQsVn0iXSxbMiwxLCIoXFxtb2RmdW4sIFxcc2VuZnVuKSJdLFswLDEsIlxcY29ke1xcdGltZXN9XFxjb2QiLDJdLFswLDEsIltmaWJdIiwwLHsib2Zmc2V0IjotNCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzMsMCwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzMsMiwiIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzMsMiwiW2ZpYl0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSwzLCJbcGJdIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{\opX{\CC^\twocat}{\times}\CC^\twocat} && {\VSatcatX{\CC^\twocat,V}} \\
	{\opX{\CC}{\times}\CC} && {\VSatcatX{\CC,V}}
	\arrow["{(\modfun, \senfun)}", from=2-3, to=2-1]
	\arrow["{\cod{\times}\cod}"', from=1-1, to=2-1]
	\arrow["{[fib]}", shift left=4, draw=none, from=1-1, to=2-1]
	\arrow[dashed, from=1-3, to=1-1]
	\arrow[dashed, from=1-3, to=2-3]
	\arrow["{[fib]}", draw=none, from=1-3, to=2-3]
	\arrow["{[pb]}"{description}, draw=none, from=2-1, to=1-3]
\end{tikzcd}\]

==> diagrams/mainTh-brief.tex <==
% https://q.uiver.app/?q=WzAsOSxbMCwxLCJcXEluc3RjYXRTaWciXSxbMSwxLCJcXHByZWRzaWdvcCJdLFswLDIsIlxcYXJyb3djYXRHRyJdLFsxLDIsIlxcR0ciXSxbMiwxLCJcXExEaWFnY2F0U2lnIixbMjQwLDYwLDYwLDFdXSxbMiwyLCJcXGFycm93Y2F0R0ciXSxbMywyLCJcXEdHIl0sWzMsMSwiXFxhcnJvd2NhdEdHIl0sWzEsMCwiXFxtb2RlbHNSZXZlcnNlU2lne30iXSxbMCwyLCJcXHRtYXBmdW4iLDJdLFswLDEsIlxcbGFiZnVuIiwyXSxbMiwzLCJcXGNvZCJdLFsxLDMsIlxcYXJmdW4iLDJdLFs0LDEsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs0LDUsIiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs1LDMsIlxcZG9tIiwyXSxbNCw2LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNyw2LCJcXGNvZCIsMl0sWzQsMywiXFx0ZXh0e1twYl19IiwxLHsibGFiZWxfcG9zaXRpb24iOjEwLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSw2LCJcXGNvZCJdLFs4LDAsIlxcdmVybGVnIiwyLHsiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjQwLDYwLDYwLDFdXSxbOCw0LCJcXGNvbnN0cmxlZyIsMix7ImxhYmVsX3Bvc2l0aW9uIjo3MCwiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMjQwLDYwLDYwLDFdXSxbOCw3LCJcXGluc3RsZWciLDAseyJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dXQ==
\begin{tikzcd}[ampersand replacement=\&]
	\& {\modelsReverseSig} 
	\\ [-10pt]
	\InstcatSig \& \predsigop \& \textcolor{rgb,255:red,92;green,92;blue,214}{\LDiagcatSig} \& \arrowcatGG \\
	\arrowcatGG \& \GG \& \arrowcatGG \& \GG
	\arrow["\tmapfun"', from=2-1, to=3-1]
	\arrow["\labfun"', from=2-1, to=2-2]
	\arrow["\cod", from=3-1, to=3-2]
	\arrow["\arfun"', from=2-2, to=3-2]
	\arrow[dashed, from=2-3, to=2-2]
	\arrow[dashed, from=2-3, to=3-3]
	\arrow["\dom"', from=3-3, to=3-2]
	\arrow["\gapnamegap{-1.5}{\cod'}{1}" , pos=0.35,  derived, from=2-3, to=3-4]
	\arrow["\cod"', from=2-4, to=3-4]
	\arrow["{\text{[pb]}}"{description, pos=0.1}, draw=none, from=2-3, to=3-2]
	\arrow["\cod", from=3-3, to=3-4]
	\arrow["\verleg"', color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-2, to=2-1]
	\arrow[" \gapnamegap{1}{\constrleg}{-1}" '{pos=0.45}, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-2, to=2-3]
	\arrow["\instleg", color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-2, to=2-4]
\end{tikzcd}


==> diagrams/mainTh-in-arrowCat.tex <==
%-------------------------------------
% -- now the diagram in ArrCat
%-------------------------------------

\begin{equation}
	\label{eqdiag:cartesianEInst-inArrowcat}
	%\mainThdiagInArrcatSpansInside
	\mainThDiamondSpansInside
\end{equation}


\endinput



==> diagrams/mainThProof--chasingPiece.tex <==
\newcommand{\horzX}[1]{\slicecatcsigXY{\GG}{#1}}
\newcommand{\vertX}[1]{\slicecatdeltaXY{\GG}{#1}}

\renewcommand{\LDx}[1]{\horzX{#1}}
\newcommand{\PsubobjX}[1]{\enma{\vDash_{#1}^{}}}
\newcommand{\PsubobjtwiX}[1]{\enma{\vDash_{\twixSymbol#1}}}

\renewcommand{\PobjX}[1]{\PreinstcatX{#1}}
\renewcommand{\PobjtwiX}[1]{\PreinstcatX{\twixSymbol#1}}

\newcommand{\QobjDLR}[3]{\enma{  % 3 arguments : Down index, Left slice and Right slice
	\begin{array}{c}
		\PobjX{#1}=
		\\
		\horzX{#2}\timm\vertX{#3}.
	\end{array}
	}}

\newcommand{\okTargetX}[1]{\PreinstcatX{#1}}

\newcommand{\OKobj}{\InstcatXdn{\csig}}
\newcommand{\okArrow}{\ok}

\newcommand{\mainThProofChasingPiece}{
% https://q.uiver.app/#q=WzAsMjEsWzAsMCwiXFxhcnJvd2NhdEdHIl0sWzIsMCwiXFxHRyJdLFs0LDAsIlxcR0cvRyIsWzExLDU2LDU1LDFdXSxbNSwwLCJcXF97XFx0aW1lc31cXF8iLFsxMSw1Niw1NSwxXV0sWzYsMCwiXFx2ZXJ0WHtHfSIsWzExLDU2LDU1LDFdXSxbMCwyLCJcXE9Lb2JqIl0sWzIsMiwiXFxjYXJyb3B7XFxwcmVkc2lnfSJdLFszLDEsIlxcTER4e0d9IixbMTEsNTYsNTUsMV1dLFs1LDIsIlxcUW9iakRMUntHfXtHfXtHfSIsWzExLDU2LDU1LDFdXSxbMSwxLCJcXG9rVGFyZ2V0WHtcXGNzaWd9IixbMjIyLDczLDQ4LDFdXSxbNCwzLCJcXHZEYXNoX3tHJ30iLFsxMSw1Niw1NSwxXV0sWzcsMV0sWzUsNCwiXFxRb2JqRExSe2Z9e0d9e0cnfSJdLFs2LDgsIlxcdmVydFh7Ryd9IixbMTIwLDYwLDM1LDFdXSxbNSw2LCJcXFFvYmpETFJ7Ryd9e0cnfXtHJ30iLFsxMjAsNjAsMzUsMV1dLFszLDcsIlxcTER4e0cnfSIsWzEyMCw2MCwzNSwxXV0sWzEsNywiXFxva1RhcmdldFh7XFxjc2lnfSJdLFs1LDgsIlxcX3tcXHRpbWVzfVxcXyIsWzEyMCw2MCwzNSwxXV0sWzQsOCwiXFxHRy9HJyJdLFswLDYsIlxcT0tvYmoiXSxbNCw1LCJcXHZEYXNoX3tHJ30iLFsxMjAsNjAsMzUsMV1dLFs1LDAsIlxcdG1hcGZ1bnNpZyJdLFswLDEsIlxcY29kIl0sWzYsMSwiXFxhcmZ1biIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo2MH1dLFs1LDYsIlxcbGFiZnVuc2lnIl0sWzUsOSwiXFxva19cXGNzaWciXSxbOSwwLCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbOSw2LCIiLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbOSwxLCJcXHRleHR7W3BiXX1fXFxjc2lnIiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwxLCJcXGRvbV97R30iLDIseyJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzcsNiwiXFxlbGxYe0d9IiwwLHsiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMSw1Niw1NSwxXV0sWzcsMiwiXFxibWFwZnVuWHtHfSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjowLCJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExLDU2LDU1LDFdXSxbMywyLCJoXzAiLDIseyJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzExLDU2LDU1LDFdXSxbOCw0LCJ2IiwxLHsibGFiZWxfcG9zaXRpb24iOjYwLCJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzgsMywiKFxcYm1hcGZ1bl5HLFxcLCAxKSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjo3MCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMSw1Niw1NSwxXV0sWzMsMCwiXFxwYmZ1bnZYe0cnfSIsMix7ImN1cnZlIjo0LCJjb2xvdXIiOlsxMSw1Niw1NV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzExLDU2LDU1LDFdXSxbOCw5LCJcXCNfe0d9IiwxLHsibGFiZWxfcG9zaXRpb24iOjQwLCJjb2xvdXIiOlsxMSw1Niw1NV19LFsxMSw1Niw1NSwxXV0sWzcsMSwiXFx0ZXh0e1twYl19X3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMSw1Niw1NSwxXV0sWzEwLDUsIlxcbGlmdGVkWHtcXCNfR30iLDAseyJjdXJ2ZSI6LTEsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTEsNTYsNTUsMV1dLFszLDQsInZfMCIsMCx7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTEsNTYsNTUsMV1dLFsxMCw5LCJcXHRleHR7W3BiXX0nX3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjoxMCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMSw1Niw1NSwxXV0sWzgsNywiaCIsMSx7ImNvbG91ciI6WzExLDU2LDU1XX0sWzExLDU2LDU1LDFdXSxbMTAsOCwiXFxsaWZ0ZWRYe1xcb2tfXFxjc2lnfSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY29sb3VyIjpbMTEsNTYsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMSw1Niw1NSwxXV0sWzEyLDEzLCJcXHR3aXhEe3Z9IiwwLHsiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzEzLDQsImZeKl9cXERlbHRhIiwyXSxbMTIsOCwiKDEsZl4qX1xcRGVsdGEpIiwyLHsiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFsxNCwxNSwiaCciLDEseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTQsMTMsInYnIiwxLHsiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzEyLDE0LCIoZl8qXlxcY3NpZywgMSkiLDIseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbNywxNSwiZl8qXlxcY3NpZyIsMl0sWzE0LDE2LCJcXCNfe0cnfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY29sb3VyIjpbMTIwLDYwLDM1XX0sWzEyMCw2MCwzNSwxXV0sWzE3LDEzLCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMTQsMTcsIihcXGJtYXBmdW5ee0cnfSwgMSkiLDIseyJjb2xvdXIiOlsxMjAsNjAsMzVdfSxbMTIwLDYwLDM1LDFdXSxbMTcsMTgsIiIsMix7ImNvbG91ciI6WzEyMCw2MCwzNV0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFsxNSwxOF0sWzksMTYsIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxOSwxNiwiXFxva19cXGNzaWciXSxbMjAsMTksIlxcbGlmdGVkWHtcXCNfe0cnfX0iLDIseyJjb2xvdXIiOlsxMjAsNjAsMzVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMjAsNjAsMzUsMV1dLFsyMCwxNCwiIiwyLHsiY29sb3VyIjpbMTIwLDYwLDM1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzUsMTksIiIsMix7ImxldmVsIjoyLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxMiw3LCIiLDAseyJjdXJ2ZSI6Miwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\arrowcatGG \&\& \GG \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\GG/G} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\_{\times}\_} \& \textcolor{rgb,255:red,205;green,100;blue,76}{\vertX{G}} \\
	\& \textcolor{rgb,255:red,33;green,87;blue,212}{\okTargetX{\csig}} \&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\LDx{G}} \&\&\&\& {} \\
	\OKobj \&\& {\carrop{\predsig}} \&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\QobjDLR{G}{G}{G}} \\
	\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\vDash_{G'}} \\
	\&\&\&\&\& {\QobjDLR{f}{G}{G'}} \\
	\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\vDash_{G'}} \\
	\OKobj \&\&\&\&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\QobjDLR{G'}{G'}{G'}} \\
	\& {\okTargetX{\csig}} \&\& \textcolor{rgb,255:red,36;green,143;blue,36}{\LDx{G'}} \\
	\&\&\&\& {\GG/G'} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\_{\times}\_} \& \textcolor{rgb,255:red,36;green,143;blue,36}{\vertX{G'}}
	\arrow["\tmapfunsig", from=3-1, to=1-1]
	\arrow["\cod", from=1-1, to=1-3]
	\arrow["\arfun"{description, pos=0.6}, from=3-3, to=1-3]
	\arrow["\labfunsig", from=3-1, to=3-3]
	\arrow["{\ok_\csig}", from=3-1, to=2-2]
	\arrow[dotted, from=2-2, to=1-1]
	\arrow[dotted, from=2-2, to=3-3]
	\arrow["{\text{[pb]}_\csig}"{description, pos=0.4}, draw=none, from=2-2, to=1-3]
	\arrow["{\dom_{G}}"', color={rgb,255:red,205;green,100;blue,76}, from=1-5, to=1-3]
	\arrow["{\ellX{G}}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=2-4, to=3-3]
	\arrow["{\bmapfunX{G}}"{pos=0}, color={rgb,255:red,205;green,100;blue,76}, dotted, from=2-4, to=1-5]
	\arrow["{h_0}"', color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-5]
	\arrow["v"{description, pos=0.6}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=1-7]
	\arrow["{(\bmapfun^G,\, 1)}"{pos=0.7}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=3-6, to=1-6]
	\arrow["{\pbfunvX{G'}}"', color={rgb,255:red,205;green,100;blue,76}, curve={height=24pt}, dashed, from=1-6, to=1-1]
	\arrow["{\#_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-2]
	\arrow["{\text{[pb]}_{G}}"{description, pos=0.4}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=2-4, to=1-3]
	\arrow["{\liftedX{\#_G}}", color={rgb,255:red,205;green,100;blue,76}, curve={height=-6pt}, dashed, from=4-5, to=3-1]
	\arrow["{v_0}", color={rgb,255:red,205;green,100;blue,76}, dotted, from=1-6, to=1-7]
	\arrow["{\text{[pb]}'_{G}}"{description, pos=0.1}, color={rgb,255:red,205;green,100;blue,76}, draw=none, from=4-5, to=2-2]
	\arrow["h"{description}, color={rgb,255:red,205;green,100;blue,76}, from=3-6, to=2-4]
	\arrow["{\liftedX{\ok_\csig}}"{pos=0.3}, color={rgb,255:red,205;green,100;blue,76}, dashed, from=4-5, to=3-6]
	\arrow["{\twixD{v}}", color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=9-7]
	\arrow["{f^*_\Delta}"', from=9-7, to=1-7]
	\arrow["{(1,f^*_\Delta)}"', color={rgb,255:red,205;green,100;blue,76}, from=5-6, to=3-6]
	\arrow["{h'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-4]
	\arrow["{v'}"{description}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-7]
	\arrow["{(f_*^\csig, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=5-6, to=7-6]
	\arrow["{f_*^\csig}"', from=2-4, to=8-4]
	\arrow["{\#_{G'}}"'{pos=0.3}, color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=8-2]
	\arrow[dotted, from=9-6, to=9-7]
	\arrow["{(\bmapfun^{G'}, 1)}"', color={rgb,255:red,36;green,143;blue,36}, from=7-6, to=9-6]
	\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=9-6, to=9-5]
	\arrow[from=8-4, to=9-5]
	\arrow[Rightarrow, dotted, no head, from=2-2, to=8-2]
	\arrow["{\ok_\csig}", from=7-1, to=8-2]
	\arrow["{\liftedX{\#_{G'}}}"', color={rgb,255:red,36;green,143;blue,36}, dotted, from=6-5, to=7-1]
	\arrow[color={rgb,255:red,36;green,143;blue,36}, dotted, from=6-5, to=7-6]
	\arrow[Rightarrow, dotted, no head, from=3-1, to=7-1]
	\arrow[curve={height=12pt}, dotted, from=5-6, to=2-4]
\end{tikzcd}
}
%\begin{figure}
\begin{equation}
\mainThProofChasingPiece
\end{equation}
%\end{figure}





\endinput

\newcommand{\mainThProofChasingHuge}{
% the full routing chasing piece 
% https://q.uiver.app/#q=WzAsMTksWzAsMiwiXFxhcnJvd2NhdEdHIl0sWzIsMiwiXFxHRyJdLFs0LDIsIlxcR0cvRyciLFsxMjAsNjAsNDIsMV1dLFs1LDIsIlxcX3tcXHRpbWVzfVxcXyIsWzEyMCw2MCw0MiwxXV0sWzYsMiwiXFxkZWx0YXNsaWNlY2F0R0dHcHJpbSIsWzEyMCw2MCw0MiwxXV0sWzAsNCwiXFxJbnN0Y2F0c2lnIl0sWzIsNCwiXFxjYXJyb3B7XFxwcmVkc2lnfSJdLFs0LDQsIlxcTERHcHJpbSIsWzEyMCw2MCw0MiwxXV0sWzUsNCwiXFxwcmVJbnN0Y2F0WHtHJ30iLFsxMjAsNjAsNDIsMV1dLFsxLDMsIlxccHJlSW5zdGNhdHNpZyIsWzIyMiw3Myw0OCwxXV0sWzMsNSwiXFx2RGFzaF97Ryd9IixbMTIwLDYwLDQyLDFdXSxbNiw1LCJcXEdHL0ciLFsxMSw1Niw1NSwxXV0sWzYsNiwiXFxMREciLFszMCw2MCw1NSwxXV0sWzcsNiwiXFxwcmVJbnN0Y2F0WHtcXHR3aXhTeW1ib2x9Il0sWzYsNywiXFx0d2l4VXtcXHZEYXNofV97Zl8qfSIsWzEyMCw2MCw0MiwxXV0sWzcsOCwiXFx0ZXh0e1xcZm9vdG5vdGVzaXplIHRvIFxccHJlSW5zdGNhdHNpZ30iLFsyNzAsNjAsNjAsMV1dLFs3LDQsIlxcX1xcdHdpeFV7XFx0aW1lc31cXF8iXSxbNiwwLCJcXHBiZnVudlh7R30iLFsxMSw1Niw1NSwxXV0sWzcsM10sWzUsMCwiXFx0bWFwZnVuc2lnIl0sWzAsMSwiXFxjb2QiXSxbNiwxLCJcXGFyZnVuIl0sWzUsNiwiXFxsYWJmdW5zaWciXSxbNSw5LCJcXCNfXFxwcmVkc2lnIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksMCwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksNiwiIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzksMSwiXFx0ZXh0e1twYl19IiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzIsMSwiXFxkb21fe0cnfSIsMix7ImNvbG91ciI6WzEyMCw2MCw0Ml19LFsxMjAsNjAsNDIsMV1dLFs3LDYsIlxcZWxsX3tHJ30iLDIseyJjb2xvdXIiOlsxMjAsNjAsNDJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMjAsNjAsNDIsMV1dLFs3LDIsIlxcYm1hcGZ1blh7R1wifSIsMCx7ImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzMsMiwiaCdfMCIsMix7ImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzgsNCwidiciLDAseyJsYWJlbF9wb3NpdGlvbiI6NjAsImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzgsMywiXFwjX3tHJ30iLDAseyJsYWJlbF9wb3NpdGlvbiI6NDAsImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzMsMCwiXFxwYmZ1bnZYe0cnfSIsMix7ImN1cnZlIjo0LCJjb2xvdXIiOlsxMjAsNjAsNDJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMjAsNjAsNDIsMV1dLFs4LDksIlxcI1xcI197Ryd9IiwyLHsiY29sb3VyIjpbMTIwLDYwLDQyXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTIwLDYwLDQyLDFdXSxbNywxLCJcXHRleHR7W3BiXX1fezFHJ30iLDEseyJsYWJlbF9wb3NpdGlvbiI6NjAsImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzEyMCw2MCw0MiwxXV0sWzEwLDUsInBeRV97Ryd9IiwyLHsiY3VydmUiOi0xLCJjb2xvdXIiOlsxMjAsNjAsNDJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMjAsNjAsNDIsMV1dLFsxMCw4LCJcXHBTTXh7Ryd9IiwwLHsiY3VydmUiOjEsImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzMsNCwididfMCIsMCx7ImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzEyLDExLCJcXGJtYXBmdW5Ye0d9IiwyLHsiY29sb3VyIjpbMzAsNjAsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFszMCw2MCw1NSwxXV0sWzEyLDYsIlxcZWxsX3tHfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo0MCwiY29sb3VyIjpbMzAsNjAsNTVdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFszMCw2MCw1NSwxXV0sWzExLDEsIlxcZG9tX3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY3VydmUiOjMsImNvbG91ciI6WzMwLDYwLDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMzAsNjAsNTUsMV1dLFsxMiwxLCJcXHRleHR7W3BiXX1fezFHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjoxMCwiY3VydmUiOjMsImNvbG91ciI6WzMwLDYwLDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMzAsNjAsNTUsMV1dLFsxMywxMiwiXFx0d2l4e2h9IiwwLHsiY29sb3VyIjpbMTEsNTYsNTVdfSxbMTEsNTYsNTUsMV1dLFsxMSwyLCJmXyoiLDIseyJsYWJlbF9wb3NpdGlvbiI6MzAsImN1cnZlIjozfV0sWzE0LDEwLCJcXGxpZnRlZFh7XFwjX3tmXyp9fSIsMix7ImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzE0LDEzLCJcXHBTTXh7Zl8qfSIsMix7ImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX0sWzEyMCw2MCw0MiwxXV0sWzEyLDcsImZfKl57TER9IiwyLHsiY3VydmUiOjEsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxNCw4LCJcXHRleHR7W3BiXX1fezJmfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjozMCwiY3VydmUiOi0yLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTQsNSwicF5FX3tmXyp9IiwwLHsiY3VydmUiOi0yLCJjb2xvdXIiOlsxMjAsNjAsNDJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsxMjAsNjAsNDIsMV1dLFsxMCw5LCJcXHRleHR7W3BiXX1fezJHJ30iLDEseyJsYWJlbF9wb3NpdGlvbiI6MjAsImNvbG91ciI6WzEyMCw2MCw0Ml0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzEyMCw2MCw0MiwxXV0sWzgsNywiaCciLDIseyJjb2xvdXIiOlsyMjIsNzMsNDhdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyMjIsNzMsNDgsMV1dLFsxNiw0LCJcXHR3aXhVe3ZfMH0iLDEseyJjdXJ2ZSI6MSwiY29sb3VyIjpbMTIwLDYwLDQyXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMTIwLDYwLDQyLDFdXSxbMTYsMTEsIiIsMix7ImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzEzLDE2LCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTMsMTUsIlxcI1xcI197Zl8qfSIsMix7ImxhYmVsX3Bvc2l0aW9uIjo4MH1dLFsxNiwzLCIiLDIseyJjdXJ2ZSI6MSwiY29sb3VyIjpbMTIwLDYwLDQyXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzEzLDgsIlxcI197Zl8qfSIsMix7ImN1cnZlIjozLCJjb2xvdXIiOlsxMjAsNjAsNDJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMjAsNjAsNDIsMV1dLFsxNiwxNywiIiwyLHsiY3VydmUiOjUsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTcsMCwiIiwyLHsiY3VydmUiOjQsImNvbG91ciI6WzExLDU2LDU1XSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzE4LDQsIiIsMix7ImN1cnZlIjoxLCJjb2xvdXIiOlsxMjAsNjAsNDJdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTMsMTgsIlxcdHdpeFV7dn0iLDIseyJjdXJ2ZSI6NSwiY29sb3VyIjpbMTIwLDYwLDQyXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsxMjAsNjAsNDIsMV1dXQ==
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\&\&\&\&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\pbfunvX{G}} \\
	\\
	\arrowcatGG \&\& \GG \&\& \textcolor{rgb,255:red,43;green,171;blue,43}{\GG/G'} \& \textcolor{rgb,255:red,43;green,171;blue,43}{\_{\times}\_} \& \textcolor{rgb,255:red,43;green,171;blue,43}{\deltaslicecatGGGprim} \\
	\& \textcolor{rgb,255:red,33;green,87;blue,212}{\preInstcatsig} \&\&\&\&\&\& {} \\
	\Instcatsig \&\& {\carrop{\predsig}} \&\& \textcolor{rgb,255:red,43;green,171;blue,43}{\LDGprim} \& \textcolor{rgb,255:red,43;green,171;blue,43}{\preInstcatX{G'}} \&\& {\_\twixU{\times}\_} \\
	\&\&\& \textcolor{rgb,255:red,43;green,171;blue,43}{\vDash_{G'}} \&\&\& \textcolor{rgb,255:red,205;green,100;blue,76}{\GG/G} \\
	\&\&\&\&\&\& \textcolor{rgb,255:red,209;green,140;blue,71}{\LDG} \& {\preInstcatX{\twixSymbol}} \\
	\&\&\&\&\&\& \textcolor{rgb,255:red,43;green,171;blue,43}{\twixU{\vDash}_{f_*}} \\
	\&\&\&\&\&\&\& \textcolor{rgb,255:red,153;green,92;blue,214}{\text{\footnotesize to \preInstcatsig}}
	\arrow["\tmapfunsig", from=5-1, to=3-1]
	\arrow["\cod", from=3-1, to=3-3]
	\arrow["\arfun", from=5-3, to=3-3]
	\arrow["\labfunsig", from=5-1, to=5-3]
	\arrow["{\#_\predsig}", dashed, from=5-1, to=4-2]
	\arrow[dashed, from=4-2, to=3-1]
	\arrow[dashed, from=4-2, to=5-3]
	\arrow["{\text{[pb]}}"{description}, draw=none, from=4-2, to=3-3]
	\arrow["{\dom_{G'}}"', color={rgb,255:red,43;green,171;blue,43}, from=3-5, to=3-3]
	\arrow["{\ell_{G'}}"', color={rgb,255:red,43;green,171;blue,43}, dashed, from=5-5, to=5-3]
	\arrow["{\bmapfunX{G"}}", color={rgb,255:red,43;green,171;blue,43}, dashed, from=5-5, to=3-5]
	\arrow["{h'_0}"', color={rgb,255:red,43;green,171;blue,43}, dotted, from=3-6, to=3-5]
	\arrow["{v'}"{pos=0.6}, color={rgb,255:red,43;green,171;blue,43}, dashed, from=5-6, to=3-7]
	\arrow["{\#_{G'}}"{pos=0.4}, color={rgb,255:red,43;green,171;blue,43}, dashed, from=5-6, to=3-6]
	\arrow["{\pbfunvX{G'}}"', color={rgb,255:red,43;green,171;blue,43}, curve={height=24pt}, dashed, from=3-6, to=3-1]
	\arrow["{\#\#_{G'}}"', color={rgb,255:red,43;green,171;blue,43}, dotted, from=5-6, to=4-2]
	\arrow["{\text{[pb]}_{1G'}}"{description, pos=0.6}, color={rgb,255:red,43;green,171;blue,43}, draw=none, from=5-5, to=3-3]
	\arrow["{p^E_{G'}}"', color={rgb,255:red,43;green,171;blue,43}, curve={height=-6pt}, dotted, from=6-4, to=5-1]
	\arrow["{\pSMx{G'}}", color={rgb,255:red,43;green,171;blue,43}, curve={height=6pt}, dotted, from=6-4, to=5-6]
	\arrow["{v'_0}", color={rgb,255:red,43;green,171;blue,43}, dotted, from=3-6, to=3-7]
	\arrow["{\bmapfunX{G}}"', color={rgb,255:red,209;green,140;blue,71}, dashed, from=7-7, to=6-7]
	\arrow["{\ell_{G}}"'{pos=0.4}, color={rgb,255:red,209;green,140;blue,71}, dotted, from=7-7, to=5-3]
	\arrow["{\dom_{G}}"{description, pos=0.8}, color={rgb,255:red,209;green,140;blue,71}, curve={height=18pt}, dotted, from=6-7, to=3-3]
	\arrow["{\text{[pb]}_{1G}}"{description, pos=0.1}, color={rgb,255:red,209;green,140;blue,71}, curve={height=18pt}, draw=none, from=7-7, to=3-3]
	\arrow["{\twix{h}}", color={rgb,255:red,205;green,100;blue,76}, from=7-8, to=7-7]
	\arrow["{f_*}"'{pos=0.3}, curve={height=18pt}, from=6-7, to=3-5]
	\arrow["{\liftedX{\#_{f_*}}}"', color={rgb,255:red,43;green,171;blue,43}, dotted, from=8-7, to=6-4]
	\arrow["{\pSMx{f_*}}"', color={rgb,255:red,43;green,171;blue,43}, dotted, from=8-7, to=7-8]
	\arrow["{f_*^{LD}}"', curve={height=6pt}, dashed, from=7-7, to=5-5]
	\arrow["{\text{[pb]}_{2f}}"{description, pos=0.3}, curve={height=-12pt}, draw=none, from=8-7, to=5-6]
	\arrow["{p^E_{f_*}}", color={rgb,255:red,43;green,171;blue,43}, curve={height=-12pt}, dotted, from=8-7, to=5-1]
	\arrow["{\text{[pb]}_{2G'}}"{description, pos=0.2}, color={rgb,255:red,43;green,171;blue,43}, draw=none, from=6-4, to=4-2]
	\arrow["{h'}"', color={rgb,255:red,33;green,87;blue,212}, dashed, from=5-6, to=5-5]
	\arrow["{\twixU{v_0}}"{description}, color={rgb,255:red,43;green,171;blue,43}, curve={height=6pt}, dotted, from=5-8, to=3-7]
	\arrow[draw={rgb,255:red,205;green,100;blue,76}, dotted, from=5-8, to=6-7]
	\arrow[dashed, from=7-8, to=5-8]
	\arrow["{\#\#_{f_*}}"'{pos=0.8}, from=7-8, to=9-8]
	\arrow[draw={rgb,255:red,43;green,171;blue,43}, curve={height=6pt}, dashed, from=5-8, to=3-6]
	\arrow["{\#_{f_*}}"', color={rgb,255:red,43;green,171;blue,43}, curve={height=18pt}, dashed, from=7-8, to=5-6]
	\arrow[draw={rgb,255:red,205;green,100;blue,76}, curve={height=30pt}, dashed, no head, from=5-8, to=1-7]
	\arrow[draw={rgb,255:red,205;green,100;blue,76}, curve={height=24pt}, dashed, from=1-7, to=3-1]
	\arrow[draw={rgb,255:red,43;green,171;blue,43}, curve={height=6pt}, dashed, from=4-8, to=3-7]
	\arrow["{\twixU{v}}"', color={rgb,255:red,43;green,171;blue,43}, curve={height=30pt}, dashed, no head, from=7-8, to=4-8]
\end{tikzcd}
}

==> diagrams/pb.tex <==
%\[
$
\xymatrix @R=4em @C=4em {
O &   
& A \ar@{>->}[ll]_{x} 
\\
& B  \ar[ul]^{y} 
& AB \ar@{>->}[l]^{x_{y}} \ar@{->}[u]^{y_x}
\\
C \ar@{>->}[uu]^{z} 
& BC \ar[l]^{y_{z}} \ar@{>->}[u]^{z_{y}} 
& ABC \ar@{>->}[l]^{x_{yz}} \ar@{>->}[u]^{z_{yx}}
% top right
\ar@{-} <129pt, -44pt>;<122pt, -44pt>  
\ar@{-} <122pt, -50pt>;<122pt, -44pt> 
% bottom right
\ar@{-} <129pt, -104pt>;<122pt, -104pt>  
\ar@{-} <122pt, -110pt>;<122pt, -104pt> 
% bottom left
\ar@{-} <54pt, -104pt>;<47pt, -104pt>  
\ar@{-} <47pt, -110pt>;<47pt, -104pt> 
}
$
%\]

==> diagrams/satAxiom-Arr-OldWrong.tex <==
\begin{tikzcd}[row sep=2ex, column sep=2ex] %, ampersand replacement = \&] 
		\Modsetsig 
			\ar[dd, "f^*" '] 
			& \modelssig \ar[l, " "] 
			\ar[r, " "] 
			& \Sensetsig 
			& \sysVerset 
			    %\ar[ll, <-, bend right = 25, "verfun"]
		\\ & \footnotesize{\modelsFtwisted} 
										\ar[lu]\ar[rd] 
										\ar[u, rightarrowtail]
										\ar[d, rightarrowtail]
										\ar[rr, bend right=10, dashed, "\gapnamegap{-1}{\verif_f}{1}" ', pos=0.65,]
										& & \vertsim_f
												\ar[u] \ar[d]
		\\
			\ModsetsigPrim
		&  \modelssigPrim \ar[l, ] \ar[r, " "]  
		& \SensetsigPrim  & \sysVerset'
			\ar[from=3-3, to=1-3, pos=0.75,  "f_*" ', crossing over]
			%\ar[from=2-2, to=2-4, "\verif" ', pos=0.75]
		    \ar[from=1-2, to=1-4, bend left=25, "\verif", pos=0.5, dashed]
		    \ar[from=3-2, to=3-4, bend right =25, "\verif'" ', pos=0.5, dashed]
\end{tikzcd}


==> diagrams/satAxiom-Arr.tex <==

% https://q.uiver.app/?q=WzAsOSxbMiwwLCJcXHZEYXNoIl0sWzMsMSwie1xcdGltZXN9Il0sWzQsMCwiXFxTZW5zZXQiXSxbMCwwLCJcXE1vZHNldCJdLFsyLDEsIlxcdHdpeHtcXHZEYXNofSJdLFs0LDIsIlxcU2Vuc2V0JyJdLFswLDIsIlxcTW9kc2V0JyJdLFsyLDIsIlxcdkRhc2gnIl0sWzEsMSwie1xcdGltZXMnfSJdLFsxLDIsIiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs0LDMsIlxcdHdpeHttfSIsMl0sWzQsMCwiXFxzYXRzYXQiXSxbMCwzLCJtIiwyXSxbMCwyLCJzIl0sWzAsMSwidV9cXHZEYXNoIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzQsMSwidShmXyopIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzQsNSwiXFx0d2l4e3N9Il0sWzEsMywiIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzMsNiwiZl4qIiwyXSxbNyw2XSxbNyw1XSxbNSwyLCJmXyoiLDJdLFs4LDYsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs4LDUsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs0LDgsInUoZl4qKSIsMCx7ImxhYmVsX3Bvc2l0aW9uIjozMCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzQsNywiXFxzYXRzYXQnIl0sWzcsOCwidV97XFx2RGFzaCd9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
\begin{mygroup}
	\renewcommand{\twix}[1]{\enma{#1_f}}
\begin{tikzcd}[row sep=3ex, column sep =6ex]
	\Modset && \vDash && \Senset \\
	& {{\times'}} & {\twix{\vDash}} & {{\times}} \\
	{\Modset'} && {\vDash'} && {\Senset'}
	\arrow[dotted, from=2-4, to=1-5]
	\arrow["{\twix{m}}", from=2-3, to=1-1]
	\arrow["\satsat", from=2-3, to=1-3]
	\arrow["m"', from=1-3, to=1-1]
	\arrow["s", from=1-3, to=1-5]
	\arrow["{u_\vDash}", dashed, from=1-3, to=2-4]
	\arrow["{u}", dashed, from=2-3, to=2-4, pos=0.35]
	\arrow["{\twix{s}}", from=2-3, to=3-5]
	\arrow[dotted, from=2-4, to=1-1]
	\arrow["{f^*}"', from=1-1, to=3-1]
	\arrow[from=3-3, to=3-1]
	\arrow[from=3-3, to=3-5]
	\arrow["{f_*}"', from=3-5, to=1-5]
	\arrow[dotted, from=2-2, to=3-1]
	\arrow[dotted, from=2-2, to=3-5]
	\arrow["{u'}"{pos=0.3}, dashed, from=2-3, to=2-2]
	\arrow["{\satsat'}", from=2-3, to=3-3]
	\arrow["{u_{\vDash'}}", dashed, from=3-3, to=2-2]
\end{tikzcd}
\end{mygroup}

==> diagrams/satAxiom-Old.tex <==
{
%	\renewcommand{\Sigmaa}{\enma{L}}
%\vspace{-0.75ex}
\begin{equation}\label{eqdiag:satisfyAxiom}
\begin{array}{c@{}c}
\input{diagrams/satAxiom-Rel}
&
\input{diagrams/satAxiom-Arr}
\end{array}	
%\vspace{-1ex}
\end{equation}
%
} %END Group
\endinput
%\END

==> diagrams/satAxiom-Rel.tex <==
\begin{tabular}{c@{\,}c@{}c} % left column= roow $f$ going vetically+instit square; right col = sat. axiom as iff sttaement 
	\begin{tikzcd}[row sep=4ex, column sep=0.5ex] 
		L
		\\ L' \ar[u, "f"]
	\end{tikzcd}
&	
	\begin{tikzcd}[row sep=4ex, column sep=2ex] %, ampersand replacement = \&] 
	 	\Modset \ar[d, "f^*" ']\ar[r, phantom, "\vDash"] 
	 		& \Senset
	\\
		\Modset' 
			\ar[r, phantom, "\vDash' "] 
			& \Senset' \ar[u, "f_*"]
	\end{tikzcd}
&
\enma{\begin{array}{c} % iff statement 
			m\vDash f_*(\phi')
			\\ [3.5pt]\text{iff}\rule{0ex}{1.ex}
			\\ [3.5pt] f^*(m) \vDash' \phi'
	 \end{array}}
\\ [10pt]
\multicolumn{2}{c}{a)} & b)
\end{tabular}


==> diagrams/satAxiom-abstract.tex <==
%\begin{mygroup}
%[row sep=2ex, column sep= 2ex ]
%[row sep=2ex,  ]
% modifications made: 
% [-15pt]  in \\ [-15pt] row  2 before \twix{P}
% [-15pt]  in \\ [15pt] row  3 after \twix{P}
% shorten >= -1 mm,shorten <= -2 mm for arrow f_*
% shorten >= -1.5mm fro arrow f^*
% 
% 
\begin{mygroup}
	\renewcommand{\Dashv}{\vDash}
	\renewcommand{\twix}[1]{\twixU{#1}}
%   old notation for arrows in the main def  \twistedSatXdn{f}
%  dito for nodes 										\twistedSatXdn{f}


%\vsatDefMainDiag
%\vsatDefMainDiagUnpacked

\begin{equation}\label{eqdiag:twistedSpans}
%\vsatDefTripleDiagram
\begin{tabular}{ccc}
	\twistedMorphDefMain 
& \twistedMorphDefPacked
& \satAxiomPacked
	\\
	a)  &  b) & c)
\end{tabular}
\end{equation}
\end{mygroup}
%

\endinput % the diagram below is excellent but its' for the next paper!

\begin{figure}
	\begin{tabular}{c@{\quad}c}
	\satAxiomWithVer
		& \satAxiomWithVerviaOk
		\\ a) & b)
	\end{tabular}
	\caption{Sat axiom}\label{figdiag:satAxiom}
\end{figure}
\end{mygroup}



==> diagrams/satAxiomVerif-Arr.tex <==
%\begin{mygroup}
%[row sep=2ex, column sep= 2ex ]
%[row sep=2ex,  ]
% modifications made: 
% [-15pt]  in \\ [-15pt] row  2 before \twix{P}
% [-15pt]  in \\ [15pt] row  3 after \twix{P}
% shorten >= -1 mm,shorten <= -2 mm for arrow f_*
% shorten >= -1.5mm fro arrow f^*
% 
% 
\begin{mygroup}
	\renewcommand{\Dashv}{\vDash}
	\renewcommand{\twix}[1]{\twixU{#1}}
\newcommand{\satAxiomVer}{
% https://q.uiver.app/#q=WzAsMTIsWzAsMl0sWzEsMCwiTSIsWzAsNjAsNjAsMV1dLFsyLDAsIlxcUG9iaiJdLFsxLDEsIlMiLFswLDYwLDYwLDFdXSxbMiwyLCJcXHR3aXh7UH0iXSxbMSwzLCJNJyIsWzEyMCw2MCw0MCwxXV0sWzEsNCwiUyciLFsxMjAsNjAsNDAsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMjAsNjAsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFswLDYwLDYwLDFdXSxbMyw0LCJcXERhc2h2JyIsWzEyMCw2MCw0MCwxXV0sWzUsMiwiXFxWZXJPYmoiXSxbNiwyLCJcXG9rT2JqIixbMCw2MCw2MCwxXV0sWzIsMywiIiwwLHsiY29sb3VyIjpbMCw2MCw2MF19XSxbMiwxLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs3LDUsIiIsMCx7ImNvbG91ciI6WzEyMCw2MCw0MF19XSxbNyw2LCIiLDAseyJjb2xvdXIiOlsxMjAsNjAsNDBdfV0sWzgsMiwidSIsMix7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSw3LCJ1JyIsMCx7ImNvbG91ciI6WzEyMCw2MCw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzEyMCw2MCw0MCwxXV0sWzQsNywiISciLDIseyJjb2xvdXIiOlsyNDAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDAsNjAsNjAsMV1dLFs0LDIsIiEiLDAseyJjb2xvdXIiOlsyNDksODAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyNDksODAsNjAsMV1dLFsxLDUsImZeKiIsMix7ImN1cnZlIjozLCJjb2xvdXIiOls2LDkwLDYwXX0sWzYsOTAsNjAsMV1dLFs2LDMsImZfKiIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbNiw5MCw2MF19LFs2LDkwLDYwLDFdXSxbMTEsMTBdLFs0LDVdLFs0LDNdLFs4LDExLCJcXHZlciIsMCx7ImNvbG91ciI6WzAsNjAsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFswLDYwLDYwLDFdXSxbOSwxMSwiXFx2ZXInIiwyLHsiY29sb3VyIjpbMTIwLDYwLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTIwLDYwLDQwLDFdXSxbNCwxMCwiXFx0d2l4e1xcdmVyfSIsMCx7ImN1cnZlIjotMn1dLFsyLDEwLCIiLDAseyJjb2xvdXIiOlswLDYwLDYwXX1dLFs3LDEwLCIiLDAseyJjb2xvdXIiOlsxMjAsNjAsNDBdfV0sWzQsMTAsIlxcdHdpc3RlZFNhdFhkbntmfSIsMSx7ImN1cnZlIjoyLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifX19XV0=
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \& \Pobj \& \textcolor{rgb,255:red,214;green,92;blue,92}{\Dashv} \\
	\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \\
	{} \&\& {\twix{P}} \&\&\& \VerObj \& \textcolor{rgb,255:red,214;green,92;blue,92}{\okObj} \\
	\& \textcolor{rgb,255:red,41;green,163;blue,41}{M'} \\
	\& \textcolor{rgb,255:red,41;green,163;blue,41}{S'} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\PobjPrim} \& \textcolor{rgb,255:red,41;green,163;blue,41}{\Dashv'}
	\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=2-2]
	\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=1-2]
	\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=4-2]
	\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=5-2]
	\arrow["u"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=1-4, to=1-3]
	\arrow["{u'}", color={rgb,255:red,41;green,163;blue,41}, dashed, from=5-4, to=5-3]
	\arrow["{!'}"', color={rgb,255:red,92;green,92;blue,214}, dashed, from=3-3, to=5-3]
	\arrow["{!}", color={rgb,255:red,96;green,71;blue,235}, dashed, from=3-3, to=1-3]
	\arrow["{f^*}"', color={rgb,255:red,245;green,80;blue,61}, curve={height=18pt}, from=1-2, to=4-2]
	\arrow["{f_*}", color={rgb,255:red,245;green,80;blue,61}, curve={height=-18pt}, from=5-2, to=2-2]
	\arrow[from=3-7, to=3-6]
	\arrow[from=3-3, to=4-2]
	\arrow[from=3-3, to=2-2]
	\arrow["\ver", color={rgb,255:red,214;green,92;blue,92}, dashed, from=1-4, to=3-7]
	\arrow["{\ver'}"', color={rgb,255:red,41;green,163;blue,41}, dashed, from=5-4, to=3-7]
	\arrow["{\twix{\ver}}", curve={height=-12pt}, from=3-3, to=3-6]
	\arrow[color={rgb,255:red,214;green,92;blue,92}, from=1-3, to=3-6]
	\arrow[color={rgb,255:red,41;green,163;blue,41}, from=5-3, to=3-6]
	\arrow["{\twistedSatXdn{f}}"{description}, curve={height=12pt}, tail reversed, from=3-3, to=3-6]
\end{tikzcd}
}

\satAxiomVer
\end{mygroup}


\endinput
% https://q.uiver.app/?q=WzAsMTQsWzEsMl0sWzIsMCwiTSJdLFszLDAsIlAiXSxbMiwxLCJTIl0sWzMsMiwiXFx0d2l4e1B9Il0sWzIsMywiTSciXSxbMiw0LCJTJyJdLFszLDQsIlAnIl0sWzQsMCwiXFxEYXNodiJdLFs0LDIsIlxcdHdpeHtcXERhc2h2fV5mIl0sWzQsNCwiXFxEYXNodiciXSxbNSwyLCJWIl0sWzAsMCwiXFxEYXNodl9WIl0sWzAsNCwiXFxEYXNodidfViJdLFsyLDNdLFsyLDFdLFs3LDVdLFs3LDZdLFs0LDFdLFs0LDZdLFs4LDIsInUiLDJdLFs5LDQsIlxcdHdpeHt1fSIsMix7ImNvbG91ciI6WzYsOTAsNjBdfSxbNiw5MCw2MCwxXV0sWzEwLDcsInUnIiwyXSxbNCw3LCIhJyIsMix7ImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0MCw2MCw2MCwxXV0sWzQsMiwiISIsMCx7ImNvbG91ciI6WzI0OSw4MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0OSw4MCw2MCwxXV0sWzksOCwiXFxiYXIgISIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs5LDEwLCJcXGJhcnshJ30iLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbNCw4LCJbcGJdIiwxLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzQsMTAsIltwYl0iLDEseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbOCwxMSwidiJdLFsxMCwxMSwidiciLDJdLFsxLDUsImZeKiIsMix7ImN1cnZlIjozLCJjb2xvdXIiOls2LDkwLDYwXX0sWzYsOTAsNjAsMV1dLFs2LDMsImZfKiIsMCx7ImN1cnZlIjotMywiY29sb3VyIjpbNiw5MCw2MF19LFs2LDkwLDYwLDFdXSxbOSwxMSwiIiwyLHsiY29sb3VyIjpbNiw5MCw2MF19XSxbOSw0LCJcXGJhciB1ID0gXFxiYXJ7dSd9IiwxLHsibGFiZWxfcG9zaXRpb24iOjYwLCJvZmZzZXQiOjIsImN1cnZlIjotMiwiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzAsNjAsNjAsMV1dLFsxMywxMiwiZiIsMV1d
\begin{equation
\[\begin{tikzcd}[column sep=4ex, row sep=2ex]
	{\Dashv_V} && M & P & \Dashv 
	\\
	&& S 
	\\ [-15pt]  % row 2
	&{} && {\twix{P}} & {\twix{\Dashv}^f} & V 
	\\ [-15pt]  % row 3
	&& {M'} 
	\\
	{\Dashv'_V} && {S'} & {P'} & {\Dashv'}
	\arrow[from=1-4, to=2-3]
	\arrow[from=1-4, to=1-3]
	\arrow[from=5-4, to=4-3]
	\arrow[from=5-4, to=5-3]
	\arrow[from=3-4, to=1-3]
	\arrow[from=3-4, to=5-3]
	\arrow["u"', from=1-5, to=1-4]
	\arrow["{\twix{u}}"', color={rgb,255:red,245;green,80;blue,61}, from=3-5, to=3-4]
	\arrow["{u'}"', from=5-5, to=5-4]
	\arrow["{!'}"', color={rgb,255:red,92;green,92;blue,214}, dashed, from=3-4, to=5-4]
	\arrow["{!}", color={rgb,255:red,96;green,71;blue,235}, dashed, from=3-4, to=1-4]
	\arrow["{\bar !}" ', dashed, from=3-5, to=1-5]
	\arrow["{\bar{!'}}" , dashed, from=3-5, to=5-5]
	\arrow["{[pb]}"{description}, draw=none, from=3-4, to=1-5]
	\arrow["{[pb]}"{description}, draw=none, from=3-4, to=5-5]
	\arrow["v", from=1-5, to=3-6]
	\arrow["{v'}"', from=5-5, to=3-6]
	\arrow["{f^*}"', color={rgb,255:red,245;green,80;blue,61}, curve={height=18pt}, from=1-3, to=4-3, shorten >= -1.5mm]
	\arrow["{f_*}", color={rgb,255:red,245;green,80;blue,61}, curve={height=-18pt}, from=5-3, to=2-3, shorten >= -1 mm,shorten <= -2 mm]
	\arrow[color={rgb,255:red,245;green,80;blue,61}, from=3-5, to=3-6]
	\arrow["{\bar u = \bar{u'}}"{description, pos=0.5}, shift right=2, color={rgb,255:red,214;green,92;blue,92}, curve={height=-10pt}, draw=none, from=3-5, to=3-4]
	\arrow["f"{description}, from=5-1, to=1-1, color={rgb,255:red,245;green,80;blue,61}, ]
\end{tikzcd}\]



\endinput
% https://q.uiver.app/?q=WzAsMTgsWzEsNSwiTSJdLFsxLDYsIlMiXSxbMSw4LCJNJyJdLFsxLDksIlMnIl0sWzMsNSwiUCJdLFszLDksIlAnIl0sWzMsNywiXFx0d2l4e1B9Il0sWzAsMl0sWzEsMCwiTSJdLFsyLDAsIlAiXSxbMSwxLCJTIl0sWzIsMiwiXFx0d2l4e1B9Il0sWzEsMywiTSciXSxbMSw0LCJTJyJdLFsyLDQsIlAnIl0sWzMsMCwiXFxEYXNodiJdLFszLDIsIlxcdHdpeHtcXERhc2h2fSJdLFszLDQsIlxcRGFzaHYnIl0sWzQsMV0sWzQsMF0sWzUsMl0sWzUsM10sWzYsMF0sWzYsM10sWzAsMiwiZl4qIiwyLHsiY3VydmUiOjN9XSxbMywxLCJmXyoiLDAseyJjdXJ2ZSI6LTN9XSxbOSwxMF0sWzksOF0sWzE0LDEyXSxbMTQsMTNdLFsxMSw4XSxbMTEsMTNdLFsxNSw5LCJ1IiwyXSxbMTYsMTEsIlxcdHdpeHt1fSIsMl0sWzE3LDE0LCJ1JyIsMl1d
\[\begin{tikzcd}[row sep=2ex]
	& M & P & \Dashv \\
	& S \\ [-15pt]
	{} && {\twix{P}} & {\twix{\Dashv}} \\ [-15pt]
	& {M'} \\
	& {S'} & {P'} & {\Dashv'} \\
	& M && P \\
	& S \\
	&&& {\twix{P}} \\
	& {M'} \\
	& {S'} && {P'}
	\arrow[from=6-4, to=7-2]
	\arrow[from=6-4, to=6-2]
	\arrow[from=10-4, to=9-2]
	\arrow[from=10-4, to=10-2]
	\arrow[from=8-4, to=6-2]
	\arrow[from=8-4, to=10-2]
	\arrow["{f^*}"', curve={height=18pt}, from=6-2, to=9-2]
	\arrow["{f_*}", curve={height=-18pt}, from=10-2, to=7-2]
	\arrow[from=1-3, to=2-2]
	\arrow[from=1-3, to=1-2]
	\arrow[from=5-3, to=4-2]
	\arrow[from=5-3, to=5-2]
	\arrow[from=3-3, to=1-2]
	\arrow[from=3-3, to=5-2]
	\arrow["u"', from=1-4, to=1-3]
	\arrow["{\twix{u}}"', from=3-4, to=3-3]
	\arrow["{u'}"', from=5-4, to=5-3]
\end{tikzcd}\]



\endinput
\begin{mygroup}
	\renewcommand{\twix}[1]{\enma{#1_f}}
	% https://q.uiver.app/?q=WzAsMTAsWzIsMCwiXFx2RGFzaCJdLFszLDEsIntcXHRpbWVzfSJdLFs0LDAsIlxcU2Vuc2V0Il0sWzAsMCwiXFxNb2RzZXQiXSxbMiwyLCJcXHZEYXNoX2YiXSxbMCw0LCJcXE1vZHNldCciXSxbMiw0LCJcXHZEYXNoJyJdLFs0LDQsIlxcU2Vuc2V0JyJdLFsxLDMsIntcXHRpbWVzJ30iXSxbNSwyLCJcXFZlcnNldCJdLFsxLDIsIiIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFswLDMsIm0iLDJdLFswLDIsInMiXSxbMCwxLCJ1X1xcdkRhc2giLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMSwzLCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNywyLCJmXyoiLDJdLFszLDUsImZeKiIsMl0sWzYsNV0sWzYsN10sWzQsNiwiXFxzYXRzYXQnX2YiLDIseyJsYWJlbF9wb3NpdGlvbiI6NDB9XSxbNCwwLCJcXHNhdHNhdF9mIl0sWzgsNSwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzYsOCwidV97XFx2RGFzaCd9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzgsNywiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzQsMSwidV9mIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzQsMywiXFxtX2YiXSxbNCw3LCJzX2YiXSxbNiw5LCJ2JyIsMix7ImxhYmVsX3Bvc2l0aW9uIjo4MCwiY3VydmUiOjJ9XSxbMCw5LCJ2IiwwLHsibGFiZWxfcG9zaXRpb24iOjgwLCJjdXJ2ZSI6LTN9XSxbMSw5LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNCw4LCJ1J19mIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzQsOSwiIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
	\begin{tikzcd}[row sep=2ex, column sep =3ex]
		\Modset && \vDash && \Senset 
		\\
		&&& {{\times}} 
		\\
		&& {\vDash_f} &&& \Verset 
		\\
		& {{\times'}} \\
		{\Modset'} && {\vDash'} && {\Senset'}
		\arrow[dotted, from=2-4, to=1-5]
		\arrow["m"', from=1-3, to=1-1]
		\arrow["s", from=1-3, to=1-5]
		\arrow["{u_\vDash}", dashed, from=1-3, to=2-4]
		\arrow[dotted, from=2-4, to=1-1]
		\arrow["{f_*}", from=5-5, to=1-5, pos=0.35]
		\arrow["{f^*}"', from=1-1, to=5-1, ]
		\arrow[from=5-3, to=5-1]
		\arrow[from=5-3, to=5-5]
		\arrow["{\satsat'_f}"'{pos=0.4}, from=3-3, to=5-3]
		\arrow["{\satsat_f}", from=3-3, to=1-3]
		\arrow[dotted, from=4-2, to=5-1]
		\arrow["{u_{\vDash'}}", dashed, from=5-3, to=4-2]
		\arrow[dotted, from=4-2, to=5-5]
		\arrow["{u_f}"', dashed, from=3-3, to=2-4]
		\arrow["{m_f}", from=3-3, to=1-1]
		\arrow["{s_f}", from=3-3, to=5-5]
		\arrow["{\verif'}"'{pos=0.8}, curve={height=12pt}, from=5-3, to=3-6]
		\arrow["\verif"{pos=0.8}, curve={height=-18pt}, from=1-3, to=3-6]
	%	\arrow[dotted, from=2-4, to=3-6]
		\arrow["{u'_f}"', dashed, from=3-3, to=4-2]
		\arrow[" \verif_f",dashed, from=3-3, to=3-6]
	\end{tikzcd}
\end{mygroup}

==> diagrams/semantics-of-skeMor.tex <==
\shortlong{\zd{a diagram is commented here}}{
\begin{figure}
\begin{equation}\label{eq:skeMor-semantics}
\begin{tabular}{c}
\begin{tikzcd}[row sep=4ex, column sep = 6ex]
	\GG^\twocat  
			\ar[r, "\cod", thick] 
& \GG 		
& \GG/G_S 
	\ar[l, "\dom_{G_S}" '] 
& \dernode{\prodnodeS} %
			\ar[l, dotderived, "h" '] 
			\ar[r, dotderived, "v"]
			\ar[lll, derived, bend right =20, "\pbfunV^S" ']
& \GG/G_{S} 
%
%
\\ % Row 2 
\Instcat_\predsig
				 \ar[r, "\labfun", thick ] 
				\ar[u,  "t^\predsig_{\_}"] 
		& \carrop{\predsig}
					\ar[u, "\arfun", pos=0.5]     
		& C_S 
					\ar[l, "\labfunSke" ', thick]
					\ar[u,  "\bmap^S_{\_}", pos=0.5]
		& \dernode{\underprodS} 
					\ar[l, dotderived, "\underX{h}" ', pos=0.8]  
					\ar[r, dotderived,  "\underX{v}" ]
					\ar[u, derived,  "\text{$(\bmapfunX{S},\tmapfunX{S})$}" ', pos=0.5] 
		& \Instcat_S 
				\ar[u,  "t^S_{\_}"]
%		\ar[ll, bend right=20, "\valfunX{t}" ']
%
%
\\  % Row 3
&& \Dashv_S 
%
&  \underline{\Dashv}_S
			%\ar[l, dotDerived, "{\Dashv}_S^{}"]  %\textuparrow
\ar[from=3-4, to=2-4, "\satfun^{'}_S" ', derived]
\ar[from=3-3, to=2-1, bend right = 10, derived] 
\ar[from=3-3, to=1-4,  "\satfun_S" , derived, pos=0.75]
\ar[from=3-4, to=3-3,  "\DashvArrowObjX{S}", derived]
\ar[from=3-3, to=1-2, phantom, "~~\pblabel", pos=0.15]
\ar[from=3-4, to=2-3, phantom, "\pblabel", pos=0.15 ]
%
\end{tikzcd}
%
%
%\\
%\begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}},
%						row sep=4ex, column sep = 8ex]
%t^\predsig_{\_} \ar[r] 
%& \arfun \ar[l,<-] 
%& \bmap^S_{\_} \ar[l]
%& \DashvArrowObjX{S}
%			\ar[l, derived] \ar[r, derived]
%			\ar[lll, derived, bend right =20, "\val_S" ']
%& t^S_{\_} 
%\end{tikzcd}
\end{tabular}
\end{equation}
\end{figure}
%}  % END LONG

\shortlong{\zd{a diagram is commented here}}{
\zd{This is the previous version}

% version before April 29
\begin{tikzcd}[row sep=4ex, column sep = 6ex]
	\GG^\twocat  \ar[r, "\cod", thick] %\ar[ru, <-, derived]
	& \GG 		
	& \GG/G_S 
	\ar[l, "\dom_{G_S}" '] 
	& \dernode{\prodnodeS} %
	\ar[l, derived, "h" '] \ar[r, derived, "v"]
	\ar[lll, derived, bend right =20, "\pbfunV^S" ']
	& \GG/G_{S} 
	\\ % Row 2 
	\Instcat_\predsig
	\ar[r, "\labfun", thick ] 
	\ar[u,  "t^\predsig_{\_}"] 
	& \carrop{\predsig}
	\ar[u, "\arfun", pos=0.5]     
	& C_S \ar[l, "\labfunSke" ', thick]
	\ar[u,  "\bmap^S_{\_}", pos=0.5]
	& \dernode{\underprodS} \ar[l, derived, "\underX{h}" ', ]  \ar[r, derived,  "\underX{v}" ]
	\ar[u,derived,  "\btgluedS" , pos=0.5] 
	& \Instcat_S 
	\ar[u,  "t^S_{\_}"]
	%		\ar[ll, bend right=20, "\valfunX{t}" ']
	\\  % Bottom row
	& PB_S \ar[lu, derived] \ar[rru, derived]
	&& \DashvForIndecesX{S}\ar[ll, derived, rightarrowtail,  "\eqr" ']
	\ar[u, derived]
	\ar[lllu, dotted] \ar[lu, dotted] \ar[ru, dotted]
\end{tikzcd}
%-----



%-------
\begin{figure}
\begin{equation}\label{eq:skeMor-semantics}
\begin{tikzcd}[row sep=4ex, column sep = 4ex]
\Instcat \ar[rr, "\labfun", thick ] 
			&& \carrop{\predsig}    
	&& C_S \ar[ll, "\labfunSke" ', thick]
			\ar[llll, bend right=20, "\valfunX{t}" ']
	&& C_{S'} \ar[ll, "f_C" ', ]
\\  % ROW 2 for middle derived nodes 
    & \dernode{\Preinst}\ar[ru, derived] 
    							\ar[lu, <-, dotDerived, "\#" ']    
								\ar[rd, phantom, gray,  "\text{[pb]}", pos=0.25]
	&&
	\dernode{\circ}\ar[lu, derived]  \ar[ru, <-, dotderived, "\#" ] 
							\ar[ll, dotderived, "\mathbf{!}" ', pos=0.75]
						\ar[ld, phantom, gray,  "\text{[pb]}", pos=0.25]
		&&
	\dernode{\circ}\ar[lu, derived]  \ar[ru, <-, dotderived, "\#" ] 
	\ar[ll, dotderived, "\mathbf{!}" ', pos=0.75]
	\ar[ld, phantom, gray,  "\text{[pb]}", pos=0.25]
\\  % Bottom row
		\GG^\twocat \ar[uu, <-, "t\_"] \ar[rr, "\cod", thick] \ar[ru, <-, derived]
&&	 \GG 				\ar[uu, <-, "\arfun", pos=0.2] 
&&   \GG/G_S \ar[uu, <-, "\bmap\_" ', pos=0.2] \ar[lu, <-, derived]
					  \ar[ll, "\dom_{G_S}" '] 
					  \ar[llll, bend left=15, "\twSubstX{t}" ']
&&
	 \GG/G_{S'} \ar[uu, <-, "\bmap'\_" ', pos=0.2]   \ar[lu, <-, derived]
	 				\ar[ll, "\GG/f_G" ']
	 				\ar[llllll, bend left=20, "\twSubstX{f_G^*(t)}"]
\end{tikzcd}
\end{equation}
\end{figure}
}
%\END
\endinput
% the xypic version of the diagram
%%
%---
\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
			%\\  row 1
	\Instcat \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
	\\   % row 2
		& \Preinst        % Begin entry at (0,0)
			\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
			\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
			\ar@{}[dr]|{(PB)}
		&            % End entry
			\opX{\arrowcatBrackX{\GG}} 	% Begin entry at (1,0)
				\ar[d]^{\codop}            
	\\      % row 3                
		& \predsig   % Begin entry at (0,1)
			\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
			&                        % End entry
		\GGop  % Begin entry (3,3)
}               % Ending xymatrix




\endinput 
% the opposite version

\begin{equation}\label{eq:skedef}
	\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
		%\\  row 1
		\opX{Inst} \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
		\\   % row 2
		& \Preinst        % Begin entry at (0,0)
		\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
		\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
		\ar@{}[dr]|{(PB)}
		&            % End entry
		\arrowcatBrackX{\GG} 	% Begin entry at (1,0)
		\ar[d]^{\cod}            
		\\      % row 3                
		& \opX{\predsig}   % Begin entry at (0,1)
		\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
		&                        % End entry
		\GG                % Begin entry (1,1)
	}               % Ending xymatrix
\end{equation}

==> diagrams/signDef-extended.tex <==
%\begin{equation}\label{eq:skedef}
\begin{tikzcd}[row sep=2ex, column sep = 3ex]
\Instcat_\predsig
			&& \arrowcatGG 
\\ & \dernode{\Instcat^?_\predsig}	&
\\
\carrop{\predsig} \ar[rr, "\arfun"]  && \GG
\ar[from=1-1, to=1-3, "\tmapfunX{\predsig}"] 
\ar[from=1-1, to=3-1, "\labfunSig" ', thick ] 
	\ar[from=1-1, to=3-1, phantom, "\gapnamegap{2.5}{\fiblabelRed}{-2.} ",  thick ]
\ar[from=1-1, to=2-2, derived, "\#_\predsig"]
\ar[from=1-3, to=3-3, "\cod" ', thick ]
	\ar[from=1-3, to=3-3, phantom, "\gapnamegap{2.5}{\fiblabelBlack}{-2.} ",  thick ]
\ar[from=2-2, to=3-1, derived]  
\ar[from=2-2, to=1-3, derived]
\ar[from=2-2, to=3-3, phantom, gray,  "\text{[pb]}", pos=0.25]
\end{tikzcd}
%\end{equation}

\endinput
% the xypic version of the diagram
%%
%---
\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
			%\\  row 1
	\Instcat \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
	\\   % row 2
		& \Preinst        % Begin entry at (0,0)
			\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
			\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
			\ar@{}[dr]|{(PB)}
		&            % End entry
			\opX{\arrowcatExpX{\GG}} 	% Begin entry at (1,0)
				\ar[d]^{\codop}            
	\\      % row 3                
		& \predsig   % Begin entry at (0,1)
			\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
			&                        % End entry
		\GGop  % Begin entry (3,3)
}               % Ending xymatrix




\endinput 
% the opposite version

\begin{equation}\label{eq:skedef}
	\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
		%\\  row 1
		\opX{Inst} \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
		\\   % row 2
		& \Preinst        % Begin entry at (0,0)
		\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
		\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
		\ar@{}[dr]|{(PB)}
		&            % End entry
		\arrowcatBrackX{\GG} 	% Begin entry at (1,0)
		\ar[d]^{\cod}            
		\\      % row 3                
		& \opX{\predsig}   % Begin entry at (0,1)
		\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
		&                        % End entry
		\GG                % Begin entry (1,1)
	}               % Ending xymatrix
\end{equation}

==> diagrams/signDef.tex <==
%\begin{equation}\label{eq:skedef}
\begin{tikzcd}[row sep=2ex, column sep = 3ex]
\Instcat_\predsig
			&& \deltaarrowcatGG 
\\ & \dernode{\Instcat^?_\predsig}	&
\\
\carrop{\predsig} \ar[rr, "\arfun"]  && \GG
\ar[from=1-1, to=1-3, "\tmapfunX{\predsig}"] 
\ar[from=1-1, to=3-1, "\labfunSig" ', thick ] 
	\ar[from=1-1, to=3-1, phantom, "\gapnamegap{2.5}{\fiblabelRed}{-2.} ",  thick ]
\ar[from=1-1, to=2-2, derived, "\#_\predsig"]
\ar[from=1-3, to=3-3, "\cod" ', thick ]
	\ar[from=1-3, to=3-3, phantom, "\gapnamegap{2.5}{\fiblabelBlack}{-2.} ",  thick ]
\ar[from=2-2, to=3-1, derived]  
\ar[from=2-2, to=1-3, derived]
\ar[from=2-2, to=3-3, phantom, gray,  "\text{[pb]}", pos=0.25]
\end{tikzcd}
%\end{equation}

\endinput
% the xypic version of the diagram
%%
%---
\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
			%\\  row 1
	\Instcat \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
	\\   % row 2
		& \Preinst        % Begin entry at (0,0)
			\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
			\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
			\ar@{}[dr]|{(PB)}
		&            % End entry
			\opX{\arrowcatExpX{\GG}} 	% Begin entry at (1,0)
				\ar[d]^{\codop}            
	\\      % row 3                
		& \predsig   % Begin entry at (0,1)
			\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
			&                        % End entry
		\GGop  % Begin entry (3,3)
}               % Ending xymatrix




\endinput 
% the opposite version

\begin{equation}\label{eq:skedef}
	\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
		%\\  row 1
		\opX{Inst} \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
		\\   % row 2
		& \Preinst        % Begin entry at (0,0)
		\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
		\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
		\ar@{}[dr]|{(PB)}
		&            % End entry
		\arrowcatBrackX{\GG} 	% Begin entry at (1,0)
		\ar[d]^{\cod}            
		\\      % row 3                
		& \opX{\predsig}   % Begin entry at (0,1)
		\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
		&                        % End entry
		\GG                % Begin entry (1,1)
	}               % Ending xymatrix
\end{equation}

==> diagrams/slicat2sat--arrows.tex <==



%% this macros (from Latex itself!) does not work! ??  \textuparrow
%%\begin{figure}[hb]
%\begin{equation}%\label{eqdiag:predsigAsSatFunctor}
%\label{eqdiag:predsigAsSatfunctor-inCat} 
%\mainThdiagInCat
%\end{equation}
%%\end{figure}
%\vspace{1mm}

%\begin{figure}[hb] %\label{eqdiag:mainTh}

%\end{figure}

\endinput 




==> diagrams/slicat2sat--objects.tex <==
% this macros (from Latex itself!) does not work! ??  \textuparrow
\begin{mygroup}
\renewcommand{\labfunSke}{\enma{\labfun_G}}
\begin{figure}[hb]
\begin{equation}\label{eqdiag:slicat2sat-objects}
\begin{tabular}{c}
\begin{tikzcd}[row sep=5ex, column sep = 6ex]
	\GG^\twocat  
			\ar[r, "\cod", thick] 
& \GG 
& \GG/G 
	\ar[l, "\dom_{G}" '] 
& \dernode{P_G} %
			\ar[l, derived, "h" '] 
			\ar[r, derived, "v"]
			\ar[lll, derived, bend right =20, "{\pbfunV}_G" ']
& \GG/G 
%
%
\\ % Row 2 
\Instcat_\predsig
				 \ar[r,				 "\labfunSig"	 ] 
				\ar[u, 				 "t^\predsig_{\_}"	] 
		& \carrop{\predsig}
					\ar[u, pos=0.5,				"\arfun"]     
		& \dernode{ \LDiagcat_G}
					\ar[l, derived,							"\labfunSke" ',		]
					\ar[u, derived, pos=0.5, 			"\bmap^G_{\_}",	]
		& \dernode{Q_G} %\underX{P_G}
					\ar[l, derived, pos=0.5,			"\senfun_G" '] % \underX{h}" ' ]  
					\ar[ru,  derived, 						"\modfun_G" '] % " \underX{v}" ]
					\ar[u, dotderived,						"!^\circ_G" ]
%					\ar[ulll, dotderived, bend right =12.5, yshift=-0.55ex]
%		&  \underX{\twix{P}} 
%		      \ar[u,  "\twix{v}"]
%		      \ar[]
\\  [-5pt]% Row 3
&&& \Dashv_G  
%
% two black pb
	% first the curved argument arrow 
	\ar["\comparrlabel " ', pos=0.2, from=2-4, to=1-1, dotderived, bend right =12.5, yshift=-0.55ex]
% now the pb stuff 
\ar[phantom, "~~\pbdiaglabelUD{}{1}", from=2-3, to=1-2,  pos=0.5 ]
\ar[phantom, "~~~~\pbdiaglabelUD{}{2}", from=3-4, to=2-3,  pos=0.5]
\ar["v_G%:=\ovr{!^\circ_G.\pbfunV}
", from=3-4, to=2-1, bend right = 4, dotDerived, pos=0.25] 
\ar["u_{G}" ', from=3-4, to=2-4,  derived, 				 pos=0.45]
\end{tikzcd}
%

%======== lower diagram
%
\\  [-10pt] % diagram with circles 
\begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.15ex}},
						row sep=4ex, column sep = 9ex]
t^\predsig_{\_} \ar[r] 
& \arfun^\predsig \ar[l,<-] 
& \bmap^G_{\_} \ar[l]
&   u_{G} % \DashvArrowObjX{G}
	\ar["\senfun_G^\uparrow" ',  l, derived] 
	\ar["\modfun_G^\uparrow",  r, derived]
	\ar["v_G^\uparrow" ', lll, derived,  bend right =25]
& \id_{\GG/G} 
%\\ [-15pt]
%&&&  u_{G} % \DashvArrowObjX{G}
%			\ar["\senfun^\uparrow" ',  lu, derived] 
%			\ar["\modfun^\uparrow",  ru, derived]
%			\ar[lllu, derived, "v_G^\uparrow"] % bend right =20, 

\end{tikzcd}
\end{tabular}
\end{equation}
\end{figure}
\end{mygroup}
\endinput
%\zd{This is the previous version}
% what is below print pout the previous veruosn 



% version before April 29
\begin{figure}[b]
\begin{tikzcd}[row sep=4ex, column sep = 6ex]
	\GG^\twocat  \ar[r, "\cod", thick] %\ar[ru, <-, derived]
	& \GG 		
	& \GG/G 
	\ar[l, "\dom_{G}" '] 
	& \dernode{\prodnodeS} %
	\ar[l, derived, "h" '] \ar[r, derived, "v"]
	\ar[lll, derived, bend right =20, "\pbfunV^S" ']
	& \GG/G_{S} 
	\\ % Row 2 
	\Instcat_\predsig
	\ar[r, "\labfunSig", thick ] 
	\ar[u,  "t^\predsig_{\_}"] 
	& \carrop{\predsig}
	\ar[u, "\arfun", pos=0.5]     
	& C_S \ar[l, "\labfunSke" ', thick]
	\ar[u,  "\bmap^S_{\_}", pos=0.5]
	& \dernode{\underprodS} \ar[l, derived, "\underX{h}" ', ]  \ar[r, derived,  "\underX{v}" ]
	\ar[u,derived,  "\btgluedS" , pos=0.5] 
	& \Instcat_S 
	\ar[u,  "t^S_{\_}"]
	%		\ar[ll, bend right=20, "\valfunX{t}" ']
	\\  % Bottom row
	& PB_S \ar[lu, derived] \ar[rru, derived]
	&& \DashvForIndecesX{S}\ar[ll, derived, rightarrowtail,  "\eqr" ']
	\ar[u, derived]
	\ar[lllu, dotted] \ar[lu, dotted] \ar[ru, dotted]
\end{tikzcd}
\caption{a previous version of  \cref{eqdiag:slicat2sat} above}
\end{figure}
%-----



%-------
\begin{figure}
\begin{equation}\label{eq:skeMor-semantics}
\begin{tikzcd}[row sep=4ex, column sep = 4ex]
\Instcat \ar[rr, "\labfun", thick ] 
			&& \carrop{\predsig}    
	&& C_S \ar[ll, "\labfunSke" ', thick]
			\ar[llll, bend right=20, "\valfunX{t}" ']
	&& C_{S'} \ar[ll, "f_C" ', ]
\\  % ROW 2 for middle derived nodes 
    & \dernode{\Preinst}\ar[ru, derived] 
    							\ar[lu, <-, dotDerived, "\#" ']    
								\ar[rd, phantom, gray,  "\text{[pb]}", pos=0.25]
	&&
	\dernode{\circ}\ar[lu, derived]  \ar[ru, <-, dotderived, "\#" ] 
							\ar[ll, dotderived, "\mathbf{!}" ', pos=0.75]
						\ar[ld, phantom, gray,  "\text{[pb]}", pos=0.25]
		&&
	\dernode{\circ}\ar[lu, derived]  \ar[ru, <-, dotderived, "\#" ] 
	\ar[ll, dotderived, "\mathbf{!}" ', pos=0.75]
	\ar[ld, phantom, gray,  "\text{[pb]}", pos=0.25]
\\  % Bottom row
		\GG^\twocat \ar[uu, <-, "t\_"] \ar[rr, "\cod", thick] \ar[ru, <-, derived]
&&	 \GG 				\ar[uu, <-, "\arfun", pos=0.2] 
&&   \GG/G \ar[uu, <-, "\bmap\_" ', pos=0.2] \ar[lu, <-, derived]
					  \ar[ll, "\dom_{G}" '] 
					  \ar[llll, bend left=15, "\twSubstX{t}" ']
&&
	 \GG/G_{S'} \ar[uu, <-, "\bmap'\_" ', pos=0.2]   \ar[lu, <-, derived]
	 				\ar[ll, "\GG/f_G" ']
	 				\ar[llllll, bend left=20, "\twSubstX{f_G^*(t)}"]
\end{tikzcd}
\end{equation}
\caption{this is an old version that may be useful a template b/c it has the middle row for pullbacks}
\end{figure}

%\END
\endinput
% the xypic version of the diagram
%%
%---
\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
			%\\  row 1
	\Instcat \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
	\\   % row 2
		& \Preinst        % Begin entry at (0,0)
			\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
			\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
			\ar@{}[dr]|{(PB)}
		&            % End entry
			\opX{\arrowcatBrackX{\GG}} 	% Begin entry at (1,0)
				\ar[d]^{\codop}            
	\\      % row 3                
		& \predsig   % Begin entry at (0,1)
			\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
			&                        % End entry
		\GGop  % Begin entry (3,3)
}               % Ending xymatrix




\endinput 
% the opposite version

\begin{equation}\label{eq:skedef}
	\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
		%\\  row 1
		\opX{Inst} \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
		\\   % row 2
		& \Preinst        % Begin entry at (0,0)
		\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
		\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
		\ar@{}[dr]|{(PB)}
		&            % End entry
		\arrowcatBrackX{\GG} 	% Begin entry at (1,0)
		\ar[d]^{\cod}            
		\\      % row 3                
		& \opX{\predsig}   % Begin entry at (0,1)
		\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
		&                        % End entry
		\GG                % Begin entry (1,1)
	}               % Ending xymatrix
\end{equation}

==> diagrams/slicat2sat.tex <==
% this macros (from Latex itself!) does not work! ??  \textuparrow
\begin{figure}
\begin{equation}\label{eqdiag:slicat2sat-arrows}
\begin{tabular}{c}
\begin{tikzcd}[row sep=5ex, column sep = 6ex]
	\GG^\twocat  
			\ar[r, "\cod", thick] 
& \GG 
& \GG/G 
	\ar[l, "\dom_{G}" '] 
& \dernode{P_G} %
			\ar[l, derived, "h" '] 
			\ar[r, derived, "v"]
			\ar[lll, derived, bend right =20, "\pbfunV" ']
& \GG/G 
%
%
\\ % Row 2 
\Instcat_\predsig
				 \ar[r,				 "\labfun_\predsig"	 ] 
				\ar[u, 				 "t^\predsig_{\_}"	] 
		& \carrop{\predsig}
					\ar[u, pos=0.5,				"\arfun"]     
		& \dernode{LD(G)}
					\ar[l, derived,							"\labfunSke" ',		]
					\ar[u, derived, pos=0.5, 			"\bmap_{\_}",	]
		& \underX{P_G}
					\ar[l, derived, pos=0.25,			" \underX{h}" ' ]  
					\ar[ru,  derived, 						" \underX{v}" ]
					\ar[u, dotderived,						"!^\circ_G" ]
		&  \underX{\twix{P}} 
		      \ar[u,  "\twix{v}"]
		      \ar[]

\\  % Row 3
& \Dashv_G  
&&  \GG/G' 
& \twix{P} \ar[l, "\twix{h}" ', pos=0.35] 
				\ar[uu, "\twix{v}"]   
%
%
\\   % Row 4
&
&    % \orangenode{\twix{\Dashv} }  %%_{\twix{}}
& \dernode{LD(G')}  
					\ar[u, derived,			"\bmapfun' "  '] 
& \underX{\twix{P}} 
				\ar[l, 					"\underX{\twix{h}}" '] 
				\ar[u, dotted,			"\twix{!^\circ}" ' ]
				\ar[uuu, "\underX{\twix{v}} " ',bend right =25, ]
%
\\ [-20pt] % row 5
&&\orangenode{\twix{\Dashv} }
%
% Diagonal Arrows for G'
\ar["f_*" ', from=3-4, to=1-3,  pos=0.1, orange]
\ar["\labfun' " ', derived, from=4-4, to=2-2]
\ar["u" ', from=4-4, to=2-3, oDashed]
\ar["\twix{!^\%}" ', from=3-5, to=1-4, odashed]
%
%  Diagonal arrows for Twist
\ar[from=4-5, to=2-4, oDashed,				"\gapnamegap{1}{\twix{!}}{-1.5}", pos=0.35]
\ar["\underX{???}" ', from=2-4, to=1-1, bend right = 8, dotderived, pos=0.15] 
%

% two black pb
\ar[from=2-3, to=1-2, phantom,				 "~~\pbdiaglabelUD{}{1}", pos=0.5 ]
\ar[from=3-2, to=2-2, phantom,				 "~~\pbdiaglabelUD{}{2}", pos=0.35]
\ar["\verif%:=\ovr{!^\circ_G.\pbfunV}
			" ', from=3-2, to=2-1, bend right = 10, dotDerived, pos=0.55] 
\ar[from=3-2, to=2-4,  dotDerived, 				"u_\Dashv", pos=0.45]

% orange pb2
\ar[from=5-3, to=2-3, phantom,				 				"~~\pbdiaglabelUDColor{}{2}{orange}", pos=0.2]
\ar[from=5-3, to=4-5, oDotted, 			"\gapnamegap{2}{\twix{u}}{-1}" , pos=0.15, ]
\ar["\ovr{\twix{!}}" ', from=5-3, to=3-2, odashed]
\ar[from=5-3, to=2-1, bend left = 15, oDotted, 			"\gapnamegap{-1}{\twix{\verif}}{0}", pos=0.5, ]


\end{tikzcd}
%
%
\\  [10pt] % diagram with circles 
\begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}},
						row sep=4ex, column sep = 8ex]
t^\predsig_{\_} \ar[r] 
& \arfun^\predsig \ar[l,<-] 
& \bmap^G_{\_} \ar[l]
& \DashvArrowObjX{G}
			\ar[l, derived] \ar[r, derived]
			\ar[lll, derived, bend right =20, "\verif_G" ']
& \id_{\GG/G} 
\end{tikzcd}
\end{tabular}
\end{equation}
\end{figure}

%\endinput
%\zd{This is the previous version}
% what is below print pout the previous veruosn 



% version before April 29
\begin{figure}[b]
\begin{tikzcd}[row sep=4ex, column sep = 6ex]
	\GG^\twocat  \ar[r, "\cod", thick] %\ar[ru, <-, derived]
	& \GG 		
	& \GG/G 
	\ar[l, "\dom_{G}" '] 
	& \dernode{\prodnodeS} %
	\ar[l, derived, "h" '] \ar[r, derived, "v"]
	\ar[lll, derived, bend right =20, "\pbfunV^S" ']
	& \GG/G_{S} 
	\\ % Row 2 
	\Instcat_\predsig
	\ar[r, "\labfun", thick ] 
	\ar[u,  "t^\predsig_{\_}"] 
	& \carrop{\predsig}
	\ar[u, "\arfun", pos=0.5]     
	& C_S \ar[l, "\labfunSke" ', thick]
	\ar[u,  "\bmap^S_{\_}", pos=0.5]
	& \dernode{\underprodS} \ar[l, derived, "\underX{h}" ', ]  \ar[r, derived,  "\underX{v}" ]
	\ar[u,derived,  "\btgluedS" , pos=0.5] 
	& \Instcat_S 
	\ar[u,  "t^S_{\_}"]
	%		\ar[ll, bend right=20, "\valfunX{t}" ']
	\\  % Bottom row
	& PB_S \ar[lu, derived] \ar[rru, derived]
	&& \DashvForIndecesX{S}\ar[ll, derived, rightarrowtail,  "\eqr" ']
	\ar[u, derived]
	\ar[lllu, dotted] \ar[lu, dotted] \ar[ru, dotted]
\end{tikzcd}
\caption{a previous version of  \cref{eqdiag:slicat2sat} above}
\end{figure}
%-----



%-------
\begin{figure}
\begin{equation}\label{eq:skeMor-semantics}
\begin{tikzcd}[row sep=4ex, column sep = 4ex]
\Instcat \ar[rr, "\labfun", thick ] 
			&& \carrop{\predsig}    
	&& C_S \ar[ll, "\labfunSke" ', thick]
			\ar[llll, bend right=20, "\valfunX{t}" ']
	&& C_{S'} \ar[ll, "f_C" ', ]
\\  % ROW 2 for middle derived nodes 
    & \dernode{\Preinst}\ar[ru, derived] 
    							\ar[lu, <-, dotDerived, "\#" ']    
								\ar[rd, phantom, gray,  "\text{[pb]}", pos=0.25]
	&&
	\dernode{\circ}\ar[lu, derived]  \ar[ru, <-, dotderived, "\#" ] 
							\ar[ll, dotderived, "\mathbf{!}" ', pos=0.75]
						\ar[ld, phantom, gray,  "\text{[pb]}", pos=0.25]
		&&
	\dernode{\circ}\ar[lu, derived]  \ar[ru, <-, dotderived, "\#" ] 
	\ar[ll, dotderived, "\mathbf{!}" ', pos=0.75]
	\ar[ld, phantom, gray,  "\text{[pb]}", pos=0.25]
\\  % Bottom row
		\GG^\twocat \ar[uu, <-, "t\_"] \ar[rr, "\cod", thick] \ar[ru, <-, derived]
&&	 \GG 				\ar[uu, <-, "\arfun", pos=0.2] 
&&   \GG/G \ar[uu, <-, "\bmap\_" ', pos=0.2] \ar[lu, <-, derived]
					  \ar[ll, "\dom_{G}" '] 
					  \ar[llll, bend left=15, "\twSubstX{t}" ']
&&
	 \GG/G_{S'} \ar[uu, <-, "\bmap'\_" ', pos=0.2]   \ar[lu, <-, derived]
	 				\ar[ll, "\GG/f_G" ']
	 				\ar[llllll, bend left=20, "\twSubstX{f_G^*(t)}"]
\end{tikzcd}
\end{equation}
\caption{this is an old version that may be useful a template b/c it has the middle row for pullbacks}
\end{figure}

%\END
\endinput
% the xypic version of the diagram
%%
%---
\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
			%\\  row 1
	\Instcat \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
	\\   % row 2
		& \Preinst        % Begin entry at (0,0)
			\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
			\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
			\ar@{}[dr]|{(PB)}
		&            % End entry
			\opX{\arrowcatBrackX{\GG}} 	% Begin entry at (1,0)
				\ar[d]^{\codop}            
	\\      % row 3                
		& \predsig   % Begin entry at (0,1)
			\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
			&                        % End entry
		\GGop  % Begin entry (3,3)
}               % Ending xymatrix




\endinput 
% the opposite version

\begin{equation}\label{eq:skedef}
	\xymatrix@C=4em{  % begins a xy matrix 2 x 2 
		%\\  row 1
		\opX{Inst} \ar[rdd]_{\plabel}\ar@{.>}[rd]|{\#}\ar[rrd]^{\pbind}
		\\   % row 2
		& \Preinst        % Begin entry at (0,0)
		\ar@{-->}[r]_{\pbind^\#} %{~~\bind^!}        
		\ar@{-->}[d]^{\plabel^\#} %{\plabel^!}       
		\ar@{}[dr]|{(PB)}
		&            % End entry
		\arrowcatBrackX{\GG} 	% Begin entry at (1,0)
		\ar[d]^{\cod}            
		\\      % row 3                
		& \opX{\predsig}   % Begin entry at (0,1)
		\ar[r]^{\arfun}            % Outgoing arrow at (0,1) going to the right, labelled \arfun
		&                        % End entry
		\GG                % Begin entry (1,1)
	}               % Ending xymatrix
\end{equation}

==> diagrams/table-sampleConstr-Old.tex <==

\begin{table}[h]
 %\begin{wraptable}{R}{0.35\textwidth}
 %\vspace{-1cm}
 \caption{Sample Constraints OLD \label{tab:sign-old}}
 \vspace{0.1cm} 
 \centering
 \begin{tabular}{|c|c|c|}
 \hline
 Name, $c$ & Arity shape, $S_c$ & Semantics for $t\models c$ (in FOL)
 \\ \hline \hline %\row 0
[1..*]	& \ArrowDiag
 			&  $\forall a\exists h\; r^t(a,h,b)$ %\wedge  r^t(a,h_2,b_2) \Rightarrow  b_1=b_2$  
\\   \hline  % row 1
[0..1] & \ArrowDiag
 			&  $ r^t(a,h_1,b_1)\wedge  r^t(a,h_2,b_2) \Rightarrow  b_1=b_2$
 \\ \hline % row 1'
[0..2] &  \ArrowDiag
 			&  % now its semantics
				$\begin{array}{l}
 					r^t(a,h_1,b_1)\wedge  r^t(a,h_2,b_2) \wedge r^t(a,h_3,b_3) \\ 
					\Rightarrow  \quad b_1=b_2 \vee b_2=b_3\vee b_1=b_3
				\end{array}$  % end semantics
\\  \hline  % row 2
[trans] & \LoopDiag 
			& $r^t(a_1,h_1,a_2) \wedge r^t(a_2,h_2,a_3) \Rightarrow \exists h\; r^t(a_1,h,a_3)$
\\  \hline % row 4 [or]
[or] & \SpanDiagHorizontally
		& $\forall a\in A^t\left( \exists h_1\, r_1^t(a,h_1,b_1) \vee \exists h_2\,r_2^t(a,h_2,b_2)\right)$
\\  \hline  % row 5 [id]
[id] & \LoopDiag
		&  $r^t=\id{(A^t)}$ (that is, $\forall a\in A^t\exists!h\;r^t(a,h,a)$)
   \\  \hline  % row 3*
[=$_2$] & \TwoParaArrowsDiag
    &  $r_1^t = r_2^t$ %$ \exists h_1\, r_1^t(a,h_1,b)\Leftrightarrow \exists h_2 r_2^t(a,h_2,b) $
\\  \hline  % row 4
[$=$] & \CommTriangleDiag
    &  $r_1^t.r_2^t = r_3^t$ %(which abbreviates a FOL formula)
 %    $\begin{array}{c}
%    	\text{ Conjunction of $[\subseteq]$ above and the folloiwng condition: }
%    	\\
%    	r^t(a,h, c) \Rightarrow \exists h_1\,r_1^t(a,h_1,b) \wedge  \exists h_2\,r_2^t(b,h_2,c) 
%    \end{array}$
\\  \hline  % row 5
$[\subseteq_2$] & \TwoParaArrowsDiag
&  $r_1^t \subseteq r_2^t$ %$ \exists h_1\, r_1^t(a,h_1,b)\Leftrightarrow \exists h_2 r_2^t(a,h_2,b) $
\\  \hline  % row 6
$[\subseteq_3]$ & \CommTriangleDiag
				& $\begin{array}{c}
					r_1^t.r_2^t \subseteq r_3^t   %\text{ (which abbreviates a FOL formula) }
				\end{array}$
\\  \hline  % row 7
$[\supseteq_3]$ & \CommTriangleDiag 
			& $\begin{array}{c}
				r_1^t.r_2^t \supseteq r_3^t   %\text{ (which abbreviates a FOL formula) }
				\end{array}$
\\    \hline  % end 
\end{tabular}
 % \vspace{-0.8cm}
 %\end{wraptable}
\end{table}

==> diagrams/twistedMorphDef--macros.tex <==

\newcommand{\twistedMorphDefTriplediag}{def}
% https://q.uiver.app/#q=WzAsMjUsWzAsMl0sWzEsMCwiTSIsWzEyLDYzLDUyLDFdXSxbMiwwLCJcXFBvYmoiLFsxMiw2Myw1MiwxXV0sWzEsMSwiUyIsWzEyLDYzLDUyLDFdXSxbMiwyLCJcXHR3aXhVe1B9X2YiXSxbMSwzLCJNJyIsWzExNSw3Myw0MCwxXV0sWzEsNCwiUyciLFsxMTUsNzMsNDMsMV1dLFsyLDQsIlxcUG9ialByaW0iLFsxMTUsNzMsNDAsMV1dLFszLDAsIlxcRGFzaHYiLFsxMiw2Myw1MiwxXV0sWzMsMiwiXFx0d2lzdGVkU2F0WGRue2Z9Il0sWzMsNCwiXFxEYXNodiciLFsxMTUsNzMsNDAsMV1dLFs1LDIsIkUiXSxbNiwzLCJNJyIsWzI0NywzOSw3NSwxXV0sWzcsMCwiTSIsWzAsNjAsNjAsMV1dLFs3LDQsIk0nIixbMTE1LDczLDQzLDFdXSxbOSwwLCJTIixbMCw2MCw2MCwxXV0sWzksNCwiUyciLFsxMTUsNzMsNDAsMV1dLFsxMCwxLCJTIixbMjQ3LDM5LDc1LDFdXSxbMTEsMCwiUCJdLFsxMywyLCJFIl0sWzExLDQsIlAnIl0sWzgsNSwiXFx0ZXh0e2EpfSJdLFsxMSw1LCJcXHRleHR7Yil9Il0sWzExLDIsIlxcdHdpeFV7UH1fZiJdLFszLDUsIlxcdGV4dHsqKX0gIl0sWzIsMywiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzIsMSwiIiwwLHsiY29sb3VyIjpbMTIsNjMsNTJdfV0sWzcsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFs3LDYsIiIsMCx7ImNvbG91ciI6WzExNSw3Myw0M119XSxbOCwyLCJyIiwyLHsiY29sb3VyIjpbMTIsNjMsNTJdfSxbMTIsNjMsNTIsMV1dLFs5LDQsInJfZiIsMl0sWzEwLDcsInInIiwyLHsiY29sb3VyIjpbMTE1LDczLDQwXX0sWzExNSw3Myw0MCwxXV0sWzQsMiwiIV4qX2YiLDAseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksOCwiXFxzYXRUb1NhdF4qX2YiLDIseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMCw2MCw2MCwxXV0sWzksMTAsIlxcc2F0VG9TYXRfKl5mIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fSxbMTE1LDczLDQwLDFdXSxbNCw4LCJcXHRleHR7W3BiXX0iLDEseyJjb2xvdXIiOlswLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fSxbMCw2MCw2MCwxXV0sWzQsMTAsIlxcdGV4dHtbcGJdfSIsMSx7ImNvbG91ciI6WzExNSw3Myw0MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX0sWzExNSw3Myw0MCwxXV0sWzgsMTEsImUiLDAseyJjb2xvdXIiOlsxMiw2Myw1Ml19LFsxMiw2Myw1MiwxXV0sWzEwLDExLCJlJyIsMix7ImNvbG91ciI6WzExNSw3Myw0MF19LFsxMTUsNzMsNDAsMV1dLFs1LDEsImZeKiIsMCx7ImN1cnZlIjotM31dLFszLDYsImZfKiIsMix7ImN1cnZlIjozfV0sWzksMTEsImVfZiJdLFs0LDMsIiIsMCx7ImNvbG91ciI6WzAsNjAsNjBdfV0sWzQsNSwiIiwwLHsiY29sb3VyIjpbMTE1LDczLDQwXX1dLFsxMiwxMywiZl4qIiwwLHsiY29sb3VyIjpbMjQ3LDM5LDc1XX1dLFsxMiwxNCwiIiwyLHsibGV2ZWwiOjIsImNvbG91ciI6WzI0NywzOSw3NV0sInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMTMsMTQsImZeeyoqfSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsxNSwxMywiXFx2RGFzaF97TVN9IiwyLHsiY29sb3VyIjpbMCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX0sWzAsNjAsNjAsMV1dLFsxNiwxNCwiXFx2RGFzaF97TSdTJ30iLDAseyJjb2xvdXIiOlsxMTUsNzMsNDBdfSxbMTE1LDczLDQwLDFdXSxbMTUsMTcsIiIsMCx7ImxldmVsIjoyLCJjb2xvdXIiOlsyNDcsMzksNzVdLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzE3LDE2LCJmXyoiLDAseyJjb2xvdXIiOlsyNDcsMzksNzVdfV0sWzE1LDE2LCJmX3sqKn0iLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMTUsMTQsIlxcdkRhc2hfe00nU31eZiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxOCwxOSwiXFx2RGFzaCIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMCwxOSwiXFx2RGFzaCciLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJiYXJyZWQifX19XSxbMjMsMTgsIiFfKl5mIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzIzLDIwLCIhXypeZiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImJhcnJlZCJ9fX1dLFsyMywxOSwiXFx0d2lzdGVkU2F0WGRue2Z9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiYmFycmVkIn19fV0sWzQsNywiIV8qXmYiLDIseyJjb2xvdXIiOlsxMTUsNzMsNDBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsxMTUsNzMsNDAsMV1dXQ==
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{M} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Pobj} \& \textcolor{rgb,255:red,210;green,86;blue,55}{\Dashv} \&\&\&\& \textcolor{rgb,255:red,214;green,92;blue,92}{M} \&\& \textcolor{rgb,255:red,214;green,92;blue,92}{S} \&\& P \\
	\& \textcolor{rgb,255:red,210;green,86;blue,55}{S} \&\&\&\&\&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{S} \\
	{} \&\& {\twixU{P}_f} \& {\twistedSatXdn{f}} \&\& E \&\&\&\&\&\& {\twixU{P}_f} \&\& E \\
	\& \textcolor{rgb,255:red,40;green,176;blue,28}{M'} \&\&\&\&\& \textcolor{rgb,255:red,172;green,166;blue,216}{M'} \\
	\& \textcolor{rgb,255:red,43;green,190;blue,30}{S'} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\PobjPrim} \& \textcolor{rgb,255:red,40;green,176;blue,28}{\Dashv'} \&\&\&\& \textcolor{rgb,255:red,43;green,190;blue,30}{M'} \&\& \textcolor{rgb,255:red,40;green,176;blue,28}{S'} \&\& {P'} \\
	\&\&\& {\text{*)} } \&\&\&\&\& {\text{a)}} \&\&\& {\text{b)}}
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=2-2]
	\arrow[draw={rgb,255:red,210;green,86;blue,55}, from=1-3, to=1-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=5-3, to=4-2]
	\arrow[draw={rgb,255:red,43;green,190;blue,30}, from=5-3, to=5-2]
	\arrow["r"', color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=1-3]
	\arrow["{r_f}"', from=3-4, to=3-3]
	\arrow["{r'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=5-3]
	\arrow["{!^*_f}", color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-3, to=1-3]
	\arrow["{\satToSat^*_f}"', color={rgb,255:red,214;green,92;blue,92}, dashed, from=3-4, to=1-4]
	\arrow["{\satToSat_*^f}", color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-4, to=5-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,214;green,92;blue,92}, draw=none, from=3-3, to=1-4]
	\arrow["{\text{[pb]}}"{description}, color={rgb,255:red,40;green,176;blue,28}, draw=none, from=3-3, to=5-4]
	\arrow["e", color={rgb,255:red,210;green,86;blue,55}, from=1-4, to=3-6]
	\arrow["{e'}"', color={rgb,255:red,40;green,176;blue,28}, from=5-4, to=3-6]
	\arrow["{f^*}", curve={height=-18pt}, from=4-2, to=1-2]
	\arrow["{f_*}"', curve={height=18pt}, from=2-2, to=5-2]
	\arrow["{e_f}", from=3-4, to=3-6]
	\arrow[draw={rgb,255:red,214;green,92;blue,92}, from=3-3, to=2-2]
	\arrow[draw={rgb,255:red,40;green,176;blue,28}, from=3-3, to=4-2]
	\arrow["{f^*}", draw={rgb,255:red,172;green,166;blue,216}, from=4-7, to=1-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=4-7, to=5-8]
	\arrow["{f^{**}}"', "\shortmid"{marking}, from=1-8, to=5-8]
	\arrow["{\vDash_{MS}}"', "\shortmid"{marking, text={rgb,255:red,214;green,92;blue,92}}, color={rgb,255:red,214;green,92;blue,92}, from=1-10, to=1-8]
	\arrow["{\vDash_{M'S'}}", color={rgb,255:red,40;green,176;blue,28}, from=5-10, to=5-8]
	\arrow[draw={rgb,255:red,172;green,166;blue,216}, Rightarrow, no head, from=1-10, to=2-11]
	\arrow["{f_*}", draw={rgb,255:red,172;green,166;blue,216}, from=2-11, to=5-10]
	\arrow["{f_{**}}", "\shortmid"{marking}, from=1-10, to=5-10]
	\arrow["{\vDash_{M'S}^f}"{description}, dashed, from=1-10, to=5-8]
	\arrow["\vDash", "\shortmid"{marking}, from=1-12, to=3-14]
	\arrow["{\vDash'}"', "\shortmid"{marking}, from=5-12, to=3-14]
	\arrow["{!_*^f}", "\shortmid"{marking}, from=3-12, to=1-12]
	\arrow["{!_*^f}"', "\shortmid"{marking}, from=3-12, to=5-12]
	\arrow["{\twistedSatXdn{f}}", "\shortmid"{marking}, from=3-12, to=3-14]
	\arrow["{!_*^f}"', color={rgb,255:red,40;green,176;blue,28}, dashed, from=3-3, to=5-3]
\end{tikzcd}

==> diagrams/twistedThProof.tex <==
%    cannot fidn the command \input{.... this diag}
\endinput
% [row sep=1.25ex, column sep=5ex]  https://q.uiver.app/?q=WzAsMTMsWzIsMCwiXFxHRyJdLFswLDEsIlBfUyJdLFs0LDEsIlBfe1MnfSJdLFsyLDEsIlxccHJvZEZ0d2lzdCJdLFswLDMsIlxcdW5kZXJwcm9kUyJdLFs0LDMsIlxcdW5kZXJwcm9kU3ByaW0iXSxbMiwzLCJcXHVuZGVycHJvZEZ0d2lzdCJdLFswLDUsIlBCX1MiXSxbMiw1LCJcXHR3aXh7UEJ9X2YiXSxbNCw1LCJQQl97Uyd9Il0sWzAsNywiXFxEYXNodl9TIl0sWzQsNywiXFxEYXNodl97Uyd9Il0sWzIsNywiXFxEYXNodl9mXntcXHR3aXh7fX0iXSxbMSwwLCJcXHBiZnVuViJdLFsyLDAsIlxccGJmdW5WJyIsMl0sWzMsMSwiKFxcdHdpeHtofS5mXkNfKiwgXFx0d2l4e3Z9KSIsMl0sWzMsMiwiKFxcdHdpeHtofSxcXHR3aXh7dn0uZl9HXiopIl0sWzQsMSwiW1xcYm1hcF97XFxffSwgXFx0bWFwX3tcXF99XSJdLFs1LDIsIltcXGJtYXAnX3tcXF99LFxcdG1hcCdfe1xcX31dIl0sWzYsMywiXFx0d2l4e3V9ICIsMCx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs2LDUsIihcXHVuZGVyWHtcXHR3aXh7aH19LFxcLFxcdW5kZXJYe1xcdHdpeHt2fX0uZl9JKSJdLFs2LDQsIihcXHVuZGVyWHtcXHR3aXh7aH19LmZeQyxcXCxcXHVuZGVyWHtcXHR3aXh7dn19KSIsMl0sWzgsNywidSIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs4LDksInUnIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzcsNCwiXFxvdmVybGluZXtcXGxhYmZ1bl9cXHByZWRzaWd9Il0sWzksNSwiXFxvdmVybGluZXtcXGxhYmZ1bidfXFxwcmVkc2lnfSJdLFs4LDYsIlxcb3ZlcmxpbmV7XFx0d2l4e1xcbGFiZnVuX1xccHJlZHNpZ319Il0sWzEwLDcsIlxcZXFyIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibW9ubyJ9fX1dLFsxMSw5LCJcXGVxciciLDAseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtb25vIn19fV0sWzEyLDgsIlxcdHdpeHtcXGVxcn0iLDAseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtb25vIn19fV0sWzEyLDEwLCJ1X1xcRGFzaHYiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTIsMTEsInUnX1xcRGFzaHYiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMywwLCJcXHZlcmlmIiwxXV0=
\[\begin{tikzcd}[row sep=1.25ex, column sep=5ex] 
	&& \GG \\
%\\
	{P_S} && \prodFtwist && {P_{S'}} \\
	\\
	\underprodS && \underprodFtwist && \underprodSprim \\
	\\
	{PB_S} && {{\twix{PB}}_f} && {PB_{S'}} \\
	\\
	{\Dashv_S} && {\Dashv_f^{\twix{}}} && {\Dashv_{S'}}
	\arrow["\pbfunV", from=2-1, to=1-3]
	\arrow["{\pbfunV'}"', from=2-5, to=1-3]
	\arrow["{(\twix{h}.f^C_*, \twix{v})}"', from=2-3, to=2-1]
	\arrow["{(\twix{h},\twix{v}.f_G^*)}", from=2-3, to=2-5]
	\arrow["{[\bmap_{\_}, \tmap_{\_}]}", from=4-1, to=2-1]
	\arrow["{[\bmap'_{\_},\tmap'_{\_}]}", from=4-5, to=2-5]
	\arrow["{\twix{u} }", dashed, from=4-3, to=2-3]
	\arrow["{(\underX{\twix{h}},\,\underX{\twix{v}}.f_I)}", from=4-3, to=4-5]
	\arrow["{(\underX{\twix{h}}.f^C,\,\underX{\twix{v}})}"', from=4-3, to=4-1]
%
	\arrow["u"', dashed, from=6-3, to=6-1]
	\arrow["{u'}", dashed, from=6-3, to=6-5]
	\arrow["{\overline{\labfun_\predsig}}", from=6-1, to=4-1]
	\arrow["{\overline{\labfun'_\predsig}}", from=6-5, to=4-5]
	\arrow["\overline{\twix{{\labfun_\predsig}}}", from=6-3, to=4-3]
	\arrow["\eqr", tail, from=8-1, to=6-1]
%
	\arrow["{\eqr'}", tail, from=8-5, to=6-5]
	\arrow["{\twix{\eqr}}", tail, from=8-3, to=6-3, shorten <= -2mm]
	\arrow["{u_\Dashv}"', dashed, from=8-3, to=8-1]
	\arrow["{u'_\Dashv}", dashed, from=8-3, to=8-5]
	\arrow["\verif", from=2-3, to=1-3, shorten <= -2mm]
\end{tikzcd}\]
\endinput


==> diagrams/twixlemmaArxiv/twistedDelta-Lemma.tex <==
\begin{equation}\label{eqdiag:cattyDiag2--withOk}
	\begin{tabular}{c}
		%	\twixlemmaDeltaCattyDiag  & 
		%   \twixlemmaDeltaCattyDiagCorollary
		\twixlemmaCattydiagTwoWithOk
	\end{tabular}
\end{equation}





\endinput






\newcommand{\twistedLemmaProofDefiningPBfunV}{
	% https://q.uiver.app/?q=WzAsOSxbNCwyLCJTIl0sWzQsMSwiXFxidWxsZXQiXSxbNCwwLCJcXGJ1bGxldCJdLFsyLDIsIlxcYnVsbGV0Il0sWzAsMiwiXFxidWxsZXQiXSxbMiwxLCJcXGNpcmMiXSxbMCwxLCJcXGNpcmMiXSxbMiwwLCJcXGNpcmMiXSxbMCwwLCJcXGNpcmMiXSxbMywwLCJoIiwyXSxbNCwzLCJnIl0sWzQsMCwiaCciLDIseyJjdXJ2ZSI6M31dLFsxLDAsInYiXSxbMiwxLCJ1IiwyXSxbMiwwLCJ2JyIsMCx7ImN1cnZlIjotMn1dLFs4LDcsIlxcYmFye1xcYmFyIGd9IiwwLHsiY29sb3VyIjpbMjM4LDc2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMjM4LDc2LDYwLDFdXSxbNywyLCIiLDIseyJjb2xvdXIiOlsyMzgsNzYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNSwzLCJcXHBiZnVudlh7fSh2LGgpIiwwLHsibGFiZWxfcG9zaXRpb24iOjQwLCJjb2xvdXIiOlsyMzgsNzYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyMzgsNzYsNjAsMV1dLFs1LDEsIiIsMix7ImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs2LDUsIlxcYmFyIGciLDAseyJjb2xvdXIiOlsyMzgsNzYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsyMzgsNzYsNjAsMV1dLFs4LDYsIiIsMSx7ImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDUsIlxcYmFyIHUiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNiw0LCJcXHBiZnVudlh7fSh2LGgnKSIsMCx7ImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzIzOCw3Niw2MCwxXV0sWzgsNCwiXFxwYmZ1bnZYe30odicsaCcpIiwyLHsiY3VydmUiOjIsImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzIzOCw3Niw2MCwxXV0sWzgsNSwiIiwwLHsiY29sb3VyIjpbMjM4LDc2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
	\begin{tikzcd}[ampersand replacement=\&]
		\circ \&\& \circ \&\& \bullet \\
		\circ \&\& \circ \&\& \bullet \\
		\bullet \&\& \bullet \&\& S
		\arrow["h"', from=3-3, to=3-5]
		\arrow["g", from=3-1, to=3-3]
		\arrow["{h'}"', curve={height=18pt}, from=3-1, to=3-5]
		\arrow["v", from=2-5, to=3-5]
		\arrow["u"', from=1-5, to=2-5]
		\arrow["{v'}", curve={height=-12pt}, from=1-5, to=3-5]
		\arrow["{\bar{\bar g}}", color={rgb,255:red,75;green,81;blue,231}, dotted, from=1-1, to=1-3]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dotted, from=1-3, to=1-5]
		\arrow["{\pbfunvX{}(v,h)}"{pos=0.4}, color={rgb,255:red,75;green,81;blue,231}, dashed, from=2-3, to=3-3]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dotted, from=2-3, to=2-5]
		\arrow["{\bar g}", color={rgb,255:red,75;green,81;blue,231}, dotted, from=2-1, to=2-3]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dashed, from=1-1, to=2-1]
		\arrow["{\bar u}"', dotted, from=1-3, to=2-3]
		\arrow["{\pbfunvX{}(v,h')}", color={rgb,255:red,75;green,81;blue,231}, dashed, from=2-1, to=3-1]
		\arrow["{\pbfunvX{}(v',h')}"', color={rgb,255:red,75;green,81;blue,231}, curve={height=12pt}, dashed, from=1-1, to=3-1]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dashed, from=1-1, to=2-3]
	\end{tikzcd}
}
%

==> diagrams/twixlemmaArxiv/twistedLemma--Proof.tex <==

% now this macros  is executed
	\vspace{-2.5mm}
\begin{equation*}\label{eqdiag:twistedLemma-Proof}
\begin{tabular}{c@{\hspace{-4ex}}c}
	\twixlemmaCattyDiag
& \twixlemmaDefiningPBfunV
\\
a)  lemma statement
& b) Construction of functor \frar{\pbfunvX{}}{\CC/\X\timm\CC/\X}{\arrowcatCCcong}
\end{tabular}
\end{equation*}

==> diagrams/twixlemmaArxiv/twistedLemma-original.tex <==
% we first define the macros for drawing the aig
\newcommand{\twistedLemmaDiag}{
\begin{tikzcd}[row sep=2ex, column sep=1.5ex, ampersand replacement=\&]
\CC/X \&\& \CC/X 
	\ar[rrrr, bend left=20, "f^*"] \&
\& \CC/X' 
	\ar[llll, bend right =20, "f_*" '] \&\& \CC/X'
\\ [-2.5pt]
\&\dernode{P}
	\ar[lu, notderived, "h" '] 
	\ar[ru, notderived, "v"] 
\&\& \dernode{\twistedX{P}}
	\ar[lu, notderived, "\twistedX{v}" ']
	\ar[ru, notderived, "\twistedX{h}"]  
	\ar[ll, derived, "!" '] 	\ar[rr, derived, "!'" ]
\&\& \dernode{P'} 
	\ar[lu, notderived, "h'" '] 
	\ar[ru, notderived, "v'"] \&
\\ [2.5pt]
\&\&\& \CC^\twocat  
	\ar[llu, <-, pos=0.35, "\pbfunV"] 
	\ar[rru, <-, "\pbfunV" ', pos=0.35 ]  \&\&\&
\\
\&\&\&\CC 
	\ar[uuulll, <-, bend left =25, "\dom_X"] 
	\ar[uuurrr, <-, bend right =25, "\dom_{X'}" '] 
	\ar[u, <-, "\cod"]
\end{tikzcd}
}
% now this macros  is executed
%\begin{equation}\label{eqdiag:twistedLemma}
\twistedLemmaDiag
%\end{equation}

==> diagrams/twixlemmaArxiv/twistedLemma.tex <==
%---------  The catty face diagram 
%
\begin{mygroup}
\renewcommand{\arrowcatCCcong}{\arrowcatX{\CC}}

 %\begin{figure}[hb]
% Old Catty lemma  b/c the NEW one is wrong
\begin{equation}\label{eqdiag:cattyDiag1}
	\twixlemmaCattydiagOne
\end{equation}
%\end{fogure}
\end{mygroup}

\endinput


% --- OLd version 
\newcommand{\twistedLemmaDiag}{
\begin{tikzcd}[row sep=2ex, column sep=2.5ex, ampersand replacement=\&]
\CC/\X \&
\& \CC/\X 
		\ar[rr, bend left=10, "f^*", <-] \&
\& \CC/\X' 
		\ar[from=1-7, to=1-1,  bend right =20, "f_*" ', <-]
 \&\& \CC/\X'
\\ [-2.5pt]
\&\dernode{P}
		\ar[lu, notderived, "h" '] 
		\ar[ru, notderived, "v"] 
\&\& \dernode{\twix{P}}
		\ar[lllu, dotted, "\gapnamegap{-1.5}{\twix{h}}{1}" ', pos=0.15, bend right = 10]
		\ar[ru, dotted, "\gapnamegap{1}{\twix{v}}{-1.5}", pos=0.3, shorten=-1ex]  
		\ar[ll, derived, "{(1_\hind, f^*)}" '] 	
		\ar[rr, derived, "{(f_*, 1_\vind)} "  ]
\&\& \dernode{P'} 
		\ar[lu, notderived, "\gapnamegap{-1}{v'}{1}" ' , pos=0.15, shorten=-1ex] 
		\ar[ru, notderived, "\gapnamegap{1}{h'}{-1.5} ", pos=0.25] 
\\ [2.5pt]
\&\&\& \arrowcatCCcong
		\ar[llu, <-, pos=0.35, "\pbfunvX{\X}"] 
		\ar[rru, <-, "\pbfunvX{\X'}" ', pos=0.35 ]  \&\&\&
\\
\&\&\&\CC 
		\ar[uuulll, <-, bend left =25, "\dom_\X"] 
		\ar[from=1-7, to=4-4, bend left =25, "\dom_{\X'}"] 
		\ar[u, <-, "\cod"]
	\end{tikzcd}
}
 %% -- > NEW version 
 \newcommand{\twistedLemmaDiagNEW}{
 	\begin{tikzcd}[row sep=4ex, column sep=4ex, ampersand replacement=\&]
 		\CC/\X \&
 		\& \CC/\X 
 		\ar[from=1-7, to=1-3, bend right=15, "f^*" '] \&
 		\& \CC/\X' 
 		\ar[from=1-1, to=1-5,  bend left =15, "f_*" ]
 		\&\& \CC/\X'
 		\\ [-2.5pt]
 \&\dernode{P}
 		\ar[lu, notderived, "h" '] 
 		\ar[ru, notderived, "v"] 
 \&\& \dernode{\twix{P}}
 		\ar[lllu, dotted, "\gapnamegap{-1.5}{\twix{h}}{1}" ', pos=0.1, bend right = 10]
 		\ar[rrru, dotted, "\gapnamegap{1}{\twix{v}}{-1.5}", pos=0.1, bend left = 10, shorten=-1ex]  
 		\ar[ll, derived, "{(1_\hind, f^*)}" ', pos=0.65] 	
 		\ar[rr, derived, "{(f_*, 1_\vind)} " , pos=0.65 ]
 \&\& \dernode{P'} 
 		\ar[lu, notderived, "\gapnamegap{-1}{h'}{1}" ' , pos=0.15, shorten=-1ex] 
 		\ar[ru, notderived, "\gapnamegap{1}{v'}{-1.5} ", pos=0.25] 
 		\\ [2.5pt]
 \CC
 		\ar[to=3-1, from=1-1, "{\dom^\hind_\X}" ']
 		\ar[to=3-1, from=1-5, "{\dom^\hind_{\X'}}" ', pos = 0.8, dotted]
 		\ar[to=3-1, from=3-4, "{\cod}" ', ]
 		%
\& \& \& \arrowcatCCcong
 		\ar[llu, <-, pos=0.35, "\pbfunvX{\X}" '] 
 		\ar[rru, <-, "\pbfunvX{\X'}" , pos=0.35 ]
 \&\&\& \CC
  		\ar[to=3-7, from=1-7, "{\dom^\vind_{\X'}}"]
 		\ar[to=3-7, from=1-3, "{\dom^\vind_{\X}}", pos = 0.8, dotted]
		\ar[to=3-7, from=3-4, "{\dom}", ]
 	\end{tikzcd}
 }
 

%
	\begin{equation}\label{eqdiag:twistedLemmaNEW}
		\twistedLemmaDiagNEW
	\end{equation}
%\end{figure}


\newcommand{\twistedLemmaProofDefiningPBfunV}{
	% https://q.uiver.app/?q=WzAsOSxbNCwyLCJTIl0sWzQsMSwiXFxidWxsZXQiXSxbNCwwLCJcXGJ1bGxldCJdLFsyLDIsIlxcYnVsbGV0Il0sWzAsMiwiXFxidWxsZXQiXSxbMiwxLCJcXGNpcmMiXSxbMCwxLCJcXGNpcmMiXSxbMiwwLCJcXGNpcmMiXSxbMCwwLCJcXGNpcmMiXSxbMywwLCJoIiwyXSxbNCwzLCJnIl0sWzQsMCwiaCciLDIseyJjdXJ2ZSI6M31dLFsxLDAsInYiXSxbMiwxLCJ1IiwyXSxbMiwwLCJ2JyIsMCx7ImN1cnZlIjotMn1dLFs4LDcsIlxcYmFye1xcYmFyIGd9IiwwLHsiY29sb3VyIjpbMjM4LDc2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fSxbMjM4LDc2LDYwLDFdXSxbNywyLCIiLDIseyJjb2xvdXIiOlsyMzgsNzYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNSwzLCJcXHBiZnVudlh7fSh2LGgpIiwwLHsibGFiZWxfcG9zaXRpb24iOjQwLCJjb2xvdXIiOlsyMzgsNzYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyMzgsNzYsNjAsMV1dLFs1LDEsIiIsMix7ImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRvdHRlZCJ9fX1dLFs2LDUsIlxcYmFyIGciLDAseyJjb2xvdXIiOlsyMzgsNzYsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19LFsyMzgsNzYsNjAsMV1dLFs4LDYsIiIsMSx7ImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs3LDUsIlxcYmFyIHUiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbNiw0LCJcXHBiZnVudlh7fSh2LGgnKSIsMCx7ImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzIzOCw3Niw2MCwxXV0sWzgsNCwiXFxwYmZ1bnZYe30odicsaCcpIiwyLHsiY3VydmUiOjIsImNvbG91ciI6WzIzOCw3Niw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzIzOCw3Niw2MCwxXV0sWzgsNSwiIiwwLHsiY29sb3VyIjpbMjM4LDc2LDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV1d
	\begin{tikzcd}[ampersand replacement=\&]
		\circ \&\& \circ \&\& \bullet \\
		\circ \&\& \circ \&\& \bullet \\
		\bullet \&\& \bullet \&\& S
		\arrow["h"', from=3-3, to=3-5]
		\arrow["g", from=3-1, to=3-3]
		\arrow["{h'}"', curve={height=18pt}, from=3-1, to=3-5]
		\arrow["v", from=2-5, to=3-5]
		\arrow["u"', from=1-5, to=2-5]
		\arrow["{v'}", curve={height=-12pt}, from=1-5, to=3-5]
		\arrow["{\bar{\bar g}}", color={rgb,255:red,75;green,81;blue,231}, dotted, from=1-1, to=1-3]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dotted, from=1-3, to=1-5]
		\arrow["{\pbfunvX{}(v,h)}"{pos=0.4}, color={rgb,255:red,75;green,81;blue,231}, dashed, from=2-3, to=3-3]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dotted, from=2-3, to=2-5]
		\arrow["{\bar g}", color={rgb,255:red,75;green,81;blue,231}, dotted, from=2-1, to=2-3]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dashed, from=1-1, to=2-1]
		\arrow["{\bar u}"', dotted, from=1-3, to=2-3]
		\arrow["{\pbfunvX{}(v,h')}", color={rgb,255:red,75;green,81;blue,231}, dashed, from=2-1, to=3-1]
		\arrow["{\pbfunvX{}(v',h')}"', color={rgb,255:red,75;green,81;blue,231}, curve={height=12pt}, dashed, from=1-1, to=3-1]
		\arrow[color={rgb,255:red,75;green,81;blue,231}, dashed, from=1-1, to=2-3]
	\end{tikzcd}
}
%

==> diagrams/twoPBsquares4sig.tex <==
\newcommand{\twoPBsquaresFromCsig}{
% https://q.uiver.app/#q=WzAsOCxbMCwwLCJcXGFycm93Y2F0ZGVsdGFHRyJdLFsyLDAsIlxcR0ciXSxbNCwwLCJcXEdHL0ciXSxbMCw0LCJcXE9Lb2JqIl0sWzIsNCwiXFxjYXJyb3B7XFxjc2lnfSJdLFszLDIsIlxcTER4e0d9IixbMjIyLDczLDQ4LDFdXSxbMSwyLCJcXG9rVGFyZ2V0c2lnIixbMjIyLDczLDQ4LDFdXSxbNywxXSxbMywwLCJcXHRtYXBmdW5zaWciLDFdLFswLDEsIlxcY29kIl0sWzMsNCwiXFxlbGxYe1xcY3NpZ30iXSxbMyw2LCJcXG9rX1xcY3NpZyIsMCx7ImNvbG91ciI6WzIyMiw3Myw0OF19LFsyMjIsNzMsNDgsMV1dLFs2LDAsIiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs2LDQsIiIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFs2LDEsIlxcdGV4dHtbcGJdfV9cXGNzaWciLDEseyJsYWJlbF9wb3NpdGlvbiI6MzAsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDEsIlxcZG9tX3tHfSIsMl0sWzUsMiwiXFxibWFwZnVuWHtHfSIsMix7ImNvbG91ciI6WzIyMiw3Myw0OF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzIyMiw3Myw0OCwxXV0sWzUsMSwiXFx0ZXh0e1twYl19X3tHfSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo0MCwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsNCwiXFxlbGxYe0d9IiwwLHsibGFiZWxfcG9zaXRpb24iOjMwLCJjb2xvdXIiOlsyMjIsNzMsNDhdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFsyMjIsNzMsNDgsMV1dLFs0LDEsIlxcYXJmdW4iLDEseyJsYWJlbF9wb3NpdGlvbiI6NjB9XSxbMCwxLCJcXHRleHR7W2ZpYl19IiwxLHsib2Zmc2V0IjozLCJjb2xvdXIiOlszMzksNzUsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFszMzksNzUsNjAsMV1dLFs2LDQsIlxcdGV4dHtbZmliXX0iLDEseyJvZmZzZXQiOi00LCJjb2xvdXIiOlsyMjIsNzMsNDhdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsyMjIsNzMsNDgsMV1dLFsyLDEsIlxcdGV4dHtbZmliXX0iLDEseyJvZmZzZXQiOi0yLCJjb2xvdXIiOlszMzksNzUsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFszMzksNzUsNjAsMV1dLFs1LDQsIlxcdGV4dHtbZmliXX0iLDIseyJvZmZzZXQiOi0xLCJjb2xvdXIiOlsyMjIsNzMsNDhdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19LFsyMjIsNzMsNDgsMV1dXQ==
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\arrowcatdeltaGG \&\& \GG \&\& {\GG/G} \\
	\&\&\&\&\&\&\& {} \\
	\& \textcolor{rgb,255:red,33;green,87;blue,212}{\okTargetsig} \&\& \textcolor{rgb,255:red,33;green,87;blue,212}{\LDx{G}} \\
	\\
	\OKobj \&\& {\carrop{\csig}}
	\arrow["\tmapfunsig"{description}, from=5-1, to=1-1]
	\arrow["\cod", from=1-1, to=1-3]
	\arrow["{\ellX{\csig}}", from=5-1, to=5-3]
	\arrow["{\ok_\csig}", color={rgb,255:red,33;green,87;blue,212}, from=5-1, to=3-2]
	\arrow[dashed, from=3-2, to=1-1]
	\arrow[dashed, from=3-2, to=5-3]
	\arrow["{\text{[pb]}_\csig}"{description, pos=0.3}, draw=none, from=3-2, to=1-3]
	\arrow["{\dom_{G}}"', from=1-5, to=1-3]
	\arrow["{\bmapfunX{G}}"', color={rgb,255:red,33;green,87;blue,212}, dashed, from=3-4, to=1-5]
	\arrow["{\text{[pb]}_{G}}"{description, pos=0.4}, draw=none, from=3-4, to=1-3]
	\arrow["{\ellX{G}}"{pos=0.3}, color={rgb,255:red,33;green,87;blue,212}, dashed, from=3-4, to=5-3]
	\arrow["\arfun"{description, pos=0.6}, from=5-3, to=1-3]
	\arrow["{\text{[fib]}}"{description}, shift right=3, color={rgb,255:red,230;green,76;blue,130}, draw=none, from=1-1, to=1-3]
	\arrow["{\text{[fib]}}"{description}, shift left=4, color={rgb,255:red,33;green,87;blue,212}, draw=none, from=3-2, to=5-3]
	\arrow["{\text{[fib]}}"{description}, shift left=2, color={rgb,255:red,230;green,76;blue,130}, draw=none, from=1-5, to=1-3]
	\arrow["{\text{[fib]}}"', shift left=1, color={rgb,255:red,33;green,87;blue,212}, draw=none, from=3-4, to=5-3]
\end{tikzcd}
}

\begin{equation}\label{eqdiag:twoPBsquares4sig}
	\twoPBsquaresFromCsig
\end{equation}

==> diagrams/xxx-inArr---backup.tex <==
% https://q.uiver.app/?q=WzAsMTEsWzMsMSwiIV9HXlxcY2lyYyJdLFs0LDEsIlxcaWRfe1xcR0cvR30iXSxbMiwxLCJcXGJtYXBmdW5eRyJdLFsxLDIsIlxcYXJmdW5eXFxwcmVkc2lnIl0sWzAsMiwiXFx0bWFwZnVuXlxccHJlZHNpZyJdLFsxLDAsIlxcc2F0YXNhcnJvd3tHfSJdLFsyLDMsIlxcYm1hcGZ1bl57Ryd9Il0sWzQsMywiXFxpZF97XFxHRy9HJ30iXSxbMywzLCIhXlxcY2lyY197Ryd9Il0sWzEsNCwiXFxzYXRhc2Fycm93X3tHJ30iXSxbMywyLCJcXHR3aXh7XFxzYXRhc2Fycm93fV9mIl0sWzAsMSwiIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzAsMiwiIiwyLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzIsM10sWzMsNF0sWzUsNCwidmVyX0ciLDJdLFs1LDIsIih1XnsyMX1fRywhX0deXFxjaXJjLmgpIiwwLHsibGFiZWxfcG9zaXRpb24iOjEwMH1dLFs1LDEsIihcXHNhdGFzYXJyb3dfRy52LFxcLHYpIiwwLHsibGFiZWxfcG9zaXRpb24iOjcwLCJjdXJ2ZSI6LTF9XSxbNiwzXSxbOCw2LCIiLDIseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOCw3LCIiLDAseyJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbOSw0LCJ2ZXJfe0cnfSJdLFs5LDZdLFs2LDIsIih1XnsxMX1fe0dHJ30sXFwsZl8qKSIsMCx7ImNvbG91ciI6WzUsODEsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19LFs1LDgxLDYwLDFdXSxbNywxLCIoZl4qLFxcLCBmXiopIiwyLHsiY29sb3VyIjpbNSw4MSw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzUsODEsNjAsMV1dLFsxMCw2LCIiLDIseyJjb2xvdXIiOls1LDgxLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZG90dGVkIn19fV0sWzEwLDEsIiIsMix7ImNvbG91ciI6WzUsODEsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkb3R0ZWQifX19XSxbMTAsOSwiIiwwLHsiY3VydmUiOjQsImNvbG91ciI6WzUsODEsNjBdLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifX19XSxbMTAsNSwiKFxcb3Zye1xcdHdpeHshfX0sXFwsIFxcdHdpeHshfV5cXCUgICkiLDAseyJsYWJlbF9wb3NpdGlvbiI6MTAwLCJvZmZzZXQiOjIsImN1cnZlIjotNCwiY29sb3VyIjpbNSw4MSw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzUsODEsNjAsMV1dLFs5LDcsIiIsMix7ImN1cnZlIjoxfV1d
\begin{tikzcd}[ampersand replacement=\&]
	\&  \id_{\Dashv_G}   %{\satasarrow{G}} 
	\\
	\&\&{\bmapfun^G} 
	\& {!_G^\circ} 
	\& {\id_{\GG/G}} 
	\\   %Row 3
	{\tmapfun^\predsig} 
	\& {\arfun^\predsig}
	\&	\& {\orangenode{\satasarrow{{}}_f}}
	\\
	\&\& {\bmapfun^{G'}} 
	\& {!^\circ_{G'}} 
	\& {\id_{\GG/G'}} 
	\\
	\&  {\satasarrow{G'}}
	\arrow[dashed, from=2-4, to=2-5]
	\arrow[dashed, from=2-4, to=2-3]
	\arrow[from=2-3, to=3-2]
	\arrow[from=3-2, to=3-1]
	\arrow["{ver_G}"', from=1-2, to=3-1]
	\arrow["{(u^{21}_G,!_G^\circ.h)}"{pos=1}, from=1-2, to=2-3]
	\arrow["{\idtoidX{G}}"{pos=0.7}, curve={height=-6pt}, from=1-2, to=2-5]
	\arrow[from=4-3, to=3-2]
	\arrow[dashed, from=4-4, to=4-3]
	\arrow[dashed, from=4-4, to=4-5]
	\arrow["{ver_{G'}}", from=5-2, to=3-1]
	\arrow[from=5-2, to=4-3]
	\arrow["{(u^{11}_{GG'},\,f_*)}", color={rgb,255:red,236;green,84;blue,70}, dashed, from=4-3, to=2-3]
	\arrow["{(f^*,\, f^*)}"', color={rgb,255:red,236;green,84;blue,70}, dashed, from=4-5, to=2-5]
	\arrow[color={rgb,255:red,236;green,84;blue,70}, dotted, from=3-4, to=4-3]
	\arrow[color={rgb,255:red,236;green,84;blue,70}, dotted, from=3-4, to=2-5]
	\arrow[color={rgb,255:red,236;green,84;blue,70}, curve={height=24pt}, dashed, from=3-4, to=5-2]
	\arrow["{(\ovr{\twix{!}^\%}, \twix{!}^\%  )}"{pos=0.75}, shift right=2, color={rgb,255:red,236;green,84;blue,70}, curve={height=-24pt}, dashed, from=3-4, to=1-2]
	\arrow[curve={height=6pt}, from=5-2, to=4-5]
\end{tikzcd}
}

==> figures/insert-ex3pb.tex <==
\begin{figure}
	\centering
\includegraphics[width=1.\linewidth
%height=1.\textheight
]
{figures/pbStories-threePBsDOSketch}	
\caption{Diagram Chasing}
\label{fig:ex3pb}
\end{figure}

\endinput

pbStories-threePBsDOSketch.pdf

\begin{figure}
	\centering
	\subfloat[Categorical notation\label{fig:univPBProp:1}]{
%	\begin{subfigure}[b]{0.35\linewidth}
				\centering
				\parbox{0.35\linewidth}{
\input{diagrams/pb}
}
}\quad
%	\end{subfigure}
	\subfloat[Sketch with operation labels\label{fig:univPBProp:2}]{
%\begin{subfigure}[b]{0.64\linewidth}
				\centering
\includegraphics[width=0.64\linewidth]{figures/pbStories-threePBsDOSketch}
}\\
%	\end{subfigure}
	\subfloat[Workflow(CHANGE GREEN TO BLUE)\label{fig:univPBProp:3}]{
%	\begin{subfigure}[b]{\linewidth}
	\centering
		\includegraphics[width=0.8\linewidth]{figures/pbStories-threePBsWorkflow.pdf}
}
%	\end{subfigure}
	\caption{Diagram Chasing}
	\label{fig:ex3pb}
\end{figure}

%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{0.8\linewidth}
%		\centering
%		\parbox{\linewidth}{
%			\input{diagrams/pb}
%		}
%		\caption{Categorical notation}
%		\label{fig:univPBProp:1}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.7\linewidth}
%		\centering
%		\includegraphics[width=0.8\linewidth]{figures/ThreePullbacksDOSketch.pdf}
%		\caption{DO-Sketch}
%		\label{fig:univPBProp:2}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.7\linewidth}
%		\centering
%		\includegraphics[width=0.8\linewidth]{figures/DOWorkflow2}
%		\caption{Workflow}
%		\label{fig:univPBProp:3}
%	\end{subfigure}
%	\caption{Diagram Chasing \zd{Operation invokations in B and C are to be named equally: either a,b,c in both or 1,2,3 in both. probbaly a,b,c would be betetr to distinguish operation diagrams from predicate diagrams}}
%	\label{fig:ex3pb}
%\end{figure}


==> figures/signature4pbm.tex <==
\begin{figure}[h]
	\centering
	\begin{tabular}{cccc}
		\parbox{0.25\linewidth}{\centering
			$\xymatrix @C=0.5em {
				\monicpred & & \commsqpred \\
				&	\pbmpred \ar@<+1ex>[ul]^{p_1} \ar@<-1ex>[ul]_{p_2}	 \ar[ur]_{p}	&
			}$
		} % end parbox
		& \parbox{0.1\linewidth}{\centering
			\includegraphics[width=0.65\linewidth]{pdfs/pbStories-arityArrow}
		} % end parbox
		& \parbox{0.25\linewidth}{\centering
			\includegraphics[width=0.95\linewidth]{pdfs/pbStories-arityPB}
		} % end parbox
		&  \parbox{0.25\linewidth}{\centering
			\includegraphics[width=0.95\linewidth]{pdfs/pbStories-aritySquare.pdf}
		} % end parbox
		\\ [-10pt] 
		a) Category ${\predsig_{\mathsf{pbm}}}$
		& b1) Arity $\monicpred^\arfun$
		& b2) Arity $\pbmpred^\arfun$
		& b3) Arity $\commsqpred^\arfun$
	\end{tabular}
	\caption{A sample signature \predsigpbm}
	\label{fig:predsigpbm}
\end{figure}


==> genMacros/4newTheorem-myXXX.tex <==
% All the macros for creating Defitions, Theorems, Proposition etc.
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
%\newtheorem{lemma}{Lemma}


%\newtheorem{example}{\bf Example}
%\newtheorem{remark}{\bf\em Remark}
\newtheorem{corollary}{Corollary}
%\theoremstyle{acmplain}
\newtheorem{fact}{Fact}
%\newtheorem{myconj}{Conjecture}
%\newtheorem{mylemma}{\bf Lemma}
%\newtheorem{myclaim}{Claim}
%\newtheorem{mycorr}{Corollary}
%\newtheorem{myparadox}{Paradox}
%\newtheorem{coro}{\bf Corollary}


\theoremstyle{definition}
\newtheorem{construction}{Construction}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
%\newtheorem{myaxiom}{Axiom}
%\newtheorem{myprinc}{Principle}
%\newtheorem{myobs}{Observation}
%\newtheorem{myreq}{Requirement}
%\newtheorem{myremark}{Remark}



\theoremstyle{remark}
%\newtheorem{example}{Example}
%\newtheorem{remark}{Remark}
%\newtheorem{myconv}{Convention}
%\newtheorem{myexerc}{Exercise}

%TODO
%\newcounter{constrCount}
%\newcounter{conjCount}

%\newtheorem{construct}[constrCount]{Construction}
%\theoremstyle{plain}\newtheorem{conjecture}[constrCount]{Conjecture} 




\newenvironment{mydef}[1][]
{
\ifthenelse{\equal{#1}{}}{ \begin{definition}  }{ \begin{definition}[{#1}]  }%
}
{
\end{definition} 
}


\newenvironment{myprop}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{prop} \ }{ \begin{prop}[{#1}] }%	
}
{\end{prop}}

%\newenvironment{mylem}[1][]
%{
%	\ifthenelse{\equal{#1}{}}{ \begin{lemma} \ }{ \begin{lemma}[{#1}] }%	
%		}
%		{\end{lemma}}



\newenvironment{mythm}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{theorem} \ }{ \begin{theorem}[{#1}] }%	
		}
		{\end{theorem}}


%\newenvironment{myfact}[1][]
%{
%	\ifthenelse{\equal{#1}{}}{ \begin{fact} \ }{ \begin{fact}[{#1}] }%	
%}
%{\end{fact}}

%\newtheorem{myfact}{Fact.}

\newenvironment{mylem}[1][]
{
\ifthenelse{\equal{#1}{}}{ \begin{lemma} \ }{ \begin{lemma}[{#1}] }%	
}
{\end{lemma}
}

%\newenvironment{mylem}[1]{\begin{lemma}[#1]} {\end{lemma}}

\newenvironment{mycor}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{corollary} \ }{ \begin{corollary}[{#1}] }%	
}
{\end{corollary}}


\newenvironment{myexa}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{example}[] \ }{ \begin{example}[{#1}] }%	
}
{\end{example}}



\newenvironment{myrem}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{remark}[] \ }{ \begin{remark}[{#1}] }%	
}
{\end{remark}}

\newenvironment{myconstr}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{construct}[] \ }{ \begin{construct}[{#1}] }%	
}
{\end{construct}}

\newenvironment{myfact}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{fact}[] \ }{ \begin{fact}[{#1}] }%	
		}
		{\end{fact}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% == my font discipline for defs for Springer ==

%-- doesn't worl for Compisitinality
%\newenvironment{defin}[1][]{\ifthenelse{\equal{#1}{}}{\definition}{\definition[#1]}\rm}{\enddefinition}
%\newenvironment{propo}[1][]{\ifthenelse{\equal{#1}{}}{\proposition}{\proposition[#1]}\rm}{\endproposition}
%\newenvironment{remar}[1][]{\ifthenelse{\equal{#1}{}}{\remark}{\remark[#1]}\rm}{\endremark}
% \newtheorem{defin}{Definition}
% \newtheorem{corol}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{propo}{Proposition}
%\newtheorem{remark}{\textit{Remark}}
% \newtheorem{example}{Example}

%% ATTENTION PLS !
%  for Elsevieer, the above macros don't work, but versions below do work
% \let\oldexample=\example
% \let\endoldexample=\endexample
% \renewenvironment{example}{\vspace{-0.6em}\begin{oldexample}}{\end{oldexample}\vspace{-0.35em}}

% \let\olddefin=\defin
% \let\endolddefin=\enddefin
% \renewenvironment{defin}{\vspace{-0.6em}\begin{olddefin}}{\end{olddefin}\vspace{-0.5em}}

% \let\oldpropo=\propo
% \let\endoldpropo=\endpropo
% \renewenvironment{propo}{\vspace{-0.6em}\begin{oldpropo}}{\end{oldpropo}\vspace{-0.5em}}

% \let\oldrema=\rema
% \let\endoldrema=\endrema
% \newenvironment{rema}{\vspace{-0.6em}\begin{oldrema}}{\end{oldrema}\vspace{-0.5em}}

% \let\oldcorol=\corol
% \let\endoldcorol=\endcorol
% \newenvironment{corol}{\vspace{-0.6em}\begin{oldcorol}}{\end{oldcorol}\vspace{-0.5em}}

% \let\oldtheorem=\theorem
% \let\endoldtheorem=\endtheorem
% \renewenvironment{theorem}{\vspace{-0.6em}\begin{oldtheorem}}{\end{oldtheorem}\vspace{-



==> genMacros/4textarrows-Nov28.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Arrows in diagrams and formulas
% normal functional arrow f: X-->Y
\newcommand{\frar}[3]{\ensuremath{ #1{:}\;#2\rightarrow #3}}
%\renewcommand{\frar}[3]{\ensuremath{{#1}{:}\;{#2}\rightarrow {#3}}}
\newcommand{\flar}[3]{\ensuremath{#1{:}\;#2\leftarrow #3}}

\newcommand{\frarxy}[2]{\enma{#1 \rightarrow #2}}
\newcommand{\flaxrar}[3]{\ensuremath{ #1{:}\;#2\xrightarrow{\mathrm{lax}}#3}}
%\renewcommand{\frar}[3]{\ensuremath{{#1}{:}\;{#2}\rightarrow {#3}}}
\newcommand{\flaxlar}[3]{\ensuremath{#1{:}\;#2\xleftarrow{\mathrm{lax}} #3}}


\newcommand{\frarind}[4]{\ensuremath{ #1{:}\;#3\stackrel{#2}{\longrightarrow} #4}}
%\renewcommand{\frar}[3]{\ensuremath{{#1}{:}\;{#2}\rightarrow {#3}}}
\newcommand{\flarind}[4]{\ensuremath{#1{:}\;#3\stackrel{#2}{\longleftarrow} #4}}

\newcommand{\monorar}[3]{\ensuremath{#1{:}\;#2\rightarrowtail #3}}
\newcommand{\monolar}[3]{\ensuremath{#1{:}\;#2\leftarrowtail #3}}
\newcommand{\incrar}[3]{\ensuremath{#1{:}\;#2\hookrightarrow #3}}
\newcommand{\inclar}[3]{\ensuremath{#1{:}\;#2\hookleftarrow #3}}

\newcommand{\trirar}[3]{\ensuremath{#1{:}\;#2 \Rrightarrow #3}}
\newcommand{\trilar}[3]{\ensuremath{#1{:}\;#2\Lleftarrow#3}}


\newcommand{\fprar}[4]{\ensuremath{#1{:}\;#2\stackrel{#4}{\rightarrow} #3}}
\renewcommand{\fprar}[4]{\ensuremath{#1{:}\;#2\rTo^{#4} #3}}
\newcommand{\fprarlong}[4]{\ensuremath{#1{:}\;#2\stackrel{#4}{\longrightarrow} #3}} 
%----> triple spaces
\newcommand\trisprightarrow{\mbox{$\lefteqn{\longrightarrow}~\,\circ$}}
\newcommand\trisprar[3]{\mbox{\ensuremath{ #1{:}\;#2\trisprightarrow~~#3}}}
\newcommand\trispprar[4]{\mbox{\ensuremath{#1{:}\;#2\stackrel{#4~~}{\trispprightarrow} #3}}}
%   newer version with 0 instead of \circ 
\renewcommand\trisprightarrow{\mbox{$\rightarrow_0$}}
\newcommand\trispprightarrow{\mbox{$\rightarrow_{00}$}}
\newcommand\trisprightarrowP{\trispprightarrow}
\renewcommand\trisprar[3]{\mbox{\ensuremath{ #1{:}\;#2\trisprightarrow#3}}}

\newcommand\trisprarP[4]{\trispprar{#1}{#2}{#3}{#4}}



%functional arrow
\newcommand\wrar[3]{\ensuremath{#1{:}\;#2\rightsquigarrow #3}} %wavy arrow
\newcommand\wbiar[3]{\ensuremath{#1{:}\;#2\leftrightsquigarrow #3}} %wavy arrow
\newcommand\farr[3]{\frar{#1}{#2}{#3}}% if typo occurs
%\newcommand\lar[3]{\flar{#1}{#2}{#3}}%
\newcommand\updar[3]{\frar{#1}{#2}{#3}}
%\newcommand\viewlar[4]{\mbox{$#1\!:#2\rightarrow^{#4} #3$}}
%\newcommand\flarcat[4]{\mbox{$#1\!:#2\rightarrow #3{:}{:}\,#4$}}

% variants
%-----------
%long
\newcommand\frarr[3]{\mbox{$#1\!:#2\longrightarrow #3$}} % long arrow
\renewcommand{\larr}[3]{\mbox{$#1\!:#2\longrightarrow #3$}} % the same
%\newcommand\lari[4]{\mbox{$#1_{i}\!:\:#2\:\longrightarrow\:#3_{i},\;i=1,\ldots,#4$}}%

%multihead
\newcommand\mlar[3]{\larlar{#1}{#2}{#3}} %multiarrow
\newcommand\larlar[3]{\mbox{$#1\!:#2\twoheadrightarrow#3$}} %needs AMS
% double body
\newcommand\drar[3]{\mbox{$#1\!\!:#2\Rightarrow #3$}} %double arrow
\newcommand\dlarcat[4]{\mbox{$#1\!:#2\Rightarrow #3{:}{:}\,#4$}}
\newcommand\trar[3]{\mbox{$#1\!:\,#2\Rightarrow #3$}}
% inclusions
\newcommand\inclarr[3]{\mbox{$#1\!:\:#2\:\rInto\:#3$}}       %$key=<AltShftRT>
%\newcommand\inclar[3] {\mbox{$#1\!:\:#2\:\hookleftarrow\:#3$}}
%\newcommand\incrar[3] {\enma{#1\!: #2\:\hookrightarrow#3}}
\newcommand\binclar[3] {\mbox{$#1\!:\:#2\:\hookleftarrow\:#3$}}
%triple body
%\newcommand\trilar[3]{\mbox{$#1\!:#2\Rrightarrow #3$}} % triple
% profunctor/span
\newcommand\spanar[3]{\mbox{$#1\!:#2\nrightarrow#3$}}
\newcommand\spanrar[3]{\mbox{$#1\!:#2\nrightarrow#3$}}
\newcommand\relrar[3]{\mbox{$#1\!:#2\nrightarrow#3$}}
\newcommand\rellar[3]{\mbox{$#1\!:#2\leftarrow#3$}}
\newcommand\trispar[3]{\spanar{#1}{#2}{#3}}  %synonym
\newcommand\backspanar[3]{\mbox{$#1\!:#2\nleftarrow#3$}}
%spans
\newcommand\spanlar[5]{\mbox{$#1\!:#2\leftarrow #3\rightarrow #4 :#5$}} %double arrow%
% -- bidir arrows version
\newcommand\spanarbi[3]{\mbox{$#1\!:#2\nleftrightarrow #3$}}
\newcommand\backspanardi[3]{\mbox{$#1\!:#3\nleftrightarrow #2$}}


%-- backward arrow
%\newcommand\flar[3]{\ensuremath{#1\!:#2\leftarrow #3}} %backward functional arrow
%\newcommand\bflar[3]{\mbox{$#1\!:#2\leftarrow #3$}} %backward functional arrow
\newcommand\dlar[3]{\mbox{$#1\!:#2\Leftarrow #3$}} %double arrow
%\newcommand\bdlar[3]{\mbox{$#1\!:#2\Leftarrow #3$}} %double arrow

% two directional
\newcommand\bilar[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\biarr[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\bidlar[3]{\mbox{$#1\!:#2\Leftrightarrow #3$}}
\newcommand\corar[3]{\bilar{#1}{#2}{#3}}
\newcommand\lelar[3]{\mbox{$#1\!:#2\rightleftarrows #3$}} %double arrow

\newcommand\lensar[3]{\mbox{$#1\!:#2\leftrightharpoons #3$}}%
\newcommand\lensarleft[3]{\mbox{$#1\!:#2\rightleftharpoons #3$}}%
\newcommand\lensarright[3]{\lensar{#1}{#2}{#3}}
%\renewcommand\lensar[3]{\mbox{$#1\!:#2\asymdoublearrow#3$}}
\newcommand\asymdoublearrow{%
\begin{array}{c}
~\rightarrow\\[-9pt]
\leftharpoondown
\end{array}}%

%%%%%%%%%%%%%%%%%%%%%%%
%---stackrel versions

% backward arrow
\newcommand\bfrarstack[3]{\mbox{$#3 \stackrel{~#1}{\longleftarrow} #2$}}
\newcommand\frarstack[3]{\bfrarstack{#1}{#2}{#3}}
\newcommand\flarstack[3]{\mbox{$#2\stackrel{#1~}{\longrightarrow} #3$}} %functyional arrow
\newcommand\spanlarstack[5]{\mbox{$#2\stackrel{~#1}{\longleftarrow} #3 %
                                                                       \stackrel{#5~}{\longrightarrow} #4$}} %double arrow%

% bidirectional

\newcommand\bilarsy[3]{\mbox{$#2\stackrel{#1}{\leftrightarrow}#3$}}
\newcommand\bidlarsy[3]{\mbox{$\left(#2\stackrel{#1}{\Leftrightarrow}#3\right)$}}
\newcommand\bixxlar[4]{\mbox{$#1\!:#2\stackrel{#3}{\longleftrightarrow} #4$}}%
\newcommand\bixlar[3]{\mbox{$#1\stackrel{#2}{\longleftrightarrow} #3$}}%
\newcommand\xxlar[4]{\mbox{$#1\!:#2\stackrel{#3}{\longrightarrow} #4$}}

%-- Now instances of the macros above for particular names of maps, thjeir sources and targets
\newcommand\updaraaa{\flar{a}{A}{A'}}
\newcommand\updarbbb{\flar{b}{B}{B'}}
\newcommand\corarrab{\bilar{r}{A}{B}}
\newcommand\corrarrab{\bilar{r}{A}{B}}
\newcommand\trisparrmn{\trispar{R}{\mmm}{\mmn}}
%
\newcommand\alifar[3]{\spanar{#1}{#2}{#3}}
\newcommand\backalifar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\alifarrmn{\spanar{\mmr}{\mmm}{\mmn}}
\newcommand\genalifarrmn{\spanar{\mmr}{\mmm}{\mmn}}
\newcommand\symalifarrmn{\spanar{\mmr^{>\!<}}{\mmm}{\mmn}}
\newcommand\asalifarrmn{\spanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\asymLalifarrmn{\spanar{\mmr^<}{\mmm}{\mmn}}
\newcommand\asymLEalifarrmn{\spanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\asymGalifarrmn{\spanar{\mmr^>}{\mmm}{\mmn}}
\newcommand\asymGEalifarrmn{\spanar{\mmr^\ge}{\mmm}{\mmn}}
\newcommand\bialifarrmn{\spanar{\mmr^{\cong}}{\mmm}{\mmn}}

\newcommand\backgenalifarrmn{\backspanar{\mmr}{\mmm}{\mmn}}
\newcommand\backsymalifarrmn{\backspanar{\mmr^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasalifarrmn{\backspanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\backasymLalifarrmn{\backspanar{\mmr^<}{\mmm}{\mmn}}
\newcommand\backasymGalifarrmn{\backspanar{\mmr^>}{\mmm}{\mmn}}

\newcommand\confar[3]{\spanar{#1}{#2}{#3}}
\newcommand\backconfar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\confarkmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\genconfarkmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\symconfarkmn{\spanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\asconfarkmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymLconfarkmn{\spanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\asymLEconfarkmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymGconfarkmn{\spanar{\mmk^>}{\mmm}{\mmn}}
\newcommand\asymGEconfarkmn{\spanar{\mmk^\ge}{\mmm}{\mmn}}
\newcommand\biconfarkmn{\spanar{\mmk^{\cong}}{\mmm}{\mmn}}
%--- outdated with *rmn instead of *kmn in the name of macros
%\newcommand\confar[3]{\spanar{#1}{#2}{#3}}
%\newcommand\backconfar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\confarrmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\genconfarrmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\symconfarrmn{\spanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\asconfarrmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymLconfarrmn{\spanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\asymLEconfarrmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymGconfarrmn{\spanar{\mmk^>}{\mmm}{\mmn}}
\newcommand\asymGEconfarrmn{\spanar{\mmk^\ge}{\mmm}{\mmn}}
\newcommand\biconfarrmn{\spanar{\mmk^{\cong}}{\mmm}{\mmn}}

\newcommand\backgenconfarkmn{\backspanar{\mmk}{\mmm}{\mmn}}
\newcommand\backsymconfarkmn{\backspanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasconfarkmn{\backspanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\backasymLconfarkmn{\backspanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\backasymGconfarkmn{\backspanar{\mmk^>}{\mmm}{\mmn}}
%--%--- outdated with *rmn instead of *kmn in the name of macros
\newcommand\backgenconfarrmn{\backspanar{\mmk}{\mmm}{\mmn}}
\newcommand\backopgenconfarrmn{\backspanar{\mmk^\circ}{\mmm}{\mmn}}
\newcommand\backopgenalifarrmn{\backspanar{\mmr^\circ}{\mmm}{\mmn}}
\newcommand\backsymconfarrmn{\backspanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasconfarrmn{\backspanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\backasymLconfarrmn{\backspanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\backasymGconfarrmn{\backspanar{\mmk^>}{\mmm}{\mmn}}



%
\newcommand\lensarlmn{\lensar{\alens}{\mmm}{\mmn}}
\newcommand\genlensarlmn{\lensar{\alens}{\mmm}{\mmn}}
\newcommand\aslensarlmn{\lensar{\alens^\leq}{\mmm}{\mmn}}
\newcommand\asymLElensarlmn{\lensar{\alens^\leq}{\mmm}{\mmn}}
\newcommand\asymGElensarlmn{\lensar{\alens^\geq}{\mmm}{\mmn}}
\newcommand\symlensarlmn{\lensar{\alens^\gtlt}{\mmm}{\mmn}}
\newcommand\lesnarlmn{\lensar{\alens}{\mmm}{\mmn}} % the same in case of typo

\newcommand\lenssupx[1]{\lensar{\alens^{{#1}}}{\mmm}{\mmn}}
\newcommand\lenssubx[1]{\lensar{\alens_{{#1}}}{\mmm}{\mmn}}
\newcommand\lensopsupx[1]{\lensar{\alens^{\circ{#1}}}{\mmn}{\mmm}}
\newcommand\lensopsubx[1]{\lensar{\alens^{\circ_{#1}}{\mmn}{\mmm}}}
\newcommand\lenssupsubx[2]{\lensar{\alens^{#1}_{#2}}{\mmm}{\mmn}}

\newcommand\cfwksubx[1]{\spanar{\mmk_{{#1}}}{\mmm}{\mmn}}
\newcommand\cfwkopsubx[1]{\spanar{\mmk^{\circ}_{{#1}}}{\mmm}{\mmn}}

\newcommand\syncar[3]{\mbox{$#1\!:#2 \rightleftarrows #3$}}%
\newcommand\syncarleft[3]{\mbox{$#1\!:#2 \leftrightarrows #3$}}%
\newcommand\syncaright[3]{\syncar{#1}{#2}{#3}}
\newcommand\async{\ensuremath{\sigma}}
\newcommand\aSync{\ensuremath{\Sigma}}
\renewcommand\aSync{\ensuremath{\Pi}}
\newcommand\syncarsab{\syncar{\async}{A}{B}}
\newcommand\gensyncarsab{\syncar{\async}{A}{B}}
\newcommand\genSyncarsab{\syncar{\async}{A}{B}}
\newcommand\gensynctypearsab{\syncar{\async}{A}{B}}
\newcommand\genSynctypearsab{\syncar{\async}{A}{B}}
\newcommand\assyncarsab{\syncar{\async^\leq}{A}{B}}
\newcommand\asymGLEsyncarsab{\syncar{\aSync_{>\!\le}}{A}{B}}
\newcommand\asymGELsyncarsab{\syncar{\aSync_{\ge\!<}}{A}{B}}
\newcommand\asymGsyncarsab{\syncar{\aSync_{>}}{A}{B}}
\newcommand\asymLsyncarsab{\syncar{\aSync_{<}}{A}{B}}
\newcommand\symsyncarsab{\syncar{\async_\gtlt}{A}{B}}
\newcommand\symsyncarsabPoor{\syncar{\async_{\ge\!\le}}{A}{B}}
\newcommand\symSyncarsab{\syncar{\aSync_\gtlt}{A}{B}}
\newcommand\symSyncarsabPoor{\syncar{\aSync_{\ge\!\le}}{A}{B}}
\newcommand\lesnarsab{\syncar{\async}{A}{B}} % the same in case of typo



\newcommand\noninclensarlmn{\lensar{\alens_\noninc}{\mmm}{\mmn}}
\newcommand\fullinclensarlmn{\lensar{\alens_\fullinc}{\mmm}{\mmn}}


\endinput










\newcommand\vilar[3]{\dlar{#1}{#2}{#3}}
\newcommand\vlar[3]{\vilar{#1}{#2}{#3}}
\newcommand\malar[3]{\flar{#1}{#2}{#3}}
\newcommand\uplar[3]{\flar{#1}{#2}{#3}}
\newcommand\ular[3]{\uplar{#1}{#2}{#3}}
%  adding :: Graph,Set,Cat etc as the 4th parameter
\newcommand\vilarcat[4]{\dlarcat{#1}{#2}{#3}{#4}} % .. ::#4
\newcommand\malarcat[4]{\flarcat{#1}{#2}{#3}{#4}}
\newcommand\uplarcat[4]{\flarcat{#1}{#2}{#3}{#4}}

\newcommand\viewOfrel{{\prec}}
\newcommand\viewofar[3]{\mbox{$#1\!:#2\Rightarrow #3$}}
\newcommand\mmvmn{\vilar{\mmv}{\mms}{\mmt}}
\newcommand\mmvab{\vilar{\mmv}{\mms}{\mmt}}
\newcommand\mmvabcat{\vilarcat{\mmv}{\mms}{\mmt}{\mmodcat}}
\newcommand\mmvmncat{\vilarcat{\mmv}{\mms}{\mmt}{\mmodcat}}
\newcommand\mvab {\vilar{\mv}{A}{B}}
\newcommand\mvabcat{\vilarcat{\mv}{A}{B}{\modcath}}


\newcommand\vrelar[3]{\mbox{$#1\stackrel{#3}{\leftarrow}#2$}}
\newcommand\mmvrel[3]{\vrelar{#1}{#2}{#3}}
\newcommand\mmabv{\mmvrel{\mma}{\mmb}{\mmv}}


==> genMacros/readme.tex <==
Nov 28
File 4textarrows.tex was replaced by 4textarrows from the EDL dir (with a few modifications). The previous file is saved unde *-Nov28 name

==> genMacros/tailOfgeneralMath.tex <==




\setlength{\marginparwidth}{3cm}
%\setlegth{\marginparsep}{1.5mm}
%\setlength{\marginparpush}{5mm}
%

\makeatletter
\def\fps@figure{tp}
\makeatother

\newcommand{\backgro}[2]{\par\noindent\framebox[\textwidth]{
		\begin{minipage}{0.98\textwidth}
			\setlength{\parindent}{0.5cm} \noindent \textbf{Background: #1} #2
	\end{minipage}}\smallskip}

%%%% macros %%%
%\newtheorem{defin}{Definition}%[section]
%\renewcommand{\thedefin}{\Alph{defin}}





%\newcommand\xxx[4]{{\it #1}\mbox{$_{#3}^{#4}{#2}$}}
%\newcommand{\s}{\star}
%\newcommand\mrk[1]{\mbox{$\langle${\tt #1}$\rangle$}}
%=================================================
% 1  Fonts and letters
%============================================

%=====================================================
% 2  Mathematical shtuchki
%=========================================================


% New Symbols allowed to use in MathMode (!)
%========= General =============
\newcommand\mylist[2]{\mbox%
	{$#1_1,\ldots,#1_{#2}$}}

\newcommand\iidots[2]{\mbox{
		$#1=1,\ldots,#2$
}}
\newcommand\ijdots[3]{\mbox{
		$#1=#2,\ldots,#3$
}}
\newcommand{\vare}{\varepsilon}
\newcommand\nr{\normalsize\rm}
\newcommand\tril{\triangleleft}
\newcommand\eqdef{\stackrel{\rm def}{=}}
\newcommand\trir{\triangleright}
\newcommand\bc{\bigcirc}








%(5)\newcommand\entails{\Rightarrow}
%\newcommand\implies{\Rightarrow}
%-------------------------------------
%\newcommand\dom[1]{\mathit{Dom}(#1)}
%\newcommand\cod[1]{\mathit{Cod}(#1)}
\newcommand\rg[1]{\mathit{Rg}(#1)}
\newcommand\DOM[1]{\Box #1}
\newcommand\COD[1]{#1 \Box}

\newcommand\tabname[1]{\mbox{$\ittt{Tab}\_#1$}}
%\newcommand\multisource[
\newcommand\mytilde[1]{\widetilde{#1}}
\newcommand\sempr[1]{\mytilde{\semm{#1}}}

\newcommand\mycount[1]{{\bf count}{(#1)}}
\newcommand\gragen[1]{\left[\mathstrut #1 \right]}

\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\enma{$\lsemm\, \mathit{#1} \, \rsemm$}}
\newcommand\semmind[2]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm^{#2}$}}
\newcommand\semmx[2]{\enma{$\lsemm\, \mathit{#2} \, \rsemm^{#1}$}}
\newcommand\semmA[2]{\enma{$\lsemm\, \mathit{#2} \, \rsemm^{A}$}}
\newcommand\semmB[2]{\enma{$\lsemm\, \mathit{#2} \, \rsemm^{B}$}}

\newcommand\semmindex[1]{\lsemm\, \mathit{#1} \, \rsemm}
\newcommand\semmstar[1]{\semm{#1}^{*}}
\newcommand\lbesemm{\left< \respace\left<}
\newcommand\rbesemm{\right> \respace\right>}
\newcommand\besemm[1]{\mbox{$\lbesemm\, \mathit{#1} \, \rbesemm$}}



%(6)%\newcommand\informalPar[1]{\nicex{{#1}$}}
%\newcommand\infParind[1]{\cal #1}
%Contents:
%--- semiotics
%--- Skesig
%--- Varset
%--- Behset



%%==== Semiotics =====
%
%%\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
%\newcommand\frmParind[1]{\mathrm{#1}}
%
%\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
%
%\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%%\newcommand\object[2]{\mbox{$#1_{#2}$}}
%\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\universeind[1]{\mathbf{#1}}
%
%\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
%\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
%\newcommand\linf{\informalParBold{L}}
%\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
%\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
%\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
%\newcommand\uinf{\informalPar{U}}
%
%\newcommand\meaninf{\informalPar{M}}
%\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}
%\newcommand\diag[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diagob[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diags{\mbox{$\mathit{Diags}$}}
%\newcommand\graph{\mbox{$\mathit{Graph}$}}
%\newcommand\skeob[1]{\object{S}{#1}}
%\newcommand\modelob[1]{\object{M}{#1}}
%\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
%\newcommand\skediag{\skeob{}[\diag{}]}
%\newcommand\meaninfdiag{\meaninf[\diag{}]}
%\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
%% synonyms
%\newcommand\meanifdiag{\meaninf[\diag{}]}
%\newcommand\meanfdiag{\meanfrm[\diag{}]}

%=======================
%==== Skesig
%\newcommand\so[1]{source(#1)}
%\newcommand\ta[1]{target(#1)}
\newcommand\U{{\cal U}}
\newcommand\M{{\cal M}}
\newcommand\Set{{\mathbf Set}}
\newcommand\Varset{{\mathbf Varset}}
\newcommand\univ{\mbox{$\mathbf U$}}
\newcommand\univind{{\mathbf U}}
\newcommand\skesig{\mbox{$\Sigma$}}

%%%% macro\Skesig.tex %%%%  June 29

\newcommand\mrkid{\mrk{ID}}
\newcommand\imID{\mbox{ID?}} %$^*$}}
\newcommand\mrkidd{\imID} % marker of IDDeficient
\newcommand\prodid{\mbox{$\times$-\ider}}
\newcommand\plusid{\mbox{$+$-\ider}}
\newcommand\prodkey{\mbox{$\times$-key}}
\newcommand\pluskey{\mbox{$+$-key}}

\newcommand\ID{\mrk{ID}}
\newcommand\IDplus{\mrk{ID$^+$}}
\newcommand\IDprod{\mrk{ID$^\times$}}

\newcommand\andiden{\emph{and}-\iden}
\newcommand\oriden{\emph{or}-\iden}


\newcommand\ssta{\mbox{${\mathsf S}_{\mathrm sta}$}}
\newcommand\sdyn{\mbox{${\mathsf S}_{\mathrm dyn}$}}

%\newcommand\mrk[1]{\mbox{[${\tt #1}$]}}
%\newcommand\mrk[1]{\mbox{[${\mathbf{#1}}$]}}
%\newcommand\mrkop[1]{\mbox{$\langle{\tt #1}\rangle$}}
\newcommand\mrkop[1]{\mbox{$\langle{\mathbf{#1}}\rangle$}}
\newcommand\mrkopr[1]{\mbox{$\mathbf{[{#1}\rangle}$}}
\newcommand\mrkopl[1]{\mbox{$\mathbf{\langle{#1}]}$}}
\newcommand\mrksemiop[1]{\mbox{$\langle{\tt #1}]$}}
\newcommand\mrkNode[1]{\mbox{${\tt #1}$}}
\newcommand\mrkn[1]{\mrkNode{#1}}
\newcommand\mrktt[1]{{\tt #1}}
\newcommand\mrkopright[1]{\mbox{$[${\tt #1}$\rangle$}}
\newcommand\mrkopleft[1]{\mbox{$\langle${\tt #1}$]$}}
%%%%%%%%%%%%%  Begin Key commands %%%%%%%%%%%%%%%%%%%%%%%

\newcommand\PredicateSignature{\Pi}
\newcommand\OperationSignature{\Sigma}
\newcommand\predFromOperSig{\Sigma_{pr}}
\newcommand\BaseSignature{\bf B}
\newcommand\DomainBase{\bf B}

\newcommand\ConstraintLanguage{CL}
\newcommand\dolan%DomainLanguage{\Delta}
{\mbox{$\Delta $}}

\newcommand\dolanm{\Delta}

\newcommand\adtm{ADT}
\newcommand\adt{{\sl \adtm}}
\newcommand\dolanadt{\dolan_{\adtm}}
\newcommand\sigadt{{\it Sig}_{\adtm}}
\newcommand\semmadt{\semm{}_{\adtm}}

\newcommand\dbauxm{DBD}
\newcommand\dbaux{{\sl \dbauxm}}
\newcommand\dolandbaux{\dolan_{\dbauxm}}
\newcommand\sigdbaux{{\it Sig}_{\dbauxm}}
\newcommand\semmdbaux{\semm{}_{\dbauxm}}

\newcommand\ba{D}
\newcommand\domba{\mbox{$\Domain(\ba)$}}
\newcommand\bam{\BasicDomainMarkerSymbol}          %  B  for using in math mode
%\newcommand\V{\mbox{$\TheValueUniverse_{\dolanm}$}}%

\newcommand\Pred{{\it Pred}}
\newcommand\Oper{{\it Op}}
\newcommand\Base{{\it Base}}
\newcommand\Dom{{\it Dom}}
\newcommand\Domain{{\it Dom}}
\newcommand\pool{V}

\newcommand\ArityMap{{\it Shp}}
\newcommand\ArityGraph{D}
\newcommand\AritySketch{{\cal D}}
\newcommand\ArityInclusion{\mbox{\Large $\iota$}}

\newcommand\rms{\rm\scriptsize}   % for writing, eg, \D^{\rms in}

\newcommand\PredicateMarkerSymbol{P}
\newcommand\OperationMarkerSymbol{F}
\newcommand\BasicDomainMarkerSymbol{B}

\newcommand\PredicateDiagramSet[1]{\PredicateMarkerSymbol^{#1}}%P^#1}
\newcommand\OperationDiagramSet[1]{\OperationMarkerSymbol^{#1}}%F^#1}
\newcommand\BasicDomainDiagramSet[1]{\BasicDomainMarkerSymbol^{#1}}%B^#1}

\newcommand\AGraph{G}
\newcommand\g{\mbox{$\AGraph$}}
\newcommand\gm{\AGraph}

\newcommand\ASketchSymbol{S}
\newcommand\ASketch{\mathsf \ASketchSymbol}
\newcommand\s{\mbox{$\ASketch$}}
\newcommand\sind{\ASketch}
\newcommand\sm{\ASketch}
\newcommand\sprim{\mbox{$\ASketch'$}}
\newcommand\sbipr{\mbox{$\ASketch''$}}


\newcommand\TheUniverseSymbol{U}
\newcommand\TheUniverseSketch{\cal \TheUniverseSymbol}
\newcommand\TheObjectUniverse{Obj }%{\cal O}
\newcommand\TheTimeUniverse{\cal T}%{T}
\newcommand\TheHistoryUniverse{\cal \TheTimeUniverse^*}%}
\newcommand\TheValueUniverse{Val}%{\cal V}

\newcommand\ASketchAlgebra{\cal A}
\newcommand\ABaseSubSketch{\cal B}    % base subsketch of

\newcommand\APermutation{\pi}

%===================================================

\newcommand\Mod[1]{\mbox{{\bf Mod}$(#1)$}}
\newcommand\Ext[1]{\mbox{{\bf Ext}$(#1)$}}
\newcommand\Inst[1]{\mbox{{\bf Inst}$(#1)$}}

%%%%%%%%%%%%%   End Key commands %%%%%%%%%%%%%%%%%


%%%%%%%%%%%%    Useful Abbreviations %%%%%%%%%%%%

%%% Sketchi


\newcommand\sdom{\mbox{$\s_{\DomainBase}$}}
\newcommand\sdomm{\s_{\DomainBase}}

\newcommand\newb{\mbox{$\DomainBase$}}
\newcommand\bm{\DomainBase}

\newcommand{\bs}{\mbox{$\ABaseSubSketch$}}
\newcommand\bsm{\ABaseSubSketch}

\newcommand\skespe{{\bf \ASketchSymbol}}

\newcommand\gras{{\it Gra}\skeob}
\newcommand\doms{{\it Dom}\skeob}
\newcommand\clas{{\it Cla}\skeob}
\newcommand\rels{{\it Rel}(\skeob)}

\newcommand\R{\nicex{ R$}}
\newcommand\OO{\mbox{$\TheObjectUniverse$}}
%\newcommand\T{\mbox{$\TheTimeUniverse$}}
%\newcommand\Hist{\mbox{$\TheHistoryUniverse}}
%\newcommand\V{\mbox{$\TheValueUniverse_{\bm}$}}%

\renewcommand\u{\mbox{$\TheUniverseSketch$}}
\newcommand\um{\TheUniverseSketch}
\newcommand\upred{\mbox{$\TheUniverseSketch_{\predsigm}$}}
\newcommand\uoper{\mbox{$\TheUniverseSketch_{\opersigm}$}}

\newcommand\predsig{\mbox{$\PredicateSignature$}}
\newcommand\predsigm{\PredicateSignature}
\newcommand\opersig{\mbox{$\OperationSignature$}}
\newcommand\opersigm{\OperationSignature}
\newcommand\predopsig{\mbox{$\predFromOperSig$}}
%\newcommand\pros{\predopsig}
\newcommand\prosm{\predFromOperSig}
\newcommand\basesig{\mbox{\BaseSignature}}
\newcommand\basesigm{{\BaseSignature}}
\newcommand\clan{\mbox{$\ConstraintLanguage$}}
\newcommand\clanm{\ConstraintLanguage}
\newcommand\colan{\mbox{\ConstraintLanguage}}
\newcommand\clanform{\mbox{$\ConstraintLanguage=(\Pred,\arimap,\semm{})$}}
\newcommand\colanm{\ConstraintLanguage}
%\newcommand\dolan{\mbox{\DomainLanguage}}
%\newcommand\dolanm{\DomainLanguage}

\newcommand\pis{$\PredicateSignature $-sketch}
\newcommand\sis{$\OperationSignature $-sketch}
\newcommand\siprs{$\predFromOperSig$-sketch}
\newcommand\sia{$\OperationSignature $-algebra}
\newcommand\clans{$\Constraint Language$-sketch}

\newcommand\arimap{\ArityMap}
\newcommand\arimapin{\mbox{\ArityMap$^{\rms in}$}}

\newcommand\os{\mbox{$\overline{\s}$}}
%\newcommand\go{\mbox{$G_{({\cal O})}$}}

\newcommand\pip{\mbox{$\APermutation^{+}$}}
\newcommand\depipComp{\mbox{$\delta \comp\APermutation^{+}$}}
\newcommand\depip{\mbox{$\APermutation^{+}\delta $}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%
%%%%%%%%%%            A R I T I E S         %%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\pr{\mbox{$\PredicateMarkerSymbol$}}  % $P$ for using in text mode
\newcommand\op{\mbox{$\OperationMarkerSymbol$}}  % $F$ for using in text mode
%\newcommand\ba{\mbox{$\BasicDomainMarkerSymbol$}}  % $P$ for using in text mode


\newcommand\myprm{\PredicateMarkerSymbol}        %  P  for using in math mode
\newcommand\opm{\OperationMarkerSymbol}          %  F  for using in math mode
%\newcommand\bam{\BasicDomainMarkerSymbol}       %  B  for using in math mode

%%%%   functions to put the arg
%%%%   as subindex near \pr,\op and \ba

\newcommand\prix[1]{\myprm_{#1}}
\newcommand\opix[1]{\opm_{#1}}
\newcommand\baix[1]{\bam_{#1}}

%%%----  end functions

\newcommand\pri{$\myprm_{i}$}    %  \pr_i for using in text mode
\newcommand\opi{$\opm_{j}$}      %  \op_j for using in text mode
\newcommand\bai{$\bam_{l}$}      %  \ba_l for using in text mode

\newcommand\prim{\myprm_{i}}     %  \pr_i for using in math mode
\newcommand\opim{\opm_{j}}       %  \op_j for using in math mode
\newcommand\baim{\bam_{l}}       %  \ba_l for using in text mode
%======================================
%  eto makrosy funcciy
\renewcommand\Pr[1]{\PredicateDiagramSet{#1}}  % P^#1
\newcommand\Op[1]{\OperationDiagramSet{#1}}    % F^#1
\newcommand\Ba[1]{\BasicDomainDiagramSet{#1}}  % B^#1
%  a eto ih znacheniya
\newcommand\PrS{\Pr{\s}}      % P^\s
\newcommand\OpS{\Op{\s}}      % F^\s
\newcommand\BaS{\Ba{\s}}      % B^\s
%\newcommand\domba{$\Domain(\ba)$}

\newcommand\PrU{\Pr{\u}}      % P^\u
\newcommand\OpU{\Op{\u}}      % F^\u
\newcommand\BaU{\Ba{\u}}      % B^\u

%------------------------------------------------
% eto makrosy funkciy s 2 argumwntami
\newcommand\Prix[2]{\Pr{#1}_{#2}}              % a set P^#1_#2
\newcommand\Opix[2]{\Op{#1}_{#2}}              % a set F^#1_#2
\newcommand\Baix[2]{\Ba{#1}_{#2}}              % a set B^#1_#2
% a eto b nih podstavleny indexy i ostalsya 1 argument
\newcommand\Pri[1]{$\Prix{#1}{i}$}             % a set og diag, P^#1_i
\newcommand\Opi[1]{$\Opix{#1}{j}$}             % a set of diag, F^#1_j
\newcommand\Bai[1]{$\Baix{#1}{l}$}             % a set of diag, B^#1_l
% a eto znacheniya
\newcommand\PriS{\Pri{\s}}      % Pi^\s
\newcommand\OpiS{\Opi{\s}}      % Fj^\s
\newcommand\BaiS{\Bai{\s}}      % Bl^\s

\newcommand\PriU{\Pri{\u}}      % Pi^\u
\newcommand\OpiU{\Opi{\u}}      % Fj^\u
\newcommand\BaiU{\Bai{\u}}      % Bl^\u

%  a eto dlya mat mode
\newcommand\Prim[1]{\Prix{#1}{i}}     %  a set of diagr,  P^#1_i for using in math mode
\newcommand\Opim[1]{\Opix{#1}{j}}     %  a set of diagr,  F^#1_j for using in math mode
\newcommand\Baim[1]{\Baix{#1}{l}}     %  a set of diagr,  B^#1_#2 for using in math mode
%====================================================

%\newcommand\pool{V}
\newcommand\vx[1]{\mbox                                  % D_arg
{$\pool_{#1}$}}
\newcommand\vinx[1]{\mbox                                % D^in_arg
{$\pool^{\mbox\rms in}_{#1}$}}
\newcommand\voutx[1]{\mbox                               % D^out_arg
{$\pool^{\mbox\rms out}_{#1}$}}
%============================================================

%\newcommand\ArityGraph{D}
%\newcommand\AritySketch{\D}                             % \D - nice D
\newcommand\sprx[1]{\mbox                                %  D_arg
{$\ArityGraph_{#1}$}}
\newcommand\sopx[1]{\mbox                                % \D_arg
{$\AritySketch_{#1}$}}
\newcommand\sinx[1]{\mbox                                % \D^in_arg
{$\AritySketch^{\rms in}_{#1}$}}
\newcommand\soutx[1]{\mbox                               % \D^out_arg
{$\AritySketch^{\rms out}_{#1}$}}

%-----   marker-subindex version
\newcommand\spr{\sprx{\myprm}}         %  D_{prop marker}
\newcommand\sop{\sopx{\opm}}         % \D_{oper marker}
\newcommand\sinop{\sinx{\opm}}       % \D^in_{oper mark}
%-----   i-subindex version
\newcommand\spri{\sprx{i}}          %  D_{i}
\newcommand\sopi{\sopx{j}}          % \D_{j}
\newcommand\sinopi{\sinx{j}}        % \D^in_{j}



\newcommand\opshaxy[2]{\inclar{#1_{#2}}  % arg1_arg2: D^in_arg2 -->D_arg2
{\sinx{#2}}
{\sopx{#2}}
}
%\newcommand\ArityInclusion{i}
\newcommand\opsha{\opshaxy{\ArityInclusion}{\opm}}   %i_f: D^in_f   --> D_f
\newcommand\opshai{\opshaxy{\ArityInclusion}{\opim}} %i_f: D^in_f_j --> D_f_j

%----------------------------------------

%\newcommand\ArityMap{{\it Shp}}
\newcommand\arix[1]{\mbox
{$\ArityMap({#1})$}}         % Shp(arg)
\newcommand\ariinx[1]{\mbox
{$\ArityInclusion_{#1}$}}    % \iota_{arg}

\newcommand\aripr{\arix{\myprm}}                  % Shp(p)
\newcommand\ariop{\arix{\opm}}                  % Shp(f)
\newcommand\arinc{\ariinx{\opm}}                % \iota_f

\newcommand\aripri{\arix{\prim}}                % Shp(p_i)
\newcommand\ariopi{\arix{\opim}}                % Shp(f_j)
\newcommand\arinci{\ariinx{\opim}}              % \iota_j

%-----------------------------------------
\newcommand\sepr{\semm{\pr}}
\newcommand\seop{\semm{\op}}
\newcommand\sepri{\semm{\pri}}
\newcommand\seopi{\semm{\op}}


\newcommand\opv{\mbox{\Oper$^+$}}

%\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%  Old Macros %%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\sig{\mbox{$\PredicateSignature$}}
%\newcommand\gra{{\bf G}}
%\newcommand\sigo{\mbox{$\Sigma_1$}}
%\newcommand\grao{\mbox{${\bf G}_1$}}
%% OOPS! \newcommand\inst{\mbox{$\lar{\vare }{S}{W}$}}
%%\newcommand\sch{\Category{Schema} }
%
%
%\newcommand\instVareps{\mbox{$\lar{\vare }{S}{W}$}}
%\newcommand\inste{\mbox{$\lar{e}{S}{W}$}}
%\newcommand\emor[1]{\lar{e}{#1}{\u}}
%\newcommand\sv{\mbox{$S_V$}}
%\newcommand\sr{\mbox{$S_R$}}
%\newcommand\vmor{\lar{v}{\sv}{\ovrs{}}}
%\newcommand\rmor{\lar{r}{S}{\ovrs{R}}}
%\newcommand\vpair{\mbox{$V=(\sv,v)$}}
%\newcommand\rpair{\mbox{$R=(\sr,r)$}}
%===
%==== Varset
%% macros for writing formulas with varsets and varfunctions

%%%%%%%%%    ..\dke96\macro\varset.tex    %%%%%%%
%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C
%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\ceind{\ltt}}                         % ||C||^t
%\newcommand\ceu{\ceind{\ltu}}                         % ||C||^u
\newcommand\ObjStt{\ittt{ObjStt}}
\newcommand\C{\textit{C}}
\newcommand\D{\textit{D}}

\newcommand\ot[1]{\mbox{$o^{\ltt_{#1}}$}}
\newcommand\otm{o^\ltt}
\newcommand\ou[1]{\mbox{$o^{\ltu_{#1}}$}}
\newcommand\otu{o^\ltu}

\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
\newcommand\ceti{\mbox{$\semm{C}^{\ltt_i}$}}                         % ||C||^t
\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
\newcommand\ceprt{\mbox{$\sempr{C}^{\ltt}$}}                         % ||C||^t
\newcommand\cepru{\mbox{$\sempr{C}^{\ltu}$}}                         % ||C||^t


\newcommand\cetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltu}$}}
\newcommand\ceut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\AClass}^{\ltt}$}}
\newcommand\detu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass}^{\ltu}$}}
\newcommand\fetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_f}^{\ltu}$}}
\newcommand\djetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_j}^{\ltu}$}}
\newcommand\dietu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_i}^{\ltu}$}}
\newcommand\deut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\ceprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\AClass}^{\ltu}$}}
\newcommand\deprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\TargetClass}^{\ltu}$}}



\newcommand\cesu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltu}$}}
\newcommand\cest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltt}$}}
\newcommand\cett{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltt}$}}

\newcommand\dest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\desu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltu}$}}

\newcommand\cestart{\mbox{${\semmstar{C}}^{\ltt}$}}                         % ||C||^t
\newcommand\cestaru{\mbox{${\semmstar{C}}^{\ltu}$}}                         % ||C||^t
\newcommand\cestartu{\mbox{${}^{\ltt}{\semmstar{C}}^{\ltu}$}}

\newcommand\ceto{\mbox{$\semm{\AClass}^{\ltt}_{o}$}}
\newcommand\ceuo{\mbox{$\semm{\AClass}^{ \ltu}_{o}$}}

\newcommand\cestarto{\mbox{${\semmstar{\AClass}}^{\ltt}_{o}$}}
\newcommand\cestaruo{\mbox{${\semmstar{\AClass}}^{ \ltu}_{o}$}}

%======================================================================

%  ----  Basic Command -----------

\newcommand\LogicalTime{\cal T}
\newcommand\SetOfHistories{\LogicalTime^*}
\newcommand\AHistory{H}%J}

%\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}
%\newcommand\IntRelSymb{\varepsilon}%rho}
%\newcommand\IntRelSymb{\mbox{\Large$\iota$}}%rho}
%\newcommand\IntersttMap{\mbox{\ittt same}}%rho}

\newcommand\AClass{C}
\newcommand\SourceClass{C}
\newcommand\TargetClass{D}
\newcommand\e{E}
\newcommand\AReference{f}
\newcommand\AnotherReference{g}
%\newcommand\Identifier{\mbox{\Large$\iota$}}
\renewcommand\g{g}
%\newcommand\h{h}
%\newcommand\hind{h}


\newcommand\farr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\farris{\lar{\AReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\farrit{\lar{\AReference_i}{\SourceClass_i}{\TargetClass}}
\newcommand\ffams{\mbox{$\f=\famm{\farris}{i\in I}$}}
\newcommand\ffamt{\mbox{$\f=\famm{\farrit}{i\in I}$}}

\newcommand\garr{\lar{\AnotherReference}{\SourceClass}{\TargetClass}}
\newcommand\garrit{\lar{\AnotherReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\garris{\lar{\AnotherReference_i}{\SourceClass_i}{\TargetClass} }
\newcommand\gfams{\mbox{$\g=\famm{\garris}{i\in I}$}}
\newcommand\gfamt{\mbox{$\g=\famm{\garrit}{i\in I}$}}


\newcommand\iarr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\iarris{\lar{\Identifier_j}{\SourceClass}{\TargetClass_j}}
\newcommand\iarrit{\lar{\Identifier_j}{\SourceClass_j}{\TargetClass} }
\newcommand\ifams{\mbox{$\Identifier=\famm{\iarris}{j\in J}$}}
\newcommand\ifamt{\mbox{$\Identifier=\famm{\iarrit}{j\in J}$}}


\newcommand\AMoment{t}%j}
\newcommand\EarlierMoment{t}%j}
\newcommand\LaterMoment{u}%k}
\newcommand\EarlierEarlierMoment{s}%i}
\newcommand\LaterLaterMoment{v}%l}

\newcommand\ttt{t1,t2}

\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}

%%%%%%%%%%%%%%%%%%%%%%
% -- Abbreviations ----
%%%%%%%%%%%%%%%%%%%%%%%%%%                    sket}}


\newcommand\T{\mbox{$\LogicalTime$}}
\newcommand\Tm{\LogicalTime}
\newcommand\Hist{\mbox{$\SetOfHistories$}}
\newcommand\Histm{\SetOfHistories}
\newcommand\IntersttMap{\mbox{\ittt{same}}}%rho}
\newcommand\same[2]{\mbox{$\IntersttMap^{#1}_{#2}$}}
\newcommand\inter[2]{\same{#1}{#2}}
\newcommand\interpr[2]{\mbox{$\mytilde\IntersttMap^#1_#2$}}
% \IndexingXupYdownZ{\IntRelSymb}{#1}{#2}}  %\vare^#1_#2
%\newcommand\interpr[2]%
%      {\IndexingXupYdownZ{\mytilde{\IntRelSymb}}{#1}{#2}}  %\vare^#1_#2

%%% The new version t is denoted by \ltt, u is denoted by  \ltu etc

\newcommand\ttu{\EarlierMoment\LaterMoment}   %tu
\newcommand\logtimet{\EarlierMoment}               %t
\newcommand\ltt{\EarlierMoment}               %t
%\newcommand\tu{\LaterMoment}                  %u
\newcommand\ltu{\LaterMoment}                  %u
\newcommand\ttlu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tleu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tlu{\mbox{$\ltt<\ltu$}}            % t < u
\newcommand\logtimes{\EarlierEarlierMoment}        %s
\newcommand\lts{\EarlierEarlierMoment}               %t
\newcommand\ltv{\LaterLaterMoment}             %l
\newcommand\tv{\LaterLaterMoment}             %l

\newcommand\J{\AHistory}                      %J

\newcommand\intertu[1]{\inter{\ltt\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interut[1]{\inter{\ltt\gets\ltu}{#1}}       % \eps^tu_#1
\newcommand\intertuut[1]{\inter{\ltt\leftrightarrow\ltu}{#1}}       % \eps^tu_#1

\newcommand\intertt[1]{\inter{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\interts[1]{\inter{\lts\gets\ltt}{#1}}       % \eps^tu_#1

\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interus[1]{\inter{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domintertu[1]{\ldom{\intertu{#1}}}  %\Box\eps^tu_#1
\newcommand\codintertu[1]{\rdom{\intertu{#1}}}  %\eps^tu_#1\Box

\newcommand\sametuut[1]{\mbox{$\same{\ltt\leftrightarrow\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sametu[1]{\mbox{$\same{\ltt\to\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sameut[1]{\mbox{$\same{\ltt\gets\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\samectu{\mbox{$\same{\ltt\to\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samecut{\mbox{$\same{\ltt\gets\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samedtu{\mbox{$\same{\ltt\to\ltu}{\dm}$}}       % \eps^tu_#1
\newcommand\samedut{\mbox{$\same{\ltt\gets\ltu}{\dm}$}}       % \eps^tu_#1

\newcommand\samett[1]{\same{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\samets[1]{\same{\lts\gets\ltt}{#1}}       % \eps^tu_#1
\newcommand\samecst{\same{\lts\to\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samects{\same{\lts\gets\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samedst{\same{\lts\to\ltt}{\dm}}       % \eps^tu_#1
\newcommand\samedts{\same{\lts\gets\ltt}{\dm}}       % \eps^tu_#1



\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\sameus[1]{\same{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domsametu[1]{\ldom{\sametu{#1}}}  %\Box\eps^tu_#1
\newcommand\codsametu[1]{\rdom{\sametu{#1}}}  %\eps^tu_#1\Box


%  Apply:
\newcommand\interctt{\inter{\ltt\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\intercst{\inter{\lts\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interctu{\inter{\ltt\to\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\intercsu{\inter{\lts\to\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\intercut{\inter{\ltt\leftarrow\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\interprctt{\interpr{\ltt\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprcst{\interpr{\lts\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprctu{\interpr{\ltt\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\interprcsu{\interpr{\lts\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\dominterctu{\domintertu{\cm}}  %\Box\eps^tu_#1
\newcommand\codinterctu{\codintertu{\cm}}  %\eps^tu_#1\Box

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
\newcommand\cm{\AClass}                              %   C
\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%--- function:
\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
%\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
%\newcommand\cetu{\mbox{${}^{\ltt}\semm{\AClass}^{\ltu}$}}
\newcommand\ces{\ceind{\lts}}                         % ||C||^u
\newcommand\cev{\ceind{\tv}}                         % ||C||^u


\newcommand\ceJ{\ceind{\J}}

\newcommand\objeq[2]{\simeq^{#1}_{#2}}
\newcommand\eqJ[1]{\objeq{\J}{#1}}

\newcommand\ciet{\cindeind{i}{\ltt}}                         % ||C_i||^t
\newcommand\ctet{\cindeind{t}{\ltt}}                         % ||C_t||^t
\newcommand\cjet{\cindeind{j}{\ltt}}                         % ||C_i||^t
\newcommand\cket{\cindeind{k}{\ltt}}                         % ||C_t||^t
\newcommand\clet{\cindeind{l}{\ltt}}                         % ||C_i||^t


\newcommand\cieJ{\ceind{\J}}
%\newcommand\cjeJ{\ceind{\J}}

% function:
\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}           %      C^#1
\newcommand\ceindl[2]{\mbox{$_{#1}\semm{\AClass}^{#2}$}}     % _{#1}C^{#2}
\newcommand\ceindr[2]{\mbox{$\semm{\AClass}_{#1}^{#2}$}}     %      C_{#1}^{#2}

%  apply:
\newcommand\ctu{\mbox{$^{\ltt}\!\AClass^{\ltu}$}}
\newcommand\ctplusu{\cindr{+\ltu}{\ltt}}
\newcommand\ctnullu{\cindr{0\ltu}{\ltt}}
\newcommand\cuminust{\cindl{-\ltt}{\ltu}}
\newcommand\cunullt{\cindl{0\ltt}{\ltu}}

%\newcommand\cetu{\cind{\ltt\ltu}}
\newcommand\cetplusu{\ceindr{+\ltu}{\ltt}}
\newcommand\cetnullu{\ceindr{0\ltu}{\ltt}}
\newcommand\ceuminust{\ceindl{-\ltt}{\ltu}}
\newcommand\ceunullt{\ceindl{0\ltt}{\ltu}}

% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
\newcommand\dm{\TargetClass}                              %   D

\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||
\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
\renewcommand\det{\deind{\ltt}}                         % ||C||^t
\newcommand\deu{\deind{\ltu}}                         % ||C||^u
\newcommand\des{\deind{\lts}}                         % ||C||^u
\newcommand\dev{\deind{\tv}}                         % ||C||^u

\newcommand\deJ{\deind{\J}}

\newcommand\dindeind[2]{\mbox{$\semm{\TargetClass_{#1}}^{#2}$}}
%  apply
\newcommand\dies{\dindeind{i}{\lts}}                         % ||C||^t
\newcommand\djet{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\djeu{\dindeind{j}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\dieJ{\deind{\J}}
\newcommand\djeJ{\deind{\J}}
\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
\newcommand\dieu{\dindeind{i}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t


\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}           %      C^#1
\newcommand\deindl[2]{\mbox{$_{#1}\semm{\TargetClass}^{#2}$}}     % _{#1}D^{#2}
\newcommand\deindr[2]{\mbox{$\semm{\TargetClass}_{#1}^{#2}$}}     %      D_{#1}^{#2}


% apply
\newcommand\dtu{\mbox{$^{\ltt}\!\TargetClass^{\ltu}$}}
\newcommand\detplusu{\deindr{+\ltu}{\ltt}}
\newcommand\detnullu{\deindr{0\ltu}{\ltt}}
\newcommand\deuminust{\deindl{-\ltt}{\ltu}}
\newcommand\deunullt{\deindl{0\ltt}{\ltu}}


%\newcommand\f{\mbox{$\AReference$}}                    %   f
\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
%\newcommand\findl[2]{\mbox{$_{#1}\AReference^{#2}$}}     % _{#1}C^{#2}
%\newcommand\findr[2]{\mbox{$\AReference_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}           %      f^#1
\newcommand\feindl[2]{\mbox{$_{#1}\semm{\AReference}^{#2}$}}     % _{#1}C^{#2}
\newcommand\feindr[2]{\mbox{$\semm{\AReference}_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\ftu{\find{\ttu}}

\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
\renewcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fet{\feind{\ltt}}
\newcommand\fes{\feind{\lts}}
\newcommand\feu{\feind{\ltu}}
\newcommand\fev{\feind{\tv}}
\newcommand\feJ{\feind{\J}}

\newcommand\femt{\mbox{$\semm{\AReference^{-1}}^{\ltt}$}}


\newcommand\findeind[2]{\mbox{$\semm{\AReference_{#1}}^{#2}$}}
\newcommand\fieu[1]{\findeind{#1}{\ltu}}
\newcommand\fiet[1]{\findeind{#1}{\ltt}}
\newcommand\fies[1]{\findeind{#1}{\lts}}                         % ||C||^t
%\newcommand\fiet{\findeind{i}{\ltt}}                         % ||C||^t
\newcommand\fjet{\findeind{j}{\ltt}}                         % ||C||^t
\newcommand\fket{\findeind{k}{\ltt}}                         % ||C||^t
\newcommand\flet{\findeind{l}{\ltt}}                         % ||C||^t
\newcommand\fkeu{\findeind{k}{\ltu}}                         % ||C||^t

\newcommand\fetplusu{\feindr{+\ltu}{\ltt}}
\newcommand\fetnullu{\feindr{0\ltu}{\ltt}}
\newcommand\feuminust{\feindl{-\ltt}{\ltu}}
\newcommand\feunullt{\feindl{0\ltt}{\ltu}}



%\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
%\newcommand\djes{\dindeind{j}{\lts}}                         % ||C||^t

\newcommand\fieJ{\feind{\J}}
\newcommand\fjeJ{\feind{\J}}

\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% The old version where \tj denotes t, \tk denotes u  etc
%%% The new version see on line 185

\newcommand\tjk{\EarlierMoment\LaterMoment}   %jk
\newcommand\tj{\EarlierMoment}               %j
\newcommand\tk{\LaterMoment}                  %k
\newcommand\tjlk{\mbox{$\tj\le\kt$}}
\newcommand\ti{\EarlierEarlierMoment}        %i
\newcommand\tl{\LaterLaterMoment}             %l

%\newcommand\J{\AHistory}                      %J

\newcommand\interjk[1]{\inter{\tjk}{#1}}                 % \eps^jk_#1
\newcommand\dominterjk[1]{\ldom{\interjk{#1}}}  %\Box\eps^jk_#1
\newcommand\codinterjk[1]{\rdom{\interjk{#1}}}  %\eps^jk_#1\Box

\newcommand\interjj[1]{\inter{\tj\tj}{#1}}                 % \eps^jk_#1
\newcommand\interij[1]{\inter{\ti\tj}{#1}}                 % \eps^jk_#1
%\newcommand\interjk[1]{\inter{\tj\tk}{#1}}                 % \eps^jk_#1
\newcommand\interik[1]{\inter{\ti\tk}{#1}}                 % \eps^jk_#1


\newcommand\intercjj{\inter{\tj\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercij{\inter{\ti\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercjk{\inter{\tj\tk}{\cm}}                 % \eps^jk_#1
\newcommand\intercik{\inter{\ti\tk}{\cm}}                 % \eps^jk_#1

\newcommand\domintercjk{\dominterjk{\cm}}  %\Box\eps^jk_#1
\newcommand\codintercjk{\codinterjk{\cm}}  %\eps^jk_#1\Box

\newcommand\interdjj{\inter{\tj\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdij{\inter{\ti\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdjk{\inter{\tj\tk}{\dm}}                 % \eps^jk_#1
\newcommand\interdik{\inter{\ti\tk}{\dm}}                 % \eps^jk_#1

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C

%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||
%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1
\newcommand\cej{\ceind{\tj}}                         % ||C||^j
\newcommand\cek{\ceind{\tk}}                         % ||C||^k
%\newcommand\ceJ{\ceind{\J}}
%--- function:
%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
\newcommand\ciej{\cindeind{i}{\tj}}                         % ||C_i||^j
\newcommand\cjej{\cindeind{j}{\tj}}                         % ||C_j||^j
\renewcommand\cieJ{\ceind{\J}}
\newcommand\cjeJ{\ceind{\J}}

% function:
%\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
%\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
%\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}
%  apply:
\newcommand\cjk{\cind{\tj\tk}}
\newcommand\cjplusk{\cindr{+\tk}{\tj}}
\newcommand\cjnullk{\cindr{0\tk}{\tj}}
\newcommand\ckminusj{\cindl{-\tj}{\tk}}
\newcommand\cknullj{\cindl{0\tj}{\tk}}


% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
%\renewcommand\dm{\TargetClass}                              %   D

%\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
%\newcommand\dindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}

%\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
%\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
%\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}



%  Apply:
\newcommand\dej{\deind{\tj}}                         % ||C||^j
\newcommand\dek{\deind{\tk}}                         % ||C||^k
%\newcommand\deJ{\deind{\J}}

\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
%\newcommand\dieJ{\deind{\J}}
%\newcommand\djeJ{\deind{\J}}

\newcommand\djk{\dind{\tj\tk}}
\newcommand\djplusk{\dindr{+\tk}{\tj}}
\newcommand\djnullk{\dindr{0\tk}{\tj}}
\newcommand\dkminusj{\dindl{-\tj}{\tk}}
\newcommand\dknullj{\dindl{0\tj}{\tk}}


%\renewcommand\f{\mbox{$\AReference$}}                    %   f
%\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
\newcommand\fjk{\find{\tjk}}

%\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
%\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fej{\feind{\tj}}
\newcommand\fei{\feind{\ti}}
\newcommand\fek{\feind{\tk}}
\newcommand\fel{\feind{\tl}}

%\newcommand\feJ{\feind{\J}}

%\newcommand\findeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
%\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
%\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
\newcommand\fiei{\findeind{i}{\ti}}                         % ||C||^j
\newcommand\fjej{\findeind{j}{\tj}}                         % ||C||^j
%\newcommand\fieJ{\feind{\J}}
%\newcommand\fjeJ{\feind{\J}}

%\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Distinctctu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}_{\cm}}^{\ltu}$}}
\newcommand\Distinctcst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}_{\cm}}^{\ltt}$}}
\newcommand\Samectu{\mbox{$^{\ltt}\!\semm{\ittt{Same}_{\cm}}^{\ltu}$}}
\newcommand\Samecst{\mbox{$^{\lts}\!\semm{\ittt{Same}_{\cm}}^{\ltt}$}}
%=============
%%%%% Behset
\newcommand\xstatei[3]{\mbox{${\mathit {#1}state}^{#3}_{#2}$}}
\newcommand\statei[2]{\xstatei{}{#1}{#2}}
\newcommand\xstate[2]{\xstatei{#1}{}{#2}}
%\newcommand\tstatei[1]{\statei{#1}{\ltt}}

\newcommand\attrName[1]{{\mathit #1}}
\newcommand\methName[1]{{\mathit #1}}
\newcommand\statepoint[1]{#1}

%%%%%
% discussing string-based  vs graph-based logics
\newcommand\cmlang{{\bf L}}
\newcommand\myindex[1]{\mbox{\scriptsize{#1}}}
\newcommand\mathsymbol[1]{\mbox{$#1$}}
%\newcommand\repr{\mathsymbol{r}}
\newcommand\world%{\ittt{world}}
{\mathsymbol{\cal W}}
\newcommand\cmter%{\ittt{computer}}
{\mathsymbol{\cal C}}
\newcommand\topos{\mathsymbol{\cal S}}


%----------------------
\newcommand\viewob[1]{\object{V}{#1}}
\newcommand\thob[1]{\object{T}{#1}}
\newcommand\uniob[1]{\object{U}{#1}}
\newcommand\uniobmath[1]{\objectmath{U}{#1}}
\newcommand\uniobind[1]{\objectind{U}{#1}}

\newcommand\UNI{\universe{U}}
\newcommand\UNIind{\universeind{U}}
\newcommand\UNImath{\universeind{U}} % the same
\newcommand\Setsind{\universeind{Sets}}

\newcommand\particularUni[1]{\mbox{$\mathbf{#1}$}}
\newcommand\particularUniInd[1]{\mathbf{#1}}
\newcommand\Sets{\particularUni{Sets}}
\newcommand\Varsets{\particularUni{VarSets}}
\newcommand\Behsets{\particularUni{BehSets}}
\newcommand\Sketches{\particularUni{Sketches}}


\newcommand\skeproc{\proc{ske}}
\newcommand\arrdlproc{\procind{Formal}{ArrDL}}
\newcommand\elmslproc{\procind{Formal}{ElmSL}}

%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
\newcommand\formalParBold[1]{\mbox{$#1$}}
\newcommand\lf{\formalParBold{L}}
\newcommand\mf{\formalPar{M(D)}}
\newcommand\uf{\formalPar{U}}
\newcommand\df{\formalPar{D}}
\newcommand\tdf{\mbox{$\thob(\diag)$}}
\newcommand\sdf{\mbox{$\skeob{}(\diag)$}}

\newcommand\str{\formalPar{\sigma}}
%(7)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Created on May 4,2001
%============================================
% Part 1: pure italic writing of names
%        formerly file italic.tex
%--------------------------------------------
% Part 2: commands for semantics extensions of classes
%         like [[Person]]^t or {^t}[[SamePerson]]^{u}
%        formerly file employ.tex
%===========================================

\newcommand\operarrow[2]{\mbox{{\sffamily%\itshape
#1}$_{#2}$}}
\newcommand\projop[1]{\operarrow{p}{#1}}
%\newcommand\concatop{\operarrow{concat}{}}
%\newcommand\pairop{\operarrow{pair}{}}
%\newcommand\idop[1]{\operarrow{id}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\ltt{\mbox{$t$}}
%\newcommand\ltu{\mbox{$u$}}
%\newcommand\lts{\mbox{$s$}}

%

\newcommand\Emplsem[1]{\mbox{$\semm{\Empl}^{#1}$}}
\newcommand\Emplt{\Emplsem{\ltt}}
\newcommand\Emplu{\Emplsem{\ltu}}
\newcommand\Empls{\Emplsem{\lts}}
\newcommand\Empltu{\mbox{$^{\ltt}\!\semm{\Empl}^{\ltu}$}}
\newcommand\Emplst{\mbox{$^{\lts}\!\semm{\Empl}^{\ltt}$}}
\newcommand\SameEmpltu{\mbox{$^{\ltt}\!\semm{\SameEmpl}^{\ltu}$}}
\newcommand\SameEmplst{\mbox{$^{\lts}\!\semm{\SameEmpl}^{\ltt}$}}

\newcommand\Compsem[1]{\mbox{$\semm{\Comp}^{#1}$}}
\newcommand\Compt{\Compsem{\ltt}}
\newcommand\Compu{\Compsem{\ltu}}
\newcommand\Comps{\Compsem{\lts}}
\newcommand\Comptu{\mbox{$^{\ltt}\!\semm{\Comp}^{\ltu}$}}
\newcommand\Compst{\mbox{$^{\lts}\!\semm{\Comp}^{\ltt}$}}
\newcommand\SameComptu{\mbox{$^{\ltt}\!\semm{\SameComp}^{\ltu}$}}
\newcommand\SameCompst{\mbox{$^{\lts}\!\semm{\SameComp}^{\ltt}$}}

\newcommand\Engrsem[1]{\mbox{$\semm{\Engr}^{#1}$}}
\newcommand\Engrt{\Engrsem{\ltt}}
\newcommand\Engru{\Engrsem{\ltu}}
\newcommand\Engrs{\Engrsem{\lts}}
\newcommand\Engrtu{\mbox{$^{\ltt}\!\semm{\Engr}^{\ltu}$}}
\newcommand\Engrst{\mbox{$^{\lts}\!\semm{\Engr}^{\ltt}$}}

\newcommand\Mngrsem[1]{\mbox{$\semm{\Mngr}^{#1}$}}
\newcommand\Mngrt{\Mngrsem{\ltt}}
\newcommand\Mngru{\Mngrsem{\ltu}}
\newcommand\Mngrs{\Mngrsem{\lts}}
\newcommand\Mngrtu{\mbox{$^{\ltt}\!\semm{\Mngr}^{\ltu}$}}
\newcommand\Mngrst{\mbox{$^{\lts}\!\semm{\Mngr}^{\ltt}$}}

\newcommand\John[1]{\mbox{$\ittt{John}^{#1}$}}

\newcommand\Marr{\ittt{Married}}
\newcommand\Marrsem[1]{\mbox{$\semm{\Marr}^{#1}$}}
\newcommand\Marrt{\Marrsem{\ltt}}
\newcommand\Marru{\Marrsem{\ltu}}
\newcommand\Marrs{\Marrsem{\lts}}
\newcommand\Marrtu{\mbox{$^{\ltt}\!\semm{\Marr}^{\ltu}$}}
\newcommand\Marrst{\mbox{$^{\lts}\!\semm{\Marr}^{\ltt}$}}

\newcommand\Famy{\ittt{Family}}
\newcommand\Famysem[1]{\mbox{$\semm{\Famy}^{#1}$}}
\newcommand\Famyt{\Famysem{\ltt}}
\newcommand\Famyu{\Famysem{\ltu}}
\newcommand\Famys{\Famysem{\lts}}
\newcommand\Famytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Famyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Famytt{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Familytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Familyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}

\newcommand\Friendship{\ittt{Friendship}}
\newcommand\Friship{\ittt{Friendship}}
\newcommand\Frishiptu{\mbox{$^{\ltt}\!\semm{\Friship}^{\ltu}$}}
\newcommand\Frishipst{\mbox{$^{\lts}\!\semm{\Friship}^{\ltt}$}}


\newcommand\Matr{\ittt{Matrimony}}
\newcommand\Matrsem[1]{\mbox{$\semm{\Matr}^{#1}$}}
\newcommand\Matrt{\Matrsem{\ltt}}
\newcommand\Matru{\Matrsem{\ltu}}
\newcommand\Matrs{\Matrsem{\lts}}
\newcommand\Matrtu{\mbox{$^{\ltt}\!\semm{\Matr}^{\ltu}$}}
\newcommand\Matrst{\mbox{$^{\lts}\!\semm{\Matr}^{\ltt}$}}

\newcommand\Distincttu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}}^{\ltu}$}}
\newcommand\Distinctst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}}^{\ltt}$}}
\newcommand\Sametu{\mbox{$^{\ltt}\!\semm{\ittt{Same}}^{\ltu}$}}
\newcommand\Samest{\mbox{$^{\lts}\!\semm{\ittt{Same}}^{\ltt}$}}

\newcommand\Wom{\ittt{Woman}}
\newcommand\Womsem[1]{\mbox{$\semm{\Wom}^{#1}$}}
\newcommand\Womt{\Womsem{\ltt}}
\newcommand\Womu{\Womsem{\ltu}}
\newcommand\Woms{\Womsem{\lts}}
\newcommand\Womtu{\mbox{$^{\ltt}\!\semm{\Wom}^{\ltu}$}}
\newcommand\Womst{\mbox{$^{\lts}\!\semm{\Wom}^{\ltt}$}}

%\newcommand\Man{\ittt{Man}}
\newcommand\Mansem[1]{\mbox{$\semm{\Man}^{#1}$}}
\newcommand\Mant{\Mansem{\ltt}}
\newcommand\Manu{\Mansem{\ltu}}
\newcommand\Mans{\Mansem{\lts}}
\newcommand\Mantu{\mbox{$^{\ltt}\!\semm{\Man}^{\ltu}$}}
\newcommand\Manst{\mbox{$^{\lts}\!\semm{\Man}^{\ltt}$}}

\newcommand\Husbsem[1]{\mbox{$\semm{\Husb}^{#1}$}}
\newcommand\Husbt{\Husbsem{\ltt}}
\newcommand\Husbu{\Husbsem{\ltu}}
\newcommand\Husbs{\Husbsem{\lts}}
\newcommand\Husbtu{\mbox{$^{\ltt}\!\semm{\Husb}^{\ltu}$}}
\newcommand\Husbst{\mbox{$^{\lts}\!\semm{\Husb}^{\ltt}$}}


\newcommand\mysemm[2]{\mbox{$\semm{#1}^{#2}$}}

\newcommand\isarrt{\mysemm{\isa}{\ltt}}
\newcommand\isarru{\mysemm{\isa}{\ltu}}

\newcommand\wifet{\mysemm{\wife}{\ltt}}
\newcommand\wifeu{\mysemm{\wife}{\ltu}}

\newcommand\husbt{\mysemm{\husb}{\ltt}}
\newcommand\husbu{\mysemm{\husb}{\ltu}}

\newcommand\mdatet{\mysemm{\mDate}{\ltt}}
\newcommand\mdateu{\mysemm{\mDate}{\ltu}}

\newcommand\liveset{\mysemm{\livesAt}{\ltt}}
\newcommand\liveseu{\mysemm{\livesAt}{\ltu}}

\newcommand\income{\ittt{income}}
\newcommand\WMHsem[2]{\mbox{$
(\semm{\Wom}^{#1}\times\semm{\Man}^{#1}\times\semm{\House}^{#1})
\times
(\semm{\Wom}^{#2}\times\semm{\Man}^{#2}\times\semm{\House}^{#2})
$}
}
\newcommand\WMHtu{\WMHsem{\ltt}{\ltu}}


\newcommand\WMWMsem[2]{\mbox{$(\semm{\Wom}^{#1}\times\semm{\Man}^{#1})
\times(\semm{\Wom}^{#2}\times\semm{\Man}^{#2})
$}
}
\newcommand\WMWMtu{\WMWMsem{\ltt}{\ltu}}


\newcommand\myview[1]{\mbox{$V_{#1}$}}
\newcommand\IndI{1}
\newcommand\SWAggr{2}
\newcommand\AggrI{3}
\newcommand\TWAggrG{4}
\newcommand\IndII{5}
\newcommand\TWAggrS{6}
\newcommand\LAggr{7}
\newcommand\LLAggr{8}
\newcommand\SWLAggr{9}
\newcommand\STWAggr{10}
\newcommand\DelAggr{11}
\newcommand\TotAggr{12}
\newcommand\WQual{13}
\newcommand\LQual{14}
\newcommand\AttrI{15}
\newcommand\SWLQual{16}
\newcommand\STWQual{17}
\newcommand\AttrII{18}



%(8)
%\newcommand\s{\mbox{$S$}}
%\newcommand\os{\mbox{$\overline{S}$}}
%\newcommand\ovr[1]{\mbox{$\overline{#1}$}}
\newcommand\into[1]{\stackrel{#1}{\hookrightarrow}}
\newcommand\repgra{\nicex{ R$}}
\newcommand\rgra{\repgra}
\newcommand\nds[1]{\mbox{$\mathit{Nds}#1$}}
\newcommand\arrs[1]{\mbox{$\mathit{Arrs}#1$}}
\newcommand\ndsr{\nds{\rgra}}
\newcommand\arrsr{\arrs{\rgra}}

\newcommand\dersetmath{\mathit{Der}}
\newcommand\derset{\mbox{$\dersetmath$}}
\newcommand\derop{\mbox{$\mathbf{der}$}}
\newcommand\algebra[1]{\mbox{$\alpha^{#1}$}}
\newcommand\algu{\algebra{\uskemath}}

%\newcommand\inss[1]{\lar{I}{\ske{#1}}{\uske}}
%\newcommand\ovri{\mbox{$\overline{I}$}}
%\newcommand\ovrinss[1]{\lar{\ovri_{#1}}{\ovrs{#1}}{\uske}}

\newcommand\ovrske[1]{\mbox{$\overline{\ske{#1}}$}}
\newcommand\ovrs[1]{\mbox{$\overline{\ske{#1}}$}}
%-----------------------------
\newcommand\sv{\mbox{$\ske{V}$}}
\newcommand\sr{\mbox{$\ske{R}$}}
\newcommand\vmor{\lar{v}{\sv}{\ovrske{}}}
\newcommand\rmor{\lar{r}{S}{\ovrske{R}}}
\newcommand\emor{\lar{e}{S}{\U}}
\newcommand\vpair{\mbox{$V=(\sv,v)$}}
\newcommand\rpair{\mbox{$R=(\sr,r)$}}



%\newcommand\dbinst{\lar{e}{S}{W} }

%---------------------------------------------------


\newcommand\ovrsig[1]{\mbox{$\overline{\sigma _{#1}}$}}
\newcommand\ovrg[1]{\mbox{$\overline{G_{#1}}$}}
%-----------------------------------------
\newcommand\ovrp{\mbox{$\overline{\pi }$}}%{#1}}$}}
\newcommand\ovreps{\mbox{$\overline{\vare}$}}     % overlined epsilon


%\renewcommand\endinput{}
%\newcommand\comp{\mathbin{\triangleright\!\!\triangleright}}
\newcommand\state[2]{\mbox{${\mathit{state}}^{#1}_{#2}$}}
\newcommand\starInherit{*-inherit}

\newcommand\sig{\mbox{$\Sigma $}}
\newcommand\sigm{\Sigma}
\newcommand\defitemotstup[1]{\par\smallskip\noindent (#1)}


\newcommand\arity[1]{\mbox{$\mathit{Arity}(#1)$}}
\newcommand\predsem[2]{\mbox{$\semm{#1}^{#2} $}}
\newcommand\psem[1]{\predsem{P}{#1}}
\newcommand\psemu{\psem{\ucatmath}}
\newcommand\lsig{\mbox{$\Lambda $}}

%%%
\newcommand\Attr{\mbox{$\mathit{Attr}$}}
\newcommand\Var{\mbox{$\mathit{Var}$}}
\newcommand\relcat{\mbox{$\categoryname{Rel}$}}
\newcommand\relske{\mbox{$\sketchname{Rel}$}}
\newcommand\itte[1]{\mbox{\textit{#1}}}
\newcommand\dbcat{\mbox{$\categoryname{DB}$}}

\newcommand\skecat[1]{\mbox{$\categoryname{Sketch}(\sig_{#1})$}}
\newcommand\sigcat{\mbox{$\categoryname{Sign}$}}

\newcommand\funor{\mbox{$\Phi$}}
\newcommand\funarr{\lar{f}{X}{Y}}
\newcommand\currfun{\mbox{\lar{\Map{A}{\_}}{\catset}{\catset}}}
\newcommand\curra{\Map{A}{\_}}

% \newcommand\ {\itte{ }}
\newcommand\target{\itte{target}}
\newcommand\source{\itte{source}}
\newcommand\conof{\itte{consistsOf}}
\newcommand\marker{\itte{marker}}
\newcommand\Node{\itte{Node}}
\newcommand\nodeit{\ittt{node}}
\newcommand\Arrow{\itte{Arrow}}
\newcommand\arrow{\ittt{arrow}}
\newcommand\diagramit{\itte{diagram}}
\newcommand\graphit{\itte{graph}}
\newcommand\shape{\itte{shape}}
\newcommand\predecl{\itte{predicate\_declarations}}
\newcommand\statements{\itte{statements}}
\newcommand\carrier{\itte{carrier}}
\newcommand\arityshape{\itte{arity\_shape}}


% semiotics
%% MACROS OF Dec 3
\newcommand\formalObj[1]{\mbox{\sffamily #1}}
\newcommand\formalOper[1]{\mbox{{\bfseries\sffamily #1}}}
\newcommand\informalObj[1]{\mbox{\textit #1}}
\newcommand\informalOper[1]{\mbox{{\bfseries\itshape #1}}}

\newcommand\lzzl{\formalObj{l}}  %logic
\newcommand\ml{\informalObj{ML}}  % modeling language

\newcommand\f{\formalObj{F}}
\renewcommand\c{\informalObj{C}}
\newcommand\derf{\formalOper{Der}}
\newcommand\deri{\informalOper{Un}}
\newcommand\derff{\derf.\f}
\newcommand\deric{\deri(\c)}
\newcommand\FormalInterpret[1]{\mbox{$\formalObj{i}_f$}}
\newcommand\SubstantInterpret[1]{\mbox{$\informalObj{i}_s$}}


%====================================

\newcommand\informalPar[1]{\nicex{{#1}$}}
\newcommand\infParind[1]{\cal #1}
\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
\newcommand\frmParind[1]{\mathrm{#1}}

\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}

\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%\newcommand\object[2]{\mbox{$#1_{#2}$}}
\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectmath[1]{\mathsf{#1}} % the same
\newcommand\universeind[1]{\mathbf{#1}}
\newcommand\umath[1]{\mathbf{U}_{#1}}

\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
\newcommand\linf{\informalParBold{L}}
\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
\newcommand\uinf{\informalPar{U}}

\newcommand\meaninf{\informalPar{M}}
\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}

\newcommand\diags{\mbox{$\mathit{Diags}$}}
\newcommand\graph{\mbox{$\mathit{Graph}$}}

\newcommand\diaob[1]{\object{D}{#1}} %\mbox{$D$}}
\newcommand\diagob[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diag[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diaind{\objectind{D}}

\newcommand\graob[1]{\object{G}{#1}}
\newcommand\graind{\objectind{G}}
\newcommand\gra[1]{\graob{#1}}

\newcommand\skeob[1]{\object{S}{#1}}
\newcommand\skeind{\objectind{S}}

\newcommand\modelob[1]{\object{M}{#1}}
\newcommand\modelind{\objectind{M}}

\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
\newcommand\skediag{\skeob{}[\diag{}]}

\newcommand\meaninfdiag{\meaninf[\diag{}]}
\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
% synonyms
\newcommand\meanifdiag{\meaninf[\diag{}]}
\newcommand\meanfdiag{\meanfrm[\diag{}]}

%%% diags, sketchs, specs, and their semantic interpretaions
\newcommand\objectWithInd[3]{\mbox{$\mathsf{#1}_{#2}^{#3}$}}
\newcommand\sketch[1]{\objectWithInd{S}{#1}{}}
\renewcommand\ske[1]{\sketch{#1}}
%\newcommand\graph[1]{\objectWithInd{S}{#1}{}}
\renewcommand\diag[1]{\objectWithInd{D}{#1}{}}
%\newcommand\inst[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}
%\newcommand\instob[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}


%\newcommand\diaob[1]{\mbox{$\diag{#1}$}}
%\newcommand\skeob{\mbox{$S$}}
\newcommand\graofske{\mbox{$G_\skeind$}}
\newcommand\graske{\graofske}
\newcommand\diaofske{\mbox{$D_\skeind$}}
\newcommand\diaske{\diaofske}


\renewcommand\eg{e.g.}
\renewcommand\C{\mbox{$C$}}

\newcommand\ext[1]{\mbox{$\mathit{Ext}(#1)$}}
\renewcommand\stt[1]{\mbox{$\mathit{Stt}(#1)$}}
\newcommand\GCS{{\bf (GCS)}}
\newcommand\AET{{\bf (AET)}}



%\newcommand\tuple[1]{\left [ \mathstrut {#1} \right ]}
\newcommand\pmrk[1]{\mbox{[{\sf #1}]}}
\newcommand\omrk[1]{\mbox{[{\sf #1} $\rangle $}}

% used in Intro
\newcommand\lanfrm{\formalPar{FL}}
\newcommand\flan{\formalPar{FL}} %the same
\newcommand\flanind{\frmParind{FL}}

\newcommand\x{\diag{}}   %\mbox{$D$}}
\renewcommand\s{\skeob{}}%\mbox{$S$}}
%\newcommand\mix{\mbox{$\meaninf$}} %(\x)
%\newcommand\mfx{\mbox{$\meanfrm{\flanind}$}} %(\x)
\newcommand\mix{\mbox{$\meaninf(\x)$}}
\newcommand\mfx{\mbox{$\meanfrm{}(\x)$}}

%\newcommand\flan{\mbox{$\meanfrm(\x)$}}

\newcommand\spex[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spem[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spexl  {\mbox{$\skeob{\flanind}$}} %(\x)$}}
\newcommand\speml  {\mbox{$\skeob{}$}} %(\mfx)$}}

\newcommand\dateit{\ittt{date}}

% used in dGetStartViaAss
\newcommand\nis{\nicex{ S$}}
\newcommand\niv{\nicex{ V$}}
\newcommand\nivind{{V}}
\newcommand\nisind{{S}}

\newcommand\mrkdual[3]{\mbox{${#2}\stackrel{{\cal\scriptsize #1}}{[><]}{#3}$}} %{[>^{\mathrm{#1}}<]}$}}
\newcommand\sgv{single-valued}
\newcommand\assgenpred{\mbox{$[\Uparrow]$}}
\newcommand\SepPred{\mrk{1-1}  }
\newcommand\CovPred{\mrk{cover}}
\newcommand\MemPred{\mrk{$\in$}}

\newcommand\binAss{1}
\newcommand\assCla{2}
\newcommand\reiAss{3}
\newcommand\terAss{4}
\newcommand\quaAss{5}
\newcommand\skeo{\skeob{\binAss}}
\newcommand\skei{\skeob{\assCla}}
\newcommand\skeii{\skeob{\reiAss}}
\newcommand\skeiii{\skeob{\terAss}}
\newcommand\skeiv{\skeob{\quaAss}}
%\newcommand\diaob[1]{\diag{#1}}
\newcommand\diao{\diaob{\binAss}}
\newcommand\diai{\diaob{\assCla}}
\newcommand\diaii{\diaob{\reiAss}}
\newcommand\diaiii{\diaob{\terAss}}
\newcommand\diaiv{\diaob{\quaAss}}


\newcommand\visfunctor{\mbox{{\sffamily\bfseries vis}}}
\newcommand\skefunctor{\mbox{{\sffamily\bfseries ske}}}

%used in eAssonBySke
\newcommand\sale{\ittt{sale}}
\newcommand\Show{\ittt{Show}}
\renewcommand\show{\ittt{show}}
\newcommand\seat{\ittt{seat}}
\newcommand\perf{\ittt{perf}}
\newcommand\Performance{\ittt{Performance}}
\newcommand\Ticket{\ittt{Ticket}}
\newcommand\ticket{\ittt{sale}}
\newcommand\Integer{\ittt{Integer}}

\newcommand\mastr[1]{\mbox{$\mathbf{#1}$}}
\newcommand\extofcla[1]{\mastr{\semm{\mathit #1}}}
\newcommand\behofcla[1]{\mastr{\besemm{\mathit{#1}}}}
\newcommand\sttofcla[1]{\lar{\statemap{}{\mathit{#1}}}{\extofcla{#1}}{\behofcla{#1}}}

%\newcommand\tlu{\mbox{$t<u$}}
%\newenvironment\mathitext%
%{
%\begin{displaymath}
%\mbox{ }
%\end{displaymath}
%} {}
\newcommand\cEngine{\ittt{carEngine}}
\newcommand\carEngine{\ittt{carEngine}}


\newcommand\mrkmon[2]{\mbox{\mrk{1-1}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkfro[2]{\mbox{\mrk{fro}$^{#1}_{\mathit{#2}}$}}
\renewcommand\mrkid[2]{\mbox{\mrk{id}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkstrongid[2]{\mbox{\mrk{id!}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkdel[2]{\mbox{\mrk{del}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkins[2]{\mbox{\mrk{ins}$^{#1}_{\mathit{#2}}$}}

\newcommand\mathand{\mbox{ and }}
\newcommand\mathor{\mbox{ or }}
\newcommand\mathif{\mbox{ if }}
\newcommand\maththen{\mbox{ then }}
\newcommand\mathiff{\mbox{ iff }}
%\newcommand\ofit{\ittt{of}}
\newcommand\wholeit{\ittt{whole}}
\newcommand\Wholeit{\ittt{Whole}}
\newcommand\partit{\ittt{part}}
\newcommand\stateit{\ittt{state}}
\newcommand\prokol{{\mathbf +}\!\!\!\!\circ}

\newcommand\mixsemm[1]{\mbox{$\lbesemm\, {\mathit #1} \, \rsemm$}}

\newcommand\logrule[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleFig[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleRow[2]{\mbox{if $#1$ then $#2$}}
\newcommand\logruleFigText[2]{\mbox{$
\frac{\mbox{\rule[-1ex]{0pt}{3ex} #1}}{\mbox{\rule{0pt}{3ex} #2}} $}
}
\newcommand\logruleRowText[2]{\mbox{if #1 then #2}}


\newcommand\ClassIndInd[3]{\mbox{$^{#1}\!\semm{\mathit{#2}}^{#3}$}}
\newcommand\ClassBeh[1]{\mbox{$\besemm{\mathit{#1}}$}}

\newcommand\refInd[2]{\mbox{$\semm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refBehInd[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refIndBeh[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}




\renewcommand\same[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
\newcommand\samemap[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
%\newcommand\sametu[1]{\samemap{tu}{#1}}
\newcommand\delset[3]{\mbox{$\semm{#3}^{#1}\mathsf{Del}^{#1\rightarrow #2}$}}
\newcommand\deltu[1]{\delset{t}{u}{#1}}
\newcommand\newset[3]{\mbox{$\semm{#3}^{#1}\mathsf{New}^{#2\rightarrow #1}$}}
\newcommand\newut[1]{\newset{u}{t}{#1}}
\newcommand\newts[1]{\newset{t}{s}{#1}}
%\newcommand\insut[1]{\newset{t}{u}{#1}}
%\newcommand\newut[1]{\newset{t\leftarrow u}{#1}} %  correct
%\newcommand\newtu[1]{\newset{t\leftarrow u}{#1}} % incorrect, to match old
%\newcommand\newts[1]{\newset{s\leftarrow t}{#1}} %correct,
%\newcommand\newst[1]{\newset{s\leftarrow t}{#1}} %incorrect, to match old
\newcommand\statemap[2]{\mbox{${\mathit{state}}^{#1}_{\mathit{#2}}$}}



\newcommand\ofit{\ittt{of}}
\newcommand\ofmap[1]{\refInd{of}{#1}}
%\newcommand\ofit{\ofmap{}}
\newcommand\oft{\ofmap{t}}
\newcommand\ofu{\ofmap{u}}

\newcommand\ofindit{\mbox{$\semm{{\mathit of}_i}^{t}$}}
%\newcommand\ofindiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
\newcommand\ofiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
%
\newcommand\isit{\ittt{is}}
\newcommand\ismap[1]{\refInd{is}{#1}}
%\newcommand\isit{\ismap{}}
\newcommand\ist{\ismap{t}}
\newcommand\isu{\ismap{u}}


\newcommand\isindt{\mbox{$\semm{{\mathit is}_i}^{t}$}}
\newcommand\isindu{\mbox{$\semm{{\mathit is}_i}^{u}$}}
%

\newcommand\hasit{\ittt{has}}
\newcommand\hasmapbeh{\besemm{has}}
\newcommand\hasbeh{\besemm{has}}
\newcommand\hasbehind[1]{\besemm{has}_{#1}}


\newcommand\supmap[1]{\refInd{sup}{#1}}
\newcommand\supit{\supmap{}}
\newcommand\supt{\supmap{t}}
\newcommand\supu{\supmap{u}}
%
\newcommand\supbeh{\besemm{sup}}
%
\newcommand\submap[1]{\refInd{sub}{#1}}
\newcommand\subit{\submap{}}
\newcommand\subt{\submap{t}}
\newcommand\subu{\submap{u}}

\newcommand\isamap[1]{\refInd{isA}{#1}}
\newcommand\isait{\isamap{}}
\newcommand\isat{\isamap{t}}
\newcommand\isau{\isamap{u}}
\newcommand\isabeh{\besemm{\isa}}

\newcommand\Persontu{\ClassIndInd{t}{Person}{u}}
\newcommand\Persont{\ClassIndInd{}{Person}{t}}
\newcommand\Personu{\ClassIndInd{}{Person}{u}}
\newcommand\PersonBeh{\ClassBeh{Person}}

\newcommand\Drivertu{\ClassIndInd{t}{Driver}{u}}
\newcommand\Drivert{\ClassIndInd{}{Driver}{t}}
\newcommand\Driveru{\ClassIndInd{}{Driver}{u}}



\newcommand\Cart{\ClassIndInd{}{Car}{t}}
\newcommand\Caru{\ClassIndInd{}{Car}{u}}
\newcommand\Cartu{\ClassIndInd{t}{Car}{u}}
\newcommand\SameCartu{\ClassIndInd{t}{SameCar}{u}}
\newcommand\CarBeh{\ClassBeh{Car}}
\newcommand\Carbeh{\ClassBeh{Car}}
\newcommand\Ownershiptu{\ClassIndInd{t}{Ownership}{u}}
\newcommand\Ownershipt{\ClassIndInd{}{Ownership}{t}}
\newcommand\Ownershipu{\ClassIndInd{}{Ownership}{u}}



\newcommand\Ownership{\ittt{Ownership}}
\newcommand\owner{\ittt{owner}}
%\newcommand\car{\ittt{car}}
%\newcommand\property{\ittt{property}}

%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
\newcommand\Enginetu{\ClassIndInd{t}{Engine}{u}}
\newcommand\Enginet{\ClassIndInd{}{Engine}{t}}
\newcommand\Engineu{\ClassIndInd{}{Engine}{u}}
\newcommand\EngineBeh{\ClassBeh{Engine}}
\newcommand\Enginebeh{\ClassBeh{Engine}}
\newcommand\Engbeh{\ClassBeh{Engine}}
\newcommand\BodyBeh{\ClassBeh{Body}}
\newcommand\ChassisBeh{\ClassBeh{Chassis}}


%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
%\newcommand\Body{\ittt{Body}}
%\newcommand\BodyBeh{\ClassBeh{Body}}
%\newcommand\Chassis{\ittt{Chassis}}
%\newcommand\ChassisBeh{\ClassBeh{Chassis}}
%%\newcommand\PartName{Part}

%\newcommand\drives{\ittt{drives}}
\newcommand\drivest{\refInd{drives}{t}}
\newcommand\drivesu{\refInd{drives}{u}}
\newcommand\drivesbeht{\refBehInd{drives}{t}}
\newcommand\drivesbehu{\refBehInd{drives}{u}}
\newcommand\drivesbehv{\refBehInd{drives}{v}}
\newcommand\drivesbeh{\refBehInd{drives}{}}

\newcommand\fuelat{\refInd{fuelAmount}{t}}
%\newcommand\fuelAm{\ittt{fuelAmount}}
%\newcommand\tankVo{\ittt{tankVolume}}
%\newcommand\fillTa{\ittt{fillTank}}
%\newcommand\car{\ittt{car}}

\newcommand\tankvt{\refInd{tankVolume}{t}}
\newcommand\tankvu{\refInd{tankVolume}{u}}

\newcommand\cart{\refInd{car}{t}}
\newcommand\caru{\refInd{car}{u}}

\newcommand\prst{\refInd{prs}{t}}
\newcommand\prsu{\refInd{prs}{u}}

\newcommand\enginet{\refInd{engine}{t}}
\newcommand\engineu{\refInd{engine}{u}}

\newcommand\persont{\refInd{person}{t}}
\newcommand\personu{\refInd{person}{u}}



\newcommand\PersonP{\Person$^+$}
\newcommand\PersonM{\Person$^-$}
\newcommand\CarP{\Car$^+$}
\newcommand\CarM{\Car$^-$}


\newcommand\floatRange[1]{\mrk{Float(#1)}}

%\newcommand\Car{\ittt{Car}}


\newcommand\becar{\besemm{\Car}}
\newcommand\beCar{\besemm{\Car}}
\newcommand\lt{$t$}
\newcommand\tstate{\statei{}{\ltt}}
\newcommand\stts{\statepoint{s}}



% === composition: begin
\newcommand\ipart[1]{\mbox{$\mathit{Part}_{#1}$}}
\newcommand\ipartmath[1]{\mathit{Part}_{#1}}
\newcommand\ipartbeh[1]{\mbox{$\besemm{\ipart{#1}}$}}

\newcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethbeh[1]{\mbox{$\besemm{\imeth{#1}}$}}
\renewcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethstar[1]{\mbox{$\mathit{Meth}^*_{#1}$}}
\newcommand\istameth[1]{\imethstar{#1}} %the same

\newcommand\iiface[1]{\mbox{$\mathbf{IFace}_{#1}$}}
\newcommand\iifacestar[1]{\mbox{$\mathbf{IFace}^*_{#1}$}}
\newcommand\iistaface[1]{\iifacestar{#1}} %the same


\newcommand\prodspace{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\prodspa{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\wholespace{\mbox{$\prod_{i}^*\ipartbeh{i}$}}

\newcommand\prodmeths{\mbox{$%\prod_{i}\imeth{i}
\methsset{prod}$}}
\newcommand\wholemeths{\mbox{$%\prod^*_{i}\imeth{i}
\someofmethsset{Prod}$}}
\newcommand\prodmethsbeh{\mbox{$\besemm{\prodmeths}$}}
\newcommand\wholemethsbeh[2]{\mbox{$\besemm{\someofmeths{#1}{#2}}$}}
\newcommand\prodiface{\mbox{$%\prod_{i}\iiface{i}
\iface{Prod}$}}
\newcommand\wholeiface{\mbox{$%\prod^*_{i}\iiface{i}
\ifacepartial{Prod}$}}



%\newcommand\reductmap[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\reductmap[2]{\mbox{$\mathit{red}^{\mathit{#1}}_{\mathit{#2}}$}}
%\newcommand\reductmapstar[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\red[2]{\reductmap{#1}{#2}}
\newcommand\redsta[1]{\reductmapstar{#1}}
\newcommand\projectmap[1]{\mbox{$\mathit{proj}_{\mathit{#1}}$}}
%\renewcommand\proj[1]{\projectmap{#1}}
\newcommand\fproj[1]{\mbox{$\pi_{#1}$}}


%==== composition: end =========

\renewcommand\Eng[1]{\mbox{$\mathit{Eng}^#1$}}
\renewcommand\eng[1]{\mbox{$\mathit{eng}^#1$}}
\newcommand\ETOC{\Eng{*}} %Engine methods transferred TO Cars
\newcommand\etoc{\eng{*}}
\newcommand\Etocbeh{\besemm{\Engine^*}}
\newcommand\etocind{EngIntoCar}
\newcommand\ctoeind{CarToEng}

\newcommand\me{\mbox{$m$}}
\newcommand\Me{\mbox{$\mathit{Meth}$}}

%\newcommand\meths1]{\mbox{$\mathit{meth}^{\mathit{#1}}$}}
\newcommand\methsset[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%the same
\newcommand\meths[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%  in short
\newcommand\mset[1]{\methsset{#1}}

\newcommand\imset[1]{\mbox{\methsset{}$_{#1}$}}
\newcommand\someofmethsset[1]{\mbox{$\mathit{#1}^{*}\mathsf{Meth}$}}
% in short
\newcommand\somset[1]{\someofmethsset{#1}}

\newcommand\iface[1]       {\mbox{$\mathit{#1}  \mathbf{IFace}$}}
\newcommand\ifacepartial[1]{\mbox{$\mathit{#1}^*\mathbf{IFace}$}}

\newcommand\methsbody[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
%  in short
\newcommand\mbody[2]{\methsbody{#1}{#2}}
\newcommand\msbody[2]{\mbox{$\besemm{\methsset{#1}}^{\mathit{#2}}$}} % the same
\newcommand\mmbody[1]{\msbody{#1}{}}



\newcommand\someofmethsiface[1]{\mbox{$\ifacepartial{#1}$}}
\newcommand\somface[1]{\someofmethsiface{#1}}

\newcommand\someofmethsbody[2]{\mbox{$\besemm{\someofmethsset{#1}}^{#2}$}}
\newcommand\sombody[2]{\someofmethsbody{#1}{#2}}

\newcommand\miface{\iface{\me}}

\newcommand\categoryname[1]{\mathbf{#1}}
\newcommand\sketchname[1]{\mathsf{#1}}

\newcommand\setcatmath{\categoryname{Sets}}
\newcommand\setskemath{\sketchname{Set}}
\newcommand\vsetcatmath{\categoryname{VarSet}}
\newcommand\bsetcatmath{\categoryname{BehSet}}
\newcommand\coalgcatmath{\categoryname{coAlg}}
\newcommand\coalgske{\sketchname{coAlg}}
\newcommand\erske{\sketchname{ER}}
\newcommand\ercat{\categoryname{ER}}
\newcommand\vsetske{\sketchname{VarSet}}
\newcommand\bsetske{\sketchname{BehSet}}

\newcommand\setcat{\mbox{$\setcatmath$}}
\renewcommand\setcat{\mbox{$\categoryname{Sets}$}}
\newcommand\gracat{\mbox{$\categoryname{Graphs}$}}
\newcommand\posetcat{\mbox{$\categoryname{Posets}$}}
\newcommand\catcat{\mbox{$\categoryname{Cats}$}}


\newcommand\vsetcat{\mbox{$\vsetcatmath$}}
\newcommand\bsetcat{\mbox{$\bsetcatmath$}}
\newcommand\coalgcat{\mbox{$\coalgcatmath$}}
\newcommand\setske{\mbox{$\setskemath$}}


\newcommand\univcat{\mbox{$\categoryname{U}$}}
\newcommand\ucatmath{\categoryname{U}}
\newcommand\univske{\mbox{$\sketchname{U}$}}
\newcommand\uskemath{\sketchname{U}}
\newcommand\ucat{\univcat}
\newcommand\uske{\univske}

\newcommand\instus[2]{\inst{\ske{#1}}{\ucatmath_{#2}}}
\newcommand\uni[1]{\mbox{$\univcat_{#1} $}}

\newcommand\reuniv{\univcat}
\newcommand\mapcatmath{\categoryname{Map}}
\newcommand\mapcat{\categoryname{Map}}
\newcommand\Map[2]{\mbox{$\mapcatmath(#1,#2)$}}
\newcommand\cariface{\iface{\car}}

\newcommand\rePlug{\ittt{rePlug}}
%=====================
%\input{../../Tools/Macros/m01-macroLogic.tex}

%=====================
%\input{../../Tools/Macros/m05-myStyle(razdels).tex}
\newtheorem{mydef}{\noindent Definition}
%\newtheorem{remark}{Remark}
\newtheorem{termin}{\noindent Terminology}

%% ===========================================================
%%the version where razdels are inside subsections not sections
%\newcounter{Razdel}[subsection]
%\newcommand\beginRazd[1]%
%{
%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par%\smallskip
%\noindent\refstepcounter{Razdel}%
%{\bf \thesubsection.\arabic{Razdel} #1} %\mylabel{#2}
%}
%%==========================================================

%% =========================================================
%%the version where razdels are inside sections not subsections
%\newcounter{RazDel}[section]
%\newcommand\beginRazD[1]%  2nd argument is dummy and inherited from old verion
%{
%\renewcommand\theRazDel{\thesection.\arabic{RazDel}}
%\par%\smallskip
%\noindent\refstepcounter{RazDel}%
%{\bf \thesection.\arabic{RazDel} #1} %\mylabel{#2}
%}
%%==============================================================
%
%%\newcommand\EndRazD{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%%\newcommand\EndRazd{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newcommand\EndRazD{\par\smallskip}
%\newcommand\EndRazd{\par\smallskip}
%%\renewcommand\EndRazD{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%%\renewcommand\EndRazd{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%\newcommand\remends{\par\smallskip}
%                   %{\mbox{\textbf{endRemark} $\blacktriangleright$}}
%
%
%\newenvironment{razdel}[2]{\beginRazd{#1}{Razd#2}}{\endRazd}
%\newenvironment{razd}[2]{\beginRazd{{%\itshape
%                                      \bfseries #1}}}{\EndRazd}
%%\newenvironment{razD}[2]{\beginRazD{#1}{RazD#2}}{\EndRazD}
%\newenvironment{razD}[2]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%\newenvironment{razzD}[1]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%
%% 1st argument is the title of the razdel,
%% 2nd - dummy, formerly it was for the label
%
%
%\newenvironment{defi}[1]{\beginRazdel{Definition.}  {Defi#1}}{\endRazdel}
%\newenvironment{cons}[1]{\beginRazdel{Construction.}{Cons#1}}{\endRazdel}
%\newenvironment{prop}[1]{\beginRazdel{Proposition.} {Prop#1}}{\endRazdel}
%\newenvironment{theo}[1]{\beginRazdel{Theorem.}     {Theo#1}}{\endRazdel}
%\newenvironment{coro}[1]{\beginRazdel{Corollary.}   {Coro#1}}{\endRazdel}
%\newenvironment{exam}[1]{\beginRazdel{Example.}     {Exam#1}}{\endRazdel}
%%\newenvironment{rema}[1]{\beginRazdel{Remark.}      {Rema#1}}{\endRazdel}
%\newenvironment{warn}[1]{\beginRazdel{Warning.}     {Warn#1}}{\endRazdel}
%\newenvironment{desc}[1]{\beginRazdel{Description.} {Desc#1}}{\endRazdel}
%\newenvironment{disc}[1]{\beginRazdel{Discussion.}  {Disc#1}}{\endRazdel}
%\newenvironment{conv}[1]{\beginRazdel{Convention.}  {Conv#1}}{\endRazdel}
%\newenvironment{nota}[1]{\beginRazdel{Notation.}    {Nota#1}}{\endRazdel}
%
%\newcommand\equnref[1]{Equation~(\ref{Equn#1})}
%\newcommand\equlref[1]{equality~(\ref{Equl#1})}
%%\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\consref[1]{Construction~\ref{Cons#1}}
%\newcommand\defref[1]{Definition~\ref{#1}}
%\newcommand\propref[1]{Proposition~\ref{Prop#1}}
%\newcommand\discref[1]{Discussion~\ref{Disc#1}}
%\newcommand\convref[1]{Convention~\ref{Conv#1}}
%\newcommand\notaref[1]{Notation~\ref{Nota#1}}
%\newcommand\descref[1]{Description~\ref{Desc#1}}
%\newcommand\remaref[1]{Remark~\ref{Rema#1}}
%\newcommand\examref[1]{Example~\ref{Exam#1}}
%\newcommand\cororef[1]{Corollary~\ref{Coro#1}}
%\newcommand\razdref[1]{Section~\ref{Razd#1}}
%%\newcommand\appref[1]{appendix~\ref{App#1}}    see pre_gen.tex
%%\newcommand\sectref[1]{section~\ref{Sect#1}}   ....
%%\newcommand\sectsectref[1]{sections~\ref{Razd#1}}
%%\newcounter{Razdel}[subsection]
%\newcommand\NachRazd[2]%
%{
%%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par\medskip\noindent%\refstepcounter{Razdel}%
%{\it #1} \mylabel{#2} }
%%\newcommand\end{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newenvironment{Example}{\NachRazd{Example}}{\end}
%\newenvironment{Remark} {\NachRazd{Remark}}{\end}
%\newenvironment{Warning}{\NachRazd{Warning}}{\end}
%=====================
%\input{../../Tools/Macros/m10-MMt-CASCON-Macros.tex}
\newcommand\instarr[1]{\mbox{$\lar{\statemap}{\igra{}{}}{#1}$}}
\newcommand\instarrt[1]{\mbox{$ \lar{\statemap}{\igraph{t}{}}{#1}$}}

\newcommand\idop{\mrksemiop{\times id}}
\newcommand\idos{\mrksemiop{+id}}

\newcommand\idoP{\mrkop{prod}}
\newcommand\idoS{\mrkop{sum}}

\newcommand\recop{\mrkop{rec}}
\newcommand\varop{\mrkop{var}}
%\newcommand\sumop{\mrkop{var}}

\renewcommand\owner{\textit{owner}}
\newcommand\types{\nicex{ T$}}

%% for Kleisly arrows section

\newcommand\ssma{\mbox{$S$}}
\newcommand\tsma{\mbox{$T$}}
\newcommand\usma{\mbox{$U$$$}}
\newcommand\mapelement{\mbox{$\rightsquigarrow$}}
\newcommand\mapel{\mapelement}

\newcommand\klear[3]{\mbox{$#1\!: #2 \rightsquigarrow #3$}}
\newcommand\kleare[2]{\mbox{$#1 \rightsquigarrow #2$}}
\newcommand\lare[2]{\mbox{$#1 \rightarrow #2$}}
%==============================================

\newcommand\corrce{correspondence}






%%% 1. Collections
%
%==1.1 Categories
% macros for names moved to macros4names.tex
%\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%%\newcommand\catname[1]{\mbox{\boldmath $#1$}}
%\newcommand\cat[1]{\catname{#1}}
%\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}
%\newcommand\catnamei[1]{{\pmb #1}}



%\newcommand\idmap[1]{\operator{id}_{#1}}
%\renewcommand\f{\mbox{$\phi$}}
%\renewcommand\c{\catname{C}}
%\renewcommand\b{\catname{B}}
%\renewcommand\r{\catname{R}}





\newcommand\clonet{\mbox{${\nia}_\mathrm{Top}$}}
\newcommand\clonem{\mbox{${\nia}_\mathrm{MMt}$}}
%
% -- overlined letters for clones ---
%\newcommand\clonet{\mbox{$\overline{\nia}_\mathrm{Top}$}}
%\newcommand\clonem{\mbox{$\overline{\nia}_\mathrm{MMt}$}}



%==1.2 Classes of nodes/arrows
\newcommand\indclassofitems[1]{{\cal #1}}
\newcommand\classofitems[1]{\mbox{$\indclassofitems{#1}$}}
\newcommand\coi[1]{\classofitems{#1}}
\newcommand\incls{\coi{I}}
\newcommand\covers{\coi{C}}
\newcommand\univs{\coi{U}}
%\renewcommand\diags{\classofitems{D}}
\renewcommand\diags{\mathit{Diags}}
\newcommand\inddiags{\indclassofitems{D}}

%\newcommand\attrset[1]{\mbox{\textit{attrs}$(#1)$}}
%\newcommand\refset[1]{\mbox{\textit{refs}$(#1)$}}
%\newcommand\varset[1]{\mbox{\textit{vars}$(#1)$}}
%\newcommand\classtab[1]{\mbox{\textsf{tab}$_#1$}}
%\newcommand\attrtab[1]{\mbox{\textsf{aTab}$_#1$}}
%\newcommand\reftab[1]{\mbox{\textsf{rTab}$_#1$}}



%===1.3 Languages
\newcommand\querylanguage[1]{\nicex{ QL_{#1}$}}
\newcommand\ql{\querylanguage}
\newcommand\qlmath[1]{{\cal QL}_{#1}}

%%% 2. MMt Objects
\renewcommand\modelob[1]{\mbox{$M_{#1}$}}
\newcommand\schemaobsymbol{S}
\newcommand\typeSyssymbol{Types}
\newcommand\instanceGraphSymbol{I}
\newcommand\relschemaobsymbol{R}
\newcommand\skeobsymbol{S}
\newcommand\universesymbol{U}
\newcommand\valueUniverseGraphSymbol{U}
\newcommand\UniverseGraphSymbol{U}
\newcommand\schemaob[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
%\newcommand\typesys[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
\newcommand\instgra[2]{\mbox{${\mathit \instanceGraphSymbol}_{#1}^{#2}$}}
\newcommand\igra[2]{\instgra{#1}{#2}}
\newcommand\itogra[1]{\instgra{}{#1}}
\newcommand\irefgra[1]{\instgra{ref}{#1}}
\newcommand\iattgra[1]{\instgra{attr}{#1}}
\newcommand\iobjgra[1]{\instgra{obj}{#1}}

\newcommand\uvalgra[1]{\mbox{$\mathit{\universesymbol Val}_{#1}$}}
\newcommand\utupgra[1]{\mbox{$\mathit{\universesymbol Tuple}_{#1}$}}
\newcommand\uval{\uvalgra{}}
\newcommand\utup{\utupgra{}}
\renewcommand\uniob[1]{\mbox{$\mathsf{\universesymbol}_{#1}$}}

\newcommand\relsob[1]{\mbox{${\mathit \relschemaobsymbol}_{#1}$}}
\newcommand\newrelske[1] {\mbox{${\mathsf R}_{#1}$}}
\newcommand\newrelinst[2]{\mbox{${\mathsf Q}_{#1}^{#2}$}}

\newcommand\schemaOB[2]{\mbox{${\mathit \schemaobsymbol}_{#1}^{#2}$}}

\newcommand\claske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{cla}#1}$}}
\newcommand\refske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{ref}#1}$}}
\newcommand\attrske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{attr}#1}$}}
\newcommand\objrefske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{objRef}#1}$}}


\renewcommand\skeob[1]{\mbox{${\mathsf\skeobsymbol}_{#1}$}}
\newcommand\skeobind[1]{{\mathsf \skeobsymbol}_{#1}}
\newcommand\indskeob[1]{\skeobind{#1}}

\newcommand\typeske[1]{\mbox{$\mathsf{Type}_{#1}$}}
\newcommand\typemap[1]{\mbox{$\mathsf{type}_{#1}$}}
\newcommand\typeskeind{\mathsf{Type}}
\newcommand\typemapind[1]{\mathsf{type}_{#1}}

\renewcommand\statemap{\mbox{$\sigma$}}
\newcommand\statemapind{\sigma}




%\newcommand\gs{\mbox{$G_{\indskeob{}}$}}
%\newcommand\ds{\mbox{$\diags_{\indskeob{}}$}}
%\newcommand\gsi[1]{\mbox{$G_{\indskeob{#1}}$}}
%\newcommand\dsi[1]{\mbox{$\G_{\indskeob{#1}}$}}

%%% 2.1  Vectors of objects (bold objects)
%\newcommand\fullvector[3]{}
%\newcommand\vectorobject[1]{\mbox{$\boldsymbol{#1}$}} % see macros4names
\newcommand\multisch{\vectorobject{\schemaobsymbol}}
\newcommand\multiSch{\vectorobject{\schemaobsymbol}}
\newcommand\multinst{\vectorobject{\instancesymbol}}
\newcommand\multinstoo[1]{\mbox{$\multinst=(\inst{1},\ldots,\inst{#1})$}}

\newcommand\multiUni{\vectorobject{\universesymbol}}
\newcommand\multiRel{\vectorobject{\relschemaobsymbol}}
\newcommand\multiuni{\vectorobject{u}}
\newcommand\multirel{\vectorobject{r}}
\newcommand\multiu{\vectorobject{u}}
\newcommand\multir{\vectorobject{r}}
\newcommand\multiroo[1]{\mbox{$\multir=(r_1,\ldots,r_{#1})$}}


%== Operators
\newcommand\operator[1]{\mbox{\sf #1}}
\newcommand\operatorInIndex[1]{{\sf #1}}

\newcommand\heoperator[1]{\mbox{\sf\bfseries #1}}
\newcommand\match{\operator{match}}

\newcommand\indexedoperator[3]{\mbox{\operator{#1}$_{#2}^{#3}$}}
\newcommand\indexedoperatorInIndex[3]{\operatorInIndex{#1}_{#2}^{#3}}

\newcommand\der[2]{\indexedoperator{der}{#1}{#2}}
\newcommand\dero[1]{\indexedoperator{der}{}{#1}}
\newcommand\derInIndex[2]{\indexedoperatorInIndex{der}{#1}{#2}}

%\newcommand\proj[1]{\indexedoperator{p}{#1}{}}
%\newcommand\merge{\operator{merge}}
%\newcommand\modgen{\operator{modelGen}}
%\newcommand\datatrans{\operator{dataTransf}}
%\renewcommand\self{\operator{self}}


\newcommand\SFW[3]{\mbox{\operator{Select} #1
\operator{from} #2
\operator{where} #3}
}

%=====================
%\input{../../Tools/Macros/m20-newMacros}
%\renewcommand\em[1]{\emph{#1}}

%\newcommand\vect[1]{\textbf{#1}}
\newcommand\veg{\vect{G}}
\newcommand\vef{\vect{f}}
\newcommand\ver{\vect{R}}
\newcommand\ves{\vect{S}}
\newcommand\vehh{\vect{H}}
\newcommand\veho{\vect{\ovr{H}}}
\newcommand\veh{\vect{h}}

\newcommand\ovr[1]{\mbox{$\overline{\mathstrut#1}$}}
\newcommand\ovri[1]{\overline{#1}}
\newcommand\ovh[1]{\ovr{H}_{#1}}
%\newcommand\ovri[1]{\mb{\ovr{\iota'}_{#1}}}

\newcommand\edge[1]{\ittt{Edge}\mb{_{#1}}}
\newcommand\Edge[2]{\ittt{Edge}\mb{_{#1}^{#2}}}


\newcommand\univarr[1]{\mb{!_{#1}}}
\newcommand\doublearrow[5]{\mbox{$#1\stackrel{#4}{\rightarrow}
#2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrdou[5]{\doublearrow{#1}{#2}{#3}{#4}{#5}}
\newcommand\arrarr{\arrdou{\gra{2}}{\gra{3}}{\gra{4}}{h_2}{h_3}}
\newcommand\scearr{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}}
\newcommand\arrsce{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}} % the same as above

\newcommand\arrspan[5]{\fbox{$#1\stackrel{#4}{\leftarrow}
#2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrcospan[5]{\fbox{$#1\stackrel{#4}{\rightarrow}
#2\stackrel{#5}{\leftarrow}#3$
}}

%\renewcommand\span[1]{\textbf{R}\mb{_{#1}}}
\newcommand\cospan[1]{\textbf{S}\mb{_{#1}}}
\newcommand\set[2]{\mb{#1=\{#2\}}}

\newcommand\integr[3]{\mb{#1\bigoplus_#3 #2}}

\newcommand\gran[1]{\mb{G_{{#1}N}}}
\newcommand\gred[1]{\mb{G_{{#1}E}}}
\newcommand\graman[1]{\mb{f_{{#1}N}}}
\newcommand\gramed[1]{\mb{f_{{#1}E}}}
\newcommand\grinman[1]{\mb{\iota'_{{#1}N}}}
\newcommand\grinmed[1]{\mb{\iota'_{{#1}E}}}

% changing from \mathsl to \mathit
\renewcommand\object[2]{\mbox{${\mathit{#1}}_{#2}$}}
\renewcommand\objectind[1]{\mathit{#1}}
\renewcommand\objectmath[1]{\mathit{#1}}

%\newcommand\DOM[1]{\Box #1}
%\newcommand\COD[1]{#1 \Box}


\newcommand\mb[1]{\mbox{$#1$}}
\newcommand\nin{\mb{\cal N}}
\newcommand\nix{\mb{\cal X}}
\newcommand\nil{\mb{\cal L}}
\newcommand\nik{\mb{\cal K}}
\newcommand\dvet{\mbox{:}}
\newcommand\ddvet{\dvet\dvet}
%\newcommand\n{\mb{n}}

\renewcommand\x{\mb{X}}

\newcommand\proxx[2]{\mb{\prod_{#1}{#2}}}
\newcommand\prox{\proxx{}{\vex}}
\newcommand\proy{\proxx{}{\vey}}
\newcommand\prodxn{\proxx{\cal L}{\vex}}
\newcommand\prodxm{\proxx{\cal K}{\vex}}

\newcommand\unixx[2]{\mb{\bigcup_{#1}{#2}}}
\newcommand\unix{\unixx{}{\vex}}

\newcommand\proj[1]{\mb{\ell_{#1}}}
\newcommand\proji{\proj{i}}






\renewcommand\ext{\mbox{\textsf{ext}}}








\newcommand\oclar{\mbox{\footnotesize $>$}}
\newcommand\myendset[1]{\mbox{$\{#1_1..#1_m\}$}}
\newcommand\fens{\myendset{f}}





\newcommand\fulla[1]{\mbox{${\mathbf F}_{#1}$}}
\newcommand\rmap[1]{\mbox{$#1^\rightarrow$}}
\newcommand\lmap[1]{\mbox{$^\leftarrow #1$}}
\newcommand\basemap[1]{\mbox{\textit{base}$_{#1}$}}


\newcommand\seq[1]{\textsf{seq}\mbox{$#1$}}
\newcommand\coll[2]{\textsf{coll}\mbox{$_{#1}(#2)$}}

\newcommand\tabschema{\mbox{$D=\{a_1:D_1,...,a_n:D_n\}$}}
\newcommand\tabschemamap{\mbox{\lar{D}{\attrset{}}{\setcat}}}



%=====================
%\input{../../Tools/Macros/m21--labelsnewMacros}
%(left) labels for formulas
\newcommand\equationNumber[1]{(\textsf{#1})}
\newcommand\eqnumber[1]{\equationNumber{#1}}
\newcommand\eqn[1]{\equationNumber{#1}}


%\newcommand\mafo[2]\mathform{#1}{#2}
\newcommand\mathfo[2]{$$#2\leqno{\mbox{(\textsf{#1})}} $$}
\newcommand\mafo[2]{$$#2 \leqno{\mbox{\eqn{#1}}} $$}


\newcommand\selflab{\eqn{self}}
\newcommand\looplab{\eqn{loop}}
\newcommand\idlelab{\eqn{idle}}
\newcommand\dolab{\eqn{do}}
\newcommand\triglab{\eqn{trigger}}

\newcommand\assonla{\eqn{fullAsson}}
\newcommand\tabla{\eqn{TAB}}
\newcommand\invla{\eqn{inverse}}
\newcommand\extla{\eqn{extension}}
\newcommand\tablatup{\eqn{TABrow}}
\newcommand\tablapro{\eqn{TABattr}}
\newcommand\sepla{\eqn{1-1}}
%=====================================
\newcommand\classn{\eqnumber{classn}}
\newcommand\indexn{\eqnumber{indexng}}

\newcommand\igralabel{\eqnumber{instGra}}
\newcommand\schemaGeneralLabel{\eqnumber{schemaGen}}
\newcommand\stlabel{\schemaGeneralLabel}
\newcommand\itablabel{\eqnumber{instTab}}
%\renewcommand\uniob[1]{\mbox{${\mathsf\universesymbol}_{#1}$}}
\newcommand\igratablabel{\eqnumber{instGraTab}}
\newcommand\igragralabel{\eqnumber{instGraGra}}
\newcommand\itabtablabel{\eqnumber{instTabTab}}

%=====================
%\input{../Tools/Macros/m21--abbrev4formulas}
%\input{../Tools/Macros/m22--abbrev4text}
%--------------------------------
%\renewcommand\zdmargin[1]{}
%\renewenvironment{razd}[2]{\subsubsection{#1}}{}
%\nocite{}
\renewenvironment{razD}[2]{\beginRazD{{%\itshape
\bfseries #1}}}{\EndRazD}

%% sle
%%%%%%%%%% sle09 macros
%\newcommand\diagi[1]{#1\mbox{$'$}}
%\newcommand\diagii[1]{#1\mbox{$''$}}
%
%\newcommand\ari[1]{\mbox{\textsl{ar}$(#1)$}}
%\newcommand\mmname[1]{\textsf{#1}}
%\newcommand\mmcd{\mmname{CD}}
%\newcommand\mmsd{\mmname{SD}}
%\newcommand\mmsc{\mmname{SC}}
%\newcommand\mmca{\mmname{CA}}
%\newcommand\mmamt{\mmname{CAT}}
%\newcommand\mmcat{\mmname{CAT}}
%\newcommand\cd{\mmname{cd}}
%\renewcommand\sd{\mmname{sd}}
%\renewcommand\sc{\mmname{sc}}
%\newcommand\ca{\mmname{ca}}
%\newcommand\amt{\mmname{cat}}
%\renewcommand\cat{\mmname{cat}}
%\newcommand\cdi{\diagi{\cd}}
%\renewcommand\sdi{\diagi{\sd}}
%\newcommand\sci{\diagi{\sc}}
%\newcommand\cdii{\diagii{\cd}}
%\newcommand\sdii{\diagii{\sd}}
%\newcommand\scii{\diagii{\sc}}





\newcommand\base{\mbox{$\pmb{MM}$}}
\newcommand\p{\textbf{P}}
\newcommand\ps{\mbox{$P$}}
\newcommand\leqnoo[1]{\leqno{\mbox{#1}}}

\newcommand\keyword[1]{{\itshape\textsf{#1}}}
\newcommand\nam{\keyword{name}}
\renewcommand\owner{\keyword{owner}}
\newcommand\type{\keyword{type}}
\newcommand\val{\keyword{value}}
\newcommand\Class{\keyword{Class}}
\renewcommand\Attr{\keyword{Attr}}
\newcommand\Type{\keyword{Type}}
\newcommand\elm[1]{\mbox{$\mathit{El}(#1)$}}

\newcommand\ueq{\mbox{$\leftrightarrow$}}
\newcommand\uneq{\mbox{$\rightsquigarrow$}}

\newcommand\meq{\mbox{$=$}}
\newcommand\mneq{\mbox{$\neq$}}


\newcommand\shot{\textsl{shot}}
\newcommand\reltile{\textsl{relTile}}
%\newcommand\tauh{\mbox{$\tau_{\textsf{h}}$}}
%\newcommand\tauv{\mbox{$\tau_{\textsf{v}}$}}



\newcommand\vso{\textsf{v}\mbox{$\partial_0$}}
\newcommand\vta{\textsf{v}\mbox{$\partial_1$}}
\newcommand\hso{\textsf{h}\mbox{$\partial_0$}}
\newcommand\hta{\textsf{h}\mbox{$\partial_1$}}

\newcommand\mmod{\nicex{ M$}}
\newcommand\id{\textsl{id}}
\renewcommand\id{\mbox{$\iota$}}
\newcommand\recon[1]{\mbox{$#1$\textbf{!}}}

\newcommand\oidd[1]{\mbox{$\overline{#1}$}}
\newcommand\oiddi[1]{\mbox{$\overline{#1}'$}}

\renewcommand\oidd[1]{\mbox{${#1}$}}
\renewcommand\oiddi[1]{\mbox{${#1}'$}}

\newcommand\oa{\oidd{a}}
\newcommand\ob{\oidd{b}}
\newcommand\oP{\oidd{P}}
\newcommand\oQ{\oidd{Q}}

\newcommand\oai{\oiddi{a}}
\newcommand\obi{\oiddi{b}}
\newcommand\oPi{\oiddi{P}}
\newcommand\oQi{\oiddi{Q}}

% icmt

%%% icmt09 macros
% the % piece below  was moved to newMacros ---
\newcommand\mrkoprr[1]{\mrkopr{\mrkopr{#1}}}
%\der{}{Q}
%\newcommand\mmview[1]{\mbox{$\textsl{v}_{#1}$}}
%\newcommand\mmarr{v}
\newcommand\mmf{\mbox{$m$}} % to be used in the row
%\renewcommand\mmview[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%%\newcommand\mmv[1]{{\pmb{\mmarr}_{#1}}} %for subscripts
%\newcommand\mmmap[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%\renewcommand\mmm{m}  % to be used for sub-sup-indexes
%\newcommand\mmap[1]{\mbox{${\mmarr}_{#1}$}}

\newcommand\unde[1]{\underline{#1}}

\newcommand\oversi[1]{\overline{\sigma}^{#1}}

\newcommand\oversig[1]{\overline{\sigma}^{Q#1}}
\newcommand\overtau[1]{\overline{\tau}^{Q#1}}
\newcommand\overover{\overline{\oversig{1}}}
\newcommand\doublesig{{\overover^{Q2}}} %
\newcommand\votono{{\overline{\oversig{}}^{R}}}

\newcommand\derqq[2]{\mbox{$\dero{Q#1}#2$}}
\newcommand\dermms[1]{\derqq{#1}{\mms}}
\newcommand\derms[1]{\derqq{#1}{\ms{}}}
\newcommand\derqmms{\derqq{}{\mms}}
\newcommand\derqms{\derqq{}{\ms{}}}
\newcommand\derq[1]{\mbox{$\der{}{Q}#1$}}
\newcommand\doubleder[1]{\derqq{1;Q2}{#1}}

\newcommand\augtymaps{\flar%
{\overline{\sigma}^{Q}}%
{\dero{Q}\ms{}}%
{\dero{Q}\mms}%
}
%\newcommand\mmarr{\mbox{$m$}}

%
\newcommand\tracemap[1]{\mbox{$\stackrel{\rightsquigarrow}{#1}$}}
\renewcommand\tracemap[1]{\mbox{$\mathit{tr}_{#1}$}}
\renewcommand\tracemap[1]{\mbox{$#1^{*}$}}
\newcommand\tram{\tracemap{\mmmap}}
%
\newcommand\reversemap[1]{\mbox{\spf$_{#1}$}}
%\newcommand\revem{\reversemap{\mmview{}}}
\newcommand\revem[1]{\mbox{$\semm{\mmmap{#1}}$}}

\renewcommand\s[1]{\mbox{$S_{#1}$}}
\renewcommand\ms[1]{\mbox{$S_{#1}$}}
\newcommand\mos[1]{\mbox{$\overline{S}_{#1}$}}
\renewcommand\mt[1]{\mbox{$T_{#1}$}}
\newcommand\mot[1]{\mbox{$\overline{T}_{#1}$}}
\newcommand\mh[1]{\mbox{$H_{#1}$}}
\renewcommand\ml[1]{\mbox{$L_{#1}$}}

\newcommand\pbop{\operator{PB}}

\newcommand\msarr{\flar{\sigma}{S}{\mms}}
\newcommand\msarrq{\flar{\overline{\sigma}^{Q}}{\der{}{Q}S}{\der{}{Q}\mms}}
\newcommand\mssym{\mbox{$\overline{\sigma}$}}
\newcommand\mssymq{\mbox{$\overline{\sigma}^Q$}}

\newcommand\mtarr{\flar{\tau}{T}{\mmt}}
\newcommand\srelarr{\flar{\sigma}{S}{\mmrel}}
\newcommand\erdarr{\flar{\tau}{D}{\mmer}}
\newcommand\srelderarr[1]{\flar{\overline{\sigma}^{Q#1}}{\der{}{Q#1}S}{\der{}{Q#1}\mmrel}}



\newcommand\ertorel[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\mmrel}}
\newcommand\ertorelder[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\der{}{{Q#1}}\mmrel}}

% gttse

%\renewcommand\mmname[1]{\mbox{$\pmb{\cal #1}$}}
%\newcommand\mmmapname[1]{\mbox{$\pmb{#1}$}}
%\newcommand\mma{\mmname{M}}
%\newcommand\mmb{\mmname{N}}
%\newcommand\mmc{\mmname{O}}
%\newcommand\mmr[1]{\mbox{\mmname{R}$_{#1}$}}
%\renewcommand\mmr[1]{\mbox{$\pmb{r}_{#1}$}}
%\newcommand\mmab{\mmname{MN}}
%\newcommand\mmac{\mmname{MO}}
%\newcommand\mmv{\mmmapname{v}}
%\newcommand\mmw{\mmmapname{w}}
%\newcommand\mmp{\mmmapname{p}}
%\newcommand\mmq{\mmmapname{q}}

\renewcommand\dvet{\mbox{:\,}}

\newcommand\newrevem[1]{\mbox{$\semm{\mmmapname{#1}}$}}
\newcommand\rev{\newrevem{v}}
\newcommand\rew{\newrevem{w}}
\newcommand\rep{\newrevem{p}}
\newcommand\req{\newrevem{q}}


\newcommand\mmnamei[1]{\pmb{\cal #1}}
\newcommand\mmabi{\mmnamei{MN}}
\newcommand\mmaci{\mmnamei{MO}}
\newcommand\amn{\mbox{$A_{\mmabi}$}}
\newcommand\bmn{\mbox{$B_{\mmabi}$}}
\newcommand\amnprim{\mbox{$A'_{\mmabi}$}}
\newcommand\bmnprim{\mbox{$B'_{\mmabi}$}}
\newcommand\amo{\mbox{$A_{\mmaci}$}}
\newcommand\cmo{\mbox{$C_{\mmaci}$}}
\newcommand\umn{\mbox{$u_{\mmabi}$}}
\newcommand\vmn{\mbox{$v_{\mmabi}$}}

\newcommand\lmmes{\left] \respace\left] }
\newcommand\rmmes{\right[\respace\right[}
\newcommand\mmes[1]{\mbox{$\lmmes\, \mathit{#1} \, \rmmes$}}

% spans

\newcommand\spancat{\category{Span}}
\newcommand\spansa{\scat\spancat}
\newcommand\spanset{\setcat\spancat}
\newcommand\cospancat{\category{Cospan}}
\newcommand\cospansa{\scat\cospancat}
\newcommand\cospanset{\setcat\cospancat}


\newcommand\spanfull[4]{\mbox{${\cal #1}$=(\flar{#2_i}{#3}{#4 i},
$i=1,2)$}}

\newcommand\lKleisly{\Leftarrow}
\newcommand\rKleisly{\Rightarrow}
\newcommand\spandiag[5]  {\fbox{$#1\lTo^{#2} #3 \rTo^{#4} #5$}}
\newcommand\kleispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\kleislispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\cospandiag[5]{\fbox{$#1\rTo^{#2} #3 \lTo^{#4} #5$}}
\newcommand\kleicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}
\newcommand\kleislicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}


\newcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\newcommand\spandiagsemm[5]{\fbox{$\semm{#1}\lTo^{#2} \semm{#3} \rTo^{#4} \semm{#5}$}}
\newcommand\cospandiagsemm[5]{\fbox{$\semm{#1}\rTo^{#2} \semm{#3} \lTo^{#4} \semm{#5}$}}


%=== with brackets
\newcommand\spandiagbra[5]
{\mbox{$%\left %
(#1\stackrel{~#2}{\leftarrow} #3
\stackrel{#4~}{\rightarrow} #5%\right
)$}}
\renewcommand\kleispandiag[5]{\mbox{$\left(#1\stackrel{~#2}{\lKleisly} #3
\stackrel{#4~}{\rKleisly} #5
\right)$}}
\renewcommand\kleislispandiag[5]{\mbox{$\left(#1\stackrel{#2}{\lKleisly} #3
\stackrel{#4}{\rKleisly} #5
\right)$}}
\renewcommand\kleicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
\stackrel{#4}{\lKleisly} #5
\right)$}}
\renewcommand\kleislicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
\stackrel{#4}{\lKleisly} #5
\right)$}}

\renewcommand\cospandiag[5]{\mbox{$\left(#1\rTo^{#2} #3 \lTo^{#4} #5\right)$}}
\renewcommand\cospandiag[5]  {\mbox{$\left(#1\stackrel{~#2}{\rightarrow} #3
\stackrel{#4~}{\leftarrow} #5\right)$}}

% without brackets
\renewcommand\spandiag[5]  {\mbox{$#1\stackrel{~#2}{\leftarrow} #3
\stackrel{#4~}{\rightarrow} #5$}}
\renewcommand\cospandiag[5]  {\mbox{$#1\stackrel{~#2}{\rightarrow} #3
\stackrel{#4~}{\leftarrow} #5$}}


%\renewcommand\kleislycospandiag[5]{\mbox{$\left(#1\rKleisly^{#2} #3 \lKleisly^{#4} #5\right)$}}

\renewcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\renewcommand\spandiagsemm[5]{\mbox{$\left(\semm{#1}\lTo^{#2} \semm{#3}\rTo^{#4} \semm{#5}\right)$}}
\renewcommand\cospandiagsemm[5]{\mbox{$\left(\semm{#1}\rTo^{#2} \semm{#3}\lTo^{#4} \semm{#5}\right)$}}


%% end macros



%%==== end newMacros


==> getPackages.tex <==
%\usepackage{GSDTR}
\usepackage{enumitem}
\usepackage[stable]{footmisc}
\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%\usepackage{bickham}
%--------
\usepackage[english]{babel}
\usepackage{hyperref}
\usepackage{tikz}
\usepackage{lipsum}
%\usepackage{boondox-cal}
%\usepackage{boondox-calo}
\usepackage{dutchcal}     %<--- ?
\usepackage[leqno]{amsmath}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{lineno}
\usepackage[misc,geometry]{ifsym}
\usepackage{graphicx}
\usepackage{color}
\usepackage{xcolor}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\usepackage[normalem]{ulem}
\usepackage{ucs}
\usepackage{url}
\usepackage{makeidx}
\usepackage{amssymb}

\usepackage[all]{xy}
\usepackage{xspace}
\usepackage{subfig}

\usepackage{algorithm}
\usepackage{verbatim}
\usepackage{multirow}
%=== previosly were in macros

\usepackage{rotating}
\usepackage{lscape}
\usepackage{epsfig}
\usepackage{color}
\usepackage{float}
\usepackage{amsbsy,wasysym}
\usepackage{amsfonts}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{array}
\usepackage{latexsym}
\usepackage{xspace}
%\usepackage[figurename=Fig.]{caption}




==> macros/4makkai.tex <==
% Sketch Categories
\newcommand{\skecat}[2]{\enma{{#1}||{#2}}}
\newcommand{\skecatop}[3]{\enma{{#1}||{#2}||{#3}}}
\newcommand{\skecatp}[1]{\skecat{#1}{\predicateSig}}
\newcommand{\skecatgp}{\skecat{\cat{G}}{\predicateSig}}
\newcommand{\skecatgpmono}{\enma{\GG|\predsig}}
\newcommand{\skecatgpfin}{\enma{\GGfin||\predsig}}

\newcommand{\skecathp}{\skecat{\II}{\predicateSig}}
\newcommand{\skecatghp}{\skecat{\GG(\II)}{\predicateSig}}

%\newcommand{\gracat}[2]{\enma{\setcat^{{#1\}}}}
%\newcommand{\gracatop}[3]{\enma{{#1}||{#2}||{#3}}}
\newcommand{\gracatph}{\enma{\setcat^{\iistarp}}}


%\newcommand{\skecatgpo}{\skecatop{\cat{G}}{\predicateSig}{\operationSig}}



\newcommand{\sketogra}{\enma{\mathsf{ske2gra}}}
\newcommand{\gratoske}{\enma{\mathsf{gra2ske}}}
\newcommand{\skettografun}[1]{\enma{\widecheck{#1}}}
\newcommand{\gratoskefun}[1]{\enma{\widehat{#1}}}
\newcommand{\stog}[1]{\enma{\skettografun{#1}}}
\newcommand{\gtos}[1]{\enma{\gratoskefun{#1}}}
\newcommand{\ftop}[1]{\stog{#1}} %\enma{\skettografun{#1}}}
\newcommand{\ptof}[1]{\gtos{#1}} %\enma{\gratoskefun{#1}}}


\newcommand\dfib{\enma{\mathrm{dfib}}}
\newcommand{\invFun}[1]{\enma{{#1}^{-1}}}
%\renewcommand{\invFun}[1]{\enma{\semm{#1}}}
\newcommand{\funSpace}[2]{\enma{\left[ #1, #2    \right]}}
\newcommand{\barr}{\enma{b}}
\newcommand{\arfunhat}{\enma{{\hat \arfun}}}
\newcommand{\arfunpro}{\enma{{\tilde \arfun}}}

\newcommand{\skeske}[1]{#1.\sketogra.\gratoske}
\newcommand{\gragra}[1]{#1.\gratoske.\sketogra}
\renewcommand{\skeske}[1]{\gratoskefun{\skettografun{#1}}}
\renewcommand{\gragra}[1]{\skettografun{\gratoskefun{ #1}}}


==> macros/4textArrowsFromEDL.tex <==
\newcommand{\wiglyrar}[3]{\enma{#1\!:#2 \rightsquigarrow #3}} % long arrow
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Arrows in diagrams and formulas
% normal functional arrow f: X-->Y
\newcommand{\frar}[3]{\ensuremath{#1{:}\;#2\rightarrow #3}}
\newcommand\frarxy[2]{\ensuremath{#1\rightarrow #2}}
\newcommand\flarxy[2]{\ensuremath{#1\leftarrow #2}}
\newcommand\fprar[4]{\ensuremath{#1{:}\;#2\stackrel{#4}{\rightarrow} #3}}
\renewcommand\fprar[4]{\ensuremath{#1{:}\;#2\rTo^{#4} #3}}
\newcommand\fprarlong[4]{\ensuremath{#1{:}\;#2\stackrel{#4}{\longrightarrow} #3}} 

\newcommand{\flaxrar}[3]{\ensuremath{ #1{:}\;#2\xrightarrow{\mathrm{lax}}#3}}
%\renewcommand{\frar}[3]{\ensuremath{{#1}{:}\;{#2}\rightarrow {#3}}}
\newcommand{\flaxlar}[3]{\ensuremath{#1{:}\;#2\xleftarrow{\mathrm{lax}} #3}}

\newcommand{\bullrightarrow}{\enma{\lefteqn{\quad\!\!\!\bullet}\longrightarrow}}
\newcommand{\bullleftarrow}{\enma{\lefteqn{\quad\!\bullet}\longleftarrow}}
\newcommand{\bullleftrightarrow}{\enma{\lefteqn{\quad \!\bullet}\longleftrightarrow}}
%\newcommand{\bullleftarrow}{\enma{\lefteqn{\quad\!\bullet}\longleftarrow}}
\newcommand{\xBulleftrightarrow}[2]{\enma{\lefteqn{\quad \!\bullet}\xleftrightarrow[#2]{#1}}}
\newcommand{\xBulleftrightarrowLong}[2]{\enma{\lefteqn{\quad \!\bullet}\xleftrightarrow[#2]{#1}}}
\newcommand{\xBulletcorrlong}[2]{\enma{\lefteqn{\quad \;\bullet}\xleftrightarrow[#2]{#1}}}
\newcommand{\xBulletcorr}[2]{\enma{\lefteqn{\;\;\;\,\bullet}\xleftrightarrow[#2]{#1}}}

%-- SPANS
\newcommand\spanrar[3]{\enma{{#1}\!:{#2}\nrightarrow{#3}}}
\newcommand\spanrarxy[2]{\enma{{#1}\nrightarrow{#2}}}
\newcommand{\spanlar}[3]{\enma{{#1}\!:{#2}\nleftarrow{#3}}}

\newcommand{\xstrokedmapstoLongName}[1]{\enma{\lefteqn{\quad \;\prime}\xmapsto[\qquad]{#1}}}

\newcommand{\xstrokedmapstoName}[1]{\enma{
		\lefteqn{\;\;\;\,\footnotesize{\prime}}\xmapsto[~~~\,]{#1}
	}}

\newcommand{\spaninstrarlong}[3]{\enma{{#1}\!:{#2}\xstrokedmapstoLongName {}{#3}}}

\newcommand{\spaninstrar}[3]{\enma{{#1}\!:{#2}\xstrokedmapstoName{}{#3}}}
\newcommand{\spaninstrarOvername}[3]{\enma{{#1}\xstrokedmapstoName{#2}{#3}}}
\newcommand{\finstrarOvername}[3]{$#1\xmapsto[\quad]{#2} #3$}

\newcommand{\spanrarinst}[3]{\spaninstrar{#1}{#2}{#3}}
\newcommand{\xstrokedmapsto}[2]{\enma{\lefteqn{\;\;\;\,\bullet}\xmapso[#2]{#1}}}







\newcommand\corrbullrar[3]{\enma{#1\!:#2\bullleftrightarrow\, #3}}
%\newcommand\corrdiagrar[3]{\enma{#1\!:#2\xBulletcorr{#1}{\qquad}\, #3}}
\newcommand\corrdiagrarlong[3]{\enma{{#1}\xBulletcorrlong{#2}{\qquad}\,{#3}}}
\newcommand\corrdiagrar[3]{\enma{{#1}\xBulletcorr{#2}{\quad\,}\,{#3}}}

%\newcommand\corrdiagrar[3]{\enma{\stackrel{\scriptsize{#1}}{#2\,\xBulletcorr\, #3}}}


%----> triple spaces
\newcommand\trisprightarrow{\mbox{$\lefteqn{\longrightarrow}~\,\circ$}}
\newcommand\trisprar[3]{\mbox{\ensuremath{ #1{:}\;#2\trisprightarrow~~#3}}}
\newcommand\trispprar[4]{\mbox{\ensuremath{#1{:}\;#2\stackrel{#4~~}{\trispprightarrow} #3}}}
%   newer version with 0 instead of \circ 
\renewcommand\trisprightarrow{\mbox{$\rightarrow_0$}}
\newcommand\trispprightarrow{\mbox{$\rightarrow_{00}$}}
\newcommand\trisprightarrowP{\trispprightarrow}
\renewcommand\trisprar[3]{\mbox{\ensuremath{ #1{:}\;#2\trisprightarrow#3}}}

\newcommand\trisprarP[4]{\trispprar{#1}{#2}{#3}{#4}}



%functional arrow
\newcommand\wrar[3]{\ensuremath{#1{:}\;#2\rightsquigarrow #3}} %wavy arrow
\newcommand\wbiar[3]{\ensuremath{#1{:}\;#2\leftrightsquigarrow #3}} %wavy arrow
\newcommand\farr[3]{\frar{#1}{#2}{#3}}% if typo occurs
%\newcommand\lar[3]{\flar{#1}{#2}{#3}}%
\newcommand\updar[3]{\frar{#1}{#2}{#3}}
%\newcommand\viewlar[4]{\mbox{$#1\!:#2\rightarrow^{#4} #3$}}
%\newcommand\flarcat[4]{\mbox{$#1\!:#2\rightarrow #3{:}{:}\,#4$}}

% variants
%-----------
%long
\newcommand\frarr[3]{\mbox{$#1\!:#2\longrightarrow #3$}} % long arrow
\renewcommand\larr[3]{\mbox{$#1\!:#2\longrightarrow #3$}} % the same
%\newcommand\lari[4]{\mbox{$#1_{i}\!:\:#2\:\longrightarrow\:#3_{i},\;i=1,\ldots,#4$}}%

%multihead
\newcommand\mlar[3]{\larlar{#1}{#2}{#3}} %multiarrow
\newcommand\larlar[3]{\mbox{$#1\!:#2\twoheadrightarrow#3$}} %needs AMS
% double body
\newcommand\drar[3]{\mbox{$#1\!:#2\Rightarrow #3$}} %double arrow
\newcommand\dlarcat[4]{\mbox{$#1\!:#2\Rightarrow #3{:}{:}\,#4$}}
\newcommand\trar[3]{\mbox{$#1\!:\,#2\Rightarrow #3$}}
% inclusions
\newcommand\inclarr[3]{\mbox{$#1\!:\:#2\:\rInto\:#3$}}       %$key=<AltShftRT>
\newcommand\inclar[3] {\mbox{$#1\!:\:#2\:\hookrightarrow\:#3$}}
\newcommand\binclar[3] {\mbox{$#1\!:\:#2\:\hookleftarrow\:#3$}}
%triple body
\newcommand\trilar[3]{\mbox{$#1\!:#2\Rrightarrow #3$}} % triple
% profunctor/span
\newcommand\spanar[3]{\enma{#1\!:#2\nrightarrow#3}}



\newcommand{\proprar}[3]{\spanrar{#1}{#2}{#3}}
\renewcommand\proprar[3]{\enma{{#1}\!:{#2}\bullrightarrow\, {#3}}}
\newcommand\proprarxy[2]{\enma{\,{#1}\bullrightarrow\; {#2}}}
%
\newcommand\corrrar[3]{\birar{#1}{#2}{#3}}
\newcommand\corrlar[3]{\bilar{#1}{#2}{#3}}


\newcommand{\proplar}[3]{\spanlar{#1}{#2}{#3}}
\renewcommand\proplar[3]{\enma{#1\!:#2\bullleftarrow\, #3}}
\newcommand\proplarxy[2]{\enma{#1\!\bullleftarrow\, #2}}
\newcommand{\lensrar}[3]{\enma{#1\!:#2\rightleftarrows#3}}
\newcommand{\lenslar}[3]{\enma{#1\!:#2\leftrightarrows#3}}

% previous lens arrows
%\newcommand\lensar[3]{\mbox{$#1\!:#2\leftrightharpoons #3$}}%
%\newcommand\lensarleft[3]{\mbox{$#1\!:#2\rightleftharpoons #3$}}%
%\newcommand\lensarright[3]{\lensar{#1}{#2}{#3}}
%\renewcommand\lensar[3]{\mbox{$#1\!:#2\asymdoublearrow#3$}}


\newcommand\relrar[3]{\mbox{$#1\!:#2\nrightarrow#3$}}
\newcommand\rellar[3]{\mbox{$#1\!:#2\leftarrow#3$}}
\newcommand\trispar[3]{\spanar{#1}{#2}{#3}}  %synonym
\newcommand\backspanar[3]{\mbox{$#1\!:#2\nleftarrow#3$}}
%spans
%\newcommand\spanlar[5]{\mbox{$#1\!:#2\leftarrow #3\rightarrow #4 :#5$}} %double arrow%
% -- bidir arrows version
\newcommand\spanarbi[3]{\mbox{$#1\!:#2\nleftrightarrow #3$}}
\newcommand\backspanardi[3]{\mbox{$#1\!:#3\nleftrightarrow #2$}}


%-- backward arrow
\newcommand\flar[3]{\ensuremath{#1{:}~#2\leftarrow #3}} %backward functional arrow
%\newcommand\bflar[3]{\mbox{$#1\!:#2\leftarrow #3$}} %backward functional arrow
\newcommand\dlar[3]{\mbox{$#1\!:#2\Leftarrow #3$}} %double arrow
%\newcommand\bdlar[3]{\mbox{$#1\!:#2\Leftarrow #3$}} %double arrow

% two directional
\newcommand\bilar[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\birar[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\biarr[3]{\mbox{$#1\!:#2\leftrightarrow #3$}}%
\newcommand\bidlar[3]{\mbox{$#1\!:#2\Leftrightarrow #3$}}
\newcommand\lelar[3]{\mbox{$#1\!:#2\rightleftarrows #3$}} %double arrow


\newcommand\asymdoublearrow{%
\begin{array}{c}
~\rightarrow\\[-9pt]
\leftharpoondown
\end{array}}%

%%%%%%%%%%%%%%%%%%%%%%%
%---stackrel versions

% backward arrow
\newcommand\bfrarstack[3]{\mbox{$#3 \stackrel{~#1}{\longleftarrow} #2$}}
\newcommand\frarstack[3]{\bfrarstack{#1}{#2}{#3}}
\newcommand\flarstack[3]{\mbox{$#2\stackrel{#1~}{\longrightarrow} #3$}} %functyional arrow
\newcommand\spanlarstack[5]{\mbox{$#2\stackrel{~#1}{\longleftarrow} #3 %
                                                                       \stackrel{#5~}{\longrightarrow} #4$}} %double arrow%

% bidirectional

\newcommand\bilarsy[3]{\mbox{$#2\stackrel{#1}{\leftrightarrow}#3$}}
\newcommand\bidlarsy[3]{\mbox{$\left(#2\stackrel{#1}{\Leftrightarrow}#3\right)$}}
\newcommand\bixxlar[4]{\mbox{$#1\!:#2\stackrel{#3}{\longleftrightarrow} #4$}}%
\newcommand\bixlar[3]{\mbox{$#1\stackrel{#2}{\longleftrightarrow} #3$}}%
\newcommand\xxlar[4]{\mbox{$#1\!:#2\stackrel{#3}{\longrightarrow} #4$}}

%-- Now instances of the macros above for particular names of maps, thjeir sources and targets
\newcommand\updaraaa{\flar{a}{A}{A'}}
\newcommand\updarbbb{\flar{b}{B}{B'}}
\newcommand\corarrab{\bilar{r}{A}{B}}
\newcommand\corrarrab{\bilar{r}{A}{B}}
\newcommand\trisparrmn{\trispar{R}{\mmm}{\mmn}}
%
\newcommand\alifar[3]{\spanar{#1}{#2}{#3}}
\newcommand\backalifar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\alifarrmn{\spanar{\mmr}{\mmm}{\mmn}}
\newcommand\genalifarrmn{\spanar{\mmr}{\mmm}{\mmn}}
\newcommand\symalifarrmn{\spanar{\mmr^{>\!<}}{\mmm}{\mmn}}
\newcommand\asalifarrmn{\spanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\asymLalifarrmn{\spanar{\mmr^<}{\mmm}{\mmn}}
\newcommand\asymLEalifarrmn{\spanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\asymGalifarrmn{\spanar{\mmr^>}{\mmm}{\mmn}}
\newcommand\asymGEalifarrmn{\spanar{\mmr^\ge}{\mmm}{\mmn}}
\newcommand\bialifarrmn{\spanar{\mmr^{\cong}}{\mmm}{\mmn}}

\newcommand\backgenalifarrmn{\backspanar{\mmr}{\mmm}{\mmn}}
\newcommand\backsymalifarrmn{\backspanar{\mmr^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasalifarrmn{\backspanar{\mmr^\le}{\mmm}{\mmn}}
\newcommand\backasymLalifarrmn{\backspanar{\mmr^<}{\mmm}{\mmn}}
\newcommand\backasymGalifarrmn{\backspanar{\mmr^>}{\mmm}{\mmn}}

\newcommand\confar[3]{\spanar{#1}{#2}{#3}}
\newcommand\backconfar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\confarkmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\genconfarkmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\symconfarkmn{\spanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\asconfarkmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymLconfarkmn{\spanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\asymLEconfarkmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymGconfarkmn{\spanar{\mmk^>}{\mmm}{\mmn}}
\newcommand\asymGEconfarkmn{\spanar{\mmk^\ge}{\mmm}{\mmn}}
\newcommand\biconfarkmn{\spanar{\mmk^{\cong}}{\mmm}{\mmn}}
%--- outdated with *rmn instead of *kmn in the name of macros
%\newcommand\confar[3]{\spanar{#1}{#2}{#3}}
%\newcommand\backconfar[3]{\backspanar{#1}{#2}{#3}}
\newcommand\confarrmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\genconfarrmn{\spanar{\mmk}{\mmm}{\mmn}}
\newcommand\symconfarrmn{\spanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\asconfarrmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymLconfarrmn{\spanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\asymLEconfarrmn{\spanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\asymGconfarrmn{\spanar{\mmk^>}{\mmm}{\mmn}}
\newcommand\asymGEconfarrmn{\spanar{\mmk^\ge}{\mmm}{\mmn}}
\newcommand\biconfarrmn{\spanar{\mmk^{\cong}}{\mmm}{\mmn}}

\newcommand\backgenconfarkmn{\backspanar{\mmk}{\mmm}{\mmn}}
\newcommand\backsymconfarkmn{\backspanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasconfarkmn{\backspanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\backasymLconfarkmn{\backspanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\backasymGconfarkmn{\backspanar{\mmk^>}{\mmm}{\mmn}}
%--%--- outdated with *rmn instead of *kmn in the name of macros
\newcommand\backgenconfarrmn{\backspanar{\mmk}{\mmm}{\mmn}}
\newcommand\backopgenconfarrmn{\backspanar{\mmk^\circ}{\mmm}{\mmn}}
\newcommand\backopgenalifarrmn{\backspanar{\mmr^\circ}{\mmm}{\mmn}}
\newcommand\backsymconfarrmn{\backspanar{\mmk^{>\!<}}{\mmm}{\mmn}}
\newcommand\backasconfarrmn{\backspanar{\mmk^\le}{\mmm}{\mmn}}
\newcommand\backasymLconfarrmn{\backspanar{\mmk^<}{\mmm}{\mmn}}
\newcommand\backasymGconfarrmn{\backspanar{\mmk^>}{\mmm}{\mmn}}



%
\newcommand\lensarlmn{\lensar{\alens}{\mmm}{\mmn}}
\newcommand\genlensarlmn{\lensar{\alens}{\mmm}{\mmn}}
\newcommand\aslensarlmn{\lensar{\alens^\leq}{\mmm}{\mmn}}
\newcommand\asymLElensarlmn{\lensar{\alens^\leq}{\mmm}{\mmn}}
\newcommand\asymGElensarlmn{\lensar{\alens^\geq}{\mmm}{\mmn}}
\newcommand\symlensarlmn{\lensar{\alens^\gtlt}{\mmm}{\mmn}}
\newcommand\lesnarlmn{\lensar{\alens}{\mmm}{\mmn}} % the same in case of typo

\newcommand\lenssupx[1]{\lensar{\alens^{{#1}}}{\mmm}{\mmn}}
\newcommand\lenssubx[1]{\lensar{\alens_{{#1}}}{\mmm}{\mmn}}
\newcommand\lensopsupx[1]{\lensar{\alens^{\circ{#1}}}{\mmn}{\mmm}}
\newcommand\lensopsubx[1]{\lensar{\alens^{\circ_{#1}}{\mmn}{\mmm}}}
\newcommand\lenssupsubx[2]{\lensar{\alens^{#1}_{#2}}{\mmm}{\mmn}}

\newcommand\cfwksubx[1]{\spanar{\mmk_{{#1}}}{\mmm}{\mmn}}
\newcommand\cfwkopsubx[1]{\spanar{\mmk^{\circ}_{{#1}}}{\mmm}{\mmn}}

\newcommand\syncar[3]{\mbox{$#1\!:#2 \rightleftarrows #3$}}%
\newcommand\syncarleft[3]{\mbox{$#1\!:#2 \leftrightarrows #3$}}%
\newcommand\syncaright[3]{\syncar{#1}{#2}{#3}}
\newcommand\async{\ensuremath{\sigma}}
\newcommand\aSync{\ensuremath{\Sigma}}
\renewcommand\aSync{\ensuremath{\Pi}}
\newcommand\syncarsab{\syncar{\async}{A}{B}}
\newcommand\gensyncarsab{\syncar{\async}{A}{B}}
\newcommand\genSyncarsab{\syncar{\async}{A}{B}}
\newcommand\gensynctypearsab{\syncar{\async}{A}{B}}
\newcommand\genSynctypearsab{\syncar{\async}{A}{B}}
\newcommand\assyncarsab{\syncar{\async^\leq}{A}{B}}
\newcommand\asymGLEsyncarsab{\syncar{\aSync_{>\!\le}}{A}{B}}
\newcommand\asymGELsyncarsab{\syncar{\aSync_{\ge\!<}}{A}{B}}
\newcommand\asymGsyncarsab{\syncar{\aSync_{>}}{A}{B}}
\newcommand\asymLsyncarsab{\syncar{\aSync_{<}}{A}{B}}
\newcommand\symsyncarsab{\syncar{\async_\gtlt}{A}{B}}
\newcommand\symsyncarsabPoor{\syncar{\async_{\ge\!\le}}{A}{B}}
\newcommand\symSyncarsab{\syncar{\aSync_\gtlt}{A}{B}}
\newcommand\symSyncarsabPoor{\syncar{\aSync_{\ge\!\le}}{A}{B}}
\newcommand\lesnarsab{\syncar{\async}{A}{B}} % the same in case of typo



\newcommand\noninclensarlmn{\lensar{\alens_\noninc}{\mmm}{\mmn}}
\newcommand\fullinclensarlmn{\lensar{\alens_\fullinc}{\mmm}{\mmn}}


\endinput










\newcommand\vilar[3]{\dlar{#1}{#2}{#3}}
\newcommand\vlar[3]{\vilar{#1}{#2}{#3}}
\newcommand\malar[3]{\flar{#1}{#2}{#3}}
\newcommand\uplar[3]{\flar{#1}{#2}{#3}}
\newcommand\ular[3]{\uplar{#1}{#2}{#3}}
%  adding :: Graph,Set,Cat etc as the 4th parameter
\newcommand\vilarcat[4]{\dlarcat{#1}{#2}{#3}{#4}} % .. ::#4
\newcommand\malarcat[4]{\flarcat{#1}{#2}{#3}{#4}}
\newcommand\uplarcat[4]{\flarcat{#1}{#2}{#3}{#4}}

\newcommand\viewOfrel{{\prec}}
\newcommand\viewofar[3]{\mbox{$#1\!:#2\Rightarrow #3$}}
\newcommand\mmvmn{\vilar{\mmv}{\mms}{\mmt}}
\newcommand\mmvab{\vilar{\mmv}{\mms}{\mmt}}
\newcommand\mmvabcat{\vilarcat{\mmv}{\mms}{\mmt}{\mmodcat}}
\newcommand\mmvmncat{\vilarcat{\mmv}{\mms}{\mmt}{\mmodcat}}
\newcommand\mvab {\vilar{\mv}{A}{B}}
\newcommand\mvabcat{\vilarcat{\mv}{A}{B}{\modcath}}


\newcommand\vrelar[3]{\mbox{$#1\stackrel{#3}{\leftarrow}#2$}}
\newcommand\mmvrel[3]{\vrelar{#1}{#2}{#3}}
\newcommand\mmabv{\mmvrel{\mma}{\mmb}{\mmv}}


==> macros/lstlistinglibrary.tex <==
\colorlet{punct}{red!60!black}
\definecolor{delim}{RGB}{20,105,176}
\colorlet{numb}{magenta!60!black}
\definecolor{gray}{rgb}{0.4,0.4,0.4}
\definecolor{darkblue}{rgb}{0.0,0.0,0.6}
\definecolor{lightblue}{rgb}{0.0,0.0,0.4}


\lstdefinelanguage{json}{
	basicstyle=\tiny\normalfont\ttfamily,
	numbers=none,
	numberstyle=\scriptsize, 
	stepnumber=1,
	numbersep=8pt,
	showstringspaces=false,
	breaklines=true,
	frame=single,
	literate=
	*{0}{{{\color{numb}0}}}{1}
	{1}{{{\color{numb}1}}}{1}
	{2}{{{\color{numb}2}}}{1}
	{3}{{{\color{numb}3}}}{1}
	{4}{{{\color{numb}4}}}{1}
	{5}{{{\color{numb}5}}}{1}
	{6}{{{\color{numb}6}}}{1}
	{7}{{{\color{numb}7}}}{1}
	{8}{{{\color{numb}8}}}{1}
	{9}{{{\color{numb}9}}}{1}
	{:}{{{\color{punct}{:}}}}{1}
	{,}{{{\color{punct}{,}}}}{1}
	{\{}{{{\color{delim}{\{}}}}{1}
	{\}}{{{\color{delim}{\}}}}}{1}
	{[}{{{\color{delim}{[}}}}{1}
	{]}{{{\color{delim}{]}}}}{1},
}

\definecolor{maroon}{rgb}{0.5,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\lstdefinelanguage{customxml}{
	basicstyle=\tiny\normalfont\ttfamily,
	numbers=none,
	numberstyle=\scriptsize, 
	stepnumber=1,
	numbersep=8pt,
	showstringspaces=false,
	frame=single,
morestring=[s]{"}{"},
morecomment=[s]{?}{?},
morecomment=[s]{!--}{--},
commentstyle=\color{darkgreen},
moredelim=[s][\color{black}]{>}{<},
moredelim=[s][\color{red}]{\ }{=},
stringstyle=\color{blue},
identifierstyle=\color{maroon}
}

\lstdefinelanguage{interrop}{
	basicstyle=\small\normalfont\ttfamily,
	numbers=left,
	numberstyle=\scriptsize, 
	morekeywords={correspondence,as,relate,check,with,exists,all,and,or,constraint},
	keywordstyle=\color{maroon}
}

\lstdefinelanguage{sigma}{
	basicstyle=\small\ttfamily,
	numbers=none,
	numberstyle=\scriptsize, 
	morekeywords={sig,sorts,opns, eqns, import},
	keywordstyle=\bfseries
}

==> macros/macros4thispaper.tex <==
% macros for this paper only

==> macros/math-lncs.tex <==
% Macros for writing latex math

\makeatletter

\newcommand{\pto}{}% just for safety
\newcommand{\pgets}{}% just for safety
\DeclareRobustCommand{\pto}{\mathrel{\mathpalette\p@to@gets\to}}
\DeclareRobustCommand{\pgets}{\mathrel{\mathpalette\p@to@gets\gets}}
\newcommand{\p@to@gets}[2]{%
	\ooalign{\hidewidth$\m@th#1\mapstochar\mkern5mu$\hidewidth\cr$\m@th#1\to$\cr}%
}
\makeatother

% Commonly used general concepts

\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\absolute}[1]{\lvert{}{#1}\rvert{}}
\newcommand{\semantics}[1]{\llbracket{}{#1}\rrbracket{}}
\newcommand{\inverse}[1]{{#1}^{-1}}
\newcommand{\kleeneStar}[1]{{#1}^*}
\newcommand{\binprod}[2]{{#1} \times {#2}}
\newcommand{\bincoprod}[2]{{#1} + {#2}}
% Arrows
\newcommand{\arrow}[3]{{#2}{:}\;{#1} \to {#3}}
\newcommand{\inlinearrow}[3]{{#1} \xrightarrow{#2} {#3}}
\newcommand{\longinlinearrow}[3]{\xymatrix{{#1} \ar[r]|{#2} & {#3}}}
\newcommand{\partialarrow}[3]{{#2}{:}\;{#1} \rightharpoonup {#3}}
\newcommand{\partialinlinearrow}[3]{{#1} \xrightharpoonup{#2} {#3}}
\newcommand{\partiallonginlinearrow}[3]{\xymatrix{{#1} \ar@{-^{`}}[r]|{#2} & {#3}}}
\newcommand{\relationarrow}[3]{{#2}{:}\;{#1} \pto {#3}}
\newcommand{\relationinlinearrow}[3]{{#1} \overset{#2}{\pto} {#3}}
\newcommand{\relationlonginlinearrow}[3]{\xymatrix{{#1} \ar@{-|>}[r]|{#2} & {#3}}}
\newcommand{\inclusionarrow}[3]{{#2}{:}\; {#1} \hookrightarrow {#3}}
\newcommand{\inlineinclusionarrow}[3]{{#1} \overset{#2}{\hookrightarrow} {#3}}
\newcommand{\longinlininclusionearrow}[3]{\xymatrix{{#1} \ar@{^{(}->}[r]|{#2} & {#3}}}
\newcommand{\monoarrow}[3]{{#2}{:}\; {#1} \rightarrowtail {#3}}
\newcommand{\inlinemonoarrow}[3]{{#1} \overset{#2}{\rightarrowtail} {#3}}
\newcommand{\longinlinemonoarrow}[3]{\xymatrix{{#1} \ar@{>->}[r]|{#2} & {#3}}}
\newcommand{\epiarrow}[3]{{#2}{:}\; {#1} \twoheadrightarrow {#3}}
\newcommand{\inlineepiarrow}[3]{{#1} \xtwoheadrightarrow{#2} {#3}}
\newcommand{\longinlineepiarrow}[3]{\xymatrix{{#1} \ar@{->>}[r]|{#2} & {#3}}}

%\newcommand{\cospan}[5]{\enma{\xymatrix @C=1em {{#1}\ar[r]^{#2} & {#3} & {#5} \ar[l]_{#4}}}}
%\newcommand{\cospanLeftMono}[5]{\enma{\xymatrix @C=1em {{#1}\ar[r]^{#2} & {#3} & {#5} \ar[l]_{#4}}}}
%\newcommand{\cospanLeftIncl}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{^{(}->}[r]^{#2} & {#3} & {#5} \ar[l]_{#4}}}}
%\newcommand{\cospanRightMono}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{>->[r]^{#2} & {#3} & {#5} \ar@{>->}[l]_{#4}}}}
%\newcommand{\cospanRightIncl}[5]{\enma{\xymatrix @C=1em {{#1}\ar[r]^{#2} & {#3} & {#5} \ar@{_{(}->}[l]_{#4}}}}
%\newcommand{\MonoCospan}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{>->}[r]^{#2} & {#3} & {#5} \ar@{>->}[l]_{#4}}}}
%\newcommand{\InclCospan}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{^{(}->}[r]^{#2} & {#3} & {#5} \ar@{_{(}->}[l]_{#4}}}}
\newcommand{\arrowspan}[5]{\enma{\xymatrix @C=2em {{#1} & {#3} \ar[l]_(0.6){#2} \ar[r]^{#4} & {#5} }}}
%\newcommand{\spanRightMono}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar[l]_{#2} \ar@{>->[r]^{#4} & {#5} }}}
%\newcommand{\spanRightIncl}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar[l]_{#2} \ar@{^{(}->}[r]^{#4} & {#5} }}}
%\newcommand{\spanLeftMono}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{>->}[l]_{#2} \ar[r]^{#4} & {#5} }}}
%\newcommand{\spanLeftIncl}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{_{(}->}[l]_{#2} \ar[r]^{#4} & {#5} }}}
%\newcommand{\MonoSpan}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{>->[l]_{#2} \ar@{>->[r]^{#4} & {#5} }}}
%\newcommand{\InclSpan}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{_{(}->}[l]_{#2} \ar@{^{(}->}[r]^{#4} & {#5} }}}


% Commonly used concepts where notions may have to be tweaked from time to time
\newcommand{\compose}[2]{{#1} \fatsemi {#2} }
\newcommand{\altCompose}[2]{{#2} \circ {#1} }
\newcommand{\powerset}[1]{\boldsymbol{2}^{#1}}
\newcommand{\identity}[1]{id_{#1}}
\newcommand{\cat}[1]{\enma{\mathbb{#1}}}
\newcommand{\homset}[3]{{#1}({#2},{#3})}
\newcommand{\functor}[1]{\mathcal{#1}}
\newcommand{\specialClass}[1]{\mathscr{#1}}
\newcommand{\catArrows}[1]{\mathsf{Arr}_{#1}}
\newcommand{\catObj}[1]{\mathsf{Ob}_{#1}}
\renewcommand{\catArrows}[1]{\enma{\mathsf{Arr}(#1)}}
\renewcommand{\catObj}[1]{\enma{\mathsf{Ob}(#1)}}
\newcommand{\sliceCat}[2]{{#1}/{#2}}
\newcommand{\cosliceCat}[2]{{#1}{\setminus}{#2}}
\newcommand{\proofStep}[1]{\langle{}\mbox{#1}\rangle{}}

\newcommand{\pbfunctor}[1]{{#1}^{-1}}
\newcommand{\pbfunctorLeftAdjoint}[1]{\exists{#1}}
\newcommand{\pbfunctorRightAdjoint}[1]{\forall{#1}}

%% Domain of an arrow
%\newcommand{\dom}{\nfont{dom}}
%\newcommand{\hdom}{\nfont{hdom}}
%\newcommand{\vdom}{\nfont{vdom}}
%% Codomain of an arrow
%\newcommand{\cod}{\nfont{cod}}
%\newcommand{\hcod}{\nfont{hcod}}
%\newcommand{\vcod}{\nfont{vcod}}



% All the macros for creating Defitions, Theorems, Proposition etc.
%\newtheorem{mytheo}{Theorem}
%\newtheorem{myprop}{\bf Proposition}
%\newtheorem{lemma}{\bf Lemma}
%\newtheorem{theorem}{\bf Theorem}
%\newtheorem{construction}{\bf Construction}
%\newtheorem{example}{\bf Example}
%\newtheorem{remark}{\bf\em Remark}
%\newtheorem{coro}{\bf\em Corollary}
%\theoremstyle{acmplain}
%\newtheorem{myfact}{Fact}
%\newtheorem{myconj}{Conjecture}
%\newtheorem{mylemma}{\bf Lemma}
%\newtheorem{myclaim}{Claim}
%\newtheorem{mycorr}{Corollary}
%\newtheorem{myparadox}{Paradox}
%\newtheorem{coro}{\bf Corollary}


%\theoremstyle{definition}
%\newtheorem{mydef}{Definition}
%\newtheorem{myaxiom}{Axiom}
%\newtheorem{myprinc}{Principle}
%\newtheorem{myobs}{Observation}
%\newtheorem{myreq}{Requirement}
%\newtheorem{myremark}{Remark}



%\theoremstyle{remark}
%\newtheorem{myexampl}{\bf\em  Example}

%\newtheorem{myconv}{Convention}
%\newtheorem{myexerc}{Exercise}

\newcounter{constrCount}
%\newcounter{conjCount}

\newtheorem{construct}[constrCount]{Construction}
%\theoremstyle{plain}\newtheorem{conjecture}[constrCount]{Conjecture} %\crefname{satz}{Satz}{S\"atze}


\newcommand{\mkTheorem}[3]{
	\begin{theorem}[{#1}]
	\label{#2}
	{#3}
	\end{theorem}
}

\newcommand{\mkProposition}[3]{
	\begin{proposition}[{#1}]
		\label{#2}
		{#3}
	\end{proposition}
}

\newcommand{\mkFact}[3]{
	\begin{fact}[{#1}]
		\label{#2}
		{#3}
	\end{fact}
}

\newcommand{\mkConjecture}[3]{
	\begin{conjecture}[{#1}]
		\label{#2}
		{#3}
	\end{conjecture}
}

\newcommand{\mkLemma}[3]{
	\begin{lemma}[{#1}]
		\label{#2}
		{#3}
	\end{lemma}
}

\newcommand{\mkClaim}[3]{
	\begin{clm}[{#1}]
		\label{#2}
		{#3}
	\end{clm}
}
\newcommand{\mkCorollary}[3]{
	\begin{cor}[{#1}]
		\label{#2}
		{#3}
	\end{cor}
}
%\newcommand{\mkParadox}[3]{
%	\begin{myparadox}[{#1}]
%		\label{#2}
%		{#3}
%	\end{myparadox}
%}


\newcommand{\mkDefinition}[3]{
	\begin{definition}[{#1}]
	\label{#2}
	{#3}
	\end{definition}
}

%\newcommand{\mkAxiom}[3]{
%	\begin{myaxiom}[{#1}]
%		\label{#2}
%		{#3}
%	\end{myaxiom}
%}

%\newcommand{\mkPrinciple}[3]{
%	\begin{myprinc}[{#1}]
%		\label{#2}
%		{#3}
%	\end{myprinc}
%}

\newcommand{\mkObservation}[3]{
	\begin{obs}[{#1}]
		\label{#2}
		{#3}
	\end{obs}
}

%\newcommand{\mkRequirement}[3]{
%	\begin{myreq}[{#1}]
%		\label{#2}
%		{#3}
%	\end{myreq}
%}

\newcommand{\mkExample}[3]{
	\begin{exa}[{#1}]
		\label{#2}
		{#3}
	\end{exa}
}

\newcommand{\mkRemark}[3]{
	\begin{rem}[{#1}]
		\label{#2}
		{#3}
	\end{rem}
}

\newcommand{\mkConvention}[3]{
	\begin{conv}[{#1}]
		\label{#2}
		{#3}
	\end{conv}
}

%\newcommand{\mkExercise}[3]{
%	\begin{myexerc}[{#1}]
%		\label{#2}
%		{#3}
%	\end{myexerc}
%}

\newenvironment{mydef}[1][]
{
\ifthenelse{\equal{#1}{}}{ \begin{definition} \ \em }{ \begin{definition}[{#1}]  \em }%
}
{
\end{definition} 
}


\newenvironment{myprop}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{proposition} \ }{ \begin{proposition}[{#1}] }%	
}
{\end{proposition}}

%\newenvironment{mylem}[1][]
%{
%	\ifthenelse{\equal{#1}{}}{ \begin{lemma} \ }{ \begin{lemma}[{#1}] }%	
%		}
%		{\end{lemma}}

\newtheorem{mylem}{Lemma}%[section]

\newenvironment{mythm}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{theorem} \ }{ \begin{theorem}[{#1}] }%	
		}
		{\end{theorem}}


%\newenvironment{myfact}[1][]
%{
%	\ifthenelse{\equal{#1}{}}{ \begin{fact} \ }{ \begin{fact}[{#1}] }%	
%}
%{\end{fact}}

\newtheorem{myfact}{Fact.}

%\newenvironment{mylem}[1][]
%{
%\ifthenelse{\equal{#1}{}}{ \begin{lemma} \ }{ \begin{lemma}[{#1}] }%	
%}
%{\end{lemma}}

%\newenvironment{mylem}[1]{\begin{lemma}[#1]} {\end{lemma}}

\newenvironment{mycor}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{corollary} \ }{ \begin{corollary}[{#1}] }%	
}
{\end{corollary}}


\newenvironment{myexa}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{example}[] \ }{ \begin{example}[{#1}] }%	
}
{\end{example}}



\newenvironment{myrem}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{remark}[] \ }{ \begin{remark}[{#1}] }%	
}
{\end{remark}}

\newenvironment{myconstr}[1][]
{
	\ifthenelse{\equal{#1}{}}{ \begin{construct}[] \ }{ \begin{construct}[{#1}] }%	
}
{\end{construct}}




==> macros/math.tex <==
% Macros for writing latex math

\makeatletter

\newcommand{\pto}{}% just for safety
\newcommand{\pgets}{}% just for safety
\DeclareRobustCommand{\pto}{\mathrel{\mathpalette\p@to@gets\to}}
\DeclareRobustCommand{\pgets}{\mathrel{\mathpalette\p@to@gets\gets}}
\newcommand{\p@to@gets}[2]{%
	\ooalign{\hidewidth$\m@th#1\mapstochar\mkern5mu$\hidewidth\cr$\m@th#1\to$\cr}%
}
\makeatother

% Commonly used general concepts

\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\absolute}[1]{\lvert{}{#1}\rvert{}}
\newcommand{\semantics}[1]{\llbracket{}{#1}\rrbracket{}}
\newcommand{\inverse}[1]{{#1}^{-1}}
\newcommand{\kleeneStar}[1]{{#1}^*}
\newcommand{\binprod}[2]{{#1} \times {#2}}
\newcommand{\bincoprod}[2]{{#1} + {#2}}
% Arrows
\newcommand{\arrow}[3]{{#2}{:}\;{#1} \to {#3}}
\newcommand{\inlinearrow}[3]{{#1} \xrightarrow{#2} {#3}}
\newcommand{\longinlinearrow}[3]{\xymatrix{{#1} \ar[r]|{#2} & {#3}}}
\newcommand{\partialarrow}[3]{{#2}{:}\;{#1} \rightharpoonup {#3}}
\newcommand{\partialinlinearrow}[3]{{#1} \xrightharpoonup{#2} {#3}}
\newcommand{\partiallonginlinearrow}[3]{\xymatrix{{#1} \ar@{-^{`}}[r]|{#2} & {#3}}}
\newcommand{\relationarrow}[3]{{#2}{:}\;{#1} \pto {#3}}
\newcommand{\relationinlinearrow}[3]{{#1} \overset{#2}{\pto} {#3}}
\newcommand{\relationlonginlinearrow}[3]{\xymatrix{{#1} \ar@{-|>}[r]|{#2} & {#3}}}
\newcommand{\inclusionarrow}[3]{{#2}{:}\; {#1} \hookrightarrow {#3}}
\newcommand{\inlineinclusionarrow}[3]{{#1} \overset{#2}{\hookrightarrow} {#3}}
\newcommand{\longinlininclusionearrow}[3]{\xymatrix{{#1} \ar@{^{(}->}[r]|{#2} & {#3}}}
\newcommand{\monoarrow}[3]{{#2}{:}\; {#1} \rightarrowtail {#3}}
\newcommand{\inlinemonoarrow}[3]{{#1} \overset{#2}{\rightarrowtail} {#3}}
\newcommand{\longinlinemonoarrow}[3]{\xymatrix{{#1} \ar@{>->}[r]|{#2} & {#3}}}
\newcommand{\epiarrow}[3]{{#2}{:}\; {#1} \twoheadrightarrow {#3}}
\newcommand{\inlineepiarrow}[3]{{#1} \xtwoheadrightarrow{#2} {#3}}
\newcommand{\longinlineepiarrow}[3]{\xymatrix{{#1} \ar@{->>}[r]|{#2} & {#3}}}

%\newcommand{\cospan}[5]{\enma{\xymatrix @C=1em {{#1}\ar[r]^{#2} & {#3} & {#5} \ar[l]_{#4}}}}
%\newcommand{\cospanLeftMono}[5]{\enma{\xymatrix @C=1em {{#1}\ar[r]^{#2} & {#3} & {#5} \ar[l]_{#4}}}}
%\newcommand{\cospanLeftIncl}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{^{(}->}[r]^{#2} & {#3} & {#5} \ar[l]_{#4}}}}
%\newcommand{\cospanRightMono}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{>->[r]^{#2} & {#3} & {#5} \ar@{>->}[l]_{#4}}}}
%\newcommand{\cospanRightIncl}[5]{\enma{\xymatrix @C=1em {{#1}\ar[r]^{#2} & {#3} & {#5} \ar@{_{(}->}[l]_{#4}}}}
%\newcommand{\MonoCospan}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{>->}[r]^{#2} & {#3} & {#5} \ar@{>->}[l]_{#4}}}}
%\newcommand{\InclCospan}[5]{\enma{\xymatrix @C=1em {{#1}\ar@{^{(}->}[r]^{#2} & {#3} & {#5} \ar@{_{(}->}[l]_{#4}}}}
\newcommand{\arrowspan}[5]{\enma{\xymatrix @C=2em {{#1} & {#3} \ar[l]_(0.6){#2} \ar[r]^{#4} & {#5} }}}
%\newcommand{\spanRightMono}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar[l]_{#2} \ar@{>->[r]^{#4} & {#5} }}}
%\newcommand{\spanRightIncl}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar[l]_{#2} \ar@{^{(}->}[r]^{#4} & {#5} }}}
%\newcommand{\spanLeftMono}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{>->}[l]_{#2} \ar[r]^{#4} & {#5} }}}
%\newcommand{\spanLeftIncl}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{_{(}->}[l]_{#2} \ar[r]^{#4} & {#5} }}}
%\newcommand{\MonoSpan}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{>->[l]_{#2} \ar@{>->[r]^{#4} & {#5} }}}
%\newcommand{\InclSpan}[5]{\enma{\xymatrix @C=1em {{#1} & {#3} \ar@{_{(}->}[l]_{#2} \ar@{^{(}->}[r]^{#4} & {#5} }}}


% Commonly used concepts where notions may have to be tweaked from time to time
\newcommand{\compose}[2]{{#1} \fatsemi {#2} }
\newcommand{\altCompose}[2]{{#2} \circ {#1} }
\newcommand{\powerset}[1]{\boldsymbol{2}^{#1}}
\newcommand{\identity}[1]{id_{#1}}
\newcommand{\cat}[1]{\enma{\mathbb{#1}}}
\newcommand{\homset}[3]{{#1}({#2},{#3})}
\newcommand{\functor}[1]{\mathcal{#1}}
\newcommand{\specialClass}[1]{\mathscr{#1}}
\newcommand{\catArrows}[1]{\mathsf{Arr}_{#1}}
\newcommand{\catObj}[1]{\mathsf{Ob}_{#1}}
\renewcommand{\catArrows}[1]{\enma{\mathsf{Arr}(#1)}}
\renewcommand{\catObj}[1]{\enma{\mathsf{Ob}(#1)}}
\newcommand{\sliceCat}[2]{{#1}/{#2}}
\newcommand{\cosliceCat}[2]{{#1}{\setminus}{#2}}
\newcommand{\proofStep}[1]{\langle{}\mbox{#1}\rangle{}}

\newcommand{\pbfunctor}[1]{{#1}^{-1}}
\newcommand{\pbfunctorLeftAdjoint}[1]{\exists{#1}}
\newcommand{\pbfunctorRightAdjoint}[1]{\forall{#1}}

%% Domain of an arrow
%\newcommand{\dom}{\nfont{dom}}
%\newcommand{\hdom}{\nfont{hdom}}
%\newcommand{\vdom}{\nfont{vdom}}
%% Codomain of an arrow
%\newcommand{\cod}{\nfont{cod}}
%\newcommand{\hcod}{\nfont{hcod}}
%\newcommand{\vcod}{\nfont{vcod}}

\endinput

\theoremstyle{definition}

==> macros/preamble-lncs.tex <==
\usepackage{diagrams}
% The collection of all the packages I usually require for writing a paper and that are compliant with most Document-Classes
%\usepackage{xypic}
% Required for the right encoding and display of characters
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
% Brings colors to your life
\usepackage{color}

%\usepackage[svgnames]{xcolor}
% Math related packages
%\usepackage{amsmath}

%\usepackage{amsthm}
\usepackage{amssymb}
%\usepackage{amsfonts}

\usepackage{mathrsfs}
% additional CS related symbols
\usepackage{stmaryrd}
% Some more missing math features
\usepackage{mathtools}
\usepackage{bbm}

%\usepackage{oz}
% Correct rendering of URLs
\usepackage{url}
% Allows to give custom labels for enum items
\usepackage{enumitem}
% The old but powerful XY package for drawing mostly commutative diagrams
\usepackage[,all,cmtip]{xy}
% Wrapfig allows to have text floating around figures
\usepackage{wrapfig}
% Necessary for \includegraphics command
\usepackage{graphicx}
% The more powerful table package
\usepackage{tabularx}
% Needed for sub-figures
%\usepackage[caption=false]{subcaption}
\usepackage{subfig}

% The free mason pigpen cypher font, that we abuse for pullback and pushout
% pullback is {\pigpenfont J}
% pushout is {\pigpenfont R}
\usepackage{pigpen}
% TiKZ 
\usepackage{tikz}
\usetikzlibrary{cd}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{shapes,shapes.arrows,shapes.geometric}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\pgfdeclarelayer{background}
\pgfdeclarelayer{overlay}
\pgfsetlayers{background,main,overlay}
% Listings
\usepackage{listings}
% Some typographical hacks
%\usepackage{microtype}
% Nicer tables
\usepackage{booktabs}






==> sections/allMisc.tex <==
\input{sections/workflows}
\input{sections/engineering}
\input{sections/categories}
\input{sections/deepSemantics}
\input{sections/squareArity}
\input{sections/outdated}

==> sections/app4notation.tex <==
%\mkRemark{Notation}{rem:notation}{
%\begin{myremark}[Notation]\label{rem:notation}
%\section{Appendixes}
\section{Notation and terminology}\label{sec:notation}


\section{Proofs}
%\input{sections/proof-prizmLemma}

==> sections/backgr2-indexedSat.tex <==
\subsection{Why indexing}\label{sec:ske4systems}

%There are several serious deficiencies of this \fwk\ wrt. its application to \IMt, %software interoperability,
%where models become many-sorted data instances (with hundreds of sorts), and sentences are sort-spanning constraints. We will briefly discuss three of them.  

We will briefly discuss two shortcomings of ordinary/non-plus sketches when it comes to modelling system design practice. 

a) For safety-critical constraints, a satisfaction instance  $m\satrelsymbol c$ is to be verified by a suitably certified procedure (of model checking, simulation, %a theorem prover, 
or an expert review), and normative documents regulating safety assurance demand those procedures to be explicitly referenced. This makes \sation\ a ternary rather than binary relation, $\models\subset M\timm C \timm V$, and we write $m\models^v c$ meaning that ``$m$ satisfies $c$ with verification assurance level $v$''. If needed, $v$ can be a reference to a richer structure than just a set $V$.

b) Both constraints and instances are considered %Yet another deficiency is considering the logical constructs in isolation from real problems they are intended to model and 
in the static change-free setting while %We will refer to such as to a {\em real system} \sysS, which logical systems aim to model. In this view, 
% Let us refer to this reality background as to a {\em system} \sysS, which encompasses several sets and functions described below. 
practically everything in the world of software and data engineering changes so that objects of interests keep their identity %(\eg, a \req\ named $r$) 
but change their state.  %(\eg, $r$'s formal model $\pii_S(r)=\phi$). Then models and sentences/constraints become trajectories, which may intersect (and have loops).
For example, a formal constraint (sentence) $c$ modelling a safety \req\ $r$ changes over time when the object $X$ that must meet $r$ changes, or a safety standard changes the content of $r$ and hence $c$ should be changed, or a fatal accident forces engineers to strengthen $c$. Then \req\ $r$ appears as a trajectory \frar{r}{T}{\Senset} in the space of sentences/constraints rather than a point in it (here $T$ is a set of (logical) time moments). Then for a given unspecified moment, we have an {\em indexing projection} function \frar{\pii_\senfun}{I_\senfun}{\Senset}, where we refer to \req s as to {\em sentence} {\em indexes} from set $I_\senfun$. Similar considerations are important also  for models. A complex system is necessarily developed by multiple teams, each one building its own subsystem, so that system design appears as a trajectory \frar{d}{T}{\Modset}.
%or designing its own view of a system, 
At a given moment, we again have indexing 
\frar{\pii_\modfun}{I_\modfun}{\Modset}, where elements from set $I_m$ are intentions/plans/goals realized by models. As a rule, both indexing functions are not injective so that collections \Modset\ and \Senset\ appear as multisets rather than sets, and the notion of satisfaction is to be correspondingly adjusted. 
%
%Similarly, set \Modset\ may be a set of version numbers and then  function \sysmodfun\  is typically injective, but imagine an audit of a model that did not reveal any changes to be made (a rare but not impossible event). Then it is reasonable to increase the version number by 1 but set $\pii_M(i)=\pii_M(i+1)$. 
%
\footnote{Remarkably, constraint indexing was introduced into the (generalized) sketch \fwk\ by Makkai \cite{makkai-ske} by purely mathematical reasons as sketches with indexed constraints 
	%(Makkai calls them \specifin s) 
	behave mathematically better. 
	%(To wit: a remarkable fact discovered by Makkai is that if sketches are built over graphical objects specifiable as functors \frarxy{\II}{\setcat}, \ie, the \caty\ of graphs underlying sketches is a copresheaf topos, then the \caty\ of sketches with indexed constraints is a copresheaf topos as well. In other words, sketches, \ie, schemas with constraints are graphs!) 
	Similarly, indexing introduced into the sketch \fwk\ in the present paper, directly leads to the third verification leg for the \sation\ relation.}
%


==> sections/backgr2-logic4sysEng.tex <==
\section{Background 2: Adapting logic for system engineering}

\zd{It's an great new stuff, but not for this paer!}

\input{sections/backgr2-verifiedSat}
\input{sections/backgr2-indexedSat}

==> sections/backgr2-verifiedSat.tex <==
%
\subsection{Around Sat: why categories, why sat-axiom, locality? }
This seemingly simple defintiuon hides several intricacies. First, it is unjustifiably discrete and missing sentence and sat-\mor s. Moreover, it makes sense to consider spans rather than relations. The twisted sat-axiom alos needs a discussion. 
We will discuss several additions, one by one, as a sequence of brief discussions, first for the homogeneous setting when a signature \Sigmaa\ is fixed, and then for the heterogeneous setting dealing with signature \mor s.

\smallskip
{\em Homogeneous setting}:
\begin{enumerate}[label=\alph*)] %[label=\roman*)] %[label=\arabic*)]
	\item {\em Why sentence \mor s.}Dependencies, sorts ``A person $x$  is a good student if $\phi(x)$, but then $\phi(x)$ implies $\nmf{Student}(x)$.  Of course, a better solution is to make \nmf{Student} a sort, and then we come to a constraint logic but again....\zd{to be finished}
	\item {\em Why sat-spans rather than relations.} Assurance, pieces of evidence etc. Thinking discretely, we have a set $\modelssig$ of pieces of {\em evidence} endowed with two functions : \flar{\satleftleg}{\Ob\Modcatsig}{\modelssig} and 
	\frar{\satrightleg}{\modelssig}{\Ob\Sencatsig}. We write   $m\modelssig^e\phi$ if $e\in\,\modelssig$ with $m=\satleftleg(e)$ and $e.\satrightleg =\phi$. 
	\item {\em Why span \mor s.}  In the system engineering setting, we have object identities and mutable object states, and thus both models and evidence elements are updated. It makes sense to consider \modelssig\ to be a \caty\ and its legs being functors rather than functions. Then a {\em sat-state update} is a triple $(u_M, u_E,\iotaa)$ of arrows in $\Modcatsig\timm\modelssig\timm\Sencatsig$:  a {\em model update} \frar{u_M}{m}{m'}, a sentence {\em inference} \frar{\iotaa}{\phi}{\phi'}, and an {\em evidence update} \frar{u_E}{e}{e'} such that the two squares formed with span's legs commute: $\satleftleg.u_M=u_E.\satleftleg$ and $\satrightleg.\iotaa=u_E.\satrightleg$. This is nothing but the standard notion of a span \mor, which does make sense in our context. 
	%	
	%	A standard notion of a span \mor\ does make sense in our context. A {\em sat-span \mor} is a triple $(u,s,\iotaa)$ of homogeneous a {\em model update} \frar{u_M}{m}{m'}, a sentence {\em inference} \frar{\iotaa}{\phi}{\phi'}, and an {\em evidence update} \frar{u_E}{\modelssig}{\modelssig} such that the two squares formed with span's legs commute: $\satleftleg.u_M=u_E.\satleftleg$ and $\satrightleg.\iotaa=u_E.\satrightleg$. 
\end{enumerate}

\smallskip
%\subsubsection
{ \em Heterogeneous setting}:,
\begin{enumerate}[label=\alph*)] %[label=\roman*)] %[label=\arabic*)]
	\item {\em Why sat-axiom.} The main law of the abstract model theory
	\item Twisted sat-spans  \zd{to be finished}
\end{enumerate}

==> sections/backgrounds/backgr-MMt.tex <==
\subsection{Algebra for model management.}\label{sec:application2}
 In \emph{model management},  models are manipulated as holistic entities, and replacement the one-object-at-a-time approach (micromanagement) by one-model-at-a-time (macromanagement)  turned out very productive \cite{Bernstein2003,%}.
% The respective research domain is called \emph{model management} \cite{
FavreNguyen2005,%Diskin2009,
PaigeKolovosRMW2013%DiskinKokalyM2013
}.  It requires considering high-level operations on models such as model slicing,
 \begin{wrapfigure}{r}{4cm}
 	\vspace{-2ex}
 	\centering
 	\includegraphics[width=\linewidth]{figures/modelMgmtsmall}
 	\caption{Model Management}
 	\label{fig:modelMgmt}
 	 \end{wrapfigure}
  %?????   model operations are inherently diagrammatic \cite{me-sle13,me-fase16}. 
  %It requires considering high-level operations on models such as  model slicing, 
  transformation, merging, and synchronization, and composing them into complex workflows  \cite{Diskin-sle13}. 
  Fig.~\ref{fig:modelMgmt} shows a simple example in which two views of the same source are first matched, and then merged. One may think of this as taking the pullback and then the pushout, but in practice these ``pure'' categorical operations are often interwoven with some normalization procedures (and may require conflict resolution) so that even in this simple case the real workflow will be much richer. 
 %
\zd{Importantly, models in SE are typically considered up to their auto-isomorphisms generated by permutations of OIDs (in the sense of OO programming)  which are irrelevant and normally not visible. It justifies making categories of models skeletal, which makes limits and colimits  deterministic algebraic operations. } 

==> sections/backgrounds/backgr-dataMod-bySke.tex <==
\subsection{Algebra for model management.}\label{sec:application2}
 In \emph{model management},  models are manipulated as holistic entities, and replacement the one-object-at-a-time approach (micromanagement) by one-model-at-a-time (macromanagement)  turned out very productive \cite{Bernstein2003,%}.
% The respective research domain is called \emph{model management} \cite{
FavreNguyen2005,%Diskin2009,
PaigeKolovosRMW2013%DiskinKokalyM2013
}. 
 \begin{wrapfigure}{r}{5cm}
 	\vspace{-2ex}
 	\centering
 	\includegraphics[width=\linewidth]{figures/PersonAge}
 	\caption{Data modelling with generalized sketches}
 	\label{fig:PersonAge}
 	 \end{wrapfigure}
  %?????   model operations are inherently diagrammatic \cite{me-sle13,me-fase16}. 
  It requires considering high-level operations on models such as model slicing, transformation, merging, and synchronization, and composing them into complex workflows  \cite{Diskin-sle13}. 
  Fig.~\ref{fig:modelMgmt} shows a simple example in which two views of the same source are first matched, and then merged. One may think of this as taking the pullback and then the pushout, but in practice these ``pure'' categorical operations are often interwoven with some normalization procedures (and may require conflict resolution) so that even in this simple case the real workflow will be much richer. 
 %
\skeletalXok{Importantly, models in SE are typically considered up to their auto-isomorphisms generated by permutations of OIDs (in the sense of OO programming)  which are irrelevant and normally not visible. It justifies making categories of models skeletal, which makes limits and colimits  deterministic algebraic operations. } 

==> sections/backgrounds/backgr-relatedWork.tex <==
\subsection{Related Work and Contributions}
%\zd{Phrase about the diversity of the pool of notions....}
By {\em logic} we refer to work on generalized sketches, and {\em algebra} refers to work on signatures of operation symbols, terms and algebras over them. 

\vspace{-0.25cm}
\subsubsection{Logic.}
Several authors noticed that Ehresmann's sketches can be applied to data modelling \cite{LellahiSpyratos1991,Piessens-tac95,JohnsonRosebrugh2002}. %,Diskin-adbis97}, 
%A majority of these application basically rely on the concept of a \emph{sketch}  introduced by Ehresmann, i.e. a graphical counterpart of a logical theory  (see \cite{Wells} for the history and  \cite{AdamekRosicky1994} for references about their equivalent expressiveness). %and classical Ehresmann's skecthes were employed in all works cited above besides those by D \cite{LellahiSpyratos1991,Piessens-,JohnsonRD-audb01}. 
%By sketch we refer the classical notion introduced by Ehresmann and promoted in \cite{BarrWells1990} and a more \emph{generalized} variant introduced by Makkai \cite{Makkai1997}).
However, these sketches are based on universal properties of the \corring\ diagrams (limit, colimit, powerobject), which (as we discussed above) is a too restrictive setting for applications. %(see \cite{DiskinWolter2008} for a discussion). 
A suitable generalization of sketches motivated by exactly this reason was proposed by Diskin \cite{Diskin-sketches96,Diskin1997}, but even earlier, in a very  different context of an abstract approach to logic, the same generalization was proposed by Makkai, whose preprints had been circulating in early 90s but a summarizing paper \cite{Makkai1997} was published later in 1997.  Makkai developed a coherent theory of generalized sketches and proved a fundamental result that any category of sketches is a presheaf topos. Hence, sketches in a signature $\PP_1$ can be considered as graphs, and hence a new signature $\PP_2$ and a new category of $\PP_2$-sketches over $\PP_1$-sketches-as-graphs can be defined, and so on. In this way, Makkai specified categories with several layers of additional structure as sketches. In our project, we use a different approach in which all discrete signatures $\PP_i$ are integrated into one signature-category $\int_i\PP_i$, whose arrows describe  dependencies between predicate symbols --- an idea first proposed by Wolter and employed in \cite{DiskinWolter2008}. % (see Sect. 4 for details). 
\shortlong{In the TR we prove}{We prove} that Makkai's theorem can be extended for categorical signatures so that the slogan ``sketches are graph'' persists (see \cref{thm:genMakkai} for a precise formulation). 
%: given a presheaf topos of graphs $\GG=\setcat^\HH$ for some schema category \HH, and a set of predicate symbols \PP\ whose arities are \HH-graphs, \PP-sketches whose carriers are \HH-graphs can be considered presheaves on a special (collage) category 
Also, while traditionally sketches are defined in an {\em indexed} way as  families of sets of diagrams indexed by predicate symbols  (for the discrete signature case), or functors {\em from} the signature (for the categorical signature case \cite{DiskinWolter2008}), we define them in an equivalent {\em fibrational} way via a discrete opfibration functor {\em into} the signature: the fibrational definition is more compact and often simplifies technicalities.  

\begin{includeLong}
To give a detailed overview of what is done in the paper in comparison with other work, we need to distinguish between several notions of signatures and sketches. We call a logic {\em basic} if signatures of predicate symbols are sets considered as discrete categories. We call it {\em advanced}, if signatures are categories whose arrows are dependencies between predicates; in addition, these arrows are required to go in one direction, which makes signature \cats\ {\em \hical} (a version of Lawvere's one-way categories). %Traditionally, sketches are defined in an indexed way as families of sets of diagrams indexed by symbols in the discrete signature case, and functors into \setcat\ for categorical signatures. We define them in an equivalent {\em fibrational} way via a discrete opfibration functor into the signature. 
There is also an important distinction between {\em multi-}sketches that allow the same labelled diagram appear in a sketch for multiple times, and {\em mono-}sketches that disallow this. Finally, a partially de-categorificated approach (due to Makkai) is to consider signatures as layered sets so that each predicate in layer $(n+1)$ implicitly depends on all predicates in layer $n$. However, when arities of $(n+1)$-predicates are defined based on $n$-predicates, the actual dependencies appear on the stage. We call this approach {\em discrete \hical (dh)} and show that it is actually equivalent to the categorical one. In these terms, Table \ref{tab:contributionsLogic1} shows the previous work and contributions of the project. Our main results here are an extension of a fundamental Makkai's theorem (that multi-sketches are actually presheaves) for the case of categorical signatures with dependencies,  Th.~\ref{thm:genMakkai}, and  an equivalence of the two approaches to sketches: internally categorical (signatures are categories) and discrete \hical\ (a hierarchy of discrete signatures), Th.~\ref{thm:dh=f}. 
%Naively speaking the contribution of our work can be described as formalization of diagram chasing as e.g. in Fig.~\ref{fig:ex3pb}:
%We formally define diagram operations, diagram algebras and queries (= terms) and show elementary results known from classical algebra to hold in this setting:
%Queries extend to a functor $Q$, algebras are arrows $\frar{a}{Q(A)}{A}$ and there is (symmetric monoidal) Kleisli-Category w.r.t. $Q$, hence the latter also becomes a monad.
%The results are first presented in a discrete setting, i.e. without relations between operations, and then extended to a more general setting with relations between operations, which are needed for syntactical reasoning.
\begin{table}[]
	%\scriptsize
	\footnotesize
	\begin{tabular}{|l|l||l|l|l|}
		\hline
		\multicolumn{2}{|l|}{\multirow{2}{*}{\diagbox{Sketch Def.}{Setting}}} & \multirow{2}{*}{\parbox{2cm}{One-Layer (Basic Logic)}} 
		& \multicolumn{2}{l|}{\qquad Multi-Layer (Advanced Logic)}                          \\ \cline{4-5} 
		\multicolumn{2}{|l|}{}                  &                                          & Discrete Hierarchical         & \qquad Categorical~~                                \\ \hline \hline
		\multirow{2}{*}{Indexed}       & mono-sketches   & \multicolumn{2}{c|}{\multirow{2}{*}{Makkai \cite{Makkai1997}}}                             & Diskin \& Wolter \cite{DiskinWolter2008}                                     \\ \cline{2-2} \cline{5-5} 
		& multi-sketches  & \multicolumn{2}{c|}{}                      & 
		\quad ~~Sect.\,\ref{sec:advancedSketchLogicDefs}  of this TR                            
		\\ \hline
		%\multirow{2}{*}{Fibrational}   & mono   
		\multicolumn{2}{|c||}{Fibrational}  %&
		& 
		\multirow{2}{*}{\parbox{2cm}{\qquad Sect.\, \ref{sec:basicLogic} \\ (Motivational)}} %\ref{sec:basicSketches}}         
		& \multirow{2}{*}{\qquad Sect.\,\ref{sec:discreteHierarchicalSketches}} 
		& \multirow{2}{*}{\qquad Sect.\,\ref{sec:advancedSketchLogicDefs}-\ref{sec:ske=gra}, Th.\ref{thm:genMakkai}} %\ref{sec:avancedSketchLogic}} 
		\\ [5pt]  
		%\cline{2-2} 
		\cline{4-5}
		%& 
		\multicolumn{2}{|c||}{(both mono \& multi)} 
		&                                         
		 &\multicolumn{2}{c|}{\strut Equivalence, Th.~\ref{thm:dh=f} }  %&                                            
		 \\ [5pt] \hline
		 %\\
	\end{tabular}

\medskip
	\caption{\strut Diagram Logic and Contributions}
\label{tab:contributionsLogic1}
\end{table}
\end{includeLong}

\subsubsection{Algebra.}
Diagram operation signatures and algebras were defined first in \cite{Diskin1997} and with some additional details in  \cite{Diskin-sketches96}, but no mathematical results were obtained. For the special case of operations over ordinary graphs, Wolter \etal\ \cite{WolterDiskinK2018} proved that any signature of such operations generates a monad (\ie, a global construct) over the category of graphs. The machinery of {\em local} Kleisli mappings explained informally was used in several papers of the first author, \eg,  \cite{Diskin-models10,Diskin-fase17}, and formalized as Kleisli mappings of a monad (\ie, globally) in \cite{Diskin-fase12}; we are not aware of an accurate formalization of Kleisli mappings considered locally as is done in the present TR,  nor of several other results reported in Sect. \ref{sec:diagramOps-disc-onelayer}. Specifically, we prove that a) sketches and local Kleisli mappings (views) between them form a symmetric monoidal category,  and b) the local Kleisli composition gives rise to a Kleisli triple and hence a  monad (as expected).  
Table~\ref{tab:contributionsAlgebra1} provides an overview of related work in this area and where to find our results in this paper.
\begin{includeLong}
\begin{table}[h]
	%\scriptsize
	\footnotesize
	\begin{tabular}{|l||p{4cm}|p{3.75cm}|}
		\hline
		\diagbox{Topic}{Setting} & Discrete                                                                                
		& \parbox{2cm}{Categorical \\ (Dependencies)} 
		\\ \hline\hline
		Signatures  and Algebras         & 
		\parbox{3.75cm}{Sect.\,\ref{sec:sigAndAlg}; \cite{WolterDiskinK2018}  (graph operations) }                   
		&  \multirow{5}{*}{Sect.\,\ref{sec:opsig-withDeps}, \ref{sec:opsig-dhVersion}}                 
		 \\ \cline{1-2}
		Multiqueries and Substitution   
		&  Sect.\,\ref{sec:mqueries-discrete}                                                                              
		&                      
		\\ \cline{1-2}
				Query Semantics   &  
				Sect.\,\ref{sec:algebraRevisited}                                                                              
				&                      
		\\ \cline{1-2}
		Complex Queries \& Composition &  Sect.\,\ref{sec:complexQueries}                                                                       
		&                     
		\\ \cline{1-2}
		Monads                          
		& \parbox{4cm}{Sect.\,\ref{sec:monadsDiscrete}; \cite{WolterDiskinK2018}  (graph term algebra adjunction)} &                  
		\\ \hline
	\end{tabular}

\medskip
	\caption{Diagram Algebra and Contributions}
	\label{tab:contributionsAlgebra1}
\end{table}

\end{includeLong}


==> sections/backgrounds/backgr-viewsX.tex <==
\subsection{Views.} \label{sec:application1} 
Developing a complex software system normally requires working with multiple \emph{views} \cite{AtkinsonStollB2010} of the system: 
This is the only way to manage complexity and a cornerstone of system engineering, see \cite{FinkelsteinKramerNFG1992} for an early discussion and \cite{FeldmannKernschmidtWV2019,BruneliereBurgerCW2019,CicchettiCicozziP2019} for more recent reports and surveys. 
A view of a {\em source} artifact $S$ is, in general, not merely a part of $S$ or a projection of $S$, but typically involves some computation over $S$,  e.g. composing references, aggregating attributes by summing up their values etc, which extends $S$ with {\em derived} elements produced by some predefined operations (we will say {\em queries}) applied to $S$. Then a {\em view} can be defined as  a mapping $\frar{v}{V}{Q_v(S)}$ in a suitable category of software artifacts where the source $S$ and the view schema $V$ live, and  $Q_v$ is a query that provides an extension $Q_v(S)$ of source $S$ with derived elements required by the view. Section~\ref{sec:viewExample} (in Appendix) presents an example. 


Note an important distinction from the ordinary Kleisli mappings defined for a given monad $\QQ$ or, equivalently, for a global mapping on objects, which only potentially exists and seems unnecessary abstract for software engineers not familiar with Haskell. In contrast, in our notion of view, each view mapping $v$ carries its own query 
 $Q_v$ and maps to its own {\em local} extension $Q_v(S)$ rather than to a unified but huge global extension $\QQ(S)$.  
 \begin{includeShort}
 A simple example in Appendix \ref{sec:viewExample} shows how it works, and also demonstrates the importance of constraints for the view mechanisms. Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
\end{includeShort} 
\begin{includeLong}
	A simple example in \sectref{viewExample}  shows how it works, and also demonstrates the importance of constraints for the view mechanisms. %\shortlong
	{It is placed aside to save time for the first reading, but we encourage the reader to take a look there to obtain a notion of the MDE world and our motivation for this paper.}{}  %Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
%\input{sections/appendix4act20}
\end{includeLong}


==> sections/backgrounds/backgr1-general.tex <==
%!TEX root = ../lics20.tex

\clearpage
\section{Background}

%First, let us introduce the theoretical background of this paper.

\input{sections/notationalConventions}


\subsection{Fibrations}

When defining the \emph{semantical} interpretation of formal structures, there are two approaches: \emph{Indexed} and \emph{Fibrational}.
Indexed semantics are arguably more prevalent in mathematics and are realized as functor into a suitable universe $\mathcal{U}$, most commonly $\catSet$.
In fibrational semantics the collection of all instances make up the semantical interpretation,
where instances are realized as \emph{typing}-morphisms.
Both notions are basically equivalent, which is a result of the Grothendieck equivalence.
While functor-categories $[\cat{C},\mathcal{U}]$ (used for indexed semantics) are well-known and widespread, fibrations are not equally widespread, thus let us recall the respective definitions.
Fibrations were introduced by Grothendieck \cite{Grothendieck2004} and further developed in \cite{Gray1966}.
We also refer to \cite{LoregianRiehl2019} for a recent a comprehensive survey on the topic.

\begin{mydef}[(Op-)Cartesian Arrow]
Let $\cat{E}$ and $\cat{B}$ be two categories and $\arrow{\cat{E}}{P}{\cat{B}}$ be a functor.
\begin{enumerate}
	\item An arrow $\arrow{X}{f}{Y}$ with $P(f) = \arrow{I}{u}{J}$ is called \emph{cartesian} over $u$ iff. for any arrow $\arrow{Z}{g}{Y}$ where there exist $\arrow{P(Z)}{w}{I}$ with $\compose{w}{u} = P(g)$ there exists a unique $\arrow{Z}{h}{X}$ such that $\compose{h}{f} = g$ and $P(h) = w$.
	\begin{equation}
	\label{eq:cartesian}
	\tag{Cartesian Arrow}
	\xymatrix @C= 5em {
		\cat{E} \ar[ddd]_{P}  & \textcolor{blue}{Z} \ar@[blue][dr]_{\textcolor{blue}{g}} \ar@[red]@{-->}[r]^{\textcolor{red}{h!}} & X \ar[d]^f \\
		& & Y \\
		&  \textcolor{blue}{P(Z)} \ar@[blue][r]^{\textcolor{blue}{w}\textcolor{red}{= P(h)}} \ar@[blue][dr]_{\textcolor{blue}{P(g)}} & I  \ar[d]^u \\
		\cat{B} & & J
	}
	\end{equation}
	\item  An arrow $\arrow{X}{f}{Y}$ with $P(f) = \arrow{I}{u}{J}$ is called \emph{cartesian} over $u$ iff. for any arrow $\arrow{Z}{g}{Y}$ iff. for any arrow $\arrow{X}{g}{Z}$ where there exists $\arrow{J}{w}{P(Z)}$ with $\compose{u}{w} = P(g)$ there exists a unique $\arrow{X}{h}{Z}$ such that $\compose{f}{g} = h$ and $P(h) = w$.
	\begin{equation}
	\label{eq:opcartesian}
	\tag{Opcartesian Arrow}
	\xymatrix @C= 5em {
		\cat{E} \ar[ddd]_{P}  & X \ar[d]^f \ar@[blue][r]^{\textcolor{blue}{g}} &  \textcolor{blue}{Z}  \\ 
		& Y \ar@[red]@{-->}[ur]_{\textcolor{red}{h!}} &  \\
		&  I  \ar[d]_u  \ar@[blue][r]^{\textcolor{blue}{P(g)}} & \textcolor{blue}{P(Z)}    \\
		\cat{B} & J \ar@[blue][ur]_{\textcolor{blue}{w}\textcolor{red}{= P(h)}} & 
	}
	\end{equation}
\end{enumerate}
A (op)cartesian arrow $f$ is called \emph{weak} if the above conditions only hold for $g$'s being identities $\identity{X}$.
\end{mydef}

\begin{mydef}[(Op-)Fibration]
A functor $\arrow{\cat{E}}{P}{\cat{B}}$ is called a \emph{fibration} iff for every $Y \in \catObj{\cat{E}}$ and $\arrow{I}{u}{P(Y)} \in \catArrows{\cat{B}}$ there exists a cartesian arrow $\arrow{X}{f}{Y}$ such that $P(f) = u$.\par
Dually, $P$ is called an \emph{opfibration} iff. for every $X \in \catObj{\cat{E}}$ and $\arrow{P(X)}{u}{J} \in \catArrows{\cat{B}}$ there exists a an opcartesian arrow $\arrow{X}{f}{Y}$ such that $P(f) = u$.

One distinguishes different kinds of (op)fibrations:
\begin{itemize}
	\item Iff. for every arrow in $\cat{B}$ there exists only a \emph{weak (op)cartesian} lifting, $P$ is called a \emph{weak}(op)fibration.
	\item Iff. $P$ is additionally endowed with a \emph{choice of liftings}, called \emph{cleavage}, $\frar{\kappa}{\catObj{\cat{E}} \times \catArrows{\cat{B}}}{\catArrows{\cat{E}}}$, the (op)fibration is called \emph{cloven}.
	\item Iff. $P$ is a cloven (op)fibration which additionally respects composition, it is called a \emph{split} (op)fibration. (for all $\frar{u}{i}{J}$ and $\frar{v}{J}{K}$ in  $\catArrows{\cat{B}}$ it holds $\kappa(u) \comp \kappa(v) = \kappa(u \comp v)$).
	\item Iff. for every pair comprising an object $X$ in $\catObj{\cat{E}}$ and arrow $u$ in $\catArrows{\cat{B}}$ there exists \emph{exactly one} (op)cartesian lift of $u$, $P$ is called a \emph{discrete} (op)fibration.
\end{itemize}
\end{mydef}

\begin{mydef}[Categories of Fibrations]
For every category $\cat{B}$, the collection of all fibrations over $\cat{B}$, denoted $\catname{Fib}(\cat{B})$, forms a subcategory of $\sliceCat{\catCat}{\cat{B}}$.
Likewise all discrete fibrations, opfibrations and discrete opfibrations $\catname{DFib}(\cat{B})$, $\catname{Opfib}(\cat{B})$, $\catname{DOpfib}(\cat{B})$.
\end{mydef}

The following equivalence is attributed to Alexandre Grothendieck

\begin{myfact}[Grothendieck Equivalence]
	There is an equivalence of 2-categories
\begin{equation}
	\boldsymbol{\int} : \catname{Fib}(\cat{B}) \cong \catname{Psd}[\cat{B}^{op}, \catCat]
\end{equation}
where $\catname{Psd}[\cat{B}^{op}, \catCat]$ is the category of pseudo-functors from $\cat{B}^{op}$ into $\catCat$.
The functor going from right to left in this equivalence is commonly known as the \emph{Grothendieck construction}.

In case of discrete fibrations, the situation is as follows:
\begin{equation}
\boldsymbol{\int}_D : \catname{DFib}(\cat{B}) \cong  [\cat{B}^{op}, \catSet]
\end{equation}
\end{myfact}




==> sections/backgrounds/backgr4act21.tex <==
\section{Background}\label{sec:backgr}

\subsection{Data modelling with generalized sketches}\label{sec:datamod-via-Ske}
%\input{figures/backgr-dataMod-bySke}



 \begin{wrapfigure}{r}{6cm}
	\vspace{-2ex}
	\centering
	\includegraphics[width=\linewidth]{figures/forAct21-PersonAge}
	\caption{Data modelling via sketches}
	\label{fig:personAge}
\end{wrapfigure}
\renewcommand{\thefig}{\cref{fig:personAge}}

\thefig\ presents a very simple example of data modelling. The colourful diagram is a directed graph $S$ with various labels, which specify some data {\em schema}. The latter is to be {\em instantiated} via a model functor \frar{\semm{\cdot}}{S}{\setcat}, which is supposed to respect the labels as explained below.%
\footnote{To be accurate, to make $S$ and \setcat\ objects in the same category so that \semm{\cdot} would be its morphism, we either should consider the underlying graph of \setcat\ so that \semm{\cdot} would be a graph morphism, or consider the category freely generated by $S$, and in either case abuse the notation by using the same symbols for two different objects.} Rectangles are nodes without labels, and there is one such called \Person. Such nodes are interpreted by finite sets, \eg, \semm{\Person} can be the set of employees of some company at some date; as a rule, such sets change over time (employee can be hired, fired, etc).  Oval nodes refer to predefined constant sets, \eg, \semm{\String} is a fixed set of all strings available in a given universe. We interpret this as shown in the callout figure: there is a constraint $C_\String$ attached to node \String, and we say that an instance \frar{\semm{\cdot}}{S}{\setcat} satisfy $C_\String$ (we then write $\semm{\cdot}\models C_\String$) iff $\semm{\String}=\text{``the set of all strings''}$. Similarly, nodes \Int\ and \Date\  refer to all integres and all dates , and node \unitt\ is interpreted by a chosen singleton. Similarly, arrows \dayy,\monthh, and \yearr\ are constant functions mapping a date to its day, month, and year.  Constraint $C^0_\Date$ requires the triple of functions $(\semm{\dayy},\semm{\monthh},\semm{\yearr)})$ to be jointly monic, and three constraints $C^{i}_\Date$, $i\in\{30,31,Feb\}$ require legal instances to respect the number of days in different months. Note that $C^{Feb}_\Date$ is a constraint for the entire triple of functions while the other two constraints constrain the pair $(\dayy, \monthh)$.  Arrow \frar{\current}{\unitt}{\Date} selects a particular element in set \semm{\Date}, and moreover, having a (global) clock attached to instantiation, this element is to be equal to the current date. Thus, arrow \current\ is also a constant but changeable by ticks of the global clock so that constraint $C_\current$ imposed on the arrow \frar{\mathit{current}}{\unitt}{\Date} is actually temporal. 

Arrows \name\ and \bDate\ are ordinary arrows (in Sanserif  in contrast to slanted constants) that give each person in \semm{\Person} its \name-string and \bDate-date.  In addition, schema $S$ requires for any legal instance \semm{\cdot}, all objects in set \semm{\Person} are to be born earlier than 2000. To declare this constraint, we first apply the operation of arrow composition to arrows \bDate\ and \yearr\ and then declare the constraint $C_\bDate:= [\_< 2000]$ for the composed arrow, which uses the predefined binary predicate $<$ on predefined set \semm{\Int}. Thus (as \semm{\cdot} is a functor), we have  
$$\semm{\cdot}\models C_\bDate \text{ iff } 
p.\semm{\bDate}.\semm{\yearr}<2000 \text{ for all $p\in\semm{\Person}$ }
$$ 

==> sections/backgrounds/backgr_fromAct20overview.tex <==
\section{Background and Contributions} 
%Motivation: Why we need a view mechanism over generalized sketches}
 
 We discuss two main applications of the \fwk\ in SE in Sect.2.1-2 (plus Sect.~\ref{sec:viewExample} in Appendix), then discuss some mathematical aspects of the \fwk\ in Sect.2.3, and describe related work and contributions in Sect.2.4. 
 %Section 2.5 	presents our main motivating example % simple example in \sectref{viewExample}  shows how it works, and also demonstrates the importance of constraints for the view mechanisms.
 Sect. 2.5 overviews our notation.
 
\input{sections/backgr-viewsX} 
 \input{sections/backgr-MMt} 
Thus, for both the inter-model and the intra-model levels of reasoning, SE needs powerful and formally specified algebraic machinery for diagrammatic operations. On the other hand, it seems that even basic universal algebraic constructs (signature, term, parsing) have not been accurately specified for diagrammatic operations, especially when the latter are considered together with pre-and post-conditions and hence are interwoven with logic; in this sense, we are developing some basic universal algebra for diagrammatic operations. 
  
\input{sections/backgr-mathAspects} 
\input{sections/backgr-relatedWork} 
%\input{sections/viewExample}
\input{sections/notationalConventions}


% not needed anymore
%\input{sections/whyConstraintsIndexed}




==> sections/backgrounds/background.tex <==
%!TEX root = ../lics20.tex

\clearpage
\section{Background 1: Categories and diagrams}

%First, let us introduce the theoretical background of this paper.

We assume that the reader is familiar with the fundamental concepts of category theory as they an be found in every standard textbook, e.g. \cite{BarrWells1990}. Our notation for basic categorical notions can be found in Appendix \sectref{notation}.  
 

\subsection{Categories} The goal is to fix our notation and terminology. To manage size issues, we consider all categories in the paper are small... \zd{check at nLab about Grothendieck universe.}
For variables referring to categories, we use blackboard font, e.g. $\cat{G}$. Names of special categories such as $\catSet$ or $\catCat$ are in bold italic. 

\subsubsection{Notation for objects and arrows}
For a small category \CC, its set of objects and set of arrows (\mor s) will be denoted by $\catObj{\cat{C}}$ and $\catArrows{\cat{C}}$ resp. We will also write $\Elem{\CC}$ for the set $\Ob{\CC}\sqcup\Arr{\CC}$. 

As a rule, for objects  we will use uppercase letters, e.g. $X \in \catObj{\cat{C}}$ and for morphisms we will use lowercase letters, e.g. $f \in \catArrows{\cat{C}}$.
In typical abuse of notation, we will usually denote memberships of objects and arrows in a specific category by simply writing $X\in \cat{C}$ or $f \in \cat{C}$.
The domain of an arrow $f$ will be denoted by $dom(f)$ and the codomain by $cod(f)$ (one may as well think of $dom$ and $cod$ as mappings from $\catArrows{\cat{C}}$ to $\catObj{\cat{C}}$).
We follow the common practice to write $\arrow{X}{f}{Y}$ (or $\inlinearrow{X}{f}{Y}$ in diagrams) for an arrow $f \in \catArrows{\cat{C}}$ with $dom(f) = X$ and $cod(f)=Y$.
The hom-set of all arrows between two objects $X,Y \in \catObj{\cat{C}}$ will be denoted $\homset{\cat{C}}{X}{Y}$.

We write $\CC(X,\_)$ for $\bigcup_{Y\inn\Ob{\CC}}\CC(X,Y)$ and similarly for $\CC(\_,Y)$.
\subsubsection{Arrow composition and application}
Composition of two arrows $\arrow{X}{f}{Y}$ and $\arrow{Y}{g}{Z}$ will be denoted either in the diagrammatic order $\arrow{X}{\compose{f}{g}}{Z}$ or the application order $\arrow{X}{\altCompose{f}{g}}{Z}$.

For a mapping \frar{f}{X}{B^A} and $x\inn X$, we will often write $f^x$ or $f_x$  rather than $f(x)$ to make reading  applications of $f(x)$ to elements of $A$ easier:  $f^x(a)$ rather than $f(x)(a)$ (although the latter form will be used too). Similarly, if $f(x)$ is a domain of another arrow \frar{g}{f(x)}{y}, we will often write $x^f$ for $f(x)$ so that \frar{g}{x^f}{y}.

To highlight special properties of morphisms, we denote a monomorphism $m$ by $\monoarrow{X}{m}{Y}$ and an epimorphism $e$ by $\epiarrow{X}{e}{Y}$
% \zd{I'd prefer $X\rCover Y$}.
\zd{and we need a big talk about $\righthookarrow$ as a synonymic symbol for monic, or not synonymic? }
Finally, we will interchangeably use expressions $\cat{C}^\cat{D}$ or $[\cat{C},\cat{D}]$ to denote the functor category between $\cat{C}$ and $\cat{D}$, $\sliceCat{\cat{C}}{X}$ for the slice category under $X \in \catObj{\cat{C}}$, $\cosliceCat{\cat{C}}{C}$ for the coslice category over $X \in \catObj{\cat{C}}$, and $\cat{C} \times \cat{D}$ for the product category.
%}
%\end{myremark}
\subsubsection{Carriers}

{
	\renewcommand\pmb[1]{#1} % juts for this piece
	In some contexts, where the domain of a mapping gives the name of the story, we will use the following (categorically, rather odd) naming for components of an arrow \frar{f}{X}{Y}. We will consider this arrow as a pair $\pmb{X}=(\carr{\pmb{X}}, f_X)$ where the domain of $f$ is now denoted by \carr{X} and called the {\em carrier} of $X$ while the arrow itself is denoted by $f_X$ and is referred to as the {\em mapping} of $X$. All these are fully terminological permutations as pair $X$ and arrow $f$ are the same formal construct. %stands for $X$ and is called the {\em carrier} of the pair $\pmb{X}$. 
	Moreover, by a common abuse of notation, we will overuse symbol $\pmb{X}$ to refer to the carrier \carr{\pmb{X}}, and will often omit the superscript $X$ in $f_X$.  
}

\newcommand\arrcatC{\arrowCat{\CC}}
\newcommand\domC{\enma{\dom_{\CC}}}
\newcommand\codC{\enma{\cod_{\CC}}}
\renewcommand\domC{\dom} %enma{\dom_{\CC}}}
\renewcommand\codC{\cod} %\enma{\cod_{\CC}}}

\subsection{Diagram categories}

We will recall a few basic definitions and results and build several new auxiliary constructs needed later. 

%\begin{mydef}{diagcats}{Diagram categories} 

A {\em diagram} in a category \CC\ is a functor \frar{\dvar}{\callid}{\CC} whose domain is a category freely generated by a graph $D$ called the {\em shape} of the diagram (and \callid\ is also called the {\em shape}). Sometimes we will make $D$ a sketch by adding to it \corring\ declarations, \eg, a valid diagram of shape $\imgmsquarepo$ must map two horizontal arrows into monics, and the entire square into a pushout square in \CC. A precise formalization of this construct in general is exactly the subject of the paper, but in the metatheory  we will only use simple sketches like above that can well be explained like above. 

 A {\em diagram \mor} is a natural \trafon\ between functors, \drar{\dmorvar}{\dvar}{\dvar'}, \ie, a family of arrows \frar{\dmorvar_x}{x^\dvar}{x^{\dvar'}} indexed by $x\in\Ob{\callid}$ such that $a^\dvar\comp\dmorvar_y =\dmorvar_x\comp a^{\dvar'}$ for any arrow \frar{a}{x}{y} in \callid. This gives us the category $\left[\callid, \CC \right]$ of all diagrams in \CC\ of shape \callid. 

In subsection \sectref{arrowcats} we will consider categories of diagrams whose shape is a single arrow, and in \sectref{msquarepo}, we consider categories of diagrams of the square shape above.
\subsubsection{Arrow categories.}\label{sec:arrowcats}
%\zd{This piece should accurately be written and explain all our notation. }
\begin{mydef}{arrcats}{Arrow categories} Any category \CC\ gives rise to an {\em arrow \caty} \arrcatC\ whose objects are \CC-arrows and \mor s are commutative squares:
 given two \CC-arrows $a,b$, their morphism is a pair of \CC-arrows, \frar{f}{\fancydom{a}}{\fancydom{b}} and \frar{f'}{\fancycod{a}}{\fancycod{b}}, such that the square commutes: $a\comp f'=f\comp b$. We call such a pair an {\em sq-arrow} and write \drar{(f,f')}{a}{b}.
 
 Any object $X\in \CC$ gives rise to a {\em dom-pointed} arrow category  
 $\dompointedarrowCat{\CC}{X}\subset\arrowCat{\CC}$ whose objects are arrows from $X$ and the \corring\ component of all sq-arrows is $\id_X$. Similarly, we have {\em cod-pointed} arrow \caty\ $\codpointedarrowCat{X}{\CC}\subset\arrowCat{\CC}$. These \cats\ usually denoted by $\cosliceCat{\CC}{X}$ and $\CC/X$ resp. 
\end{mydef}
The following facts are proved straightforwardly.
\begin{mylem}{arrcatfibr}{}
 There are two obvious functors \frar{\domC}{\arrcatC}{\CC} and \frar{\codC}{\arrcatC}{\CC}, for which the following holds.
 
 a) For any \CC, functor \domC\ is a {\em split} fibration, its  restriction \frar{\dom_X}{\CC/X}{\CC} (for a given object $X$) is a {\em discrete} fibration, and if \CC\ has pushouts, then \domC\ is also an opfibration.

b) For any \CC, functor \codC\ is a {\em split} opfibration, its restriction \frar{\cod_X}{\cosliceCat{\CC}{X}}{\CC} is a {\em discrete} opfibration, and if \CC\ has pullbacks, then \codC\ is also a fibration.
%
  %Thus, if \CC\ has both pushouts and pullbacks, then both \domC\ and \codC\ are bifibrations.
\end{mylem}
%A bit more formally, $m$ is a diagram in \SS\ of shape \fbox{\frar{\IE}{\I}{\E}} whose image is a monic, and we write $I_m$  and $E_m$ for sketches $m(\I)$ and $m(\E)$ resp., and $m$ for the monic $m(\IE)$.

%\zd{Content of \defref{diagcats}, \defref{diagsubcats}, the lemma in-between and diagram \eqref{codopfib4diag} may also go here}
In \sectref{opsig-depend}, we will heavily use the following construct.
\begin{mydef}{diagcats}{Diagonal arrow \cats}
	%Recall that for any \caty\ \CC,  the arrow \caty\ $\arrowCat{\CC}$ has \CC-arrows as objects and commutative squares of \CC-arrows as morphisms: given two \CC-arrows $a,b$, their morphism is a pair of \CC-arrows, \frar{f}{\fancydom{a}}{\fancydom{b}} and \frar{f'}{\fancycod{a}}{\fancycod{b}}, such that the square commutes: $a\comp f'=f\comp b$. We call such a pair a {\em sq-arrow} and write \drar{(f,f')}{a}{b}. Similarly, \monicarrowCat{\CC} is a full subcategory of \arrowCat{\CC} whose objects are monic arrows (but sq-arrow are pairs of ordinary arrows).
	%
	In an arrow \caty\ \arrcatC,  a sq-arrow \drar{(f,f')}{a}{b} is called {\em diagonal} if there is a ``diagonal'' arrow \frar{d}{\fancycod{a}}{\fancydom{b}} such that $f=a\comp d$, $f'=d\comp b$; then we write $(f,f')=\diagOP{d}$.
\end{mydef}
The associativity of composition ensures the following result.
\begin{mylem}{diagcats}{}
	Composition of two diagonal arrows is again diagonal: if \drar{(f_1,f_1')=\diagOP{d_1}}{a}{b} and \drar{(f_2,f'_2)=\diagOP{d_2}}{b}{c}, then $(f_1,f'_1)\comp(f_2,f'_2) = \diagOP{(d_1\comp b\comp d_2)}$. 
\end{mylem}
\begin{mydef}{diagsubcats}{Diagonal subcategories}
	Given a category \CC, category \arrowdiagCat{\CC} has the same objects as \arrowCat{\CC}, diagonal sq-arrows as arrows between different objects (\ie, different \CC-arrows), and the only looping sq-arrows \drar{(f,f')}{a}{a} being (non-diagonal) identity sq-arrows $f=\id({\fancydom{a}})$, $f'=\id({\fancycod{a}})$. 
	
	\newcommand{\wide}{\nfont{[wide]}}
	\newcommand{\full}{\nfont{[full]}}
	Category \madCat{\CC} is a full subcategory of \adCat{\CC}, whose objects are monic arrows in \CC, and we have the following obvious commutative diagrams:
	\begin{equation}\label{eq:codopfib4diag}
	\begin{array}{c@{\qquad}c}
	\xymatrix{
		\madCat{\CC} \ar@{^{(}->}[rr]^{\wide} \ar@{^{(}->}[dd]_{\full} \ar[rd]|{\dom'}
		&&
		\maCat{\CC} \ar@{^{(}->}[dd]^{\full} \ar[ld]|{\dom''}
		\\
		&\CC &
		\\
		\adCat{\CC} \ar[ru]|{\dom'''} \ar@{^{(}->}[rr]^{\wide}
		&& 
		\arrowCat{\CC} \ar[lu]|{\dom}	
	}
&
	\xymatrix{
	\madCat{\CC} \ar@{^{(}->}[rr]^{\wide} \ar@{^{(}->}[dd]_{\full} \ar[rd]|{\cod'}
	&&
	\maCat{\CC} \ar@{^{(}->}[dd]^{\full} \ar[ld]|{\cod''}
	\\
	&\CC &
	\\
	\adCat{\CC} \ar[ru]|{\cod'''} \ar@{^{(}->}[rr]^{\wide}
	&& 
	\arrowCat{\CC} \ar[lu]|{\cod}	
}
\end{array}
	\end{equation}
	with labels \wide\ and \full\ referring to wide and full embedding resp.  %and the functor \cod\ the standard opfibration given by composition (not to be confused with the Cartesian fibration given by pullbacks). 
	Note that functor $\cod'$ is faithful: if two parallel diagonals are different, %$d_1\noteq d_2$, 
	then their compositions with the target monic arrow are different too.
	To ease notation, below we will denote all four \dom-functors and all four \cod-functors by name \dom\ and \cod, resp., without primes. 
\end{mydef}
\subsubsection{Categories of square shaped diagrams}

\begin{mydef}{bSqcats}{Binding squares and diagrams} %\label{def:squarecats}
The {\em binding square shape} is a fixed category \bSquare\ specified in diagram \eqrefx{bSqFacts}{a}. Diagrams of this shape, \ie, mappings \frar{\dvar}{\bSquare}{\CC}, are required to be pushouts and called {\em binding squares (b-squares)} (note the small corner near node $E_*$ that declares the square as a pushout). For any element $X\in\bSquare$, we write $X^\dvar$ for $\dvar(x)$. Morphisms of b-squares, \trirar{\dmorvar^4}{\dvar}{\dvar'}, are quadruple of arrows $%\pmb{\dmorvar}=
\comprfam{\frar{\dmorvar^4_{X}}{X^\dvar}{X^{\dvar'}}}
	{X\in\{I, E, I_*, E_* \}  }$ making a commutative prism. 

A {\em pointed} binding square is a diagram with one node fixed. We will use pointed diagrams in which......  

Embeddings \frar{\nfont{e}}{\fbox{$\cdot\rightarrow\cdot$}}{\bSquare} 
%and   \frar{IE_*}{\fbox{$\cdot\rightarrow\cdot$}}{\bSquare} 
gives us a projecting functor
  \frar{\nfont{e}\comp\_}{\squarepoCat{\CC}}{\arrowCat{\CC}} denoted by \proj{X} where $X\in\{ IE,b_E,b_I,IE_*  \}$ is the image of \nfont{e}. 
 % and  \frar{\Dom}{\squarepoCat{\CC}}{\arrowCat{\CC}} 
 \end{mydef}
 \begin{mylem}{bSqFacts}{Binding Square Diagrams: Some  Facts}
 %	Functor \frar{\Dom}{\squarepoCat{\CC}}{\arrowCat{\CC}} is a fibration. Moreover, functor 
 %	\frar{\Dom_X} {\squarepoXCat{\CC}{X}} {\arrowCat{\CC}} is a discrete fibration.
Let category \CC\ has pushouts and hence binding diagrams. Then there is a commutative diagram shown in diagram \eqrefx{bSqFacts}{b}, in which (i) functor \proj{IE} is a fibration,  (ii) functor $\proj{IE}^X$ (for a given predefined \CC-object $X$) is a discrete fibration, and (iii) (conjecture) pair $(\cod, \proj{b_E})$ is a fibration \mor.
 \end{mylem}
%\endinput
 \begin{equation}\label{eq:bSqFacts}
%\[
\begin{array}{c@{\quad}c}%@{\quad}l}
\xymatrix{   % diagram a)
	\inputArity{} \ar[r]^{IE} 
	\ar[d]_{b_I} 
	\ar@{}[dr]|(.8){\Large \ulcorner} 
	&  \scopeArity{} 
	\ar@{->}[d]^{b_E} 
%	\\ 	&\nfont{[po]}&
	\\
	I_* \ar[r]^{IE_*} & E_*
}
&  % the commut square diag  b)
\xymatrix{
	\squareXCat{X}{\CC} \ar@{^{(}->}[r]^{I_*=X}
	\ar[d]^{\proj{IE}^X}	
	&\squareXCat{\cdot}{\CC}  % 1st argument is \cdot
	\ar@{->}[d]_{\qquad\proj{IE}} \ar[r]^{\proj{b_E}}
	& \downarrowCat{\CC}\ar[d]^\dom
	\\
    \arrowCat{\CC}\ar@{<=>}[r]^\id 
   &\arrowCat{\CC}\ar[r]^\cod 
   &\CC
}
\\[40pt]
&
\\
\text{a) b-square elements} 
& \text{b) facts about b-square diagrams} 
\end{array}
\end{equation}

{\em Proof.} i) Functor \proj{IE} is a fibration. Given are a binding diagram \dvar\ (whose projection on \arrowCat{\CC} is $IE^\dvar$) and a sq-arrow \drar{\dmorvar^2}{IE^{\dvar'}}{IE^\dvar} (see the black part of the left diagram in \figref{bSqFacts}). We need to build a binding diagram $\dvar'$ and a prism \mor\ \trirar{\dmorvar^4}{\dvar'}{\dvar} such that its upper face is $\dmorvar^2$ --- this is done with the blue-colour workflow in the left diagram in \figref{bSqFacts}. Finally, we need to show that this blue thing is maximal amongst similar $\Rrightarrow$ -- see the red workflow. 

The right diagram in  \figref{bSqFacts} shows a special case where $\dmorvar^2$ is diagonal -- we will need it later for considering queries.

ii) Discrete fibration -- see the green workflow.

iii) Fibr. \mor. Pushout 3D-pasting lemma should work?? 

\begin{figure}
\centering
	\includegraphics[width=0.75\linewidth]{figures/pic-fibrPrism}
\caption{For the proof of lemma \ref{lem:bSqFacts}: lifting workflow}
\label{fig:bSqFacts}
\end{figure}

\section{Background 2: Presheaf toposes}
%\subsection{Presheaf toposes}
%In this paper, presheaf topoi will play an important role. 
In Computer science and Software Engineering context, {\em presheaf} toposes or {\em presheaves} have also been referred to as \emph{``graph-like structures''}, e.g. \cite{Loewe1993}. 

\zdhllok{There is an important difference between sets and presheaves, the latter can usually not be represented as a coproduct (sum) of its elements.}{this is to be said in the intro}{-10}

{\renewcommand{\II}{\enma{\mathcal{S}}}
\begin{mydef}{presheaf}{Presheaf}
Let $\II$ be a small category.
A functor \frar{G}{\II}{\setcat} is called an {\em \II-presheaf} or just a {\em presheaf} if \II\  is clear from the context or is not important, and the category $\setcat^\II$ of all such presheaves and their natural transformations is called a {\em presheaf topos}. \footnote{Usually presheaves are defined as contravariant functors \frar{G}{\II^{op}}{\setcat} %$\arrow{\II^{op}}{P}{\catSet}$ 
	due to their relation and importance for the Yoneda Lemma. For our applications throughout this paper,  it is more convenient to work with the covariant definition.}.

A presheaf  \frar{G}{\II}{\setcat} is called {\em finite} if all sets $G(v)$, $v\in\Ob{\II}$ are finite. 

A presheaf topos is called {\em finitary} if the schema category \II\ is finite. (Makaki says that in ref [3] in his paper 1, such toposes are called finite. 
\end{mydef} 

\mkFact{Presheaf Topos}{fact:presheafTopos}{
Any category of presheaves is a \emph{topos} and thus has 
\begin{itemize}
\item all limits and colimits,
%\item has all colimits.
\item exponents, \ie, is cartesian closed,
\item epi-mono factorizations,
\item a subobject classifier.
\end{itemize}
}

If \II\ is \Graph, then 'graphs' are nothing but ordinary directed multigraph, and if \II\ is \nfont{rGraph}, then 'graphs' are reflexive graphs. If \II\ is \PNet, 'graphs' are Petri nets (bipartite graphs of places and transitions).

Several fixed schema categories we will use are shown in \figref{shapes}. Objects and arrows in these categories are fixed and have fixed names.
% Let $G \in \cat{G}$ an object (graph) in $\cat{G}$.
\begin{figure}[b]
	\begin{tabular}{c@{\qquad}c@{\qquad}c}
		$
		\xymatrix{
			\Node  \\
			\Edge \ar@<+0.5ex>[u]^{\so} \ar@<-0.5ex>[u]_{\ta} 
		}
		$
		&
		$
		\xymatrix{
			\Place & \Trans \\
			\Pre \ar[u]^{\so^i} \ar[ur]_(0.65){\ta^i} & \Post \ar[ul]^(0.65){\ta^o} \ar[u]_{\so^o}
		}
		$
		& 

		$
		\xymatrix @C=0.01cm {
			& & \Node & & \\
			\Edge_{(1,0)} \ar[urr]^(0.7){\so_{(1,0)}} & \Edge_{(0,1)} \ar[ur]^(0.3){\ta_{(0,1)}} & \Edge_{(1,1)} \ar@<+0.5ex>[u]^{\so} \ar@<-0.5ex>[u]_{\ta}  & \Edge_{(2,1)} \ar@<+0.5ex>[ul]_{\so^1_{(2,1)}} \ar@/_/[ul]_{\so^2_{(2,1)}} \ar@/_2pc/[ul]_{\ta_{(2,1)}}   &  \ldots 
		}
		$
		\\
		   a) \Graph 
		& c) \nfont{PNet}
		& d) \nfont{HypGraph}
	\end{tabular}
	\caption{Fixed shape categories}
	\label{fig:shapes}
\end{figure}


 %We assume that for any presheaf \frar{G}{\II}{\catSet} we consider, classes $\abs{\II}$ and $\abs{G}\eqdef\compr{G(i)}{i\in\abs{\II}}$ are disjoint. \zd{here $\abs{\II}$ denotes the class of \II's elements -- should be placed in notation}. We will sometime use the same names for elements in $\abs{\II}$ and $\abs{G}$, which means that with a full notation, those names are to be qualified, say, $x_\II$ and $x_G$, but the subindexes are omitted.  We will also write $x\in G$ for an element $x\in\abs{G}$. %  If we use the same names for elements 

%For the remainder of the paper we will fix a category $\GG := \catSet^\II$ with $\II$ being an arbitrary but \emph{finite category}, whose objects will be called {\em 'graphs'} (often just graphs). If $\II$ is \graph, then 'graphs' are ordinary directed multigraphs, the corresponding presheaf topos is denoted by $\catGraph$. if $\II$ is equal to the following category (identities omitted): \[\xymatrix{ N &  E \ar@<-0.5ex>[l]_{s} \ar@<0.5ex>[l]^{t} }
%\]
%\mkRemark{Set thoeretical notions in Presheaves}{rem:setTheory}{

\subsection{Set-theoretical constructs in presheaf toposes}
Presheaves in many ways behave as sets and we will make use of some set-theoretic concepts throughout the paper. As we have already said, we can speak of \emph{elements} $x \in G$ meaning that there exists an object $I \in \cat{I}$ such that $x \in G(I)$.
Categorically, such a (global) element is modelled by an arrow $x: \boldsymbol{1} \to G$.

\subsubsection{Inclusions }
%Another concept are \emph{inclusions}, which are given by abstract subobjects.
Let $G$ %$G \in \cat{G}$ 
be an object in $\cat{G}$. Two monics \monorar{x}{X}{G} and \monorar{y}{Y}{G} are {\em equivalent}, $x\simeq_G y$, if  %A class of monomorphisms $M_G\subset\GG_\monoind/G$ % \inlinemonoarrow{X}{x}{G} $ 
%is called \emph{abstract subobject} of $G$ when for any two members $\monoarrow{X}{x}{G}, \monoarrow{Y}{y}{G} \in M_G$, %[\inlinemonoarrow{X}{x}{G}]$ and $ \in [\inlinemonoarrow{X}{x}{G}]$ in $[\inlinemonoarrow{X}{x}{G}]$ 
there exists an isomorphism $\arrow{X}{i}{Y}$ such that the triangle  commutes, $\compose{i}{y} = x$. An $\simeq_G$-equivalence class is called an {\em (abstract) subobject} of $G$. Thus, any monic \monorar{x}{X}{G} gives rise to a subobject [\monorar{x}{X}{G}].
%It is easy to see that if $x\simeq y$, then $\Img(x)=\Img(y)$ 
 %\monoarrow{X}{x}{G} is an element of $M_G$, we will call it a representative of the subobject and denote the latter by $[\monoarrow{X}{x}{G}]$  (thus $[\monoarrow{X}{x}{G}]=\monoarrow{Y}{y}{G})$ for any two equivalent  
 Among the members of the class $[\monorar{x}{X}{G}]$, there is a monomorphism $\monoarrow{H}{\subseteq}{G}$ whose domain $H$ consists only of elements which are also elements in $G$ 
 --- we call it {\em inclusion} and denote by $H \hookrightarrow G$. Thus, for any object $I\in \II$, we have subsetting $H(I)\subseteq G(I)$.  %$\incrar{x}{H}{G}$ 
%Thus, when working with a class of monomorphisms we will often choose this special inclusion morphism, denoted $\inlinemonoarrow{H}{}{G}$, as the representative of this class.\zd{May be rewritten shorter; I'll do it later}

\zd{the problem is that we need to prove that for any subobject $[\monorar{x}{X}{G}]$ there is an inclusion representing it. For this, we need the image factorization.}
\subsubsection{Images}
The third an final concept we are borrowing from set theory are \emph{images}.
Categorically, the are given by epi-mono factorizations.
Let $\arrow{H}{f}{G}$ be an arbitrary arrow in $\cat{G}$, because $\cat{G}$ has epi-mono factorizations $f$ is equal to the composite $\compose{e}{m}$ where $e$ is an epimorphism and $m$ is a monomorphism. 
The codomain $\image{f}$ object of $e$ (domain of $m$) is called the image and it is unique up to isomorphism, thus we can choose $m$ to be an inclusion morphism. \zd{but see my remark above!}
The situation is depicted in the following diagrams.
\[
\xymatrix{ 
	H \ar[rr]^f \ar@{->>}[dr]_{e} & & G \\
	& \image{f} \ar@{^{(}->}[ur]
}
\]
%\zd{Still I prefer $\rCover^e$ for epis, especially that here we deal with images, not epics as such (see Freyd-Scedrov)}

\subsubsection{Subobject lattices}
From the above it follows that for every object $G \in \cat{G}$, there exists a \emph{subobject lattice} denoted $\subobjlattice{G}$.
It is given by the subcategory $\subobjlattice{G} \subseteq \sliceCat{\cat{G}}{G}$ of the slice category whose objects are abstract subobjects, meets are given by pullbacks in $\cat{G}$, and joins are given by $\image{[\iota_H,\iota_K]}$ the image of the universal coproduct arrow for $H \xrightarrow{\iota_H} H+K \xleftarrow{\iota_K} K$ being the coproduct of the abstract subjects $H \in \subobjlattice{G}$ and $K \in \subobjlattice{G}$.
Furthermore, for a morphism $\arrow{H}{f}{G} \in \cat{G}$ we denote the pullback-functor (change of base) on the subject lattices of $G$ and $H$ by $\arrow{\subobjlattice{G}}{\pbfunctor{f}}{\subobjlattice{H}}$.
Note, that this functor has both a left (post-composition) adjoint $\arrow{\subobjlattice{H}}{\pbfunctorLeftAdjoint{f}}{\subobjlattice{G}}$ and a right (bundling) adjoint $\arrow{\subobjlattice{H}}{\pbfunctorRightAdjoint{f}}{\subobjlattice{G}}$.
%}
\zd{Shorter: Any topos is a regular category. Hence, we have adjunctions $\pbfunctorLeftAdjoint{f}\dashv\pbfunctor{f}\dashv\pbfunctorRightAdjoint{f}$ (see Freyd-Scedrov). For presheaf toposes, these adjunctions are given component-wise(?)}
} % END OF THE renewcommand for \II

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{figures/BasicUniverse}
	\caption{Semantical Universes: Overview}
	\label{fig;semanticalUniverses}
\end{figure}

==> sections/backgrounds/differentDiagramsCategory.tex <==
\begin{myrem}[Diagram Categories] \ \\
	\begin{equation}
	\label{eq:diagrams}
	\begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c}
	\xymatrix{
		X \ar[d]_{XX} \\
		X_*
	}
	&
	\xymatrix{
		I \ar@{>->}[r]^{IE} & E
	}
	&
	\xymatrix{ % new diag b  
		I \ar@{>->}[r]^{IE} 
		\ar[d]_{II} 
		\ar@{}[dr]|(.8){\Large \ulcorner} 
		& E
		\ar@{->}[d]^{EE} 
		\\
		I_* \ar@{>->}[r]^{IE_*} &E_*
	}
	&
	\xymatrix{
		I \ar@{>->}[rr]^{IE} \ar[dr]_{II} & & E \ar[dl]^{EE} \\
		& E_* &
	}
	\\
	\text{a) \parbox{2.5cm}{Arity (shape) of \normalArrow}}
	&\text{b) \parbox{2.5cm}{Arity (shape) of \mArrow}}
	& \text{c) \parbox{2.5cm}{Arity (shape) of \bSquare}} 
	& \text{d) \parbox{2.5cm}{Arity (shape) of \eTriangle}}
	\end{array}
	\end{equation}
The finite index categories in \eqref{diagrams} (identities and composition omitted) give rise to the diagram categories $\downarrowCat{\SS}, \monicarrowCat{\SS}, \msquarepoCat{\SS}$ and $\mtriangleCat{\SS}$ where $\SS = \skecatgp$ is the category of $\predsig$-sketches over $\GG$. 
The objects in $\monicarrowCat{\SS}$ are all monic arrows in $\SS$, the objects in $\mtriangleCat{\SS}$ are all commutative triangles in $\SS$ and the objects in $\msquarepoCat{\SS}$ are all pushout squares where the top and bottom are monics (called \emph{binding squares}).
We also define specific diagram subcategories $\pointedDownarrowCat{X}{\SS}, \msquareXCat{X}{\SS}$ and $\mtriangleXCat{X}{\SS}$ where the respective index is mapped to a fixed sketch $X \in \SS$. 
Furthermore, every arrow in $\bSquare$ gives rise to a functor between diagram categories, e.g. $\frar{\proj{IE}}{\msquarepoCat{\SS}}{\monicarrowCat{\SS}}$.
\end{myrem}

==> sections/backgrounds/overview-fromAct20.tex <==
\section{Background and Contributions} %Motivation: Why we need a view mechanism over generalized sketches}
%  \newcommand{\QQ}{\enma{\mathbf{Q}}}
  
 We discuss two main applications of the \fwk\ in SE in Sect.2.1-2, then discuss some mathematical aspects of the \fwk\ in Sect.2.3, and describe related work and contributions in Sect.2.4
   
\subsection{Views over sketches.} \label{sec:application1} 
Developing a complex software system normally requires working with multiple \emph{views} \cite{AtkinsonStollB2010} of the system: 
This is the only way to manage complexity and a cornerstone of system engineering, see \cite{FinkelsteinKramerNFG1992} for an early discussion and \cite{FeldmannKernschmidtWV2019,BruneliereBurgerCW2019,CicchettiCicozziP2019} for more recent reports and surveys. 
A view of a {\em source} artifact $S$ is, in general, not merely a part of $S$ or a projection of $S$, but typically involves some computation over $S$,  e.g. composing references, aggregating attributes by summing up their values etc, which extends $S$ with {\em derived} elements produced by some predefined operations (we will say {\em queries}) applied to $S$. Then a {\em view} can be defined as  a mapping $\frar{v}{V}{Q_v(S)}$ in a suitable category of software artifacts where the source $S$ and the view schema $V$ live, and  $Q_v$ is a query that provides an extension $Q_v(S)$ of source $S$ with derived elements required by the view. Note an important distinction from the ordinary Kleisli mappings defined for a given monad $\QQ$ or, equivalently, for a global mapping on objects, which only potentially exists and seems unnecessary abstract for software engineers not familiar with Haskell. In contrast, in our notion of view, each view mapping $v$ carries its own query 
 $Q_v$ and maps to its own {\em local} extension $Q_v(S)$ rather than to a unified but huge global extension $\QQ(S)$.  
 \begin{includeShort}
 A simple example in Appendix \ref{sec:viewExample} shows how it works, and also demonstrates the importance of constraints for the view mechanisms. Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
\end{includeShort} 
\begin{includeLong}
	A simple example in \sectref{viewExample}  shows how it works, and also demonstrates the importance of constraints for the view mechanisms. It is placed aside to save time for the first reading, but we encourage the reader to take a look there to obtain a notion of the MDE world and our motivation for this paper.  %Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
%\input{sections/appendix4act20}
\end{includeLong}

\subsection{Algebra for model management.}\label{sec:application2}
 In \emph{model management},  models are manipulated as holistic entities, and replacement the one-object-at-a-time approach (micromanagement) by one-model-at-a-time (macromanagement)  turned out very productive \cite{Bernstein2003,%}.
% The respective research domain is called \emph{model management} \cite{
FavreNguyen2005,%Diskin2009,
PaigeKolovosRMW2013%DiskinKokalyM2013
}. 
 \begin{wrapfigure}{r}{4cm}
 	\vspace{-2ex}
 	\centering
 	\includegraphics[width=\linewidth]{figures/modelMgmtsmall}
 	\caption{Model Management}
 	\label{fig:modelMgmt}
 	 \end{wrapfigure}
  %?????   model operations are inherently diagrammatic \cite{me-sle13,me-fase16}. 
  It requires considering high-level operations on models such as model slicing, transformation, merging, and synchronization, and composing them into complex workflows  \cite{Diskin-sle13}. 
  Fig.~\ref{fig:modelMgmt} shows a simple example in which two views of the same source are first matched, and then merged. One may think of this as taking the pullback and then the pushout, but in practice these ``pure'' categorical operations are often interwoven with some normalization procedures (and may require conflict resolution) so that even in this simple case the real workflow will be much richer. 
 %
\skeletalX{Importantly, models in SE are typically considered up to their auto-isomorphisms generated by permutations of OIDs (in the sense of OO programming)  which are irrelevant and normally not visible. It justifies making categories of models skeletal, which makes limits and colimits  deterministic algebraic operations. } 

Thus, for both the inter-model and the intra-model levels of reasoning, SE needs powerful and formally specified algebraic machinery for diagrammatic operations. On the other hand, it seems that even basic universal algebraic constructs (signature, term, parsing) have not been accurately specified for diagrammatic operations, especially when the latter are considered together with pre-and post-conditions and hence are interwoven with logic; in this sense, we are developing some basic universal algebra for diagrammatic operations. 

\subsection{Mathematical aspects}
\subsubsection{Why generalized graphs and generalized sketches} %, and categorical signatures}

As discussed above, categories hosting software models are categories of sketches. % and their models (in the mathematical sense). 
In general, a sketch is a graphical structure endowed with labelled diagrams (a.k.a. constraints); in the project, we consider a very general version of the notion: our 'graphs' are finitary presheaves, and our constraints of shape $G$ are any ``devices'' that classify mappings from $G$ as either valid or invalid. The generality of our graphs is caused by the great diversity and complexity of graphical structures used in SE  \cite{Kent2002}, and graphs used for behavioural and workflow  models can even be more complex. %Hence, we consider a very general notion of a graph as being a presheaf \frar{G}{\HH}{\setcat}  whose schema $\HH$ is any finite category. \footnote{In the long version, we consider an important requirement to \HH\ motivated by other parts of the project, but it is not needed for results described in the present paper.}
Similarly, constraints used in domain modelling (banking, e-commerce, automotive etc.) can be complex and very elementwise-oriented so that their representation in a standard categorical way via universal properties can be rather bulky and unwieldy (a detailed discussion can be found in \cite{DiskinWolter2008}, see also Appendix). Thus, we need  constraints and sketches of a very general nature that Michael Makkai called {\em generalized sketches} \cite{Makkai1997}.  %Diagrammatic constraints are an integral part of the domain and software modelling, and  important for specifying correct view mappings. Hence, we need to consider graphs endowed with constraints declared over them, \ie, graphical/diagrammatic theories or {\em ()generalized) sketches}. Thus, our category of artifacts and their mappings should be a category of sketches and sketch \mor s.
%
%\subsubsection{Signatures are categories}
%DEPENDENCIES ARE IMPORTANT ...... BLAH-BLAH
%\subsection{Mathematical issues}
\subsubsection{String diagrams do not work for diagram operations}
\newcommand{\propcat}{\enma{\catname{PROP}}}
%The objects in a PROP are natural numbers (arities) and arrows represent operations where domain and codomain denote in- and output arity. Being symmetric monoidal (sm) categories, $\catname{PROPs}$ can be  visualized with String Diagrams \cite{Selinger2011}, an intuitive yet formal graphical syntax.
For \propcat s, terms can be specified by string diagrams as shown in 
Fig.~\ref{fig:exSMC}, which depicts a ternary term $(x + y) * (x + z)$ built from two binary operations. % in string diagram notation, which is a ternary operation ($\in \catname{PROP}(3,1)$) where 
Note that reuse of the middle variable $y$  is shown explicitly with  $\nfont{Copy}$-operation (visualized via \includegraphics[width=1em]{figures/Copy}). This is possible as 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/StringDiagram}
	\caption{String diagram notation for ordinary algebraic terms}
	\label{fig:exSMC}
\end{figure}
%Unfortunately, we cannot use this machinery for diagram operations. The classical operations are \setcat-based and 
set $\{x, y, z\}$ is the coproduct of its elements $\{x\}\sqcup\{y\}\sqcup \{z\}$.
However,  diagram operations are graph-based,  %\footnote{Throughout this paper we will use the term ``graph'' in a more general sense, see Sect.~\PAST{Reminder to put the correct reference}}.
and a graph (while being a colimit of its elements) is not their coproduct!
\input{figures/insert-ex3pb}
Consider Fig.~\ref{fig:ex3pb} presenting a simple diagram chasing piece. % \} as used in many categorical proofs denoted in different visual syntaxes. 
Part (A) uses a typical categorical notation: the diagram presents a workflow consisting of two pullbacks taken in parallel over spans with one monic leg, followed by yet another pullback. Monic preservation by pullbacks is also shown. %In addition,  by naming conventions and respective symbols in the corners we show that some elements in the diagram are constructed via pullbacks, and via arrow decorations we specify some of the arrows to have special properties (being monic).
Part (B) makes the above explicit by using labels for constraint declarations (ovals) and operation applications (chevrons), and showing their scope. % make the stion elements in the diagram are explicated. 
Note that arrows going in and out of chevrons  show the workflow and what elements are constructed/derived (blue and dashed) rather than given. 
Part (C) is similar to Fig.~\ref{fig:exSMC} and highlights the workflow of the query by making the order of operation applications explicit, e.g. the pullback \nfont{c} depends on elements produced by the other two pullbacks.

Note several important differences with Fig.~\ref{fig:exSMC}. First, in discrete $\catname{PROP}$-setting, the elements produced by an operation have no further relationship with the input elements, while in the graph-based setting, there is an overlap between the input and the output, e.g. element $B$ in \figref{ex3pb}(B) is both in the input and the output of the pullback application \nfont{a}, and similarly for application \nfont{b} so that $B$ is also shared by \nfont{a}-output and \nfont{b}-output. Second, the workflow shown in \figref{ex3pb}(C) is a rather poor view of the actual workflow under the hood, which consists of several pushouts (POs): three POs are needed to produce graph $X'$ and yet another one to produce $X''$. Workflow arrows with hollow ends are, in fact, pairs, $(X,a)$, $(X,b)$ etc.,  while mappings that do the job, \eg, the one showing what part of graph $X$ is used as an input for \nfont{a{:}[pb]}, are not shown. %etc., and monics from $X$ to $X'$ to $X''$, are not shown. 
Thus, in contrast to \figref{exSMC}, diagram \figref{ex3pb}(C) is an incomplete specification of the story.  

\subsection{Related Work and Contributions}
%\zd{Phrase about the diversity of the pool of notions....}
By {\em logic} we refer to work on generalized sketches, and {\em algebra} refers to work on signatures of operation symbols, terms and algebras over them. 

\vspace{-0.25cm}
\subsubsection{Logic.}
Several authors noticed that Ehresmann's sketches can be applied to data modelling \cite{LellahiSpyratos1991,Piessens-tac95,JohnsonRosebrugh2002}. %,Diskin-adbis97}, 
%A majority of these application basically rely on the concept of a \emph{sketch}  introduced by Ehresmann, i.e. a graphical counterpart of a logical theory  (see \cite{Wells} for the history and  \cite{AdamekRosicky1994} for references about their equivalent expressiveness). %and classical Ehresmann's skecthes were employed in all works cited above besides those by D \cite{LellahiSpyratos1991,Piessens-,JohnsonRD-audb01}. 
%By sketch we refer the classical notion introduced by Ehresmann and promoted in \cite{BarrWells1990} and a more \emph{generalized} variant introduced by Makkai \cite{Makkai1997}).
However, these sketches are based on universal properties of the \corring\ (limit, colimit, powerobject) diagrams, which (as we discussed above) is a too restrictive setting for applications. %(see \cite{DiskinWolter2008} for a discussion). 
A suitable generalization of sketches by exactly this reason was proposed by Diskin \cite{Diskin-sketches96,Diskin1997}, and independently and even earlier, in a very  different context of an abstract approach to logic, by Makkai \cite{Makkai1997} (whose preprints had been circulating in early 90s). Makkai developed a coherent theory of generalized sketches and proved a fundamental result that any category of sketches is a presheaf topos. Hence, sketches in a signature $\PP_1$ can be considered graphs over which a new signature $\PP_2$ and hence a new category of $\PP_2$-sketches can be defined, and so on. In this way, Makkai specified categories with several layers of additional structure as sketches. In our project, we use a different approach in which all discrete signatures $\PP_i$ are integrated into one signature-category $\int_i\PP_i$, whose arrows describe  dependencies between predicate symbols extracted from arities (
\shortlong{details can be found in \cite[Sect.3]{THETR}}{see Sect. 4 for details}
	). \shortlong{In the TR we prove}{We prove} that Makkai's theorem can be extended for categorical signatures so that the slogan ``sketches are graph'' persists (see Th.~\ref{thm:genMakkai} for a precise formulation). 
%: given a presheaf topos of graphs $\GG=\setcat^\HH$ for some schema category \HH, and a set of predicate symbols \PP\ whose arities are \HH-graphs, \PP-sketches whose carriers are \HH-graphs can be considered presheaves on a special (collage) category 
Also, while traditionally sketches are defined in an {\em indexed} way as  families of sets of diagrams indexed by predicate symbols  (for the discrete signature case), or functors {\em from} the signature (for the categorical signature case \cite{DiskinWolter2008}), we define them in an equivalent {\em fibrational} way via a discrete opfibration functor {\em into} the signature: the fibrational definition is more compact and often simplifies technicalities.  

\begin{includeLong}
To give a detailed overview of what is done in the paper in comparison with other work, we need to distinguish between several notions of signatures and sketches. We call logic {\em basic} if signatures of predicate symbols are sets considered as discrete categories. We call it {\em advanced}, if signatures are categories whose arrows are dependencies between predicates; in addition, these arrows are required to go in one direction, which makes signature \cats\ {\em \hical} (a version of Lawvere's one-way categories). %Traditionally, sketches are defined in an indexed way as families of sets of diagrams indexed by symbols in the discrete signature case, and functors into \setcat\ for categorical signatures. We define them in an equivalent {\em fibrational} way via a discrete opfibration functor into the signature. 
There is also an important distinction between {\em -multi-}sketches that allow the same labelled diagram appear in a sketch for multiple times, and {\em mono-}sketches that disallow this. Finally, a partially de-categorificated approach (due to Makkai) is to consider signatures as layered sets so that each predicate in layer $(n+1)$ implicitly depends on all predicates in layer $n$. However, when arities of $(n+1)$-predicates are defined based on $n$-predicates, the actual dependencies appear on the stage. We call this approach {\em discrete \hical (dh)} and show that it is actually equivalent to the categorical one. In these terms, Table \ref{tab:contributionsLogic1} shows the previous work and contributions of the project. Our main results here are an extension of a fundamental Makkai's theorem (that multi-sketches are actually presheaves) for the case of categorical signatures with dependencies,  Th.~\ref{thm:genMakkai}, and  an equivalence of the two approaches to sketches: internally categorical (signatures are categories) and discrete \hical\ (a hierarchy of discrete signatures), Th.~\ref{thm:dh=f}. 
%Naively speaking the contribution of our work can be described as formalization of diagram chasing as e.g. in Fig.~\ref{fig:ex3pb}:
%We formally define diagram operations, diagram algebras and queries (= terms) and show elementary results known from classical algebra to hold in this setting:
%Queries extend to a functor $Q$, algebras are arrows $\frar{a}{Q(A)}{A}$ and there is (symmetric monoidal) Kleisli-Category w.r.t. $Q$, hence the latter also becomes a monad.
%The results are first presented in a discrete setting, i.e. without relations between operations, and then extended to a more general setting with relations between operations, which are needed for syntactical reasoning.
\begin{table}[]
	%\scriptsize
	\footnotesize
	\begin{tabular}{|l|l||l|l|l|}
		\hline
		\multicolumn{2}{|l|}{\multirow{2}{*}{\diagbox{Sketch Def.}{Setting}}} & \multirow{2}{*}{\parbox{2cm}{One-Layer (Basic Logic)}} 
		& \multicolumn{2}{l|}{\qquad Multi-Layer (Advanced Logic)}                          \\ \cline{4-5} 
		\multicolumn{2}{|l|}{}                  &                                          & Discrete Hierarchical         & \qquad Categorical~~                                \\ \hline \hline
		\multirow{2}{*}{Indexed}       & mono-sketches   & \multicolumn{2}{c|}{\multirow{2}{*}{Makkai \cite{Makkai1997}}}                             & Diskin \& Wolter \cite{DiskinWolter2008}                                     \\ \cline{2-2} \cline{5-5} 
		& multi-sketches  & \multicolumn{2}{c|}{}                      & 
		\quad ~~Sect.\,\ref{sec:advancedSketchLogicDefs}                              
		\\ \hline
		%\multirow{2}{*}{Fibrational}   & mono   
		\multicolumn{2}{|c||}{Fibrational}  %&
		& 
		\multirow{2}{*}{\parbox{2cm}{\qquad Sect.\, \ref{sec:basicLogic} \\ (Motivational)}} %\ref{sec:basicSketches}}         
		& \multirow{2}{*}{\qquad Sect.\,\ref{sec:discreteHierarchicalSketches}} 
		& \multirow{2}{*}{\qquad Sect.\,\ref{sec:advancedSketchLogicDefs}-\ref{sec:ske=gra}, Th.\ref{thm:genMakkai}} %\ref{sec:avancedSketchLogic}} 
		\\ [5pt]  
		%\cline{2-2} 
		\cline{4-5}
		%& 
		\multicolumn{2}{|c||}{(both mono \& multi)} 
		&                                         
		 &\multicolumn{2}{c|}{\strut Equivalence, Th.~\ref{thm:dh=f} }  %&                                            
		 \\ [5pt] \hline
		 %\\
	\end{tabular}

\medskip
	\caption{\strut Diagram Logic and Contributions}
\label{tab:contributionsLogic1}
\end{table}
\end{includeLong}

\subsubsection{Algebra.}
Diagram operation signatures and algebras were defined first in \cite{Diskin1997} and with some additional details in  \cite{Diskin-sketches96}, but no mathematical results were obtained. For the special case of operations over ordinary graphs, Wolter \etal\ \cite{WolterDiskinK2018} proved that any signature of such operations generates a monad (\ie, a global construct) over the category of graphs. The machinery of {\em local} Kleisli mappings explained informally was used in several papers of the first author, \eg,  \cite{Diskin-models10,Diskin-fase17}, and formalized as Kleisli mappings of a monad (\ie, globally) in \cite{Diskin-fase12}; we are not aware of an accurate formalization of Kleisli mappings considered locally as is done in our project,  nor of several other results reported in Sect. \ref{sec:diagramOps-disc-onelayer}. Specifically, we prove that a) sketches and local Kleisli mappings (views) between them form a symmetric monoidal category,  and b) the local Kleisli composition gives rise to a Kleisli triple and hence a  monad (as expected).  
Table~\ref{tab:contributionsAlgebra1} provides an overview of related work in this area and where to find our results in this paper.
\begin{includeLong}
\begin{table}[h]
	%\scriptsize
	\footnotesize
	\begin{tabular}{|l||p{4cm}|p{3.75cm}|}
		\hline
		\diagbox{Topic}{Setting} & Discrete                                                                                
		& \parbox{2cm}{Categorical \\ (Dependencies)} 
		\\ \hline\hline
		Signatures  and Algebras         & 
		\parbox{3.75cm}{Sect.\,\ref{sec:sigAndAlg}; \cite{WolterDiskinK2018}  (graph operations) }                   
		&  \multirow{5}{*}{Sect.\,\ref{sec:opsig-withDeps}, \ref{sec:opsig-dhVersion}}                 
		 \\ \cline{1-2}
		Multiqueries and Substitution   
		&  Sect.\,\ref{sec:mqueries-discrete}                                                                              
		&                      
		\\ \cline{1-2}
				Query Semantics   &  
				Sect.\,\ref{sec:algebraRevisited}                                                                              
				&                      
		\\ \cline{1-2}
		Complex Queries \& Composition &  Sect.\,\ref{sec:complexQueries}                                                                       
		&                     
		\\ \cline{1-2}
		Monads                          
		& \parbox{4cm}{Sect.\,\ref{sec:monadsDiscrete}; \cite{WolterDiskinK2018}  (graph term algebra adjunction)} &                  
		\\ \hline
	\end{tabular}

\medskip
	\caption{Diagram Algebra and Contributions}
	\label{tab:contributionsAlgebra1}
\end{table}
\input{sections/viewExample}
\input{sections/notationalConventions}
\end{includeLong}


\clearpage


\endinput
\zd{more refs would be useful} and then queries become complex diagram operations over graphical structures. \zd{In practice, queries and operations are formally defined on the level of code but rather dirty (informal, approximate) on the level of models -- hence, our interest to make it clean... } %Conceptual graphical artifacts play an important role in SE and are used to specify different aspects of the system under development \cite{Kent2002}.
%
%The above notion can be further abstracted into a Kleisli-arrow $\relationarrow{V}{v}{S}$, which was discovered and presented to the SE-community in \cite{me-fase12}.
\zd{Note also that we cannot use monads as ...... }

==> sections/backgrounds/overview.tex <==
\section{Diagram Logic and Algebra: Overview}\label{sec:basicLogic}

We will give three brief introductions:  to a sketch version of \diatic\ predicate logic in Sect. 3.1, to a \diatic\ algebra in Sect. 3.2, and to \diatic\ reasoning in Sect. 3.3
%\input{sections/viewExample}
%\input{sections/whyConstraintsIndexed}

\input{sections/genSketches-overview}

% ----- Now algebra

%\newcommand{\thisdiagrx}[1]{diagram \eqrefx{mQ-subst-abcDiag}{#1}}
\input{sections/diagOp-overview}
%\input{sections/opsig-discrete}

\input{sections/diagReasoning-overview}



%\input{sections/predske-syntax}
% the content of predske
%\renewcommand{\HH}{\enma{\mathbb{H}}}
%\input{sections/genGraphs}
%\input{sections/genSketches}
%% the short version of Advanced Logic
%\input{sections/advancedLogic-short}
%\input{sections/advancedLogic-long}


==> sections/bits-and-pieces-2.tex <==
	\section{Algebra pieces}
	\begin{mydef} ???
%%		\begin{figure}
%%		\centering
%		\begin{equation}\label{eq:alg-disc-presheaf}
%		\begin{array}{c@{\qquad}c}
%		\xymatrix{  % diag a)
%			&&&\operSet{B}
%			      \ar[ldd]^{\arfun_B}
%			      \ar[ld]_{\operSet{h}}
%			\\
%			\opsig 
%			\ar@/^1.5pc/[rrru]^{\semm{}_B}
%			\ar[rr]^{\semm{}_A} \ar[rrd]_{\arfun}
%			&&\operSet{A}\ar[d]^{\arfun_A}
%						\\
%			&&\maCat{\SS}&
%		}
%	\end{array}
%	\end{equation}
%%\end{figure}
	
%	\begin{figure}
%		\centering
	\begin{equation}\label{eq:alg-disc-fibr}
\begin{array}{c} %@{\qquad}c}
%	& % 2nd diag
			\xymatrix{
		% row 1
				\LDiagr{B}
				\ar@[blue]@/_5pc/@{-->}[dddd]_{\labell_B}  
				\ar@{-->}[rrr]^{\bind_B}%{\arfun'_B} 
				\ar[dr]^{\semm{}_B}
				%\ar@{-->}[dd]_{(\proj{IE})'} %{\olabel}
				&
				& 
				& \msquareXCat{\carr{B}}{\SS}  
				 \ar@/^5pc/@{->}[dddd]^{\proj{IE}}  
				 %\ar[dd]^{\proj{IE}}
				\ar@{->}[dl]^{\proj{E}} %{\olabel}
				\\  %row 2
				& %\pointedDownarrowCat{\carr{B}}{\SS} 
				\mtriangleXCat{\carr{B}}{\SS}
				 \ar[r]^(0.6){\proj{II}}
				&	\pointedDownarrowCat{\carr{B}}{\SS} 
				&
				%==
		\\ % row 3
		\LDiagr{A}  
		\ar@[red]@{->}[uu]^-{\textcolor{red}{h!}}
		%\ar@{->}[uu]_{!} %{\olabel}
		\ar@{-->}[rrr]^{\bind_A} %{\arfun'_A} %{\bind\quad}
		\ar[dr]^{\semm{}_A}
		\ar@{-->}[dd]|{\labell_A} %{\olabel}
		 &
		 & 
		 & \msquareXCat{\carr{A}}{\SS} 
		 	\ar@[red]@{->}[uu]^-{\textcolor{red}{h^\square}}
		 %\ar[uu]_{h^\square}
		 \ar[dd]^{\proj{IE}}
		 \ar@{->}[dl]_{\proj{II}} 
		 \\  %row 4
		& %\pointedDownarrowCat{\carr{A}}{\SS}  
			\mtriangleXCat{\carr{A}}{\SS} 
                  \ar[drr]_{\proj{IE}}				 
	 	          \ar[r]^(0.6){\proj{II}}
		\ar@[red]@{->}[uu]^-{\textcolor{red}{h^\triangle}}
		%\ar@[red][uu]^(0.5)^{h^\triangle}
		&\pointedDownarrowCat{\carr{A}}{\SS}
			\ar@[red]@{->}[uu]^-{\textcolor{red}{\_\comp h}}
		&
		\\   % row 5
		\opsig \ar[rrr]^\arfun 
		& 
		&
		&
		\monicarrowCat{\SS} %\ar[ul]^\cod 
	}
	\\
%	\text{a) Semantic definition (presheaf style)}  
%	& 
\text{Algebra moprhism --ver.1} 
%	\\
%	&\text{\zd{\parbox{5cm}{it should be like \eqref{skedef}
%				to expalin the diff between all facts and true facts}}
	\end{array}
	\end{equation}
%	\caption{An algebra for a discrete signature: The diagrams are in \setcat }
%	\label{fig:alg-disc}
%\end{figure}
%============
	\begin{equation}\label{eq:alg-disc-fibr-2}
\begin{array}{c} %@{\qquad}c}
%	& % 2nd diag
\xymatrix{
	% row 1
	\LDiagr{B}
	\ar@[blue]@/_5pc/@{-->}[dddd]_{\labell_B}  
	\ar@{-->}[rrr]^{\arfun'_B} 
	\ar[dr]^{\semm{}_B}
	%\ar@{-->}[dd]_{(\proj{IE})'} %{\olabel}
	&
	& 
	& \msquareXCat{\carr{B}}{\SS}  
	\ar@/^5pc/@{->}[dddd]^{\proj{IE}}  
	%\ar[dd]^{\proj{IE}}
	\ar@{->}[dl]^{\proj{E}} %{\olabel}
	\\  %row 2
	& \pointedDownarrowCat{\carr{B}}{\SS} 
	\ar[r]^(0.7){\dom_{\carr{B}}}
	&\SS
	&
	%==
	\\ % row 3
	\LDiagr{A}  
	\ar@{->}[uu]_{!} %{\olabel}
	\ar@{-->}[rrr]^{\arfun'_A} %{\bind\quad}
	\ar[dr]^{\semm{}_A}
	\ar@{-->}[dd]|{\labell_A} %{\olabel}
	&
	& 
	& \msquareXCat{\carr{A}}{\SS} 
	\ar[uu]_{h^\square}
	\ar[dd]^{\proj{IE}}
	\ar@{->}[dl]^{\proj{E}} %{\olabel}
	\\  %row 4
	& \pointedDownarrowCat{\carr{A}}{\SS}  
	\ar@{->}[uu]^-{\_\comp h}
	%\ar[uu]^(0.5){\_\comp h}
	\ar[r]^(0.7){\dom_{\carr{A}}}
	&\SS
	&
	\\   % row 5
	\opsig \ar[rrr]^\arfun 
	& 
	&
	&
	\monicarrowCat{\SS} \ar[ul]^\cod 
}
\\
%	\text{a) Semantic definition (presheaf style)}  
%	& 
\text{Algebra \mor\- ver.2 (equiv.)} 
%	\\
%	&\text{\zd{\parbox{5cm}{it should be like \eqref{skedef}
%				to expalin the diff between all facts and true facts}}
\end{array}
\end{equation}
%	\caption{An algebra for a discrete signature: The diagrams are in \setcat }
%	\label{fig:alg-disc}
%\end{figure}


		
		The above is a presheaf-style definition. Its {\em fibrational} counterpart is the following definition. An {\em algebra} $A$ is given by 
		
		a) its {\em carrier} sketch  $\carr{A}\in \SS$, which gives rise to a pullback square shown in the left part of \eqrefx{alg-disc}{b}. Its apex is the set of all correctly labelled binding diagrams over \carr{A}.
		
		b) a mapping $\semm{}_A$ as shown by the curved arrow such that the outer rectangle commutes. 
		
		It is easy to see that the diagram \eqrefx{alg-disc}{b} is just a rephrasing of \eqrefx{alg-disc}{a} in the monadic-style manner with $LDiagr(A)$ playing the role of a monad.  
%and a span of functions  $(\olabel, \bind)$ (whose apex is a set  \iConstr{A} of {\em indexes}) such that diagram \eqrefx{predsigdisc}{b} commutes. For an index $i\in\iConstr{A}$, the pair $(\opvar,d)$ with $\opvar=\olabel(i)$ and \drar{d=\bind(i)}{\opvar^\arfun}{\id_{A}} is a labelled diagram that we interpret as an instance of relation $\semm{\opvar}\eqdef\comprcolon{\bind(i)}{i\in\olabel^{-1}(\opvar)}\subset \arrowCatExp{\SS}(\opvar^\arfun,\id_A) $. To ensure this relation is a totally defined operation, we require that for any \frar{b}{I_\opvar}{A} there is at least one $i_b$ such that $\hdom(\bind(i_b))=b$, and if $j_b$ is yet another such index, then $\hcod(\bind(i_b))=\hcod(\bind(j_b))$. Finally, we require function \olabel\ to be surjective so that any operation symbol is interpreted over $A$. 
\qed
\end{mydef}
%It is easy to see that if the pair $(\olabel, \bind)$ is jointly monic in \setcat, then definition (b) is equivalent to definition (a). 
\zd{\em\bf If \opsig\ is a signature with pre- but without post-condition dependencies (\ie, category $\opsigEE$ is derived from $\opsigIE$ and thus not needed in the definition), then by considering diagram \eqrefx{alg-disc}{b} in \catcat\ rather than  \setcat\ we obtain diagrammatic algebras for signatures with only pre-dependencies. }

\subsection{===========}
===

\subsection{Example of a query}\label{queryexample}

Consider again the example depicted in Figure~\ref{fig:runningExample} and this time especially at sub figure \ref{fig:univPBProp:2}.
It makes the application of the three pullback operations (shown as chevrons) including their in- and output (shown as arrows) explicit.
Furthermore, we visually distinguish elements that are given (colored black) and those computed by operations (colored blue).
A straightforward way of formalizing this concept is by utilizing existing sketch machinery.

\subsection{intro piece for complex q}

We will begin with an example showing what a query is and how queries are often encoded (\sectref{queryexample}). Then we will formalize queries as {\em graphs with diagram operations (DO-graphs {\em in short})}.  We will first consider atomic (or elementary) queries and then proceed to complex queries/DO-graphs. For the latter, we will give two formalizations: the first is data-centric, in which queries are encoded as sketches (similarly to encoding equational theories and algebras by Horn predicate logic ), and the second is workflow-centric, in which a query is seen as a workflow (similarly to seeing terms as abstract syntax trees)

\subsubsection{Playing with signatures as fibrations}

see text below the endinput
\endinput
\zd{
	(A) Long ago I played with some abstract spec of sketches but now I know cat patterns better, and found interesting things. 
	\\
	{\bf Def.} A {\em morphism (map)} of predicate signatures is a functor commuting with arities. In other words, the category of pred signatures \psigcat\ is the slice category $\catCat/\GG$. 
	\\
	Now we redefine a sketch map as a triple \frar{f=(\abs{f},\psigfun{f},\constrfun{f})}{S}{S'} where $\abs{f}$ as above, \frar{\psigfun{f}}{\predsig}{\predsig'} a signature map, and \constrfun{f} is as above but now we require  $\compose{\constrfun{f}}{\labell'}=\compose{\labell}{\psigfun{f}}$ (\ie, the square rather than the triangle commutes).  This gives us a \caty\ \skecat\ equipped with two functors, \ie, a span in \catCat:
	\begin{equation}\label{eq:fibspan}
		\psigcat\lTo^{sig} \skecat\rTo^{\abs{\_}}\GG
	\end{equation}
	%	\frar{sig}{\skecat}{\psigcat} \mbox { and  } \frar{\abs{\_}}{\skecat}{\GG}.$$ 
	The left leg is a (split) fibration, whose lifts are vertical wrt. the second functor (\ie, are carrier identities). Dually, the right functor is a (split) opfibration, whose lifts are vertical wrt. $\abs{\_}$ (signature identities). (This nice correspondence could be called {\em orthogonality}. Moreover, most probably, the span should satisfy one more condition (a version of Beck-Chevalley):
	%	\begin{equation}
	~~for any sketch  $S\in\abs{\skecat}$  with signature $\predsig=sig.S$ and carrier $G=\abs{S}$,  and arrows \frar{u}{\bullet}{\predsig}, \frar{v}{G}{\bullet}, 
	there is a unique isomorphism 
	\begin{equation}\label{eq:BC}
		S.u^*.v_* \cong S.v_*.u^*
	\end{equation}
	Then it will be a gadget called {\em Street fibration}. This gadget under the name {\em fibred span} is defined by Jacobs in his book (Def. 9.1.5 on p.514) but his condition (b) seems to be not the same as the Beck-Chevalley above; and Jacob's formulation is awkward, so, let's use \eqref{BC}. 
	\\
	The span representation \eqref{fibspan} is a sort of a proper general view of logical theories: each of them (\ie a sketch) must have a) a signature and b) a carrier object (of variables) providing connectivity, which play dual roles (fibration and opfibration) for theory maps -- I think that this general philosophy should be more or less explicit in Jacobs book. Jacobs also shows a version of Grothendieck: any fibred span is equivalent to a functor
	\begin{equation}\label{eq:fibgroth}
		\frar{\skefun}{\psigcat^{op}\times\GG}{\catCat}
	\end{equation}
	so that \skecat\ in \eqref{fibspan} is $\int \skefun$. We should have a similar fibred span description of diagram algebra, but for algebra it should be something richer.
}

\zd{(B) Another useful description of sketches is this. Any sketch $S$ can be see as a predicate symbol with arity $\abs{S}$. % and the respective dependencies from $S$ to \predsig. 
	Then the category $\skecat(\predsig)$ can be seen as a big signature whose arrows are sketch morphisms. We thus have a functor \frar{\skecat}{\psigcat}{\psigcat}. I proved (long ago) that this functor is a monad over \psigcat.
}

\begin{figure}
	\centering
	\includegraphics[width=0.75\linewidth]{figures/kleisliCat-1-pic.jpeg}
	\caption{View composition 1}
	\label{fig:kleislicat-1}
\end{figure}
\begin{mythm}[View composition]
	Views can be associatively composed and make a category
\end{mythm}
the proof should go along the lines of \figref{kleislicat-2}.

\begin{figure}
	\centering
	\includegraphics[width=0.75\linewidth]{figures/kleisliCat-2-pic.jpeg}
	\caption{View composition 2}
	\label{fig:kleislicat-2}
\end{figure}

\subsection{===========}
\begin{mydef}[Diagram Algebra Morphism]
	Given two multialgebras $A, A'$, their {\em \mor}  \frar{f}{A}{A'} is a pair of mappings \frar{\carr{f}}{\carr{A}}{\carr{A'}} and \frar{f_{\indd}}{\iConstr{A}}{\iConstr{A'}} such that
	\zd{to be completed to subsume the def below} 
	
	%$\find\comp\plabel' =\plabel$ and $\find\comp\bind'=\bind\comp(\GG/\carr{f})$ with \frar{\GG/\carr{f}}{\GG/\carr{A}}{\GG/\carr{A'}} defined by postcomposition with \carr{f}. Thus, a multimodel \mor\ maps true facts about $A$ into true facts about $A'$.
	
	Let $\operationSig$ be a operation signature and $A$ and $B$ be two $\opsig$-algebras.
	An algebra morphism $\arrow{A}{f}{B}$ is given by a sketch morphism $\arrow{\carrier{A}}{\carrier{f}}{\carrier{B}}$ obeying 
	\begin{equation}
		\label{eq:diagAlgebraMoprhism}
		\opInterpret{\opVar}{B}_{IE}(\compose{b}{\carrier{f}}) = \compose{\opInterpret{\opVar}{A}_E(b)}{\carrier{f}}
	\end{equation}
	for all $b : \inputArity{\opVar} \to \carrier{A}$. Diagrammatically:
	\[
	\xymatrix{
		I_\opvar \ar@{>->}[rr]^{IE_\opvar} \ar[dr]_b \ar@/_/[ddr]_{\compose{b}{\carrier{f}}} & & E_\opvar \ar[dl]^{\opInterpret{\opVar}{A}_{IE}(b)} \ar@/^/[ddl]^{\opInterpret{\opVar}{B}_{IE}(\compose{b}{\carrier{f}})} \\
		& \carrier{A}  \ar[d]^{\carrier{f}} & \\
		& \carrier{B} &
	}
	\]
\end{mydef}
\begin{mylem}[Algebra category]
	All $\opsig$-algebras and their morphisms form a category $\GG||\predsig||\opsig$ supplied with a forgetful functor \frar{\nfont{alg2ske}}{\GG||\predsig||\opsig}{\skecatgpo}.
\end{mylem}
\begin{proof}\zd{to be revised}
	Follows immediately from the fact that $\skecatgp$ is a category and the identity in Eq.~\ref{eq:diagAlgebraMoprhism} is transitive.
\end{proof}
\begin{myexa}[Universal algebra cont'd]
	Hence, categories ... and  ..... are isomorphic. Thus, diagram algebra subsumes universal algebra.
\end{myexa}
%While \defref{opsig} defines syntax of graph operations, their semantics is given by the notion of a \emph{diagram algebra}.
%\begin{mydef}{diagOpSemantics}{Diagram Algebra}
%Let $\operationSig$ be an operation signature over predicate signature \predsig.
%An $\operationSig$-algebra is a pair $A = (\carr{A}, {\semm{\_}}^A)$ that comprises a \emph{carrier} sketch $\carr{A} \in \SS\eqdef \skecatgp$ and for each operation symbol $\opvar$, its  {interpretation} $\semm{\opvar}^{A}$ as a {\em diagrammatic operation over $A$}, \ie, a mapping 
%%$$
%%\frar{\opInterpret{\opvar}{A}_{IO}}{\homsetXA{I_\opvar}}{\homsetXA{O_\opvar}}%{\carrier{A}^{O_\opvar}} 
%%$$
%%such that the following diagram commutes for any \frar{b}{\inputArity{\opVar}}{\carrier{A}}:
%%\begin{equation}\label{eq:algviaE1}
%%\xymatrix{
%%	& K_\opvar \ar@{>->}[dl]_{KI_\opvar} \ar@{>->}[dr]^{KO_\opvar} \ar@{}[dd]|{}  & \\
%%	I_\opvar \ar@{>->}[dr]_b & & O_\opvar  \ar@{>->}[dl]^{\opInterpret{\opvar}{A}_{IO}(b)}\\
%%	& \carrier{A}&
%%}
%%\end{equation}
%%\end{mydef}
%%
%%
%%It is easy to see that because the square $\arfun(\omega)$ is a pushout, the data above determines a unique mapping 
%$$
%\frar{\opInterpret{\opvar}{A}}{\SS(I_\opvar,\carr{A})}{\SS(E_\opvar,\carr{A})}
%$$
%such that the following diagram commutes for any binding \frar{b}{I_\opvar}{\carr{A}} 
%\begin{equation}\label{eq:algviaE2}
%%\[
%\xymatrix{
%I_\opvar \ar@{>->}[rr]^{IE_\opvar} \ar[dr]_b & & E_\opvar \ar[dl]^{\opInterpret{\opVar}{A}(b)} \\
%& \carrier{A} 
%}
%%\]
%\end{equation}
%%Below we will mainly work with the interpretation $\semm{\_}^A_{IE}$ rather than $\semm{\_}^A_{IO}$ and normally omit the subscript $IE$. 
%
%W.l.o.g., we let the arity functor $\arfun$ map every monomorphism in $\MonoSquare$ to an inclusion in $\skecatgp$ since it simplifies notation. \zd{hm, probably, a monic seen as an equiv. class can well be identified with inclusion.}
%\renewcommand\opInterpret[]


==> sections/complexConstr-i-Sketches.tex <==
\subsection{Complex constraints and sketches} %, theories, and sketches} %, and extended signatures}
\zd{\Large this is a very long, old and too detailed and messily written version. all that I really need is the notion of sketches and validity of an instance over a sketch} 

\subsubsection{How it is done in the universal FOL (UFOL) ...} In FOL, if $P$ is, say, a ternary predicate, we build atomic formulas by a) fixing some set of variables $Var=\{v_1, v_2, ..\}$ (not necessarily infinite), and b) constructing formulas $P(v_1, v_2, v_2)$, $P(v_2,v_1,v_3)$ etc. Each such a formula is  actually a pair $(P,\bmap)$ where \frar{\bmap}{\{\bullet_1,\bullet_2, \bullet_3\}}{Var} is a {\em binding} mapping from the set of $P$'s placeholders (that can be seen as $P$'s arity shape $S_P$) into the set of variables. In the diagrammatic logic, such a binding mapping would be called a diagram in $Var$ of shape $S_P=\{\bullet_1,\bullet_2, \bullet_3\}$. 

Complex formulas are expressions built from atomic diagrams with logical connectives, \eg, 
$P(v_1,v_2,v_2)\vee Q(v_2,v_3)$ or $P(v_1,v_2,v_2)\wedge Q(v_2,v_3) \Rightarrow P(v_1,v_2,v_3)$.
As explained in \cite{jacobs-catLogicBook99}, it is important to keep with a complex formula $\phi$ a set $V$ of variables 
%(called $\phi$'s {\em context}) 
that may be used in the formula; this set is called formula's {\em context}, \eg, 
\begin{equation}\label{eq:ske-string-based-example}
\{v_1,v_2,v_3, v_4\}  \,|\; P(v_1,v_2,v_2)\wedge Q(v_2,v_3) \Rightarrow P(v_1,v_2,v_3)
\end{equation}
(note that variables actually used in the formula may form a proper subset of the context). Thus, in an accurate setting, a {\em formula} is a pair $\phi=(V_\phi, \skelogicX{\phi})$ of a set of variables $V_\phi$  (called $\phi$'s context) and a logical formula $\skelogicX{\phi}$ that uses variables from $V_\phi$ (not necessarily all of them). A {\em theory} is given by a (global) set of variables  $Var$ and a set  $\Phi$ of formulas whose contexts are subsets of $Var$, \ie, $V_\phi\subset Var$ for all $\phi\in\Phi$. % \compr{\phi}{V_\phi\subset Var}

\subsubsection{... and diagrammatically with \cdecla s}
We fix a base category with pullbacks \GG\ and a constraint signature \csig\ over \GG. Similarly to the above, in order to build a complex diagrammatic constraint $\phi$ from, say, constraints $c$ and $c'$, we fix its shape (context) $S_\phi\in\Ob\GG$, build atomic statements $(c,\bmap)$ and $(c',\bmap')$ with binding mappings \frar{\bmap}{G_c}{S_\phi}, \frar{\bmap'}{S_{c'}}{S_\phi}, and form their logical combinations with connectives $\wedge, \vee, \Rightarrow, \neg$, \eg, $(c,\bmap)\wedge(c',\bmap')$ or $(c,\bmap)\Rightarrow(c',\bmap')$. A preinstance \frar{t}{X}{S_\phi} {\em satisfies} $(c,\bmap)\wedge(c',\bmap')$ if we have both $t_\bmap\models c$ and $t_{\bmap'}\models c'$, where instances \frar{t_\bmap}{X_b}{G_c}, \frar{t_{\bmap'}}{X_{\bmap'}}{S_{c'}} are obtained by pulling back instance $t$ along $\bmap$ and, resp., $\bmap'$ as shown in diagram \cref{eqdiag: twoPBs}. Similarly, $t \models (c,\bmap)\vee(c',\bmap')$ if $t_\bmap\models c$ or $t_{\bmap'}\models c'$; $t\models (c,\bmap) \Rightarrow (c',\bmap')$ if either $t_\bmap\notin\semm{c}$ or $t_{\bmap'}\in\semm{c'}$; and $t\models \neg(c,\bmap)$ if $t_\bmap\notin\semm{c}$ (so that implication $\__1\Rightarrow\__2$ is nothing but $\neg\__1\vee\__2$ ).  
\begin{equation}\label{eqdiag: twoPBs}
\begin{tikzcd}
\dernode{X}_{\bmap}\ar[r, derived, "\bar \bmap "]	\ar[d, derived, "t_{\bmap}" ' ]
% [pb] version 
\ar[rd, "\text{[pb]}", phantom, near start] %, very near start]
% corner version works badly 
%\ar[rd, "\lrcorner", phantom, pos=0.01]
& X \ar[r, <-, derived, "\bar \bmap'"]  \ar[d,"t"] & \dernode{X}_{\bmap'}\ar[d, derived, "t_{\bmap'}"]
\ar[ld, "\text{[pb]}", phantom, near start]
\\
S_{c} \ar[r,"\bmap "]	 & S_\phi \ar[r, <-, "\bmap' "]  & S_{c'}
\end{tikzcd}
\end{equation}
In the \DCL\ context, a binding mapping \frar{\bmap}{\arityX{c}}{\arityX{c'}} would be called a diagram in \arityX{\phi} of shape \arityX{c}, and a pair $(c,\bmap)$ a {\em labelled diagram}. Such pairs are also called {\em \cdecla s}. We will often write a constraint declaration $(c,\bmap)$ as $c(\bmap)$ to refer to the parallelism with string-based formulas like $P(v_1,v_2,v_1)$. 
\begin{warn}[Notational \& terminological synonyms and homonyms]\hspace{5cm}
%\renewcommand{\item}{--} %{\newline}

\begin{itemize}%[keyvals]
\item Term 'formula' is used for both $\phi$ and $\skelogicX{\phi}$
\item Term 'constraint' will sometimes refer to 'constraint declarations', \ie, pairs $(c,\bmap)$
\item \Cdecla s $(c,\bmap)$ will often be written as $c(\bmap)$ similarly to string-based logics
\end{itemize}
\end{warn}

\myendinputX{a big and messy piece from the old version of the Nov 2022 paper on constraints }

\begin{example}[Complex constraints]\label{ex:complex-constr1}
The upper row in \cref{tab:signComplexConj} specifies a constraint that requires spans $p$ and $q$ to be mutually inverse: it is a conjunction of the four atomic constraints specified in the rightmost column %
\footnote{The specification is not too elegant as we need to include into the arity shape two loops and declare them to be identity spans. A better solution would be to require graph \spansetcat\ to be reflexive upfront (\ie, to make it an algebra with operation \frar{\id}{\Arrow}{\Node} where \Arrow,\Node\ are vertices in the \GG's metaschema \II), but we do not use diagram algebras in this paper and thus need to include identities (and arrow composition) into our constraints explicitly.
%\endinput
\zd{(We also omit the requirement that in graph \spansetcat\ identity loops are unique for each node; we will return to this discussion later in \cref{sec:?})}
}
In this specification, we employ the fact that arrows in the arity shapes of all constraints involved are enumerated, and thus the corresponding list of $S_\phi$'s arrows uniquely determines a binding map, \eg,  the list $(p,q,e)$ specifies binding map \frar{\bmap}{S_{[\subseteq]}} {S_\mathrm{[inverse]}}  that maps $r_1$ to $p$, $r_2$ to $q$ and $r_3$ to $e$ (which is a correct graph \mor); hence, $[\subseteq](p,q,e)$ is a correct constraint declaration/labelled diagram in $S_\mathrm{[inverse]}$. The three other terms in formula \skelogictxt{[inverse]} are labelled diagrams too whose shapes can be found in \cref{tab:sign}. 

The second row specifies another complex constraint \bndRsrcX{1} (read it as [boundedResources]$_1$), whose carrier graph consists of six elements with suggestive names, and the logical part is conjunction of three constraint declarations (for the first term, its binding map sends $r_1$ to $\owns_1$ and $r_2$ to $\owns_2$). 
\qed\end{example}
\zd{\sc Merge (and shuffle two tables and two examples to make them one table and one example!!! )} 
\begin{example}[complex constraints] \label{ex:complex-constr2}
The first row in \cref{tab:signComplexImpl} states that if two spans are mutually inverse (as defined in \cref{tab:signComplexConj}), then each of them must be a partial (single-valued) function. Note that this constraint essentially differs from constraint [inverse] in that the latter only holds for some but not for all instances, whereas constraint [inv2inj] holds for all instances (and thus is a valid axiom of the universe \spansetcat). We then write $\models \text{inv2inj}$. This universality of constraint [inv2inj] is not anyhow captured in our formalism so far, and we will address the issue later by adding to the formalism a new type of constraints. 

The second row presents another resource constraint \bndRsrcX{2} of the same arity shape as \bndRsrcX{1}  in  \cref{tab:signComplexConj}  but with a different  (more intelligent) semantics, which  limits Owners' resources in the following way: for an instance $t$ over $S_{\bndRsrcX{2}}$, if an Owner  $x\in\Owner^t$ owns some resource units from either set $\Resr_1^t$ or set $\Resr_2^t$, then $x$ is not allowed to own more than one resource unit from set $\Resr_3^t$ while there are no limits on $\Resr_3$ if neither of resources $\Resr_{1,2}$ is owned, whereas constraint \bndRsrcX{1} limits $\owns_3$ unconditionally.  
\qed \end{example}
% -- leftUnit example]
%For another  example, to specify that id-loops are left units of composition for the signature in \cref{tab:sign}, we build the  implicational diagrammatic constraint [leftUnit] specified in the second row of \cref{tab:signComplex}  where  the binding mapping $b,b', b''$ are defined as follows. Note that formula [leftUnit] does not actually constrain.... 
%
%\endinput -------------
%
%\clearpagezd
\input{sections/tab-sig2}
\input{sections/tab-sig3}
%


%In this way we can enrich an original constraint signature with complex constraints. 


% -->>>  outtdated
%%\subsubsection{Complex constraints: Beyond conjunction}
% 
% A major deficiency of simple sketches as above is that the only logical connective it uses is conjunction. However, this deficiency can be fixed in the following straightforward way.  
% 
% % We can treat disjunction in a similar way:  $t \models (c,\bmap)\vee(c',\bmap')$ if $t_\bmap\models c$ or $t_{\bmap'}\models c'$. 
% Disjunction is obvious: \eg, in the situation of diagram \cref{eqdiag: twoPBs}, we define $t \models (c,\bmap)\vee(c',\bmap')$ if $t_\bmap\models c$ or $t_{\bmap'}\models c'$. 
% % 
% We also have negation. First, for each symbol $c\in\csig$ we form its negated counterpart  $\neg c$ with $S_{\neg c}=G_c$ and $t\in\semm{\neg c}$ iff $t\notin\semm{c}$ Then for a declaration $(c,\bmap)$ over some $S$, we state  $t\models\neg (c,\bmap)$ iff $t_\bmap\models \neg c$. Note that $\semm{\neg\neg c}=\semm{\neg c}$ as in Boolean logic.  Also following the latter, implication is defined via negation:  
% $t\models (c,\bmap)\Rightarrow(c',\bmap')$ if either $t_\bmap\models \neg c$ or $t_{\bmap'}\models c'$. 
%%Thus, as is typical for Boolean logic, implication is a derived connective: $\__1\Rightarrow \__2$ is considered as abbreviation of $\neg\__1\vee\__2$.
% %
%%\input{sections4notes/tab-sig3}
%%
% %\cref{tab:signComplexImpl} presents two simple examples. 
Formalization of these examples is straightforward. {First, for each symbol $c\in\csig$, we can form its negated counterpart  $\neg c$ with $S_{\neg c}=G_c$ and set $t\in\semm{\neg c}$ iff $t\notin\semm{c}$ Then for a declaration $(c,\bmap)$ over some $S$, we state  $t\models\neg (c,\bmap)$ iff $t\models (\neg c,\bmap)$, which is equivalent to $t_\bmap\notin\semm{c}$ as we formulated it above. Note that usual Boolean logic identities hold: $\semm{\neg\neg c}=\semm{c}$ and implication is defined via negation:  
$t\models (c,\bmap)\Rightarrow(c',\bmap')$ if either $t_\bmap\models \neg c$ or $t_{\bmap'}\models c'$.}.
%Thus, as is typical for Boolean logic, implication is a derived connective: $\__1\Rightarrow \__2$ is considered as abbreviation of $\neg\__1\vee\__2$.
\begin{defN}
A {\em complex constraint (diagrammatic formula)}  is a pair $\phi=(S_\phi, \skelogicX{\phi})$ of a graph $S_\phi\in\Ob\GG$ called the {\em carrier (context)} and a Boolean term 
$\skelogicX{\phi}\in Fr(\csig/S_\phi)$, where $Fr(\csig/S_\phi)$ is the free Boolean algebra generated by class %$\csig/S_\phi$
\[ \csig/S_\phi := %\text{ denotes class } 
\compr{(c, \bmap)}{c\in\csig \text{ and }\bmap\in\GG(G_c, S_\phi) }.\]
We will write $(c,\bmap) \in  \carrskelogX{\phi}$ for a subterm $(c,\bmap)$ of this term (\eg, formula [inv2inj] is a term conssting of three subterms). 
\end{defN}
\begin{constrN}[Extended signature]\label{con:extended-sig}
Given a formula $\phi$, any preinstance \frar{t}{X}{S_\phi} provides a Boolean evaluation $\ev{t}(c,\bmap)\in \{0,1\}$ for each subterm in \carrskelogX{\phi}: $\ev{t}(c,\bmap)=1$ iff $t_\bmap\in\semm{c}$, where $t_\bmap$ is produced by pullback as shown in \cref{eqdiag: twoPBs}. As $Fr(\csig/S_\phi)$ is freely generated, evaluation \ev{t} is uniquely extended to the entire term \skelogicX{\phi} and 
%all its elements and specifically for term \skelogicX{\phi}; thus, 
we obtain a uniquely determined value $\ev{t}(\phi)\in\{0,1\}$. We define $t\models\phi$ iff $\ev{t}(\phi)=1$. This makes any formula $\phi$ a constraint with arity shape $S_\phi$ and semantics $\checkfun_\phi(t)=1$ iff $\ev{t}(\phi)=1$. In this way, a(n interpreted) constraint signature \csig\ gives rise to a(n interpreted) signature \csigplus\ of all complex constraints (formulas) built over \csig\ as explained above. 

There is an obvious embedding $\csig\hookrightarrow \csigplus$ that sends an atomic constraint $c$ to formula $\phi(c)$, whose arity $S_{\phi(c)}=G_c$ 
%(or $S_{\phi(c)}\cong G_c$ via some isomorphism $i$ if we want to choose $S_{\phi(c)}$ in some predefined pools of graphs), 
and term $\skelogicX{\phi(c)}$ consists of the only subterm $ (c,\id[G_c])$. 
Obviously, $t\models \phi(c)$ iff $t\models c$ so that syntactically and semantically $\phi(c)$ is equivalent to $c$. 
% $\csigplus\superset\csig$. % in the following way. For a given $S\in\Ob\GG$, we form the set of all declarations $(c,\bmap)$ over $S$, which freely generates a Boolean algebra $\csigplus[S]$. Then we join the carrier sets of all these algebras into a class 
% $\csigplus=\bigcup_{S\in\Ob\GG} \csigplus[S]$ (which is a set iff \GG\ is small). \qed
\qed\end{constrN}
Now we can consider sketches over signature \csigplus, whose constraints are (possibly infinite) conjunctions of constraint declarations built form \csigplus, that is, diagram labels are Boolean combinations of elementary/atomic constraint declarations. 
\begin{defN}%[Complex sketches]
A {\em complex} sketch in signature \csig\ is an ordinary (generalized)  sketch in signature \csigplus.
\end{defN}
\begin{remark}[{\bf Application:Modularization and information hiding}]
Given a complex sketch $S$, binding mappings constituting complex constraints occurring into $S$  can be composed with binding mappings of diagrams in \carr{S}, which would flatten sketch  $S$ into a set of Boolean terms built from { atomic} \cdecla s in \carr{S}. However, the intermediate packaging provided by complex constraints may be useful (and sufficiently often very useful) in practice of software engineering (cf. classical ideas of information hiding \cite{parnas-infohide}). 
%From the viewpoint of a complex \csig-sketch, the difference between atomic constraints in \csig\ and complex constraints in $\csigplus\setminus\csig$ is invisible. This provides an additional layer of modularization and information  hiding, which is useful  in software engineering (\cite{parnas-infohide}). 
For example, suppose we have a sketch $S$ including a labelled diagram (\cdecla) labelled by \bndRsrcX{2}. We can re-implement constraint \bndRsrcX{2} in a more optimal way while keeping its shape and semantics intact, and thus nothing should be changed in $S$. Moreover, sometimes it makes sense to allow changes in semantics, \eg, we may want to weaken constraint \bndRsrcX{2} by reimplementing it with subterm $[0..2](\owns_3)$ instead of the subterm $[0..1](\owns_3)$ in its specification. Then for any instance $t$ over \bndRsrcX{2},  we have $t\models\bndRsrcX{2}^{\text{old}}$ implies $t\models\bndRsrcX{2}^{\text{new}}$ but not the other way round. Although semantics of sketch $S$ would change, its syntactical correctness is not violated as we do not allow changing the arity shape. Thus, it makes sense first to build complex Boolean constraints as needed and form signature \csigplus, and then build ordinary sketches over \csigplus. 
\end{remark}
%Generalized sketches as they were initially defined by Makkai \cite{makkai97} and Diskin \cite{me-sketchDef}, only consider conjunctions (perhaps, infinite) of atomic constraints, \ie,  conjunctions of pairs $(c,b)$ with \frar{b}{G_c}{S} a binding map into some object $S\in\Ob\GG$ called the sketch {\em carrier} (think of a data schema). 

%\endinput
These and similar other examples of conjunctive constraints (with, perhaps, infinite number of terms) are subsumed by the notion of a generalized sketch. 
%An accurate definition of (generalized) sketches is presented in \cref{sec:skeDef}

%The notion of sketch slightly generalizes the idea of the examples  by admitting infinite conjunctions. 
\subsection{Sketches as \DCL-theories}\label{sec:sketches}
The \DCL\ counterpart of the UFOL notion of a theory is the notion of a generalized sketch.   
\begin{defN}[Generalized sketches: Syntax (Makkai \cite{Makkai97-fullRef}, Diskin  \cite{Diskin-sketchesTR-1996,Diskin--bsl97}] \label{def:skeDef-syntax-mono}
Let \csigsyn\ be a fixed signature of uninterpreted constraints over base \GG. 
A {\em generalized (mono)sketch} $S$ in signature \csigsyn\ is given by  its {\em carrier} graph $\carr{S}\in\Ob\GG$, 
and a set %\skeindsetX{S} of {\em constraint indexes}, and
$D_S$ of diagrams in \carr{S} whose shapes are arity shapes of \csigsyn-constraints. That is, an element of $D_S$ is a pair $(c,\bmap)$ of a constraint $c\in\csigsyn$ and a binding map \frar{\bmap}{G_c}{\carr{S}} (recall that we also write such pairs as $c(\bmap)$). Diagrams $(c_i,\bmap_i)$ are called {\em constraint declarations} included into $S$. 

A {\em sketch \mor} %\frar{f}{S}{S'}
$S\rightarrow S'$  is given by a \GG-\mor\ \frar{f}{\carr{S}}{\carr{S'}} such that any constraint declaration $(c,\bmap)$ in $D_S$ is mapped into a \cdecla\ $(c,\bmap.\carr{f})$ in $D_{S'}$.
This gives rise to a category of all \csigsyn-sketches $\GG|\csigsyn$. 
\end{defN}
For example, two complex constraints in \cref{tab:signComplex} which only use conjunction are sketches in the signature specified by \cref{tab:sign}.  
\begin{defN}[Generalized sketches: Indexed and Fibred semantics (Diskin and Wolter,  \cite{Diskin-sketchesTR-1996,%Diskin--bsl97}\cite{
DiskinWolter-entcs08}]\label{def:skeDef-semantics}


b) Let \csigsyn\ is an  {\bf uninterpreted} signature. An {\em indexed semantics} for a \csigsyn-sketches is given by a chosen \csigsyn-sketch $U$ called {\em semantic universe}, and a \GG-\mor\ \frar{m}{\carr{S}}{\carr{U}} for a given sketch $S$ is called $S$'s {\em premodel}. A premodel is a {\em valid model} (and we write $m\models S$) if it gives rise to a correct \csigsyn-sketch \mor \frar{m}{S}{U}. We may thus say that choosing $U$ provides a semantic interpretation to  

Then for a \csigsyn-sketch $S=(\carr{S}, D_S)$,  (called a {\em premodel}) is a {\em valid} model if 

A {\em sketch instance} is an instance over the carrier, \frar{t}{X}{\carr{S}}, which satisfies all constraint declarations in $D_S$: $t_\bmap\models c$ for any $(c,\bmap)$ in $D_S$ (where $t_\bmap$ is the result of pullback specified in \cref{eqdiag: twoPBs}). Then we write $t\models S$.
\end{defN}


%In the language of generalized sketches (Makkai \cite{Makkai97-fullRef}, Diskin \cite{Diskin-sketches96,Diskin1997}, see \cref{def:skeDef-mono} below for an accurate formulation)), 
Now we may say that constraint [inverse] is a sketch in the signature given by \cref{tab:sign}, whose carrier is graph $S_\text{inverse}$ and the set of labelled diagrams consists of four constraint declarations (connected by $\wedge$) specified in the rightmost column.  Their conjunction in assumed by default in the sketch \fwk.  Similarly, constraint \bndRsrcX{1} is a  sketch with carrier specified in the middle column  %$S_{\mathrm[bndRsrc]_1}$ 
and two labelled diagrams. 
%
As yet another example, the premise of implication   \cref{eq:ske-string-based-example}    is also a sketch in $\GG=\setcat$ with carrier $V\in\Ob\setcat$ and two labelled diagrams $P(v_1,v_2,v_2)$ and  $Q(v_2, v_3)$ in the signature $\csig=\{P(\bullet_1,\bullet_2, \bullet_3),\,  Q(\bullet_1, \bullet_2) \}$. 
\begin{propo}[Change of base for sketch instances] Given a sketch \mor\ \frar{f}{S}{S'} and an instance $t\models S'$, the latter can be pulled back in \GG\ along \carr{f} into an $\carr{S'}$-instance $t_f$ and, moreover, $t_f\models S$.
\end{propo} 
{\em Proof.} Checking $t_f\models (c,\bmap)$ for a $(c,\bmap)\in D_S$ amounts to checking $(t_f)_\bmap\in\semm{c}$, which amounts to checking $t_{\bmap.f}\in\semm{c}$ by the Pullback Lemma (tiling two pb-squares is again a pb-square).  But $(c,\bmap.f)\in D_{S'}$ as $f$ is a sketch \mor, hence  $t_{\bmap.f}\in\semm{c}$ as $t\models S'$. \qed
\begin{remark}[Multisketches]
Makkai had defined a sightly more general notion of a generazalized sketch, in which the diagram part $D_S$ of a sketch $S$ is a {\em family} of diagrams rather than a set, \ie, the same diagram can be repeated in $D_S$ (an accurate definition is in \cref{sec:multiskeDef}). We will call such sketches {\em multisketches}. The category of multisketches in signature \csig\ is denoted by $\GG||\csig$, and the obvious embedding $\GG|\csig$ into $\GG||\csig$ (a set is trivially a family) has  

\zd{to be completed!!!}
\end{remark}


\subsection{From graphs to categories}
\zd{Below is a very old and probably stupid version -- it'd 'endinputed'}

%\endinput

In a majority of SE applications, as soon as you have a directed graph $G$, it makes sense to compose it arrows and consider identity arrows, thus arriving to the category $\bar G$ freely generated by $G$.\footnote{As is well known, the forgetful functor \frar{U}{\catcat}{\graphcat} has a left adjoint \frar{Fr}{\graphcat}{\catcat}, and we write $\bar G$ for $Fr(G)$.}
This makes sense for both graph-schemas and graph-instances, and the typing mapping \frar{t}{X}{S} freely generates a functor \frar{\bar t}{\bar X}{\bar S}. Not all functors appearing in practice are freely generated in this way: it is often the case that a basic arrow in $X$ is to be typed by a composed arrow in $S$. For example, diagram \cref{eqdiag:drivesTo-2} shows a data schema graph  \drivinggraphSch\ consisting of two solid arrows, which together with the derived dashed arrow and identities (not shown) makes category \drivingcatSch\ (ignore [..]-labels  for a while). %Its instance is a typing functor \frar{t}{\bar X}{\namedSchema{S}{Driving}} n which arrow \drivesTo\ can be considered as composition and 
\begin{equation}\label{eqdiag:drivesTo-2}
\begin{tikzcd}[row sep=8ex, column sep=7ex,cells={nodes={draw=black, %circle, 
		outer sep=0pt,inner sep=.35ex}}]
&
\Company \ar[rd, "\locAt"] 
\ar[ld, <-, "\gapnamegap{1}{\worksFor}{-1}" ', pos=0.5] 
& \\
\Person \ar[rr, derived, "\drivesTo"{name=dri,}' ]
\ar[from=1-2, to=dri, gray, phantom, description, "\text{[$\subseteq$]}", pos=0.8]
\ar[from=1-2, to=dri, red, phantom, description, "\text{[$=$]}", pos=0.4]
&& \Address
\end{tikzcd}
\end{equation}
Instances are typing functors \frar{t}{\drivingcatInst}{\drivingcatSch}, and it is clear that in a typical practical context, there may be persons who drive to an address without necessarily working for a company located at that address.\footnote{Such \drivesTo-typed links belong to the original instance {\em graph} \drivinggraphInst\ rather than being freely generated by arrow composition, which makes typing a Kleisli mapping of the monad \frar{Fr\comp U}{\graphcat}{\graphcat} (while \catcat\ is the Eilenberg=Moore category of this monad).} Hence, the inverse mapping $t^{-1}$ or $\semm{.}^t$ is a {\em lax} rather than strict  functor \frar{\semm{.}^t}{\drivingcatSch}{\spansetcat}. (Moreover, for any category $S$, categories $\catcat/S$ and $\pmb{Lax}(S,\spansetcat)$ are equivalent, see, \eg, \cite{}[neisfield].) %Thus, is is the semantic meaning of label $[\subseteq]$ in the drawing \cref{eqdiag:drivesTo}. 
Thus, we work in category $\GG=\catcat$ so that sketches' carrier objects are categories. If $S$ a sketch playing the role of a data schema, and $\bigtriangleup$  %\frar{\bmap}{\bigtriangleup}{\carr{S}} 
is a triangular commutative diagram in  \carr{S}, we visualize this fact with label $[\subseteq]$ that conveys its semantic meaning for \GG-instances over $S$, ie, functors \frar{t}{X}{\carr{S}} equivalent to lax functors \frar{\semm{.}^t}{\carr{S}}{\spansetcat}. In this sense, label $[\subseteq]$ belongs to the meta-\fwk\ that regulates correctness of general instances over \carr{S} rather than to sketch $S$ as such: indeed, any \GG-arrow into category \carr{S} automatically satisfies the $[\subseteq]$-requirement. In contrast, the red label [=] visualizes a real constraint declared in sketch $S$, which can be violated by some \carr{S}-instances, \ie, functors into \carr{S}. 

Formally, the data schema shown in \cref{eqdiag:drivesTo-2} can be seen as a sketch $S=(\carr{S}, D_S)$ over category $\GG=\catcat$, whose carrier is category $\carr{S}:=\drivingcatSch$ consisting of three non-identity arrows subjected to one non-trivial commutativity condition $\worksFor\comp\locAt = \drivesTo$. The set of \cdecla s (labelled diagrams) $D_S$ is a singleton, whose only element is a pair $([=], \bmap)$ of a label [=] from the signature in \cref{tab:sign} and a binding functor \frar{\bmap}{S_{[=]}}{\drivingcatSch} defined in the obvious way. % by formula $[=](\worksFor,\locAt,\drivesTo)$. 
%
Alternatively, the same data schema can be seen as a sketch $S'=(\carr{S'}, D_{S'})$ over category $\GG=\graphcat$, whose carrier is graph $\drivinggraphSch'$ consisting of three arrows. The set of \cdecla s  $D_{S'}$ consists of two labelled diagrams: $d=[\subseteq](\worksFor,\locAt, \drivesTo))$ and $d'=[eq](\worksFor,\locAt, \drivesTo))$ sharing the same binding map. However, as any instance \frar{t}{X}{\carr{S'}} satisfies the condition $d' \Rightarrow d$, diagram $d$ can be omitted in sketch $S'$. 

\zd{it should be written clearer: the semantics \fwk\ of lax functors forces any commutativity constraint [=] actually be a subsetting constraint $\subseteq$, from which two specialization constraints are formed: proper subsetting $[\subset]$ and equality $[=]$. Hence, it would be reasonable to refer to these three constraints as to ... as above. }
For more complex data schemas, the amount of `grey' labelled diagrams may be big and it does make sense to encapsulate them all in the metalevel by considering category \GG\ to be \catcat\ rather than \graphcat.  
%-- an old presentation of the story 
%To make it formal, we slightly generalize the notion of sketch by making its carrier objects and diagram shapes categories rather than graphs; then drawing \cref{eqdiag:drivesTo} with the green label, shows a sketch $S_\mathrm{green}$ whose carrier is the category \drivingcatSch\ and the set of diagrams is the singleton $\{[\subseteq](\bmap)\}$, where \frar{\bmap}{S_\subseteq}{\drivingcatSch} is the obvious functor. However, having this label in a sketch is superfluous as any instance satisfies the constraint. In contrast, considering  drawing \cref{eqdiag:drivesTo} with the red label is formalized as sketch $S_\mathrm{red}$ with the same carrier category  \drivingcatSch\ and the only diagram \frar{\bmap}{S_{[=]}}{\drivingcatSch}. Now an instance $t\models S_\mathrm{red}$ iff the exact equality holds: $\worksFor^t \comp \locAt^t =\drivesTo^t$, \ie, \frar{\_^t}{\drivingcatSch}{\spansetcat} is a strict functor. 

%The next section describes a different mechanism of implementing semantics of diagrammatic constraints. 
%Correspondingly, a concrete constraint should provide such a mechanism, and the next definition presents one such possibility.

%\endinput

==> sections/eInst-theoryAbstractNewToOld.tex <==
\newcommand{\tcatCC}{\enma{\tcat_\CC}}
\renewcommand{\twix}[1]{\twixU{#1}}

\renewcommand{\Sencat}{S}
\renewcommand{\Modcat}{M}
\renewcommand{\Evicat}{E}

\renewcommand{\projXY}[2]{\enma{p_{#1#2}}}
\newcommand{\projXYtwi}[2]{\enma{p_{#1#2}^\twimor}}

\newcommand{\pM}{\projXY{M}{}}
\newcommand{\pS}{\projXY{S}{}}
\newcommand{\pE}{\projXY{E}{}}
\newcommand{\pMS}{\projXY{M}{S}}
\newcommand{\pSE}{\projXY{S}{E}}
\newcommand{\pME}{\projXY{M}{E}}

\newcommand{\pEtwi}{\projXYtwi{E}{}}
\newcommand{\pMStwi}{\projXYtwi{M}{S}}
\newcommand{\pSEtwi}{\projXYtwi{S}{E}}
\newcommand{\pMtwiPrim}{\projXYtwi{M'}{}}



\subsection{Abstract institutions without elements}\label{sec:eInst-abstract}
 The goal of this section is to consider Sat-axiom in the new setting with evidence in an abstract setting. We begin  with a ternary span diagram (see  \cref{eqdiag:ternarySpan-in-CC} below)
 where nodes and arrows are objects and \mor s  of an arbitrary \caty\ \CC\ with finite limits (the diagram above uses products). An abstract setting will make them more transparent. Then we will return to categorical institutions with \CC\ being \catcat.  Although for our constructs, it is sufficient to require \CC\ to have pullbacks, we will assume \CC\ to be finitely complete \caty\ (FCC) as
 some of the constructs  can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcatCC$. Moreover, we need the abstract setting to clarify working with institutions in \catcat, and the latter does have products.   
%\input{sections/piece--institution-as-4tuple}
%

Through this section (except \cref{sec:spans})  \CC\ is an arbitrary given FCC. 
We begin with recalling some basics of the notion of a span.
\subsubsection{Spans}\label{sec:spans}
Let \CC\ be an arbitrary \caty\ with pullbacks.
\begin{constrN}[Spans]\label{constr:spans}
	Given a pair of \CC-objects $A$ and $B$, a {\em span in \CC\ from $A$ to $B$} is a pair of arrows \spandiag{A}{p_r}{\hat r}{q_r}{B} with a common source called the {\em apex} of the span (and arrows $p_r$, $q_r$ are the {\em legs} of the span, and objects $A$, $B$ are its {\em feet}). We then write \spanrar{r}{A}{B}. To ease notation, we will normally write $p$, $q$, and $r$ for $p_r$, $q_r$, and $\hat r$ (thus denoting a span and its apex by the same symbol). 
	
	Two parallel spans 
	\spanrar{r}{A}{B}, \spanrar{r'}{A}{B} are {\em equivalent}, $r\cong r'$, if there is an iso\mor\ \frar{i}{\hat r}{\hat r'} such that $i.r'=r$ and $i.q'=q$. Pullbacks in \CC\ provide span composition, which is associative up to coherent iso\mor s and constitutes a bi\caty\ \spanfunX{\CC}. Considering spans up to equivalence \congg, gives us a \caty\ \spanfuncongX{\CC}, which we will use below and silently identify spans with their equivalence classes.  
\end{constrN}
\begin{constrN} \label{constr:morAsspans}%For any \caty\ \CC\ with pullbacks, there 
	There are two embedding: 
\begin{equation}\label{eq:mor2spans}
\frar{\morAsspanXdn{\_}}{\CC}{\spanfuncongX{\CC}}   \text{~~and~~ } 
\frar{\morAsspanXup{\_}}{\CC}{\spanfuncongX{\opX{CC}}} 
\end{equation}
which map a \CC-\mor\ \frar{f}{A}{B} to spans 
\spanrar{\morAsspanXdn{f}}{A}{B}, where $\morAsspanXdn{f}= (\spandiag{A}{\id_A}{A}{f}{B} )$, and 
\spanlar{\morAsspanXup{f}}{A}{B}, where  $\morAsspanXup{f}= (\spandiag{B}{f}{A}{\id_A}{B} )$. 
 %
 Composition is strictly preserved due to \congg-factorization, %up to coherent iso\mor s in the bi\caty\ \spanfunX{\CC}: $(f.g)_{_\%}\cong f_{_\%}.g_{_\%}$ and $(f.g)^{\%}\cong g^{\%}.f^{\%}$, while identity is preserved strictly (we consider \CC\ as a bi\caty\ whose only 2-cells are 2-identities).  
 %
 %To ease notation, if \frar{f}{A}{B} in \CC\ and \spanrar{r}{B}{C} in \spanfunX{\CC}, we will often write $f.r$ for \spanrar{f_{_\%}.r}{A}{C}.  
 \end{constrN}
\begin{remark}
	Without \congg-factorization, \spanfunX{\CC} is a bi\caty\ and  hence supports the notion of adjointness. It can be proved that $\morAsspanXdn{f}\dashv \morAsspanXup{f}$ (see \cite{pare-spanConstr-tac10} for details). 
\end{remark}

% NOW THIS SWITH IS OUTDATED -- I CHENGED IT ALL!!!!!
% here is an impotant SWITCH in how abstract eSat is presented
%		\input{sections/piece--eSatDef--withProd}
%			%\input{diagrams/esatDefwithProd--macros}  IT DOES NOIT WIRK WHEN INPUTED HERE!!
		%\input{sections/piece--eSatDef--noProd}
%			%\input{diagrams/esatDefnoProd--macros}   IT DOES NOIT WIRK WHEN INPUTED HERE!!
%
\subsubsection{eSat spans}
\begin{defN}[Sat-base]\label{def:satBase}
	A {\em  %verified institution 
		base} is a quadruple  $(\CC, \CC_\senind, \CC_\modind, E)$ of a finitely complete \caty\ (FCC) \CC, two its FCC sub\caties\ (not necessarily disjoint) $\CC_\senind$ and $\CC_\modind$ closed under iso\mor s, whose objects are thought of as collections of {\em sentences} and {\em models} resp., and an  object  $E\in \Ob\CC$ thought of as a collection of {\em pieces of evidence}.  We will write $(\CC,E)$ for a base with $\CC_\senind=\CC =\CC_\modind$; such a base is just a pointed \caty. % (or to shorten notation if the subcategoires are not under discussion). 
	%To ease notation, we will often refer to such a base as to a pointed \caty\ $(\CC, E)$, and 
	We denote objects of $\CC_\modind$ and $\CC_\senind$ by $M, M', ..$ and $S, S',...$  resp. and omit explicit mentioning of \caties\ they belong.  
\end{defN}
%	The FCC \fwk\ is actually not needed for our work below: having pullbacks would be sufficient. However, some of the constructs below can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcat_\CC$. Moreover, in this paper we only need the abstract \fwk\ for clarifying what we will later do with institutions in \catcat, which is FCC. %We will provide these interpretation prefixed  with phrasing `with products' or `with elements'. (Recall that pullbacks and the terminal object provide all finite limits, \ie, make \CC\ an FCC.)
\begin{defN}[ESats: Sat-spans with evidence]\label{def:esatSpan}
	A {\em  \satty\ span with evidence} ({\em eSat})  over base \satbaseXY{\CC}{E} is a ternary span in \CC, \ie, a triple of \CC-arrows $(\pM, \pS, \pE)$ %\in \CC$\CCmod\timm\CCsen\timm \Evicat$ 
	with a common source $\modelsd$ and feet (target objects)  $M$, $S$, $E$, resp. Using products, this ternary span can be written as a binary span in three different equivalent ways, two of which are shown in diagrams \cref{eqdiag:trispans2bispans--twoDiags}a),b)
\begin{equation}\label{eqdiag:trispans2bispans--twoDiags}
	\begin{array}{cc}
		\TrispanToBispanMS
		& \TrispanToBispanSE
		\\ a)  %\text{(further \pMS\ is $p$, and \pE\ is $q$)} 
		 & b)
	\end{array}
	\end{equation}
(which are two different views of the same ternary diagram, which can be restored from the either view). In this paper, representation a) will be the main  one as the object $\M\timm\S$ is especially  important in our context and models the notion of preinstances, \ie, all possible pairs (model, sentence). To ease notation, we will write $p$ for \pMS\ and $q$ for \pE. Thus, an eSat is 
 binary span  	$\M\timm\S\xleftarrow{p}\;\vDash\;\xrightarrow{q}\E$ or \spanrar{\modelsd}{\M\timm\S}{\E} (\ie, we denote the span and its apex by the same symbol). 
%
%If objects $S$ and $M$ in a diagram are placed with $S$ on the right of  $M$, we will denote the same data (\ie, $q$ points to $S\timm E$ and $p$ to $M$) by using more customary symbol $\vDash$ rather than $\Dashv$. 
%The binary subspan $(p_S, p_M)$  will be denoted by \spanrar{\Dashv_{SM}}{S}{M} or  \spanlar{\vDash_{MS}}{M}{S} (but note that the arrow goes from $S$ to $M$ in both cases). %$\vDash_{MS}$ but directed as \spanlar{\vDash_{MS}}{M}{S}. 
	
	If a triple of elements \frar{(m,\phi,e)}{\tcat}{\M\timm\S\timm\E} factors through \modelsd, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $\phi$  as {evidenced} by a {\em (piece of) evidence} $e$ 
	%{\em verified assurance of level} $e$,  
	and write $m\satUD{e}{}\phi$.  
	
	We require \satty\ to be invariant under iso\mor s: for any iso\mor s \frar{i_X}{X}{X} 	in the corresponding \caty\ (where $X\in\{\S, \M, \E\}$), there is a \CC-iso\mor\ \frar{i}{\vDash}{\vDash} such that $p_X.i_X =i.p_X$ with $X\in \{S, M, E\}$.  %and $e.i_\E=i.e$. \qquad \qquad \qquad.  
\end{defN}
%
\subsubsection{Twisted \mor s of eSats} % -- SUBSECTION FOR THE M x S to E version. There is also M to S x E version
%Now we consider twisted \mor s of eSats
\begin{defN}
		A {\em twisted pair (of arrows)} is a pair $\twip=(s, r)$ of \mor s \frar{s}{S}{S'} in $\CCsen\subset\CC$ and  \frar{r}{M'}{M} in $\CCmod\subset\CC$, considered as an arrow  \frar{\twip}{(S,M)}{(S',M')} so that $r$ goes againt \twip\ (hence the name {\em twisted} and symbol \twip\ as a visual reminder).% 
		\footnote{Symbol $r$ also reminds about 'reversing' and the 'model reduct' functor in the institution theory. Symbol $s$ is then appropriate for 'substitution' functors.} 
		Such pairs form category $\twixD{\CC}:=\CC_\senind\times\opX{\CC_\modind}$. 
\end{defN}
\begin{defN}[Twisted \mor s (MS-view)]\label{def:twistedMorph}	%MStoE
 	Let  \spanrar{\modelsd}{\M\timm\S}{E} and  \spanrar{\modelsd'}{M'\timm S'}{E} be two eSat spans, and 
 	\frar{\twip=(s,r)}{(S,M)}{(S',M')} a twisted pair between their feet as shown in diagram \cref{eqdiag:twistedMorphDef--MStoE}a).  Then we can form two new parallel eSat spans, 
 	\spanrar{\modelsd_\twimor}{P_\twimor}{\E} and
 	\spanrar{\modelsd'_\twimor}{P_\twimor}{\E}, defined by span composition:
%$\modelsd_\twimor=\morAsspanXdn{(r\timm1_S)}.\modelsd$ and 
%$\modelsd'_\twimor=\morAsspanXdn{( 1_{M'}\timm s)}.\modelsd'$
%(see  the diagram where the subscript \morAsspanXdn{} is omitted:)
 as specified in diagram \cref{eqdiag:twistedMorphDef--MStoE}a). %in which both spans are glued together)
 	
	 A twisted pair \twimor\  is called a {\em (twisted) eSat \mor}, if spans $\modelsd_\twimor$ and $\modelsd'_\twimor$ are \congg-equivalent and can be identified in $\spanfuncongX{\CC}$. 	Then we write  \frar{\twimor}{\modelsd}{\modelsd'}. 
	 %
	 Diagram \cref{eqdiag:twistedMorphDef--MStoE}b shows this definition unpacked in \CC\ after the two equivalent spans are glued together.
%
	%	\renewcommand{\Dashv}{\vDash}
	%\begin{figure}
\begin{equation}\label{eqdiag:twistedMorphDef--MStoE}
		%\vsatDefTripleDiagram
		\begin{tabular}{c@{\quad}cc} % see first rows of the file for macros
			\twiMorphDefViaSpansMStoE
			& \twiMorphDefUnpackedMStoE
			%& \twistedMorphDefPackedMStoE
%			& \satAxiomPackedMStoE
&	$\begin{array}{c} % iff statement 
	m'.r \models^e \phi
	\\ [5pt]\text{iff}\rule{0ex}{1.ex}
	\\ [5pt] m' \models'^e \phi.s
\end{array}$
			\\
			a)  &  b)  & c)
		\end{tabular}
	\end{equation}
%i) two pullbacks specified in diagram a)  (the upper orange and the lower green) produce the same (up to iso\mor\ of its domain) arrow $p_f$ (whose domain can be seen as a twisted Sat --- this is the ``iff'' of the Sat-axiom  in \cref{eqdiag:eSatAxiom}) %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $\twip$, but we omit it.)
%
%ii) the rightmost square (shown triangularly) commutes  and $q_f$ denotes its diagonal (defined up to iso\mor\ of its domain  $\modelsd_\twimor$). 
\end{defN}
 %  eSat as commute -- now commented
%\begin{propo}[eSat-axiom as commutativity]\label{prop:satAxiom-asCommut}
%%\newline 
%A twisted pair $(r, s)$ is a twisted \mor\ of eSats  iff the square of span \mor s specified in diagram \cref{eqdiag:twistedMorph--MStoE}b) commutes (up to a span iso\mor). The counterpart of the strict definition of a twisted \mor\ is a specified diagonal span such that both triangles commute. 
%\end{propo}
%{\em Proof.} Unpack the definition of span composition. \qed %Diagram chasing with pullbacks. 
\begin{defN}[eSat axiom]
	We say  a twisted pair \frar{(s,r)}{(\S,\S')}{(\M,\M')} {\em satisfies eSat axiom} if for any triple of elements \frar{(m', \phi, e)}{\tcat}{\M'\timm\S\timm\E}, the logical equivalence  in diagram \cref{eqdiag:twistedMorphDef--MStoE}c) holds, \ie, $(m'.r, \phi, e)$ factors through \modelsd\ iff  $(m',\phi.s, e)$ factors through $\modelsd'$. \qed
\end{defN}
	%b) Note the \id-component of the right-most arrow in diagrams a) and b), which states that the same piece of evidence serves both sides of the iff statement. It means the twisted \mor\ condition implies  the Sat-axiom but the converse should not be true: 
\begin{remark}eSat axiom is stronger than the usual Sat axiom as it requires preservation of the evidence $e$ for both passaged (the top-down and the bottom-up) in implications c). We can probably construct a case where the Sat-axiom holds but the eSat one fails (when  $m'.r \models^e \phi$ for some \frar{e}{\tcat_\CC}{E} iff $m'\models'^{e'} \phi.s$ for some \frar{e'}{\tcat_\CC}{E}). We consider such cases as violating the triviality of the Sat-axiom. 
\end{remark}
\begin{propo}
	If a twisted pair $(r,s)$ is a twisted \mor, then it satisfies the eSat axiom.
\end{propo}
{\em Proof.} The upper and lower pullbacks in diagram \cref{eqdiag:twistedMorphDef--MStoE}b) produce the upper and the lower statements in equivalence c). \qed 
% --- the SEto M section
\begin{defN}[Twisted \mor s: SE-view]\label{def:twistedMorph-SEtoM}	%MStoE
	Let  \spanrar{\modelsr}{\S\timm\E}{\M} and  \spanrar{\modelsr'} {S'\timm E} {\M'} be two eSat spans, and 
	\frar{\twip=(s,r)}{(S,M)}{(S',M')} a twisted pair as above. 
	%shown in diagram \cref{eqdiag:twistedMorph--MStoE} a)  
	Then we can form two new parallel eSat spans, 
	\spanrar{\modelsr_\twimor}{S\timm E}{\M'} and
	\spanrar{\modelsr'_\twimor}{S \timm E}{\M'}, defined by span composition as specified in diagram \cref{eqdiag:twistedMorphDef--SEtoM}a)

	A twisted pair \twimor\  is called a {\em (twisted) eSat \mor}, if spans $\modelsr_\twimor$ and $\modelsr'_\twimor$ are \congg-equivalent and can be identified in $\spanfuncongX{\CC}$. 	Then we write  \frar{\twimor}{\modelsr}{\modelsr'}. 
	%
	Diagram \cref{eqdiag:twistedMorphDef--SEtoM}b shows this definition unpacked in \CC. 
	%
	%	\renewcommand{\Dashv}{\vDash}
	%\begin{figure}
	\begin{equation}\label{eqdiag:twistedMorphDef--SEtoM}
		%\vsatDefTripleDiagram
		\begin{tabular}{c@{\quad}cc} % see first rows of the file for macros
			\twiMorphDefViaSpansSEtoM
			& \twiMorphDefUnpackedSEtoM
			%& \twistedMorphDefPackedMStoE
			%			& \satAxiomPackedMStoE
			&	$\begin{array}{c} % iff statement 
				m'.r \models^e \phi
				\\ [5pt]\text{iff}\rule{0ex}{1.ex}
				\\ [5pt] m' \models'^e \phi.s
			\end{array}$
			\\
			a)  &  b)  & c)
		\end{tabular}
	\end{equation}
	%i) two pullbacks specified in diagram a)  (the upper orange and the lower green) produce the same (up to iso\mor\ of its domain) arrow $p_f$ (whose domain can be seen as a twisted Sat --- this is the ``iff'' of the Sat-axiom  in \cref{eqdiag:eSatAxiom}) %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $\twip$, but we omit it.)
	%
	%ii) the rightmost square (shown triangularly) commutes  and $q_f$ denotes its diagonal (defined up to iso\mor\ of its domain  $\modelsd_\twimor$). 
\qed\end{defN}
The two definitions of a twisted \mor\ should be equivalent, and it is indeed so per the result below, but the diagram chasing proving it turned out unexpectedly ``twisted''. 
\begin{propo}
	Two definitions of a twisted \mor, Def.\ref{def:twistedMorph} and Def. \ref{def:twistedMorph-SEtoM}, are equivalent.
\end{propo}
{\em Proof.} We first prove that for any twisted pair  $\twimor=(s,r)$, there is an iso\mor\
\frar{\switchX{\twimor}} {\modelsd_\twimor} {\modelsr_\twimor} (whose domain is the upper twisted eSat in diagram \cref{eqdiag:twistedMorphDef--MStoE}a) and the codomain is the upper twisted eSat in diagram \cref{eqdiag:twistedMorphDef--SEtoM}a) ) such that  diagram \cref{eqdiag:switchDiags-a4result-and-b4twistedPB}a) commutes. The proof is based on diagram \cref{eqdiag:switchDiags-a4result-and-b4twistedPB}b), in which span \spanrar{\modelsd}{\M\timm\S}{\E} is shown orange (with orange wiggly arc connecting the legs), and span \spanrar{\modelsd}{\S\timm\E}{\M} (with the same apex) is purple (and wiggly purple arc connects its legs). 
\begin{equation}\label{eqdiag:switchDiags-a4result-and-b4twistedPB}
	\begin{array}{cc}
 \switchDiag
 & 		\twistedPBdiag
		\\ a) & b) 
	\end{array}
\end{equation}
Span $\modelsd_\twimor$ is built as specified in diagram \cref{eqdiag:twistedMorphDef--MStoE}b) with PB denoted [pb]$_0$ (shown orange), and now we build span $\modelsr_\twimor$ (shown purple) as specified in diagram \cref{eqdiag:twistedMorphDef--SEtoM}b). We notice that $w=\pMS.\pi_M$, and hence the PB of cospan $(r,w)$ is given by two (purple) PB squares [pb]$_1$ and [pb]$_2$ as specified in the diagram. Next we build four $!$-arrows with subscripts due to universal properties: $!_{\#1}$ is by the universality of [pb]$_1$, which allows us to obtain a unique $!_{\#2}$ by the universality of [pb]$_2$. Arrow $!_{\timm3}$ is by the universality of product $M'\timm S$, which provides a unique $!_{\#4}$ by the universality of [pb]$_0$.  Arrows $!_{\#2}$ and $!_{\#4}$ are mutually inverse by the standard argument that otherwise their  uniqueness would be violated. Thus, we have built an iso\mor\ \switchX{\twimor} from diagram a). In the same way we can build an iso\mor\  \frar{\switchPrimX{\twimor}}{\modelsd'_\twimor}{\modelsr'_\twimor}. It is now clear that $\modelsd_\twimor\cong\modelsd'_\twimor$ iff $\modelsr_\twimor\cong\modelsr'_\twimor$ so that the two definitions equivalent. \qed
%%  remark on Gogiuen 
%\begin{remark}[On the Sat-axiom]
%	If $(\CC,E)$ is $(\setcat, \tcat)$ (so that evidencing is trivial),  and eSats are binary relations over sets, then diagram b) is immediately Sat-axiom as formulated in \cref{eqdiag:satAxiom}. It was noted by Goguen and Burstall \cite{GoguenBurstall-jofacm92}
%\end{remark}
%
%
%  not needed anymore but very useful to keep
%\input{sections/piece--eSatMorDef--MtoSEversion}
%

An advantage of \cref{def:twistedMorph-SEtoM} is an easy proof of the following fundamental result. 
\begin{propo}[Twisted \mor s compose]\label{prop:twistedMorph--Compose}
	Given a composable pair of twisted pairs,  \[
	(S,M) \xrightarrow{\twimor=(s,r)} (S',M') \xrightarrow{\twimor'=(s',r')} (S'', M'') 
	\] 
	%\frar{\twimor=(r,s)}{(S,M)}{(S',M')} and  \frar{\twimor'=(r',s')}{(S',M')}{(S'',M'')}, 
	if both pairs are twisted \mor s, then the composed pair $\twimor.\twimor'=(s.s', r'.r)$ is also a twisted \mor. 
\end{propo} 
{\em Proof.} As operators \cref{eq:mor2spans} are functors, diagrams \cref{eqdiag:twistedMorphDef--SEtoM}a) for \twimor\ and $\twimor'$ can be tiled. The resulting rectangle again commutes, which means that twisted pair $\twimor.\twimor'= (s.s', r'.r)$ is a twisted \mor. \qed
%--- anothe rproof --DIRECT-
%\input{sections/piece--directProofOfTwistedMorphCompose}
%
\begin{remark}[On type-theoretic proofs] As mentioned, the result above can be obtained without products; having pullbacks would be sufficient. Moreover, according to Michael Shulman,.. \zd{\Large to be filled-in}
\end{remark}
For the composition above, triples $(1_M, 1_S, 1_E)$ are identities, and we thus obtain a \caty\ \twistedSatcat\ of twisted \mor s between evidential  Sats. 
\begin{corol}[Category of twisted ESats] \label{corol:eSat-is-cat}
ESats and their twisted \mor s form a \caty\  (denoted 

\noindent $\twistedSatcat\satbaseCC$ or just \twistedSatcat\ if the base is clear) 
supplied with three projection functors: %a projection span $(p_\senind, p_\modind)$ and a projection functor $p_\evind$:
\begin{equation}\label{eq:twistedSpans-(mod-sen)}
% https://q.uiver.app/#q=WzAsNCxbMCwwLCJcXHR3aXN0ZWRTYXRjYXQiXSxbMCwyLCJcXG9wWHtcXENDbW9kfSJdLFsxLDIsIlxcQ0NzZW4iXSxbMiwxLCJcXHtcXEVcXH0iXSxbMCwxLCJwIiwyXSxbMCwyLCJcXHFzZW4iLDJdLFswLDMsIiFfXFxFIl1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\twistedSatcat \\
	\&\& {\{\E\}} \\
	{\opX{\CCmod}} \& \CCsen
	\arrow["\pmod"', from=1-1, to=3-1]
	\arrow["\psen"', from=1-1, to=3-2]
	\arrow["{!_\E}", from=1-1, to=2-3]
\end{tikzcd}
\end{equation}
where $\{E\}$ is a singleton \caty\ whose the only object is $E$ and the only arrow is $1_E$ (and hence $!_E(\twip)=1_E$ for any \mor\ \frar{\twip}{\models}{\models'} in \twistedSatcat). 
%	Moreover, the pair $(p_M,p_S)$ forms a two-sided discred fibration, \ie, $q$ is a discrete fibration whose lifts are $p$-vertical, $p$ is a discrete opfibration whose lifts are $p_M$-vertical, and the Beck-Chavalier condition (described below) holds. 
\end{corol}
%{\em Proof.} Given \frar{\twip}{\vDash}{\vDash'} and \frar{\twimor'}{\vDash'}{\vDash''}, we define $(\twip.\twimor')_*=s.\twimor'_*$ and $(\twip.\twimor')^*=\twimor'^*.r$, but we now need to prove that twisted pair $(\twip.\twimor')$ satisfies the condition in dia\twimor'ram \cref{eqdia\twimor':twistedSpans}a) % of \cref{def:twistedMorph}. 
%%
%As operators \cref{eq:mor2spans} are functors, dia\twimor'rams \cref{eqdia\twimor':twistedSpans} b) for $\twip$ and $\twimor'$ can be tiled, which \twimor'ives us $\twixsatXdn{\twip.\twimor'}$ as the dia\twimor'onal of the composed rectan\twimor'le tile, \ie, $\twixsatXdn{\twip.\twimor'}\;=\; \twixsatXdn{\twip}.\twimor'^{**}\;= \;f_{**}. \twixsatXdn{\twimor'}$ in \spanfunX{\CC}, and thus the condition a) holds for $\twip.\twimor'$ by \cref{prop:satAxiom-asCommut} \qed. 
%
% --> the following piece if for signature morphisms -- not for this paper
%As any CPB  (\ie, pullback preserving) functor \frar{F}{\CC}{\CC'} gives rise to a functor \frar{\spanfunX{F}}{\spanfunX{\CC}}{\spanfunX{\CC'}}, the following is obvious. %checked by routine diagram chasing.
%\begin{propo}[\VSatcat-construct is functorial]\label{prop:VSat-is-functorial}
%	Any base \mor, \ie, pointed CPB functor \frar{F}{(\CC,E)}{(\CC', E')} respecting sub\caties\ of models and sentences, % (\ie, such that $F(V)=W$) 
%	gives rise to a functor \frar{F^\vDash}{\VSatcat(\CC,E)}{\VSatcat(\CC',E')}
%\end{propo}
%
\begin{defN}[E-Institutions] % with \verity] 
An {\em evidential institution} ({\em e-institution})  over a base \satbaseCCE\  is a functor
%
\[ 
\frar{\satfun} {\Sigcatt} {\twistedSatcat\satbaseCCE},
\]
 where \Sigcatt\ is a \caty\  of {\em signatures}. \cref{corol:eSat-is-cat} immediately gives us the usual presentation of an institution as a triple $(\modfun, \senfun, \modelsd)$ of functors \frar{\modfun=\;\modelsd.\pmod}{\Sigcatt}{\opX{\CCmod}} and  \frar{\senfun=\;\modelsd.\psen}{\Sigcatt}{\CCsen}, and a family of Sat-spans (now eSat-spans) of functors  indexed by signatures $\Sigmaa\in\Obb\Sigcatt$: % and evidence $e\in\Ob\E$:
 $$   
 [\modfun(\Sigmaa)\timm\senfun(\Sigmaa)]\xleftarrow{~~\pMsig~~}\;\modelsd_\Sigmaa\; \xrightarrow{~~\pSsig~~}\E
 $$
 such that the eSat-axiom holds: if a signature changes by a \mor\ \frar{f}{\Sigmaa}{\Sigmaa'}, then the twisted pair $(\senfun(f), \modfun(f))$ is a twisted \mor\ \frarxy{\modelsd_\Sigmaa}{\modelsd_{\Sigmaa'}}
 %For a signature $\Sigma$,  objects of \caties\  $\Sigma.\vsfun.\modfun$ and $\Sigma.\vsfun.\specfun$ are called {\em $\Sigma$-models} and {\em $\Sigma$-sentences} resp. 
\qed\end{defN}

\endinput

As any CPB  (\ie, pullback preserving) functor \frar{F}{\CC}{\CC'} gives rise to a functor \frar{\spanfunX{F}}{\spanfunX{\CC}}{\spanfunX{\CC'}}, the following is obvious. %checked by routine diagram chasing.
\begin{propo}[\VSatcat-construct is functorial]\label{prop:VSat-is-functorial}
	Any base \mor, \ie, pointed CPB functor \frar{F}{(\CC,E)}{(\CC', E')} respecting sub\caties\ of models and sentences, % (\ie, such that $F(V)=W$) 
	gives rise to a functor \frar{F^\vDash}{\VSatcat(\CC,E)}{\VSatcat(\CC',E')}
\end{propo}

%\begin{propo}
%	The pair $(\modfun, \senfun)$ is a two sided (Street)) fibration (fibred span), \ie, \modfun\ is a fibration whose lifts are vertical wrt. \senfun, and \senfun\ is an opfibration whose lifts are vertical wrt. \modfun, and the `interchange' equality holds (see \cite[Fibred spans]{jacobs-catLogicBook99} or nLab's site%
%	\footnote{ \verb| https://ncatlab.org/nlab/show/two-sided+fibration| }.
%\end{propo}
%{\em Proof (sketch).} 
%goes beyond the goals of this paper. 

==> sections/future.tex <==
\clearpage
\section{Conclusion and Future work}

{\sc To be completed.}

\endinput

\begin{includeShort}
In this extended abstract we presented central definitions and results about diagram logic and diagram algebra.
The accompanying technical report \cite{THETR} provides proofs, and an outlook of our future work plans. The main point is to extend the results currently obtained for one-layer operation signatures  for signatures with pre- and postconditions to allow for diagrammatic reasoning.
\end{includeShort}




==> sections/future/commaCat4inst.tex <==
%\clearpage 
\subsection{Institutions and comma categories}
%
%-->  has a detailed pictre of how fubred spans work!!!
%
%\begin{lemma}[Jacobs]
%	\input{diagrams/commalemma-General}
%\end{lemma}

\input{sections/mathBackgr-fibredSpans} 

%\input{sections/vsatSpans}



\subsubsection{Towards inst as fibrations}
\begin{lemma}[Comma \caties\ and Fibred spans] \label{lemma:commaGenSpecial}
	Let $(p,q)$ be a cospan of two functors.  Then  we have the following two results.
	
	a)  There is a span of functors $(\liftedX{q}, \liftedX{p})$  (see \cref{figdiag:commaCats}a), whose apex is the comma \caty\ \commacatYX{q}{p}, first leg \liftedX{q} is a fibration whose lifts are \liftedX{p}-vertical, the second \liftedX{p} is an opfibration whose lifts are \liftedX{q}-vertical, and the Beck-Chevalier conditions (see Appendix \cref{lemma:comma2fibredSpans}, p.\pageref{lemma:comma2fibredSpans}) hold.\footnote{Note our notation: the first leg of span $(p,q)$ ``dominates'' in the  $\setminus$ notation for the comma \caty\ so that symbols  \commacatYX{q}{p} and \commacatXY{p}{q} denote the same comma \caty: we use that one which is better aligned with the layout of the feet \AA\ and \BB.} 
	A span satisfying these conditions is called a {\em fibred span} (see Jacobs \cite{jacobs-catLogicBook99}) or {\em two-sided fibration}. note that the diagram does not commute (denoted by a puncture symbol $\odot$). 
	
	b) If, additionally, $p$ is an opfibration while $q$ is a fibration, then there are two new legs, $\commafibLegUp$ and $\commafibLegDn$ (see diagram b), whose notation stems form  the fact that the core of a comma object is an \XX-\mor\ ``in-between'' $q$ and $p$ projections, and the $\setminus$ symbol refers to these \mor s in-between) such that $\liftedX{p}.q = \commafibLegDn.p$ and $\liftedX{q}.p=\commafibLegUp.q$, \ie, we have two commutative squares. Then we have uniquely defined functors $!_*$ and $!^*$ into the pullback as shown in the diagram. 
%
	\input{diagrams/commalemma-GenSpec}
%
\end{lemma}
{\em Proof.} Statement a) in the strict form (the comma \caty\ is chosen and legs \liftedX{p}, \liftedX{q} are split) is proved in \cite{jacobs-catLogicBook99}, and is directly verified --- see Appendix. A weak version is specifies in nLab  (originated b y Shulman). Construction of span $(\commafibLegUp, \commafibLegDn)$ is specified by diagram b') above, where Cartesian and opCartesian lifts along $q$ and $p$ resp, are shown with $\tilde\cdot$ and $\bar\cdot$ resp.  Arrows $!_x$ are due to (op)Cartesianity of arrow $x$. Functoriality of mappings \commafibLegUp\ and \commafibLegDn\ is due to functoriality of (op)Cartesian lifting (\eg, see \cite[Exercise 1.1.6]{jacobs-catLogicBook99}). Commutativty of two squares follows from diagram b'), and functors $!_*$, $!^*$ are due to the universality of PB $\BB\times_{_\XX}\AA$. \qed

\begin{propo}[Institutions: Two definitions are equivalent]

	%	Institution Definition \rule{0mm}{7mm}
\end{propo}
{\em Proof.} It is well known that functors into \catcat\ and \opX{\catcat} are equivalent to op- and fibrations resp. The difficult part is to prove equivalence of the elementwise definition of the Sat-axiom and its fibred counterpart.


{\em From indexed to fibred.}
	\input{diagrams/instDef--Ind2fib}
{\em From fibred to indexed.}
\input{diagrams/instDef--Fib2ind}



\endinput
% OLd piece of inst via VSats

%\renewcommand{\Sigmaa}{\enma{L}}
\renewcommand{\Modsetsig}{\ModsetX{\Sigmaa}}
\renewcommand{\Sensetsig}{\SensetX{\Sigmaa}}
\renewcommand{\ModsetsigPrim}{\enma{\Modsetsig'}}
\renewcommand{\SensetsigPrim}{\enma{\Sensetsig'}}
\renewcommand{\modelssig}{\enma{\vDash}}
\renewcommand{\modelssigPrim}{\enma{\vDash'}}

\newcommand{\V}{\enma{V}}
\newcommand{\M}{\enma{M}}
\renewcommand{\S}{\enma{S}}
\renewcommand{\vsfun}{\enma{\mathsf{vsat}}}
\renewcommand{\vsatfun}{\enma{\mathsf{vsat}}}

\newcommand{\vsatfunLifted}{\ovr{\vsfun}}
\newcommand{\vsfunLifted}{\vsatfunLifted}



\subsection{Abstract verifiable \satty\ over a pointed \caty. V-institutions}
  
%\input{sections/piece--institution-as-4tuple}

\begin{defN}[Verifiable \satty]\label{def:verSat}
Let \CC\ be an FCC, and \V\ a fixed object in \CC. A {\em \verible\ \satty\ span} ({\em VS-span} or just {\em VSat})  is a span 
$\M\timm\S\xleftarrow{u}\,\vDash_\V\,\xrightarrow{v}\V$ in \CC, which we will often write as \spanrar{\vDash_\V}{\M\timm\S}{\V} (\ie, we denote the spans and its apex by the same symbol), and omit %the subindex \V. 
the subindex \V.  If a triple of elements
\frar{(m,s,v)}{\tcat}{\M\timm\S\timm\V} factors through $\vDash$, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $s$  
%(the institution community would say {\em sentence} $S$)
 with {\em verified assurance of level} $v$,  and write $m\satUD{v}{}s$.  We require \satty\ to be invariant under iso\mor s: for any triple of iso\mor s in \CC, \frar{i_X}{X}{X}, where $X\in\{\M, \S, \V\}$, there is an iso\mor\ \frar{i}{\vDash}{\vDash} such that $u.(i_\M,i_\S)=i.u$ and $v.i_\V=i.v$. \qquad \qquad \qquad %\textcolor{red}{\hspace{\qqquad}}

\noindent 
\begin{minipage}[h]{0.65\linewidth}
~~~~~A {\em \mor} of VSats,  \frar{f}{\vDash'}{\vDash},  is a pair  $(f^*, f_*)$  %\zd{$ \sattwistedD{f})$}
of an arrow \frar{f^*}{\M}{\M'} and an arrow \frar{f_*}{\S'}{\S} (note that directions of $f$ and $f^*$ are the opposite), 
such that the following two conditions hold (see the inset diagram, where $P$, $P'$, \twixU{P} denote products  (the last one is twisted),  and arrows $!$ and $!'$ are due by  the universality of products $P$ and $P'$): a) two pullbacks produce the same horizontal arrow denoted $u_f$ (this is the Sat-axiom's ``iff''),  and b) the right
 most rectangle (shaped triangularly) commutes
 and provides a unique 
\end{minipage}
\;\begin{minipage}[h]{0.35\linewidth}
		%
	\input{diagrams/satAxiomVerif-Arr}
		%
	\end{minipage}
%
%most rectangle (shaped triangularly) commutes 
%and provides a unique 
diagonal denoted $v_f$.  We thus have a correct VS-span \spanrar{(u_f,v_f)}{\M\timm\S'}{V} further denoted by $\vDash_f$ or sometimes $\twixU{\vDash}_f$ to recall that it is twisted. 
\end{defN}
\begin{constrN}[Category of VSats]
Morphism composition $f.g$ is given by $(f.g)_*=f_*.g_*$, $(f.g)^*=g^*.f^*$ and $\vDash_{f.g}$ is given by the pullback of cospan $(u_f.!'_f,\;u_g.!_g)$: the \pblemma\ ensures that conditions a) and b) hold for $\vDash_{f.g}$. Strict associativity is immediate and  $(\id_\M, \id_{\S})$ is the unit, which gives us \caty\ $\VSspancatX{\CC,\V}$ supplied with two projection functors $\opX{\CC}\xleftarrow{\modfun}\VSspancatX{\CC,\V}\xrightarrow{\senfun}\CC$. 
%\zdmoddok{Morphisms are obviously associatively composable and $(\id_\M, \id_{\S'})$ is the unit, hence, we have a \caty\ $\VSspancatX{\CC,\V}$ supplied with two projection functors $\opX{\CC}\xleftarrow{\modfun}\VSspancatX{\CC,\V}\xrightarrow{\senfun}\CC$.}{}{really??}{-5}
This span has several important properties (see \cite[Fibred Spans]{jacobs-catLogicBook99}) but their discussion is left for future work. 
\end{constrN}
The following is checked by routine diagram chasing.
\begin{propo}[\VSatcat-construct is functorial]\label{prop:VSat-is-functorial}
	Any pointed FCC functor \frar{F}{(\CC,V)}{(\DD, W)} (\ie, such that $F(V)=W$) gives rise to a functor \frar{F^\vDash}{\VSatcat(\CC,V)}{\VSatcat(\DD,W)}
\end{propo}
%\begin{propo}
%	The pair $(\modfun, \senfun)$ is a two sided (Street)) fibration (fibred span), \ie, \modfun\ is a fibration whose lifts are vertical wrt. \senfun, and \senfun\ is an opfibration whose lifts are vertical wrt. \modfun, and the `interchange' equality holds (see \cite[Fibred spans]{jacobs-catLogicBook99} or nLab's site%
%	\footnote{ \verb| https://ncatlab.org/nlab/show/two-sided+fibration| }.
%\end{propo}
%{\em Proof (sketch).} 
%goes beyond the goals of this paper. 
%
\begin{defN}[V-Institutions] % with \verity] 
An {\em institution with verification} ({\em v-institution})  over a pointed FCC $(\CC, \V)$ is a functor
%
\frar{\vsfun} {\signcat} {\VSspancatX{\CC,V} }, where \signcat\ is a \caty\  whose objects are called {\em signatures}. %For a signature $\Sigma$,  objects of \caties\  $\Sigma.\vsfun.\modfun$ and $\Sigma.\vsfun.\specfun$ are called {\em $\Sigma$-models} and {\em $\Sigma$-sentences} resp. 
\qed\end{defN}
%\begin{corol}
	%Classical Goguen-Burstall's 
Note that standard institutions are v-institutions over $(\Catcat, \tcat)$, in which the image of functor 
%
\frar{\vsfun.\senfun}{\signcat}{\CC} consists of discrete \caties \ only. % and elements of set $\Sigma.\vsfun.\senfun$ are called $\Sigma$-sentences rather than $\Sigma$-\specifin s. 
%\end{corol}
%
Discussion of indexing in \cref{sec:ske4systems} motivates the following. %necessity to define an indexed version of the institution concept. 
\begin{defN}[Indexing v-institutions]\label{def:indexedInstitutions}
	Let \frar{\vsatfun}{\signcat}{\VSatcatX{\CC,V}} be a v-institution over $(\CC,V)$. Its {\em indexing} is given by 
a pair functors %providing indexing projections:
%two \signcat-indexed choices of indexing projections: for any $\Sigmaa\in\signcat$, there are \CC-arrows  
\frar{\pii_S}{\signcat}{\CC^\twocat} with $\pii_S.\cod=\vsatfun.\senfun$ and 
\frar{\pii_M}{\signcat}{\opX{(\CC^\twocat)}} with $\pii_M.\cod=\vsatfun.\modfun$ (\ie, for each signature \Sigmaa, there are indexing projections for \Sensetsig\ and \Modsetsig). 
\qed\end{defN}
We need to build the corresponding VS-span for indexes, which is our real interest in system design. % applications. 
\begin{constrN}[Indexed VS-spans]\label{constr:liftingVSat}
	Let \spanrar{\vDash_\V=(u,v)}{\M\timm\S}{\V} be a VS-span over $(\CC, V)$. Let \frar{\pii_M}{\ovr{M}}{M}, \frar{\pii_S}{\ovr{S}}{S} be two \CC-arrows understood as model and  sentence objects indexing as discussed in \cref{sec:intro}. Then we can pullback $u$ along \frar{(\pii_M, \pii_S)}{\ovr{M}\timm\ovr{S}}{M\timm S} and get a {\em lifted} (or {\em indexed}) VS-span \spanrar{(\ovr{u},\ovr{v}}{\ovr{M}\timm\ovr{S}}{V} for model and sentence indexes. (Thinking elementwise, given a pair of indexes \frar{(\bar i, \bar j)}{\tcat}{\ovr{M}\timm\ovr{S}}, we define $\ovr{i}\; \ovr{\satrelsymbol_v}\; \ovr{j}$ iff 
	$\ovr{i}.\pii_M\satrelsymbol_v\ovr{j}.\pii_S$.) A routine diagram chasing shows that lifting works for VSat-\mor s, and actually we can define the category of lifted VSats by the following pullback diagram in \Catcat\ (recall that fibrations are stable under pullbacks):
	\input{diagrams/liftingVSat}
%\qed
\end{constrN}
\begin{corol}
	It is easy to see that Def. \ref{def:indexedInstitutions} gives us commutative square $\vsatfun.(\modfun, \senfun) = (\pii_M, \pii_S).\cod\timm\cod$ and hence a unique functor
\frar{\vsatfunLifted}{\signcat}{\VSatcatLiftedX{\CC, \id_V}} (see diagram \cref{eqdiag:lifitngVSats}) that does the job.
\end{corol} 
%Composition 
%\opX{\CC}, \VSatcat, \VSatcatX{Hru}, \VSatcatLiftedX{Hru}
\endinput

% \prodnodeS, \prodnodeSprim, \prodnodeFtwist\, 
 % \underprodS, \underprodSprim, \underprodFtwist



==> sections/future/eInst-theoryAbstractAssurLevels.tex <==
\subsection{Abstract institutions without elements}\label{sec:vInst-abstract}
 The goal of this section is to consider Sat-axiom in the new setting with evidence in an abstract setting. We begin  with a ternary span diagram (see  \cref{eqdiag:ternarySpan-in-CC} below)
 where nodes and arrows are objects and \mor s  of an arbitrary \caty\ \CC\ with finite limits (the diagram above uses products). An abstract setting will make them more transparent. Then we will return to categorical institutions with \CC\ being \catcat.  Although for our constructs, it is sufficient to require \CC\ to have pullbacks, we will assume \CC\ to be finitely complete \caty\ (FCC) as
 some of the constructs  can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcat_\CC$. Moreover, we need the abstract setting to clarify working with institutions in \catcat, and the latter does have products.   
%\input{sections/piece--institution-as-4tuple}
%
\begin{constrN}[Well-known: Morphisms as spans]\label{constr:mor2spans}
For any \caty\ \CC\ with pullbacks, there are two embedding: 
\begin{equation}\label{eq:mor2spans}
\frar{\_ _*}{\CC}{\spanfunX{\CC}}   \text{~~and~~ } 
\frar{\_ ^*}{\CC}{\spanfunopX{\CC}} 
\end{equation}
which map a \CC-\mor\ \frar{f}{A}{B} to spans \spanrar{f_*}{A}{B} with $f_*= (\spandiag{A}{\id_A}{A}{f}{B} )$ and 
\spanrar{f^*}{B}{A} with 
 $f^*= (\spandiag{B}{f}{A}{\id_A}{B} )$. Composition is preserved up to coherent iso\mor s in the bi\caty\ \spanfunX{\CC}: $(f.g)_*\cong f_*.g_*$ and $(f.g)^*\cong g^*.f^*$, while identity is preserved strictly (we consider \CC\ as a bi\caty\ whose only 2-cells are 2-identities).  
Moreover, as a bi\caty, \spanfunX{\CC} supports the notion of adjointness, and it can be proved that $f_*\dashv f^*$ (see \cite{pare-spanConstr-tac10} for details).

If \frar{f}{A}{B} in \CC, and \spanrar{g}{B}{C} in \spanfunX{\CC}, then we will often write $f.g$ for \spanrar{f_*.g}{A}{C}.  
\end{constrN}
%% NOW THIS SWITH IS OUTDATED -- I CHENGED IT ALL!!!!!
%% here is an impotant SWITCH in how abstract eSat is presented
%		\input{sections/piece--eSatDef--withProdNew}
%%			%\input{diagrams/esatDefwithProd--macros}  IT DOES NOIT WIRK WHEN INPUTED HERE!!
%		%\input{sections/piece--eSatDef--noProd}
%%			%\input{diagrams/esatDefnoProd--macros}   IT DOES NOIT WIRK WHEN INPUTED HERE!!
%%
\begin{defN}[Sat-base]\label{def:satBase}
	A {\em  %verified institution 
		base} is a quadruple  $(\CC, \CC_\senind, \CC_\modind, E)$ of a finitely complete \caty\ (FCC) \CC, two its FCC sub\caties\ (not necessarily disjoint) $\CC_\senind$ and $\CC_\modind$ closed under iso\mor s, whose objects are thought of as collections of {\em sentences} and {\em models} resp., and an  object  $E\in \Ob\CC$ thought of as a collection of {\em pieces of evidence}.  We will write $(\CC,E)$ for a base with $\CC_\senind=\CC =\CC_\modind$; such a base is just a pointed \caty. % (or to shorten notation if the subcategoires are not under discussion). 
	%To ease notation, we will often refer to such a base as to a pointed \caty\ $(\CC, E)$, and 
	We denote objects of $\CC_\modind$ and $\CC_\senind$ by $M, M', ..$ and $S, S',...$  resp. and omit explicit mentioning of \caties\ they belong.  
\end{defN}
%	The FCC \fwk\ is actually not needed for our work below: having pullbacks would be sufficient. However, some of the constructs below can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcat_\CC$. Moreover, in this paper we only need the abstract \fwk\ for clarifying what we will later do with institutions in \catcat, which is FCC. %We will provide these interpretation prefixed  with phrasing `with products' or `with elements'. (Recall that pullbacks and the terminal object provide all finite limits, \ie, make \CC\ an FCC.)
\begin{defN}[ESats: Sat-spans with evidence]\label{def:esatSpan}
	A {\em  \satty\ span with evidence} ({\em eSat})  over base \satbaseXY{\CC}{E} is a ternary span in \CC, \ie, a triple of \CC- arrows $(p, q_S, q_E)$ %\in \CC$\CCmod\timm\CCsen\timm \Evicat$ 
	with a common source $\models$ and feet (target objects)  $M$, $S$, $E$, resp. 
  \begin{mygroup}
	\renewcommand{\Sencat}{S}
	\renewcommand{\Modcat}{M}
	\renewcommand{\Evicat}{E}
	\begin{equation}\label{eqdiag:ternarySpan-in-CC}
		% https://q.uiver.app/#q=WzAsNSxbMSwwLCJcXG1vZGVscyJdLFswLDEsIlxcTW9kY2F0Il0sWzEsMSwiXFxTZW5jYXQiXSxbMywwLCJcXEV2aWNhdCJdLFszLDEsIlxcU2VuY2F0XFx0aW1tXFxFdmljYXQiLFsyNDAsNjAsNjAsMV1dLFswLDMsInFfRSJdLFswLDEsInAiLDJdLFswLDIsInFfUyIsMl0sWzQsMiwiIiwwLHsiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzQsMywiIiwyLHsiY29sb3VyIjpbMjQwLDYwLDYwXSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzAsNCwicSIsMSx7ImNvbG91ciI6WzI0MCw2MCw2MF0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX0sWzI0MCw2MCw2MCwxXV1d
		\begin{tikzcd}[ampersand replacement=\&,column sep=small,row sep=scriptsize]
			\& \models \&\& \Evicat \\
			\Modcat \& \Sencat \&\& \textcolor{rgb,255:red,92;green,92;blue,214}{\Sencat\timm\Evicat}
			\arrow["{q_E}", from=1-2, to=1-4]
			\arrow["p"', from=1-2, to=2-1]
			\arrow["{q_S}"', from=1-2, to=2-2]
			\arrow[color={rgb,255:red,92;green,92;blue,214}, dashed, from=2-4, to=2-2]
			\arrow[color={rgb,255:red,92;green,92;blue,214}, dashed, from=2-4, to=1-4]
			\arrow["q"{description}, color={rgb,255:red,92;green,92;blue,214}, dashed, from=1-2, to=2-4]
		\end{tikzcd}
	\end{equation}
\end{mygroup}
With products, it can be written as a  binary span  	$\M\xleftarrow{p}\;\vDash\;\xrightarrow{q}\S\timm \E$ or 
\spanrar{\vDash}{M}{\S\timm\E} (\ie, we denote the span and its apex by the same symbol). 
%
%If objects $S$ and $M$ in a diagram are placed with $S$ on the right of  $M$, we will denote the same data (\ie, $q$ points to $S\timm E$ and $p$ to $M$) by using more customary symbol $\vDash$ rather than $\Dashv$. 
%The binary subspan $(p_S, p_M)$  will be denoted by \spanrar{\Dashv_{SM}}{S}{M} or  \spanlar{\vDash_{MS}}{M}{S} (but note that the arrow goes from $S$ to $M$ in both cases). %$\vDash_{MS}$ but directed as \spanlar{\vDash_{MS}}{M}{S}. 
	
	If a triple of elements \frar{(m,s,e)}{\tcat}{\M\timm\S\timm\E} factors through $\vDash$, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $s$  as {evidenced} by a {\em (piece of) evidence} $e$ 
	%{\em verified assurance of level} $e$,  
	and write $m\satUD{e}{}s$.  
	
	We require \satty\ to be invariant under iso\mor s: for any iso\mor s \frar{i_X}{X}{X}, 
	where $X\in\{\S, \M, \E\}$ (in the corresponding \caty), there is a \CC-iso\mor\ \frar{i}{\vDash}{\vDash} such that $p_X.i_X =i.p_X$ with $X\in \{S, M, E\}$.  %and $e.i_\E=i.e$. \qquad \qquad \qquad.  
\end{defN}
\begin{mygroup}
\begin{defN}[Twisted \mor s of eSats]\label{def:twistedMorph}	
	A {\em twisted pair (of arrows)} is a pair $f=(f_*, f^*)$ of \mor s \frar{f_*}{S}{S'} in $\CCsen$ and  \frar{f^*}{M'}{M} in $\CCmod$, written as \frar{f}{(S,M)}{(S',M')}. Such pairs form (twisted) category $\twixD{\CC}:=\CC_\senind\times\opX{\CC_\modind}$. 
	
	Given eSats \spanrar{\Dashv}{S\timm\E}{M} and \spanrar{\Dashv'}{S'\timm\E}{M'}, their {\em (twisted) \mor} %over base $(\CC,\L)$, \frar{f}{\Dashv}{\Dashv'},  
	is a twisted pair \frar{f=(f^*, f_*)}{(S,M)}{(S',M')} 
	such that the following condition holds: %where  $P$, $P'$, and  \twixU{P} denote products, the latter one  is twisted)) %,  and arrows $!^*_f$ and $!_*^F$ are due to products' universality), 
	%
	two pullbacks specified in diagram \cref{eqdiag:twistedSpans}a)  (the upper-left (orange) and the lower-right (green)) produce the same (up to iso\mor) object denoted $\twixU{\Dashv}_f$ (this is the ``iff'' of the eSat-axiom  in \cref{eqdiag:eSatAxiom}) %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $f$, but we omit it.)
		%	\renewcommand{\Dashv}{\vDash}
		\renewcommand{\twix}[1]{\twixU{#1}}
		\renewcommand{\id}{\enma{\mathsf{id}}}
		%\begin{figure}
		\begin{equation}\label{eqdiag:twistedSpans}
			%\vsatDefTripleDiagram
			\begin{tabular}{c@{\quad}c} % see first rows of the file for macros
				\twistedMorphDefMain 
				& \twistedMorphDefPacked
				%		& \satAxiomPacked
				\\
				a)  &  b)  %& c)
			\end{tabular}
		\end{equation}
		%\caption{For \cref{def:twistedMorph} of twisted \mor s between eSats\label{figdiag:twistedSpans}}
		%\end{figure}
		%\end{mygroup}
	%The definition above above is {\em weak} in the sense that conditions i-ii) are properties that define a structure up to iso\mor. 
	Thus, a  twisted \mor\ is a twisted pair possessing some property. 
	We can give an equivalent but more constructive {\em strict} formulation that defines a twisted \mor\ as a triple $f=(f^*, f_*, \twixU{\Dashv}_f)$, where the third component is a quadruple of arrows with a common source (as specified in the diagram a) above) such that the two corresponding squares are pullbacks. 
\end{defN}
%
\begin{propo}[Sat-axiom as commutativity]\label{prop:satAxiom-asCommut}
	A twisted pair $(f^*, f_*)$ is a twisted \mor\  iff diagram \cref{eqdiag:twistedSpans}b) 
	commutes (up to a span iso\mor). (The shaded triangles with identity sides == are not parts ofthe diagram: they recall definitions of two ways \cref{eq:mor2spans} of converting morphisms to spans).  The counterpart of the strict definition of a twisted \mor\ is a specified diagonal span such that both triangles commute. 
\end{propo}
{\em Proof.} Unpack the definition of span composition. %Diagram chasing with pullbacks. 
\end{mygroup}
\begin{remark}[On the Sat-axiom]
If $(\CC,E)$ is $(\setcat, \tcat)$ (so that evidencing is trivial),  and eSats are binary relations over sets, then diagram b) is immediately Sat-axiom as formulated in \cref{eqdiag:satAxiom}. It was noted by Goguen and Burstall \cite{GoguenBurstall-jofacm92}
\end{remark}
\begin{remark}	
Note the $1_E$-component of the right-most arrow in diagrams a) and b), which states that the same piece of evidence serves both sides of the iff statement. It means that the twisted \mor\ condition implies  the ordinary Sat-axiom but the converse should not be true: we can probably construct a case where Sat-axiom holds in  a weaker sense with different evidence: $f^*(m')\models^e s$ for some \frar{e}{\tcat_\CC}{E} iff $m'\models'^{e'} f_*(s)$ for some \frar{e'}{\tcat_\CC}{E}. We consider such cases as violating the triviality of the Sat-axiom. 
\end{remark}

\begin{propo}[Category of twisted ESats] \label{prop:eSat-is-cat}
ESats and their twisted \mor s form a \caty\  (denoted 

\noindent $\twistedSatcat\satbaseCCE$ or just \twistedSatcat\ if the base is clear) 
supplied with three projection functors: %a projection span $(p_\senind, p_\modind)$ and a projection functor $p_\evind$:
\begin{equation}\label{eq:twistedSpans-(mod-sen)}
% https://q.uiver.app/#q=WzAsNCxbMCwwLCJcXHR3aXN0ZWRTYXRjYXQiXSxbMCwyLCJcXG9wWHtcXENDbW9kfSJdLFsxLDIsIlxcQ0NzZW4iXSxbMiwxLCJcXHtcXEVcXH0iXSxbMCwxLCJwIiwyXSxbMCwyLCJcXHFzZW4iLDJdLFswLDMsIiFfXFxFIl1d
\begin{tikzcd}[ampersand replacement=\&,sep=small]
	\twistedSatcat \\
	\&\& {\{\E\}} \\
	{\opX{\CCmod}} \& \CCsen
	\arrow["\pmod"', from=1-1, to=3-1]
	\arrow["\qsen"', from=1-1, to=3-2]
	\arrow["{!_\E}", from=1-1, to=2-3]
\end{tikzcd}
\end{equation}
where $\{E\}$ is a singleton \caty\ whose the only object is $E$ and the only arrow is $1_E$ (and hence $!_E(f)=1_E$ for any \mor\ \frar{f}{\models}{\models'} in \twistedSatcat). 
%	Moreover, the pair $(p_M,p_S)$ forms a two-sided discred fibration, \ie, $q$ is a discrete fibration whose lifts are $p$-vertical, $p$ is a discrete opfibration whose lifts are $p_M$-vertical, and the Beck-Chavalier condition (described below) holds. 
\end{propo}
{\em Proof.} Given \frar{f}{\vDash}{\vDash'} and \frar{g}{\vDash'}{\vDash''}, we define $(f.g)_*=f_*.g_*$ and $(f.g)^*=g^*.f^*$, but we now need to prove that twisted pair $(f.g)$ satisfies the condition in diagram \cref{eqdiag:twistedSpans}a) % of \cref{def:twistedMorph}. 
%
As operators \cref{eq:mor2spans} are functors, diagrams \cref{eqdiag:twistedSpans} b) for $f$ and $g$ can be tiled, which gives us $\twixsatXdn{f.g}$ as the diagonal of the composed rectangle tile, \ie, $\twixsatXdn{f.g}\;=\; \twixsatXdn{f}.g^{**}\;= \;f_{**}. \twixsatXdn{g}$ in \spanfunX{\CC}, and thus the condition a) holds for $f.g$ by \cref{prop:satAxiom-asCommut} \qed. 

Triples $(1_M, 1_S, 1_E)$ are identities, and we thus obtain a \caty\ \twistedSatcat\ of twisted \mor s between eSats. Projection functors are obvious. \qed
%
% --> the following piece if for signature morphisms -- not for this paper
%As any CPB  (\ie, pullback preserving) functor \frar{F}{\CC}{\CC'} gives rise to a functor \frar{\spanfunX{F}}{\spanfunX{\CC}}{\spanfunX{\CC'}}, the following is obvious. %checked by routine diagram chasing.
%\begin{propo}[\VSatcat-construct is functorial]\label{prop:VSat-is-functorial}
%	Any base \mor, \ie, pointed CPB functor \frar{F}{(\CC,E)}{(\CC', E')} respecting sub\caties\ of models and sentences, % (\ie, such that $F(V)=W$) 
%	gives rise to a functor \frar{F^\vDash}{\VSatcat(\CC,E)}{\VSatcat(\CC',E')}
%\end{propo}
%
\begin{defN}[E-Institutions] % with \verity] 
An {\em evidential institution} ({\em e-institution})  over a base \satbaseCCE\ is a functor
%
\[ 
\frar{\satfun} {\Sigcat} {\twistedSatcat\satbaseCCE },
\]
 where \Sigcat\ is a \caty\  whose objects are called {\em signatures}. %For a signature $\Sigma$,  objects of \caties\  $\Sigma.\vsfun.\modfun$ and $\Sigma.\vsfun.\specfun$ are called {\em $\Sigma$-models} and {\em $\Sigma$-sentences} resp. 
\qed\end{defN}

\endinput

As any CPB  (\ie, pullback preserving) functor \frar{F}{\CC}{\CC'} gives rise to a functor \frar{\spanfunX{F}}{\spanfunX{\CC}}{\spanfunX{\CC'}}, the following is obvious. %checked by routine diagram chasing.
\begin{propo}[\VSatcat-construct is functorial]\label{prop:VSat-is-functorial}
	Any base \mor, \ie, pointed CPB functor \frar{F}{(\CC,E)}{(\CC', E')} respecting sub\caties\ of models and sentences, % (\ie, such that $F(V)=W$) 
	gives rise to a functor \frar{F^\vDash}{\VSatcat(\CC,E)}{\VSatcat(\CC',E')}
\end{propo}

%\begin{propo}
%	The pair $(\modfun, \senfun)$ is a two sided (Street)) fibration (fibred span), \ie, \modfun\ is a fibration whose lifts are vertical wrt. \senfun, and \senfun\ is an opfibration whose lifts are vertical wrt. \modfun, and the `interchange' equality holds (see \cite[Fibred spans]{jacobs-catLogicBook99} or nLab's site%
%	\footnote{ \verb| https://ncatlab.org/nlab/show/two-sided+fibration| }.
%\end{propo}
%{\em Proof (sketch).} 
%goes beyond the goals of this paper. 

==> sections/future/eInst-theoryConcreteNew.tex <==
\subsection{Concrete institutions with elements}\label{sec:vInst-concrete}




\begin{defN}[Categorical E-institutions]
	A {\em categorical e-institution} is an e-institution over base $(\catcat, \E, \L)$, \ie, a functor \frar{\models}{\Sigcat}{\twistedSatcat(\catcat, \E, \L)} for some predefined functor \frar{\ellE}{\E}{\L}.  Unpacking this definition with \cref{def:esatSpan} and notation \cref{eq:twistedSpans-(mod-sen)},  gives us functors
	\[ 
	 \frar{\modfun=\vDash.\pmod}{\Sigcat}{\opX{\catcat}} \text{~ and ~} \frar{\senfun=\vDash.\psen}{\Sigcat}{\catcat},
	 \] and a %double-indexed ($\Sigmaa\in\Ob\,\Sigcat$, $e\in\Ob E$) 
	family of spans of functors indexed by $\Sigmaa\in\Obb\predsig$:
	\[
	%(\spanlar{\modelssig}{\Modcatsig}{\eSencatsig}) _{\Sigmaa\in\Ob\Sigcat}
	\spandiag{\Modcatsig}{~\pMsig~}{~\modelssig~}{~\pSsig~}{\Sencatsig\timm_L\,\E}
	\]
	 %\spanlar{\satfun_\Sigmaa^e}{\modfun(\Sigmaa)}{\senfun(\Sigmaa)} in \catcat\  
	 such that for any signature \mor \frar{f}{\Sigmaa}{\Sigmaa'}, we have diagram \cref{eqdiag:esatAxiom-concrete} a), in which the left-upper and the right-lower squares are pullbacks. (Equivalently, the diagram \cref{eqdiag:twistedSpans}b) for the institution data commutes.) In terms of elements, it amounts to the {\em evidence preserving Sat-axiom} specified in \cref{eqdiag:esatAxiom-concrete}b) (where, recall, sentences $s$ and $s'$ have the same assurance level label). 
	%
	\input{diagrams/eSatAxiom}
	%
	%In diagram a) above,  the left-upper and the right-lower squares are PBs (\ie, we have a commuting diagram in \spanfunX{\catcat} by \cref{prop:satAxiom-asCommut}). %The diagonal in the commuting diagram a) is explained above in \cref{eqdiag:twistedSpans}b), and the 
%	The iff-statement b) is  commutativity applied to arbitrary pair $(m'\in\Ob\ModcatsigPrim, \, s\in\Ob\Sencat)$.  
%	%$f^*(m')\vDash^e_\Sigmaa s$ iff $m'\vDash_{\Sigmaa'} ^e f_*(s)$ for any $m'\in\Ob\,\modfun(\Sigmaa')$ and $s\in\Ob\, \senfun(\Sigmaa)$  
	\qed\end{defN}
\begin{corol}
	Goguen-Burstall's institutions are e-institutions over base $(\catcat, \catcat, (\setcat, \tcat, \tcat)$ (\ie, all sentence \caties\ are discrete, and labelling and evidencing are trivial), and in which all apex categories \modelssig\ are discrete. Thus, these institutions can be seen as significantly decategorificited categorical e-institutions. 
	%
	%That is, any such institution amounts to functors \frar{\modfun=\satfun.p}{\Sigcat}{\opX{\catcat}}, \frar{\senfun=\satfun.q}{\Sigcat}{\catcat}, and a family of satisfaction spans \spanlar{\satfun_\Sigmaa}{\modfun(\Sigmaa)}{\senfun(\Sigmaa)}
\end{corol}
\begin{remark}[Sizes]
	\zd{...  over base $(\Catcat, \Catcat, \setcat, \tcat)$ or $(\Catcat, \Catcat, \catcat, \tcat)$ for the fully categorical version.}
\end{remark}
\begin{defN}[Inst. with sound argument]
	We say that a categorical e-institution 
	$$\frar{\modelss}{\Sigcat}{\twistedSatcat(\satbaseX{\CC})}$$ 
	 is an institution with {\em sound arguments} if for any  signature \Sigmaa,   functor \pSsig\ is an opfibrtaion whose lifts are \pMsig-vertical. 
	
	This statements  unpacked means that for any $m\modelssig^e s$,  any arrow \frar{r}{s}{s'} in \Sencatsig\ (called an {\em argument}) can be lifted to \frar{\liftedX{r}}{\modelssig}{\modelssig'} for which $\pMsig(\liftedX{r})=1_m$. Hence, $m\modelssig^{e'}\!s'$ with evidence $e'=\cod(\pEsig(\liftedX{r}))$. 
\end{defN}


\endinput % a good piece about indexing but some tech problems to save it seorately 

\input{sections/piece--indexing4v-institutions}
Discussion of indexing in \cref{sec:ske4systems} motivates the following. %necessity to define an indexed version of the institution concept. 
\begin{defN}[Indexing v-institutions]\label{def:indexedInstitutions}
	Let \frar{\vsatfun}{\signcat}{\VSatcatX{\CC,V}} be a v-institution over $(\CC,V)$. Its {\em indexing} is given by 
	a pair functors %providing indexing projections:
	%two \signcat-indexed choices of indexing projections: for any $\Sigmaa\in\signcat$, there are \CC-arrows  
	\frar{\pii_S}{\signcat}{\CC^\twocat} with $\pii_S.\cod=\vsatfun.\senfun$ and 
	\frar{\pii_M}{\signcat}{\opX{(\CC^\twocat)}} with $\pii_M.\cod=\vsatfun.\modfun$ (\ie, for each signature \Sigmaa, there are indexing projections for \Sensetsig\ and \Modsetsig). 
	\qed\end{defN}
We need to build the corresponding VS-span for indexes, which is our real interest in system design. % applications. 
\begin{constrN}[Indexed VS-spans]\label{constr:liftingVSat}
	Let \spanrar{\vDash_\V=(u,v)}{\M\timm\S}{\V} be a VS-span over $(\CC, V)$. Let \frar{\pii_M}{\ovr{M}}{M}, \frar{\pii_S}{\ovr{S}}{S} be two \CC-arrows understood as model and  sentence objects indexing as discussed in \cref{sec:intro}. Then we can pullback $u$ along \frar{(\pii_M, \pii_S)}{\ovr{M}\timm\ovr{S}}{M\timm S} and get a {\em lifted} (or {\em indexed}) VS-span \spanrar{(\ovr{u},\ovr{v}}{\ovr{M}\timm\ovr{S}}{V} for model and sentence indexes. (Thinking elementwise, given a pair of indexes \frar{(\bar i, \bar j)}{\tcat}{\ovr{M}\timm\ovr{S}}, we define $\ovr{i}\; \ovr{\satrelsymbol_v}\; \ovr{j}$ iff 
	$\ovr{i}.\pii_M\satrelsymbol_v\ovr{j}.\pii_S$.) A routine diagram chasing shows that lifting works for VSat-\mor s, and actually we can define the category of lifted VSats by the following pullback diagram in \Catcat\ (recall that fibrations are stable under pullbacks):
	\input{diagrams/liftingVSat}
	%\qed
\end{constrN}
\begin{corol}
	It is easy to see that Def. \ref{def:indexedInstitutions} gives us commutative square $\vsatfun.(\modfun, \senfun) = (\pii_M, \pii_S).\cod\timm\cod$ and hence a unique functor
	\frar{\vsatfunLifted}{\signcat}{\VSatcatLiftedX{\CC, \id_V}} (see diagram \cref{eqdiag:lifitngVSats}) that does the job.
\end{corol} 
%Composition 
%\opX{\CC}, \VSatcat, \VSatcatX{Hru}, \VSatcatLiftedX{Hru}





\endinput

% \prodnodeS, \prodnodeSprim, \prodnodeFtwist\, 
% \underprodS, \underprodSprim, \underprodFtwist



==> sections/future/piece--assuranceLevels.tex <==
\subsubsection{Homogeneous Sat: Levels of evidence and logical dependencies}
\label{sec:instDiscussion--levels} 

A sentence is a model of a \req\ to a product, and there are different levels of assurance that a product conforms to a \req, \eg, safety critical \req s must have much stronger evidence of conformance. Hence, we refine the discussion above  by adding a category \L\ of {\em levels} of evidence and their \mor s, and label sentences by their required assurance levels so that the diagram below commutes (recall that pullbacks provide products in slice \caties)
\begin{equation}\label{eqdiag:inst:Levels-of-evidence}
	% https://q.uiver.app/#q=WzAsNSxbMSwwLCJcXG1vZGVscyJdLFswLDEsIlxcTW9kY2F0Il0sWzIsMSwiXFxTZW5jYXQiXSxbMywwLCJcXEV2aWNhdCJdLFs0LDEsIlxcTCJdLFswLDMsInBfRSJdLFswLDEsInBfTSIsMl0sWzAsMiwicF9TIiwyXSxbMyw0LCJcXGVsbFh7RX0iXSxbMiw0LCJcXGVsbFh7U30iLDJdLFszLDIsIlxcdGltZXMiLDEseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzAsMTAsIlxcZWxsc2F0IiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjEwfSwibGV2ZWwiOjEsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMCw0LCJcXHRleHR7W3BiXX0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
	\begin{tikzcd}[ampersand replacement=\&,column sep=small,row sep=normal]
		\& \models \&\& \Evicat \\
		\Modcat \&\& \Sencat \&\& \L
		\arrow["{q_E}", from=1-2, to=1-4]
		\arrow["{p_M}"', from=1-2, to=2-1]
		\arrow["{q_S}"', from=1-2, to=2-3]
		\arrow["{\ellX{E}}", from=1-4, to=2-5]
		\arrow["{\ellsen}"', from=2-3, to=2-5]
		\arrow[""{name=0, anchor=center, inner sep=0}, "\times"{description}, dashed, tail reversed, from=1-4, to=2-3]
		\arrow["q_\vDash"{description}, shorten >=5pt, dashed, from=1-2, to=0]
		\arrow["{\text{[pb]}}"{description}, draw=none, from=0, to=2-5]
	\end{tikzcd}
\end{equation}
Thus, a Sat becomes a binary span \spanrar{\models}{\Modcat}{\Sencat\timm_L\,\Evicat}. We will denote this product \caty\ by \eSencat\ and call its objects {\em e-sentences}. 


==> sections/future/piece--assuranceLevelsContd-2.tex <==
  \begin{mygroup}
	\renewcommand{\Sencat}{S}
	\renewcommand{\Modcat}{M}
	\renewcommand{\Evicat}{E}
	\begin{equation}
		% https://q.uiver.app/#q=WzAsNSxbMSwwLCJcXG1vZGVscyJdLFswLDEsIlxcTW9kY2F0Il0sWzIsMSwiXFxTZW5jYXQiXSxbMywwLCJcXEV2aWNhdCJdLFs0LDEsIlxcTCJdLFswLDMsInBfRSJdLFswLDEsInBfTSIsMl0sWzAsMiwicF9TIiwyXSxbMyw0LCJcXGVsbFh7RX0iXSxbMiw0LCJcXGVsbFh7U30iLDJdLFszLDIsIlxcdGltZXMiLDEseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJhcnJvd2hlYWQifSwiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzAsMTAsIlxcZWxsc2F0IiwxLHsic2hvcnRlbiI6eyJ0YXJnZXQiOjEwfSwibGV2ZWwiOjEsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dLFsxMCw0LCJcXHRleHR7W3BiXX0iLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
		\begin{tikzcd}[ampersand replacement=\&,column sep=small,row sep=normal]
			\& \models \&\& \Evicat \\
			\Modcat \&\& \Sencat \&\& \L
			\arrow["{p_E}", from=1-2, to=1-4]
			\arrow["{p_M}"', from=1-2, to=2-1]
			\arrow["{p_S}"', from=1-2, to=2-3]
			\arrow["{\ellX{E}}", from=1-4, to=2-5]
			\arrow["{\ellsen}"', from=2-3, to=2-5]
			\arrow[""{name=0, anchor=center, inner sep=0}, "\times"{description}, dashed, tail reversed, from=1-4, to=2-3]
			\arrow["\ellsat"{description}, shorten >=5pt, dashed, from=1-2, to=0]
			\arrow["{\text{[pb]}}"{description}, draw=none, from=0, to=2-5]
		\end{tikzcd}
	\end{equation}
where nodes and arrows are objects and \mor s  of an arbitrary \caty\ \CC. An abstract setting will make them more transparent. Then we will return to categorical institutions with \CC\ being \catcat.  Although for our constructs, it is sufficient to require \CC\ to have pullbacks, we will assume \CC\ to be finitely complete \caty\ (FCC) as
some of the constructs  can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcat_\CC$. Moreover, we need the abstract setting to clarify working with institutions in \catcat, and the latter does have products.   
%\input{sections/piece--institution-as-4tuple}

%---

\begin{defN}[Sat-base]\label{def:satBase}
	A {\em  %verified institution 
		base} is a triple  $(\CC, \CCmod, \CCsen^\e)$ of  of a finitely complete \caty\ (FCC)  \CC,
	its sub\caty\ $\CCmod\subset\CC$  of {\em collections of models} (think of \caties\ \Modcat\ above), and an {\em assurance} structure $\CCsen^e=(L, \CCsen, \ellE)$, where $L\in\Ob\CC$ is an object  of {\em levels} (of required evidence), $\CCsen\subset \CC/L$ is a \caty\ of{\em collections of labelled sentences}, and an arrow $E\xrightarrow{\ellX{\E}}L\; \in\CC/L$ provides an object $\E$ of {\em (labelled) pieces of evidences}. We will write an object of \CCsen\ as a pair  $(S, \ell_S)$, in which \ellX{S} is to be thought of as a mapping providing logical sentences with their required levels of assurance; then a \mor\ in $\CC/L$, \ie, a commuting triangle $f.\ell'=\ell$, is written as \frar{f}{S}{S'}. Similarly, arrow \ellE\ will be referred to by \E. 
	
	We will write $(\CC,L,E)$ for a base with $\CCmod=\CC$ and $\CCsen=\CC/L$ (and arrow  \frar{\ellE}{\E}{\L} is assumed by default). 
	%; such a base is just a pointed arrow  \caty\ $(\arrowcatCC,\ellE)$. % (or to shorten notation if the subcategoires are not under discussion). 
	%To ease notation, we will often refer to such a base as to a pointed \caty\ $(\CC, L)$, and 
	We denote objects of $\CCmod$ and $\CCsen$ by $M, M', ..$ and $S, S',...$ resp.   (labelling arrows \ellX{S}, \ellX{S'} etc are assumed by default) and omit explicit mentioning of \caties\ they belong.  
\end{defN}
\end{mygroup}


\begin{example}
	The institution theory is developed over the base $(\Catcat, \tcat, \tcat)$ with $\ellE=\id_\tcat$.  
\end{example}

\begin{defN}[eSats: Sat-spans with evidence]\label{def:esatSpan}
	Recall that any slice \caty\ has products defined by pullbacks, and let $S\timm_L \E$ be such for a sentence object $S\in\Ob\CCsen$. 
	
	A {\em  \satty\ span with evidence} ({\em eSat})  over base \satbaseX{\CC}  is a span 
	$M\xleftarrow{p}\;\vDash\;\xrightarrow{q}S\timm_L \E$ or 
	\spanrar{\Dashv}{\S\timm_L \E}{\M} (\ie, we denote the spans and its apex by the same symbol). 
	%  not needed now!
	If objects $S$ and $M$ in a diagram are placed with $S$ on the right of  $M$, we will denote the same data (\ie, $q$ points to $S\timm_L\, \E$ and $p$ to $M$) by using more customary symbol $\vDash$ rather than $\Dashv$ (but note that the span-as-arrow goes into $M$ in both cases). %$\vDash_{MS}$ but directed as \spanlar{\vDash_{MS}}{M}{S}. 
	
	If a triple of elements \frar{(m,s,e)}{\tcat_\CC}{\M\timm\S\timm\E} factors through $\vDash$, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $s$  as {evidenced} by a {\em (piece of) evidence} $e$ 
	%{\em verified assurance of level} $e$,  
	and write $m\satUD{e}{}s$.  
	
	We require e-\satty\ to be invariant under iso\mor s: for any iso\mor s \frar{i_X}{X}{X}, 
	where $X\in\{\M, \S, \E\}$ (in the corresponding \caty), there is a \CC-iso\mor\ \frar{i}{\vDash}{\vDash} such that $p_X.i_X =i.p_X$ with $X\in \{M, S, E\}$.  %and $e.i_\L=i.e$. \qquad \qquad \qquad.  
\end{defN}

It is easy to see that the assurance structure diagram \cref{eqdiag:inst:Levels-of-evidence} on p.~\pageref{eqdiag:inst:Levels-of-evidence} for an institution is instantiated for a $G\in\Ob\GG$ by taking \slicecatdeltaGGG\ as \Modcatsig\ and arrow $\liftedX{\ok_G}.v$ ( see diagram \cref{eqdiag:cattyDiag2--withOk} where such arrow is shown for $G'$), 
\slicecatcsigGGG\ as \Sencatsig\ and arrow $\liftedX{\ok_G}.h$ as $q_\senind$ while 
arrow \frar{\ellX{G}}{\slicecatcsigGGG}{\carrop{\csig}} (see \cref{eqdiag:mainThProof-chasing}) as labelling \frar {\ellsen} {\slicecatcsigGGG}{\L}.
Finally, arrow \frar{\ellE}{\E}{\L} in diagram \cref{eqdiag:inst:Levels-of-evidence} is instantiated by functor \frar{\ellsig}{\Instcatsig}{\carrop{\predsig}}, 
and $q_E$ in \cref{eqdiag:inst:Levels-of-evidence} is $\liftedX{\#}_G$ in the right part of  \cref{eqdiag:cattyDiag3--withOk}

==> sections/future/piece--assuranceLevelsContd.tex <==

In addition, we now want to consider labelled sentences and functor $f_*$ to respect it. We thus require  
$f^\ell_*(\phi, l) = (f_*(\phi), l)$, where $(\phi, l)$ is a labelled sentence and $f_*^\ell$ denotes our new labelling-aware substitution.  Now sat-axiom becomes eSat-axiom specified below:
\begin{equation}\label{eqdiag:eSatAxiom}
	\begin{array}{c@{\quad}c} %c}
	\esatAxiomNew
	&
	\begin{array}{c} % iff statement 
		f^*(m') \modelssig^e (\phi, l)
		\\ [5pt]\text{iff}\rule{0ex}{1.ex}
		\\ [5pt] m' \modelssigPrim^e \ (f_*(\phi), l)
	\end{array}
\end{array}
\end{equation}
Our goal in the rest of the section is to enrich the notion of institution with evidence and make it fully categorical with non-trivial arrows in all ingredients, which model their updates. We will begin with an abstract element-free \fwk, whose ingredients are objects and arrows of some \caty\ \CC\  (\cref{sec:vInst-abstract}) and then consider concrete evidential institutions, whose ingredients are \caties\ and functors (\cref{sec:vInst-concrete}). 


==> sections/genGraphs.tex <==
%\renewcommand{\HH}{\enma{H}}
\subsection{Generalized Graphs}\label{sec:genGraphs}
%The rationale  behind this terminology is due to arguably the most import representative: \emph{directed multigraphs}.
As our discussion in Sect.2 suggests, we need a very general notion of graphs as presheaves  \frar{G}{\II}{\setcat} for a suitable schema category $\II$. In all our applications, graphs have \hical\ structure that allows their traversal from the top elements to the bottom. 
%our with the only restriction is an arbitrary but fixed finite category whose objects are called {\em cell types}, and for object $H\in\HH$, elements of set $G(H)$ are called $G$'s {\em cells of type $H$}. 
For example, ordinary directed multigraphs are given by schema $\II=\Graph$ with $\Ob{\Graph}=\{\nfont{Node},\nfont{Arrow}\}$ and two non-identity arrows \frar{\so,\ta}{\nfont{Arrow}}{\nfont{Node}} so that object \nfont{Arrow} is above \nfont{Node}
\shortlong{Other examples can be found in the TR.
}{
	(Below we will show other examples below.)}
Hence, we require category \II\ to be \hical\ in the folloiwng sense. 

\subsubsection{Hierarchical categories}
\zdzd{I'll write a short motivating piece later}
\begin{mydef}[Hierarchical categories]\label{def:hcat}
	We consider a natural number $N$ as a category 
	$$\NN= \{ 0\rightarrow 1\rightarrow \ldots\rightarrow (N-1)\}$$
	consisting of $N$ objects and $N-1$ non-identity arrows.%
	\footnote{The reason we start counting at 0 rather than 1 is to make the generalization for the first infinite ordinal $\omega$ straightforward: category $\ovr{\omega}$ has all natural numbers $n<\omega$ as objects.} 
	
	A {\em \hical\ category (\hcaty\ {\em in brief}) of height $N$} is given by a small category \HH\ along with a surjective on objects functor \frar{\heifun}{\HH}{\NNop} so that all {\em layers} $\HH_n=L_n(\HH)=\heifun^{-1}(n)$ for $n<N$ are not empty.  We refer to $N$ by $\Hei(\HH)$. Note that if $N=0$, then category \NN\ is empty and we have an empty \hical\ \caty\ of height 0. Thus, $\HH=\varnothing$ iff $\Hei(\HH)=0$. 
	% 	, then all layers $L_{n'}(\HH)$, $n<n'<N$, are empty as well. We call a natural number $\Nact=\nfont{max}\compr{n<N}{\HH_n\noteq\varnothing}$ the {\em actual} height of \HH\ (in contrast to the {\em nominal} height $N$). 
	
	Moreover, the following {\bf\em acyclicity} condition holds for any two objects $x,y$ in \HH: if $\HH(x,y)\noteq\varnothing$, then either $\heifun(x) >\heifun(y)$ or $x=y$, but in the latter case we require $\HH(x,x)=\{\id_x \}$. Thus, all \HH-arrows go down from higher to lower layers, and the only arrows within a layer are identities. 
	\zdzd{there was also the Parenting condition but it is now commented in the text}
	%b) Parenting. For any $0<n$ %with $C_n\noteq\varnothing$ 
	%and any $x\in C_n$, the set $\HH(x,\_)$ is not empty. Elements of set $\prt(x)\eqdef\compr{\cod(f)}{f\in\HH(x,\_)}$ are called $x$'s {\em parents}. Moreover, we require $\max\compr{\heifun(y)}{y\in\prt(x)}=n-1$ (otherwise object $x$ is to be moved into another layer). 
	%
	For an h-\caty\ \HH, we call elements of layer $L_n(\HH)$ {\em n-cell types} or {\em n-(hyper)edge  types} and typically denote them by $H$. We will also call 0-cell types  {\em node types}. % and $(n>0)$-cells  {\em arcs}. 
\end{mydef}
%\begin{mycor}\label{cor:hcat}\zd{could be strengthened?}
%	If category \HH\ is \hical, then $\Arr{\HH}=\bigcup_{H\in\HH_0}\HH(\_,H)$
%\end{mycor}
\begin{mycor}\label{cor:hcat}
	If \HH\ is an h-\caty, then for any $n<N$, the full subcategory $\HH_n\subset\HH$ generated by objects of height less than $n$ is a h-\caty\ as well. We have a cumulative chain of h-\cats
	$$%\varnothing=
	\HH_0 \subset \HH_1 \subset\ldots\subset\HH_{N-1}=\HH
	$$
	and for any object $H\in\HH$, $\heifun(H)=\nfont{min}\compr{n}{H\in\HH_n}$.
\end{mycor}
\begin{mydef}[Discrete h-\cats]\label{def:hcat-disc}
	A \hical\ \caty\ is called {\em discrete} if its only arrows are identities. However, a discrete \hcaty\ is more than a set: it is a set equipped with a height function, \ie, a layered set  $\HH=\bigcup_{n<N}L_n(\HH)$. We will also write $L_{\le n}(\HH)$ for the set $\bigcup_{0\le i\le n}L_i(\HH)$
\end{mydef}
\begin{mydef}[Finitary hierarchical categories]\label{def:hcatfin}
	A \hcaty\ is called {\em finitary} if for any object $x$ the set $\HH(x,\_)$ is finite. \sizeXno{In this paper, we will assume all \hcats\ to be finitary.} 
\end{mydef}
\begin{mycor}[Finite h-\cats]
	\label{cor:finiteHCats}
	A finitary  \hcaty\ \HH\ is finite as soon as its object set $\Ob{\HH}$ is finite
\end{mycor}
\begin{myrem}[Finitarity conditions]\label{rem:finty}
	\defref{hcatfin} is the first in the family of similar definitions, which require finiteness of some construct assigned to the notion at hand. If an h-\caty\ \HH\ is finite, then it is finitary, but the converse is obviously not true, and we will often deal with infinite but finitary objects (signatures, sketches, graphs). 
\end{myrem}

%%%%%%%
%====> end of renew command for \HH
%%%%%%%%%%%

%Recall that  {\em a sieve} on an object $X$ in a category \CC\ is a subset $S_X\subset\CC(\_,X)$ closed under precomposition: if $f\in S_X$, then $x\comp f \in S_X$ for any arrow $x$ in \CC. Similarly, a {\em cosieve} is a set $cS_X\subset\CC(X,\_)$ closed under postcomposition.
%\begin{mylem}  
%\end{mylem}
\begin{mydef}[Graphs]
	\label{def:hgraph}
	Let \II\ be an \hcaty. An {\em \II-graph} is a functor \frar{G}{\II}{\setcat}, \ie, a presheaf over {\em schema} \II. We will normally refer to such functors as merely graphs, but if we want to stress their distinction from ordinary directed multigraphs (which are functors \frar{G}{\Graph}{\setcat} over schema specified in \eqref{schema4graphs}), we will refer to them as \II-graphs or, sometimes, as 'graphs' in single quotes. 
%	\begin{equation}\label{eq:schema4graphs}
%	\begin{tabular}{c}
%	$	\xymatrix{
%		\nfont{Node} 
%		& \nfont{Arrow} \ar@/^4pt/[l]^{\ta}\ar@/_4pt/[l]_{\so}	
%	} $
%	\\
%	Schema \Graph\ for ordinary (directed multi-)graphs
%	\end{tabular}
%	\end{equation}
	For a graph \hgrarr, elements of set $G(H)$ with $H\in\II_n$ are called {\em n-cells (of type $H$)}, and if $\II_n$ is not a singleton, we say that $n$-cells are multi-sorted. We write $\Elem{G}$ for the set $\bigcup_{H\in\Ob{\II}}G(H)$. 
	
	The presheaf topos of all \II-graphs will be denoted by \GG, and we assume that throughout the paper the schema \II\ is arbitrary but fixed. A graph $G$ is {\em finite} if $\Elem{G}$ is finite.  All finite graphs form a (sub)category (of \GG) denoted by $\GGfin$. \zdzd{we can replace $\GGfin$ by $\GG_\mathsf{fin}$ to make it less sexy.}
\end{mydef}
We will try to depict 'graphs' as graphical objects. For example, if object $H\in \II$ has exactly two non-looping outgoing arrows, say, $x,y$, we will call them {\em source} and {\em target}, and depict each element $a\in G(H)$ as an arrow from element $a.G(x)$ to element $a.G(y)$. %If $I \in \cat{I}$ has no other outgoing morphisms than the identity $\identity{I} : I \to I$, we call elements $x \in G(I)$ \emph{nodes} otherwise \emph{edges} or \emph{arcs}.
%\zdhll{If there exists a morphism $\arrow{I}{j}{J} \in \II$ and $J$ has outgoing non-identity morphisms we further call an element $x \in G(I)$ a \emph{hyperedge}.}{to be checked}{-7}

\zdzd{hm, most probably, to give the name 'graph' more intuitive sense, we need to pose some conditions on \II, say, require \II\ to be a rooted dag, whose root is called \Node, children are different sorts of 1-hyperesges, then we will have 2-hyper-edges, etc. Binary hyperedges (exactly two arrows to the parents) are called arrows. ...I guess having such a structure would be very useful for parsing, but maybe it's even necessary for parsing?? If so, then parsing would be a much nicer result. I once came to having some structure over \II\ when thinking about equations as a result of parsing.}

%\mkRemark{Presheaf notation}{rem:presheaf}
\begin{myexa}[Fancy Graph]
	\label{exa:samplepresheaf}
	Assume $\II$ is the category in \figref{exgraph}(a) (identities omitted):
	and \figref{exgraph}(b) depicts a graph given by the following functor $G : \II \to \catSet$:
	\begin{align*}
	G(\Node) =  &\{P, Q, A, B\}  
	&  	G(\so_{_\text{@2-\Edge}}) =  \alpha \mapsto f \\
	G(\Edge) = &\{f,g,i\}  %\text{~(three edges)~}
	& 	G(\ta_{_\text{@2-\Edge}})  = \alpha \mapsto g \\
	G(\text{2-\Edge}) =& \{\alpha\}  & G(\ta_1) =  m \mapsto A \\
	G(\mathsf{HEdge}) = & \{m\} & G(\ta_2) =  m \mapsto B \\
	G(\so_{_\text{@\Edge}}) = &\{f \mapsto A, g \mapsto A, i \mapsto Q \}& G(\ta_3) =  m \mapsto P  \\
	G(\ta_{_\text{@\Edge}}) =  & \{f \mapsto B, g \mapsto B, i \mapsto Q\} & G(\ta_4) =  m \mapsto Q \\
	\end{align*}
	%The example exemplifies different features graphical features. 
	Elements of $G(0)$ can be called nodes, elements of $G(1)$ and $G(2)$ can be visualized as arrows (since the respective object in $\II$ has exactly two outgoing non-identity morphisms.
	There is an edge between edges, $\alpha$,  and a hyperegde $n$ connecting four elements (``sources'' of the hyperedge) as shown (as the respective object in $\II$ has more than two outgoing non-identity morphisms).
	Lines connecting a hyperedge to its sources  will be called \emph{tentacles}.
	%}
\end{myexa}
\begin{figure}[h]
	\centering
	%\begin{subfigure}[b]{0.49\linewidth}
	\subfloat[Metaschema for `graphs']{
		\parbox{0.45\linewidth}{
			$\xymatrix @C=1em @R=3em {
				& \Node & \\
				\mathsf{HEdge}_{} \ar@/^1.7pc/[ur]^{\ta_1} \ar@<0.5ex>[ur]^{\ta_2} \ar@<-0.5ex>[ur]_{\ta_3} \ar@/_1.7pc/[ur]_{\ta_4} 
				& & &\Edge \ar@<-0.5ex>[ull]_{\ta} \ar@<0.5ex>[ull]^{\so}  %\\
				&& \text{2-{\sf Edge}} \ar@<-0.5ex>[ll]_{\nfont{\ta}} \ar@<0.5ex>[ll]^{\nfont{\so}}
			}$
		}
	}\quad
	\subfloat[A sample `graph' $G$ (an instance of $S$)]{
%%%%{		\centering
\parbox{0.45\linewidth}{\centering
		\includegraphics[width=0.95\linewidth]{figures/Presheaves}
}
}
	\caption{Example of a higher-order graph
\zd{\large a) fix subcaption (b) way below (a) :replace "subflost" by tabular -- then I can control everything}	
\\ \zd{consider joining $\ta_{1,2}$ into a span, say,  $\ta_{12}$, then node $P$ is to be renamed into, say, $B$, while $B$ is to be renamed into, say, $P$, so that the hyperedge $h$ would include set $\{A,C\}$ at the filed name $\ta_{12}$. Then $Q$ is to be renamed into, say, $X$.}
}
	\label{fig:exgraph}
\end{figure}
%\subsubsection{Complements in h-graphs}
%\label{sec:complement}  
%\end{includeLong}


==> sections/hypercat-stuff.tex <==

\subsection{Hypercat structure? }

Our next goal is to build an sm-category from DOI-sketches.
To do this we employ the idea of \emph{decorated cospans} \cite{Fong2015} since DOI-sketches (Def.~\ref{def:doigraph}) already provide us with a cospan and recite the central notion below:

\newcommand\decfun{\enma{\mathit{Dec}}}
\newcommand\dectra{\enma{\delta}}

From now on, we assume that our signatures of operation symbols are finite. (Or another finiteness condition is to be assumed to avoid size problems below.)
\begin{mydef}{decoratedCospan}{Decorated Cospans}
Let $\cat{C}$ be a category with finite colimits, and $(\decfun, \dectra) : (\cat{C}, +) \to (\catSet, \times)$
be a \textcolor{red}{LAX} symmetric monoidal functor (see \defref{smfunctor} in Appendix~\ref{sec:smcs}) called the {\em decoration} functor.
An {\em ($\decfun$-)decorated cospan} is a pair consisting of a cospan $A \xrightarrow{i} N \xleftarrow{o} B$ in $\cat{C}$ together with an element $s \in \decfun(N)$ called the {\em decoration}.
%We call $(\decfun, \dectra)$ the decoration functor and $s$ the decoration.
\end{mydef}
Consider forgetful functor $$\frar{F_\opsig}{\skecatgpo}{\skecatgp}$$ that strips an operational sketch over $(\opsig,\predsig)$ of its \opsig-diagrams (see \eqref{forgetfultriangle} on p.\pageref{eq:forgetfultriangle}  above). It gives rise to an inverse  mapping
$$\flar{\decfun_\opsig}{\Ob{\catSet}}{\Ob{\skecatgp}}$$ that assigns to any predicate \predsig-sketch $S$, the SET of all possible operational sketches over it:
$$
\decfun_\opsig(S) =\comprcolon{\opske\in\Ob{\opskecatgpo}}{F_\opsig(\opske)=S}
$$
It is easy to see that an DOI-sketch in the signature \opsig\ (over \predsig) is nothing but a $\decfun_\opsig$-decorated cospan. Hence, to make the decorated cospan \fwk\ applicable, we need to find the comparison \trafon\ $\delta_\opsig$ and prove that 
$$
\frar{(\decfun_\opsig, \delta_\opsig)}{(\skecatgp,+)}{(\catSet,\times)}
	$$
	 is a lax sm-functor.   

\clearpage
We provide the presentation how DOI graphs fit into the decorated cospan framework in two steps.
First, we will define a suitable decoration functor and afterwards reformulated the definition of DOI-sketches in terms of Def.~\ref{def:decoratedCospan}.
This requires a few technical definitions

\begin{mydef}{specialOSketchProps}{Operational sketch properties}
Let $\opsig$ be an operation signature over $\predsig$ and $S \in \skecatgpo $ a sketch w.r.t $\oppredsig$.
We define two functions
\begin{eqnarray}
	ins : \begin{cases}
	\catObj{\constr{S}} \to \powerset{\carrier{S}} \\
	c \mapsto \{ x \in \carrier{S} \mid x \in \image{\compose{IE_{\labell(c)}}{\bind}} \}
	\end{cases} \\
	outs : \begin{cases}
	 \catObj{\constr{S}} \to \powerset{\carrier{S}}  \\
	 c \mapsto \{ x \in \carrier{S} \mid x \in \image{\compose{OE_\labell(c)}{\bind}} \}
	\end{cases}
\end{eqnarray}
which, given a diagram $c \in \constr{S}$ with $\labell(c) \in \opsig$, returns a set of all carrier elements in the input and output scope respectively (for a diagram $c'$ with $\labell(c) \in \predsig$ it will just return the empty set).
Furthermore, we define a relation $\prec \subseteq \catObj{\constr{S}} \times \catObj{\constr{S}}$ that is defined on a pair $(c, c')$ iff. there exists an element $x \in outs(c) \cap ins(c)$. The transitive and reflexive close is denoted $\preceq$.

The sketch $S$ is said
\begin{itemize}
	\item to have \emph{no confusion} w.r.t. produced elements when every element is in the output scope of at most one operation diagram, i.e. for each $c, c' \in \constr{S}$ and any element $x \in outs(c) \cap outs(c')$ if follows that $c = c'$.
	\item to have \emph{no junk} w.r.t. a subgraph $G \subseteq \carrier{S}$ when for every additional element there exist an operation producing it, i.e. for each  $x \in \carrier{S} \setminus G$ there exists a diagram $c \in \constr{S}$ such that $x \in outs(c)$.
	\item to have \emph{no cycles} w.r.t. operation applications when every operation diagram does not depend on elements transitively produces by itself, i.e. $\preceq \subseteq \catObj{\constr{S}} \times \catObj{\constr{S}}$ is a partial order.
\end{itemize}
\end{mydef}

\zd{The def. above seems conceptually wrong: the three conditions look like as a reformulation of the notion of a DO-sketch defined above, that is, this def. should be a theorem that any DO-sketch also has properties above. Also, why you work with objects only? It's easy to see that for any $c\in Constr(S)$ such that $pred(c)\in\opsig$ we have the entire square diagram $\Square\rightarrow\skecatgp$ as explained in Lemma \ref{lem:atomicQuery}.  It all was written, or am I missing the point?
}
\begin{mydef}{opDecorator}{Operation Decoration}
	Let $\opsig$ be an operationg signature.
	We define a sm-functor $(\decorator, \phi) : (\skecatgp,+) \to (\catSet, \times)$ as follows:\par
	\textbf{Object mapping:} Let $S \in \skecatgp$ be a sketch, $\decorator$ assigns to $S$ a set $\{ S' \mid S' \in \skecat{\GG}{\oppredsig} \}$ for which
	\begin{enumerate}
		\item The carrier of each $S' \in \decorator(S)$ is equal to $S$, i.e. $\carrier{S} = \carrier{S'}$
		\item For each $S' \in \decorator(S)$, the diagrams of $S$ is a subobject of the diagrams in $S'$ added diagrams are mapped to operation symbols, i.e. $\constr{S} \subseteq \constr{S'}$ and for all $c \in \constr{S'} \setminus \constr{S}$ it holds $\labell(c) \in \opsig$.
		\item \label{item:opDecorationItem1} Every $S' \in \decorator(S)$ has no confusion.
		\item \label{item:opDecorationItem2} Every $S' \in \decorator(S)$ has no cycles.
	\end{enumerate}
	\textbf{Arrow mapping:} Let $S = (\carrier{S}, \constr{S})$ and $T = (\carrier{T}, \constr{T})$ be two sketches in $\skecatgp$ and $\arrow{S}{f}{T}$ be a sketchmorphism.
	\begin{equation}
		\decorator(f) : \begin{cases}
		\decorator(S) \to \decorator(T) \in \catArrows{\catSet} \\
		(\carrier{S'}, \constr{S'}) \mapsto (\carrier{f}(\carrier{S'}), \constr{T'})
		\end{cases}
	\end{equation}
	where $\constr{T'}$ is given by the pushout object in the following diagram:
	\begin{equation}
		\xymatrix{
		\constr{S} \ar[d]_{\constr{f}} \ar@{^{(}->}[r] & \constr{S'} \ar[d]^{\constr{f}^*} \\
		\constr{T} \ar@{^{(}->}[r] & \constr{T'}
		}
	\end{equation}
	To verify that this mapping is well-defined note that $\constr{T'}$ is a pushout object, thus every diagram $c$ in $\constr{T'}$ either stem from $\constr{T}$ or $\constr{S'}$ (or both). If it stems from $\constr{T}$ is must be necessarily mapped to a predicate, i.e. $\labell(c) \in \predsig$, and thus unaffected by \ref{item:opDecorationItem1} and \ref{item:opDecorationItem1}. If it stems from $\constr{S'}$ note that $S$ has to already fulfill  \ref{item:opDecorationItem1} and \ref{item:opDecorationItem1} by the definition of $\decorator$ on object. \par
	\textbf{Coherence Maps:}
	The value of $\phi_{\boldsymbol{I}}$ is the empty sketch $(\emptyset, \emptyset)$ since there are elements that operation diagrams can be bound to.
	\PAST{We may need the requirement that the scope of an operation must not be empty.}
	The definition of the coherence maps w.r.t. monoidal product is straighforward and it is easy to see that it is both well-defined and compatible with associators, unitors, and symmetries.
	\begin{equation}
		\phi_{S,T} = \begin{cases}
			\decorator(S) \times \decorator(T) \to \decorator(S + T) \\
			( (\carrier{S}, \constr{S}), (\carrier{T},\constr{T} ) \mapsto ( \carrier{S} + \carrier{T}, \constr{S} + \constr{T} )
		\end{cases}
	\end{equation}
\end{mydef}

This functor is indeed a decoration in a sense that it takes a sketch $S$ over $\predsig$ as input and produces the set of all sketches over $\oppredsig$ that can be produced by adding arbitrary operation diagrams to $S$ obeying the no-confusion and no-cycle properties.

\begin{mydef}{doiDecorated}{DOI-graphs as Decorated Cospan (Reformulated)}
A DOI graph is given by a cospan $I \overset{i}{\hookrightarrow} K \overset{o}{\hookleftarrow} O$ of monomorphism in $\skecatgp$ and a sketch $S \in \decorator(K)$ (the decoration) obeying 
\begin{enumerate}
\item \label{item:noJunkDOI} $S$ has no-junk w.r.t. $I \subseteq K$.
\end{enumerate}
\end{mydef}

Not that the no-junk condition in Def.~\ref{def:doiDecorated} and the no-confusion condition imposed by $\decorator$ ensure conditions a) and b) in Def.\ref{def:dograske} to hold. 
And the no-cycle condition imposed through $\decorator$ directly implies c) in Def.\ref{def:dograske}.
Thus, Definitions \ref{def:doiDecorated} and \ref{def:doigraph} are equivalent.

\mkTheorem{Composition of DOI-graphs (Definition~\ref{def:doiDecorated}) }{theo:wellDefined}{
DOI graphs can be composed via pushouts.
}

\begin{proof}
Let $(I_l \overset{i_l}{\hookrightarrow} K_l \overset{o_l}{\hookleftarrow} O_l, S_l \in \decorator(K_l))$ and $(I_r \overset{i_r}{\hookrightarrow} K_r \overset{o_r}{\hookleftarrow} O_r, S_r \in \decorator(K_r))$ be two DOI-graphs.
\begin{equation}
\xymatrix{
	& & K \ar@{}[dd]|{(1)} & & \\
	& K_l \ar[ur]^{u} & & K_r \ar[ul]_v & \\
	I_l \ar@{^{(}->}[ur]^{i_l} &  & O_l = I_r \ar@{_{(}->}[ul]_{o_l} \ar@{^{(}->}[ur]^{i_r} & & O_r \ar@{_{(}->}[ul]_{o_r} 
}
\end{equation}
Consider the diagram above where (1) is given by pushout.
Since $\skecatgp$ is a topos and thus adhesive and pushouts therefore preserve monomorphisms $u$ and $v$ are both mono and can be chosen as inclusions.
Therefore, we get a composite $I_l \overset{\compose{i_l}{u}}{\hookrightarrow} K \overset{\compose{o_r}{v}}{\hookleftarrow} O_r$.
The decoration object $S \in \decorator(K)$ for thus cospan is produced by $S = \decorator([u,v])(\phi_{K_l,K_r}(S_l,S_r))$.
It remains to show that is satisfies \ref{item:noJunkDOI}.
We will proof this by contradiction and assume there is an element $x \in \carrier{K} \setminus I$ such that there is no $c \in \constr{S}$ with $c \in outs(c)$.
Because $K$ is a pushout object and the hypothesis it most hold that $x \in \carrier{K_r}$ and further $x \in \carrier{I_r}$ because of the no-junk property of the right DOI-graphs co-span.
The element must have an image under $\carrier{o_l}$ denoted $x'$ and because of the no-junk property of the left DOI co-span there most be some diagram $c' \in \constr{S_l}$ such $x' \in outs(c')$. 
The sketch morphism $\arrow{S_l}{\decorator(u)}{S}$ must preserve the definedness of this diagram which however contradicts the hypothesis.
\end{proof}


\endinput
Finally, we want to return to a more abstract level and put our work in context with other recent trends in Applied Category Theory, namely SMCs and String Diagrams, cf. Appendix \ref{sec:smcs}.
We mentioned earlier that diagrammatic queries, i.e. DO-graphs or equivalently DO-workflows, are the diagrammatic equivalent of a term.
Thus, they could be represented as a category.
\begin{mydef}{intervalSketches}{Predicate Interval Sketches}
Let $\predicateSig$ and $\mathcal{Q}$ be two predicate signatures and let $\predicateSig$ be a subcategory of $\mathcal{Q}$.
We define a category $\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$:
Its objects being all sketches $S \in \skecat{\GG}{\predicateSig'}$ for any predicate signature $\predicateSig'$ such that  $\predicateSig \subseteq \predicateSig' \subseteq \mathcal{Q}$.
A hom-set $\homset{\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}}{S}{S'}$ for objects $S \in \skecat{\GG}{\predicateSig'}$ and $S' \in \skecat{\GG}{\predicateSig''}$ contains all $\skecat{\GG}{\predicateSig'}$ between $S$ ans $S'$.
\end{mydef}

\mkProposition{Initial objects in $\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$}{prop:initialObjectsIntervalSkeCat}{
$\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$ has an initial object $\boldsymbol{0}$.
Its carrier $\carrier{\boldsymbol{0}}$ is the initial object $\emptyset$ in $\GG$ and its diagrams $\constr{\boldsymbol{0}}$ is the empty category.
}
\begin{proof}
Obviously there is a unique morphism into every object of $\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$, which immediately arises from the initial object properties of carrier and constraints in $\GG$ and $\catCat$.
\end{proof}

\mkProposition{Pushouts in $\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$}{prop:pushoutIntervalSkeCat}{
$\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$ has pushouts for every span of $\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$ -morphisms.
}
\begin{proof}
\PAST{TODO}
\end{proof}

\mkProposition{$\intervalskecat{\GG}{\predicateSig}{\mathcal{Q}}$ is adhesive}{prop:intervalSkeCatAdhesive}{
	See Appendix \ref{sec:dpo}.
}
\begin{proof}
	\PAST{TODO: Show existence of pullbacks along monos and Van-Kampen property}
\end{proof}

\begin{mydef}{doGraphCoSpan}{DO-graph Co-Span representation}
Every DO-graph $D$ according to Def.\ref{def:doGraph} is actually a co-span of inclusion morphisms in $\intervalskecat{\GG}{\predicateSig}{\oppredsig}$ where the apex is subject to the additional conditions \ref{enum:doGraphCond1} and \ref{enum:doGraphCond2} in Def.\ref{def:doGraph}.
\end{mydef}


\mkProposition{DO-graph composition}{prop:doGraphComp}{
Let $D$ and $E$ be two DO-graphs represented as co-spans, cf. Def.\ref{def:doGraphCoSpan} where $\doGraphOutput{D} = \doGraphInput{E}$.
We can define their composite $\compose{D}{E}$ with co-span composition by pushouts and the result is a DO-graph:

}
\begin{proof}
Due to proposition \ref{prop:pushoutIntervalSkeCat} the square (1) exists, yielding $u$ and $v$.
Due to proposition \ref{prop:intervalSkeCatAdhesive}, the pushout (1) preserves monomorphisms such that $u$ and $v$ are monic and since pushouts are determined up to isomorphism, we can chose $u$ and $v$ as inclusions.
It remains to show that the conditions  \ref{enum:doGraphCond1} and \ref{enum:doGraphCond2} from Def.\ref{def:doGraph} are fulfilled.
\PAST{The latter is a TODO}
\end{proof}

\mkProposition{DO-graph category}{prop:doGraphCat}{
For any predicate signature $\predicateSig$ and $\operationSig$, there exists a category $\doGraphCat{\predicateSig}{\operationSig}$ whose objects are sketches in $\intervalskecat{\GG}{\predicateSig}{\operationSig}$ and arrows are DO-graphs.
}
\begin{proof}
Unitality and Associativity are immediately given because pushouts preserve identities and their application is associative.
\end{proof}

The equivalence of DO-graphs and DO-workflows lifts to the categorical level:

\mkCorollary{$\doGraphCat{\predicateSig}{\operationSig} \equiv \doWFCat{\predicateSig}{\opsig}$}{corr:dogDowEquiv}{
The parsing-mapping from Theorem~\ref{theo:parsing} extends to an identity on objects functor which is an equivalence.
}

\mkTheorem{$\doGraphCat{\predicateSig}{\opsig}$ is a hypergraph category}{theo:hypergraphCat}{}
\begin{proof}
Follows immediately from propositions \ref{prop:initialObjectsIntervalSkeCat}, \ref{prop:pushoutIntervalSkeCat} and \ref{prop:doGraphComp}.
\end{proof}

This last theorems allows us to interpret diagrammatic queries in a SMC, which can be visualized as a String Diagram.


\begin{mydef}{termalg}{Term Algebra}
	Given a sketch $X$ of {\em variables} and an operation signature \opsig, we build...
\end{mydef}
\mkTheorem{Term Algebra Adjunction}{theo:adjunction}{
	There is an adjunction $\mathsf{T} \dashv \mathsf{U}$ with $\mathsf{U}: \catOpsigAlg{\skecatgp}{\opsig} \to \skecatgp$ being the (forgetful) projection on the underlying carrier and $\mathsf{T}: \skecatgp \to \catOpsigAlg{\skecatgp}{\opsig}$ being the (free) term algebra functor over a sketch.
}
\begin{proof}
	Was basically given in \cite{WolterDiskinK2018}.
	\PAST{We have to adapt it to the slightly changed situation, though.}
\end{proof}

\zd{Oops: at this point, we are very far from this result. We need first to define what is a term=complex query over a sketch $X$, and show that the set of all terms over $X$ is an \opsig-algebra $T_\opsig(X)$. Then we need to show that the mapping $X\mapsto T_\opsig(X)$ is functorial (and I expect it could be a hassle). Only after that we are ready to prove that there is an adjunction.}

==> sections/injectivity.tex <==
\clearpage
\renewcommand{\Ob}{\enma{\mathsf{Ob}}}
\renewcommand{\tauu}{\enma{\phi}}
\subsection{Injectivity and lifting constraints:  Diagrammatic implementation of diagrammatic constraints}
\label{sec:diagImpl}

%A distinctive feature of the \fwk\ defined above is its two-level nature 

The main goal of this section is to show that lifting constraints introduced by Spivak \cite{spivak-lifting14} are an instance of the classical idea of injectivity. It is almost obvious once you know both definitions but despite the technical equivalence, there is a conceptual distinctions that is useful to discuss in detail. We will begin with a very brief introduction of injectivity; then we proceed to lifting and its equivalence to injectivity. % to the equivalence between the two constructs. 

Injectivity is a far reaching generalization of regular logic, whose sentences are built according to the pattern $\forall \bar x (P(\bar x) \rightarrow \exists \bar y Q(\bar x, \bar y))$. Such an implication is modelled  by a \mor, and sets of variables $\bar x$ and $\bar y$ are \mor s too (the idea goes back to Banashewsky and Herrlich's work on quasi-implications and quasi-variaties in universal algebra \cite{?}). \cref{sec:injectivityPrimer} provides some basics, including the main definition of injectivity-as-satisfiability relation $\modelsInjX{\CC} \subset \Ob\CC \times \Arr\CC$ for any \caty\ \CC. %,  $A\modelsInjX{\CC} a$,  for an object $A\in \Ob \CC$ and arrow $a\in \Arr\CC$ in a \caty\ \CC. % w.r.t arrow $f$ in a category by an object $A$ of that category, .
\begin{defN}[Regular constraints]Let \GG\ be an arbitrary category (of 'graphs').
	A constraint $(c,G_c, \semm{c})$ is called {\em regular} if its semantics $\semm{c}\subset \Ob (\GG/G_c)$ can be specified as injectivity over a suitable $\GG/G_c$ arrow \tauu, \ie, $t\models c$  iff $t\modelsInjX{\GG/G_c} \tauu$  as shown in diagram \cref{eqdiag:injectivity}(a) (so that arrow \tauu\ plays the role of a regular logic formula).    
		\input{diagrams/injectivity}
	Diagram \cref{eqdiag:injectivity}(a') unpacks this definition as a commutative diagram in \GG\ (arrows \tauu, $x$, $y$ in diagram a) become commutative triangles $(\tauu, q_\tauu, p_\tauu)$, $(x,t,p_\tauu)$, $(y,t,q_\tauu)$ in diagram a'). Ignore diagram (b)  until \cref{constr:lifting}.
\end{defN}
%
% \begin{constrN}[Diagrammatic implications]
%	Let \GG\ be an arbitrary category (of 'graphs'), and $S$ an object considered as a {\em schema}. A {\em diagrammatic implication} in $\GG$ over schema $S$  is a commutative triangle $\tauu=(p_\tauu, \bar\tauu, q_\tauu)$ where $p_\tauu = \bar \tauu.q_\tauu$, and the shared object $\cod p_\tauu = \cod q_\tauu$ is $S$ --- see the bottom of the prism in digram \cref{eqdiag:injectivity}(a'). Arrow  $\bar\tauu$ will be referred to as {\em formula-arrow}.
%	
%	\input{diagrams/injectivity}
%	
%	%A triangle as above  is a \mor\  \frarxy{p_\tauu}{q_\tauu} in the slice \caty\ $\GG/S_\tauu$.  %, but by a common abuse of notation, we will often write  \frar{\bar \tauu}{p_\tauu}{q_\tauu} rather than \frar{\tauu}{p_\tauu}{q_\tauu}, and similarly ofr other \mor s in $\GG/S_\tauu$. 
%	
%	Triangle \tauu\  is an arrow \frar{\tauu}{p_\tauu}{q_\tauu} in the slice \caty\ $\GG/S$, instances \frar{t}{X_t}{S} are objects in $\GG/S$, and we thus can consider injectivity as an instance validity mechanism. To wit: we introduce a constraint $c(\tauu)$ of shape $S_{c(\tauu)}=S$ and semantics  $\semm{c(\tauu)}=\InjMod_{\GG/S}(\tauu)$. % in the carrier \caty\ $\GG/S$. 
%	That is, unpacking the definition for the carrier category $\GG/S$, a $c(\tauu)$-preinstance \frar{t}{X_t}{S} satisfies  \tauu, if for any \frar{\hat x}{p_\tauu}{t} in $\GG/S$ there is \frar{\hat y}{q_\tauu}{t} in $\GG/S$ such that $\hat x= \tauu.\hat y$ --see diagram \cref{eqdiag:injectivity}(a), which is unpacked by diagram \cref{eqdiag:injectivity}(a') in \caty\ \GG: $\hat x$ in diagram (a) is the commutative triangle $x.t=p_\tauu$ in (a') and similarly for $\hat y$. %Then we write $t\InjModX{\GG/S
%	We will call such $c(\tauu)$ a {\em triangle constraint}. Thus, $t\models c(\tauu)$  iff (by definition) $t\modelsInjX{\GG/S} \tau$.  (Ignore diagram (b)  until \cref{constr:lifting}).
%\qed\end{constrN}
\input{diagrams/injectivity}
\begin{figure}[h]
	\centering
	\begin{tabular}{c@{\qquad}c}
		%		\centering
		\includegraphics[width=0.485\linewidth]{pdfs/triangle4leftTotality}
		&
		%      \centering
		\includegraphics[width=0.485\linewidth]{pdfs/triangle4uniqueness}
		\\  [10pt]
		a) \parbox{0.35\linewidth}{Constraint $\tauu_1$: Left totality (not all links are shown in mapping $t$)}
		&  b) Constraint $\tauu_2$: Uniqueness 
	\end{tabular}
	\caption{Two triangle constraints for \cref{ex:two-triangle-constr}}
	\label{fig:two-triangle-constraints}
\end{figure}
\begin{example}[Two regular constraints in \catcat]\label{ex:two-triangle-constr}
We will consider two triangle constraints $\tauu_1$, $\tauu_2$ over the same schema \StauX{}. %=\StauX{1}=\StauX{2}.  
	The first one is specified in \cref{fig:two-triangle-constraints}(a).
The bottom part shows commutative diagram of functors $\XtauY{p}{1}=\bar \tauu_1.\XtauY{q}{1}$ presented by graph mappings, and hence defines a triangle constraint  $\tauu_1$  in \catcat. This constraint forces any instance $t$ over schema $S_{\tauu}$, \ie, a span \spanrar{\semmXt{r}}{\semmXt{A}}{\semmXt{B}}, to be (left) totally defined. For example, a sample instance $t$ shown in the upper-right part of diagram (a) violates the constraint and has to be considered invalid because (while testing map $x$ can be completed with map $y$) there is no completion $y'$ for testing map $x'$. The trouble-maker is node $2{:}A$ which is typed by $A$ but does not have any arrow originating at it. Surjectivity of $r$ in schema \StauX{} can be specified analogously by mapping the only node in \XtauY{P}{1} to node $B$ in \StauX{}.

%Hence, instance $t$ violates constraint $\tauu_1$. 
%\zd{write in the construction above that we call $c_\tauu$ a {\em triangle constraint}, and often refer to it as $\tauu$ rather than $c_\tauu$.} However, instance $t'$ over the same schema shown in \cref{fig:two-triangle-constraints}(b) does satisfy $\tauu_1$.  
%
Similarly, diagram \cref{fig:two-triangle-constraints}(b) specifies a triangle constraint $\tauu_2$ that  forces any span instantiating the schema to be single-valued, \ie, to be a  function (possibly partial). Indeed, an injective testing mapping \frar{x}{\XtauY{P}{2}}{X_t} cannot be completed. Taken together, these two constraints force valid instances over schema \StauX{}  to be total functions \semm{r} from set \semm{A} to set \semm{B}.  
\qed\end{example}
For both constraint above, mapping $q_\tauu$ is an iso\mor; the next example shows a more interesting constraint where this is not  the case.  
\begin{figure}%[h]
	\centering
%	\begin{tabular}{c@{\qquad}c}
%		%		\centering
		\includegraphics[width=0.485\linewidth]{pdfs/triangle4transitive}
%		&
%		%      \centering
%		\includegraphics[width=0.485\linewidth]{pdfs/Uniqueness}
%		\\  [10pt]
%		a) \parbox{0.35\linewidth}{Constraint $\tauu_1$: Left totality (not all links are shown in mapping $t$)}
%		&  b) Constraint $\tauu_2$: Uniqueness 
%	\end{tabular}
	\caption{Yet another triangle constraints for \cref{ex:transitivity}}
	\label{fig:transitivity}
\end{figure}
\begin{example}\label{ex:transitivity}
	Diagram of graph mappings in \cref{fig::transitivity}
	\vspace{5cm}
\qed\end{example}
%\END
\begin{defN}[Lifting constraints, Spivak \cite{spivak-lifting14}]\label{constr:lifting}
	In a category \CC, take an object $S$ called a {\em schema}, and 
	 then \mor s into $S$ are called {\em (pre)instances}.  

\noindent 
\begin{minipage}[h]{0.75\linewidth}
 %then \mor s into $S$ are called {\em (pre)instances}.  
 ~~~A {\em lifting constraint} over $S$ is a pair $\lamm=(m_ \lamm, n_\lamm)$ of  \mor s \frar{m_\lamm}{W_\lamm}{R_\lamm} and \frar{n_\lamm}{R_\lamm}{S}. An instance \frar{t}{X_t}{S} {\em satisfies} \lamm\ if for any \frar{x}{W}{X_t} making commutative square  in the inset diagram %\cref{eqdiag:injectivity}(c)) 
 there is a diagonal arrow \frar{\ell}{R}{X_t} (called a {\em lift}) such that both triangles commute. Then we write $t\modelsLiftX{\CC}\lamm$. \qed
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.2\linewidth}
\vspace{-2ex}\(
	\xymatrix{ % row 1
		W_\lamm \ar@{->}[r]^{x}
		\ar[d]_{m_\lamm}
		& X_t \ar[d]^t
		\\
		R_\lamm	
		\ar@{->}[r]^{n_\lamm}
		\ar@{-->}[ru]^\ell
		& S}  %S_\lamm}
	\)
\end{minipage}
\end{defN}
Returning to the injectivity-based definition specified in diagrams \cref{eqdiag:injectivity}(a,a'), it is immediate to see that the diagram \cref{eqdiag:injectivity}(a'), and the inset diagram above reproduced with (a') names as diagram \cref{eqdiag:injectivity}(b), are the same diagram -- the only difference is that the composed arrow $p_\tauu$ is not shown in \cref{eqdiag:injectivity}(b). 
% In terms of Spivak's {\em lifting constraints} \cite{spivak-lifting14},  pair $(\arrowInj{\tauu}, q_\tauu)$ is a lifting constraint (say, $\ell(\tauu)$) over $S_\tauu$ in the carrier category $\GG$, and an instance $t$ over $S_\tauu$ is said to {\em  satisfy} $\ell(\tauu)$ if for any $x\in\GG(P_\tauu, X_t)$ making the square in \cref{eqdiag:injectivity} commutative, there is an arrow $\lifft$ (called a lift) such that both triangles commute. Then we write $t\modelsLiftX{\GG}\ell(\tauu)$. 
\begin{propo}[Regular and lifting constraints are equivalent]\label{propo:impl2injectivity} 
	\zd{\large IT MAY BE SHORTEN}
A \dimpl\ $\tauu=(p_\tauu, \bar \tauu, q_\tauu)$ \ over schema $S$ gives rise to a lifting constraint $\lamm(\tauu)$ over the same schema with $m_{\lamm(\tauu)}=\bar \tauu$ and $n_{\lamm(\tauu)}=q_\tauu$, for which for any preinstance $t$ over $S$, the following equivalence holds: $t\modelsLiftX{\GG}\lamm(\tauu)$ ~iff~ $t\modelsInjX{\GG/S}\tauu$  ~~(note the change of the carrier category).

Conversely, any lifting constraint $\lamm=(m_\lamm, n_\lamm)$ over schema $S$ gives rise to a \dimpl\ $\tauu(\lamm)=(m_\lamm.n_\lamm, m_\lamm, n_\lamm)$ over $S$, for which ~~ $t\modelsInjX{\GG/S}\tauu(\lamm)$  ~iff~ $t\modelsLiftX{\GG}\lamm$ for any $S$-preinstance $t$.  Obviously, $\tauu(\lamm(\tauu))=\tauu$ and $\lamm(\tauu(\lamm))=\lamm$. 
%	The following two conditions are equivalent for any commutative triangle $\tauu$ with  formula-arrow $\bar \tauu$  and apex object $S_\tau$, and its preinstance  \frar{t}{X_t}{S_\tauu}:
%	
%	a) $t\modelsInjX{\GG/S_\tauu}$
%%(defined by injectivity $t\modelsInj \tauu$ in $\GG/S_\tauu$)% \ie, by definition, $t\modelsInj\tauu$
%	
%	b) $t\modelsLiftX{\GG}\ell(\tauu)$ (in the sense of having a lift as described above). %, \ie, by definition, there is a solution to the lifting problem $[ (t,\alphaa_\tauu), (x, q_\tauu)]$.
\qed\end{propo} 



\begin{corol}
	Four inference rules in \cref{eq:injLogic-rules} provide a sound and complete deductive calculus for the lifting constraint logic. 
\end{corol}
\begin{corol}
	Any lifting constraint is an abstract constraint as specified in \cref{def:abstrConstr}. Moreover, a set of constraints over a schema $S$ as defined in \cite{spivak-lifting14} is a sketch..... 
\end{corol}

\endinput




\begin{defN}[Diagrammatic implications]\label{def:implConstr }
	Given a category \GG \zdmoddok{with pullbacks}{}{Nope!}{-1}, a {\em triangle (diagrammatic) implication} is a commutative triangle $\tauu=(\arrowInj{\tauu}, p_\tau, q_\tau)$ in \GG\ as shown by the bottom of the prism in diagram \cref{eq:three-defs}(a). 
	%Object $S_\diagImpl$ is the {\em arity (scope)} of $\tau$, and arrow $\implPart_\diagImpl$ is the {\em implicational part} of  $\tau$'s(do not confuse it with logical implications $\Rightarrow$ considered earlier).  
	A preinstance \frar{t}{X_t}{S_\tauu} {\em satisfies} $\tauu$ (and we write $t\modelsInj\tauu$) if for any \frar{x}{P_\tauu}{X_t} such that $x.t=p_\tauu$, there is \frar{\lifft}{Q_\tau}{X_t} such that both $\lifft.t=q_\tau$ and $\arrowInj{\tauu}.\lifft=x$. %Then we write $t\vDash^.\tau$.
	
	In this way we obtain a procedure that filters instances $t$ into valid/invalid and thus any triangle implication gives rise to an abstract constraint $c(\tauu)$ of arity shape $S_{c(\tauu)}= S_\tauu$ and semantics 
	$\semm{c(\diagImpl)}=\compr{t\in\GG/S_{\diagImpl}}{t\modelsInj_*\diagImpl}$, \ie, $t\modelsInj c(\tauu)$ and $t\modelsInj_* \tauu$ are equivalent. % and we will omit the dot superscript. 
	\qed
\end{defN}

%Obviously, any diagrammatic implication $\tau$ gives rise to an abstract interpreted constraint $c(\tau)$ with scope $S_{c(\diagImpl)}=S_\diagImpl$ and semantics $\semm{c(\diagImpl)}=\compr{t\in\GG/S_{\diagImpl}}{t\modelsInj^.\diagImpl}$. 
An evident but important reformulation of the definition above in terms of slice categories is specified in diagram \cref{eq:three-defs}(b). Indeed, arrows $p_\tauu$, $q_\tauu$ and $t$ are objects of the slice category $\GG/S_\diagImpl$ and arrow $\arrowInj{\diagImpl}$ gives us a \mor\ in $\GG/S_\diagImpl$ denoted by the same symbol   \frar{\implPart{\tauu}}{p_\diagImpl}{q_\diagImpl}. Then for any preinstance $t$, $t\modelsInj\tauu$ iff for any \frar{x}{p_\tauu}{t} in $\GG/S_\tauu$, there is \frar{y}{q_\tauu}{t} in $\GG/S_\tauu$ such that $\implPart{\tauu}.y = x$. This is exactly the definition of $t$'s injectivity w.r.t. arrow $\implPart{\tauu}$, which we will denote by $t\modelsInjInj\arrowInj{\tauu}$


%\input{diagrams/injectivity}

Yet another equivalent formulation in terms of the {\em lifting problem} is shown in diagram (c), which is nothing but diagram (a) from which composed arrow $p_\tau$ is removed. In terms of Spivak's {\em lifting constraints} \cite{spivak-lifting14},  pair $(\arrowInj{\tauu}, q_\tauu)$ is a lifting constraint (say, $\ell(\tauu)$) over $S_\tauu$, and an instance $t$ over $S_\tauu$ is said to {\em  satisfy} $\ell(\tauu)$ if for any $x\in\GG(P_\tauu, X_t)$ making square shown in \cref{eqdiag:injectivity} commutative, there is an arrow $\lifft$ (called a lift) such that both triangles commute. Then we write $t\modelsInjLift\ell(\tauu)$.%
\footnote{\zd{I guess it's not needed but let it be here for the record. If $t$ is mono, then commutativity of the lower triangle implies comm. of the upper one. If $h_\tauu$ is epi, then the converse holds.}} 
\begin{propo}\label{propo:impl2injectivity} The following three conditions are equivalent for any diagrammatic implication $\tauu$ and its preinstance  \frar{t}{X}{S_\tauu}:
	
	a) $t\modelsInj c(\tauu)$, \ie, by definition, $t\modelsInj\tauu$
	
	b) $t\modelsInjInj \arrowInj{\tauu}$ in $\GG/S_\tauu$, \ie, $t$ is injective w.r.t. $\arrowInj{\tauu}$ in the slice category $\GG/S$.
	
	c) $t\modelsInjLift\ell(\tauu)$ in the sense of having a lift as described above. %, \ie, by definition, there is a solution to the lifting problem $[ (t,\alphaa_\tauu), (x, q_\tauu)]$.
\end{propo} 
\begin{remark}\label{rema: employing-inj}
	Injectivity is a well-studied categorical subject.  Equivalence (a) $\Leftrightarrow$ (b) allows us to employ a pool of well-known results, \eg, a sound and complete deductive calculus for injectivity (both finitary and infinitary) \cite{injLogic--Adamek2007}, and closure Birkgoff-style theorems \cite{injBirkhoff--Rosicky2002}, for studying diagrammatic implicational constraints.
\end{remark}
%\zd{\sc Million \$\ question: What is better for denoting arity scope: $S_c$ as (arity) scope of $c$, or $A_c$ as {\em ariry (scope)} of $c$???? It seems $A_c$ would be better as $S$ is used for the carrier graphs etc}
\begin{remark}
	In Spivak's definition of lifting constraints, schema $S$ does not belong to a constraint: his lifting constraint $\ell$ over a pre-given schema $S$ is a pair of arrows  $(\frar{\bar \ell}{P_\ell}{Q_\ell}, \frar{q_\ell}{Q_\ell}{S} )$, and a {\em set of lifting constraints} is a set of such pairs over the same $S$. The triangle-constraint counterpart of this notion would be a set $\nit$ of {\em triangle declarations} over $S$, \ie, pairs $(\tauu,\bmap)$ of a triangle and a binding map \frar{\bmap}{S_\tauu}{\S}. We will discuss pros and cons of such a choice later in ...  
\end{remark}



==> sections/intro4act23--April30.tex <==
\newcommand{\DMKR}{DMKR}
\newcommand{\iAMT}{iAMT}
\renewcommand{\iAMT}{\instfwk}
\newcommand{\instfwk}{{\em inst}-\fwk}


\section{Introduction}

\begin{itemize}
\item  Graphical databases are burgeoning...the need for semantics... \DMKR\ thing...
\item The ACT's community normal view of data as either a functor from $S$ to \setcat, or to \relcat\ or \catname{Birel} (cite Evar Patterson) but it's too restrictive. We need it as a lax functor into \spanbicat. 
\item Heterogeneous model management, the notion of mapping between such diverse artefacts as ....But designing such a notion needs an {\em abstract} notion of a constraint. Hence, a slogan: {\em Any data schema  is a generalized sketch in a suitable constraint signature, and a schema mapping is a sketch \mor.} {\em A valid Instance of such a sketch is.... }%
\footnote{ \zd{see in section bits-and -pieces for:a) MMt from SLE13 megamod paper; b)A big quote from Makkai's paper p.52
}}  
\end{itemize}
\endinput

\begin{mygroup} % redefine \Sigmaa
%\input{diagrams/satAxiom}
%\clearpage 
 Building very abstract data modelling \fwk s has a long history that in a modern time can be traced back to abstract model theory \cite{Barwise} and institutions \cite{Goguen-Burstall-92} further jointly referred to as \iAMT\ %(to be read as ``institutional AMT'').  
%\input{sections/piece--institution-as-4tuple}

		\renewcommand{\Sigmaa}{\enma{L}}
		\renewcommand{\Modsetsig}{\ModsetX{}}
		\renewcommand{\Sensetsig}{\SensetX{}}
		\renewcommand{\ModsetsigPrim}{\enma{\Modsetsig'}}
		\renewcommand{\SensetsigPrim}{\enma{\Sensetsig'}}
		\renewcommand{\modelssig}{\enma{\vDash}}
		\renewcommand{\modelssigPrim}{\enma{\vDash'}}
		
  An {\em institution} is a functor \frar{\logfun}{\signcat}{\logsyscat} from a small category \signcat\ whose objects are called {\em signatures} (think, \eg, of a signature of operation and relation symbols) to a \caty\ of {\em logical systems}, whose objects are binary {\em satisfiability} relations $\vDash\subset \ModsetX{} \timm \SensetX{}$. A {\em \mor} of logical systems \frar{f}{L'}{L} is a pair of functions $(f^*, f_*)$ specified in diagram \cref{eqdiag:satisfyAxiom}a) such that for all $m\in\Modsetsig$ and all $\phi'\in\SensetsigPrim$, the {\em twisted satisfiability} condition specified in \cref{eqdiag:satisfyAxiom}b) holds. 
 \vspace{-1em}
 \input{diagrams/satAxiom}
\noindent 
%where diagram \cref{eqdiag:satisfyAxiom}a) shows directions of functions $f^*=\ModsetX{}(f)$ and $f_*=\SensetX{}(f)$ (note the reversal of arrow for $f^*$). 
The rightmost diagram (ignore for a moment three dashed arrows and their targets) expresses this condition diagrammatically as the existence of jointly monic span {\modelsFtwisted} (its legs are diagonals), which is embedded into both (jointly monic) satisfiability spans so that the diagram commutes. 
%
It is this diagram, which is a basis for  much of the \instfwk\ theory and applications. 
\end{mygroup}
% \prodnodeS, \prodnodeSprim, \prodnodeFtwist\, 
 % \underprodS, \underprodSprim, \underprodFtwist
 
There are three deficiencies in the \instfwk\ for practical data modelling applications.

\input{sections/piece--realSysFunctions}

\bfem{Deficiency 1.}
Considering the logical constructs in isolation from real problems they intended to model and help to manage. We will refer to such as to a {\em real system} \sysS, which logical systems aim to model. In this view, 
% Let us refer to this reality background as to a {\em system} \sysS, which encompasses several sets and functions described below. 
logical formulas appear as formal models of requirements that real world object should satisfy, and the latter are formally modelled by logical models, \ie., elements of set \Modset. A rough model of this setting would be a pair of functions, 
$$ 
\frar{\syssenfun}{\sysReqset}{\Senset} \andform\ \frar{\sysmodfun}{\sysInstset}{\Modset},
$$ which may be non-injective.  
For example, it may happen that different \req s $r$, $r'$ can be modelled by the same logical sentence $\phi$ at some moment $t$, and by different sentences at some moment $t'$ later. Then we cannot equalize $r$ and $r'$, but at moment $t$ we have $\syssenfun(r)=\syssenfun(r')=\phi$. Similarly, set \Modset\ may be a set of version numbers and then  function \sysmodfun\  is typically injective but imagine an audit of a model that did not reveal any changes to be made (a rare but not impossible event). Then it is reasonable to increase the version number by 1 but set $\sysmodfun(n)=\sysmodfun(n+1)$. 
%
In general, practically everything in the world of software and data engineering changes so that objects of interests keep their identity ()a \req\ named $r$) but change their attribute values (\eg, formal model $\phi$). 
%
It may seem that additional indexing from functions \syssenfun\ and \sysmodfun\  is not needed when we consider the logical stage at a concrete time moment but, surprisingly, some mathematical aspects of abstract logic become simpler in the indexed setting. This was first found by Makkai, who irrespective to any applicability considerations, discovered that diagrammatic theories with   .... (cf. Makkai !!!). 
 %
 We will often refer to the setting above as {\em indexed} or {\em multi}: the latter stems from the {\em multiset} terminology. %meaning that it gives a sentence $\phi\in\Senset$ a number of its occurrences \nmf{card}$[{(\syssenfun)}^{-1}\!(\phi)]$ into the set. 
  MultiXX vs. MonoXX.  
 
 \bfem{Deficiency 2.} The necessity to verify satisfiability, especially for safety-critical systems.....
 
$$
\frar{\syssatfun}{\sysVerset}{\Modset\timm\Senset}
$$  
so that satisfiability is recovered as the image of \syssatfun.
  
Now  the satisfiability axiom becomes richer and includes verification:
$$
m\models_{v} f_*(\phi) \text{~iff~} f^*(m)\models'_{v'}\phi \text{~for a pair of verifiers $v\vertsim_f v'$}
%$(v,v')\in\vertsim_f$}
$$ 
where symbol  \verifier\ refers to a verification procedure confirming satisfiability at hand.%
\footnote{In a even richer model, we could consider different verifiers for different signatures but then the notion of \mor\ should somehow relate them. In the present paper we follow a simpler approach.}
The diagrammatic form of the axiom is specified the full rightmost diagram in \cref{eqdiag:satisfyAxiom} with two dashed arrows included.  
 %\endinput

 \bfem{Deficiency 3.} The \instfwk\ is good for ... but its treatment of syntax is far too abstract. What skecthes do is ... $\Sigmaa\mapsto S(G_S, C_S)$ where.... ...

This will be collectively referred to as the {\em system  dimension}.
 

% \END

==> sections/intro4act23--May3.tex <==
%\newcommand{\DMKR}{DMKR}
%\newcommand{\iAMT}{iAMT}
%\renewcommand{\iAMT}{\instfwk}
%\newcommand{\instfwk}{{\em inst}-\fwk}
%
%%\renewcommand{\Sigmaa}{\enma{L}}
%%\renewcommand{\Modsetsig}{\ModsetX{}}
%%\renewcommand{\Sensetsig}{\SensetX{}}
%%\renewcommand{\ModsetsigPrim}{\enma{\Modsetsig'}}
%%\renewcommand{\SensetsigPrim}{\enma{\Sensetsig'}}
%\renewcommand{\modelssig}{\enma{\vDash}}
%\renewcommand{\modelssigPrim}{\enma{\vDash'}}
%\newcommand{\satrelsig}{\enma{\vDash_\Sigmaa}}
%\newcommand{\satrelsigPrim}{\enma{\vDash_{\Sigmaa'}}}


\section{Introduction}\label{sec:intro}

\begin{itemize}
%\item  Graphical databases are burgeoning...the need for semantics... \DMKR\ thing...
%\item The ACT's community normal view of data as either a functor from $S$ to \setcat, or to \relcat\ or \catname{Birel} (cite Evar Patterson) but it's too restrictive. We need it as a lax functor into \spanbicat. 
\item Heterogeneous model management, the notion of mapping between such diverse artefacts as ....But designing such a notion needs an {\em abstract} notion of a constraint. Hence, a slogan: {\em Any data schema  is a generalized sketch in a suitable constraint signature, and a schema mapping is a sketch \mor.} {\em A valid Instance of such a sketch is.... }%
\footnote{ \zd{see in section bits-and -pieces for:a) MMt from SLE13 megamod paper; b)A big quote from Makkai's paper p.52
}}  
\end{itemize}
%When you move data from one application to another, the way the data is structured may not be compatible between the two systems. Data exchange is the transformation or restructure of the data to suit the new system. The aim of a data exchange is not to lose or change the meaning of the information in the transfer.

In a modern industrial software environment, one normally deals with a diversity of data formats for storage and manipulation, which range from ad hoc file systems to relational data to XML to graphical databases. This often makes the issues of tools' interoperability and data exchange and integration a major stumbling block for effective software development and productive work.  An obvious idea to manage these issues via developing a unifying \fwk\ for data representation has shown its reasonable effectiveness within separated software ecosystems (\eg, such as EMF or XML) but modern software environments often span different ecosystems, which brings us to the same problem on a deeper level. Hence, the technological sense of being a unified \fwk\ should be replaced with a truly abstract, mathematical sense of unification. 

The following mathematical model can nowadays be considered established as being vastly universal. To understand and manipulate data, we need (data) types. The latter can be organized into a structure usually called a {\em schema}, and then a data instance $D$ over schema $S$ can be seen as a {\em typing} mapping \frar{t_D}{X_D}{S} that maps each data element in structure $X_D$ to its type in $S$. With a suitable \caty\ encompassing data and schemas, a mapping \frar{f}{D'}{D} between data instances is a commutative square formed by the quadruple $t_D$, $t_{D'}$, \frar{f_S}{S'}{S} and \frar{f_D}{X_{D'}}{X_{D}}. This model is a bare skeleton, and much is to be added to it to make it adequate to practical applications.The present paper deals with the problem of constraints. 

A {\em constraint} $c$ declared over schema $S$  is a device that classifies all instances over $S$ into {\em valid} (we then write $D\vDash c$) and (otherwise) {\em invalid}. Such a classification plays at least two important roles. i) Applications usually assume that data do satisfy some constraints $c', c'',...$ so that it makes sense to include them into schema $S^+= (S, c', c'')$ and disallow instances that violate constraints upfront (this is often called data integrity). ii) In safety-critical applications, there are constraints whose violation can compromise safety and thus instances violating such are to be prohibited. 

Studying binary \satty\ relation $\vDash$ is a classical subject of mathematical logic. %, in which constraints are logical sentences. 
Many constraint \specifin\ languages were developed, \eg, FOL and its fragments, Ehresmann's sketches, data dependencies developed in the relational database theory, and Spivak's lifting constraints popular within the ACT community, or, \eg,  industrially usable OCL \cite{oclBook-99} and B \cite{B-book}.  However, they are not applicable for the interoperability problem as they are too concrete and only work within their own logical ecosystem. 
%
%Moreover, there are constraints that cannot de decomposed ... no syntax???
%
We need a far more abstract theory of $\vDash$, which is not being bound to specifics of a concrete constraint \specifin\ language. Attempts to develop such a theory 
%for purely mathematical reasons 
can be traced back to {\em abstract model theory} \cite{barwise-axioms4amt-AML74}
and, more recently, Goguen and Burstall's {\em institutions} \cite{Goguen-Burstall-92}. 
% (well-known in the Algebraic \specifin\ community....
The latter is practically a bare-bone \fwk\ for describing translation of binary relation $\Modsetsig \satrelsig\Sensetsig$ between  sets  \Modsetsig\ of {\em \Sigmaa-models} and \Sensetsig\ of {\em \Sigmaa-sentences} (\ie, constraints),  when the logical signature changes ({\em \satrelsymbol-interoperability} in the technological speak). If such changes are specified by a signature \mor\ \frar{f}{\Sigmaa'}{\Sigmaa}, then the main and in fact the only substantial postulate of the institution construct states that sat-relation translates in a twisted way: for models with a function  \frar{f^*}{\Modsetsig}{\ModsetsigPrim} in the direction opposite to $f$, for sentences with function \frar{f_*}{\SensetsigPrim}{\Sensetsig} in the same direction, and such that for all $m\in\Modsetsig$ and all $\phi'\in\SensetsigPrim$, the {\em twisted \sation} 
condition \fbox{$f^*(m)\satrelsigPrim \phi' \text{~iff~} m\satrelsig f_*(\phi')$}
holds. 
%
%\input{diagrams/satAxiom-Rel}
%
%\input{sections/piece--aboutInstit4briefExpo}
%%specified in \cref{eqdiag:satisfyAxiom} holds. 

There are several serious deficiencies of the  \instfwk\ wrt. its application to software interoperability, where models become data instances and hence many-sorted, and sentences are sort-spanning constraints. We will briefly discuss three of them.  A major deficiency is that institutions ignore the local nature of the sat-relations appearing in practice: %(and logic with finitary signatures): 
to find if a model $m$ satisfies a constraint $c$, normally a small part of $m$ is to be examined and fixed if the constraint is violated. For industrial instances/models comprising thousands of elements over dozens/hundreds of sorts, locality of constraints is their crucial feature (\eg, see \cite{me-ecmfa17} for how it can be used to make inter-model consistency checking more effective) and needs to be included into a principled \fwk.  Another institutions' shortcoming is that for safety-critical constraints, satisfaction instance $m\satrelsymbol c$ is to be verified by a suitably certified procedure (a model checking procedure, simulation, %a theorem prover, 
or an expert review), and safety assurance norms demand those procedures to be explicitly referenced. This makes \sation\ a ternary rather than binary relation (where the third leg can be refined into a separate structure if needed). 

Yet another deficiency is considering the logical constructs in isolation from real problems they are intended to model and in the static change-free setting. %We will refer to such as to a {\em real system} \sysS, which logical systems aim to model. In this view, 
 % Let us refer to this reality background as to a {\em system} \sysS, which encompasses several sets and functions described below. 
However, practically everything in the world of software and data engineering changes so that objects of interests keep their identity %(\eg, a \req\ named $r$) 
but change their state %(\eg, $r$'s formal model $\pii_S(r)=\phi$). Then models and sentences/constraints become trajectories, which may intersect (and have loops).
For example, a formal constraint (sentence) $c$ modelling a safety \req\ $r$ changes over time when the object $X$ that must meet $r$ changes, or a safety standard changes the content of $r$ and hence $c$ should be changed, or a fatal accident forced engineers to strengthen $c$. Then \req\ $r$ appears as a trajectory \frar{r}{T}{\Senset} in the space \Senset\ rather than a point\ (here $T$ is a set of (logical) time moments). Then for a given unspecified moment, we have an {\em indexing projection} function \frar{\pii_\senfun}{I_\senfun}{\Senset}, where we refer to \req s as to sentence {\em indexes} from set $I_\senfun$. Similar considerations are important also  for models. Indeed, a complex system is necessarily developed by multiple teams, each one building its own subsystem or designing its own view of a system, and at certain moments, these subsystems/views are to be synchronized. We thus again come to trajectories and indexing \frar{\pii_\modfun}{I_\modfun}{\Modset} at an unspecified logical moment (with subsystems/views being elements of set $I_\modfun$). As a rule, both indexing projections are not injective so that collections \Modset\ and \Senset\ are to be multisets rather than plain sets, and the notion of satisfaction is to be correspondingly adjusted. 
%
 %Similarly, set \Modset\ may be a set of version numbers and then  function \sysmodfun\  is typically injective, but imagine an audit of a model that did not reveal any changes to be made (a rare but not impossible event). Then it is reasonable to increase the version number by 1 but set $\pii_M(i)=\pii_M(i+1)$. 
 %
 Remarkably, constraint indexing was introduced into the (generalized) sketch \fwk\ by Makkai \cite{makkai-ske} by purely mathematical reasons as sketches with indexed constraints (Makkai calls them \specifin s) behave mathematically better. (To wit: a remarkable fact discovered by Makkai is that if sketches are built over graphical objects specifiable as functors \frarxy{\II}{\setcat}, \ie, the \caty\ of graphs underlying sketches is a copresheaf topos, then the \caty\ of sketches with indexed constraints is a copresheaf topos as well. In other words, sketches, \ie, schemas with constraints are graphs!) Similarly, model indexing introduced into the sketch \fwk\ in the prresent paper, adds the third verification leg to the \sation\ relation almost for free.   
 %\vspace{3cm}
%\input{sections/piecde--threeDeficiencies-of-institutions}
%
Methodologically, the place of sketches in a general landscape of \specifin\ formalism is illustrated by the following diagram. 

\zd{\large To be drawn in drawio and inserted}

Our plan for the paper is as follows. Sect 2 -- example. Sect 3 -- mild sketch intro to get the feel. Sect 4 -- fornal theory. 

{xxx}\footnote{Remark for the reviewers: }
%\endinput


% \END

==> sections/intro4act23.tex <==
\section{Introduction}\label{sec:intro}

In a modern industrial software environment, one normally deals with a diversity of data formats for storage and manipulation, which range from ad hoc file systems to relational data to XML to graphical databases. This often makes the issues of data exchange and tools' interoperability (further referred to as \interopy\ management, {\em \IMt}) a major stumbling block for software development and productive work.  An obvious idea to manage these issues via developing a unified format for data representation has shown its reasonable effectiveness within separated software ecosystems (\eg, such as UML/EMF or XML) but a modern software environment often spans different ecosystems, which brings us to the same problem on a deeper level. Hence, the technological sense of unification should be replaced with a truly abstract, mathematical sense of being a unified \fwk.  

The following mathematical model can nowadays be considered established as vastly universal. To understand and manipulate data, we need (data) types. The latter can be organized into a structure usually called a {\em schema}, and then a data instance $D$ over schema $S$ can be seen as a {\em typing} mapping \frar{t_D}{X_D}{S} that maps each data element in structure $X_D$ to its type in $S$. With a suitable \caty\ encompassing data and schemas, a mapping \frar{f}{D'}{D} between data instances is a commutative square formed by the quadruple $t_D$, $t_{D'}$, \frar{f_S}{S'}{S} and \frar{f_D}{X_{D'}}{X_{D}}. This model is fundamental for many \IMt\ problems (cf. \cite{spivak-algMMt-arxiv16}), but it is a bare skeleton, and much is to be added to it to make it adequate to practical applications. In the paper, we will deal with the problem of constraints, \ie, specifications that being added to schema $S$ classify instances over $S$ into {\em valid} or (otherwise) invalid. 


We aim at two goals. One is expository: discussions at the last NIST workshop\footnote{ https://www.nist.gov/news-events/events/2022/11/compositional-structures-systems-engineering-and-design-0}
showed an interest within the ACT community towards generalized sketches (further just sketches) and their accurate presentation explaining Why, What and How with an emphasis on Why. The paper takes on this duty and goes further by presenting sketches with several novel features, specifically, verification aspects crucial for modelling safety assurance. Moreover, sketches of this paper essentially depart from Makkai's sketches and their version described in \cite{me-entcs08} in that semantics is built-in it into the very notion of a constraint signature. In this sense, it is a return to classical Ehresmannian sketches, whose signatures consist of universal properties which do have a predefined semantics in \setcat, and it makes sense to call them somehow differently from Makkai's sketches, \eg {\em Ehresmann's generalized sketches}. %The paper also shows that semantic universe better aligned with data modelling needs is \spancat\ rather than \setcat\ or even \relcat\ (it is discussed in detail in Sect. 2.1  ).  

The second goal is to present several simple but interesting mathematical results about what we will call Cartesian \sation\ relation. Let \GG\ be a finitely complete \caty\ (of {\em graphs}). A {\em constraint} over \GG\ is a triple $(c, G_c, \semm{c})$ of a {\em constraint name} $c$, its {\em arity} graph $G_c\in Ob\GG$, and a set $\semm{c}\subset \GG/G_c$ of {\em valid} instances. Then any graph/object $G$ determines a satisfaction relation $\models_G \subset \GG/G\times\GG(G_c,G)$ by setting $\tmap\models_G (c,\bmap)$ iff pulling \tmap\ back along \bmap\ results in $\tmap_\bmap\in\semm{c}$; then we say that instance \tmap\ (a logician would say {\em model}) satisfies constraint ({\em sentence}) $(c,\bmap)$. (Although this only needs pullbacks, having \tcat\ and  elements will  also be useful.) If $G$ changes via \GG-\mor\ \frar{f}{G}{G'}, then we require that $\models_G$ changes contravariantly on the left via pullbacks  \frar{f^*}{\GG/G'}{\GG/G}, and covariantly on the right via post-composition \frar{f_*}{\GG(G_c,G)}{\GG(G_c, G')}. Then for any $\tmap'\in\GG/G'$ and $\bmap\in\GG(G_c,G)$, the following {\em (twisted) satisfaction axiom} of the abstract model theory \cite{barwise-axioms4amt-AML74} %(in which constraints and instances are sentences and models )
\fbox{$f^*(\tmap')\models_G (c,\bmap)$ iff $\tmap'\models_{G'} f_*(c, \bmap))$} (where $f_*(c,\bmap):=(c,f_*(\bmap))$holds  due to the \pblemma. In the technological speak, it may be called the main {\em interoperability law} for constraint satisfaction (while logicians talk about {\em the invariance of truth wrt. the language translation}). 
%
%A {\em constraint} $c$ declared over schema $S$  is a device that classifies all instances over $S$ into {\em valid} (we then write $D\vDash c$) or (otherwise) {\em invalid}. Such a classification plays at least two important roles. i) Applications usually assume that data do satisfy some constraints and it makes sense to include them into schema and disallow instances that violate constraints upfront (this is often called data integrity). ii) In safety-critical applications, there are constraints whose violation can compromise safety and thus instances violating such are to be prohibited. Hence, we should revise the notion of schema and make it a tuple $S^+=(S, c', c'',...)$ so that a valid data instance is typed graph \frar{t_D}{X_D}{S} such that $D\vDash c$ for all constraints in $S^+$.  

Studying the  twisted sat-axiom in the very abstract setting is  the main subject of Goguen-Burstall's institutions introduced to manage a proliferation of logics employed in computer science. 
%
Its major deficiency for practical \IMt\ is that institutions ignore the {\em local} nature of $\models$-relations appearing in practice: %(and logic with finitary signatures): 
to find if a model/instance $\tmap$ satisfies a constraint $c$, normally a small part of $\tmap$ is to be examined and fixed if $c$  is violated. For industrial models comprising thousands of elements over hundreds of sorts, locality of constraints is their crucial feature (\eg, see \cite{me-ecmfa17} for how it can be used to make inter-model consistency checking more effective) and needs to be included into a principled \fwk. In contrast, as is seen from the above, sketches place locality at the centre of the $\models$-management  \fwk, and, in fact, are as abstract as possible after locality is respected.


The place of sketches in a general landscape of constraint \specifin\ formalisms is illustrated by diagram in \cref{fig:bigPicture}. \zd{to be FULLY rewritten!!}
%Diagram in \cref{fig:bigPicture} presents a methodological view of the story described in the paper. 
The sketch \fwk\ in the upper row takes its place between extremely abstract \instin s and concrete logical formalisms including string-based logics (such as FOL and its fragments) and diagrammatic logics (injectivity, lifting constraints).
\begin{figure}[ht]\label{fig:bigPicture}
	\centering
	\includegraphics[width=0.8\linewidth]{pdfs/bigPicture}
	\caption{A big picture of constraint specification \fwk s
	\zd{the right [PBC] is nonsense!!}
	}
	\label{fig:bigPicture}
	\vspace{-2ex}
\end{figure}
 These are ``classical'' generalized sketches of the 90s.
{\em \Sketchesplus} in the lower row  refer to an enriched \fwk\ considered in this paper: it includes a) dependencies between constraints and models as typing mappings 
introduced in \cite{me-entcs08}, and novel features:
b) indexing, and c) verification (plus the fibred rather than (co)presheaveal form of main definitions used so far).%
\footnote{Remarkably, constraint indexing was introduced into the (generalized) sketch \fwk\ by Makkai \cite{makkai-ske} by purely mathematical reasons: sketches with indexed constraints behave mathematically better. 
	%(To wit: a remarkable fact discovered by Makkai is that if sketches are built over graphical objects specifiable as functors \frarxy{\II}{\setcat}, \ie, the \caty\ of graphs underlying sketches is a copresheaf topos, then the \caty\ of sketches with indexed constraints is a copresheaf topos as well. In other words, sketches, \ie, schemas with constraints are graphs!) 
Similarly, instance indexing added to the sketch \fwk\ in the paper  directly leads to the third verification leg for the \sation\ relation, and hence feature c).}
%
Ordinary sketches can be seen as \sketchesplus\ with trivial extra structure (discrete \caties, bijective indexing). We will also see that it is possible to suitably enrich \instin s to \instinsplus\ so that \sketchesplus\ specialize  \instinsplus\ as shown in the lower row. We can consider the left square as something like a pullback completion (PBC), and hopefully with a suitable categorical arrangement it can indeed be formalized as PBC. 

The right upper cell of the figure shows multiple constraint \specifin\ languages, %: regular logic as a sublogic of FOL,  %Ehresmann's sketches, relational data dependencies, and 
%Spivak's lifting constraints popular within the ACT community, injectivity, and industrially usable \OCLTM \cite{oclBook-99}, which supersets FOL. %B \cite{B-book}.
which can be used for specifying semantics of constraints. 
%seen as different implementations of non-plus sketches.%
\footnote{Note the  iso\mor\ of the lifting constraint \fwk\ to the classical injectivity logic, which we will prove in the paper.}
% Now PBC-like procedures can enrich these logics for being capable to  implement \sketchesplus. 
 We thus have a template for enriching existing logics with verification and indexing. (\OCLTMplus\ may especially be attractive for practitioners). 

Our plan for the rest of the paper is as follows. 

...

We begin with a formal notion of a verified \sation, and the corresponding notion  of an enriched institution  both within an arbitrary but fixed finitely complete \caty\ (further, FCC)  \CC. This will serve as an abstract pattern of a {\em well-behaved logic}. 
...

%\shortlong{
%In Sect. 2,  we consider a detailed example of data modelling to demonstrate the importance, and possibly intricate nature of constraints appearing in practice. A special goal is to give the reader a touch and feel of a special world of data modelling, where one often needs to think out many fine details of data interconnection. Complimentary section motivating novel features of \sketchesplus\ is placed in \cref{sec:ske4systems} to save space. Sect. 3 provides a mild introduction to sketches to give the reader a basic intuition of basic concepts. Sect.4 presents a formal theory, including a novel \fwk\ of \instinsplus. In Sect.5 related work is briefly discussed, and Sect.6 concludes. Some auxiliary material and proofs are placed in Appendix.%
%\footnote{If the paper is accepted, by the time of camera-ready copy, the corresponding full text will be placed in arxiv and be referenced from the paper.}
%}
{
Section 2 is a motivational background.  Sect. 3 provides a mild introduction to sketches to give the reader a basic intuition of basic concepts. Sect.4 presents a formal theory, including a novel \fwk\ of \instinsplus. In Sect.5 related work is briefly discussed, and Sect.6 concludes. Some auxiliary material and proofs are placed in Appendix.%
\footnote{If the paper is accepted, by the time of camera-ready copy, the corresponding full text will be placed in arxiv and be referenced from the paper.}  
}
\endinput

{\em Remark for reviewers.}
{xxx}\footnote{Remark for the reviewers: }
\endinput
\begin{itemize}
	%\item  Graphical databases are burgeoning...the need for semantics... \DMKR\ thing...
	%\item The ACT's community normal view of data as either a functor from $S$ to \setcat, or to \relcat\ or \catname{Birel} (cite Evar Patterson) but it's too restrictive. We need it as a lax functor into \spanbicat. 
	\item Sketches considered in the present paper are called generalized sketches to distinguish them from Ehresmann's sketches
	\item Heterogeneous model management, the notion of mapping between such diverse artefacts as ....But designing such a notion needs an {\em abstract} notion of a constraint. Hence, a slogan: {\em Any data schema  is a generalized sketch in a suitable constraint signature, and a schema mapping is a sketch \mor.} {\em A valid Instance of such a sketch is.... }%
	\footnote{ \zd{see in section bits-and -pieces for:a) MMt from SLE13 megamod paper; b)A big quote from Makkai's paper p.52
	}}  
\end{itemize}
%When you move data from one application to another, the way the data is structured may not be compatible between the two systems. Data exchange is the transformation or restructure of the data to suit the new system. The aim of a data exchange is not to lose or change the meaning of the information in the transfer.


% \END

==> sections/intros/intro-act.tex <==
\section{Introduction}


A diagrammatic operation takes a diagram of a specified shape as its input, and extends it with new elements forming a bigger diagram of a specified shape; we will say that the input diagram is {\em completed} by the operation. 
For example,  arrow composition takes two consecutive arrows and completes them with a third arrow forming the \corring\ triangle.  %This list of examples can be extended indefinitely: 
The resulting diagram often satisfies some postconditions, \eg, a chosen pullback completes a cospan with a {\em commutative} square, and a chosen powerobject completes an object with its {\em jointly-monic} membership span. Preconditions are needed too, \eg, adhesive 
%HLR categories \cite{EhrigHabelPP2004} 
categories only provide pushouts for one-leg-monic spans (and then we know that the \corring\ leg of the resulting cospan is also monic). Thus, categorical diagram operations come together with reasoning over them so that diagram algebra and logic are smoothly integrated in diagram chasing routines. 

This paper stems from the observation that the diagram chasing idea transcends Category Theory (CT) and finds numerous applications in the practice of Software Engineering (SE), in which, however,  it is currently used in an ad-hoc way: implicit, semi-formal or formal but buried in code so that the underlying diagram chasing procedures are blurred and distorted.  
The negative impact of these issues increases with the recent advent of Model Driven Engineering (MDE), in which \diatic\ models rather than code become the primary artifacts of software development. 

\shortlong{
Our goal in the project reported in the present  paper%
\footnote{which is an extended abstract of ongoing work in progress, whose current state is reported in the technical report \citeTR (further referred to as ``the TR'')}
 is to provide an accurate formalization of diagrammatic reasoning routines adequate to their practical use in MDE. We will discuss this in more detail in the next section along with several mathematically interesting structures and results emerged along the course, and our contributions.  Sections 3 and 4 provide basic formal definitions and results, and Sect.5 concludes.  Appendix A is optional but helpful: it illustrates main motivating ideas with a simple example.
}{ %endShort/BeginLOng
\zd{so far, the copy-paste from the short version. To be reworked with tables etc for the long version}
Our goal in the project reported in the present  paper%
\footnote{which is an extended abstract of ongoing work in progress, whose current state is reported in the technical report \citeTR (further referred to as ``the TR'')}
is to provide an accurate formalization of diagrammatic reasoning routines adequate to their practical use in MDE. We will discuss this in more detail in the next section along with several mathematically interesting structures and results emerged along the course, and our contributions.  Sections 3 and 4 provide basic formal definitions and results, and Sect.5 concludes.  Appendix A is optional but helpful: it illustrates main motivating ideas with a simple example.
}


\section{Overview} %Motivation: Why we need a view mechanism over generalized sketches}
  \newcommand{\QQ}{\enma{\mathbf{Q}}}
  
 We discuss two main applications of the \fwk\ in SE in Sect.2.1-2, then discuss some mathematical aspects of the \fwk\ in Sect.2.3, and describe related work and contributions in Sect.2.4
  
%\subsection{Two Practical Applications}
%There are two practical issues that we aim to address with our \fwk. %: A) clean and formal notion of a view, and B) clean and formal algebra for model management, which we now discuss. 
\subsection{Views over sketches.} 
\label{sec:application1} 
Developing a complex software system normally requires working with multiple \emph{views} \cite{AtkinsonStollB2010} of the system: 
This is the only way to manage complexity and a cornerstone of system engineering, see \cite{FinkelsteinKramerNFG1992} for an early discussion and \cite{FeldmannKernschmidtWV2019,BruneliereBurgerCW2019,CicchettiCicozziP2019} for more recent reports and surveys. 
A view of a {\em source} artifact $S$ is, in general, not merely a part of $S$ or a projection of $S$, but typically involves some computation over $S$,  e.g. composing references, aggregating attributes by summing up their values etc, which extends $S$ with {\em derived} elements produced by some predefined operations (we will say {\em queries}) applied to $S$. Then a {\em view} can be defined as  a mapping $\frar{v}{V}{Q_v(S)}$ in a suitable category of software artifacts where the source $S$ and the view schema $V$ live, and  $Q_v$ is a query that provides an extension $Q_v(S)$ of source $S$ with derived elements required by the view. Note an important distinction from the ordinary Kleisli mappings defined for a given monad $\QQ$ or, at least, a global object mapping, which only potentially exists and seems unnecessary abstract for software engineers not familiar with Haskell. In contrast, in our notion of view, each view mapping $v$ carries its own query 
 $Q_v$ and maps to its own {\em local} extension $Q_v(S)$ rather than to a unified but huge global extension $\QQ(S)$.  
 \begin{includeShort}
 A simple example in Appendix \ref{sec:viewExample} shows how it works, and also demonstrates the importance of constraints for the view mechanisms. Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
\end{includeShort} 
\begin{includeLong}
	\input{sections/appendix4act20}
\end{includeLong}

\subsection{Algebra for model management.}\label{sec:application2}
 In \emph{model management},  models are manipulated as holistic entities, and replacement the one-object-at-a-time approach (micromanagement) by one-model-at-a-time (macromanagement)  turned out very productive \cite{Bernstein2003,%}.
% The respective research domain is called \emph{model management} \cite{
FavreNguyen2005,%Diskin2009,
PaigeKolovosRMW2013%DiskinKokalyM2013
}. It requires considering high-level operations on models such as model slicing, transformation, merging, and synchronization, and composing them into complex workflows  \cite{Diskin-sle13}. 
 \begin{wrapfigure}{r}{4cm}
 	\vspace{-2ex}
 	\centering
 	\includegraphics[width=\linewidth]{figures/modelMgmtsmall}
 	\caption{Model Management}
 	\label{fig:modelMgmt}
 	 \end{wrapfigure}
  %?????   model operations are inherently diagrammatic \cite{me-sle13,me-fase16}. 
  Fig.~\ref{fig:modelMgmt} shows a simple example in which two views of the same source are first matched, and then merged. One may think of this as taking the pullback and then the pushout, but in practice these ``pure'' categorical operations are often interwoven with some normalization procedures (and may require conflict resolution) so that even in this simple case the real workflow will be much richer. 
 %
 Importantly, models in SE are typically considered up to their auto-isomorphisms generated by permutations of OIDs (in the sense of OO programming)  which are irrelevant and normally not visible. It justifies making categories of models skeletal and having only identical auto\mor s, which makes limits and colimits  deterministic algebraic operations.  

Thus, for both the inter-model and the intra-model levelsof reasoning, SE needs powerful and formally specified algebraic machinery for diagrammatic operations. On the other hand, it seems that even basic universal algebraic constructs (signature, term, parsing) have not been accurately specified for diagrammatic operations, especially when the latter are considered together with pre-and post-conditions and hence are interwoven with logic; in this sense, we are developing some basic universal algebra for diagrammatic operations. 

\subsection{Mathematical aspects}
\subsubsection{Why generalized graphs and generalized sketches} %, and categorical signatures}

As discussed above, categories hosting software models are categories of sketches. % and their models (in the mathematical sense). 
In general, a sketch is a graphical structure endowed with labelled diagrams (a.k.a. constraints); in the project, we consider a very general version of the notion: our 'graphs' are finitary presheaves, and our constraints of shape $G$ are any ``devices'' that classify mappings from $G$ as either valid or invalid. The generality of our graphs is caused by the great diversity and complexity of graphical structures used in SE  \cite{Kent2002}, and graphs used for behavioural and workflow  models can even be more complex. %Hence, we consider a very general notion of a graph as being a presheaf \frar{G}{\HH}{\setcat}  whose schema $\HH$ is any finite category. \footnote{In the long version, we consider an important requirement to \HH\ motivated by other parts of the project, but it is not needed for results described in the present paper.}
Similarly, constraints used in domain modelling (banking, e-commerce, automotive etc.) can be complex and very elementwise-oriented so that their representation in a standard categorical way via universal properties can be rather bulky and unwieldy (a detailed discussion can be found in \cite{DiskinWolter2008}, see also Appendix). Thus, we need  constraints and sketches of a very general nature that Michael Makkai called {\em generalized sketches} \cite{Makkai1997}.  %Diagrammatic constraints are an integral part of the domain and software modelling, and  important for specifying correct view mappings. Hence, we need to consider graphs endowed with constraints declared over them, \ie, graphical/diagrammatic theories or {\em ()generalized) sketches}. Thus, our category of artifacts and their mappings should be a category of sketches and sketch \mor s.
%
%\subsubsection{Signatures are categories}
%DEPENDENCIES ARE IMPORTANT ...... BLAH-BLAH
%\subsection{Mathematical issues}
\subsubsection{String diagrams do not work for diagram operations}
\newcommand{\propcat}{\enma{\catname{PROP}}}
%The objects in a PROP are natural numbers (arities) and arrows represent operations where domain and codomain denote in- and output arity. Being symmetric monoidal (sm) categories, $\catname{PROPs}$ can be  visualized with String Diagrams \cite{Selinger2011}, an intuitive yet formal graphical syntax.
For \propcat s, terms can be specified by string diagrams as shown in 
Fig.~\ref{fig:exSMC}, which depicts a ternary term $(x + y) * (x + z)$ built from two binary operations. % in string diagram notation, which is a ternary operation ($\in \catname{PROP}(3,1)$) where 
Note that reuse of the middle variable $y$  is shown explicitly with  $\nfont{Copy}$-operation (visualized via \includegraphics[width=1em]{figures/Copy}). This is possible as 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/StringDiagram}
	\caption{String diagram notation for ordinary algebraic terms}
	\label{fig:exSMC}
\end{figure}
%Unfortunately, we cannot use this machinery for diagram operations. The classical operations are \setcat-based and 
set $\{x, y, z\}$ is the coproduct of its elements $\{x\}\sqcup\{y\}\sqcup \{z\}$.
However,  diagram operations are graph-based,  %\footnote{Throughout this paper we will use the term ``graph'' in a more general sense, see Sect.~\PAST{Reminder to put the correct reference}}.
and a graph (while being a colimit of its elements) is not their coproduct!
\input{figures/insert-ex3pb}
Consider Fig.~\ref{fig:ex3pb} presenting a simple diagram chasing piece. % \} as used in many categorical proofs denoted in different visual syntaxes. 
Part (A) uses a typical categorical notation: the diagram presents a workflow consisting of two pullbacks taken in parallel over spans with one monic leg, followed by yet another pullback. Monic preservation by pullbacks is also shown. %In addition,  by naming conventions and respective symbols in the corners we show that some elements in the diagram are constructed via pullbacks, and via arrow decorations we specify some of the arrows to have special properties (being monic).
Part (B) makes the above explicit by using labels for constraint declarations (ovals) and operation applications (chevrons), and showing their scope. % make the stion elements in the diagram are explicated. 
Note that arrows going in and out of chevrons  show the workflow and what elements are constructed/derived (blue and dashed) rather than given. 
Part (C) is similar to Fig.~\ref{fig:exSMC} and highlights the workflow of the query by making the order of operation applications explicit, e.g. the pullback \nfont{c} depends on elements produced by the other two pullbacks.

Note several important differences with Fig.~\ref{fig:exSMC}. First, in discrete $\catname{PROP}$-setting, the elements produced by an operation have no further relationship with the input elements, while in the graph-based setting, there is an overlap between the input and the output, e.g. element $B$ in \figref{ex3pb}(B) is both in the input and the output of the pullback application \nfont{a}, and similarly for application \nfont{b} so that $B$ is also shared by \nfont{a}-output and \nfont{b}-output. Second, the workflow shown in \figref{ex3pb}(C) is a rather poor view of the actual workflow under the hood, which consists of several pushouts (POs): three POs are needed to produce graph $X'$ and yet another one to produce $X''$. Workflow arrows with hollow ends are, in fact, pairs, $(X,a)$, $(X,b)$ etc.,  while mappings that do the job, \eg, the one showing what part of graph $X$ is used as an input for \nfont{a{:}[pb]}, are not shown. %etc., and monics from $X$ to $X'$ to $X''$, are not shown. 
Thus, in contrast to \figref{exSMC}, diagram \figref{ex3pb}(C) is an incomplete specification of the story.  

\subsection{Related Work and Contributions}
%\zd{Phrase about the diversity of the pool of notions....}
By {\em logic} we refer to work on generalized sketches, and {\em algebra} refers to work on signatures of operation symbols, terms and algebras over them. 

\vspace{-0.25cm}
\subsubsection{Logic.}
Several authors noticed that Ehresmann's sketches can be applied to data modelling \cite{LellahiSpyratos1991,Piessens-tac95,JohnsonRosebrugh2002}. %,Diskin-adbis97}, 
%A majority of these application basically rely on the concept of a \emph{sketch}  introduced by Ehresmann, i.e. a graphical counterpart of a logical theory  (see \cite{Wells} for the history and  \cite{AdamekRosicky1994} for references about their equivalent expressiveness). %and classical Ehresmann's skecthes were employed in all works cited above besides those by D \cite{LellahiSpyratos1991,Piessens-,JohnsonRD-audb01}. 
%By sketch we refer the classical notion introduced by Ehresmann and promoted in \cite{BarrWells1990} and a more \emph{generalized} variant introduced by Makkai \cite{Makkai1997}).
However, these sketches are based on universal properties of the \corring\ (limit, colimit, powerobject) diagrams, which (as we discussed above) is a too restrictive setting for applications. %(see \cite{DiskinWolter2008} for a discussion). 
A suitable generalization of sketches by exactly this reason was independently introduced by Diskin \cite{Diskin-sketches96,Diskin1997}, and even earlier, in a very  different context of an abstract approach to logic, by Makkai \cite{Makkai1997} (whose preprints had been circulating in early 90s). Makkai developed a coherent theory of generalized sketches and proved a fundamental result that any category of sketches is a presheaf topos. Hence, sketches in a signature $\PP_1$ can be considered graphs over which a new signature $\PP_2$ and hence a new category of $\PP_2$-sketches can be defined, and so on. In this way, Makkai specified categories with several layers of additional structure as sketches. In our project, we use a different approach in which all discrete signatures $\PP_i$ are integrated into one signature-category $\int_i\PP_i$, whose arrows describe  dependencies between predicate symbols extracted from arities (details can be found in \cite[Sect.3]{THETR}). In the TR we prove that Makkai's theorem can be extended for categorical signatures so that the slogan ``sketches are graph'' persists (see Th.~\ref{thm:genMakkaiShort} below for a precise formulation). 
%: given a presheaf topos of graphs $\GG=\setcat^\HH$ for some schema category \HH, and a set of predicate symbols \PP\ whose arities are \HH-graphs, \PP-sketches whose carriers are \HH-graphs can be considered presheaves on a special (collage) category 
Also, while traditionally sketches are defined in an {\em indexed} way as  families of sets of diagrams indexed by predicate symbols  (for the discrete signature case), or functors {\em from} the signature (for the categorical signature case \cite{DiskinWolter2008}), we define them in an equivalent {\em fibrational} way via a discrete opfibration functor {\em into} the signature: the fibrational definition is more compact and often simplifies technicalities.  

\begin{includeLong}
We need to distinguish between several notions of signatures and sketches. We call logic {\em basic} if signatures of predicate symbols are sets considered as discrete categories. We call it {\em advanced}, if signatures are categories whose arrows are dependencies between predicates; in addition, these arrows are required to go in one direction, which makes signature \cats\ {\em \hical} (a version of Lawvere's one-way categories). Traditionally, sketches are defined in an indexed way as families of sets of diagrams indexed by symbols in the discrete signature case, and functors into \setcat\ for categorical signatures. We define them in an equivalent {\em fibrational} way via a discrete opfibration functor into the signature. There is also an important distinction between {\em -multi-}sketches that allow the same labelled diagram appear in a sketch for multiple times, and {\em mono-}sketches that disallow this. Finally, a partially de-categorificated approach (due to Makkai) is to consider signatures as layered sets so that each predicate in layer $(n+1)$ implicitly depends on all predicates in layer $n$. However, when arities of $(n+1)$-predicates are defined based on $n$-predicates, the actual dependencies appear on the stage. We call this approach {\em discrete \hical (dh)} and show that it is actually equivalent to the categorical one. In these terms, Table \ref{tab:contributionLogic} shows the previous work and contributions of our project. Our main result is an extension of a fundamental Makkai's theorem (that multi-sketches are actually presheaves) for the case of categorical signatures with dependencies: see Th.~\ref{thm:genMakkaiShort} in the paper. 
%Naively speaking the contribution of our work can be described as formalization of diagram chasing as e.g. in Fig.~\ref{fig:ex3pb}:
%We formally define diagram operations, diagram algebras and queries (= terms) and show elementary results known from classical algebra to hold in this setting:
%Queries extend to a functor $Q$, algebras are arrows $\frar{a}{Q(A)}{A}$ and there is (symmetric monoidal) Kleisli-Category w.r.t. $Q$, hence the latter also becomes a monad.
%The results are first presented in a discrete setting, i.e. without relations between operations, and then extended to a more general setting with relations between operations, which are needed for syntactical reasoning.
\begin{table}[]
	\scriptsize
	\begin{tabular}{|l|l||l|l|l|}
		\hline
		\multicolumn{2}{|l|}{\multirow{2}{*}{\diagbox{Sketch Notion}{Setting}}} & \multirow{2}{*}{One-Layer (Basic Logic)} & \multicolumn{2}{l|}{Multi-Layer (Advanced Logic)}                          \\ \cline{4-5} 
		\multicolumn{2}{|l|}{}                  &                                          & Discrete Hierarchical         & Categorical                                \\ \hline \hline
		\multirow{2}{*}{Indexed}       & mono   & \multicolumn{2}{c|}{\multirow{2}{*}{\cite{Makkai1997}}}                             & \cite{DiskinWolter2008}                                     \\ \cline{2-2} \cline{5-5} 
		& multi  & \multicolumn{2}{c|}{}                                                    & TR: Sect.3.2                               \\ \hline
		\multirow{2}{*}{Fibrational}   & mono   & \multirow{2}{*}{TR: Sect.2.2.-2.3}       & \multirow{2}{*}{TR: Sect.3.4} & \multirow{2}{*}{Paper: Sect.3; TR: Sect.3} \\ \cline{2-2}
		& multi  &                                          &                               &                                            \\ \hline
	\end{tabular}
	\caption{Contributions: Diagram Logic}
\label{tab:contributionsLogic}
\end{table}
\end{includeLong}

\subsubsection{Algebra.}
Diagram operation signatures and algebras were defined first in \cite{Diskin1997} and with some additional details in  \cite{Diskin-sketches96}, but no mathematical results were obtained. For the special case of operations over ordinary graphs, Wolter \etal\ \cite{WolterDiskinK2018} proved that any signature of such operations generates a monad (\ie, a global construct) over the category of graphs. The machinery of {\em local} Kleisli mappings explained informally was used in several papers of the first author, \eg,  \cite{Diskin-models10,Diskin-fase17}, and formalized as Kleisli mappings of a monad (\ie, globally) in \cite{Diskin-fase12}; we are not aware of an accurate formalization of Kleisli mappings considered locally as is done in our project,  nor of several other results reported in Sect.4. Specifically, we prove that a) sketches and local Kleisli mappings (views) between them form a symmetric monoidal category,  and b) the local Kleisli composition gives rise to a Kleisli triple and hence a  monad (as expected).  
\begin{includeLong}
\begin{table}[h]
	\scriptsize
	\begin{tabular}{|l||p{4cm}|p{3.75cm}|}
		\hline
		\diagbox{Topic}{Setting} & Discrete                                                                                & \parbox{3cm}{Categorical \\ (Dependencies)} \\ \hline\hline
		Signatures  and Algebras         & 
		\parbox{3.75cm}{Paper: Sect.4; TR: Sect.5.1; \cite{WolterDiskinK2018}  (graph operations) }                   & TR: Sect.6.1.1 (Defs. only)                     \\ \hline
		Multiqueries and Substitution   & Paper: Sect.4 (Defs. only); TR: Sect.5.2                                                                                & TR: Sect.6.1.2 (Defs. only)                     \\ \hline
		Complex Queries and Composition & Paper: Sect.4; TR: Sect.5.3                                                                               & TR: Sect.6.1.3 (Defs. only)                     \\ \hline
		Monads                          & \parbox{4cm}{Paper: Sect.4; TR: Sect.5.4; \cite{WolterDiskinK2018}  (graph term algebra adjunction)} & TR: Sect.6.1.4 (Conjecture)                    \\ \hline
	\end{tabular}
	\caption{Contributions: Diagram Algebra}
	\label{tab:contributionsAlgebra}
\end{table}
\end{includeLong}
\subsection{Notation.}

\endinput
\zd{more refs would be useful} and then queries become complex diagram operations over graphical structures. \zd{In practice, queries and operations are formally defined on the level of code but rather dirty (informal, approximate) on the level of models -- hence, our interest to make it clean... } %Conceptual graphical artifacts play an important role in SE and are used to specify different aspects of the system under development \cite{Kent2002}.
%
%The above notion can be further abstracted into a Kleisli-arrow $\relationarrow{V}{v}{S}$, which was discovered and presented to the SE-community in \cite{me-fase12}.
\zd{Note also that we cannot use monads as ...... }

==> sections/intros/intro-new.tex <==

\section{Introduction}


A diagrammatic operation takes a diagram of a specified shape as its input, and extends it with new elements forming a bigger diagram of a specified shape; we will say that the input diagram is {\em completed} by the operation. 
For example,  arrow composition takes two consecutive arrows and completes them with a third arrow forming the \corring\ triangle.  %This list of examples can be extended indefinitely: 
The resulting diagram often satisfies some postconditions, \eg, a chosen pullback completes a cospan with a {\em commutative} square, and a chosen powerobject completes an object with its {\em jointly-monic} membership span. Preconditions are needed too, \eg, adhesive 
%HLR categories \cite{EhrigHabelPP2004} 
categories only provide pushouts for one-leg-monic spans (and then we know that the \corring\ leg of the resulting cospan is also monic). Thus, categorical diagram operations come together with reasoning over them so that diagram algebra and logic are smoothly integrated in diagram chasing routines. 

This paper stems from the observation that the diagram chasing idea transcends Category Theory (CT) and finds numerous applications in the practice of Software Engineering (SE), in which, however,  it is currently used in an ad-hoc way: implicit, semi-formal or formal but buried in code so that the underlying diagram chasing procedures are blurred and distorted.  
The negative impact of these issues increases with the recent advent of Model Driven Engineering (MDE), in which \diatic\ models rather than code become the primary artifacts of software development. 

\shortlong{
Our goal in the project reported in the present  paper%
\footnote{which is an extended abstract of ongoing work in progress, whose current state is reported in the technical report \citeTR (further referred to as ``the TR'')}
 is to provide an accurate formalization of diagrammatic reasoning routines adequate to their practical use in MDE. We will discuss this in more detail in the next section along with several mathematically interesting structures and results emerged along the course, and our contributions.  Sections 3 and 4 provide basic formal definitions and results, and Sect.5 concludes.  Appendix A is optional but helpful: it illustrates main motivating ideas with a simple example.
}{ %endShort/BeginLOng
Our goal in the project reported in the present technical report (further TR) 
%\footnote{which is an extended abstract of ongoing work in progress, whose current state is reported in the technical report \citeTR (further referred to as ``the TR'')}
is to provide an accurate formalization of diagrammatic reasoning routines adequate to their practical use in MDE. We will briefly discuss this in the next section (Sect. 2.1-2) along with several mathematically interesting structures and results emerged along the course (in Sect. 2.3); a brief survey of related work and our contributions are in %, and a road map of the TR (Sect.2.4)
Sect. 2.4. We also describe a simple example of domain modelling motivating generalized sketches as the main underlying machinery in Sect. 2.5, and overview our notation in Sect. 2.6. Section 3 gives three brief introductions to our three main subjects: \diatic\ logic, \diatic\ algebra, and \diatic\ reasoning. Sections 4-6 present technical development: in Sect.4 we consider sketches over predicate signatures (with or without dependencies between predicates), and in Sections 5-6 complex queries built from \diatic\ operations (the case of operation without dependencies is in Sect. 5 and the general case with dependencies in Sect. 6; the latter is is in progress and currently only provides basic definitions). %Since Section 5, we assume categories of sketches to be skeletal
Section 7 concludes.  % Sections 3 and 4 provide basic formal definitions and results, and Sect.5 concludes.  Appendix A is optional but helpful: it illustrates main motivating ideas with a simple example.
}

\endinput


\section{Overview} %Motivation: Why we need a view mechanism over generalized sketches}
  \renewcommand{\QQ}{\enma{\mathbf{Q}}}
  
 We discuss two main applications of the \fwk\ in SE in Sect.2.1-2, then discuss some mathematical aspects of the \fwk\ in Sect.2.3, and describe related work and contributions in Sect.2.4
  
%\subsection{Two Practical Applications}
%There are two practical issues that we aim to address with our \fwk. %: A) clean and formal notion of a view, and B) clean and formal algebra for model management, which we now discuss. 
\subsection{Views over sketches.} 
\label{sec:application1} 
Developing a complex software system normally requires working with multiple \emph{views} \cite{AtkinsonStollB2010} of the system: 
This is the only way to manage complexity and a cornerstone of system engineering, see \cite{FinkelsteinKramerNFG1992} for an early discussion and \cite{FeldmannKernschmidtWV2019,BruneliereBurgerCW2019,CicchettiCicozziP2019} for more recent reports and surveys. 
A view of a {\em source} artifact $S$ is, in general, not merely a part of $S$ or a projection of $S$, but typically involves some computation over $S$,  e.g. composing references, aggregating attributes by summing up their values etc, which extends $S$ with {\em derived} elements produced by some predefined operations (we will say {\em queries}) applied to $S$. Then a {\em view} can be defined as  a mapping $\frar{v}{V}{Q_v(S)}$ in a suitable category of software artifacts where the source $S$ and the view schema $V$ live, and  $Q_v$ is a query that provides an extension $Q_v(S)$ of source $S$ with derived elements required by the view. Note an important distinction from the ordinary Kleisli mappings defined for a given monad $\QQ$ or, at least, a global object mapping, which only potentially exists and seems unnecessary abstract for software engineers not familiar with Haskell. In contrast, in our notion of view, each view mapping $v$ carries its own query 
 $Q_v$ and maps to its own {\em local} extension $Q_v(S)$ rather than to a unified but huge global extension $\QQ(S)$.  
 \begin{includeShort}
 A simple example in Appendix \ref{sec:viewExample} shows how it works, and also demonstrates the importance of constraints for the view mechanisms. Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
\end{includeShort} 
%\begin{includeLong}
%	\input{sections/appendix4act20}
%\end{includeLong}

\subsection{Algebra for model management.}\label{sec:application2}
 In \emph{model management},  models are manipulated as holistic entities, and replacement the one-object-at-a-time approach (micromanagement) by one-model-at-a-time (macromanagement)  turned out very productive \cite{Bernstein2003,%}.
% The respective research domain is called \emph{model management} \cite{
FavreNguyen2005,%Diskin2009,
PaigeKolovosRMW2013%DiskinKokalyM2013
}. It requires considering high-level operations on models such as model slicing, transformation, merging, and synchronization, and composing them into complex workflows  \cite{Diskin-sle13}. 
 \begin{wrapfigure}{r}{4cm}
 	\vspace{-2ex}
 	\centering
 	\includegraphics[width=\linewidth]{figures/modelMgmtsmall}
 	\caption{Model Management}
 	\label{fig:modelMgmt}
 	 \end{wrapfigure}
  %?????   model operations are inherently diagrammatic \cite{me-sle13,me-fase16}. 
  Fig.~\ref{fig:modelMgmt} shows a simple example in which two views of the same source are first matched, and then merged. One may think of this as taking the pullback and then the pushout, but in practice these ``pure'' categorical operations are often interwoven with some normalization procedures (and may require conflict resolution) so that even in this simple case the real workflow will be much richer. 
 %
 Importantly, models in SE are typically considered up to their auto-isomorphisms generated by permutations of OIDs (in the sense of OO programming)  which are irrelevant and normally not visible. It justifies making categories of models skeletal and having only identical auto\mor s, which makes limits and colimits  deterministic algebraic operations.  

Thus, for both the inter-model and the intra-model levelsof reasoning, SE needs powerful and formally specified algebraic machinery for diagrammatic operations. On the other hand, it seems that even basic universal algebraic constructs (signature, term, parsing) have not been accurately specified for diagrammatic operations, especially when the latter are considered together with pre-and post-conditions and hence are interwoven with logic; in this sense, we are developing some basic universal algebra for diagrammatic operations. 

\subsection{Mathematical aspects}
\subsubsection{Why generalized graphs and generalized sketches} %, and categorical signatures}

As discussed above, categories hosting software models are categories of sketches. % and their models (in the mathematical sense). 
In general, a sketch is a graphical structure endowed with labelled diagrams (a.k.a. constraints); in the project, we consider a very general version of the notion: our 'graphs' are finitary presheaves, and our constraints of shape $G$ are any ``devices'' that classify mappings from $G$ as either valid or invalid. The generality of our graphs is caused by the great diversity and complexity of graphical structures used in SE  \cite{Kent2002}, and graphs used for behavioural and workflow  models can even be more complex. %Hence, we consider a very general notion of a graph as being a presheaf \frar{G}{\HH}{\setcat}  whose schema $\HH$ is any finite category. \footnote{In the long version, we consider an important requirement to \HH\ motivated by other parts of the project, but it is not needed for results described in the present paper.}
Similarly, constraints used in domain modelling (banking, e-commerce, automotive etc.) can be complex and very elementwise-oriented so that their representation in a standard categorical way via universal properties can be rather bulky and unwieldy (a detailed discussion can be found in \cite{DiskinWolter2008}, see also Appendix). Thus, we need  constraints and sketches of a very general nature that Michael Makkai called {\em generalized sketches} \cite{Makkai1997}.  %Diagrammatic constraints are an integral part of the domain and software modelling, and  important for specifying correct view mappings. Hence, we need to consider graphs endowed with constraints declared over them, \ie, graphical/diagrammatic theories or {\em ()generalized) sketches}. Thus, our category of artifacts and their mappings should be a category of sketches and sketch \mor s.
%
%The classic Ehresmann sketches consider signatures that only contain classes of limit and colimit predicates whose semantics are given by the respective universal properties. Generalized sketches moreover consider arbitrary predicates, where semantics are defined externally. This allows for more compact specifications because one does not need to add auxiliary structures as it is often required with classical sketches, cf. \cite{JohnsonRosebrugh2002}.


\subsubsection{String diagrams do not work for diagram operations}
\newcommand{\propcat}{\enma{\catname{PROP}}}
%The objects in a PROP are natural numbers (arities) and arrows represent operations where domain and codomain denote in- and output arity. Being symmetric monoidal (sm) categories, $\catname{PROPs}$ can be  visualized with String Diagrams \cite{Selinger2011}, an intuitive yet formal graphical syntax.
For \propcat s, terms can be specified by string diagrams as shown in 
Fig.~\ref{fig:exSMC}, which depicts a ternary term $(x + y) * (x + z)$ built from two binary operations. % in string diagram notation, which is a ternary operation ($\in \catname{PROP}(3,1)$) where 
Note that reuse of the middle variable $y$  is shown explicitly with  $\nfont{Copy}$-operation (visualized via \includegraphics[width=1em]{figures/Copy}). This is possible as 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/StringDiagram}
	\caption{String diagram notation for ordinary algebraic terms}
	\label{fig:exSMC}
\end{figure}
%Unfortunately, we cannot use this machinery for diagram operations. The classical operations are \setcat-based and 
set $\{x, y, z\}$ is the coproduct of its elements $\{x\}\sqcup\{y\}\sqcup \{z\}$.
However,  diagram operations are graph-based,  %\footnote{Throughout this paper we will use the term ``graph'' in a more general sense, see Sect.~\PAST{Reminder to put the correct reference}}.
and a graph (while being a colimit of its elements) is not their coproduct!
\input{figures/insert-ex3pb}
Consider Fig.~\ref{fig:ex3pb} presenting a simple diagram chasing piece. % \} as used in many categorical proofs denoted in different visual syntaxes. 
Part (A) uses a typical categorical notation: the diagram presents a workflow consisting of two pullbacks taken in parallel over spans with one monic leg, followed by yet another pullback. Monic preservation by pullbacks is also shown. %In addition,  by naming conventions and respective symbols in the corners we show that some elements in the diagram are constructed via pullbacks, and via arrow decorations we specify some of the arrows to have special properties (being monic).
Part (B) makes the above explicit by using labels for constraint declarations (ovals) and operation applications (chevrons), and showing their scope. % make the stion elements in the diagram are explicated. 
Note that arrows going in and out of chevrons  show the workflow and what elements are constructed/derived (blue and dashed) rather than given. 
Part (C) is similar to Fig.~\ref{fig:exSMC} and highlights the workflow of the query by making the order of operation applications explicit, e.g. the pullback \nfont{c} depends on elements produced by the other two pullbacks.

Note several important differences with Fig.~\ref{fig:exSMC}. First, in discrete $\catname{PROP}$-setting, the elements produced by an operation have no further relationship with the input elements, while in the graph-based setting, there is an overlap between the input and the output, e.g. element $B$ in \figref{ex3pb}(B) is both in the input and the output of the pullback application \nfont{a}, and similarly for application \nfont{b} so that $B$ is also shared by \nfont{a}-output and \nfont{b}-output. Second, the workflow shown in \figref{ex3pb}(C) is a rather poor view of the actual workflow under the hood, which consists of several pushouts (POs): three POs are needed to produce graph $X'$ and yet another one to produce $X''$. Workflow arrows with hollow ends are, in fact, pairs, $(X,a)$, $(X,b)$ etc.,  while mappings that do the job, \eg, the one showing what part of graph $X$ is used as an input for \nfont{a{:}[pb]}, are not shown. %etc., and monics from $X$ to $X'$ to $X''$, are not shown. 
Thus, in contrast to \figref{exSMC}, diagram \figref{ex3pb}(C) is an incomplete specification of the story.  

\subsection{Related Work and Contributions}
%\zd{Phrase about the diversity of the pool of notions....}
By {\em logic} we refer to work on generalized sketches, and {\em algebra} refers to work on signatures of operation symbols, terms and algebras over them. 

\vspace{-0.25cm}
\subsubsection{Logic.}
Several authors noticed that Ehresmann's sketches can be applied to data modelling \cite{LellahiSpyratos1991,Piessens-tac95,JohnsonRosebrugh2002}. %,Diskin-adbis97}, 
%A majority of these application basically rely on the concept of a \emph{sketch}  introduced by Ehresmann, i.e. a graphical counterpart of a logical theory  (see \cite{Wells} for the history and  \cite{AdamekRosicky1994} for references about their equivalent expressiveness). %and classical Ehresmann's skecthes were employed in all works cited above besides those by D \cite{LellahiSpyratos1991,Piessens-,JohnsonRD-audb01}. 
%By sketch we refer the classical notion introduced by Ehresmann and promoted in \cite{BarrWells1990} and a more \emph{generalized} variant introduced by Makkai \cite{Makkai1997}).
However, these sketches are based on universal properties of the \corring\ (limit, colimit, powerobject) diagrams, which (as we discussed above) is a too restrictive setting for applications. %(see \cite{DiskinWolter2008} for a discussion). 
A suitable generalization of sketches by exactly this reason was independently introduced by Diskin \cite{Diskin-sketches96,Diskin1997}, and even earlier, in a very  different context of an abstract approach to logic, by Makkai \cite{Makkai1997} (whose preprints had been circulating in early 90s). Makkai developed a coherent theory of generalized sketches and proved a fundamental result that any category of sketches is a presheaf topos. Hence, sketches in a signature $\PP_1$ can be considered graphs over which a new signature $\PP_2$ and hence a new category of $\PP_2$-sketches can be defined, and so on. In this way, Makkai specified categories with several layers of additional structure as sketches. In our project, we use a different approach in which all discrete signatures $\PP_i$ are integrated into one signature-category $\int_i\PP_i$, whose arrows describe  dependencies between predicate symbols extracted from arities (details can be found in \cite[Sect.3]{THETR}). In the TR we prove that Makkai's theorem can be extended for categorical signatures so that the slogan ``sketches are graph'' persists (see Th.~\ref{thm:genMakkai} below for a precise formulation). 
%: given a presheaf topos of graphs $\GG=\setcat^\HH$ for some schema category \HH, and a set of predicate symbols \PP\ whose arities are \HH-graphs, \PP-sketches whose carriers are \HH-graphs can be considered presheaves on a special (collage) category 
Also, while traditionally sketches are defined in an {\em indexed} way as  families of sets of diagrams indexed by predicate symbols  (for the discrete signature case), or functors {\em from} the signature (for the categorical signature case \cite{DiskinWolter2008}), we define them in an equivalent {\em fibrational} way via a discrete opfibration functor {\em into} the signature: the fibrational definition is more compact and often simplifies technicalities.  

\begin{includeLong}
We need to distinguish between several notions of signatures and sketches. We call logic {\em basic} if signatures of predicate symbols are sets considered as discrete categories. We call it {\em advanced}, if signatures are categories whose arrows are dependencies between predicates; in addition, these arrows are required to go in one direction, which makes signature \cats\ {\em \hical} (a version of Lawvere's one-way categories). Traditionally, sketches are defined in an indexed way as families of sets of diagrams indexed by symbols in the discrete signature case, and functors into \setcat\ for categorical signatures. We define them in an equivalent {\em fibrational} way via a discrete opfibration functor into the signature. There is also an important distinction between {\em -multi-}sketches that allow the same labelled diagram appear in a sketch for multiple times, and {\em mono-}sketches that disallow this. Finally, a partially de-categorificated approach (due to Makkai) is to consider signatures as layered sets so that each predicate in layer $(n+1)$ implicitly depends on all predicates in layer $n$. However, when arities of $(n+1)$-predicates are defined based on $n$-predicates, the actual dependencies appear on the stage. We call this approach {\em discrete \hical (dh)} and show that it is actually equivalent to the categorical one. In these terms, Table \ref{tab:contributionsLogic} shows the previous work and contributions of our project. Our main result is an extension of a fundamental Makkai's theorem (that multi-sketches are actually presheaves) for the case of categorical signatures with dependencies: see Th.~\ref{thm:genMakkai} in the paper. 
%Naively speaking the contribution of our work can be described as formalization of diagram chasing as e.g. in Fig.~\ref{fig:ex3pb}:
%We formally define diagram operations, diagram algebras and queries (= terms) and show elementary results known from classical algebra to hold in this setting:
%Queries extend to a functor $Q$, algebras are arrows $\frar{a}{Q(A)}{A}$ and there is (symmetric monoidal) Kleisli-Category w.r.t. $Q$, hence the latter also becomes a monad.
%The results are first presented in a discrete setting, i.e. without relations between operations, and then extended to a more general setting with relations between operations, which are needed for syntactical reasoning.
\begin{table}[]
	\scriptsize
	\begin{tabular}{|l|l||l|l|l|}
		\hline
		\multicolumn{2}{|l|}{\multirow{2}{*}{\diagbox{Sketch Notion}{Setting}}} & \multirow{2}{*}{One-Layer (Basic Logic)} & \multicolumn{2}{l|}{Multi-Layer (Advanced Logic)}                          \\ \cline{4-5} 
		\multicolumn{2}{|l|}{}                  &                                          & Discrete Hierarchical         & Categorical                                \\ \hline \hline
		\multirow{2}{*}{Indexed}       & mono   & \multicolumn{2}{c|}{\multirow{2}{*}{\cite{Makkai1997}}}                             & \cite{DiskinWolter2008}                                     \\ \cline{2-2} \cline{5-5} 
		& multi  & \multicolumn{2}{c|}{}                                                    & TR: Sect.3.2                               \\ \hline
		\multirow{2}{*}{Fibrational}   & mono   & \multirow{2}{*}{TR: Sect.2.2.-2.3}       & \multirow{2}{*}{TR: Sect.3.4} & \multirow{2}{*}{Paper: Sect.3; TR: Sect.3} \\ \cline{2-2}
		& multi  &                                          &                               &                                            \\ \hline
	\end{tabular}
	\caption{Contributions: Diagram Logic}
\label{tab:contributionsLogic}
\end{table}
\end{includeLong}

\subsubsection{Algebra.}
Diagram operation signatures and algebras were defined first in \cite{Diskin1997} and with some additional details in  \cite{Diskin-sketches96}, but no mathematical results were obtained. For the special case of operations over ordinary graphs, Wolter \etal\ \cite{WolterDiskinK2018} proved that any signature of such operations generates a monad (\ie, a global construct) over the category of graphs. The machinery of {\em local} Kleisli mappings explained informally was used in several papers of the first author, \eg,  \cite{Diskin-models10,Diskin-fase17}, and formalized as Kleisli mappings of a monad (\ie, globally) in \cite{Diskin-fase12}; we are not aware of an accurate formalization of Kleisli mappings considered locally as is done in our project,  nor of several other results reported in Sect.4. Specifically, we prove that a) sketches and local Kleisli mappings (views) between them form a symmetric monoidal category,  and b) the local Kleisli composition gives rise to a Kleisli triple and hence a  monad (as expected).  
\begin{includeLong}
\begin{table}[h]
	\scriptsize
	\begin{tabular}{|l||p{4cm}|p{3.75cm}|}
		\hline
		\diagbox{Topic}{Setting} & Discrete                                                                                & \parbox{3cm}{Categorical \\ (Dependencies)} \\ \hline\hline
		Signatures  and Algebras         & 
		\parbox{3.75cm}{Paper: Sect.4; TR: Sect.5.1; \cite{WolterDiskinK2018}  (graph operations) }                   & TR: Sect.6.1.1 (Defs. only)                     \\ \hline
		Multiqueries and Substitution   & Paper: Sect.4 (Defs. only); TR: Sect.5.2                                                                                & TR: Sect.6.1.2 (Defs. only)                     \\ \hline
		Complex Queries and Composition & Paper: Sect.4; TR: Sect.5.3                                                                               & TR: Sect.6.1.3 (Defs. only)                     \\ \hline
		Monads                          & \parbox{4cm}{Paper: Sect.4; TR: Sect.5.4; \cite{WolterDiskinK2018}  (graph term algebra adjunction)} & TR: Sect.6.1.4 (Conjecture)                    \\ \hline
	\end{tabular}
	\caption{Contributions: Diagram Algebra}
	\label{tab:contributionsAlgebra}
\end{table}
\end{includeLong}
\subsection{Notation.}

\endinput
\zd{more refs would be useful} and then queries become complex diagram operations over graphical structures. \zd{In practice, queries and operations are formally defined on the level of code but rather dirty (informal, approximate) on the level of models -- hence, our interest to make it clean... } %Conceptual graphical artifacts play an important role in SE and are used to specify different aspects of the system under development \cite{Kent2002}.
%
%The above notion can be further abstracted into a Kleisli-arrow $\relationarrow{V}{v}{S}$, which was discovered and presented to the SE-community in \cite{me-fase12}.
\zd{Note also that we cannot use monads as ...... }

==> sections/intros/intro.tex <==
%!TEX root = ../lics20.tex

\section{Introduction}

\marginpar{xx} bbbb
\subsection{Motivation}

A diagrammatic operation takes a diagram of graphical elements (nodes, arrows, 2-arrows or, say, hyperedges, which can also be labelled) as its input, and completes it with new elements forming a bigger predefined shape. For example, the arrow composition takes two consecutive arrows and produces a third arrow making the triangle, pullback takes an arrow span and completes it up to a square, and  the universal property of pullback takes a pullback square and an commutative square completing the same span, and produces the universal comparison arrow. Besides being routinely used in categorical diagram chasing, such operations (and not necessarily categorical ones) are heavily used in practice of software engineering and databases. We can distinguish two major areas of their use. 

The first encompasses numerous applications in software engineering, in which one artifact/model/schema $V$ is a {\em view} of another (source) artifact $S$ in the technical sense that each element of $V$ is mapped to a basic or {\em derived} element of $S$. Such a mapping can be described as a Kleisli mapping for a suitable monad generated by operations with which $S$-elements are derived (see \eg, \cite{me-fase12}), but this description is far too general for practical tasks. In the latter, each view of $S$ comes with its own complex operation (term), say, \frar{v_1}{V_1}{Q_1(S)} and \frar{v_2}{V_2}{Q_2(S)}, where $Q_i$ is a term (we will say {\em query}) built from basic operations over an object $S$ of ``variables'', while the total ({\em global}) closure operator $\boldsymbol{Q}(S)$ encompassing all possible $Q_i(S)$ is not feasible and not used in practical reasoning. Thus, we need a {\em local} notion of a Kleisli mapping for diagrammatic operations over various graphical structures used in software engineering: graphs, bipartite graphs like Petri nets, 2-graphs, hypergraphs (including their various labelled versions), block diagrams, workflows, etc.

The second area is {\em model management}, in which one needs to operate complex models as holistic entities: merge and intersect them, slice them, transform and synchronize them, and consider complex workflows composed from elementary operations \cite{me-sle13}.   
%in general, manipulate models in an algebraic way.  
It is now generally well understood that a natural way of doing model management is to organize models into a category, and model typical model management operations by suitable compositions of typical categorical operations, specifically limits and colimits (see, \eg, \cite{me-ecmfa15}). This effectively turns model management into an applied diagram chasing, in which the notion of a diagrammatic term/query/workflow is again central and requires an accurate formalization including parsing. Note that as models are typically considered up to their iso\mor\ caused by permutations of invisible object identifiers, categories of models are skeletal and hence limits and colimits become uniquely determined. 

Thus, in both areas we need a term-oriented algebraic \fwk, in which we can define and parse terms, and specify their composition. For the ordinary algebra, this is done with the notion of Lawvere theory, where atomic terms are arrows in a category and complex terms are built by (co)product and sequential composition; ultimately, this results in the notion of \nfont{Prop}. Unfortunately, this approach does not work for \diatic\ operations because of two (interrelated) issues. 

a) The output of a \diatic\ operation may (and typically does) overlap with the input: the arrow $a\comp b$ produced by composition has the same source with $a$ and the same target with $b$; the span produced by pullback shares its feet with the input cospan. Moreover, declaring postconditions of an operation, \eg, the commutativity of a pullback square, needs considering the entire diagram ``covered'' by the operation, which we will call its {\em scope}. Thus, rather than viewing an operation as an Input-Output (IO) device, diagram algebra needs the Input-scopE (IE) approach, in which the result of an operation is considered as a completion of its input. 

b) For the \nfont{Prop} machinery, it is crucial that a set is a coproduct of its elements, say, $\{x, y\} =\{x\}\sqcup\{y\}$, which does not hold for graphs: the latter are colimits of the \corring\ diagrams of their elements but not coproducts. 
%
The difference is illustrated by \figref{ex++} and \figref{ex3pb}. The former shows a string diagram specifying a simple term in a signature consisting of two binary operations $+$ and $*$ built with  a set of variables $X=\{x,y,z\}$.   
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/StringDiagram}
	\caption{String diagram notation for ordinary algebraic terms}
	\label{fig:ex++}
\end{figure}
%A major construct in the ordinary algebra is the notion of a derived operation (term) built from operation symbols and variables, \eg, $(x+y)\ast(y+z)$. 
Although the abstract syntax tree (AST) of this term has four leaves (inputs), the term denotes a ternary operation because two leaves refer to the same variable $y$. In the string diagram notation, the term would be encoded as shown in \figref{ex++}, where reuse of the same variable is shown with explicit $\nfont{Copy}$-operation (visualized via \includegraphics[width=1em]{figures/Copy}). 

\input{figures/insert-ex3pb}

However, this idea does not work for diagram operations because of the non-additive nature of graph formation as illustrated by \figref{ex3pb}. Diagram (A) shows a simple diagram chasing consisting of three pullback applications in a typical categorical notation (ignore the fact that some arrows are monic for a while); diagram (B) makes the workflow explicit by showing inputs and outputs of pullback applications \nfont{a,b,c} (note also that the input elements of the entire term are shown in black while derived are blue). % and makes the \diatic\ term structure explicit. %: while sets are coproducts of their elements, \eg, $\{x,y,z\}=\{x\}\uplus\{y\}\uplus\{z\}$, graphs cannot be represented in this way: a graph is a colimit of its arrows rather than a coproduct. 
Similarly to variable $y$ in the term in \figref{ex++}, the middle arrow $y$ in the input graph $X=\{x,y,z\}$ is reused twice but we cannot describe this by a string diagram similar to that in \figref{ex++} and need something different. We have two variants: diagram \figref{ex3pb}(b) specifies our \diatic\ term as a generalized sketch with operation (rather than predicate) labels, and diagram \figref{ex3pb}(c) specifies the term in an explicit workflow manner somewhat similar to \figref{ex++}. However, this similarity can be confusing as ``signal'' lines connecting functional blocks, for the \diatic\ case carry much more information than for ordinary string diagrams. 

%\subsection{Example of a query}\label{sec:queryexample}
%
%Consider again the example depicted in Figure~\ref{fig:runningExample} and this time especially at sub figure \ref{fig:univPBProp:2}. It makes the application of the three pullback operations (shown as chevrons) including their in- and output (shown as arrows) explicit. Furthermore, we visually distinguish elements that are given (colored black) and those computed by operations (colored blue). A straightforward way of formalizing this concept is by utilizing existing sketch machinery.

====
\zd{finish the piece about constraints and logic/reasoning below}
Constraints are a fundamental ingredient of the \mmt\ machinery: models are graphical structures satisfying a set of constraints declared in the (so called) metamodel; mathematically, a metamodel is a generalized sketch $S$, whose valid instances (models in the categorical logic sense) are sketch \mor s $S\rightarrow U$ into an appropriate semantic universe $U$. Typically, for normalized metamodels, $U=\setcat$, and for a general non-normalized case, $U=\nfont{Span}(\setcat)$. 
%The second source is purely mathematical: we would like to formalize the routine of diagram chasing in precise algebraic terms of diagrammatic operations over (generalized) sketches. 
A central feature of diagram chasing is integration of algebra and logic: if one leg of a span is monic, then the \corring\ leg of its pullback cospan is also monic so that pullback generates both new elements and statements about them. Makkai formalized diagram chasing in logical terms of {\em sketch implications} \cite{makkai-ske}, \ie, sketch morphisms \frar{i}{S}{S'}: a model sketch $M$ {\em satisfies} $i$, $M\models i$, if for any sketch morphism \frar{m}{S}{M} there is a \mor\ \frar{m'}{S'}{M} such that $i\comp m' =m$. This is a good mechanism for logical rules, but if $i$ actually specifies an algebraic operations so that there is only one such $m'$, we need to introduce an additional axiom \frar{u(i)}{S'_u}{S''_u} specifying the uniqueness of $m'$ in a direct logical way. %\footnote
{This is analogous to specifying a binary operation on numbers, say, +, by a ternary predicate $P_+$ along with an axiom $P_+(x,y,z)=P_+(x,y,z')\Rightarrow z=z'$.}
Of course, a direct specification of + as a binary operation is preferable in many contexts \zd{not sure the entire makkai piece is needed here}

\subsection{Contributions and the Structure of the paper}

\zd{Two tables and some comments around them}

%\subsection{Structure of the Paper}
%\zd{a piece about the structure of the paper. Examples are categorical just for ACT}

%\vspace{2cm}




%=======
%\END

\endinput
\zd{the previous text is in the intro file below the ``endinput''}


\zd{The previous Intro piece}

Lately there has been a significant rise of interest in \emph{Symmetric Monoidal Categories (SMCs)} across various areas of computer science and related disciplines: {control theory} and signal flow graphs \cite{BaezErbele2015},  {quantum computation} and the ZX calculus \cite{CoeckeDuncan2008} as well as \emph{concurrency} and Petri nets \cite{SobocinskiStephens2014}.
One of the reasons behind this rise is the fact that SMCs have powerful and intuitive visual representation mechanism given by \emph{string diagrams} \cite{Selinger2011}. Conversely, 
 string diagrams have rigorous formal interpretation and can thus be used for rigorous syntactical reasoning as shown in \cite{BonchiGaducciKSZ2018}
To put it in terms of \emph{logic}: String diagrams provide the basis for a sound and complete inference mechanism.
The theories that have been analyzed in these formal graphical reasoning systems so far, have been mainly of algebraic nature.
In terms of programming this means immutable data structures, i.e. every operation is a function that always produces new elements and never manipulates given input elements.
Moreover, do these new elements have no relation to the arguments, e.g. there is nor further structure that relates the number $5$, as a result of the addition $2+3$, to the numbers $2$ nor $3$. 

In Software Engineering (SE), however, internal structure and inter-relations between elements play an important role, think e.g. associations between classes in an UML class diagram, foreign keys between tables in a database schema, etc.
The precise definition of such structural relationships is paramount within the \emph{Model-Based} branch of Software Engineering (MBSE) which promotes shifting the focus from \emph{program code} to \emph{abstract models}, i.e. a structured assemblies of information representing aspects of the system under development.
Categories have played an important role in formal MBSE, namely (1) for formal constraint-based specification \cite{JohnsonRosebrugh2002,DiskinWolter2008} and (2) for implementation of rule-based transformation languages \cite{EhrigPfenderS1973}.
The latter has produced the more or less well-known \emph{Double-Pushout-Rewriting (DPO)} approach, a variant \cite{GaducciHeckel1998} of which, actually, has been used to implement the syntactic reasoning engine in \cite{BonchiGaducciKSZ2018}.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/ProcessWithData}
\caption{Process with Data}
\label{fig:processWithData}
\end{figure}
To motivate the importance of relations between input and outputs of an operation, consider figure~\ref{fig:processWithData}.
It shows a simplified model of a conference management system.
The models comprises a \emph{process} part, here denoted in the popular \emph{Business Process Model and Notation (BPMN}, and a \emph{data} part, denoted as an \emph{Unified Modeling Language (UML) class diagram (CD)}.
The process part specifies what activities are to be executed in which order, where every activity may consume or produce elements from the data part, e.g. after the activity \emph{Receive Review} has been executed the data structure \emph{Review} will be available.
Thus, we could consider the \emph{Review} entity as an output of \emph{Receive Review}, if we additionally consider the latter as an operation.
Furthermore, the resulting entity is not considered in isolation: It has an association back to the \emph{manuscript} it was based on.
Following this line of thought, process models, like those depicted in BPMN and similar notation can be interpreted as terms over operations that act on an underlying (data) structure.

Thus, in this paper we do not only want to bridge research on SMCs/String Diagrams and categorical data modeling but also provide the formal underpinning for workflow languages that consist of operations data structures.
The aforementioned bridge is given by a transition from $\mathbf{FinSet}$ to general \emph{sketches} \cite{Makkai1997} over arbitrary presheaf topoi.
The operations here are given through \emph{diagrammatic operations}, which represent a generalization of ``regular'' operations known from universal algebra.


==> sections/intros/intro4act21.tex <==
\section{Introduction}
% this piece is for mathematicians

Let $X$ be a system (an airplane, a vehicle, a robot, a video-conferencing  system, a vaccine, ...), or a new feature to be added to such a system (\eg, an Airplane Collision Avoidance System, Lane Keep Assist system in a vehicle,  a new interface to a video-conferencing system, or a new vaccine transportation system, ...), whose safety, security, reliability or other critical property is to be reliably assured in order to allow using this system in the everyday life.%
\footnote{\label{fnote:newFeature} 
If $F$ is a new feature to be added to $X$, then what is to be assured (for, say, safety assurance) is the claim $\Safe(X+F)$, which is not followed from $\Safe(X)$ and $\Safe(F)$; the latter claim cannot even be correctly defined. This aspect of assurance is often referred to as {\em non-compositionality}.
}
An {\em assurance case} is a document providing evidence and an argument based on it that the dependability claim about $X$ holds, %(briefly, providing sufficient evidence that $X$ is safe/secure... for its intended use), 
which $X$'s manufacturer/producer has to submit to a certifying authority (the {\em regulator}) to obtain a permission to produce and market $X$. The regulator is typically a federal or international  agency, but sometimes the producer and the regulator are two teams in the same company playing the corresponding roles. Irrespective to the organizational side, the regulator must intensely try to find breaches in the case and defeat it. In practice, the process often turns out to be  iterative but its final result is necessarily Boolean: either the assurance case is approved and the system is accepted for production and use, or the case is defeated and rejected.
%%
%The following quote from NASA's Technical Report \cite{RushbyNASA2015} 
%%by Rushby \etal\  
%describes the content and goals of assurance cases in a bit more detail:
%%Let us begin with a working definition of the goals of assurance cases taken from NASA's report \cite{RushbyNASA2015}: % by Rushby \etal:
%\begin{quote}
%	Assurance cases are a method for providing assurance for a system by giving an argument to justify a claim about the system, based on evidence about its design, development, and tested behaviour.  In comparison with assurance based on guidelines or standards (which essentially specify only the evidence to be produced), the chief novelty in assurance cases is provision of an explicit argument. In principle, this can allow assurance cases to be more finely tuned to the specific circumstances of the system, and more agile than guidelines in adapting to new techniques and applications.
%\end{quote}
%The last feature is rapidly becoming crucial in our time of the total AI expansion in all spheres of life with new types of systems and/or new use cases and interactions for  previous systems appearing ``daily''. Perhaps, we are moving in the direction of building and assessing assurance cases on the scale of a daily routine rather than an exceptionally complex project done by exceptionally skilled experts  as assurance experts seemingly tend to think---see Holloway's online course on assurance \cite{hollowayOnlineCourse}, where the exceptionality of assurance is stated in an elegant and  crystal clear way: 
%%\xend{}
%\begin{quotation}
%	I am quite sure that A. A. Milne did not have creating assurance cases in mind when he had Eeyore say {\em We can’t all, and some of us don’t. That’s all there is to it.} (Alan Milne, Winnie the Pooh \cite{Milne1928}). But it is apt none-the-less. Creating cogent assurance cases is not something that everyone can do.  
%\end{quotation}
%%\xend{}
%We will refer to this mismatch between `daily' and `exceptional' as the {\em exeptionality issue} of assurance.%
%\footnote{Here and further in the paper, I will write `the author' when expressing my subjective opinions, and `we' when  the reader is invited to join the author in considering a construct or discussing a subject.}
% A potentially detrimental impact of the issue on the development of the assurance industry is amplified by considerable costs of preparing and assessing assurance cases, which can even be greater than the cost of building the system (cf. \cite{MultilegBloomfield:2003} that points to two impressive examples: the French RER railway with a safety-critical system of about 20,000 lines of code  with 100 person years spent on safety assurance \cite{RailwayDBLP:conf/icse/GuihoH90}, and Space Shuttle code whose production and assurance according to NASA cost \$1,000 per line). %, and it is known that this contains many faults. For some systems, the levels of confidence needed seem so high as to be beyond what can be claimed from the deployment of feasible amounts of evidence in conventional arguments.
Assurance can (and often does) incur considerable costs, which can even be greater than the cost of building the system (cf. \cite{MultilegBloomfield:2003,adelard10} that point to two impressive examples: the French RER railway with a safety-critical system of about 20,000 lines of code  with 100 person years spent on safety assurance \cite{RailwayDBLP:conf/icse/GuihoH90}, and Space Shuttle code whose production and assurance according to NASA cost \$1,000 per line). %, and it is known that this contains many faults. For some systems, the levels of confidence needed seem so high as to be beyond what can be claimed from the deployment of feasible amounts of evidence in conventional arguments.
An essential part of this cost is due to what is considered to be an inherent non-automatability of assurance....

\endinput 
@inproceedings{DBLP:journals/corr/abs-2101-10484,
	author    = {Georgios Bakirtzis and
		Christina Vasilakopoulou and
		Cody Harrison Fleming},
	editor    = {David I. Spivak and
		Jamie Vicary},
	title     = {Compositional Cyber-Physical Systems Modeling},
	booktitle = {Proceedings of the 3rd Annual International Applied Category Theory
		Conference 2020, {ACT} 2020, Cambridge, USA, 6-10th July 2020},
	series    = {{EPTCS}},
	volume    = {333},
	pages     = {125--138},
	year      = {2020},
	url       = {https://doi.org/10.4204/EPTCS.333.9},
	doi       = {10.4204/EPTCS.333.9},
	timestamp = {Fri, 09 Apr 2021 18:27:18 +0200},
	biburl    = {https://dblp.org/rec/journals/corr/abs-2101-10484.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}
The exceptionality issue and the costs provide a practical justification for the quest of this paper for a transparent and well-structured formal \fwk\ for assurance %(in a much stronger sense of being structured than currently assumed in the assurance literature) 
\zdneww{based on established patterns of object-oriented modelling (OOM) and category theory. Indeed, first, a transparent structure and patterns could significantly reduce the complexity of building assurance cases and thus address the exceptionality issue and, second, a formalized \fwk\ makes assurance amenable to automation; both factors would significantly reduce the cost if properly realized.}{revise!!!}{-2em}    

\zd{What about adding a phrase about low value of automation in Holloway's course}

\zd{also, it's agood place to talk about Explicitness as a major proeprty of the argument but Alas, Rushby's def does not mentions it. }

==> sections/intros/intro4mathns.tex <==
\section{Introduction}
% this piece is for mathematicians

Let $X$ be a system (an airplane, a vehicle, a robot, a video-conferencing  system, a vaccine, ...), or a new feature to be added to such a system (\eg, an Airplane Collision Avoidance System, Lane Keep Assist system in a vehicle,  a new interface to a video-conferencing system, or a new vaccine transportation system, ...), whose safety, security, reliability or other critical property is to be reliably assured in order to allow using this system in the everyday life.%
\footnote{\label{fnote:newFeature} 
If $F$ is a new feature to be added to $X$, then what is to be assured (for, say, safety assurance) is the claim $\Safe(X+F)$, which is not followed from $\Safe(X)$ and $\Safe(F)$; the latter claim cannot even be correctly defined. This aspect of assurance is often referred to as {\em non-compositionality}.
}
An {\em assurance case} is a document providing evidence and an argument based on it that the dependability claim about $X$ holds, %(briefly, providing sufficient evidence that $X$ is safe/secure... for its intended use), 
which $X$'s manufacturer/producer has to submit to a certifying authority (the {\em regulator}) to obtain a permission to produce and market $X$. The regulator is typically a federal or international  agency, but sometimes the producer and the regulator are two teams in the same company playing the corresponding roles. Irrespective to the organizational side, the regulator must intensely try to find breaches in the case and defeat it. In practice, the process often turns out to be  iterative but its final result is necessarily Boolean: either the assurance case is approved and the system is accepted for production and use, or the case is defeated and rejected.
%%
%The following quote from NASA's Technical Report \cite{RushbyNASA2015} 
%%by Rushby \etal\  
%describes the content and goals of assurance cases in a bit more detail:
%%Let us begin with a working definition of the goals of assurance cases taken from NASA's report \cite{RushbyNASA2015}: % by Rushby \etal:
%\begin{quote}
%	Assurance cases are a method for providing assurance for a system by giving an argument to justify a claim about the system, based on evidence about its design, development, and tested behaviour.  In comparison with assurance based on guidelines or standards (which essentially specify only the evidence to be produced), the chief novelty in assurance cases is provision of an explicit argument. In principle, this can allow assurance cases to be more finely tuned to the specific circumstances of the system, and more agile than guidelines in adapting to new techniques and applications.
%\end{quote}
%The last feature is rapidly becoming crucial in our time of the total AI expansion in all spheres of life with new types of systems and/or new use cases and interactions for  previous systems appearing ``daily''. Perhaps, we are moving in the direction of building and assessing assurance cases on the scale of a daily routine rather than an exceptionally complex project done by exceptionally skilled experts  as assurance experts seemingly tend to think---see Holloway's online course on assurance \cite{hollowayOnlineCourse}, where the exceptionality of assurance is stated in an elegant and  crystal clear way: 
%%\xend{}
%\begin{quotation}
%	I am quite sure that A. A. Milne did not have creating assurance cases in mind when he had Eeyore say {\em We can’t all, and some of us don’t. That’s all there is to it.} (Alan Milne, Winnie the Pooh \cite{Milne1928}). But it is apt none-the-less. Creating cogent assurance cases is not something that everyone can do.  
%\end{quotation}
%%\xend{}
%We will refer to this mismatch between `daily' and `exceptional' as the {\em exeptionality issue} of assurance.%
%\footnote{Here and further in the paper, I will write `the author' when expressing my subjective opinions, and `we' when  the reader is invited to join the author in considering a construct or discussing a subject.}
% A potentially detrimental impact of the issue on the development of the assurance industry is amplified by considerable costs of preparing and assessing assurance cases, which can even be greater than the cost of building the system (cf. \cite{MultilegBloomfield:2003} that points to two impressive examples: the French RER railway with a safety-critical system of about 20,000 lines of code  with 100 person years spent on safety assurance \cite{RailwayDBLP:conf/icse/GuihoH90}, and Space Shuttle code whose production and assurance according to NASA cost \$1,000 per line). %, and it is known that this contains many faults. For some systems, the levels of confidence needed seem so high as to be beyond what can be claimed from the deployment of feasible amounts of evidence in conventional arguments.
Assurance can (and often does) incur considerable costs, which can even be greater than the cost of building the system (cf. \cite{MultilegBloomfield:2003,adelard10} that point to two impressive examples: the French RER railway with a safety-critical system of about 20,000 lines of code  with 100 person years spent on safety assurance \cite{RailwayDBLP:conf/icse/GuihoH90}, and Space Shuttle code whose production and assurance according to NASA cost \$1,000 per line). %, and it is known that this contains many faults. For some systems, the levels of confidence needed seem so high as to be beyond what can be claimed from the deployment of feasible amounts of evidence in conventional arguments.
An essential part of this cost is due to what is considered to be an inherent non-automatability of assurance....

\endinput 
@inproceedings{DBLP:journals/corr/abs-2101-10484,
	author    = {Georgios Bakirtzis and
		Christina Vasilakopoulou and
		Cody Harrison Fleming},
	editor    = {David I. Spivak and
		Jamie Vicary},
	title     = {Compositional Cyber-Physical Systems Modeling},
	booktitle = {Proceedings of the 3rd Annual International Applied Category Theory
		Conference 2020, {ACT} 2020, Cambridge, USA, 6-10th July 2020},
	series    = {{EPTCS}},
	volume    = {333},
	pages     = {125--138},
	year      = {2020},
	url       = {https://doi.org/10.4204/EPTCS.333.9},
	doi       = {10.4204/EPTCS.333.9},
	timestamp = {Fri, 09 Apr 2021 18:27:18 +0200},
	biburl    = {https://dblp.org/rec/journals/corr/abs-2101-10484.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}
The exceptionality issue and the costs provide a practical justification for the quest of this paper for a transparent and well-structured formal \fwk\ for assurance %(in a much stronger sense of being structured than currently assumed in the assurance literature) 
\zdneww{based on established patterns of object-oriented modelling (OOM) and category theory. Indeed, first, a transparent structure and patterns could significantly reduce the complexity of building assurance cases and thus address the exceptionality issue and, second, a formalized \fwk\ makes assurance amenable to automation; both factors would significantly reduce the cost if properly realized.}{revise!!!}{-2em}    

\zd{What about adding a phrase about low value of automation in Holloway's course}

\zd{also, it's agood place to talk about Explicitness as a major proeprty of the argument but Alas, Rushby's def does not mentions it. }

==> sections/intros/intro4tr.tex <==
\section{Introduction}


A diagrammatic operation takes a diagram of a specified shape as its input, and extends it with new elements forming a bigger diagram of a specified shape; we will say that the input diagram is {\em completed} by the operation. 
For example,  arrow composition takes two consecutive arrows and completes them with a third arrow forming the \corring\ triangle.  %This list of examples can be extended indefinitely: 
The resulting diagram often satisfies some postconditions, \eg, a chosen pullback completes a cospan with a {\em commutative} square, and a chosen powerobject completes an object with its {\em jointly-monic} membership span. Preconditions are needed too, \eg, adhesive 
%HLR categories \cite{EhrigHabelPP2004} 
categories only provide pushouts for one-leg-monic spans (and then we know that the \corring\ leg of the resulting cospan is also monic). Thus, categorical diagram operations come together with reasoning over them so that diagram algebra and logic are smoothly integrated in diagram chasing routines. 

This paper stems from the observation that the diagram chasing idea transcends Category Theory (CT) and finds numerous applications in the practice of Software Engineering (SE), in which, however,  it is currently used in an ad-hoc way: implicit, semi-formal or formal but buried in code so that the underlying diagram chasing procedures are blurred and distorted.  
The negative impact of these issues increases with the recent advent of Model Driven Engineering (MDE), in which \diatic\ models rather than code become the primary artifacts of software development. 

\shortlong{
Our goal in the project reported in the present  paper%
\footnote{which is an extended abstract of ongoing work in progress, whose current state is reported in the technical report \citeTR (further referred to as ``the TR'')}
 is to provide an accurate formalization of diagrammatic reasoning routines adequate to their practical use in MDE. We will discuss this in more detail in the next section along with several mathematically interesting structures and results emerged along the course, and our contributions.  Sections 3 and 4 provide basic formal definitions and results, and Sect.5 concludes.  Appendix A is optional but helpful: it illustrates main motivating ideas with a simple example.
}{ %endShort/BeginLOng
Our goal in the project reported in the present technical report (further TR) 
%\footnote{which is an extended abstract of ongoing work in progress, whose current state is reported in the technical report \citeTR (further referred to as ``the TR'')}
is to provide an accurate formalization of diagrammatic reasoning routines adequate to their practical use in MDE. We will briefly discuss this in the next section (Sect. 2.1-2) along with several mathematically interesting structures and results emerged along the course (in Sect. 2.3); a brief survey of related work and our contributions are in %, and a road map of the TR (Sect.2.4)
Sect. 2.4. We also describe a simple example of domain modelling motivating generalized sketches as the main underlying machinery in Sect. 2.5, and overview our notation in Sect. 2.6. Section 3 gives three brief introductions to our three main subjects: \diatic\ logic, \diatic\ algebra, and \diatic\ reasoning. Sections 4-6 present technical development: in Sect.4 we consider sketches over predicate signatures (with or without dependencies between predicates), and in Sections 5-6 complex queries built from \diatic\ operations (the case of operation without dependencies is in Sect. 5 and the general case with dependencies in Sect. 6; the latter is is in progress and currently only provides basic definitions). %Since Section 5, we assume categories of sketches to be skeletal
Section 7 concludes.  % Sections 3 and 4 provide basic formal definitions and results, and Sect.5 concludes.  Appendix A is optional but helpful: it illustrates main motivating ideas with a simple example.
}

\endinput


\section{Overview} %Motivation: Why we need a view mechanism over generalized sketches}
  \renewcommand{\QQ}{\enma{\mathbf{Q}}}
  
 We discuss two main applications of the \fwk\ in SE in Sect.2.1-2, then discuss some mathematical aspects of the \fwk\ in Sect.2.3, and describe related work and contributions in Sect.2.4
  
%\subsection{Two Practical Applications}
%There are two practical issues that we aim to address with our \fwk. %: A) clean and formal notion of a view, and B) clean and formal algebra for model management, which we now discuss. 
\subsection{Views over sketches.} 
\label{sec:application1} 
Developing a complex software system normally requires working with multiple \emph{views} \cite{AtkinsonStollB2010} of the system: 
This is the only way to manage complexity and a cornerstone of system engineering, see \cite{FinkelsteinKramerNFG1992} for an early discussion and \cite{FeldmannKernschmidtWV2019,BruneliereBurgerCW2019,CicchettiCicozziP2019} for more recent reports and surveys. 
A view of a {\em source} artifact $S$ is, in general, not merely a part of $S$ or a projection of $S$, but typically involves some computation over $S$,  e.g. composing references, aggregating attributes by summing up their values etc, which extends $S$ with {\em derived} elements produced by some predefined operations (we will say {\em queries}) applied to $S$. Then a {\em view} can be defined as  a mapping $\frar{v}{V}{Q_v(S)}$ in a suitable category of software artifacts where the source $S$ and the view schema $V$ live, and  $Q_v$ is a query that provides an extension $Q_v(S)$ of source $S$ with derived elements required by the view. Note an important distinction from the ordinary Kleisli mappings defined for a given monad $\QQ$ or, at least, a global object mapping, which only potentially exists and seems unnecessary abstract for software engineers not familiar with Haskell. In contrast, in our notion of view, each view mapping $v$ carries its own query 
 $Q_v$ and maps to its own {\em local} extension $Q_v(S)$ rather than to a unified but huge global extension $\QQ(S)$.  
 \begin{includeShort}
 A simple example in Appendix \ref{sec:viewExample} shows how it works, and also demonstrates the importance of constraints for the view mechanisms. Thus, the basic category hosting models like $S$ and $V$ is a category of generalized sketches over graphical structures rather than pure graphs. 
\end{includeShort} 
%\begin{includeLong}
%	\input{sections/appendix4act20}
%\end{includeLong}

\subsection{Algebra for model management.}\label{sec:application2}
 In \emph{model management},  models are manipulated as holistic entities, and replacement the one-object-at-a-time approach (micromanagement) by one-model-at-a-time (macromanagement)  turned out very productive \cite{Bernstein2003,%}.
% The respective research domain is called \emph{model management} \cite{
FavreNguyen2005,%Diskin2009,
PaigeKolovosRMW2013%DiskinKokalyM2013
}. It requires considering high-level operations on models such as model slicing, transformation, merging, and synchronization, and composing them into complex workflows  \cite{Diskin-sle13}. 
 \begin{wrapfigure}{r}{4cm}
 	\vspace{-2ex}
 	\centering
 	\includegraphics[width=\linewidth]{figures/modelMgmtsmall}
 	\caption{Model Management}
 	\label{fig:modelMgmt}
 	 \end{wrapfigure}
  %?????   model operations are inherently diagrammatic \cite{me-sle13,me-fase16}. 
  Fig.~\ref{fig:modelMgmt} shows a simple example in which two views of the same source are first matched, and then merged. One may think of this as taking the pullback and then the pushout, but in practice these ``pure'' categorical operations are often interwoven with some normalization procedures (and may require conflict resolution) so that even in this simple case the real workflow will be much richer. 
 %
 Importantly, models in SE are typically considered up to their auto-isomorphisms generated by permutations of OIDs (in the sense of OO programming)  which are irrelevant and normally not visible. It justifies making categories of models skeletal and having only identical auto\mor s, which makes limits and colimits  deterministic algebraic operations.  

Thus, for both the inter-model and the intra-model levelsof reasoning, SE needs powerful and formally specified algebraic machinery for diagrammatic operations. On the other hand, it seems that even basic universal algebraic constructs (signature, term, parsing) have not been accurately specified for diagrammatic operations, especially when the latter are considered together with pre-and post-conditions and hence are interwoven with logic; in this sense, we are developing some basic universal algebra for diagrammatic operations. 

\subsection{Mathematical aspects}
\subsubsection{Why generalized graphs and generalized sketches} %, and categorical signatures}

As discussed above, categories hosting software models are categories of sketches. % and their models (in the mathematical sense). 
In general, a sketch is a graphical structure endowed with labelled diagrams (a.k.a. constraints); in the project, we consider a very general version of the notion: our 'graphs' are finitary presheaves, and our constraints of shape $G$ are any ``devices'' that classify mappings from $G$ as either valid or invalid. The generality of our graphs is caused by the great diversity and complexity of graphical structures used in SE  \cite{Kent2002}, and graphs used for behavioural and workflow  models can even be more complex. %Hence, we consider a very general notion of a graph as being a presheaf \frar{G}{\HH}{\setcat}  whose schema $\HH$ is any finite category. \footnote{In the long version, we consider an important requirement to \HH\ motivated by other parts of the project, but it is not needed for results described in the present paper.}
Similarly, constraints used in domain modelling (banking, e-commerce, automotive etc.) can be complex and very elementwise-oriented so that their representation in a standard categorical way via universal properties can be rather bulky and unwieldy (a detailed discussion can be found in \cite{DiskinWolter2008}, see also Appendix). Thus, we need  constraints and sketches of a very general nature that Michael Makkai called {\em generalized sketches} \cite{Makkai1997}.  %Diagrammatic constraints are an integral part of the domain and software modelling, and  important for specifying correct view mappings. Hence, we need to consider graphs endowed with constraints declared over them, \ie, graphical/diagrammatic theories or {\em ()generalized) sketches}. Thus, our category of artifacts and their mappings should be a category of sketches and sketch \mor s.
%
%The classic Ehresmann sketches consider signatures that only contain classes of limit and colimit predicates whose semantics are given by the respective universal properties. Generalized sketches moreover consider arbitrary predicates, where semantics are defined externally. This allows for more compact specifications because one does not need to add auxiliary structures as it is often required with classical sketches, cf. \cite{JohnsonRosebrugh2002}.


\subsubsection{String diagrams do not work for diagram operations}
\newcommand{\propcat}{\enma{\catname{PROP}}}
%The objects in a PROP are natural numbers (arities) and arrows represent operations where domain and codomain denote in- and output arity. Being symmetric monoidal (sm) categories, $\catname{PROPs}$ can be  visualized with String Diagrams \cite{Selinger2011}, an intuitive yet formal graphical syntax.
For \propcat s, terms can be specified by string diagrams as shown in 
Fig.~\ref{fig:exSMC}, which depicts a ternary term $(x + y) * (x + z)$ built from two binary operations. % in string diagram notation, which is a ternary operation ($\in \catname{PROP}(3,1)$) where 
Note that reuse of the middle variable $y$  is shown explicitly with  $\nfont{Copy}$-operation (visualized via \includegraphics[width=1em]{figures/Copy}). This is possible as 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/StringDiagram}
	\caption{String diagram notation for ordinary algebraic terms}
	\label{fig:exSMC}
\end{figure}
%Unfortunately, we cannot use this machinery for diagram operations. The classical operations are \setcat-based and 
set $\{x, y, z\}$ is the coproduct of its elements $\{x\}\sqcup\{y\}\sqcup \{z\}$.
However,  diagram operations are graph-based,  %\footnote{Throughout this paper we will use the term ``graph'' in a more general sense, see Sect.~\PAST{Reminder to put the correct reference}}.
and a graph (while being a colimit of its elements) is not their coproduct!
\input{figures/insert-ex3pb}
Consider Fig.~\ref{fig:ex3pb} presenting a simple diagram chasing piece. % \} as used in many categorical proofs denoted in different visual syntaxes. 
Part (A) uses a typical categorical notation: the diagram presents a workflow consisting of two pullbacks taken in parallel over spans with one monic leg, followed by yet another pullback. Monic preservation by pullbacks is also shown. %In addition,  by naming conventions and respective symbols in the corners we show that some elements in the diagram are constructed via pullbacks, and via arrow decorations we specify some of the arrows to have special properties (being monic).
Part (B) makes the above explicit by using labels for constraint declarations (ovals) and operation applications (chevrons), and showing their scope. % make the stion elements in the diagram are explicated. 
Note that arrows going in and out of chevrons  show the workflow and what elements are constructed/derived (blue and dashed) rather than given. 
Part (C) is similar to Fig.~\ref{fig:exSMC} and highlights the workflow of the query by making the order of operation applications explicit, e.g. the pullback \nfont{c} depends on elements produced by the other two pullbacks.

Note several important differences with Fig.~\ref{fig:exSMC}. First, in discrete $\catname{PROP}$-setting, the elements produced by an operation have no further relationship with the input elements, while in the graph-based setting, there is an overlap between the input and the output, e.g. element $B$ in \figref{ex3pb}(B) is both in the input and the output of the pullback application \nfont{a}, and similarly for application \nfont{b} so that $B$ is also shared by \nfont{a}-output and \nfont{b}-output. Second, the workflow shown in \figref{ex3pb}(C) is a rather poor view of the actual workflow under the hood, which consists of several pushouts (POs): three POs are needed to produce graph $X'$ and yet another one to produce $X''$. Workflow arrows with hollow ends are, in fact, pairs, $(X,a)$, $(X,b)$ etc.,  while mappings that do the job, \eg, the one showing what part of graph $X$ is used as an input for \nfont{a{:}[pb]}, are not shown. %etc., and monics from $X$ to $X'$ to $X''$, are not shown. 
Thus, in contrast to \figref{exSMC}, diagram \figref{ex3pb}(C) is an incomplete specification of the story.  

\subsection{Related Work and Contributions}
%\zd{Phrase about the diversity of the pool of notions....}
By {\em logic} we refer to work on generalized sketches, and {\em algebra} refers to work on signatures of operation symbols, terms and algebras over them. 

\vspace{-0.25cm}
\subsubsection{Logic.}
Several authors noticed that Ehresmann's sketches can be applied to data modelling \cite{LellahiSpyratos1991,Piessens-tac95,JohnsonRosebrugh2002}. %,Diskin-adbis97}, 
%A majority of these application basically rely on the concept of a \emph{sketch}  introduced by Ehresmann, i.e. a graphical counterpart of a logical theory  (see \cite{Wells} for the history and  \cite{AdamekRosicky1994} for references about their equivalent expressiveness). %and classical Ehresmann's skecthes were employed in all works cited above besides those by D \cite{LellahiSpyratos1991,Piessens-,JohnsonRD-audb01}. 
%By sketch we refer the classical notion introduced by Ehresmann and promoted in \cite{BarrWells1990} and a more \emph{generalized} variant introduced by Makkai \cite{Makkai1997}).
However, these sketches are based on universal properties of the \corring\ (limit, colimit, powerobject) diagrams, which (as we discussed above) is a too restrictive setting for applications. %(see \cite{DiskinWolter2008} for a discussion). 
A suitable generalization of sketches by exactly this reason was independently introduced by Diskin \cite{Diskin-sketches96,Diskin1997}, and even earlier, in a very  different context of an abstract approach to logic, by Makkai \cite{Makkai1997} (whose preprints had been circulating in early 90s). Makkai developed a coherent theory of generalized sketches and proved a fundamental result that any category of sketches is a presheaf topos. Hence, sketches in a signature $\PP_1$ can be considered graphs over which a new signature $\PP_2$ and hence a new category of $\PP_2$-sketches can be defined, and so on. In this way, Makkai specified categories with several layers of additional structure as sketches. In our project, we use a different approach in which all discrete signatures $\PP_i$ are integrated into one signature-category $\int_i\PP_i$, whose arrows describe  dependencies between predicate symbols extracted from arities (details can be found in \cite[Sect.3]{THETR}). In the TR we prove that Makkai's theorem can be extended for categorical signatures so that the slogan ``sketches are graph'' persists (see Th.~\ref{thm:genMakkai} below for a precise formulation). 
%: given a presheaf topos of graphs $\GG=\setcat^\HH$ for some schema category \HH, and a set of predicate symbols \PP\ whose arities are \HH-graphs, \PP-sketches whose carriers are \HH-graphs can be considered presheaves on a special (collage) category 
Also, while traditionally sketches are defined in an {\em indexed} way as  families of sets of diagrams indexed by predicate symbols  (for the discrete signature case), or functors {\em from} the signature (for the categorical signature case \cite{DiskinWolter2008}), we define them in an equivalent {\em fibrational} way via a discrete opfibration functor {\em into} the signature: the fibrational definition is more compact and often simplifies technicalities.  

\begin{includeLong}
We need to distinguish between several notions of signatures and sketches. We call logic {\em basic} if signatures of predicate symbols are sets considered as discrete categories. We call it {\em advanced}, if signatures are categories whose arrows are dependencies between predicates; in addition, these arrows are required to go in one direction, which makes signature \cats\ {\em \hical} (a version of Lawvere's one-way categories). Traditionally, sketches are defined in an indexed way as families of sets of diagrams indexed by symbols in the discrete signature case, and functors into \setcat\ for categorical signatures. We define them in an equivalent {\em fibrational} way via a discrete opfibration functor into the signature. There is also an important distinction between {\em -multi-}sketches that allow the same labelled diagram appear in a sketch for multiple times, and {\em mono-}sketches that disallow this. Finally, a partially de-categorificated approach (due to Makkai) is to consider signatures as layered sets so that each predicate in layer $(n+1)$ implicitly depends on all predicates in layer $n$. However, when arities of $(n+1)$-predicates are defined based on $n$-predicates, the actual dependencies appear on the stage. We call this approach {\em discrete \hical (dh)} and show that it is actually equivalent to the categorical one. In these terms, Table \ref{tab:contributionsLogic} shows the previous work and contributions of our project. Our main result is an extension of a fundamental Makkai's theorem (that multi-sketches are actually presheaves) for the case of categorical signatures with dependencies: see Th.~\ref{thm:genMakkai} in the paper. 
%Naively speaking the contribution of our work can be described as formalization of diagram chasing as e.g. in Fig.~\ref{fig:ex3pb}:
%We formally define diagram operations, diagram algebras and queries (= terms) and show elementary results known from classical algebra to hold in this setting:
%Queries extend to a functor $Q$, algebras are arrows $\frar{a}{Q(A)}{A}$ and there is (symmetric monoidal) Kleisli-Category w.r.t. $Q$, hence the latter also becomes a monad.
%The results are first presented in a discrete setting, i.e. without relations between operations, and then extended to a more general setting with relations between operations, which are needed for syntactical reasoning.
\begin{table}[]
	\scriptsize
	\begin{tabular}{|l|l||l|l|l|}
		\hline
		\multicolumn{2}{|l|}{\multirow{2}{*}{\diagbox{Sketch Notion}{Setting}}} & \multirow{2}{*}{One-Layer (Basic Logic)} & \multicolumn{2}{l|}{Multi-Layer (Advanced Logic)}                          \\ \cline{4-5} 
		\multicolumn{2}{|l|}{}                  &                                          & Discrete Hierarchical         & Categorical                                \\ \hline \hline
		\multirow{2}{*}{Indexed}       & mono   & \multicolumn{2}{c|}{\multirow{2}{*}{\cite{Makkai1997}}}                             & \cite{DiskinWolter2008}                                     \\ \cline{2-2} \cline{5-5} 
		& multi  & \multicolumn{2}{c|}{}                                                    & TR: Sect.3.2                               \\ \hline
		\multirow{2}{*}{Fibrational}   & mono   & \multirow{2}{*}{TR: Sect.2.2.-2.3}       & \multirow{2}{*}{TR: Sect.3.4} & \multirow{2}{*}{Paper: Sect.3; TR: Sect.3} \\ \cline{2-2}
		& multi  &                                          &                               &                                            \\ \hline
	\end{tabular}
	\caption{Contributions: Diagram Logic}
\label{tab:contributionsLogic}
\end{table}
\end{includeLong}

\subsubsection{Algebra.}
Diagram operation signatures and algebras were defined first in \cite{Diskin1997} and with some additional details in  \cite{Diskin-sketches96}, but no mathematical results were obtained. For the special case of operations over ordinary graphs, Wolter \etal\ \cite{WolterDiskinK2018} proved that any signature of such operations generates a monad (\ie, a global construct) over the category of graphs. The machinery of {\em local} Kleisli mappings explained informally was used in several papers of the first author, \eg,  \cite{Diskin-models10,Diskin-fase17}, and formalized as Kleisli mappings of a monad (\ie, globally) in \cite{Diskin-fase12}; we are not aware of an accurate formalization of Kleisli mappings considered locally as is done in our project,  nor of several other results reported in Sect.4. Specifically, we prove that a) sketches and local Kleisli mappings (views) between them form a symmetric monoidal category,  and b) the local Kleisli composition gives rise to a Kleisli triple and hence a  monad (as expected).  
\begin{includeLong}
\begin{table}[h]
	\scriptsize
	\begin{tabular}{|l||p{4cm}|p{3.75cm}|}
		\hline
		\diagbox{Topic}{Setting} & Discrete                                                                                & \parbox{3cm}{Categorical \\ (Dependencies)} \\ \hline\hline
		Signatures  and Algebras         & 
		\parbox{3.75cm}{Paper: Sect.4; TR: Sect.5.1; \cite{WolterDiskinK2018}  (graph operations) }                   & TR: Sect.6.1.1 (Defs. only)                     \\ \hline
		Multiqueries and Substitution   & Paper: Sect.4 (Defs. only); TR: Sect.5.2                                                                                & TR: Sect.6.1.2 (Defs. only)                     \\ \hline
		Complex Queries and Composition & Paper: Sect.4; TR: Sect.5.3                                                                               & TR: Sect.6.1.3 (Defs. only)                     \\ \hline
		Monads                          & \parbox{4cm}{Paper: Sect.4; TR: Sect.5.4; \cite{WolterDiskinK2018}  (graph term algebra adjunction)} & TR: Sect.6.1.4 (Conjecture)                    \\ \hline
	\end{tabular}
	\caption{Contributions: Diagram Algebra}
	\label{tab:contributionsAlgebra}
\end{table}
\end{includeLong}
\subsection{Notation.}

\endinput
\zd{more refs would be useful} and then queries become complex diagram operations over graphical structures. \zd{In practice, queries and operations are formally defined on the level of code but rather dirty (informal, approximate) on the level of models -- hence, our interest to make it clean... } %Conceptual graphical artifacts play an important role in SE and are used to specify different aspects of the system under development \cite{Kent2002}.
%
%The above notion can be further abstracted into a Kleisli-arrow $\relationarrow{V}{v}{S}$, which was discovered and presented to the SE-community in \cite{me-fase12}.
\zd{Note also that we cannot use monads as ...... }

==> sections/mathBackgr--cats-of-diags.tex <==
\renewcommand{\arrcatC}{\enma{\CC^\twocat}}
%\renewcommand{\arrowCat}[1]{\enma{#1}^\twocat}
\renewcommand{\fancydom}[1]{\enma{\dom( #1)}}
\renewcommand{\fancycod}[1]{\enma{\cod( #1)}}
\section{%Appendix. 
Several facts about arrow \caties
}\label{sec:arrowCats}
%We will recall a few basic definitions and results and provide several new auxiliary constructs needed in the paper. 

%\begin{ddefN}{diagcats}{Diagram categories} 
%A {\em diagram} in a category \CC\ is a functor \frar{\dvar}{\callid}{\CC} whose domain is a category freely generated by a graph $D$ called the {\em shape} of the diagram (and \callid\ is also called the {\em shape}). Sometimes we will make $D$ a sketch by adding to it \corring\ declarations, \eg, a valid diagram of shape $\imgmsquarepo$ must map two horizontal arrows into monics, and the entire square into a pushout square in \CC. A precise formalization of this construct in general is exactly the subject of the paper, but in the metatheory  we will only use simple sketches like above that can well be explained like above. 
%
% A {\em diagram \mor} is a natural \trafon\ between functors, \drar{\dmorvar}{\dvar}{\dvar'}, \ie, a family of arrows \frar{\dmorvar_x}{x^\dvar}{x^{\dvar'}} indexed by $x\in\Ob{\callid}$ such that $a^\dvar\comp\dmorvar_y =\dmorvar_x\comp a^{\dvar'}$ for any arrow \frar{a}{x}{y} in \callid. This gives us the category $\left[\callid, \CC \right]$ of all diagrams in \CC\ of shape \callid. 

\beign{mygroup}
Let \twocat\ be a fixed \caty\  having two objects 0 and 1, and the only non-identity arrow \frar{01}{0}{1} (it is often called the {\em interval} category) and denoted $I$). 
%\zd{This piece should accurately be written and explain all our notation. }
\begin{constrN}[Arrow Categories]
\label{def:arrcats}
 Any category \CC\ gives rise to an {\em arrow \caty} \arrcatC\ whose objects are \CC-arrows and \mor s are commutative squares:
 given two \CC-arrows $a,b$, their morphism is a pair of \CC-arrows, \frar{f}{\fancydom{a}}{\fancydom{b}} and \frar{f'}{\fancycod{a}}{\fancycod{b}}, such that the square commutes: $a.f' = f.b$. 
 %$a\comp f'=f\comp b$. 
 We call such a pair an {\em sq-arrow} and write \drar{(f,f')}{a}{b}.
 %
Given an object $X\in\CC$, slice and coslice \caties,  $\CC/X$ and $\CC{\setminus}X$ are sub\caties\ of $\CC^\twocat$.  
% Any object $X\in \CC$ gives rise to a {\em dom-pointed} arrow category  
% $\dompointedarrowCat{\CC}{X}\subset\arrowCat{\CC}$ whose objects are arrows from $X$ and the \corring\ component of all sq-arrows is $\id_X$. Similarly, we have {\em cod-pointed} arrow \caty\ $\codpointedarrowCat{X}{\CC}\subset\arrowCat{\CC}$. These \cats\ usually denoted by $\cosliceCat{\CC}{X}$ and $\CC/X$ resp. \zd{this is too heavy and bulky. $\CC/X$ and $\CC\X$ are knowsn and there is no need to introduce {\em dom/cod-pointed} terms.}
\end{constrN}
The following facts can be proven easily for any category \CC:
\begin{lemma}
	\label{lemma:arrcatfibr}
 There are two obvious functors \frar{\domC}{\arrcatC}{\CC} and \frar{\codC}{\arrcatC}{\CC}, for which:
  \begin{enumerate}[label=\roman*)]
 \item Functor \domC\ is a {\em split} fibration (lifts are provided by  precomposition).
 \item The  restriction \frar{\dom_X}{\CC/X}{\CC} (for a given object $X$) is a {\em discrete} fibration.
\item Functor \codC\ is a {\em split} opfibration (lifts are provided by postcomposition)
\item The restriction \frar{\cod_X}{\cosliceCat{\CC}{X}}{\CC} is a {\em discrete} opfibration, 
 \end{enumerate}
 %Thus, if \CC\ has both pushouts and pullbacks, then both \domC\ and \codC\ are bifibrations.
\end{lemma}
%If \CC\ has all pushouts (pullbacks) we can state more. 
\begin{lemma}
	\label{lemma:arrcatfibrPBPO} If, in addition, \CC\ has
\begin{enumerate}[label=\roman*)]
\item all pushouts, then functor \domC\ is also an opfibration, where lifts are constructed via pushouts.
\item all pullbacks, then functor  \codC\ is also a fibration, where lifts are constructed via pullbacks. 
\end{enumerate}
\end{lemma}
%A bit more formally, $m$ is a diagram in \SS\ of shape \fbox{\frar{\IE}{\I}{\E}} whose image is a monic, and we write $I_m$  and $E_m$ for sketches $m(\I)$ and $m(\E)$ resp., and $m$ for the monic $m(\IE)$.
\end{mygroup}
\subsection{Slice \caties}\label{sec:sliceCats}
The following results are basic for slice \caties. 
%Let \CC\ be any \caty\ with pullbacks and \frar{f}{S'}{S} is an \CC-arrow.
\begin{lemma}[Substitution functors, P. Freyd \cite{Freyd-aspects}]\label{lemma:dirSubst-inAppendix}
	Let \CC\ be a \caty\ with pullbacks and \frar{f}{S'}{S} is a \CC-arrow. There is an adjunction between slice \caties:
	$f_*{:}\, \CC/S' \rightleftarrows\CC/S\,{:}f^* $,
	%\begin{tikzcd}[row sep=2ex, column sep=4ex]
	%\CC/S' \ar[r, "\CC/f", bend left=25] %\ar[r, phantom, "\footnotesize \perp"]
	%& \CC/S \ar[l, "f^*" , bend left=25]
	%\end{tikzcd}
	where functor $f_*:=\CC/f$ is defined by postcomposition with $f$, and functor $f^*$ is defined by pulling back over $f$. 
	\qed
\end{lemma}
%
		%\input{sections/piece--twistedLemmaOld} % with wrapped ddiagram 
% twisted lemma without wrapping 
\begin{lemma}[Twisted substitution]\label{lemma:twistedSubstProof}
	Let \CC\ be a \caty\ with pullbacks and \frar{f}{\X}{\X'} is a \CC-arrow. %For any \caty\ \CC\ with pullbacks and any \CC-arrow \frar{f}{X'}{X},
	Then diagram  a) below commutes,  %on the right %\cref{eqdiag:twistedSubst}d) above,  
	where \caties\ $P$, \twistedX{P}, and $P'$ are products (whose projections are referred to as  `horizontal' (h) and 'vertical' (v) ), arrows $f_*$ and $f^*$ are as defined above,
	\arrowcatX{\CC} is the arrow \caty\ of \CC, and functors \pbfunvX{\cdot} will be defined (see diagram b) explained below).  % \ref{constr:twistedPBfunctor}, 
%---
	\input{diagrams/twistedLemma--Proof}
		%----
\end{lemma}
%\begin{remark} {\em Remark.}
%Note that product \caties\ $P$ and $P'$ are similar: %in terms of Constr. \ref{constr:twistedPBfunctor}, 
%one of their components is a ``vertical'' and the other is a ``horizontal'' copy of the same slice \caty. Product \twistedX{P} is twisted and takes its vertical and horizontal elements from different slice \caties\ % (but again one of them is vertical and the other is horizontal). 
%so that there is no a direct vertical arrow from \twistedX{P} to $\CC^\twocat$. However,  each of the substituting functors $f_*$ and $f^*$ allows for an indirect path from \twistedX{P} to $\CC^\twocat$.   The lemma states that these two paths are equal (actually up to iso\mor\ as pullbacks are defined up to iso). % is the statement of commutativity of the central  arrow rectangle  (visualized as a triangle): $!.\pbfunV = !'.\pbfunV'$. 
%\end{remark}

{\em Proof (in which the \pblemma\ is heavily employed by default).} We begin with defining functor  \frar{\pbfunvX{}}{\CC/\X\timm\CC/\X}{\arrowcatCC}
for any object $\X$ in \CC, where 
	%\arrowcatCCcong\ denotes the arrows \caty\ over \CC, in which arrows $v,v'\in \CC/X$ for some $X$ are identified (we  write $v\cong_X v'$) if their domains are iso\moric.  
\arrowcatCCcong\ is the \caty\ of \CC-arrows with commutative squares as \mor s.
Then for a given $\X$, pullback gives rise to a single-valued up to iso operation \pbfunvX{} on objects and arrows as shown in diagram b) above (where all squares are PB): pair 
$(\bar{\bar g}.\bar{u},\, g )$ is a representative of \arrowcatCC-\mor\ \frar{\pbfunvX{}(u,g)}{\pbfunvX{}(v',h')}{\pbfunvX{}(v,h)}. Composition and identity are strictly preserved after quotienting wrt. the corresponding $\cong_X$.  

Now consider diagram a). Note that product \caties\ $P$ and $P'$ are similar: %in terms of Constr. \ref{constr:twistedPBfunctor}, 
one of their components is a ``vertical'' and the other is a ``horizontal'' copy of the same slice \caty. Product \twistedX{P} is twisted and takes its vertical and horizontal elements from different slice \caties\ % (but again one of them is vertical and the other is horizontal). 
so that there is no a direct vertical arrow from \twistedX{P} to \arrowcatCCcong. However,  each of the substituting functors $f_*$ and $f^*$ allows for an indirect path from \twistedX{P} to \arrowcatCCcong. The equality of these two paths is guaranteed by yet another application of the \pblemma.   
%%\begin{corol} %went to appendix
%%	Currying provides that any ``vertical'' arrow $v\in \Ob \CC/X$ gives rise to a functor \frar{\pbfunV(v,\_)}{\CC/X}{\CC^\twocat} further denoted by \twSubstX{v}.  Now for any \frar{f}{X'}{X}, we have $(\CC/f).\twSubstX{v} = \twSubstX{f^*(v)}$. 
%%\end{corol}
%\begin{corol}
%	Currying provides that any ``vertical'' arrow $v\in \Ob \CC/X$ gives rise to a functor \frar{\pbfunV(v,\_)}{\CC/X}{\CC^\twocat} further denoted by \twSubstX{v}.  Now for any \frar{f}{X'}{X}, we have $f_*.\twSubstX{v} = \twSubstX{f^*(v)}$. 
%\end{corol}
%
%\input{diagrams/twistedSubst}



==> sections/mathBackgr--diagCats-forTR.tex <==
\renewcommand{\arrcatC}{\enma{\CC^\twocat}}
%\renewcommand{\arrowCat}[1]{\enma{#1}^\twocat}
\renewcommand{\fancydom}[1]{\enma{\dom( #1)}}
\renewcommand{\fancycod}[1]{\enma{\cod( #1)}}

\section{%Appendix. 
	Diagram Categories}\label{sec:arrowCats}

We will recall a few basic definitions and results and provide several new auxiliary constructs needed in the paper. 

%\begin{ddefN}{diagcats}{Diagram categories} 

A {\em diagram} in a category \CC\ is a functor \frar{\dvar}{\callid}{\CC} whose domain is a category freely generated by a graph $D$ called the {\em shape} of the diagram (and \callid\ is also called the {\em shape}). Sometimes we will make $D$ a sketch by adding to it \corring\ declarations, \eg, a valid diagram of shape $\imgmsquarepo$ must map two horizontal arrows into monics, and the entire square into a pushout square in \CC. A precise formalization of this construct in general is exactly the subject of the paper, but in the metatheory  we will only use simple sketches like above that can well be explained like above. 

 A {\em diagram \mor} is a natural \trafon\ between functors, \drar{\dmorvar}{\dvar}{\dvar'}, \ie, a family of arrows \frar{\dmorvar_x}{x^\dvar}{x^{\dvar'}} indexed by $x\in\Ob{\callid}$ such that $a^\dvar\comp\dmorvar_y =\dmorvar_x\comp a^{\dvar'}$ for any arrow \frar{a}{x}{y} in \callid. This gives us the category $\left[\callid, \CC \right]$ of all diagrams in \CC\ of shape \callid. 

\ActTR{Below are several basic facts about {\em arrow \caties}, whose shape is \caty\ \twocat\ having two objects 0 and 1, and the only non-identity arrow \frar{01}{0}{1} (it is often called the {\em interval} category).}
{In the next subsection we will consider categories of diagrams whose \nowlater{.}{, and in \sectref{msquarepo}, we consider categories of diagrams of the square shape above.}
\subsection{Common arrow categories.}
\label{sec:arrowCats}
} % END TR piece 
%\zd{This piece should accurately be written and explain all our notation. }
\begin{constrN}[Arrow Categories]
\label{def:arrcats}
 Any category \CC\ gives rise to an {\em arrow \caty} \arrcatC\ whose objects are \CC-arrows and \mor s are commutative squares:
 given two \CC-arrows $a,b$, their morphism is a pair of \CC-arrows, \frar{f}{\fancydom{a}}{\fancydom{b}} and \frar{f'}{\fancycod{a}}{\fancycod{b}}, such that the square commutes: $a.f' = f.b$. 
 %$a\comp f'=f\comp b$. 
 We call such a pair an {\em sq-arrow} and write \drar{(f,f')}{a}{b}.
 
Note that given an object $X\in\CC$, slice and coslice \caties\  $\CC/X$ and $cosliceCat{\CC}{X}$ are sub\caties\ of $\CC^\twocat$.  
% Any object $X\in \CC$ gives rise to a {\em dom-pointed} arrow category  
% $\dompointedarrowCat{\CC}{X}\subset\arrowCat{\CC}$ whose objects are arrows from $X$ and the \corring\ component of all sq-arrows is $\id_X$. Similarly, we have {\em cod-pointed} arrow \caty\ $\codpointedarrowCat{X}{\CC}\subset\arrowCat{\CC}$. These \cats\ usually denoted by $\cosliceCat{\CC}{X}$ and $\CC/X$ resp. \zd{this is too heavy and bulky. $\CC/X$ and $\CC\X$ are knowsn and there is no need to introduce {\em dom/cod-pointed} terms.}
\end{constrN}

The following facts can be proven easily for any category \CC:
\begin{myfact}
	\label{fact:arrcatfibr}
 There are two obvious functors \frar{\domC}{\arrcatC}{\CC} and \frar{\codC}{\arrcatC}{\CC}, for which the following holds.
 
 \begin{enumerate}[label=\roman*)]
 \item Functor \domC\ is a {\em split} fibration (lifts are provided by  precomposition).
 \item The  restriction \frar{\dom_X}{\CC/X}{\CC} (for a given object $X$) is a {\em discrete} fibration.
\item Functor \codC\ is a {\em split} opfibration (lifts are provided by postcomposition)
\item The restriction \frar{\cod_X}{\cosliceCat{\CC}{X}}{\CC} is a {\em discrete} opfibration, 
 \end{enumerate}
 %Thus, if \CC\ has both pushouts and pullbacks, then both \domC\ and \codC\ are bifibrations.
\end{myfact}

	If \CC\ has all pushouts (pullbacks) we can state more. 
\begin{myfact}
	\label{fact:arrcatfibrPBPO}
\begin{enumerate}[label=\roman*)]
\item If \CC\ has all pushouts, the functor \domC\ is also an opfibration, where lifts are constructed via pushouts.
\item If \CC\ has all pullbacks, the functor  \codC\ is also a fibration, where lifts are constructed via pullbacks. 
\end{enumerate}
\end{myfact}
%A bit more formally, $m$ is a diagram in \SS\ of shape \fbox{\frar{\IE}{\I}{\E}} whose image is a monic, and we write $I_m$  and $E_m$ for sketches $m(\I)$ and $m(\E)$ resp., and $m$ for the monic $m(\IE)$.


\endinput % below is a very special Diagonal cats thing 



%\zd{Content of \defref{diagcats}, \defref{diagsubcats}, the lemma in-between and diagram \eqref{codopfib4diag} may also go here}
\subsection{Diagonal arrow categories}\label{sec:diagArrowCats}

In \sectref{opsig-withDeps} we will heavily use the following construct.
\begin{mydef}[Diagonal arrow \cats]
	\label{def:diagcats}
	%Recall that for any \caty\ \CC,  the arrow \caty\ $\arrowCat{\CC}$ has \CC-arrows as objects and commutative squares of \CC-arrows as morphisms: given two \CC-arrows $a,b$, their morphism is a pair of \CC-arrows, \frar{f}{\fancydom{a}}{\fancydom{b}} and \frar{f'}{\fancycod{a}}{\fancycod{b}}, such that the square commutes: $a\comp f'=f\comp b$. We call such a pair a {\em sq-arrow} and write \drar{(f,f')}{a}{b}. Similarly, \monicarrowCat{\CC} is a full subcategory of \arrowCat{\CC} whose objects are monic arrows (but sq-arrow are pairs of ordinary arrows).
	%
	In an arrow \caty\ \arrcatC,  a sq-arrow \drar{(f,f')}{a}{b} is called {\em diagonal} if there is a ``diagonal'' arrow \frar{d}{\fancycod{a}}{\fancydom{b}} such that $f=a\comp d$, $f'=d\comp b$; then we write $(f,f')=\diagOP{d}$.
\end{mydef}
%\PAST{The $\fancycod{x}$ and $\fancydom{x}$ for domains ans codomains seems a bit unusual to me, should we maybe use something different or better plain \dom\ and \cod\ ? Also why does the diagonal goes from right to left, I would think it would go from left to right?!}
\zdzd{Freyd\&Scedrov use this notation and it's often very useful. In our case am not sure. }

The associativity of composition ensures the following result.
\begin{mylem} \
\label{lem:diagcats}
	Composition of two diagonal arrows is again diagonal: if \drar{(f_1,f_1')=\diagOP{d_1}}{a}{b} and \drar{(f_2,f'_2)=\diagOP{d_2}}{b}{c}, then $(f_1,f'_1)\comp(f_2,f'_2) = \diagOP{(d_1\comp b\comp d_2)}$. 
\end{mylem}
\begin{mydef}[Diagonal subcategories]
	\label{def:diagsubcats}
	Given a category \CC, category \arrowdiagCat{\CC} has the same objects as \arrowCat{\CC}, diagonal sq-arrows as arrows between different objects (\ie, different \CC-arrows), and the only looping sq-arrows \drar{(f,f')}{a}{a} being (non-diagonal) identity sq-arrows $f=\id({\fancydom{a}})$, $f'=\id({\fancycod{a}})$. 
	
	Category \madCat{\CC} is a full subcategory of \adCat{\CC}, whose objects are monic arrows in \CC, and we have the following obvious commutative diagrams:
	\begin{equation}\label{eq:codopfib4diag}
	\begin{array}{c@{\qquad}c}
	\xymatrix{
		\madCat{\CC} \ar@{^{(}->}[rr]^{\wide} \ar@{^{(}->}[dd]_{\full} \ar[rd]|{\dom'}
		&&
		\maCat{\CC} \ar@{^{(}->}[dd]^{\full} \ar[ld]|{\dom''}
		\\
		&\CC &
		\\
		\adCat{\CC} \ar[ru]|{\dom'''} \ar@{^{(}->}[rr]^{\wide}
		&& 
		\arrowCat{\CC} \ar[lu]|{\dom}	
	}
&
	\xymatrix{
	\madCat{\CC} \ar@{^{(}->}[rr]^{\wide} \ar@{^{(}->}[dd]_{\full} \ar[rd]|{\cod'}
	&&
	\maCat{\CC} \ar@{^{(}->}[dd]^{\full} \ar[ld]|{\cod''}
	\\
	&\CC &
	\\
	\adCat{\CC} \ar[ru]|{\cod'''} \ar@{^{(}->}[rr]^{\wide}
	&& 
	\arrowCat{\CC} \ar[lu]|{\cod}	
}
\end{array}
	\end{equation}
	with labels \wide\ and \full\ referring to wide and full embedding resp.  %and the functor \cod\ the standard opfibration given by composition (not to be confused with the Cartesian fibration given by pullbacks). 
	Note that functor $\cod'$ is faithful: if two parallel diagonals are different, %$d_1\noteq d_2$, 
	then their compositions with the target monic arrow are different too.
	To ease notation, below we will denote all four \dom-functors and all four \cod-functors by name \dom\ and \cod, resp., without primes. 
\end{mydef}
\tempendinput

\subsubsection{Categories of square shaped diagrams}
\label{sec:msquarepo}
\begin{mydef}[Binding squares and diagrams] %\label{def:squarecats}
\label{def:bSqcats}
The {\em binding square shape} is a fixed category \bSquare\ specified in diagram \eqref{bindingDiagram} below:
\begin{equation}
\label{eq:bindingDiagram}
\xymatrix{   % diagrams a)
	\inputArity{} \ar[r]^{IE} 
	\ar[d]_{b_I} 
	\ar@{}[dr]|(.8){\Large \ulcorner} 
	&  \scopeArity{} 
	\ar@{->}[d]^{b_E} 
	%	\\ 	&\nfont{[po]}&
	\\
	I_* \ar[r]^{IE_*} & E_*
}
\end{equation}
Diagrams of this shape, \ie, mappings \frar{\dvar}{\bSquare}{\CC}, are required to be pushouts and called {\em binding squares (b-squares)} (note the small corner near node $E_*$ that declares the square as a pushout).
 For any element $X\in\bSquare$, we write $X^\dvar$ for $\dvar(x)$. 
 Morphisms of b-squares, \trirar{\dmorvar^4}{\dvar}{\dvar'}, are quadruple of arrows $%\pmb{\dmorvar}=
\comprfam{\frar{\dmorvar^4_{X}}{X^\dvar}{X^{\dvar'}}}
	{X\in\{I, E, I_*, E_* \}  }$ making a commutative prism. 
\end{mydef}

Fig.~\ref{fig:squarepoCatArrows} shows how these arrows can be visualized (ignore the colors for the moment) either as a three dimensional prism (a) or unfolded as commutative squares (b).

%\newcommand{\liftSourceName}{\delta}
%\newcommand{\liftTargetName}{\delta'}
%\newcommand{\liftName}{\Delta}
%\newcommand{\liftComparisonName}{\Delta'}
%\newcommand{\liftComparisonTargetName}{\delta''}
%\newcommand{\mediator}{(i,e)}
%
%\newcommand{\topBackI}{I^\delta}
%\newcommand{\topBackE}{E^\delta}
%\newcommand{\topBackIE}{IE^\delta}
%\newcommand{\topFrontI}{I^\delta_*}
%\newcommand{\topFrontE}{E^\delta_*}
%\newcommand{\topFrontIE}{IE^\delta_*}
%\newcommand{\topBackToFrontI}{b_I^\delta}
%\newcommand{\topBackToFrontE}{b_E^\delta}
%\newcommand{\bottomBackI}{I^{\delta'}}
%\newcommand{\bottomBackE}{E^{\delta'}}
%\newcommand{\bottomBackIE}{IE^{\delta'}}
%\newcommand{\bottomFrontI}{I^{\delta'}_*}
%\newcommand{\bottomFrontE}{E^{\delta'}_*}
%\newcommand{\bottomFrontIE}{IE^{\delta'}_*}
%\newcommand{\backDownI}{\Delta_I}
%\newcommand{\backDownE}{\Delta_E}
%\newcommand{\frontDownI}{\Delta_I^*}
%\newcommand{\frontDownE}{\Delta_E^*}
%\newcommand{\bottomBackToFrontI}{b_I^{\delta'}}
%\newcommand{\bottomBackToFrontE}{b_E^{\delta'}}	
%\newcommand{\explain}[1]{\mbox{~~ by {#1}}}
%
%\newcommand{\thirdSquareBackI}{I^{\delta''}}
%\newcommand{\thirdSquareBackE}{E^{\delta''}}
%\newcommand{\thirdSquareBackIE}{IE^{\delta''}}
%\newcommand{\thirdSquareFrontI}{I^{\delta''}_*}
%\newcommand{\thirdSquareFrontE}{E^{\delta''}_*}
%\newcommand{\thirdSquareFrontIE}{IE^{\delta''}_*}
%\newcommand{\thirdSquareBackToFrontI}{b_I^{\delta''}}
%\newcommand{\thirdSquareBackToFrontE}{b_E^{\delta''}}	

\begin{figure}
	\begin{tabular}{c@{\qquad}c}
		$
		\xymatrix{
			& \topBackI\ \ar[rr]^{\topBackIE}  \ar[dl]_{\topBackToFrontI} \ar[dd]|{\hole}_(.6){{\backDownI}} & & \topBackE\  \ar[dl]_{\topBackToFrontE} \ar[dd]_(.6){{\backDownE}} \\
			\topFrontI\ \ar[rr]^(.6){\topFrontIE} \ar@[blue][dd]_(.6){\textcolor{blue}{\frontDownI}} & & \topFrontE\ \ar@[blue][dd]_(.6){\textcolor{blue}{\frontDownE}} & \\
			& \bottomBackI\ \ar[rr]|{\hole}^(.6){\bottomBackIE}  \ar@[blue][dl]_{\textcolor{blue}{\bottomBackToFrontI}}  & & \bottomBackE \ar@[blue][dl]_{\textcolor{blue}{\bottomBackToFrontE}} \\
			\textcolor{blue}{\bottomFrontI} \ar@[blue][rr]^{\textcolor{blue}{\bottomFrontIE}} & &\textcolor{blue}{ \bottomFrontE} & \\
		}
		$
		& 
		$
		\xymatrix{
			\topBackI \ar[rrr]^{\topBackIE} \ar[ddd]_{\topBackToFrontI} \ar[dr]^{\backDownI} \ar@{}[dddr]|{(ii)} \ar@{}[drrr]|{(i)} & & & \topBackE \ar[ddd]^{\topBackToFrontE} \ar[dl]_{\backDownE} \ar@{}[dddl]|{(iv)} \\
			& \bottomBackI \ar[r]^{\bottomBackIE} \ar@[blue][d]_{\textcolor{blue}{\bottomBackToFrontI}} \ar@{}[dr]|{(iii)} & \bottomBackE \ar@[blue][d]^{\textcolor{blue}{\bottomBackToFrontE}} & \\
			& \textcolor{blue}{\bottomFrontI} \ar@{}[dr]|{(v)} \ar@[blue][r]^{\textcolor{blue}{\bottomFrontIE}} & \textcolor{blue}{\bottomFrontE} & \\
			\topFrontI \ar[rrr]_{\topFrontIE} \ar@[blue][ur]_{\textcolor{blue}{\frontDownI}} & & & \topFrontE \ar@[blue][ul]^{\textcolor{blue}{\frontDownE}}
		}
		$ 
		\\
		(a) Arrows in $\squarepoCat{\CC}$  (3D - visualization) 
		& 
		(b) Arrows in $\squarepoCat{\CC}$  (flat visualization)
	\end{tabular}
	\caption{Prisms}
	\label{fig:squarepoCatArrows}
\end{figure}	

A {\em pointed} binding square is a diagram with one node fixed. We will use pointed diagrams in which......  \PAST{Something seems to be missing, here?}

Embeddings \frar{\nfont{e}}{\fbox{$\cdot\rightarrow\cdot$}}{\bSquare} 
%and   \frar{IE_*}{\fbox{$\cdot\rightarrow\cdot$}}{\bSquare} 
gives us a projecting functor
\frar{\nfont{e}\comp\_}{\squarepoCat{\CC}}{\arrowCat{\CC}} denoted by \proj{X} where $X\in\{ IE,b_E,b_I,IE_*  \}$ is the image of \nfont{e}. 


There is a corresponding statement for Fact~\ref{lem:arrcatfibr} (i-ii) concerning binding squares. 

 \begin{mylem}
 	\label{lem:bSqFacts}
 %	Functor \frar{\Dom}{\squarepoCat{\CC}}{\arrowCat{\CC}} is a fibration. Moreover, functor 
 %	\frar{\Dom_X} {\squarepoXCat{\CC}{X}} {\arrowCat{\CC}} is a discrete fibration.
Let category \CC\ with pushouts and hence binding diagrams. Then ...
\begin{enumerate}[label=(\roman*)]
\item ...the projection functor $\frar{\proj{IE}}{\squarepoCat{\CC}}{\arrowCat{\CC}}$  is an opfibration
\item ... the pointed projection functor $\frar{\proj{IE}^X}{\squareXCat{X}{\CC}}{\arrowCat{\CC}}$ (for a given predefined \CC-object $X$) is a discrete fibration.
\end{enumerate}
 \end{mylem}
\begin{proof}
(i) The proof is more or less trivial:
For every $\squarepoCat{\CC}$-object $\delta$ as in \eqref{liftSource} and arrow $\frar{(\backDownI,\backDownE)}{\inlinearrow{\bottomBackI}{\bottomBackIE}{\bottomBackE}}{\inlinearrow{\topBackI}{\topBackIE}{\topBackE}}$ in $\arrowCat{\CC}$ we can easily construct a trivial lift (cube) as follows
\begin{equation}
\label{eq:proofPrismLifting}
\xymatrix{
	& \bottomBackI \ar[rr]^{\bottomBackIE}  \ar@{=}[dl]_{id} \ar[dd]|{\hole}_(.6){{\backDownI}} & & \bottomBackE  \ar@{=}[dl]_{id} \ar[dd]_(.6){{\backDownE}} \\
	\bottomBackI \ar[rr]^(.6){\bottomBackIE} \ar[dd]_(.6){\compose{\backDownI}{\topBackToFrontI}} & & \bottomBackE \ar[dd]_(.6){\compose{\backDownE}{\topBackToFrontE}} & \\
	& \topBackI\ \ar[rr]|{\hole}^(.6){\topBackIE}  \ar[dl]_{\topBackToFrontI}  & & \topBackE \ar[dl]_{\topBackToFrontE} \\
	\topFrontI \ar[rr]^{\topFrontIE} &   & \topFrontE \\
}
\end{equation}
where the top square is a pushout and the prism evidently is also a cartesian arrow.\par
(ii) Of course, there might be more lift choices than the one presented in \eqref{proofPrismLifting}, however when fix the left front one corner there is only a single choice left (up to isomorphism).
\end{proof}

\begin{mylem}
	The pair $(\proj{b_E}, \cod)$ of functors, depicted in \eqref{bSqFacts} is a functor between fibrations.
	 \begin{equation}
	\label{eq:bSqFacts}
	\xymatrix{
		\squareXCat{X}{\CC} \ar@{^{(}->}[r]^{I_*=X}
		\ar[d]^{\proj{IE}^X}	
		&\squareXCat{\cdot}{\CC}  % 1st argument is \cdot
		\ar@{->}[d]_{\qquad\proj{IE}} \ar[r]^{\proj{b_E}}
		& \downarrowCat{\CC}\ar[d]^\dom
		\\
		\arrowCat{\CC}\ar@{=}[r]^\id 
		&\arrowCat{\CC}\ar[r]^\cod 
		&\CC
	}
	\end{equation}
\end{mylem}
\begin{proof}
	\PAST{I wonder if there is actually anything that must be shown here: $(\proj{b_E}, \cod)$ is an arrow in $\arrowCat{\catCat}$, and $\proj{IE}$ and $\dom$ are fibrations, so what?! I also did not find the concept of ``fibration-morphism'' anywhere...} \zd{Fibr \mor\ is in Jacobs. Without this notion u cannot prove Groth. equiv.}
\end{proof}


% The following is probaly not needed in this version of the paper. The proof was thus in vain....

%There is also a counterpart of Fact~\ref{fact:arrcatfibrConstr}:
%\begin{mylem}
%The functor is $\proj{IE}$ is an opfibration, which can be constructed by pushouts.
%\end{mylem}

%\input{sections/backgroundFibrationProofs}

%\endinput







==> sections/mathBackgr--presheafToposes.tex <==
\section{Presheaf Toposes}
%\subsection{Presheaf toposes}
%In this paper, presheaf topoi will play an important role. 
In Computer science and Software Engineering context, {\em presheaf} toposes or {\em presheaves} have also been referred to as \emph{``graph-like structures''}, e.g. \cite{Loewe1993}. 

\zdhllok{There is an important difference between sets and presheaves, the latter can usually not be represented as a coproduct (sum) of its elements.}{this is to be said in the intro}{-10}


\begin{mydef}[Presheaf]
\label{def:presheaf}
Let $\callS$ be a small category.
A functor \frar{G}{\callS}{\setcat} is called an {\em \callS-presheaf} or just a {\em presheaf} if \callS\  is clear from the context or is not important, and the category $\setcat^\callS$ of all such presheaves and their natural transformations is called a {\em presheaf topos}. \footnote{Usually presheaves are defined as contravariant functors \frar{G}{\callS^{op}}{\setcat} %$\arrow{\callS^{op}}{P}{\catSet}$ 
	due to their relation and importance for the Yoneda Lemma. For our applications throughout this paper,  it is more convenient to work with the covariant definition.}.

A presheaf  \frar{G}{\callS}{\setcat} is called {\em finite} if all sets $G(v)$, $v\in\Ob{\callS}$ are finite. 

A presheaf topos is called {\em finitary} if the schema category \callS\ is finite. (Makaki says that in ref [3] in his paper 1, such toposes are called finite. 
\end{mydef} 

\begin{myfact}[Presheaf Topos]
\label{fact:presheafTopos}
Any category of presheaves is a \emph{topos} and thus has 
\begin{itemize}
\item all limits and colimits,
%\item has all colimits.
\item exponents, \ie, is cartesian closed,
\item epi-mono factorizations,
\item a subobject classifier.
\end{itemize}
\end{myfact}

If \callS\ is \Graph, then 'graphs' are nothing but ordinary directed multigraph, and if \callS\ is \nfont{rGraph}, then 'graphs' are reflexive graphs. If \callS\ is \PNet, 'graphs' are Petri nets (bipartite graphs of places and transitions).
%\zd{in the source, closing bracket is inserted here}
%} 

Several fixed schema categories we will use are shown in \figref{shapes}. Objects and arrows in these categories are fixed and have fixed names.
% Let $G \in \cat{G}$ an object (graph) in $\cat{G}$.
\begin{figure}[b]
	\begin{tabular}{c@{\qquad}c@{\qquad}c}
		$
		\xymatrix{
			\Node  \\
			\Edge \ar@<+0.5ex>[u]^{\so} \ar@<-0.5ex>[u]_{\ta} 
		}
		$
		&
		$
		\xymatrix{
			\Place & \Trans \\
			\Pre \ar[u]^{\so^i} \ar[ur]_(0.65){\ta^i} & \Post \ar[ul]^(0.65){\ta^o} \ar[u]_{\so^o}
		}
		$
		& 
		$
		\xymatrix @C=0.01cm {
			& & \Node & & \\
			\Edge_{(1,0)} \ar[urr]^(0.7){\so_{(1,0)}} & \Edge_{(0,1)} \ar[ur]^(0.3){\ta_{(0,1)}} & \Edge_{(1,1)} \ar@<+0.5ex>[u]^{\so} \ar@<-0.5ex>[u]_{\ta}  & \Edge_{(2,1)} \ar@<+0.5ex>[ul]_{\so^1_{(2,1)}} \ar@/_/[ul]_{\so^2_{(2,1)}} \ar@/_2pc/[ul]_{\ta_{(2,1)}}   &  \ldots 
		}
		$
		\\
		   a) \Graph 
		& c) \nfont{PNet}
		& d) \nfont{HypGraph}
	\end{tabular}
	\caption{Fixed shape categories}
	\label{fig:shapes}
\end{figure}


 %We assume that for any presheaf \frar{G}{\II}{\catSet} we consider, classes $\abs{\II}$ and $\abs{G}\eqdef\compr{G(i)}{i\in\abs{\II}}$ are disjoint. \zd{here $\abs{\II}$ denotes the class of \II's elements -- should be placed in notation}. We will sometime use the same names for elements in $\abs{\II}$ and $\abs{G}$, which means that with a full notation, those names are to be qualified, say, $x_\II$ and $x_G$, but the subindexes are omitted.  We will also write $x\in G$ for an element $x\in\abs{G}$. %  If we use the same names for elements 

%For the remainder of the paper we will fix a category $\GG := \catSet^\II$ with $\II$ being an arbitrary but \emph{finite category}, whose objects will be called {\em 'graphs'} (often just graphs). If $\II$ is \graph, then 'graphs' are ordinary directed multigraphs, the corresponding presheaf topos is denoted by $\catGraph$. if $\II$ is equal to the following category (identities omitted): \[\xymatrix{ N &  E \ar@<-0.5ex>[l]_{s} \ar@<0.5ex>[l]^{t} }
%\]
%\mkRemark{Set thoeretical notions in Presheaves}{rem:setTheory}{

%\subsection{Set-theoretical constructs in presheaf toposes}
Presheaves in many ways behave as sets and we will make use of some set-theoretic concepts throughout the paper. As we have already said, we can speak of \emph{elements} $x \in G$ meaning that there exists an object $I \in \cat{I}$ such that $x \in G(I)$.
Categorically, such a (global) element is modelled by an arrow $x: \boldsymbol{1} \to G$.

\subsubsection{Inclusions}
%Another concept are \emph{inclusions}, which are given by abstract subobjects.
Let $G$ %$G \in \cat{G}$ 
be an object in $\cat{G}$. Two monics \monorar{x}{X}{G} and \monorar{y}{Y}{G} are {\em equivalent}, $x\simeq_G y$, if  %A class of monomorphisms $M_G\subset\GG_\monoind/G$ % \inlinemonoarrow{X}{x}{G} $ 
%is called \emph{abstract subobject} of $G$ when for any two members $\monoarrow{X}{x}{G}, \monoarrow{Y}{y}{G} \in M_G$, %[\inlinemonoarrow{X}{x}{G}]$ and $ \in [\inlinemonoarrow{X}{x}{G}]$ in $[\inlinemonoarrow{X}{x}{G}]$ 
there exists an isomorphism $\arrow{X}{i}{Y}$ such that the triangle  commutes, $\compose{i}{y} = x$. An $\simeq_G$-equivalence class is called an {\em (abstract) subobject} of $G$. Thus, any monic \monorar{x}{X}{G} gives rise to a subobject [\monorar{x}{X}{G}].
%It is easy to see that if $x\simeq y$, then $\Img(x)=\Img(y)$ 
 %\monoarrow{X}{x}{G} is an element of $M_G$, we will call it a representative of the subobject and denote the latter by $[\monoarrow{X}{x}{G}]$  (thus $[\monoarrow{X}{x}{G}]=\monoarrow{Y}{y}{G})$ for any two equivalent  
 Among the members of the class $[\monorar{x}{X}{G}]$, there is a monomorphism $\monoarrow{H}{\subseteq}{G}$ whose domain $H$ consists only of elements which are also elements in $G$ 
 --- we call it {\em inclusion} and denote by $H \hookrightarrow G$. Thus, for any object $I\in \II$, we have subsetting $H(I)\subseteq G(I)$.  %$\incrar{x}{H}{G}$ 
%Thus, when working with a class of monomorphisms we will often choose this special inclusion morphism, denoted $\inlinemonoarrow{H}{}{G}$, as the representative of this class.\zd{May be rewritten shorter; I'll do it later}

\zd{the problem is that we need to prove that for any subobject $[\monorar{x}{X}{G}]$ there is an inclusion representing it. For this, we need the image factorization.}
\subsubsection{Images}
The third an final concept we are borrowing from set theory are \emph{images}.
Categorically, the are given by epi-mono factorizations.
Let $\arrow{H}{f}{G}$ be an arbitrary arrow in $\cat{G}$, because $\cat{G}$ has epi-mono factorizations $f$ is equal to the composite $\compose{e}{m}$ where $e$ is an epimorphism and $m$ is a monomorphism. 
The codomain $\image{f}$ object of $e$ (domain of $m$) is called the image and it is unique up to isomorphism, thus we can choose $m$ to be an inclusion morphism. \zd{but see my remark above!}
The situation is depicted in the following diagrams.
\[
\xymatrix{ 
	H \ar[rr]^f \ar@{->>}[dr]_{e} & & G \\
	& \image{f} \ar@{^{(}->}[ur]
}
\]
%\zd{Still I prefer $\rCover^e$ for epis, especially that here we deal with images, not epics as such (see Freyd-Scedrov)}

\subsubsection{Subobject lattices}
From the above it follows that for every object $G \in \cat{G}$, there exists a \emph{subobject lattice} denoted $\subobjlattice{G}$.
It is given by the subcategory $\subobjlattice{G} \subseteq \sliceCat{\cat{G}}{G}$ of the slice category whose objects are abstract subobjects, meets are given by pullbacks in $\cat{G}$, and joins are given by $\image{[\iota_H,\iota_K]}$ the image of the universal coproduct arrow for $H \xrightarrow{\iota_H} H+K \xleftarrow{\iota_K} K$ being the coproduct of the abstract subjects $H \in \subobjlattice{G}$ and $K \in \subobjlattice{G}$.
Furthermore, for a morphism $\arrow{H}{f}{G} \in \cat{G}$ we denote the pullback-functor (change of base) on the subject lattices of $G$ and $H$ by $\arrow{\subobjlattice{G}}{\pbfunctor{f}}{\subobjlattice{H}}$.
Note, that this functor has both a left (post-composition) adjoint $\arrow{\subobjlattice{H}}{\pbfunctorLeftAdjoint{f}}{\subobjlattice{G}}$ and a right (bundling) adjoint $\arrow{\subobjlattice{H}}{\pbfunctorRightAdjoint{f}}{\subobjlattice{G}}$.
%}
\zd{Shorter: Any topos is a regular category. Hence, we have adjunctions $\pbfunctorLeftAdjoint{f}\dashv\pbfunctor{f}\dashv\pbfunctorRightAdjoint{f}$ (see Freyd-Scedrov). For presheaf toposes, these adjunctions are given component-wise(?)}
 % END OF THE renewcommand for \II

\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{figures/BasicUniverse}
	\caption{Semantical Universes: Overview}
	\label{fig;semanticalUniverses}
\end{figure}

\subsubsection{Adhesiveness}

Thus, it is important to recall that every presheaf topos $\catSet^\cat{B}$ is adhesive and adhesiveness is closed under the ``operations'' product-,slice, coslice- and functor-category \cite{LackSobocinski2004}.

In every adhesive category the following facts hold


\begin{myfact}[Adhesive Category Properties \cite{LackSobocinski2004}]
\label{fact:adhesive}
	\begin{itemize}
		\item Monomorphisms are stable under pushouts.
		\item Pushouts along monomorphisms are pullbacks.
		\item Pushout complements of monos are unique up to isomorphism.
		\item Pushout can be decomposed along pullbacks.
	\end{itemize}
\end{myfact}
These properties are required to establish the major theorems in DPO rewriting regarding Concurrency, Parallelism, Embedding and Critical Pairs of productions, for details see \cite{EhrigEhrigPT2006}.
Critical Pairs are important for analysis of confluence.
In general, confluence for a DPO rewriting system known to be terminating is undecidable \cite{Plump1993}.
However, when considering a variation of DPO with interfaces \cite{GaducciHeckel1998} confluence is decidable \cite{BonchiGaducciKSZ2017}.
This fact is basis for theorem proving for SMTs described in \cite{BonchiGaducciKSZ2018}.

==> sections/mathBackgr--sliceCats.tex <==
\zd{this is a very useful link to why fibrations are preserved by PB}
\verb|https://math.stackexchange.com/q/157075|

\begin{mygroup}
	\renewcommand{\CC}{\GG}
	\renewcommand{\X}{G}

\subsection{Slice \caties\ over a \caty\ with pullbacks}\label{sec:sliceCats}
The following results are basic for slice \caties. 
%Let \CC\ be any \caty\ with pullbacks and \frar{f}{S'}{S} is an \CC-arrow.
\begin{lemma}[Substitution functors, P. Freyd \cite{Freyd-aspects}]\label{lemma:dirSubst-inAppendix}
	Let \CC\ be a \caty\ with pullbacks and \frar{f}{\X}{\X'} is a \CC-arrow. There is an adjunction between slice \caties:
	$f_*{:}\, \CC/\X\rightleftarrows\CC/\X'\,{:}f^* $, $f_* \dashv f^*$,
	%\begin{tikzcd}[row sep=2ex, column sep=4ex]
	%\CC/S' \ar[r, "\CC/f", bend left=25] %\ar[r, phantom, "\footnotesize \perp"]
	%& \CC/S \ar[l, "f^*" , bend left=25]
	%\end{tikzcd}
	where functor $f_*$ (or $\CC/f$) is defined by postcomposition with $f$, and functor $f^*$ is defined by pulling back over $f$. 
	\qed
\end{lemma}
\begin{constrN}[in which the \pblemma\ is heavily employed by default.]\label{constr:PBfunVconstr}
	Let $\GG$ be  a \caty\ with pullbacks and $G\in\Obb\GG$. We take a product $\GG/G\timm\GG/G$ in \catcat,  in which one copy of $\GG/G$ is considered {\em horizontal} (h) and the other is {\em vertical} (v). Having an arrow $v$ in the v-copy of $GG/G$ and an arrow $h$ in the h-copy of $\GG/G$, pulling $v$ back along $h$ gives rise to an operation \frar{\pbfunvX{G}}{\GG/G\timm\GG/G}{\arrowcatX{\GG}} on objects and arrows as shown in the diagram below (where all squares are PB, and pair $(\bar{\bar g}.\bar{u},\, g )$ is a \arrowcatCC-\mor\ \frar{\pbfunvX{}(u,g)}{\pbfunvX{}(v',h')}{\pbfunvX{}(v,h)}.
	We prefer to identify objects of \arrowcatX{GG}, which have the same codomain and iso\moric\ domains, which makes \pbfunvX{G} a single-valued operation. % into $\arrowcatX{\GG}_\cong$, 
	 Composition and identity are strictly preserved after $\cong$-factorization. Thus, we have a   
	 functor \frar{\pbfunvX{G}}{\GG/G\timm\GG/G}{\arrowcatX{\GG}_\cong}, where$\cong$ denotes the equivalence just specified.
	%equivalence $\cong$ identifies two \GG-arrows if they have the same codomain and iso\moric\ domains. 
\begin{equation}\label{eqdiag:PBfunVconstruction}
	\twixlemmaDefiningPBfunV		
\end{equation}
\end{constrN}
%
		%\input{sections/piece--twistedLemmaOld} % with wrapped ddiagram 
% twisted lemma without wrapping 
Now yet another application of the \pblemma\ provides the following result. 
\begin{lemma}[Twisted substitution]\label{lemma:twistedSubstProof}
Let \CC\ be a \caty\ with pullbacks and \frar{f}{\X}{\X'} is a \CC-arrow. Then diagram  below commutes, where 
	\caties\ $P$, \twistedX{P}, and $P'$ are products (whose projections are referred to as  `horizontal' (h) and 'vertical' (v) ), 
	arrows $f_*$ and $f^*$ are the postcomposition and the pullback functors, 
	$\arrowcatGGcong$ is the arrow \caty\ of \GG\ factorized as specified above, 
	%by an equivalence $\cong$, which 	 identifies two arrows if they have the same codomain and iso\moric\ domains, 
	and  functors \pbfunvX{X} for $X\in\Obb\GG$ are defined above. %will be defined (see diagram b) explained below).  % \ref{constr:twistedPBfunctor}, 
%---
%	\input{diagrams/twistedLemma--Proof}
\begin{equation*}\label{eqdiag:twistedLemma-Proof}
	\begin{tabular}{c} %@{\hspace{-4ex}}c}
		\twixlemmaCattyDiag
%		& \twixlemmaDefiningPBfunV
%		\\
%		a)  lemma statement
%		& b) Construction of functor \frar{\pbfunvX{}}{\CC/\X\timm\CC/\X}{\arrowcatCCcong}
	\end{tabular}
\end{equation*}
\end{lemma}
%\begin{remark} {\em Remark.}
%Note that product \caties\ $P$ and $P'$ are similar: %in terms of Constr. \ref{constr:twistedPBfunctor}, 
%one of their components is a ``vertical'' and the other is a ``horizontal'' copy of the same slice \caty. Product \twistedX{P} is twisted and takes its vertical and horizontal elements from different slice \caties\ % (but again one of them is vertical and the other is horizontal). 
%so that there is no a direct vertical arrow from \twistedX{P} to $\CC^\twocat$. However,  each of the substituting functors $f_*$ and $f^*$ allows for an indirect path from \twistedX{P} to $\CC^\twocat$.   The lemma states that these two paths are equal (actually up to iso\mor\ as pullbacks are defined up to iso). % is the statement of commutativity of the central  arrow rectangle  (visualized as a triangle): $!.\pbfunV = !'.\pbfunV'$. 
%\end{remark}
%{\em Proof.} 
%We begin with defining functor  \frar{\pbfunvX{}}{\CC/\X\timm\CC/\X}{\arrowcatCCcong} for any object $\X$ in \CC. %Having an arrow $v$ in a v-copy of $GG/G$ and an arrow $h$ in a h-copy of $\GG/G$, pulling $v$ back along $h$ gives rise to a single-valued operation \pbfunvX{} on objects and arrows as shown in diagram b) above (where all squares are PB). Pair 
%$(\bar{\bar g}.\bar{u},\, g )$ is a representative of \arrowcatCC-\mor\ \frar{\pbfunvX{}(u,g)}{\pbfunvX{}(v',h')}{\pbfunvX{}(v,h)}. Composition and identity are strictly preserved after $\cong$-factorization. %quotienting wrt. the corresponding $\cong_X$.  
%
Note that products $P$ and $P'$ take their h- and v-elements from the same slice \caty, while  product  \twistedX{P} is twisted and take sits elements from different slice \caties\ % (but again one of them is vertical and the other is horizontal). 
so that there is no a direct operation from \twistedX{P} to \arrowcatCCcong. However,  each of the substituting functors $f_*$ and $f^*$ allows for an indirect path from \twistedX{P} to \arrowcatCCcong. The equality of these two paths is guaranteed by yet another application of the \pblemma.  
Hence, for any arrow \frar{f}{G}{G'}, there is an operation (functor) \pbfunvX{f} as specified in the diagram. \qed 
%%\begin{corol} %went to appendix
%%	Currying provides that any ``vertical'' arrow $v\in \Ob \CC/X$ gives rise to a functor \frar{\pbfunV(v,\_)}{\CC/X}{\CC^\twocat} further denoted by \twSubstX{v}.  Now for any \frar{f}{X'}{X}, we have $(\CC/f).\twSubstX{v} = \twSubstX{f^*(v)}$. 
%%\end{corol}
%\begin{corol}
%	Currying provides that any ``vertical'' arrow $v\in \Ob \CC/X$ gives rise to a functor \frar{\pbfunV(v,\_)}{\CC/X}{\CC^\twocat} further denoted by \twSubstX{v}.  Now for any \frar{f}{X'}{X}, we have $f_*.\twSubstX{v} = \twSubstX{f^*(v)}$. 
%\end{corol}
%
%\input{diagrams/twistedSubst}
\end{mygroup}


==> sections/mathBackgr-fibredSpans.tex <==
\begin{lemma}[Jacobs]\label{lemma:comma2fibredSpans}
	Let $(p,q)$ be a cospan of two functors.  Then span $(\liftedX{p}, \liftedX{q})$ of projections (see diagram a) below) is a fibred span as shown in diagram a'). 
	
\noindent 
	\begin{tabular}{cc}
		\commalemmaGeneralDiamond
		& \commalemmaGeneralElementsFull
		\\
		a) & a')
	\end{tabular}
\end{lemma}
%

==> sections/mathBackgr-grothEquivalences.tex <==

\clearpage
\section{Grothendieck equivalences}\label{sec:grothEquiv-table}

Grothendieck \equce s are a major vehicle for the mathematics underlying data modelling semantics, and we need a reference section. We begin with a very special simple case for graphs. \zd{\large Nope: it's better to begin with the table for cats, and then consider the graph case as in \cref{prop:grothEqv4graphs} together with its immediate continuation for freely gen cats and functors. }
\begin{propo}[Grothendieck equivalence for graphs] \label{prop:grothEqv4graphs}
	For any small graph $G$, there is a canonical bijection $\Graphcat(G, \carr{\spancat}) \cong \ObX{\graphcat/G}$, where \Graphcat\ and \graphcat\ refer to the categories of graphs, resp., small graphs, and their \mor s. \qed
\end{propo}
This result can be extended for the entire  slice \caty\ $\graphcat/G$ by introducing suitably defined transformations between graph \mor s, but we do not need it as below we consider a whole series of such results for categories and functors rather than graphs and graph \mor s.

The table in \cref{fig:grothEquivalences} summarizes main results. It presents eight equivalences between fibred (left) and 
%
\input{figures/grothEquiv-table}
%  
\noindent
 indexed (right column) categories that may appear in data modelling. Equivalences i-iii) and viii) are well known (\eg, \cite{neifield}): subscripts \nmf{fful} and $\void$ in the left column mean that we only consider faithful, resp., discrete-fiber functors between small categories, while \dofcat\ denotes the \caty\ of categories and discrete opfibrations as \mor s, which is a full sub\caty\ of \catcat. In the right column, \spanbicat\ and \relbicat\ are bicategories of, resp., spans and relations between small sets, $S$ is a small \caty\ considered as a 2-discrete bi\caty, and \Laxcat\ is the \caty\ of lax functors and {\em functional} oplax natural \transf s, whose transformational \mor s  are functions between sets rather than spans (resp., relations) as it should be in the general case, for which the transformational \mor s are general \mor s in the target \caty.  Below we will omit adjective 'functional' as all \transf s we consider are functional. 
 
 \Equce s iv-vii) involve a family of {\em factorization lifting} properties that functor into $S$ may (or may not) have. Given a functor \frar{p}{E}{S}, an arrow \frar{f}{a}{b} in $E$ and a factorization of its image $p(f)=v.w$ in $S$, we say that this factorization can be {\em lifted} if there are arrow $g\in p^{-1}(v)$, $h\in p^{-1}(w)$ in $E$ such that $g.h=f$.  If, for any arrow $f$ in $E$  and any factorization of $p(f)$ in $S$, there is at least one lift, we say that $p$ possesses a {\em weak factorization lifting} property (or is a {\em wfl} functor), and if there is only one lift for each factorization  of $p(f)$ for all $f$, then $p$ is a {\em unique factorization lifting (ufl)} functor. It is easy to see wfl functors are closed under composition and identity, and the same holds for ufl functors. Hence, we have wide \catcat-subcategories \wflcat\ and \uflcat. Moreover, if a composed functor $p.p'{:}\, E\xrightarrow{p}S\xrightarrow{p'}B$ is wfl (or ufl), and the second component is also wfl (resp. ufl) then the first component $p$ is wfl (resp. ufl) too. Then slice \caties\ $\wflcat/S$ and $\uflcat/S$ are full subcategories of $\catcat/S$.%
 \footnote{Write about Conduche fibrations} 
 \zd{\sc  TO be finished: write about \equce s iv-vii)}

==> sections/mathBackgr-smcats.tex <==
\section{SMCs and String Diagrams}
\label{sec:smcs}
Composition of arrows in a category is actually \emph{sequential} composition.
The concept providing us with \emph{parallel} composition is called a \emph{symmetric monoidal category}, short sm-cat or SMC.

\begin{mydef}{}{(Symmetric Monoidal Category)}\label{def:smcat}
Let $\cat{C}$ be a category.
A \emph{monoidal structure} $(\cat{C}, \boldsymbol{I}_\cat{C}, \otimes_\cat{C})$  on $\cat{C}$ is given by an object $\boldsymbol{I}_\cat{C}$ called \emph{monoidal unit}, a bifunctor $\otimes_\cat{C} : \cat{C} \times \cat{C} \to \cat{C}$ called \emph{monoidal product} and families of natural isomorphisms.
\begin{description}
	\item[Left Unitor] $\lambda_C : I \otimes C \cong C$ for all $C \in \catObj{\cat{C}}$
	\item[Right Unitor] $\rho_C : C \otimes I \cong C$ for all $C \in \catObj{\cat{C}}$
	\item[Associator] $\alpha_{C,D,E} : (C \otimes D) \otimes E \cong C \otimes (D \otimes E)$ for all $C, D, E \in \catObj{\cat{C}}$
\end{description}
If these isomorphisms are actual identities, the monoidal structure is called \emph{strict}.
If there is additionally the following fourth family of natural isomorphisms, the monoidal structure is called \emph{symmetric}.
\begin{description}
	\item[Symmetry] $\sigma_{C, D} : C \otimes D \cong D \otimes C$ for all $C, D \in \catObj{\cat{C}}$
\end{description}
The above families of isomorphisms have to obey the \emph{pentagon} and \emph{triangle} laws expressed through the following commutative diagrams:
\begin{eqnarray}
\label{eq:pentagon}
\resizebox{0.9\linewidth}{!}{
	\xymatrix @C=-1cm {
		& (A \otimes (B \otimes C)) \otimes D \ar[rr]^{\alpha_{A,B\otimes C,D}}  & & A \otimes ((B \otimes C) \otimes D) \ar[dr]^{id_A \otimes \alpha_{B,C,D}} & \\
		((A \otimes B) \otimes C) \otimes D \ar[ur]^{\alpha_{A,B,C} \otimes id_D} \ar[drr]_{\alpha_{A\otimes B,C,D}}   & & & & A \otimes (B \otimes (C \otimes D)) \\
		& & (A \otimes B) \otimes (C \otimes D) \ar[urr]_{\alpha_{A,B,C\otimes D}} & &
}} \\
\label{eq:triangle}
\resizebox{0.9\linewidth}{!}{
	\xymatrix{
		(A \otimes I) \otimes B \ar[dr]_{\rho_A \otimes id_B} \ar[rr]^{\alpha_{A,I,B}} & & A \otimes (I \otimes B) \ar[dl]^{id_A \otimes \lambda_B} &  B \otimes A \ar[dr]^{\sigma_{B,A}} & \\
		& A \otimes B &  A \otimes B \ar@{=}[rr] \ar[ur]^{\sigma_{A,B}} & & A \otimes B
}}
\end{eqnarray}
\end{mydef}

%\mkExample{Examples of SMC}{ex:SMC}{
\begin{myexa}[Examples of SMC]\label{ex:SMC}
There are some well known examples of SMC:
\begin{itemize}
	\item $(\catSet, \times)$: The symmetric monoidal structure given by choosing the monoidal product to be given as the cartesian product $\times$ and the monoidal unit given by the singletong set $\{\bullet\}$ in category of sets and mappings $\catSet$.
	\item $(\catSet, \sqcup)$: The symmetric monoidal structure given by choosing the monoidal product to be given as the disjoint union $\sqcup$ and the monoidal unit given by the empty set $\emptyset$ in category of sets and mappings $\catSet$.
	\item $(\cat{C}, +)$: Any category which posses all pushouts and an initial object provides a symmetric monoidal structure given by binary coprodutct as monoidal unit and the initial object being the monoidal unit. Arrows in $(\cat{C}, +)$ are given by co-spans of $\cat{C}$-morphisms.
\end{itemize}
%}
\end{myexa}

The equivalent of a functor for SMCs is called a (lax) symmetric monoidal functor:
\begin{mydef}{smFunctor}{Symmetric Monoidal Functor}
Let $(\cat{C}, \boldsymbol{I}_\cat{C}, \otimes_\cat{C})$ and $(\cat{D}, \boldsymbol{I}_\cat{D}, \otimes_\cat{D})$ be two symmetric monoidal categories.
A symmetric monoidal functor $(F, \phi)$ between these categories is given by
\begin{enumerate}
	\item A functor $F : \cat{C} \to \cat{D}$;
	\item A morphism $\phi_{\boldsymbol{I}} : \boldsymbol{I}_\cat{D} \to F(\boldsymbol{I}_\cat{C})$;
	\item A family of morphisms $\phi_{C,C'} : F(C) \otimes_{\cat{D}} F(C') \to F(C \otimes_\cat{C} C')$ for each $C, C' \in \cat{C}$, which are both natural for $C$ and $C'$.
\end{enumerate}
such that the coherence maps $\phi$ are compatible with natural isomorphisms in both symmetric monoidal categories.
If all coherence maps are isomorphisms $(F, \phi)$ is called a \emph{strong} symmetric monoidal functor\footnote{Otherwise it is called \emph{lax} but we omit this adjective as we generally work with lax symmetric monoidal functors.}.
\end{mydef}

SMCs provide a powerful visualization given by \emph{string diagrams}.
String diagrams go back to Feynman and Penrose that used them more or less informally.
Their formal nature was first investigated in \cite{JoyalStreet1991} and has since then found more and more application areas.
We refer to \cite{Selinger2011} for a comprehensive survey.
The benefit of string diagrams is that they \emph{internalize} the congruences among arrows induces by the category property of $\cat{C}$, bifunctor property of $\otimes$, natural isomorphisms $\lambda, \rho, \alpha, \sigma$ and equations \ref{eq:pentagon} and \ref{eq:triangle}:
When two arrows have the same representation as a string diagram, they are equal modulo the above congruences.
Table~\ref{tab:stringDiagramVizz} briefly sketches the inductive structure of string diagrams.
\begin{table}
\begin{tabularx}{\linewidth}{|X|c|}
\hline
\textbf{Arrow in} $\catArrows{\cat{C}}$ & \textbf{Visualization} \\
\hline
%Identities  $\id{C}: C \to C $ & $\scalebox{0.4}{\tikzfig{identity}}$ \\ \hline
%Symmetries $\sigma_{C,D} : C \otimes D \to D \otimes C$ &  $\scalebox{0.4}{\tikzfig{symmetry}}$ \\ \hline
%All other arrows $\arrow{C}{f}{D}$ &  $ \scalebox{0.4}{\tikzfig{arrow}}$ \\ \hline
%Sequential composition $\compose{f}{g}$ of  $\arrow{C}{f}{D}$ and $\arrow{D}{g}{E}$ & $\scalebox{0.4}{\tikzfig{sequentialComp}}$ \\ \hline
%Parallel composition $f \otimes g$ of $\arrow{C}{f}{D}$ and $\arrow{C'}{g}{D'}$ & $\scalebox{0.4}{\tikzfig{parallelComp}}$ \\ \hline
\end{tabularx}
\caption{String Diagram constituents}
\label{tab:stringDiagramVizz}
\end{table}

An important class of SMCs is given by so called \emph{\textbf{pro}duct and \textbf{p}ermutation} (short PROP) category \cite{MacLane1965}, which is a strict SMC where the objects are given by the natural numbers, monoidal unit is the number 0 and monoidal product is given by addition. 
Natural numbers can be thought of as the free monoid over a one-element set, thus every natural number can be identified with the number of wires going in and out of each block representing an arrow.
Concretely, this means that in a PROP the label on the wires can be removed.
PROPS provide the syntax for \emph{symmetric monoidal theories (SMT)}, the SMC equivalent of \emph{algebraic theories} for regular categories, hence they play an important role for algebraic reasoning in several practical application areas \cite{CoeckeDuncan2008,BaezErbele2015,SobocinskiStephens2014}.


==> sections/mathBackgrounds/backgr-mathAspects.tex <==
\subsection{Mathematical aspects}
\subsubsection{Why generalized graphs and generalized sketches} %, and categorical signatures}

As discussed above, categories hosting software models are categories of sketches; Sect.~\ref{sec:viewExample} (in Appendix) presents an example).  % and their models (in the mathematical sense). 
In general, a sketch is a graphical structure endowed with labelled diagrams (a.k.a. constraints); in the project, we consider a very general version of the notion: our 'graphs' are finitary presheaves, and our constraints of shape $G$ are any ``devices'' that classify mappings from $G$ as either valid or invalid. The generality of our graphs is caused by the great diversity and complexity of graphical structures used in SE  \cite{Kent2002}, and graphs used for behavioural and workflow  models can even be more complex. %Hence, we consider a very general notion of a graph as being a presheaf \frar{G}{\HH}{\setcat}  whose schema $\HH$ is any finite category. \footnote{In the long version, we consider an important requirement to \HH\ motivated by other parts of the project, but it is not needed for results described in the present paper.}
Similarly, constraints used in domain modelling (banking, e-commerce, automotive etc.) can be complex and very elementwise-oriented so that their representation in a standard categorical way via universal properties can be rather bulky and unwieldy (a detailed discussion can be found in \cite{DiskinWolter2008}, see also Appendix). Thus, we need  constraints and sketches of a very general nature; Michael Makkai called them {\em generalized sketches} in \cite{Makkai1997}.  %Diagrammatic constraints are an integral part of the domain and software modelling, and  important for specifying correct view mappings. Hence, we need to consider graphs endowed with constraints declared over them, \ie, graphical/diagrammatic theories or {\em ()generalized) sketches}. Thus, our category of artifacts and their mappings should be a category of sketches and sketch \mor s.
%
%\subsubsection{Signatures are categories}
%DEPENDENCIES ARE IMPORTANT ...... BLAH-BLAH
%\subsection{Mathematical issues}
\subsubsection{Why sketches with diagrams operations rather than string diagrams} % do not work for diagram operations}
\renewcommand{\propcat}{\enma{\catname{PROP}}}


The objects in a \propcat\ are natural numbers, and arrows represent operations, where domain and codomain denote in- and output arity (operations are multiary but one-sorted). Being symmetric monoidal (sm) categories, $\catname{PROPs}$ can be  visualized with String Diagrams \cite{Selinger2011}, an intuitive yet formal graphical syntax. For example, string diagrams in 
Fig.~\ref{fig:exSMC} depicts a ternary term $(x + y) * (x + z)$ built from two binary operations. % in string diagram notation, which is a ternary operation ($\in \catname{PROP}(3,1)$) where 
Note that reuse of the middle variable $y$  is shown explicitly with  $\nfont{Copy}$-operation (visualized via \includegraphics[width=1em]{figures/Copy}). This is possible as 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/pbStories-StringDiagram.pdf}
	\caption{String diagram notation for ordinary algebraic terms}
	\label{fig:exSMC}
\end{figure}
%Unfortunately, we cannot use this machinery for diagram operations. The classical operations are \setcat-based and 
set $\{x, y, z\}$ is the coproduct of its elements $\{x\}\sqcup\{y\}\sqcup \{z\}$.
However,  diagram operations are graph-based,  %\footnote{Throughout this paper we will use the term ``graph'' in a more general sense, see Sect.~\PAST{Reminder to put the correct reference}}.
and a graph (while being a colimit of its elements) is not their coproduct!
\input{figures/insert-ex3pb}

%\zd{this piece is to be rewritten for the new version of Fig.~\ref{fig:ex3pb} }
Figure~\ref{fig:ex3pb} presents a simple example showing how the machinery of sketches work. Diagram (a) is a typical example of categorical diagram chasing. Suppose we have a diagram operation \pbpred\ defined over any graph: it takes a cospan of arrows as its input and returns a span of arrows, which together with the input cospan forms a square in a familiar way. In addition, we assume there is a predicate symbol \monicpred, which can be declared for an arrow. Moreover, if an input arrow for a \pbpred-application is monic, then the corresponding output arrow is monic too; this is usually termed as ``monics are stable under \pbpred''. The left (black and blue) sub-diagram in (a) shows a diagrammatic term formed by three applications of \pbpred. 

We begin with a graph consisting of three arrows $\{x,y,z\}$ with a common target $O$. Applications $a$ and $b$ of \pbpred\  extend the graph with four arrows as shown, and two of them are monic according to the ``monic are stable'' property. (We paint the operation chevron and elements it produces into blue to recall the mechanical computation nature of these operations.)  Then we apply \pbpred\ yet another time and produce two more monic arrows. In everyday categorical routines, the tentacle arrows are not needed because i) any user of categorical routines knows the arity shape of operation \pbpred, and ii) the operation is commutative in the sense that $(y_1,y_2)=\pbpred(x_1,x_2)$  implies $(y_2,y_1)=\pbpred(x_2,x_1)$. We will refer to the entire black-blue sketch as to a {\em term-sketch} or {\em a query} $Q(X)$, which can roughly be considered as an application of query $Q=(a+b);c$  to sketch $X$. 
Note that queries extend a given input sketches so that we always have embedding \frar{\eta_Q}{X}{Q(X)}. 

Suppose now that for further processing, we only need a part of the entire black-blue sketch as shown by mapping $v$ (in orange) that maps the interface sketch $V$ to sketch $Q(X)$; note that \flar{v}{Q(X)}{V} is a correct sketch morphism as it respects all diagrams  in sketch $V$ (in the example, $V$ has just one diagram, but if it has more, they all are to be respected by mapping $v$). Thus, pair $(Q,v)$ makes a cospan $X\xrightarrow{\eta_X}Q(X)\xleftarrow{v}V$, which van be seen as an arrow from $X$ to $V$. In different terminological disciplines, such a cospan could be called {\em open} term-sketch, or {\em rooted} term-sketch (and then sketch $X$ would be referred to as a sketch of {\em variables}). We will refer to pair $(Q,v)$ as to a {\em view} of $X$ with {\em schema} $V$ and {\em view (definition)} mapping $v$; or else as a {\em combinatorial Kleisli mapping}.  

Although notation in diagram (a) is accurate, it is not entirely formal: the actual formal procedures underlying diagram (a) are shown in diagram (b). Arity of \pbpred\ is specified as a monic between two graphs, and the presence of the monic label in the input implies yet another monic label in the output. It is clear that in diagram a), input tentacle arrows into chevrons $a{:}\pbpred$, $b{:}\pbpred$ actually denote  mappings $\beta_a$, $\beta_b$, and together with output tentacles they denote mappings  $\beta'_a$, $\beta'_b$ into sketches produced by the corresponding pushouts $PO_a$, $PO_b$ (arrows with stroked tails and hollow triangle heads (like for inheritance in the UML) denote monics). Note that we need yet another PO to produce the resulting sketch $X_a+_X X_b$ formally. Then we can apply \pbpred\ yet another time by defining a mapping $\beta_c$, and so on. Thus, notation in diagram a) hides a series of PO computations under the hood similarly to how string diagrams hide axioms of hypercategories.  

In the report, we will show that sketches and views can be endowed with a structure of a {\em semi-hyper-category (sHyp-category)}, \ie, symmetric monoidal category with two additional operations, duplicator/copying and discharger (garbage collector), which satisfy the monoidality and coherence axioms. Such categories under the name of {\em gs-monoidal} categories are discussed in \cite{CorradiniG-acs99} in detail.  The tensor product is played by the (chosen) sketch coproduct, and the sequential composition is done via pushout, which is nothing but query substitution.  

Diagram c) presents a set-based counterpart of the term a), in which operation \pbpred\ is simulated by operation $*$ of arity (2,2) (in fact, (2,2) is an arity-coarity pair but we will call it arity): it takes two elements as its input and outputs two elements denoted by $\_*_1\_$ and $\_*_2\_$. Sharing of variable $y$ can be modelled by applying operation \nmf{copy} of arity (1,2), and exclusion of elements from the view is modelled by applying discharger operation of arity (1,0). The string diagram c) can thus be seen as a term in the signature of semi-hyper-categories. In contrast, diagrammatic term a) is not an sHyp-term: although arrow $y$ is shared, we cannot model it by copying due to the graphical structure: while a set is a tensor (coproduct) of its elements, a graph is not. Similarly, we cannot model exclusion of arrows $y_x$ and $y_z$, and label $c_1{:}\monicpred$, from the view by applying an ``arrow discharger'' or a ``label discharger'' due to structural constraints imposed on those elements.  The structure of sH-category over diagrammatic term-sketches only appears on the macro level, when we consider ports whose types are sketches rather than elements.  

\endinput



 
Part (A) uses a typical categorical notation: the diagram presents a workflow consisting of two pullbacks taken in parallel over spans with one monic leg, followed by yet another pullback. Monic preservation by pullbacks is also shown. %In addition,  by naming conventions and respective symbols in the corners we show that some elements in the diagram are constructed via pullbacks, and via arrow decorations we specify some of the arrows to have special properties (being monic).
Part (B) makes the above explicit by using labels for constraint declarations (ovals) and operation applications (chevrons), and showing their scope. % make the stion elements in the diagram are explicated. 
Note that arrows going in and out of chevrons  show the workflow and what elements are constructed/derived (blue and dashed) rather than given. 
Part (C) is similar to Fig.~\ref{fig:exSMC} and highlights the workflow of the query by making the order of operation applications explicit, e.g. the pullback \nfont{c} depends on elements produced by the other two pullbacks.

\zd{This piece is to be revised wrt. the new version of Fig.~\ref{fig:ex3pb}(C)!!!}

Note several important differences with Fig.~\ref{fig:exSMC}. First, in discrete $\catname{PROP}$-setting, the elements produced by an operation have no further relationship with the input elements, while in the graph-based setting, there is an overlap between the input and the output, e.g. element $B$ in \figref{ex3pb}(a) is both in the input and the output of the pullback application \nfont{a}, and similarly for application \nfont{b} so that $B$ is also shared by \nfont{a}-output and \nfont{b}-output. Second, the workflow shown in \figref{ex3pb}(C) is a rather poor view of the actual workflow under the hood, which consists of several pushouts (POs): three POs are needed to produce graph $X'$ and yet another one to produce $X''$. Workflow arrows with hollow ends are, in fact, pairs, $(X,a)$, $(X,b)$ etc.,  while mappings that do the job, \eg, the one showing what part of graph $X$ is used as an input for \nfont{a{:}[pb]}, are not shown. %etc., and monics from $X$ to $X'$ to $X''$, are not shown. 
Thus, in contrast to \figref{exSMC}, diagram \figref{ex3pb}(C) is an incomplete specification of the story.  


==> sections/mathBackgrounds/backgroundFibrationProofs.tex <==


\begin{proof}
(To prove that $\proj{IE}$ is a opfibration, let $\frar{\topBackIE}{\topBackI}{\topBackE}$ and $\frar{\bottomBackIE}{\bottomBackI}{\bottomBackE}$ be two objects in  $\arrowCat{\CC}$ and $\frar{(\backDownI,\backDownE)}{\inlinearrow{\topBackI}{\topBackIE}{\topBackE}}{\inlinearrow{\bottomBackI}{\bottomBackIE}{\bottomBackE}}$ an arrow between them, i.e.
\begin{equation}
	\label{eq:toLift}
	\compose{\topBackIE}{\backDownE} = \compose{\bottomBackIE}{\backDownE}
\end{equation}

Let now 
\begin{equation}
\label{eq:liftSource}
\xymatrix{
	\topBackI  \ar[d]_{\topBackToFrontI} \ar[r]^{\topBackIE} &  \topBackE \ar[d]^{\topBackToFrontE}  \\
	\topFrontI \ar[r]_{\topFrontIE}  & \topFrontE 
}
\end{equation}
be an object in fibre $\proj{IE}^{-1}(\topBackIE)$, i.e. a pushout binding square.

First, we now have to construct the lift of $(\backDownI,\backDownE)$, i.e. an arrow in $\squarepoCat{\CC}$.
Such arrows can be visualized as prisms/cubes, see Fig.~\ref{fig:squarepoCatArrows}.
In Fig.~\ref{fig:squarepoCatArrows}, we depict the given elements from \eqref{toLift} and \eqref{liftSource} in black.
The blue elements are constructed.
We explain this stepwise construction using the ``flat'' presentation of the prism shown in part b) of Fig.~\ref{fig:squarepoCatArrows}.
First, note that $(i)$ is commutative because of \eqref{toLift} and the outline $(i) + (ii) + (iv) + (v)$ is pushout because of \eqref{liftSource}.
First we construct $(ii)$ and $(iv)$ as pushouts, which is possible since $\cat{C}$ has all pushouts.
Now, the following commutative diagrams:
\begin{align*}
	\backDownI\comp \bottomBackIE \comp \bottomBackToFrontE  & = \topBackIE \comp \backDownE \comp \bottomBackToFrontE \explain{Commutativity \eqref{toLift}} \\
	  &=  \topBackIE \comp \topBackToFrontE \comp \frontDownE \explain{Commutativity of Pushout $(iv)$} \\
	   & =  \topBackToFrontI \comp \topFrontIE \comp \frontDownE \explain{Commutativity of Pushout \eqref{liftSource}}
\end{align*}
establish a cocone over $\backDownI$ and $\topBackToFrontI$ such that from the universal pushout colimit property of $(ii)$, there is a unique arrow $\frar{\bottomFrontIE}{\bottomFrontI}{\bottomFrontE}$ such that 
\begin{eqnarray}
	\frontDownI\comp\bottomFrontIE = \topFrontIE\comp\frontDownE \label{eq:CommutativityOfV} \\
	\bottomBackToFrontI\comp\bottomFrontIE = \bottomBackIE\comp\bottomBackToFrontE \label{eq:CommutativityOfIII}
\end{eqnarray}
Thus. $(iii)$ and $(v)$ are commutative.


\newcommand{\comparisonApex}{C}
\newcommand{\comparisonInApexE}{c_1}
\newcommand{\comparisonInApexI}{c_2}
\newcommand{\universalArrow}{u}
\newcommand{\universalArrowHelper}{v}
\newcommand{\universalArrowCompare}{w}
Next, we have to show that $(iii)$ is indeed a pushout.
For this assume there exists in object $\comparisonApex$ and two morphisms $\frar{\comparisonInApexE}{\bottomBackE}{\comparisonApex}$ and $\frar{\comparisonInApexI}{\bottomFrontI}{\comparisonApex}$ such that
\begin{equation}
\label{eq:coconeComparison}
\bottomBackIE \comp \comparisonInApexE = \bottomBackToFrontI \comp \comparisonInApexI
\end{equation} 
We, now have to show the existence of a unique arrow $\frar{\universalArrow}{\bottomFrontE}{\comparisonApex}$ which makes the triangles $\compose{\bottomBackToFrontE}{\universalArrow} = \comparisonInApexE$ and $\compose{\bottomFrontIE}{\universalArrow} = \comparisonInApexI$ commute.

Starting by precomposing \eqref{coconeComparison} with $\frar{\backDownI}{\topBackI}{\bottomBackI}$ leads to
\begin{align*}
	\backDownI \comp \bottomBackIE \comp \comparisonInApexE & = \topBackIE \comp \backDownE \comp \comparisonInApexE \explain{Commutativity \eqref{toLift}} 
\end{align*}
and
\begin{align*}
	\backDownI \comp\bottomBackToFrontI \comp \comparisonInApexI & = 
	\topBackToFrontI \comp \frontDownI \comp \comparisonInApexI  \explain{Commutativity of $(ii)$}
\end{align*}
and thus from the universal pushout property of \eqref{liftSource} there exists a unique arrow $\frar{\universalArrowHelper}{\topFrontE}{\comparisonApex}$ such that 
\begin{eqnarray}
\label{eq:comparisonForIV}
\backDownE \comp  \comparisonInApexE  = \topBackToFrontE \comp \universalArrowHelper \\
\frontDownI \comp  \comparisonInApexI  = \topFrontIE \comp \universalArrowHelper  \label{eq:universalPropHelper}
\end{eqnarray}
The commutative diagram in \eqref{comparisonForIV} establishes a cocone for $\backDownE$ and $\topBackToFrontE$ and thus from the universal pushout property of $(iv)$ there is a unique arrow $\frar{\universalArrow}{\bottomFrontE}{\comparisonApex}$ such that
\begin{eqnarray}
\label{eq:IIIPOuniversalProp1} \bottomBackToFrontE \comp \universalArrow = \comparisonInApexE \label{eq:firstUniversalityOfIV} \\
	\frontDownE \comp \universalArrow = \universalArrowHelper \label{eq:secondUniversalityOfIV}
\end{eqnarray}
Equation \ref{eq:IIIPOuniversalProp1} already assures the first triangle commutativity to show universality of $\universalArrow$ (w.r.t $\comparisonInApexE$).
To verify the second triangle commutativity (w.r.t $\comparisonInApexE$) consider on the one hand:
\begin{align*}
\frontDownI \comp \bottomFrontIE \comp \universalArrow & = 
\topFrontIE \comp \frontDownE \comp \universalArrow \explain{Commutativity \eqref{CommutativityOfV}} \\ & = 
\topFrontIE \comp  \universalArrowHelper \explain{Commutativity \eqref{secondUniversalityOfIV}} \\ & = 
\frontDownI \comp  \comparisonInApexI \explain{Commutativity \eqref{universalPropHelper}}
\end{align*}
and on the other hand:
\begin{align*}
	\bottomBackToFrontI \comp \bottomFrontIE \comp \universalArrow & = \bottomBackIE \comp \bottomBackToFrontE \comp \universalArrow \explain{Commutativity \eqref{CommutativityOfIII}} \\
	 & =
	\bottomBackIE \comp \comparisonInApexE \explain{Commutativity \eqref{firstUniversalityOfIV}} \\ &  = 
	\bottomBackToFrontI \comp  \comparisonInApexI \explain{Commutativity \eqref{coconeComparison}}
\end{align*}
Since, $\bottomBackToFrontI$ and $\frontDownI$ are jointly epic due to $(ii)$ being a pushout, we have:
\begin{equation}
\label{eq:universalArrowPart2}
\bottomFrontIE \comp \universalArrow = \comparisonInApexI
\end{equation}
Finally, we have to show uniqueness of $\universalArrow$:
For this assume there exists another arrow such that. $\frar{\universalArrowCompare}{\bottomFrontE}{\comparisonApex}$ such that
\begin{eqnarray}
	\bottomBackToFrontE \comp \universalArrowCompare = \comparisonInApexE \\
	\bottomFrontIE \comp \universalArrowCompare = \comparisonInApexI
\end{eqnarray}
Now,
\begin{align*}
		\bottomBackToFrontE \comp \universalArrowCompare = \bottomBackToFrontE \comp \universalArrow  \explain{\eqref{IIIPOuniversalProp1}}
\end{align*}
and 
\begin{align*}
	\bottomFrontIE \comp \universalArrowCompare = \bottomFrontIE \comp \universalArrow  \explain{\eqref{universalArrowPart2}}
\end{align*}
\PAST{Oops, Am I missing something but I do not see a way to prove that $\universalArrow=\universalArrowCompare$?!}
Hence, we have just shown that the construction in Fig.~\figref{squarepoCatArrows} is indeed an arrow in $\squarepoCat{\CC}$.



Next, we have to show that it also \emph{opcartesian}.
Thus, we assume that there is another arrow $\frar{\liftComparisonName}{\liftSourceName}{\liftComparisonTargetName}$ in $\squarepoCat{\CC}$ and an arrow $\frar{\mediator}{\bottomBackIE}{\thirdSquareBackIE}$ in   $\arrowCat{\CC}$ such that
\begin{equation}
\label{eq:liftingAssumption}
	\proj{IE}(\liftName)\comp\mediator = \proj{IE}(\liftComparisonName)
\end{equation}
We can think of $\liftComparisonTargetName$ as yet another pushout square lying below $\liftTargetName$ in Fig.~\ref{fig:squarepoCatArrows} and $\liftName$ establishes a long prism where $\liftSourceName$ is the top face.
We have to show that this prism can be factored through $\liftTargetName$.
For this consider the rear left face of this big prism which is depicted below:
\begin{equation}
\xymatrix @C=4em {
\topBackI \ar@{}[dr]|{(ii)} \ar[r]_{\backDownI} \ar[d]_{\topBackToFrontI} \ar@/^1pc/[rr]^{\liftComparisonName_I} & \bottomBackI \ar[r]_i \ar[d]^{\bottomBackToFrontI} & \thirdSquareBackI \ar[d]^{\thirdSquareBackToFrontI} \\
\topFrontI \ar[r]^{\frontDownI} \ar@/_1pc/[rr]_{{\liftComparisonName_I}^*} & \bottomFrontI \ar@{-->}[r]^x & \thirdSquareFrontI
}
\end{equation}
In this diagram the following commutativity holds due to \eqref{liftingAssumption}:
\begin{equation}
	\backDownI \comp i = \liftComparisonName_I
\end{equation}
Since, $(ii)$ is a pushout we get the universal arrow $\frar{x}{\bottomFrontI}{\thirdSquareFrontI}$ such that 
\begin{eqnarray}
 i \comp \thirdSquareBackToFrontI = \bottomBackToFrontI \comp x \\
 \frontDownI \comp x = {\liftComparisonName_I}^*
\end{eqnarray}
The same can be done for the front right cube face the get the analoque for $x$, which provides the sought factorization.
\end{proof}




==> sections/mathBackgrounds/decorCospans.tex <==
\subsubsection{Views via Decorated Cospans}

Definition of a lax monoidal (or weak monoidal) functor can be found at nLab
https://ncatlab.org/nlab/show/monoidal+functor


In our case, we need the following instance of the notion. 
\begin{mydef}[Functor extending predicate sketches to operational sketches]
	\label{eq:laxmonfunctor4views}
We build a lax monoidal functor
%\begin{equation}\label{eq:laxmonfunctor4views}
$$
\frar{(\extfun,\extnat,\epsilon)}{(\skecatgp,\sqcup, 0)}{(\setcat,\times, 1)} 
$$
in the following four steps.%
\footnote{What we denote by \extnat, is  $\mu$ in nLab, and $\varphi$ in Fong's Decorated cospans} 

a)  For a \PP-sketch $S$, we define set $\extfun(S)$ to be the set of all \PPOO-sketch structures extending $S$:
$$\extfun(S)=\comprcolon{S'\in\skecatgpo}{\frestr{S'}{\PP}=S};$$

b)  For a sketch \mor\ \frar{g}{S_1}{S_2} in \skecatgp\ and $S'_1\in \extfun(S_1)$, sketch $S'_2:= \extfun(g)(S'_1)$ is the least \PPOO-sketch extending $S_2$ such that $g$ would be a correct sketch \mor\ \frar{g}{S'_1}{S'_2}, that is, 
$$ 
\iQueryset{S'_2}=\iQuery{S_2}\sqcup \frestr{\iQuery{S'_1}}{(\PPOO\;\setminus\;\PP)}
$$
and for any new index $q\in \iQueryset{S'_2}\setminus\iQuery{S_2}$, we define $\diagr_{S'_2}(q) :=\diagr_{S'_1}(q)\comp\carr{g}$%

c)  For any two \PP-sketches $S_1, S_2 \in\skecatgp$, we define a natural transformation 
$$\frar{\extnat_{S_1,S_2}}{\extfun(S_1)\times\extfun(S_2)}{\extfun(S_1\sqcup S_2)}$$ %(S'_1, S'_2)$$
by setting for any $S'_1\in\extfun(S_1)$, $S'_2\in\extfun(S_2)$, 
$$
\extnat(S'_1,S'_2) := S'_1 \sqcup S'_2 \text{~in \skecatgpo}
$$

d) Function \frar{\epsilon}{1_{\setcat}}{\extfun(0_{\skecatgp})}, where $1_{\setcat}=\{*\}$ and $0_{\skecatgp}$ is the empty \PP-sketch is defined by setting $\epsilon(*)$ to be the empty \PPOO-sketch, $\epsilon(*)=0_{\skecatgpo}$. 

\end{mydef}
%for any $\opvar\in\PPOO\setminus\PP$, $$\semm{\opvar}_{S'_2}=\compr{\dvar\comp \carr{g}{\dvar\in \semm{O}_{S'_1}} $$ 
%\zd{it needs polishing as i wrote it for the monosketch case}
%and for any two \PP-sketches $S_1, S_2$, 

--- 
%


==> sections/mathBackgrounds/dpo.tex <==
\section{DPO rewriting and Adhesive Categories}
\label{sec:dpo}
The DPO approach was invented in 1973 \cite{EhrigPfenderS1973} as an algebraic variant for rewriting in graph grammars, the latter representing a generalization of string-based BNF grammars.
DPO considers \emph{productions} $p = (L \xleftarrow{l} K \xrightarrow{r} R)$ as spans span in ``suitable'' category $\cat{G}$.
Given a morphism $\arrow{L}{m}{G}$, called \emph{match}, $G$ can be rewritten to $H$ denoted $G \rightsquigarrow_{(p,m)} H$ iff there exists the diagram
\begin{equation}
\label{eq:DPO}
\xymatrix {
	L \ar[d]_{m}   & K \ar@{>->}[l]_{l} \ar@{>->}[r]^{r} \ar[d]_{d}   & R \ar[d]_{n} \\
	G & D \ar@{>->}[l]^{l^*} \ar@{>->}[r]_{r^*} & H
}
\end{equation} 
in $\cat{G}$ such that both squares in \ref{eq:DPO} are pushouts.

To clarify the notion of ``suitable'' category:
Originally DPO was solely applied to the category of colored directed multigraphs.
To capture a bigger range of application areas, the concept of \emph{High Level Replacement (HLR)} category \cite{EhrigHabelKP1991} was introduced. 
The rather technical nature of the characterization of HLR categories motivated the pursuit of a more succinct characterization, which resulted in the concept of \emph{adhesive categories} \cite{LackSobocinski2004}.
An adhesive category posses all pullbacks and pushouts along monomorphisms which are additionally Van Kampen squares.
This Van Kampen property, specifies a well-behaved interplay of pullbacks and pushouts and is formally defined as follows:
A pushout square $D \leftarrow B \leftarrow A \rightarrow C \rightarrow D$ (1.) is said to have the Van Kampen property iff for all commutative diagrams of the form depicted in Equation~\ref{eq:vanKampen} where (1.) is in the center it holds: (2.) and (3.) are pullback squares imply (4.) and (5.) are pullback squares iff. the outer square $D' \leftarrow B' \leftarrow A' \rightarrow C' \rightarrow D'$ is a pushout.
\begin{equation}
\label{eq:vanKampen}
\xymatrix{
A' \ar[rrr] \ar[ddd] \ar[dr] \ar@{}[drrr]|{(2.)} \ar@{}[dddr]|{(3.)} & & & B' \ar[ddd] \ar[dl] \\
& A \ar[r] \ar[d] \ar@{}[dr]|{(1.)} & B \ar[d] & \\
& C \ar[r] & D & \\
C' \ar[rrr] \ar[ur] \ar@{}[urrr]|{(4.)} & & & D' \ar[ul] \ar@{}[uuul]|{(5.)}
}
\end{equation}
Finally, the Van-Kampen is not only relevant for DPO rewriting, it has also been discovered to be required for the \emph{amalgamation}-condition for fibered semantics \cite{WolterKoenig2015}.

\endinput %  the piece below went into Background
Thus, it is important to recall that every presheaf topos $\catSet^\cat{B}$ is adhesive and adhesiveness is closed under the ``operations'' product-,slice, coslice- and functor-category \cite{LackSobocinski2004}.

In every adhesive category the following facts hold
\mkFact{Adhesive Category Properties \cite{LackSobocinski2004}}{fact:adhesive}{ \
	
\begin{itemize}
	\item Monomorphisms are stable under pushouts.
	\item Pushouts along monomorphisms are pullbacks.
	\item Pushout complements of monos are unique up to isomorphism.
	\item Pushout can be decomposed along pullbacks.
\end{itemize}
}
These properties are required to establish the major theorems in DPO rewriting regarding Concurrency, Parallelism, Embedding and Critical Pairs of productions, for details see \cite{EhrigEhrigPT2006}.
Critical Pairs are important for analysis of confluence.
In general, confluence for a DPO rewriting system known to be terminating is undecidable \cite{Plump1993}.
However, when considering a variation of DPO with interfaces \cite{GaducciHeckel1998} confluence is decidable \cite{BonchiGaducciKSZ2017}.
This fact is basis for theorem proving for SMTs described in \cite{BonchiGaducciKSZ2018}.

==> sections/mathBackgrounds/mathBackgr-injectivity.tex <==
\section{Injectivity}

Injectivity is a far reaching generalization of regular logic, whose sentences are built according to the pattern $\forall \bar x (P(\bar x) \rightarrow \exists \bar y Q(\bar x, \bar y))$. Such an implication is modelled  by a \mor, and sets of variables $\bar x$ and $\bar y$ are \mor s too (the idea goes back to Banashewsky and Herrlich's work on quasi-implications and quasi-variaties in universal algebra \cite{?}). 
\begin{defN}[Injectivity (well-known, \eg,  \cite{adamek-lpaCatsBook-94})]
	Let \frar{f}{P}{Q} be an arrow in an arbitrary category \CC. An object $A\in\Ob\CC$ is {\em injective} \wrt\ $f$ if for any \mor\ \frar{x}{P}{A} there is \mor\ \frar{y}{Q}{A} such that $x=f.y$. Then we write $A\modelsInjX{\CC}f$ and interpret $A$ as a 'model of formula' $f$. We will omit one or both scripts unless we deal with different carrier categories or different $\models$-relations in the same category. 
	
	A binary relation $\models\,\subset\Ob \CC\times\Arr \CC$ gives rise to two mappings: from a set of arrows (theory) $\Fset \subset\Arr\CC$ to its class of models 
	$\InjMod(\Fset) =\compr{A\in\Ob\CC}{A\models{} f \text{ for all } f\in \Fset}$, and from a set of objects (models) \nia\ to its theory $\InjTh(\nia)=\compr{f\in\Arr\CC}{A\models f \text{ for all } A\in\nia}$. %The subscript \CC\ will be omitted if it is clear. 
	We write $\Fset\models f$ if $A\in\InjMod(\Fset)$ implies $A\models f$ for any object $A$.
	\qed\end{defN}
The 'model theory and logic' of injectivity are well studied. Closure Birkgoff-style operators for classes of objects are built by Rosicky \etal \cite{adamek-injBirkhoff-2002}. Sound and complete deductive calculi for injectivity (both finitary and infinitary)  are found by Ad{\' a}mek \etal \cite{adamek-injLogic-2007}. The calculus for finitary injectivity (when all formula-\mor s are finitary, \ie, their domains and codomains are finitely presented) is especially simple and elegant: it is  a set \dedSys\  (read it as {\em Injectivity Logic}) of the following four inference rules:
\begin{equation}\label{eq:injLogic-rules}
	\begin{tabular}[f]{cccc}
		$\dfrac{f_1,\; f_2}{f_1.f_2}$
		& $\dfrac{}{\id_A}$
		& $\dfrac{f_1.f_2}{f_1}$
		& $\dfrac{~f~}{~f'~}$ for every pushout $(g,f,g',f')$
		\\ [20pt] 
		a) {\sc Composition}
		& b) {\sc Idenity}
		& c) {\sc Cancellation}
		& d) {\sc PushOut}
		\\ &&&(validity of $g$ is not required)
	\end{tabular}
\end{equation}
%Their soundness is straightforward to check, but completeness of set \dedSys\ is very non-trivial.  
The rules give rise to an entailment relation $\Fset\vdash^\dedSys f$, whose soundness is straightforward to check: if $\Fset\vdash^\dedSys f$ then $\Fset\modelsInj{}f$.  Specifically, {\sc Coproduct} rule specified in \cref{eqdiag:coproduct-derived}(a) can be derived as shown in diagrams\cref{eqdiag:coproduct-derived}(b$_1$), (b$_2$) and (c):  % by using {\sc Pushout}
\begin{equation}\label{eqdiag:coproduct-derived}
	\begin{tabular}{c@{\qquad}c@{\qquad}c}
		$\dfrac{f_1, f_2}{f_1+f_2}$
		&    % 2nd column 
		\begin{tikzcd}
			P_1\ar[r, "f_1"] \ar[d, "\iota_{_{P_1}}" '] 
			& Q_1\ar[d, derived, "(\iota_{_{P_1}})' "]
			\\
			P_1+P_2 \ar[r, derived, "(f_1+P_2) "] & \dernode{Q_1+P_2}
		\end{tikzcd}
		& % 3rd column 
		\begin{tikzcd}
			P_1+P_2 \ar[r, "f_1+P_2"] \ar[d, "P_1+f_2" '] 
			& Q_1+P_2\ar[d, derived, "(P_1+f_2)' "]
			\\
			P_1+Q_2 \ar[r, derived, "(f_1+P_2)' "  '] 
			& Q_1+Q_2\ar[lu, {<-}, derived, "\gapnamegap{-1}{f_1+f_2}{0}" ', pos=0.35
			]
		\end{tikzcd}
		\\ [7.5pt]
		a) {\sc Coproduct} 
		&  b$_1$) apply {\sc Pushout}
		& c) apply {\sc Pushout} (twice) %derivation of the rule using {\sc Id},  {\sc Pushout}
		\\
		& b$_2$) the same  for $P_1+f_2$
		&  followed by {\sc Composition}
	\end{tabular}
\end{equation}
The system \dedSys\ is also complete: semantic entailment $\Fset\modelsInj f$ implies syntactic derivability (inference) $\Fset\vdash^\dedSys f$, which is of course much more difficult to prove \cite{adamek-injLogic-2007}. 
\zd{I guess it's not needed but let it be here for the record. If $t$ is mono, then commutativity of the lower triangle implies comm. of the upper one. If $h_\tauu$ is epi, then the converse holds.}

==> sections/mathBackgrounds/monadsInHaskellRemark.tex <==
\begin{myrem}[Local and Global Monad Notions]
Note that complex queries actually constitute a \emph{monad} $\boldsymbol{Q}$ and views $\relationarrow{V}{v}{S}$ are arrows in the Kleisli category w.r.t this monad.
However, we did not define $\boldsymbol{Q}$ in the classical way by defining it as an endofunctor on $\skecatgp$ together with the natural transformations $\drar{\eta}{\boldsymbol{1}_{\skecatgp}}{\boldsymbol{Q}}$ (unit) and $\drar{\mu}{{\boldsymbol{Q}^2}}{\boldsymbol{Q}}$  (multiplication).
Instead, we defined this monad implicitly by defining kleisli composition.
This principle is well known by Haskell programmers:
There are multiple equivalent ways to implement the typeclass \texttt{Monad} in Haskell, one can either implement the functions \texttt{fmap} (functorial lift), \texttt{unit} ($\eta$) and \texttt{join} ($\mu$) in the classical way or by implementing \texttt{unit} and \texttt{>=>}, where the latter is called the ``fish''-operator and denotes Kleisli-composition.
The definition via kleisli composition is a \emph{local} one, whereas the classical definition is \emph{global}.
The local definition avoids working with (rather big) set of all possible $\opsig$-queries over $\skecatgp$.
\end{myrem}

==> sections/notation.tex <==
%!TEX root = ../lics20.tex

\section{Background: Presheaves}

%First, let us introduce the theoretical background of this paper.
\zdhllok{In Computer science and Software Engineering context, {\em presheaf} toposes or {\em presheaves} have also been referred to as \emph{``graph-like structures''}, e.g. \cite{Loewe1993}}{lets mention this in the intro}{-10}
We assume that the reader is familiar with the fundamental concepts of category theory as they an be found in every standard textbook, e.g. \cite{BarrWells1990}. Our notation for basic categorical notions can be found in Appendix \sectref{notation}.  
 

\subsection{Categories} The goal is to fix our notation and terminology. To manage size issues, we consider all categories in the paper are small... \zd{check at nLab about Grothendieck universe.}
For variables referring to categories, we use blackboard font, e.g. $\cat{G}$. Names of special categories such as $\catSet$ or $\catCat$ are in bold italic. 

\subsubsection{Notation for objects and arrows}
The class of all objects in a category $\cat{C}$ will be referred to by $\catObj{\cat{C}}$ and class of all arrows (we will use the terms morphism and arrow interchangeably) $\catArrows{\cat{C}}$.
As a rule, for objects  we will use uppercase letters, e.g. $X \in \catObj{\cat{C}}$ and for morphisms we will use lowercase letters, e.g. $f \in \catArrows{\cat{C}}$.
In typical abuse of notation, we will usually denote memberships of objects and arrows in a specific category by simply writing $X\in \cat{C}$ or $f \in \cat{C}$.
The domain of an arrow $f$ will be denoted by $dom(f)$ and the codomain by $cod(f)$ (one may as well think of $dom$ and $cod$ as mappings from $\catArrows{\cat{C}}$ to $\catObj{\cat{C}}$).
Sometime we use an integrated arrow notation: $\arrow{X}{f}{Y}$ ($\inlinearrow{X}{f}{Y}$ in diagrams) for an arrow $f \in \catArrows{\cat{C}}$ with $dom(f) = X$ and $cod(f)=Y$.
The hom-set of all arrows between two objects $X,Y \in \catObj{\cat{C}}$ will be denoted $\homset{\cat{C}}{X}{Y}$.

We write $\CC(X,\_)$ for $\bigcup_{Y\inn\Ob{\CC}}\CC(X,Y)$ and similarly for $\CC(\_,Y)$.
\subsubsection{Arrow composition and application}
Composition of two arrows $\arrow{X}{f}{Y}$ and $\arrow{Y}{g}{Z}$ will be denoted either in the diagrammatic order $\arrow{X}{\compose{f}{g}}{Z}$ or the application order $\arrow{X}{\altCompose{f}{g}}{Z}$.

For a mapping \frar{f}{X}{B^A} and $x\inn X$, we will often write $f_x$ rather than $f(x)$ to make reading  applications of $f(x)$ to elements of $A$ easier:  $f_x(a)$ rather than $f(x)(a)$ (although the latter form will be used too).

To highlight special properties of morphisms, we denote a monomorphism $m$ by $\monoarrow{X}{m}{Y}$ and an epimorphism $e$ by $\epiarrow{X}{e}{Y}$
% \zd{I'd prefer $X\rCover Y$}.
Finally, we will interchangeably use expressions $\cat{C}^\cat{D}$ or $[\cat{C},\cat{D}]$ to denote the functor category between $\cat{C}$ and $\cat{D}$, $\sliceCat{\cat{C}}{X}$ for the slice category under $X \in \catObj{\cat{C}}$, $\cosliceCat{\cat{C}}{C}$ for the coslice category over $X \in \catObj{\cat{C}}$, and $\cat{C} \times \cat{D}$ for the product category.
%}
%\end{myremark}
\subsubsection{Carriers \zd{new piece}}

\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figures/BasicUniverse}
\caption{Semantical Universes: Overview}
\label{fig;semanticalUniverses}
\end{figure}

{
	\renewcommand\pmb[1]{#1} % juts for this piece
	In some contexts, where the domain of a mapping gives the name of the story, we will use the following (categorically, rather odd) naming for components of an arrow \frar{f}{X}{Y}. We will consider this arrow as a pair $\pmb{X}=(\carr{\pmb{X}}, f_X)$ where the domain of $f$ is now denoted by \carr{X} and called the {\em carrier} of $X$ while the arrow itself is denoted by $f_X$ and is referred to as the {\em mapping} of $X$. All these are fully terminological permutations as pair $X$ and arrow $f$ are the same formal construct. %stands for $X$ and is called the {\em carrier} of the pair $\pmb{X}$. 
	Moreover, by a common abuse of notation, we will overuse symbol $\pmb{X}$ to refer to the carrier \carr{\pmb{X}}, and will often omit the superscript $X$ in $f_X$.  
}

\subsection{Presheaf toposes}
%In this paper, presheaf topoi will play an important role. 
\zdhllok{There is an important difference between sets and presheaves, the latter can usually not be represented as a coproduct (sum) of its elements.}{this is to be said in the intro}{-10}

{\renewcommand{\II}{\enma{\mathcal{S}}}
\begin{mydef}{presheaf}{Presheaf}
Let $\II$ be a small category.
A functor \frar{G}{\II}{\setcat} is called an {\em \II-presheaf} or just a {\em presheaf} if \II\  is clear from the context or is not important, and the category $\setcat^\II$ of all such presheaves and their natural transformations is called a {\em presheaf topos}. \footnote{Usually presheaves are defined as contravariant functors \frar{G}{\II^{op}}{\setcat} %$\arrow{\II^{op}}{P}{\catSet}$ 
	due to their relation and importance for the Yoneda Lemma. For our applications throughout this paper,  it is more convenient to work with the covariant definition.}.

A presheaf  \frar{G}{\II}{\setcat} is called {\em finite} if all sets $G(v)$, $v\in\Ob{\II}$ are finite. 

A presheaf topos is called {\em finitary} if the schema category \II\ is finite. (Makaki says that in ref [3] in his paper 1, such toposes are called finite. 
\end{mydef} 

\mkFact{Presheaf Topos}{fact:presheafTopos}{
Any category of presheaves is a \emph{topos} and thus has 
\begin{itemize}
\item all limits and colimits,
%\item has all colimits.
\item exponents, \ie, is cartesian closed,
\item epi-mono factorizations,
\item a subobject classifier.
\end{itemize}
}

If \II\ is \Graph, then 'graphs' are nothing but ordinary directed multigraph, and if \II\ is \nfont{rGraph}, then 'graphs' are reflexive graphs. If \II\ is \PNet, 'graphs' are Petri nets (bipartite graphs of places and transitions).

Several fixed schema categories we will use are shown in \figref{shapes}. Objects and arrows in these categories are fixed and have fixed names.
% Let $G \in \cat{G}$ an object (graph) in $\cat{G}$.
\begin{figure}[b]
	\begin{tabular}{c@{\qquad}c@{\qquad}c@{\qquad}c}
		$
		\xymatrix{
			\Node  \\
			\Edge \ar@<+0.5ex>[u]^{\so} \ar@<-0.5ex>[u]_{\ta} 
		}
		$
		&
		$
		\xymatrix{
			\Node 
			\ar@<0ex>[r]^{\refl}
			&  
			\Edge 
			\ar@/^1.5pc/[l]^{\so} 
			\ar@/_1.5pc/[l]_{\ta} 
		}
		$
		&
		$
		\xymatrix{
			\Place & \Trans \\
			\Pre \ar[u]^{\so^i} \ar[ur]_(0.65){\ta^i} & \Post \ar[ul]^(0.65){\ta^o} \ar[u]_{\so^o}
		}
		$
		& 

		$
		\xymatrix @C=0.01cm {
			& & \Node & & \\
			\Edge_{(1,0)} \ar[urr]^(0.7){\so_{(1,0)}} & \Edge_{(0,1)} \ar[ur]^(0.3){\ta_{(0,1)}} & \Edge_{(1,1)} \ar@<+0.5ex>[u]^{\so} \ar@<-0.5ex>[u]_{\ta}  & \Edge_{(2,1)} \ar@<+0.5ex>[ul]_{\so^1_{(2,1)}} \ar@/_/[ul]_{\so^2_{(2,1)}} \ar@/_2pc/[ul]_{\ta_{(2,1)}}   &  \ldots 
		}
		$
		\\
		   a) \Graph 
		& b) \nfont{rGraph}
		& c) \nfont{PNet}
		& d) \nfont{HypGraph}
	\end{tabular}
	\caption{Fixed shape categories\zd{probably it'd better to give them names in sf, say, $\mathsf{N,E}$ etc}}\label{fig:shapes}
\end{figure}


 %We assume that for any presheaf \frar{G}{\II}{\catSet} we consider, classes $\abs{\II}$ and $\abs{G}\eqdef\compr{G(i)}{i\in\abs{\II}}$ are disjoint. \zd{here $\abs{\II}$ denotes the class of \II's elements -- should be placed in notation}. We will sometime use the same names for elements in $\abs{\II}$ and $\abs{G}$, which means that with a full notation, those names are to be qualified, say, $x_\II$ and $x_G$, but the subindexes are omitted.  We will also write $x\in G$ for an element $x\in\abs{G}$. %  If we use the same names for elements 

%For the remainder of the paper we will fix a category $\GG := \catSet^\II$ with $\II$ being an arbitrary but \emph{finite category}, whose objects will be called {\em 'graphs'} (often just graphs). If $\II$ is \graph, then 'graphs' are ordinary directed multigraphs, the corresponding presheaf topos is denoted by $\catGraph$. if $\II$ is equal to the following category (identities omitted): \[\xymatrix{ N &  E \ar@<-0.5ex>[l]_{s} \ar@<0.5ex>[l]^{t} }
%\]
%\mkRemark{Set thoeretical notions in Presheaves}{rem:setTheory}{

\subsection{Set-theoretical constructs in presheaf toposes}
Presheaves in many ways behave as sets and we will make use of some set-theoretic concepts throughout the paper. As we have already said, we can speak of \emph{elements} $x \in G$ meaning that there exists an object $I \in \cat{I}$ such that $x \in G(I)$.
Categorically, such a (global) element is modelled by an arrow $x: \boldsymbol{1} \to G$.

\subsubsection{Inclusions }
%Another concept are \emph{inclusions}, which are given by abstract subobjects.
Let $G$ %$G \in \cat{G}$ 
be an object in $\cat{G}$. Two monics \monorar{x}{X}{G} and \monorar{y}{Y}{G} are {\em equivalent}, $x\simeq_G y$, if  %A class of monomorphisms $M_G\subset\GG_\monoind/G$ % \inlinemonoarrow{X}{x}{G} $ 
%is called \emph{abstract subobject} of $G$ when for any two members $\monoarrow{X}{x}{G}, \monoarrow{Y}{y}{G} \in M_G$, %[\inlinemonoarrow{X}{x}{G}]$ and $ \in [\inlinemonoarrow{X}{x}{G}]$ in $[\inlinemonoarrow{X}{x}{G}]$ 
there exists an isomorphism $\arrow{X}{i}{Y}$ such that the triangle  commutes, $\compose{i}{y} = x$. An $\simeq_G$-equivalence class is called an {\em (abstract) subobject} of $G$. Thus, any monic \monorar{x}{X}{G} gives rise to a subobject [\monorar{x}{X}{G}].
%It is easy to see that if $x\simeq y$, then $\Img(x)=\Img(y)$ 
 %\monoarrow{X}{x}{G} is an element of $M_G$, we will call it a representative of the subobject and denote the latter by $[\monoarrow{X}{x}{G}]$  (thus $[\monoarrow{X}{x}{G}]=\monoarrow{Y}{y}{G})$ for any two equivalent  
 Among the members of the class $[\monorar{x}{X}{G}]$, there is a monomorphism $\monoarrow{H}{\subseteq}{G}$ whose domain $H$ consists only of elements which are also elements in $G$ 
 --- we call it {\em inclusion} and denote by $H \hookrightarrow G$. Thus, for any object $I\in \II$, we have subsetting $H(I)\subseteq G(I)$.  %$\incrar{x}{H}{G}$ 
%Thus, when working with a class of monomorphisms we will often choose this special inclusion morphism, denoted $\inlinemonoarrow{H}{}{G}$, as the representative of this class.\zd{May be rewritten shorter; I'll do it later}

\zd{the problem is that we need to prove that for any subobject $[\monorar{x}{X}{G}]$ there is an inclusion representing it. For this, we need the image factorization.}
\subsubsection{Images}
The third an final concept we are borrowing from set theory are \emph{images}.
Categorically, the are given by epi-mono factorizations.
Let $\arrow{H}{f}{G}$ be an arbitrary arrow in $\cat{G}$, because $\cat{G}$ has epi-mono factorizations $f$ is equal to the composite $\compose{e}{m}$ where $e$ is an epimorphism and $m$ is a monomorphism. 
The codomain $\image{f}$ object of $e$ (domain of $m$) is called the image and it is unique up to isomorphism, thus we can choose $m$ to be an inclusion morphism. \zd{but see my remark above!}
The situation is depicted in the following diagrams.
\[
\xymatrix{ 
	H \ar[rr]^f \ar@{->>}[dr]_{e} & & G \\
	& \image{f} \ar@{^{(}->}[ur]
}
\]
%\zd{Still I prefer $\rCover^e$ for epis, especially that here we deal with images, not epics as such (see Freyd-Scedrov)}

\subsubsection{Subobject lattices}
From the above it follows that for every object $G \in \cat{G}$, there exists a \emph{subobject lattice} denoted $\subobjlattice{G}$.
It is given by the subcategory $\subobjlattice{G} \subseteq \sliceCat{\cat{G}}{G}$ of the slice category whose objects are abstract subobjects, meets are given by pullbacks in $\cat{G}$, and joins are given by $\image{[\iota_H,\iota_K]}$ the image of the universal coproduct arrow for $H \xrightarrow{\iota_H} H+K \xleftarrow{\iota_K} K$ being the coproduct of the abstract subjects $H \in \subobjlattice{G}$ and $K \in \subobjlattice{G}$.
Furthermore, for a morphism $\arrow{H}{f}{G} \in \cat{G}$ we denote the pullback-functor (change of base) on the subject lattices of $G$ and $H$ by $\arrow{\subobjlattice{G}}{\pbfunctor{f}}{\subobjlattice{H}}$.
Note, that this functor has both a left (post-composition) adjoint $\arrow{\subobjlattice{H}}{\pbfunctorLeftAdjoint{f}}{\subobjlattice{G}}$ and a right (bundling) adjoint $\arrow{\subobjlattice{H}}{\pbfunctorRightAdjoint{f}}{\subobjlattice{G}}$.
%}
\zd{Shorter: Any topos is a regular category. Hence, we have adjunctions $\pbfunctorLeftAdjoint{f}\dashv\pbfunctor{f}\dashv\pbfunctorRightAdjoint{f}$ (see Freyd-Scedrov). For presheaf toposes, these adjunctions are given component-wise(?)}
} % END OF THE renewcommand for \II


==> sections/notationalConventions.tex <==
%We assume that the reader is familiar with the fundamental concepts of category theory as they an be found in every standard textbook, e.g. \cite{BarrWells1990}.
 
\subsection{Notation}
%\subsection{Categories} 

We fix some of our notation and terminology. To manage size issues, we consider all categories in the paper are small and refer to the idea of Grothendieck universes for handling categories whose collections of objects and morphisms are ``bigger'' than sets.
For variables referring to categories, we use blackboard font, e.g. $\cat{G}$. Names of special categories such as $\catSet$ or $\catCat$ are in bold italic. 

\subsubsection{Notation for objects and arrows.}
For a small category \CC, its set of objects and set of arrows (\mor s) will be denoted by $\catObj{\cat{C}}$ and $\catArrows{\cat{C}}$ resp. We will also write $\Elem{\CC}$ for the set $\Ob{\CC}\sqcup\Arr{\CC}$. 

As a rule, we will use uppercase letters for objects   and %, e.g. $X \in \catObj{\cat{C}}$ 
lowercase letters for \mor s; then we can use this agreement to ease formulas and write $X\in\CC$ meaning $X\in\Ob{\CC}$ and $f\in\CC$ meaning $f\in\Arr{\CC}$. %, e.g. $f \in \catArrows{\cat{C}}$.
%In typical abuse of notation, we will usually denote memberships of objects and arrows in a specific category by simply writing $X\in \cat{C}$ or $f \in \cat{C}$.
The domain of an arrow $f$ will be denoted by $dom(f)$ or sometimes \fancydom{f}, and the codomain by $cod(f)$ or \fancycod{f} (one may as well think of $dom$ and $cod$ as mappings from $\catArrows{\cat{C}}$ to $\catObj{\cat{C}}$).
We  write $\arrow{X}{f}{Y}$ (or $\inlinearrow{X}{f}{Y}$ in diagrams) for an arrow $f \in \catArrows{\cat{C}}$ with $dom(f) = X$ and $cod(f)=Y$.

The hom-set of all arrows between two objects $X,Y \in \cat{C}$ will be denoted $\homset{\cat{C}}{X}{Y}$. We write $\CC(X,\_)$ for $\bigcup_{Y\inn\Ob{\CC}}\CC(X,Y)$ and similarly for $\CC(\_,Y)$. \zddel{Normally  we assume that $\CC(X,Y)$ is the set of arrows from $X$ to $Y$, but in sect. we will have a special exception..... } 
\subsubsection{Arrow composition and application.}
Composition of two arrows $\arrow{X}{f}{Y}$ and $\arrow{Y}{g}{Z}$ will be denoted either in the diagrammatic order $\arrow{X}{\compose{f}{g}}{Z}$ or the application order $\arrow{X}{\altCompose{f}{g}}{Z}$.

For a mapping \frar{f}{X}{B^A} and $x\inn X$, we will often write $f^x$ or $f_x$  rather than $f(x)$ to make reading  applications of $f(x)$ to elements of $A$ easier:  $f^x(a)$ rather than $f(x)(a)$ (although the latter form will be used too). Similarly, if $f(x)$ is a domain of another arrow \frar{g}{f(x)}{y}, we will often write $x^f$ for $f(x)$ so that \frar{g}{x^f}{y}.

To highlight special properties of morphisms, we denote a monomorphism $m$ by $\monoarrow{X}{m}{Y}$ and an epimorphism $e$ by $\epiarrow{X}{e}{Y}$
% \zd{I'd prefer $X\rCover Y$}.
\zdzd{and we need a big talk about $\righthookarrow$ as a synonymic symbol for monic, or not synonymic? }
Finally, we will interchangeably use expressions $\cat{C}^\cat{D}$ or $[\cat{C},\cat{D}]$ to denote the functor category between $\cat{C}$ and $\cat{D}$, $\sliceCat{\cat{C}}{X}$ for the slice category under $X \in \catObj{\cat{C}}$, $\cosliceCat{\cat{C}}{X}$ for the coslice category over $X \in \catObj{\cat{C}}$, and $\cat{C} \times \cat{D}$ for the product category. Class $\Ob{[\CC,\DD]}$ will be often denoted by $[\CC,\DD]^\bullet$ or just $[\CC,\DD]$ if the context makes discretization clear. 
%}
%\end{myremark}

If \frar{f}{\CC}{\DD} is a functor and $\CC'\subset\CC$ is a subcategory, then the restriction of $f$ on $\CC'$ (\ie, composition $i_{\CC'}\comp f$ where $i_{\CC'}$ is the \corring\ embedding) is denoted by \frestr{f}{\CC'}.  
\subsubsection{Carriers.}

{
	\renewcommand\pmb[1]{#1} % juts for this piece
	In some contexts, where the domain of a mapping gives the name of the story, we will use the following (categorically, rather odd) naming for components of an arrow \frar{f}{X}{Y}. We will consider this arrow as a pair $\pmb{X}=(\carr{\pmb{X}}, f_X)$ where the domain of $f$ is now denoted by \carr{X} and called the {\em carrier} of $X$ while the arrow itself is denoted by $f_X$ and is referred to as the {\em mapping} of $X$. All these are fully terminological permutations as arrow $f$ and pair $X$ are the same formal construct. %stands for $X$ and is called the {\em carrier} of the pair $\pmb{X}$. 
	Moreover, by a common abuse of notation, we will overuse symbol $\pmb{X}$ to refer to the carrier \carr{\pmb{X}}, and will often omit the superscript $X$ in $f_X$.  
}
%\PAST{What do we need this notion carriers for? I find this a bit confusing}
\zdzd{it is confusing and that's why this piece is written. Example are everywhere in the paper, \eg, a signature \frar{\arfun}{\PP}{\GG} is referred to by \PP\ rather than \arfun.}


==> sections/piece--SEtoMversionOfTwistedMorphCompose.tex <==
% --- the SEto M section
\begin{defN}[Twisted \mor s: SE-view]\label{def:twistedMorph-SEtoM}	%MStoE
	Let  \spanrar{\modelsr}{\S\timm\E}{\M} and  \spanrar{\modelsr'} {S'\timm E} {\M'} be two eSat spans, and 
	\frar{\twip=(s,r)}{(S,M)}{(S',M')} a twisted pair as above. 
	%shown in diagram \cref{eqdiag:twistedMorph--MStoE} a)  
	Then we can form two new parallel eSat spans, 
	\spanrar{\modelsr_\twimor}{S\timm E}{\M'} and
	\spanrar{\modelsr'_\twimor}{S \timm E}{\M'}, defined by span composition as specified in diagram \cref{eqdiag:twistedMorphDef--SEtoM}a)
	
	A twisted pair \twimor\  is called a {\em (twisted) eSat \mor}, if spans $\modelsr_\twimor$ and $\modelsr'_\twimor$ are \congg-equivalent and can be identified in $\spanfuncongX{\CC}$. 	Then we write  \frar{\twimor}{\modelsr}{\modelsr'}. 
	%
	Diagram \cref{eqdiag:twistedMorphDef--SEtoM}b shows this definition unpacked in \CC. 
	%
	%	\renewcommand{\Dashv}{\vDash}
	%\begin{figure}
	\begin{equation}\label{eqdiag:twistedMorphDef--SEtoM}
		%\vsatDefTripleDiagram
		\begin{tabular}{c@{\quad}cc} % see first rows of the file for macros
			\twiMorphDefViaSpansSEtoM
			& \twiMorphDefUnpackedSEtoM
			%& \twistedMorphDefPackedMStoE
			%			& \satAxiomPackedMStoE
			&	$\begin{array}{c} % iff statement 
				m'.r \models^e \phi
				\\ [5pt]\text{iff}\rule{0ex}{1.ex}
				\\ [5pt] m' \models'^e \phi.s
			\end{array}$
			\\
			a)  &  b)  & c)
		\end{tabular}
	\end{equation}
	%i) two pullbacks specified in diagram a)  (the upper orange and the lower green) produce the same (up to iso\mor\ of its domain) arrow $p_f$ (whose domain can be seen as a twisted Sat --- this is the ``iff'' of the Sat-axiom  in \cref{eqdiag:eSatAxiom}) %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $\twip$, but we omit it.)
	%
	%ii) the rightmost square (shown triangularly) commutes  and $q_f$ denotes its diagonal (defined up to iso\mor\ of its domain  $\modelsd_\twimor$). 
	\qed\end{defN}
The two definitions of a twisted \mor\ should be equivalent, and it is indeed so per the result below, but the diagram chasing proving it turned out unexpectedly ``twisted''. 
\begin{propo}
	Two definitions of a twisted \mor, Def.\ref{def:twistedMorph} and Def. \ref{def:twistedMorph-SEtoM}, are equivalent.
\end{propo}
{\em Proof.} We first prove that for any twisted pair  $\twimor=(s,r)$, there is an iso\mor\
\frar{\switchX{\twimor}} {\modelsd_\twimor} {\modelsr_\twimor} (whose domain is the upper twisted eSat in diagram \cref{eqdiag:twistedMorphDef--MStoE}a) and the codomain is the upper twisted eSat in diagram \cref{eqdiag:twistedMorphDef--SEtoM}a) ) such that  diagram \cref{eqdiag:switchDiags-a4result-and-b4twistedPB}a) commutes. The proof is based on diagram \cref{eqdiag:switchDiags-a4result-and-b4twistedPB}b), in which span \spanrar{\modelsd}{\M\timm\S}{\E} is shown orange (with orange wiggly arc connecting the legs), and span \spanrar{\modelsd}{\S\timm\E}{\M} (with the same apex) is purple (and wiggly purple arc connecting the legs). 
\begin{equation}\label{eqdiag:switchDiags-a4result-and-b4twistedPB}
	\begin{array}{cc}
		\switchDiag
		& 		\twistedPBdiag
		\\ a) & b) 
	\end{array}
\end{equation}
Span $\modelsd_\twimor$ is built as specified in diagram \cref{eqdiag:twistedMorphDef--MStoE}b) with PB denoted [pb]$_0$ (shown orange), and now we build span $\modelsr_\twimor$ (shown purple) as specified in diagram \cref{eqdiag:twistedMorphDef--SEtoM}b). We notice that $w=\pMS.\pi_M$, and hence the PB of cospan $(r,w)$ is given by two (purple) PB squares [pb]$_1$ and [pb]$_2$ as specified in the diagram. Next we build four $!$-arrows with subscripts due to universal properties: $!_{\#1}$ is by the universality of [pb]$_1$, which allows us to obtain a unique $!_{\#2}$ by the universality of [pb]$_2$. Arrow $!_{\timm3}$ is by the universality of product $M'\timm S$, which provides a unique $!_{\#4}$ by the universality of [pb]$_0$.  Arrows $!_{\#2}$ and $!_{\#4}$ are mutually inverse by the standard argument that otherwise their  uniqueness would be violated. Thus, we have built an iso\mor\ \switchX{\twimor} from diagram a). In the same way we can build an iso\mor\  \frar{\switchPrimX{\twimor}}{\modelsd'_\twimor}{\modelsr'_\twimor}. It is now clear that $\modelsd_\twimor\cong\modelsd'_\twimor$ iff $\modelsr_\twimor\cong\modelsr'_\twimor$ so that the two definitions equivalent. \qed
%%  remark on Gogiuen 
%\begin{remark}[On the Sat-axiom]
%	If $(\CC,E)$ is $(\setcat, \tcat)$ (so that evidencing is trivial),  and eSats are binary relations over sets, then diagram b) is immediately Sat-axiom as formulated in \cref{eqdiag:satAxiom}. It was noted by Goguen and Burstall \cite{GoguenBurstall-jofacm92}
%\end{remark}
%
%
%  not needed anymore but very useful to keep
%\input{sections/piece--eSatMorDef--MtoSEversion}
%

An advantage of \cref{def:twistedMorph-SEtoM} is an easy proof of the following fundamental result. 
\begin{propo}[Twisted \mor s compose]\label{prop:twistedMorph--Compose}
	Given a composable pair of twisted pairs,  \[
	(S,M) \xrightarrow{\twimor=(s,r)} (S',M') \xrightarrow{\twimor'=(s',r')} (S'', M'') 
	\] 
	%\frar{\twimor=(r,s)}{(S,M)}{(S',M')} and  \frar{\twimor'=(r',s')}{(S',M')}{(S'',M'')}, 
	if both pairs are twisted \mor s, then the composed pair $\twimor.\twimor'=(s.s', r'.r)$ is also a twisted \mor. 
\end{propo} 
{\em Proof.} As operators \cref{eq:mor2spans} are functors, diagrams \cref{eqdiag:twistedMorphDef--SEtoM}a) for \twimor\ and $\twimor'$ can be tiled. The resulting rectangle again commutes, which means that twisted pair $\twimor.\twimor'= (s.s', r'.r)$ is a twisted \mor. \qed


==> sections/piece--aboutInstit4briefExpo.tex <==
\begin{mygroup} % redefine \Sigmaa
	An {\em institution} is a functor \frar{\logfun}{\signcat}{\logsyscat} from a small category \signcat\ whose objects are called {\em signatures} (think, \eg, of a signature of operation and relation symbols) to a \caty\ of {\em logical systems}, whose objects are binary {\em satisfiability} relations $\vDash\subset \ModsetX{} \timm \SensetX{}$. A {\em \mor} of logical systems \frar{f}{L'}{L} is a pair of functions $(f^*, f_*)$ specified in diagram \cref{eqdiag:satisfyAxiom}a) such that for all $m\in\Modsetsig$ and all $\phi'\in\SensetsigPrim$, the {\em twisted satisfiability} condition specified in \cref{eqdiag:satisfyAxiom}b) holds. 
	\vspace{-1em}
	\input{diagrams/satAxiom}
	\noindent 
	%where diagram \cref{eqdiag:satisfyAxiom}a) shows directions of functions $f^*=\ModsetX{}(f)$ and $f_*=\SensetX{}(f)$ (note the reversal of arrow for $f^*$). 
	The rightmost diagram (ignore for a moment three dashed arrows and their targets) expresses this condition diagrammatically as the existence of jointly monic span {\modelsFtwisted} (its legs are diagonals), which is embedded into both (jointly monic) satisfiability spans so that the diagram commutes. 
	%
	It is this diagram, which is a basis for  much of the \instfwk\ theory and applications. 
\end{mygroup}
% \prodnodeS, \prodnodeSprim, \prodnodeFtwist\, 
% \underprodS, \underprodSprim, \underprodFtwist


==> sections/piece--eSatDef--noProd.tex <==
%\input{diagrams/satAxiom-abstract}
				%\input{diagrams/vsatDefnoProd--macros} -- went into the upper section 
\input{diagrams/esatDefwithProd--macros}

\begin{defN}[Sat-base]\label{def:satBase}
	A {\em (logical) %verified institution 
		base} is a quadruple  $(\CC, \CC_\senind, \CC_\modind, E)$ of a \caty\ \CC\ with pullbacks (CPB) , two its sub\caties\ (not necessarily disjoint) $\CC_\senind$ and $\CC_\modind$ closed under iso\mor s, whose objects are thought of as collections of {\em sentences} and {\em models} resp., and an  object  $E\in \Ob\CC$ thought of as a collection of {\em pieces of evidence}.  We will write $(\CC,E)$ for a base with $\CC_\senind=\CC =\CC_\modind$; such a base is a just a pointed \caty. % (or to shorten notation if the subcategoires are not under discussion). 
	%To ease notation, we will often refer to such a base as to a pointed \caty\ $(\CC, E)$, and 
	We denote objects of $\CC_\modind$ and $\CC_\senind$ by $M, M', ..$ and $S, S',...$  resp. and omit explicit mentioning of \caties\ they belong.  
	
	Some of the constructs below can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcat_\CC$ if \CC\ has such. We will provide these interpretation prefixed  with phrasing `with products' or `with elements'. (Recall that pullbacks and the terminal object provide all finite limits, \ie, make \CC\ an FCC.)
\end{defN}
\begin{defN}[ESats: Sat-spans with evidence]\label{def:esatSpan}
A {\em  \satty\ span with evidence} ({\em eSat})  over base \satbaseXY{\CC}{E} is a ternary span, \ie, a triple of arrows $(p_S, p_M, p_E) \in \CC_\senind\timm\CC_\modind\timm \CC/E$ with a common source $\Dashv$ and a triple of targets $S$, $M$, $E$, resp.  With products, it can be written as a  binary span  
$\S\timm\M\xleftarrow{(p_S,p_M)}\;\Dashv\;\xrightarrow{p_E}\E$ or 
\spanrar{\Dashv}{\S\timm\M}{\E} (\ie, we denote the spans and its apex by the same symbol). If objects $S$ and $M$ in a diagram are placed with $S$ on the right of  $M$, or vertically, we will denote the same data (\ie, $p_S$ points to $S$ and $p_M$ to $M$) by using more customary symbol $\vDash$ rather than $\Dashv$. 
The binary subspan $(p_S, p_M)$  will be denoted by \spanrar{\Dashv_{SM}}{S}{M} or  \spanlar{\vDash_{MS}}{M}{S} %$\vDash_{MS}$ but directed as \spanlar{\vDash_{MS}}{M}{S}. 

With elements, if a triple of elements \frar{(m,s,e)}{\tcat}{\M\timm\S\timm\E} factors through $\vDash$, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $s$  as {evidenced} by a {\em (piece of) evidence} $e$ 
%{\em verified assurance of level} $e$,  
and write $m\satUD{e}{}s$.  

We require \satty\ to be invariant under iso\mor s: for any iso\mor s \frar{i_X}{X}{X}, 
where $X\in\{\S, \M, \E\}$ (in the corresponding \caty), there is a \CC-iso\mor\ \frar{i}{\vDash}{\vDash} such that $p_X.i_X =i.p_X$ with $X\in \{S, M, E\}$.  %and $e.i_\E=i.e$. \qquad \qquad \qquad.  
\end{defN}
\begin{defN}[Twisted \mor s of VSats]\label{def:twistedMorph}
A {\em (twisted) \mor} of VSats %over base $(\CC,\E)$, 
\frar{f}{\vDash}{\vDash'},  is a pair of \mor s, \frar{f_*}{S}{S'}  in $\CC_\senind$ and \frar{f^*}{M'}{M} in $\CC_\modind$, as specified in diagram \cref{eqdiag:twistedSpans}a) such that the following two conditions i) and ii) hold: 
\begin{mygroup}
	\renewcommand{\Dashv}{\vDash}
	\renewcommand{\twix}[1]{\twixU{#1}}
	\begin{equation}\label{eqdiag:twistedSpans}
		%\vsatDefTripleDiagram
		\begin{tabular}{ccc}
			\twistedMorphDefMain 
			& \satAxiomPacked
			& \twistedMorphDefPacked
			\\
			a)  &  b) & c)
		\end{tabular}
	\end{equation}
\end{mygroup}

\noindent i) The two pullbacks (the upper (orange) and the lower (green)) produce the same (up to iso\mor) object denoted $\twixU{\vDash}_f$ (this is the Sat-axiom's ``iff'') %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $f$, but we omit it.)

ii) The rightmost arrow  square (shaped triangularly) commutes (up to iso) and arrow $p_E^f$ (defined up to iso)  denotes its diagonal. 

The definition above above is {\em weak} in the sense that conditions i-ii) are properties that define a structure up to iso\mor. We can give a slightly stronger {\em strict} formulation that defines a twisted \mor\ as a triple $f=(f^*, f_*, \twixU{\vDash}_f)$, where the third component is a pentuple of arrows with a common source such that the two corresponding squares are pullbacks, and the two triangles commute. %  squares.span $(\liftedX{f^*}, \liftedX{f_*})$ making 
\end{defN}
\begin{propo}[Sat-axiom as commutativity]\label{prop:satAxiom-asCommut}

a) Condition i) above is equivalent to commutativity of diagram \cref{eqdiag:twistedSpans}b) in \spanfunX{\CC} (where triangles shown in grey are not part of the diagram: they recall the definitions of functors \cref{eq:mor2spans}). 

b) If \CC\ has products, then a pair $f=(f^*, f_*)$ is a twisted \mor\ iff diagram c) commutes. 
\end{propo}
{\em Proof.} Unpack the definition of span composition. %Diagram chasing with pullbacks. 
\begin{remark}[On the Sat-axiom]
a) If $(\CC,E)$ is $(\setcat, \tcat)$ (so that evidencing is trivial),  and eSats are binary relations over sets, then diagram b) is immediately Sat-axiom as formulated in \cref{eqdiag:satAxiom}. It was noted by Goguen and Burstall \cite{GoguenBurstall-jofacm92}

b) Two conditions i-ii) for twisted \mor\ imply the Sat-axiom but not the converse: we can probably construct a \CC-case where Sat-axiom i) holds but commutativity ii) fails. We consider such cases as violating the triviality of the Sat-axiom. 
\end{remark}


==> sections/piece--eSatDef--withProd.tex <==
%\input{diagrams/satAxiom-abstract}
			%\input{diagrams/esatDefnoProd--macros}


%\input{diagrams/esatDefwithProd--macros}

\begin{defN}[Sat-base]\label{def:satBase}
	A {\em (logical) %verified institution 
		base} is a quadruple  $(\CC, \CC_\senind, \CC_\modind, E)$ of a finitely complete \caty\ (FCC)  \CC, two its FCC sub\caties\ (not necessarily disjoint) $\CC_\senind$ and $\CC_\modind$ closed under iso\mor s, whose objects are thought of as collections of {\em sentences} and {\em models} resp., and an  object  $E\in \Ob\CC$ thought of as a collection of {\em pieces of evidence}.  We will write $(\CC,E)$ for a base with $\CC_\senind=\CC =\CC_\modind$; such a base is just a pointed \caty. % (or to shorten notation if the subcategoires are not under discussion). 
	%To ease notation, we will often refer to such a base as to a pointed \caty\ $(\CC, E)$, and 
	We denote objects of $\CC_\modind$ and $\CC_\senind$ by $M, M', ..$ and $S, S',...$  resp. and omit explicit mentioning of \caties\ they belong.  
\end{defN}
%	The FCC \fwk\ is actually not needed for our work below: having pullbacks would be sufficient. However, some of the constructs below can be written more compactly if \CC\ has products, and can usefully be illustrated with elements, \ie, mappings from a terminal object $\tcat_\CC$. Moreover, in this paper we only need the abstract \fwk\ for clarifying what we will later do with institutions in \catcat, which is FCC. %We will provide these interpretation prefixed  with phrasing `with products' or `with elements'. (Recall that pullbacks and the terminal object provide all finite limits, \ie, make \CC\ an FCC.)
\begin{defN}[ESats: Sat-spans with evidence]\label{def:esatSpan}
A {\em  \satty\ span with evidence} ({\em eSat})  over base \satbaseXY{\CC}{E} is a ternary span, \ie, a triple of arrows $(p_S, p_M, q) \in \CC_\senind\timm\CC_\modind\timm \CC/E$ with a common source $\Dashv$ and a triple of targets $S$, $M$, $E$, resp.  With products, it can be written as a  binary span  
$\S\timm\M\xleftarrow{p}\;\Dashv\;\xrightarrow{q}\E$ or 
\spanrar{\Dashv}{\S\timm\M}{\E} (\ie, we denote the spans and its apex by the same symbol). If objects $S$ and $M$ in a diagram are placed with $S$ on the right of  $M$, we will denote the same data (\ie, $p_S$ points to $S$ and $p_M$ to $M$) by using more customary symbol $\vDash$ rather than $\Dashv$. 
The binary subspan $(p_S, p_M)$  will be denoted by \spanrar{\Dashv_{SM}}{S}{M} or  \spanlar{\vDash_{MS}}{M}{S} (but note that the arrow goes from $S$ to $M$ in both cases). %$\vDash_{MS}$ but directed as \spanlar{\vDash_{MS}}{M}{S}. 

If a triple of elements \frar{(m,s,e)}{\tcat}{\M\timm\S\timm\E} factors through $\vDash$, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $s$  as {evidenced} by a {\em (piece of) evidence} $e$ 
%{\em verified assurance of level} $e$,  
and write $m\satUD{e}{}s$.  

We require \satty\ to be invariant under iso\mor s: for any iso\mor s \frar{i_X}{X}{X}, 
where $X\in\{\S, \M, \E\}$ (in the corresponding \caty), there is a \CC-iso\mor\ \frar{i}{\vDash}{\vDash} such that $p_X.i_X =i.p_X$ with $X\in \{S, M, E\}$.  %and $e.i_\E=i.e$. \qquad \qquad \qquad.  
\end{defN}
\begin{defN}[Twisted \mor s of eSats]\label{def:twistedMorph}	
A {\em twisted pair (of arrows)} is a pair $f=(f_*, f^*)$ of \mor s \frar{f_*}{S}{S'} in $\CC_\senind$ and  \frar{f^*}{M'}{M} in $\CC_\modind$, written as \frar{f}{(S,M}{(S',M')}. Such pairs form category $\twixD{\CC}:=\CC_\senind\times\opX{\CC_\modind}$. 
 
Given eSats \spanrar{\Dashv}{S\timm M}{E} and \spanrar{\Dashv'}{S'\timm M'}{E}, their {\em (twisted) \mor} %over base $(\CC,\E)$, \frar{f}{\Dashv}{\Dashv'},  
is a twisted pair \frar{f=(f^*, f_*)}{(S,M}{(S',M')} 
such that the following two conditions i) and ii) hold (see diagram \cref{figdiag:twistedSpans}a) where  $P$, $P'$, and  \twixU{P} denote products, the latter one  is twisted)) %,  and arrows $!^*_f$ and $!_*^F$ are due to products' universality), 
% 
\begin{mygroup}
%	\renewcommand{\Dashv}{\vDash}
	\renewcommand{\twix}[1]{\twixU{#1}}
\begin{figure}
\begin{equation*}\label{eqdiag:twistedSpans}
		%\vsatDefTripleDiagram
	\begin{tabular}{c@{}cc} % see first rows of the file for macros
		\twistedMorphDefMain 
		& \twistedMorphDefPacked
		& \satAxiomPacked
			\\
		a)  &  b) & c)
	\end{tabular}
\end{equation*}
\caption{For \cref{def:twistedMorph} of twisted \mor s between eSats\label{figdiag:twistedSpans}}
\end{figure}
\end{mygroup}
i) Two pullbacks (the upper (orange) and the lower (green)) produce the same (up to iso\mor) object denoted $\twixU{\Dashv}_f$ (this is the Sat-axiom's ``iff'') %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $f$, but we omit it.)

b) The rightmost arrow  square (shaped triangularly) commutes (up to iso) and arrow $q_f$ (defined up to iso)  denotes its diagonal. 

The definition above above is {\em weak} in the sense that conditions i-ii) are properties that define a structure up to iso\mor. We can give an equivalent {\em strict} formulation that defines a twisted \mor\ as a triple $f=(f^*, f_*, \twixU{\Dashv}_f)$, where the third component is a quadruple of arrows with a common source such that the two corresponding squares are pullbacks, and the two triangles commute. %  squares.span $(\liftedX{f^*}, \liftedX{f_*})$ making 
\end{defN}
\begin{propo}[Sat-axiom as commutativity]\label{prop:satAxiom-asCommut}
A twisted pair $(f^*, f_*)$ is a twisted \mor\ of eSats  iff diagram b) in \cref{figdiag:twistedSpans} commutes. 
Moreover, condition i) is equivalent to commutativity of diagram \cref{eqdiag:twistedSpans}c) in \spanfunX{\CC}, where triangles shown in grey are not part of the diagram: they recall the definitions of functors \cref{eq:mor2spans}. (To be accurate, we should use the lower star operator in diagram b) too, but we omitted it to ease notation.) 
\end{propo}
{\em Proof.} Unpack the definition of span composition. %Diagram chasing with pullbacks. 



==> sections/piece--eSatDef--withProdNew.tex <==
%\input{diagrams/satAxiom-abstract}
			%\input{diagrams/esatDefnoProd--macros}


%\input{diagrams/esatDefwithProd--macros}

\begin{defN}[Sat-base]\label{def:satBase}
	A {\em  %verified institution 
		base} is a triple  $(\CC, \CCmod, \CCsen^\e)$ of  of a finitely complete \caty\ (FCC)  \CC,
		its sub\caty\ $\CCmod\subset\CC$  of {\em collections of models} (think of \caties\ \Modcat\ above), and an {\em assurance} structure $\CCsen^e=(L, \CCsen, \ellE)$, where $L\in\Ob\CC$ is an object  of {\em levels} (of required evidence), $\CCsen\subset \CC/L$ is a \caty\ of{\em collections of labelled sentences}, and an arrow $E\xrightarrow{\ellX{\E}}L\; \in\CC/L$ provides an object $\E$ of {\em (labelled) pieces of evidences}. We will write an object of \CCsen\ as a pair  $(S, \ell_S)$, in which \ellX{S} is to be thought of as a mapping providing logical sentences with their required levels of assurance; then a \mor\ in $\CC/L$, \ie, a commuting triangle $f.\ell'=\ell$, is written as \frar{f}{S}{S'}. Similarly, arrow \ellE\ will be referred to by \E. 
		
		  We will write $(\CC,L,E)$ for a base with $\CCmod=\CC$ and $\CCsen=\CC/L$ (and arrow  \ellE\ is assumed by default). 
		  %; such a base is just a pointed arrow  \caty\ $(\arrowcatCC,\ellE)$. % (or to shorten notation if the subcategoires are not under discussion). 
	%To ease notation, we will often refer to such a base as to a pointed \caty\ $(\CC, L)$, and 
	We denote objects of $\CCmod$ and $\CCsen$ by $M, M', ..$ and $S, S',...$ resp.   (labelling arrows \ellX{S}, \ellX{S'} etc are assumed by default) and omit explicit mentioning of \caties\ they belong.  
\end{defN}
\begin{example}
	The institution theory is developed over the base $(\Catcat, \tcat, \tcat)$ with $\ellE=\id_\tcat$.  
\end{example}

\begin{defN}[eSats: Sat-spans with evidence]\label{def:esatSpan}
Recall that any slice \caty\ has products defined by pullbacks, and let $S\timm_L \E$ be such for a sentence object $S\in\Ob\CCsen$. 

A {\em  \satty\ span with evidence} ({\em eSat})  over base \satbaseX{\CC}  is a span 
$M\xleftarrow{p}\;\vDash\;\xrightarrow{q}S\timm_L \E$ or 
\spanrar{\Dashv}{\S\timm_L \E}{\M} (\ie, we denote the spans and its apex by the same symbol). 
%  not needed now!
If objects $S$ and $M$ in a diagram are placed with $S$ on the right of  $M$, we will denote the same data (\ie, $q$ points to $S\timm_L\, \E$ and $p$ to $M$) by using more customary symbol $\vDash$ rather than $\Dashv$ (but note that the span-as-arrow goes into $M$ in both cases). %$\vDash_{MS}$ but directed as \spanlar{\vDash_{MS}}{M}{S}. 

If a triple of elements \frar{(m,s,e)}{\tcat}{\M\timm\S\timm\E} factors through $\vDash$, then we say that  {\em model} $m$ satisfies {\em sentence} (or {\em specification}) $s$  as {evidenced} by a {\em (piece of) evidence} $e$ 
%{\em verified assurance of level} $e$,  
and write $m\satUD{e}{}s$.  

We require e-\satty\ to be invariant under iso\mor s: for any iso\mor s \frar{i_X}{X}{X}, 
where $X\in\{\M, \S, \E\}$ (in the corresponding \caty), there is a \CC-iso\mor\ \frar{i}{\vDash}{\vDash} such that $p_X.i_X =i.p_X$ with $X\in \{M, S, E\}$.  %and $e.i_\L=i.e$. \qquad \qquad \qquad.  
\end{defN}
\begin{defN}[Twisted \mor s of eSats]\label{def:twistedMorph}	
A {\em twisted pair (of arrows)} is a pair $f=(f_*, f^*)$ of \mor s \frar{f_*}{S}{S'} in $\CCsen$ and  \frar{f^*}{M'}{M} in $\CCmod$, written as \frar{f}{(S,M)}{(S',M')}. Such pairs form category $\twixD{\CC}:=\CC_\senind\times\opX{\CC_\modind}$. 
 
Given eSats \spanrar{\Dashv}{S\timm_L\,\E}{M} and \spanrar{\Dashv'}{S'\timm_L\,\E}{M'}, their {\em (twisted) \mor} %over base $(\CC,\L)$, \frar{f}{\Dashv}{\Dashv'},  
is a twisted pair \frar{f=(f^*, f_*)}{(S,M)}{(S',M')} 
such that the following condition holds: %where  $P$, $P'$, and  \twixU{P} denote products, the latter one  is twisted)) %,  and arrows $!^*_f$ and $!_*^F$ are due to products' universality), 
%
two pullbacks specified in diagram \cref{eqdiag:twistedSpans}a)  (the upper-left (orange) and the lower-right (green)) produce the same (up to iso\mor) object denoted $\twixU{\Dashv}_f$ (this is the ``iff'' of the eSat-axiom  in \cref{eqdiag:eSatAxiom}) %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $f$, but we omit it.)
\begin{mygroup}
	%	\renewcommand{\Dashv}{\vDash}
	\renewcommand{\twix}[1]{\twixU{#1}}
%\begin{figure}
	\begin{equation}\label{eqdiag:twistedSpans}
		%\vsatDefTripleDiagram
		\begin{tabular}{c@{\quad}c} % see first rows of the file for macros
			\twistedMorphDefMain 
			& \twistedMorphDefPacked
			%		& \satAxiomPacked
			\\
			a)  &  b)  %& c)
		\end{tabular}
	\end{equation}
%\caption{For \cref{def:twistedMorph} of twisted \mor s between eSats\label{figdiag:twistedSpans}}
%\end{figure}
%\end{mygroup}
\end{mygroup}
%The definition above above is {\em weak} in the sense that conditions i-ii) are properties that define a structure up to iso\mor. 
The definition above defined a \mor\ as a twisted pair possessing some property. 
We can give an equivalent but constructive {\em strict} formulation that defines a twisted \mor\ as a triple $f=(f^*, f_*, \twixU{\Dashv}_f)$, where the third component is a quadruple of arrows with a common source (as specifed in the diagram above) such that the two corresponding squares are pullbacks. 
\end{defN}
\begin{propo}[Sat-axiom as commutativity]\label{prop:satAxiom-asCommut}
A twisted pair $(f^*, f_*)$ is a twisted \mor\ of eSats  iff diagram \cref{eqdiag:twistedSpans}b) 
commutes (up to span iso\mor). The counterpart of the strict definition of a twisted \mor\ is a specified diagonal span such that both triangles commute. 
\end{propo}
{\em Proof.} Unpack the definition of span composition. %Diagram chasing with pullbacks. 


==> sections/piece--eSatMorDef--MtoSEversion.tex <==


%
%  -- SUBSECTION FOR THE M to S x E 
%
\begin{defN}[Twisted \mor s of eSats: version MtoSE]\label{def:twistedMorph}	 % MtoSE
	Given eSats \spanrar{\Dashv}{S\timm\E}{M} and \spanrar{\Dashv'}{S'\timm\E}{M'}
	their {\em (twisted) \mor} %over base $(\CC,\L)$, \frar{\twip}{\Dashv}{\Dashv'},  
	is a twisted pair \frar{\twip=(r, s)}{(S,M)}{(S',M')} 
	such that the following condition holds: %where  $P$, $P'$, and  \twixU{P} denote products, the latter one  is twisted)) %,  and arrows $!^*_f$ and $!_*^F$ are due to products' universality), 
	%
	two pullbacks specified in diagram \cref{eqdiag:twistedSpans}a)  (the upper-left (orange) and the lower-right (green)) produce the same (up to iso\mor) object denoted $\twixU{\Dashv}_f$ (this is the ``iff'' of the eSat-axiom  in \cref{eqdiag:eSatAxiom}) %(Actually arrows $!$, $\satToSat$ and their prime counterparts should also be subscripted with $\twip$, but we omit it.)
	%	\renewcommand{\Dashv}{\vDash}
	\renewcommand{\twix}[1]{\twixU{#1}}
	\renewcommand{\id}{\enma{\mathsf{id}}}
	%\begin{figure}
	\begin{equation}\label{eqdiag:twistedSpans}
		%\vsatDefTripleDiagram
		\begin{tabular}{c@{\quad}c} % see first rows of the file for macros
			\twistedMorphDefMtoSE 
			& \twistedMorphDefPackedMtoSE
			%%		& \satAxiomPacked
			\\
			a)  &  b) % & c)
		\end{tabular}
	\end{equation}
	%\caption{For \cref{def:twistedMorph} of twisted \mor s between eSats\label{figdiag:twistedSpans}}
	%\end{figure}
	%\end{mygroup}
	%The definition above above is {\em weak} in the sense that conditions i-ii) are properties that define a structure up to iso\mor. 
	The definition above defined a \mor\ as a twisted pair possessing some property. 
	We can give an equivalent but constructive {\em strict} formulation that defines a twisted \mor\ as a triple $\twip=(r, s, \twixU{\Dashv}_f)$, where the third component is a quadruple of arrows with a common source (as specifed in the diagram above) such that the two corresponding squares are pullbacks. 
\end{defN}
\begin{propo}[eSat-axiom as commutativity]\label{prop:satAxiom-asCommut}
	A twisted pair $(r, s)$ is a twisted \mor\ of eSats  iff diagram \cref{eqdiag:twistedSpans}b) 
	commutes (up to span iso\mor). The counterpart of the strict definition of a twisted \mor\ is a specified diagonal span such that both triangles commute. 
\end{propo}
{\em Proof.} Unpack the definition of span composition. %Diagram chasing with pullbacks. 
%
\begin{propo}[Equivalence] Two definitions of a twisted \mor\ are equivalent. 
	
\end{propo}



==> sections/piece--indexing4institutions.tex <==
Discussion of indexing in \cref{sec:ske4systems} motivates the following. %necessity to define an indexed version of the institution concept. 
\begin{defN}[Indexing v-institutions]\label{def:indexedInstitutions}
	Let \frar{\vsatfun}{\signcat}{\VSatcatX{\CC,V}} be a v-institution over $(\CC,V)$. Its {\em indexing} is given by 
	a pair functors %providing indexing projections:
	%two \signcat-indexed choices of indexing projections: for any $\Sigmaa\in\signcat$, there are \CC-arrows  
	\frar{\pii_S}{\signcat}{\CC^\twocat} with $\pii_S.\cod=\vsatfun.\senfun$ and 
	\frar{\pii_M}{\signcat}{\opX{(\CC^\twocat)}} with $\pii_M.\cod=\vsatfun.\modfun$ (\ie, for each signature \Sigmaa, there are indexing projections for \Sensetsig\ and \Modsetsig). 
	\qed\end{defN}
We need to build the corresponding VS-span for indexes, which is our real interest in system design. % applications. 
\begin{constrN}[Indexed VS-spans]\label{constr:liftingVSat}
	Let \spanrar{\vDash_\V=(u,v)}{\M\timm\S}{\V} be a VS-span over $(\CC, V)$. Let \frar{\pii_M}{\ovr{M}}{M}, \frar{\pii_S}{\ovr{S}}{S} be two \CC-arrows understood as model and  sentence objects indexing as discussed in \cref{sec:intro}. Then we can pullback $u$ along \frar{(\pii_M, \pii_S)}{\ovr{M}\timm\ovr{S}}{M\timm S} and get a {\em lifted} (or {\em indexed}) VS-span \spanrar{(\ovr{u},\ovr{v}}{\ovr{M}\timm\ovr{S}}{V} for model and sentence indexes. (Thinking elementwise, given a pair of indexes \frar{(\bar i, \bar j)}{\tcat}{\ovr{M}\timm\ovr{S}}, we define $\ovr{i}\; \ovr{\satrelsymbol_v}\; \ovr{j}$ iff 
	$\ovr{i}.\pii_M\satrelsymbol_v\ovr{j}.\pii_S$.) A routine diagram chasing shows that lifting works for VSat-\mor s, and actually we can define the category of lifted VSats by the following pullback diagram in \Catcat\ (recall that fibrations are stable under pullbacks):
	\input{diagrams/liftingVSat}
	%\qed
\end{constrN}
\begin{corol}
	It is easy to see that Def. \ref{def:indexedInstitutions} gives us commutative square $\vsatfun.(\modfun, \senfun) = (\pii_M, \pii_S).\cod\timm\cod$ and hence a unique functor
	\frar{\vsatfunLifted}{\signcat}{\VSatcatLiftedX{\CC, \id_V}} (see diagram \cref{eqdiag:lifitngVSats}) that does the job.
\end{corol} 
%Composition 
%\opX{\CC}, \VSatcat, \VSatcatX{Hru}, \VSatcatLiftedX{Hru}

==> sections/piece--institution-as-4tuple.tex <==
An {\em institution} is given by i) a small category \signcat\ of {\em signatures} (think, \eg, of a signature of operation and relation symbols), ii) functors \frar{\senfunX{}}{\signcat}{{\setcat}} and  \frar{\modfunX{}}{\signcat}{\opX{\Setcat}} giving each signature $\Sigmaa\in\Ob\signcat$ its set of logical sentences and models, and a family of  binary {\em satisfaction} relations $\models_{\Sigmaa}\subset \modfunsig\times\senfunsig$ such that for any signature \mor\ $f$ and all $m\in\modfunsig$, $\phi\in\senfunsigPrim$, the {\em twisted satisfiability condition} specified in \cref{eqdiag:satisfyAxiom}b) holds. 
\vspace{-1em}
\input{diagrams/satisfyAxiom}
\noindent where diagram \cref{eqdiag:satisfyAxiom}a) shows directions of functions $f^*=\modfunX{}(f)$ and $f_*=\senfunX{}(f)$ (note the reversal of arrow for $f^*$). The rightmost diagram (ignore for while two dashed arrows and their target) expresses this condition diagrammatically as the existence of jointly monic span {\modelsFtwisted} embedded into both (jointly monic) satisfiability spans so that the diagram commutes. It is this diagram is a basis for  much of the \instfwk\ theory and applications. 


==> sections/piece--realSysFunctions.tex <==
\begin{equation}
	\begin{array}{cc}
		\begin{array}{r@{\;}l@{\quad}l}
			\sysverfun{:}&\frarxy{\Modset\timm\Senset\timm\Verset}{\{0,1\}}
			\\
			{\syssenfun}{:}& \frarxy{\sysReqset}{\Senset}
			\\
			{\sysmodfun}{:}& \frarxy{\sysInstset} {\Modset}
			\\
			\syssatfun{:} & \frarxy{\sysVerset}{\Modset\timm\Senset}
		\end{array}
		&
		%	\begin{tikzcd}[row sep=4ex, column sep=3ex] %, ampersand replacement = \&] 
			%	\funnamesig{LogTime}\timm\funnamesig{Req}\timm\funnamesig{Exp}
			%		\ar[d, "\text{(\funnamesig{inst},\,\funnamesig{constr},\, \funnamesig{opn})}" ']
			%		\ar[drr,"\modelssig^{\#}"]
			%		\\
			%		\Modfunsig\timm\Senfunsig\timm\funnamesig{ExpOpn}\ar[rr,"\modelssig" '] && \{0,1\}
			%	\end{tikzcd}
		%\\
		%\text{a)} & \text{b)}
	\end{array}
\end{equation}
% 


==> sections/piece-lax-general-story-v1.tex <==
% version 1 of the piece
\zd{version 1 of the story}
Now we discuss three constraint declarations  in the upper-right part of the schema graph, whose scope is a triangle of arrows (scope lines for the left $[=^!]$ are omitted), which declare two different types of commutativity %and they all represent different types of commutativity constraints 
(discussed purely mathematically in \cref{sec:grothEquiv-table} ). 
The most general one is the {\em general} commutativity [=] (without any scripts) declared for the upper-most triangle of arrows. It requires existence for a valid instance $D$ a comparison function (laxator)
\begin{equation}\label{eq:laxator4drivesprim}
	\frar{\laxator{D}{(\drives, \of)}}{\semmD{\drives}.\semmD{\of}}{\semmD{\drivesprim}} 
\end{equation}
(the notation shows that there is no any arrow $\ell$ in the schema graph). This function is not required to be injective as if even span \semmD{\drives} is a proper span and hence composition $\semmD{\drives}.\semmD{\of}$ is also a proper span, we may want to eliminate duplicated elements in \semmD{\drivesprim} as non-relevant for the semantics of association \drivesprim. The laxator is also not required to be surjective if we admit in instance $D$ direct rather than composed references from a driver $d$ to a vehicle type $V$ (\eg, if the driver drove a vehicle of type $V$ for some time in the past while none of the vehicles she currently drives is of type $V$). 

The situation with composed \asson\
%\frar{\lcdprim=\lcdBy.\covers}{\Driver}{\Vehicle} %\Type} 
$~\lcdprim=\lcdBy.\covers~$ may seem similar, %to the case of $\drives.\of$ composition, 
but  is actually very different in our context. We do not want to admit non-composed references over $\lcdprim$  in a valid $D$: a link from driver $d$ to type $V$ typed by \lcdprim\ is only to be possible via the composition $d\xrightarrow[{:}\lcdBy]{l}L\xrightarrow[{:}\covers]{c}V$. Then we can consider \asson\ \lcdprim\ as a derived rather than basic in schema $S$: its extension \semmD{\lcdprim} does not need to be stored as it can be computed if needed: $\semmD{\lcdprim}=\semmD{\lcdBy}.\semmD{\covers}$ (up to iso). Existence of an iso\moric\ laxator
\begin{equation}\label{eq:laxator4lcdprim}
\laxator{D}{(\lcdBy,\covers)}{:}\,\semmD{\lcdprim}\cong \semmD{\lcdBy}.\semmD{\covers}
\end{equation}
is exactly what the constraint $[=^!]$ (called {\em strict commutativity}) demands. Now an important safety \req\ that a driver can drive a vehicle of type $V$ if only she is licenced to drive $V$-type vehicles is captured by constraint $[\Rightarrow]$, which demands a span \mor\ 
%\[ 
%\frar{f_D^R}{\semmD{\drives}}{\semmD{\lcdBy}.\semmD{\covers}}
%\]
\begin{equation}\label{eq:constr4drivesImpliesLicenced}
\frar{f_D}{\semmD{\drives}}{\semmD{\lcdprim}}
\end{equation}
(If we eliminate duplicates in span \semmD{\lcdprim}, this function will be injective.)
%

\endinput

==> sections/piece-lax-general-story-v2.tex <==
% version 2 of the piece, wand version 1 is below the enedinput
%\zd{version 2 of the story}
The uppermost note $[=]$ declares a major commutativity declaration (we may write it as ~$\drivesprim=\drives.\of$~), and needs discussion.  First of all we note that instance $D$ may have direct rather than composed references from a driver $d$ to a vehicle type $V$ if, \eg, driver $d$  drove a vehicle of type $V$ for some time in the past so that we have a link $(d,V)$ over \drivesprim\ even though  none of the vehicles she currently drives is of type $V$. We denote so formed span by \semmDzero{\drivesprim}. Now commutativity declaration  forces us to redefine this span as specified in the upper row (left) of table \cref{eq:laxator4drivesprim},
%\begin{equation}\label{eq:redefinition4drivesprim}
%	%\frar{\laxator{D}{[=]}}{\semmD{\drives}.\semmD{\of}}{\semmD{\drivesprim}} 
%	\semmD{\drivesprim} = \semmDzero{\drivesprim}\uplus\,\semmD{\drives}.\semmD{\of}
%\end{equation}
where span composition $\semmD{\drives}.\semmD{\of}$ is, in general, a multispan (\ie, non-jm, if even both constituents would be jm). This gives us an injective laxing function ({\em laxator}) as specified in the 3rd column. The last column specifies the corresponding factorization lifting property---partial Ufl: if factorization can be lifted, then it is unique. \zd{\large Note that commutativity declaration is, in fact, {\bf not} a constraint: it redefines any given instance rather than subject it to a Boolena check!!}
%
%	\incrar{\laxator{D}{[=]}}{\semmD{\drives}.\semmD{\of}}{\semmD{\drivesprim}} 
%
\begin{equation}\label{eq:laxator4drivesprim}
{%footnotesize 
	\small 
\begin{array}[h]{|c|l|c|c|}
	\hline
	\text{Comm} 
	&\text{Def. of composed span} %\semmD{\drivesprim}}
	& \text{Laxator} % \frar{\laxator{D}{[=]}}{\semmD{\drives}.\semmD{\of}}{\semmD{\drivesprim}} }
	& \text{FLPr}
	\\ \hline\hline  % the \drivesprim story 
\multirow{2}{*}{[=]} 
	&\semmD{\drivesprim}= \semmDzero{\drivesprim}\uplus\,\semmD{\drives}.\semmD{\of} 
	& %\incrar{\laxator{D}{[=]}}{\semmD{\drives}.\semmD{\of}}{\semmD{\drivesprim}} 
		\laxator{D}{[=]}{:} \semmD{\drives}.\semmD{\of}\xrightarrow{\text{inj}}\, \semmD{\drivesprim}
	& \mathsf{pUfl}
	\\ [2.5pt]
	&\semmXUD{\drivesprim}{D}{\vDash\jmpred } = \semmDzero{\drivesprim}\uplus\,(\semmD{\drives}.\semmD{\of})\!/{\simeq}
	& \frar{\laxator{D}{[=]}}{\semmD{\drives}.\semmD{\of}}{\semmD{\drivesprim}} 
	& \text{none}
\\ [2.5pt] \hline  % now \lcdprim story
\multirow{2}{*}{[=$^!$]} 
	&\semmD{\lcdprim} = %\semmDzero{\lcdprim}\uplus\,
									\semmD{\lcdBy}.\semmD{\covers} 
	& %\frar{\laxator{D}{[=]}}{\semmD{\lcdBy}.\semmD{\covers}}{\semmD{\lcdprim}} 
	\laxator{D}{[=^!]}{:} \semmD{\lcdBy}.\semmD{\covers}\xrightarrow{\cong}\, \semmD{\lcdprim}
	& \mathsf{Ufl}
\\ [2.5pt]
	&\semmXUD{\lcdprim}{D}{\vDash\jmpred} = %\semmDzero{\lcdprim}\uplus\,
									(\semmD{\lcdBy}.\semmD{\covers})/\simeq
	&  %\frar{\laxator{D}{[=]}}{\semmD{\lcdBy}.\semmD{\covers}}{\semmD{\lcdprim}} 
		\laxator{D}{[=^!]}{:} \semmD{\lcdBy}.\semmD{\covers}\xrightarrow{\text{surj}}\, \semmD{\lcdprim}
	& \mathsf{Wfl}
\\ \hline 
\end{array}
}
\end{equation}
However, we may want to eliminate duplicated elements in \semmD{\drivesprim} as non-relevant for the semantics of association \drivesprim, and redefine the span to make jm as specified in the second row, which gives us a general laxator. %which results in a surjective
%(note that there is no any arrow $\ell$ in the schema graph). Moreover, if we admit in instance $D$ direct rather than composed references from a driver $d$ to a vehicle type $V$ (\eg, if the driver drove a vehicle of type $V$ for some time in the past while none of the vehicles she currently drives is of type $V$), then the laxator becomes a general function neither injective nor surjective. 
%---
%\zd{This previous phrase is misleading: \textcolor{black}{``Possible specializations of the general case are considered in \cref{sec:grothEquiv-table}.''} \\ 	The point is that the Table in Appendix  describes the story for a general cat as the source of the typing map, while here we deal with freely gen cats, which may be factiorized then} 
The {\em strict} commutativity constraint  $[=^!]$ essentially differs from [=] and forces a different formal semantics adequate to the semantics of licencing. % , requires the laxator to be an iso\mor, and this is what we need for semantics of the composed \asson\ $~\lcdprim=\lcdBy.\covers~$. 
Indeed, now we  do not want to admit non-composed references over $\lcdprim$  in a valid $D$: a link from driver $d$ to vehicle type $V$ over \asson\ \lcdprim\ is only to be possible via the composition $d\xrightarrow[{:}\lcdBy]{l}L\xrightarrow[{:}\covers]{c}V$. Then we can consider  \lcdprim\ as a derived rather than basic \asson\ in schema $S$: its extension \semmD{\lcdprim} does not need to be stored but can be computed if needed: $\semmD{\lcdprim}:=\semmD{\lcdBy}.\semmD{\covers}$ (up to iso), the corresponding laxator \laxator{D}{[=^!]} is an iso\mor, and the factorization are lifted uniquely (see the third row in table \cref{eq:laxator4drivesprim}). The forth rwo specifies the case if we want to eliminate duplicates in span \semmD{\lcdprim}.
%Existence of an iso\moric\ laxator
%\begin{equation}\label{eq:laxator4lcdprim}
%\laxator{D}{(\lcdBy,\covers)}{:}\,\semmD{\lcdprim}\cong \semmD{\lcdBy}.\semmD{\covers}
%\end{equation}
%is exactly what the constraint $[=^!]$ (called {\em strict commutativity}) demands. 
Now an important safety \req\ that a driver can drive a vehicle of type $V$ if only she is licenced to drive $V$-type vehicles is captured by constraint $[\Rightarrow]$, which demands a span \mor\ 
%\[ 
%\frar{f^D_R}{\semmD{\drives}}{\semmD{\lcdBy}.\semmD{\covers}}
%\]
\begin{equation}\label{eq:constr4drivesImpliesLicenced}
\frar{f^D_{[\Rightarrow]}}{\semmD{\drives}}{\semmD{\lcdprim}}
\end{equation}
\zdmoddok{(If we eliminate duplicates in span \semmD{\lcdprim}, this function will be injective.)}{}{Nope!!!}{-2}{}
Similarly to the above, %\cref{eq:laxator4lcdprim}, 
(left) constraint $[=^!]'$ %(on the left) 
demands an iso\moric\ laxator   $\laxator{D}{[=^!]'}{:}\;(\semmD{\of}.\semmD{\subjTo})\xrightarrow{\cong}\semmD{\subjToprim}$,
%\begin{equation}\label{eq:laxator4subjToprim}
%$ \laxator{D}{(\of,\subjTo)}{:}\,\semmD{\subjToprim}\cong\semmD{\of}.\semmD{\subjTo}$.% 
%\end{equation}
\ie, %which means that 
each wheel \req\ a vehicle is to satisfy, is a \req\ for this vehicle type.%


\endinput

\zd{this formula may be useful further}
 $\semmD{\drivesprim}= \pmb{Elim}(\semmD{\drives}.\semmD{\of})\uplus{(\drivesprim_0)}^D$



==> sections/pieces--from_older_longlongIntro.tex <==
 

For the {\em generalized sketches} \fwk (below called just {\em sketches}, which should not be confused with Ehresmann's sketches and their variants), a data schema $S=(G_S, C_S)$ is a pair of a graphical object $G_S$ in some \caty\ \GG\ of {\em graphs}, and a set $C_S$  of constraint declarations over $G_S$, \ie, pairs $(c,\bmap )$ of a constraint name $c$ and a \GG-arrow  \frar{\bmap}{G_c}{G_S} from $c$'s predefined {\em arity} graph $G_c$. A model is a typing mapping, \ie, a \GG-arrow  \frar{\tmap}{\cdot}{G_S}, and satisfaction $\tmap \vDash (c,\bmap)$ 
is checked by pulling  \tmap\ back along $\bmap$  and checking that the result  \frar{\tmap_\bmap}{\cdot}{G_c} belongs to a predefined set \semm{c} of graphs typed over $G_c$. This is a much more concrete setting than with \instin s, and it is perfectly local as only a part $\tmap_\bmap$ of the entire data instance \tmap\ is responsible for constraint satisfaction.  Yet it is sufficiently abstract as all we need can be done in a finitely complete \caty\ (the terminal object and elements will also be important for us). Hence the name {\em Cartesian \sation} for the story. The sketch \fwk\ readily accommodates this by indexing the membership relation $\tmap_\bmap \in_v \semm{c}$ with index $v$ referring to some verification level. 


%---


Studying binary \sation\ relation $\vDash$ is a classical subject of mathematical logic, where constraints are logical sentences. 
Many constraint \specifin\ languages were developed, \eg, FOL and its fragments, Ehresmann's sketches, relational data dependencies, and Spivak's lifting constraints popular within the ACT community, or, \eg,  industrially usable OCL \cite{oclBook-99}. %B \cite{B-book}.  
This diversity does contribute to \IMt\ problems, and calls for a abstract unifying \fwk\ for $\models$
%Moreover, there are constraints that cannot de decomposed ... no syntax???
%
which is not being bound to specifics of a concrete constraint \specifin\ language. Attempts to develop such a theory 
%for purely mathematical reasons 
can be traced back to {\em abstract model theory} \cite{barwise-axioms4amt-AML74}
and, more recently, to Goguen and Burstall's {\em institutions} \cite{Goguen-Burstall-92}. 
% (well-known in the Algebraic \specifin\ community....
The latter is practically a bare-bone \fwk\ for describing translation of an abstract binary relation $ \satrelsig\subset \Modsetsig\timm\Sensetsig$ between  sets of {\em \Sigmaa-models} and {\em \Sigmaa-sentences} (\ie, constraints),  when the logical signature \Sigmaa\ changes ({\em \satrelsymbol-interoperability} in the technological speak). If such changes are specified by a signature \mor\ \frar{f}{\Sigmaa'}{\Sigmaa}, then the main and in fact the only substantial postulate of the institution construct states that sat-relation translates in a twisted way: for models with a function  \frar{f^*}{\Modsetsig}{\ModsetsigPrim} in the direction opposite to $f$, for sentences with function \frar{f_*}{\SensetsigPrim}{\Sensetsig} in the same direction, and such that for all $m\in\Modsetsig$ and all $\phi'\in\SensetsigPrim$, the {\em twisted \sation} 
condition \fbox{$f^*(m)\satrelsigPrim \phi' \text{~iff~} m\satrelsig f_*(\phi')$}
holds. This is the famous Sat-axiom of the institution theory, which is often phrased as {\em the invariance of truth wrt. the language translation} . 
%
%\input{diagrams/satAxiom-Rel}
%
%\input{sections/piece--aboutInstit4briefExpo}
%%specified in \cref{eqdiag:satisfyAxiom} holds. 


==> sections/predske-semantics.tex <==
\myendinput

\subsection{Semantics}
\zd{this sect needs an essential rework}
%\zd{Every generalized {\bf multisketch} is an object of a presheaf topos}
\begin{mydef}[Model of a sketch]
	\label{def:modofske}
	A {\em model} of a \predsig-sketch $S$ is a \predsig-model $A$ (the carrier) together with a sketch morphism \frar{m}{S}{A} (see also Example~\ref{ex:modelSketches}). % \frar{\semm{\_}^A}{S}{\semm{\predsig}^{\abs{A}}}.
	
	In logical terms, if theory $S$ has an axiom $c^\#=p(b)$ for some $c\in Constr(S)$, then formula $p(\compose{b}{\carrier{m}})$ is an axiom of $S'$: indeed, $p(\compose{b}{\carrier{m}})={(\constrfun{m}(c))}^\#$ and thus
	%In more detail, given a \predsig-sketch $S$, a \predsig-model $A$ and a map \frar{\semm{\_}^A}{\abs{S}}{A}, we say that the map  satisfies a constraint $c\in\constr{S}$ in sketch $S$ if... . Then we write $\semm{\_}^A\models c$. We write $\semm{\_}^A\models S$ if 
	$\interpret{\_}{A}\models c$ for all $c\in\constr{S}$. %
%	\footnote{Actually our def can be made tensorial. The abiove def, assumes AND interpretation of sketches. We can also consider OR interpretation so that $\semm{\_}^A\models S$ if 		$\semm{\_}^A\models c$ for at least one $c\in\constr{S}$ } 
\end{mydef}
\begin{myexa}[Sketches as Predicates]
\label{exa:sketchPredicate}
The text above Definition~\ref{def:dpgra} gives rise to another interesting example.
Every sketch $S$ can be turned into a \emph{new} predicate $q \in \predicateSig^+$.
Its arity $\arityOf{q}$ is given by $\carrier{S}$.
\PAST{What are its \emph{intended} models?!}
\end{myexa}
%The above example exemplifies how new predicates can be defined in terms of known ones.



==> sections/predskeSemantics.tex <==
\subsection{Semantics: Algebras and their morphisms}
%While \defref{opsig} defines syntax of graph operations, their semantics is given by the notion of a \emph{diagram algebra}.
\begin{defin}[Diagram Algebra]{diagOpSemantics}
Let $\operationSig$ be an operation signature over predicate signature \predsig.
An $\operationSig$-algebra is a pair $A = (\carrier{A}, {\semm{\_}}^A_{IO})$ that comprises a \emph{carrier} sketch $\carrier{A} \in \skecatgp$ and for each operation symbol $\omega$, its  {interpretation} $\semm{\omega}^{A}_{IO}$ as a {\em diagrammatic operation over $A$}, \ie, a mapping 
% $\_^\mathcal{A}$, that is a family $\{ \omega^\mathcal{A} : A^{I_\opvar} \to A^{O_\opvar} \mid \omega \in \opsig \}$ of maps obeying for all $b \in A^{I_\opvar}$ 
%\frar{\semm{\omega}^{A}_{IO}}{\carrier{A}^{I_\opvar}}{\carrier{A}^{O_\opvar}} 
$$
\frar{\opInterpret{\opvar}{A}_{IO}}{\homsetXA{I_\opvar}}{\homsetXA{O_\opvar}}%{\carrier{A}^{O_\opvar}} 
$$
such that the following diagram commutes for any \frar{b}{\inputArity{\opVar}}{\carrier{A}}:
\begin{equation}\label{eq:algviaE1}
\xymatrix{
	& K_\opvar \ar@{>->}[dl]_{KI_\opvar} \ar@{>->}[dr]^{KO_\opvar} \ar@{}[dd]|{}  & \\
	I_\opvar \ar@{>->}[dr]_b & & O_\opvar  \ar@{>->}[dl]^{\opInterpret{\opvar}{A}_{IO}(b)}\\
	& \carrier{A}&
}
\end{equation}
\end{defin}


It is easy to see that because the square $\arfun(\omega)$ is a pushout, the data above determines a unique mapping 
$$
\frar{\opInterpret{\opvar}{A}_{IE}}{\homsetXA{I_\opvar}}{\homsetXA{E_\opvar}}
$$
such that the following diagram commutes: 
\begin{equation}\label{eq:algviaE2}
%\[
\xymatrix{
I_\opvar \ar@{>->}[rr]^{IE_\opvar} \ar[dr]_b & & E_\opvar \ar[dl]^{\opInterpret{\opVar}{A}_{IE}(b)} \\
& \carrier{A} 
}
%\]
\end{equation}
Below we will mainly work with the interpretation $\semm{\_}^A_{IE}$ rather than $\semm{\_}^A_{IO}$ and normally omit the subscript $IE$. 

Note the fundamental nature of the condition \eqref{algviaE1}: It ensures that the input data for an operation are not changed.
%W.l.o.g., we let the arity functor $\arfun$ map every monomorphism in $\MonoSquare$ to an inclusion in $\skecatgp$ since it simplifies notation. \zd{hm, probably, a monic seen as an equiv. class can well be identified with inclusion.}


\mkExample{Universal Algebra}{ex:univAlgebra}{
Universal algebra is subsumed by diagrammatic operations: Consider $\cat{I} := \boldsymbol{1}$ so that $\cat{G}\cong\catSet$,  and $\predicateSig := \emptyset$ so that $\skecatgp \cong \cat{G} \cong \catSet$.
Every ``classical'' operation signature $ \Omega$ with an arity function $a : \absolute{\Omega} \to \catname{Nat}$ can be interpreted as a diagrammatic signature $(\opsig, \arfun)$ such that for each symbol $\omega$, its arity square $\arfun(\omega)(\Square)$ consists of  $I_\opvar=a(\omega)$, $O_\opvar=\{*\}$, $K_\opvar=\varnothing$ and hence $E_\opvar=a(\omega)+1$ with the obvious four inclusions. %where $\operationSig$ is the discrete category over $\absolute{\Omega}$  and the arity of an operation symbol $\omega \in \absolute{\opsig}$ is given by $\alpha(\omega)(IE) = \inlineinclusionarrow{\underline{a(\omega)}}{}{\underline{a(\omega)} + 1}$, where for a natural number $n$, {\em underlined} $n$, $\underline{n}$, denotes the set $\{0, 1, \ldots, n-1\}$ and $\underline{n} + 1$ denotes the disjoint union of $\underline{n}$ and the one-element set $\{\star\}$. Thus, the overlap arity $K_\opvar$ for every operation symbol $\omega \in \opsig$ in universal algebra is always \emph{empty}.
The notion of an $\opsig$-algebra is restored because every set $A^n$ %{\underline{n}}$ 
can equivalently be represented as an $n$-ary product $A \times \ldots \times A$. 
To define the operation interpretation, it suffices to specify the value of $A(\star)$ w.r.t. to a given $(a_0,\ldots,a_{n-1}) \in A\times\ldots\times A$ since the commutativity requirement in Def.~\ref{def:diagOpSemantics} requires that the input tuples $(a_0,\ldots,a_{n-1})$ remains unchanged.
}

%\renewcommand\opInterpret[]
\begin{defin}[Diagram Algebra Morphism]{diagOpAlgerbaMorphism}
Let $\operationSig$ be a operation signature and $A$ and $B$ be two $\opsig$-algebras.
An algebra morphism $\arrow{A}{f}{B}$ is given by a sketch morphism $\arrow{\carrier{A}}{\carrier{f}}{\carrier{B}}$ obeying 
\begin{equation}
\label{eq:diagAlgebraMoprhism}
\opInterpret{\opVar}{B}_{IE}(\compose{b}{\carrier{f}}) = \compose{\opInterpret{\opVar}{A}_E(b)}{\carrier{f}}
\end{equation}
for all $b : \inputArity{\opVar} \to \carrier{A}$. Diagrammatically:
\[
\xymatrix{
I_\opvar \ar@{>->}[rr]^{IE_\opvar} \ar[dr]_b \ar@/_/[ddr]_{\compose{b}{\carrier{f}}} & & E_\opvar \ar[dl]^{\opInterpret{\opVar}{A}_{IE}(b)} \ar@/^/[ddl]^{\opInterpret{\opVar}{B}_{IE}(\compose{b}{\carrier{f}})} \\
& \carrier{A}  \ar[d]^{\carrier{f}} & \\
& \carrier{B} &
}
\]
\end{defin}

\mkProposition{Algebra category}{prop:algebraCat}{
	The classes of all $\opsig$-algebras and all algebra morphisms between them form a category $\skecatgpo$.
}
\begin{proof}
Follows immediately from the fact that $\skecatgp$ is a category and the identity in Eq.~\ref{eq:diagAlgebraMoprhism} is transitive.
\end{proof}


\mkExample{Precategories}{ex:freeAlgebras}{
Consider $\skecatgp$ with $\cat{G} = \catGraph$, $\predsig = \emptyset$, and $\opsig=\{\langle id\rangle, \langle comp\rangle\}$.
The respective arities being:
\[  %\text{this figure is commented}
\xymatrix  {
 \alpha(\langle id\rangle )	& *+<7pt>[F:<3pt>]{\tikzfig{singleNode}} &  \ar@{^{(}->}[r]   &  &*+<7pt>[F:<3pt>]{\tikzfig{arityAddIdOp}} \\
 \alpha(\langle comp\rangle ) & 	*+<7pt>[F:<3pt>]{\tikzfig{TwoArrows}} &  \ar@{^{(}->}[r] & & *+<7pt>[F:<3pt>]{\tikzfig{arityCompOperation}}
}
\]
\zd{I'd use makkai's notation to denote arrows by 01, 12 etc}
\PAST{Needs completion}
}


==> sections/related-1.tex <==
\section{Related work}

==> sections/sketches-discreteDef.tex <==
\subsection{Discrete Hierarchical Signatures and Sketches}
\label{sec:discreteHierarchicalSketches}

We will redefine the notions of a predicate signature with dependencies and sketches over it in a discrete (but \hical) way: it is somewhat unexpected that this partial de-categorification does not actually lose information and the semi-discrete (below) and the fully categorical (above) notions are equivalent. To distinguish the two families, we will refer to the definition of a signature with dependencies as {\em functorial} (or {\em f-signature}) and a \corring\ notion of a sketch as {\em fibtrational ( f-sketch)}. Their counterparts defined below are {\em dh-signature} and {\em dh-sketch}  with prefix 'dh' referring to {\em discrete \hical}. 

Also, in this section we will denote discrete signatures and categories of sketches over them (defined in Def. \ref{def:predsig}) by symbols  $\PPdh$ and $\SS||\PPdh$, where superscript \dhind\ is intended to recall that a signature carrier is a set rather than a category, and \SS\ refers to the category of carriers which can be the category of graphs \GG, or some category of sketches defined before (recall that ``sketches are graphs'' by Makkai's theorem). Finally, in this section we will begin counting layers of \hical\ constructs at 1 rather than 0 simply because it's convenient to assign an empty signature of predicate symbols to index 0 rather than -1.   
%Recall that a predicate signature with dependencies is a \hical\ \caty:
%\PAST{Below I changed $\subset$ into $\subseteq$ since some layers may be empty and thus not add new predicates, moreover $\subset$ is not a partial order since it is not reflexive...}
%\zd{actually i changed the def of \hical\ cats yesterday but probably forgot to mention: no empty layers now}
%\clearpagezd
\begin{mydef}[Dh-signatures and (dh-)sketches over them] 
	Let $\GG$ be a presheaf topos of \II-graphs as before. A {\em predicate dh-signature  of height $N$} is given by the inductively defined data specified by the commutative diagram \eqref{psig-dh-def}. 
	\begin{equation}\label{eq:psig-dh-def}
	\xymatrix{
		\varnothing \ar@{>->}[r]
		\ar@{<.|}[rd]|{{:}\nfont{sig}}
		&  \PPdh_{0} \ar@{>->}[r]
		\ar@{<.|}[rd]|{{:}\nfont{sig}} \ar[d]^{\arfundh_0}
		&  \PPdh_{1} \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar[d]^{\arfundh_1}
		&  \hdots \ar@{>->}[r]
			\ar@{.}[d]
		&  \PPdh_{N-1} % \ar@{>->}[r]
		\ar@{<.|}[rd]|{{:}\nfont{sig}} \ar[d]_{\arfundh_{N-1}}
		\\ % Row 2
		&\GG \ar@{>->}[r] 
		&\SS_{0}\ar@{>->}[r]   \ar@/^/[l]^{\carr{.}}
		&\hdots\ar@{>->}[r]  \ar@/^/[l]^{\carr{.}} 
		&\SS_{N-2}\ar@{>->}[r] \ar@/^/[l]^{\carr{.}}
		&\SS_{N-1} \ar@/^/[l]^{\carr{.}}
	}
	\end{equation} 
The upper row is provided by a discrete \hical\ \caty\ \PPdd\ of {\em predicate symbols} of height $N$,  \ie, a finite chain of non-empty sets shown in the top row of the diagram. Each of these sets $\PPdh_i$ is equipped with an arity function $\arfundh_i$ into the \corring\ category of sketches $\SS_{i-1}\eqdef\SS_{i-2}||\PPdh_{i-1}$, $i<N$ as shown in the bottom row of the diagram. Note that this sequence starts from $\GG=\SS_{}$, \ie,  sketches with the empty signature, which allows us to defined mapping $\arfundh_0$, which in turn defines sketch category $\SS_0$ and so on. Bottom arc arrows show the carriers. Diagonal dotted arrows labelled ${:}\nfont{sig}$ are pairs rather than mappings (and can be seen as instances of some big mapping \nfont{sig} from the big category of all sketches to the big category of all signatures, which we don't consider in the paper). 


The above defines a dh-signature \PPdh. {\em Sketches over \PPdh} and their {\em \mor s} are defined as objects and arrows of the category $\SS_{N-1}\eqdef \SS_{N-2}||\PPdh_{N-1}$. We will denote this category by $\GG||\PPdh$: strictly speaking, we should write $\GG||^\dhind\,\PPdh$ as it's another construct of building sketches, but we will usually omit the superscript near $||$ if the right term unambiguously shows the dh-context of $||$. 
\end{mydef}
%\begin{mycor}\label{coro:discSketchesAsTrees}
%Any sketch $S\in \GG||\PPdd$ is decomposed into a tree $T(S)$ of labelled diagrams \zd{to be specified}
%%$$\comprfam{S_{ij}}{i\in \{N-1, N-2,....,1,0\}, j\in \iConstrset{S_i}},$$
%% \corring\ to the chain of sketch categories c) above. 
%\end{mycor}
\begin{mythm}\label{thm:dh=f}
Any dh-signature \PPdd\ gives rise to a functorial signature \dideP, and any functorial signature \PP\ %(\ie, we have a \hical\ category \carr{\PP} and a functor \frar{\arfun}{\carr{\PP}}{\GGop}) 
gives rise to a dh-signature \dediP. Moreover, $\disctodep{(\dediP)}\cong\PP$ and  $\deptodisc{(\dideP)}\cong\PPdd$.
\end{mythm}
\begin{proof} Let \PPdh\ be a dh-signature as defined above. Makkai's theorem  	
allows us to rewrite 
	\flar{\arfun_2}{\SS_1}{\PPdd_2} as 	\flar{\arfun_2}{\setcat^{\II\star_{\arfun_1}\PPdd_1}}{\PPdd_2}, then  currying gives us a profunctor 
$$	\flar{\hat\arfun_2}{\setcat}{\left(\II  \star_{\arfun_1}\PPdd_1\right)\times \PPdd_2}$$
 (we don't write ${\PPdd}_2^\oppind$ as $\PPdd_2$ is discrete), whose collage is the category 
	$$\left(\II \star_{\arfun_1}\PPdd_1\right)\star_{\arfun_2}\PPdd_2.$$
	 The latter, for any $P\in\PPdh_2$ and $P'\in\PPdh_1$, has a wavy arrow \frar{\ovr{c}}{P}{P'} iff there is a diagram index $c\in P^{\arfun_2}(P')$ (\ie, an element in $\semm{P'}$ for sketch $P^{\arfun_2}$), and similarly, any wavy arrow  \frar{\ovr{a}}{P}{H} is generated by a cell $a\in P^{\arfun_2}(H)$ in the carrier of sketch $P^{\arfun_2}$--- we use overlining and underlining as earlier in definitions \eqref{wavyarr-ovr} and \eqref{wavyarr-und} (Example in \figref{collage-pbm} shows how it works). We continue for $i=3...N$ and obtain the  commutative diagram formed by the upper lane of squares in \eqref{psig-dh-collageChain}:
	 
\begin{equation}\label{eq:psig-dh-collageChain}	
		\xymatrix{
		\varnothing \ar@{>->}[r]
		\ar@{>->}[d] %|{{:}\nfont{sig}}
		&  \PPdh_1 \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar@{>->}[d] %^{\arfun_1}
		&  \PPdh_2 \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar@{>->}[d] %^{\arfun_2}
		&  \hdots \ar@{>->}[r]
		\ar@{.}[d]
		&  \PPdh_N % \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar@{>->}[d] %^{\arfun_N}
		  \\ %Row 2
		\II \ar@{>->}[r]
		\ar@{<-<}[d] %|{{:}\nfont{sig}}
		&  \HPP{\arfun_1}_1 \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar@{<-<}[d] %^{\arfun_1}
		&  \HPP{\arfun_2}_2 \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar@{<-<}[d] %^{\arfun_2}
		&  \hdots \ar@{>->}[r]
		\ar@{.}[d]
		&  \HPP{\arfun_N}_N % \ar@{>->}[r]
		%\ar@{<.|}[rd]|{{:}\nfont{sig}} 
		\ar@{<-<}[d] %^{\arfun_N}
				\\ % Row 3
		\varnothing \ar@{>->}[r] 
		&\PPstar{\arfun_1}_1\ar@{>->}[r]   
		& \PPstar{\arfun_2}_2 \ar@{>->}[r]
		&\hdots\ar@{>->}[r]  %\ar@/^/[l]^{\carr{.}} 
		%&\HPstar{}_{N-1}\ar@{>->}[r]  %\ar@/^/[l]^{\carr{.}}
		&\PPstar{\arfun_N}_N  %\ar@/^/[l]^{\carr{.}}
	}
	\end{equation}
In this lane, the lower line (starting at \II) is a chain of collage categories obtained by inductively adding binding/wavy arrows (taken from the arity sketches elements) layer by layer. (Example in \figref{collage-pbm} would illustrate the idea if we make all orange arrows black wavy arrows.)	By removal of the subcategory \II\ (and resp. all arrows from predicates to \II-objects) from each of the collages, we obtain the bottom chain of categories $\PPstar{\arfun_{i}}_i$. (With the colour legend of the example in \figref{collage-pbm}, we remove all black arrows from predicate symbols to \II\ but keep arrows between predicates and colour them in orange. Thus, the difference between set $\PPdh_i$ and category $\PPstar{}_i$ is the presence of (formerly wavy and black but now) orange arrows $\ovr{c}$ between predicate symbols specified above.) The arrows that left in categories  $\PPstar{}_i$ actually specify dependencies,  and we can consider category $\PPstar{}_N$ as the carrier of a f-signature with dependencies. To complete the story and make $\PPstar{}_N$ a signature, we need to define the \corring\ (integrated) arity functor 	

\begin{equation}\label{eq:intArity-def} %\label{eq:composedCollage}
\mbox{\frar{\intAr}{\PPstar{}_N}{\GGop}}
% \left(\ldots\left(\PPdd_1\star_{\arfun_1}\II\right)\star_{\arfun_2}\PPdd_2\right)...\star_{\arfun_N}\PP_N
	\end{equation}	 
	On objects, for any $i\le N$ and $P\in\PPdh_i$, we set    $\intAr(P)\eqdef\carr{\arfun_i(P)}$. 	
	
	For arrows, given a binding/wavy arrow \frar{\ovr{c}}{P}{P'} for $P'\in\PPdh_{i-1}$,  we define 
	 \begin{equation}\label{eq:arrowDefFordh2f}
	 \mbox{
	 \frar{\intAr(\ovr{c})\eqdef
	 	\diagr^{\arfun_i(P)}(c)}{\carr{\arfun_{i-1}(P')}} {\carr{\arfun_i(P)}}
 	}
 \end{equation}
Checking the functoriality of so defined \intAr\ is straightforward, which makes the pair $(\PPstar{}_N, \intAr)$ a correct f-signature. We will denote it by \intP\ (so that now the carrier $\PPstar{}_N$ is also denoted by \intP~).
	 
	 \medskip
	 Now we consider the transition in the opposite direction. Let \PP\ be an f-signature of height $N$ with arity functor \frar{\arfun}{\PP}{\GGop}. Recall that f-signatures are layered, layers are sets, and we define $\PPdh_i=\PP_i$ for all $1\le i\le N$. For each $P\in \PPdh_i$, we define sketch $\arfun_i(P)$ as follows. The carrier $\carr{\arfun_i(P)}=\arfun(P)$. Diagrams are given by dependency arrows: for any $P'\in \PPdh_{i-1}{=}\PP_{i-1}$, we set 
	 $P^{\arfun_{i}}(P')=\semm{P'}=\compr{\und{p}}{p\in\PP(P,P')}$ (recall that formally $\und{p}$ is just a couple $(p,*)$ of $p$ with any aside token *), and for any index $\und{p}\in\semm{P'}$, the diagram $\diagr(\und{p})$ is defined to be mapping $\arfun(p)$ (the construction is exactly the inverse to \eqref{arrowDefFordh2f}).  Thus, we have decomposed f-signature into a dh-signature $\dediP$, in which dependency arrows are hidden in diagrams of the arity sketches.
	%
	Iso\mor s immediately follow from the constructions above. 
\end{proof}
\begin{mycor}\label{thm:hier=func} a) Given an f-signature (\ie, predicate signature with dependencies) \PP, two categories of sketches, \skecatgp\ and $G||\dediP$
%	$$ \mbox{
%		\skecatgp\ and $G||\dediP = (\!...((G||\PP_1)||\PP_1)...)||\PP_{N}$ 
%	}$$ 
are iso\moric. %(Note that all \cats\ $\PP_i$ are discrete \hical\ \cats, and arity mappings are functions rather than functors.) 
b) Given a dh-signature \PPdh, two categories of sketches, $G||\PPdh$ and $\GG||\dideP$, 
% 	$$ \mbox{
% 	$\GG||\dideP$ and $G||\PPdd = (\!...((G||\PPdd_1)||\PPdd_1)...)||\PPdd_{N}$ 
% }$
are iso\moric\ as well.%
\footnote{The bulky formulation of this theorem should shorter and properly be stated if we introduce categories of f-signatures and dh-signatures, the \corring\ categories of sketches over them, and two functorial iso\mor s. We leave it for future work. 
} 
\end{mycor} 
\tempendinput
\begin{proof}{\em (sketch)} Let \PP\ be an f-signature and $S\in\GG||\PP$ an f-sketch over it. By our generalized Makkai's theorem, $S$ is equivalent to a presheaf \frar{\stog{S}}{\pstarii}{\setcat}
\zdzd{to be completed%: the previously done proof-sketch  can be stated more accurately based on  \eqref{composedCollage} and Corollary \ref{coro:discSketchesAsTrees}
}
\end{proof}

\endinput
Having a signature with dependencies \PP, any sketch $S\in\skecatgp$ is a presheaf \stog{S} on the \corring\ collage category by our generalized Makkai theorem. This collage category is decomposed as described in \eqref{composedCollage}, and presheaf \stog{S} is \corring ly decomposed into a tree of presheaves $\stog{S}_{ij}$. we thus have a family of presheaves  into a hierarchy $(...((G||\PP_0)||\PP_1)...)||\PP_{N-1}$ (not necessarily the full sequence  is needed) is straightforward by Makkai's theorem. The converse translation is based on the collage category construction \eqref{composedCollage} and Makkai's constructions. 

\zd{Based on \eqref{composedCollage}, the argument below can be stated more accurately}
We note that 
$$\PP=\bigcup_{0\le i<N}\PP_{i,i+1},$$
where each $\PP_{i,i+1}$ is a category consisting of two sets of objects and a set of parallel (wavy/binding) arrows between those sets. Then given a sketch $S\in (...((G||\PP_0)||\PP_1)...)||\PP_{N-1}$,  which is actually a series of sketches $S_i$, Makkai's construction gives us a series of presheaves \frar{\stog{S_i}}{\PP^\oppind_{i,i+1}\star_{\arfun_i}\II}{\setcat}. Treating the union above as a \corring\ colimit (overlaps between object layers of $\PP_{i,i+1}$ are to be specified), and having the commutative cocone formed by the presheaves $\stog{S_i}$, the universal property of the colimit gives us a presheaf \frar{\bigcup_i\stog{S_i}}{\PP^\oppind\star_\arfun\II}{\setcat}. The latter gives us a sketch $\widehat{\bigcup_i\stog{S_i}}$ in \skecatgp\ by our generalized Makkai's theorem.  
\end{proof}
%Suppose we have a predicate signature with dependencies $\PP=(\carr{\PP}, \arfun)$ and a 
\zd{the piece with fibrational def of \hical\ sketches is commented}


\endinput

%	We define the category of dh-sketches over \PPdd\ as the category $\SS_{N-1}||\PPdd_{N}$, which unravels as 
%	$$\left(\SS_{N-2}||\PPdd_{N-1}\right)||\PPdd_{N}=\ldots= 
%	\left(\!...\!\left( \left(\GG||\PPdd_1\right) ||\PPdd_2\right)||\ldots\right)||\PPdd_{N}
%	$$ 
%	We may write this as a definition of the category of dh-sketches over a dh-signature:
%	$$%\GG||^\dhind\left( \PPdd_0||\ldots||\PPdd_{N-1}\right) 
%	\GG||^\dhind\PPdd\eqdef\left(\!...\!\left( \left(\GG||\PPdd_0\right) ||\PPdd_1\right)||\ldots\right)||\PPdd_{N-1}
%	$$
%	whose right part only uses ordinary one-layer signatures and sketches.
%\PAST{Something is broken in the equation above what should $\carr{\arfun}_{n+1|\predsig_n}$ mean? I think is undefined! Maybe your macro $\backslash$ frestr is used wrongly but I also have no idea what ``frestr'' should mean...}
%\zd{$\backslash$frestr means "function's restriction" and was HEAVILY  used in the makkai's  section just above}


==> sections/squareArity.tex <==
\section{Square arity}

\zd{this sect is intended to collect all considerations in which an operation arity is \Square\ rather than monic}
\input{sections/complements}
\subsection{Syntax: From IE to IKO}

Data above give rise to the following collection of sketches, graphs, and their mappings.
\begin{myconstr}[Arity Square]
	\label{constr:arsquare}
	%{\em 
	Let $\Square$ be a fixed finite category specified in diagram \eqref{Square} (a), where identities are omitted and commutativity is assumed:  $\KI\comp \IE =\KO\comp \OE$. The nodes $\I,\O,\K,\E$ are called, %  $I_\opvar, O_\opvar, K_\opvar, E_\opvar$ are called, 
	resp., the {\em Input, Output, Overlap}%
	\footnote{denoted by $K$ due to historic reasons: overlap or interface graphs play an important rule in DPO rewriting, and the German speaking founders of the DPO approach called this interface graph \emph{``Klebegraph''} meaning \emph{``gluing graph''} in German}, 
	and {\em scopE} of an operation.
	%}
	\begin{equation}\label{eq:Square}
	%	\[
	\begin{array}{ccc}
	\xymatrix{ % diag a)
		& \K \ar@{->}[dl]_{\KI} \ar@{->}[dr]^{\KO} \ar@{}[dd]|{}  & \\
		\I \ar@{->}[dr]_{\IE} & & \O  \ar@{->}[dl]^{\OE} \\
		& \E& \\
		%	\ar@{-} <25pt,-58pt>;<33pt,-50pt>  
		%	\ar@{-} <41pt,-58pt>;<33pt,-50pt> 
		%	\ar@{-} <25pt,-12pt>;<33pt,-20pt>  
		%	\ar@{-} <41pt,-12pt>;<33pt,-20pt> 
	}
	%	\]
	&
	\xymatrix{ % diag b)
		& K_\opvar \ar@{>->}[dl]_{KI_\opvar} \ar@{>->}[dr]^{KO_\opvar} \ar@{}[dd]|{}  & \\
		I_\opvar\ar@{>->}[dr]_{IE_\opvar} & & O_\opvar  \ar@{>->}[dl]^{OE_\opvar} \\
		& E_\opvar& \\
	}
	&
	\xymatrix{ % diag c)
		& K^\GG_\opvar=\carr{K_\opvar} \ar@{>->}[dl]_{KI^\GG_\opvar=\carr{KI_\opvar}} \ar@{>->}[dr]^{KO^\GG_\opvar=\carr{KO_\opvar}} \ar@{}[dd]|{}  & \\
		\carr{I_\opvar}\ar@{>->}[dr]_{\carr{IE_\opvar}} & & O_\opvar^\GG=\carr{O_\opvar}  \ar@{>->}[dl]^{OE^\GG_\opvar=\carr{OE_\opvar}} \\
		& \carr{E_\opvar}& \\
	}
	\\
	\text{a) \Square}  
	&
	\text{b) $\arfun(\opvar)(\Square)$ in \skecatgp}
	&
	\text{c) $\carr{\arfun(\opvar)(\Square)}$ in \GG}
	\\
	&  \text{\zd{Pls add PB corner}}
	&  \text{\zd{Pls add cPO corner}}
	\\
	&  \text{\zd{\& make der elem blue}}
	&  \text{\zd{ditto}}
	\end{array}
	\end{equation}
	Given a signature \frar{\arfun}{\opsig}{\monicspacegp}  and an operation $\opvar\in\opsig$, we obtain a sketch monic $\arfun(\opvar)$ shown in diagram  \eqref{Square}(b) as $IE_\opvar$, and the corresponding graph monic $\carr{IE_\opvar}$ in diagram (c).
	%, whose domain and codomain are carrier graphs of sketches $I_\opvar=\dom(\arfun(\opvar))$ and $E_\opvar=\cod(\arfun(\opvar))$.  
	As category \GG\ has weak compliments \sectref{complement}, monic  \carr{IE_\opvar}
	%\incrar{\carr{IE_\opvar}}{\carr{I_\opvar}}{\carr{E_\opvar}} (we now denote $\opvar^\arfun$ by $IE_\opvar$) 
	generates a cPO-square $(IE^\GG_\opvar, OE^\GG_\opvar, KO^\GG_\opvar, KI^\GG_\opvar)$ as shown in diagram c). (ignore equations in the labels of the elements for a moment). 
	% \zd{It seems it'd be nice to have a symmetric notion of a cPO ({\em complementary pushout}) square: it's a PO plus some additional property}
	As \GG\ is adhesive, this square is a pullback too. 
	
	As for diagram b), so far we only havee a sketch monic $IE_\opvar$. To obtain the entire square, we proceed in the following way. We first obtain monic $OE_\opvar$ as a chosen Cartesian lifting of monic $OE^\GG_\opvar$ (see Prop. \ref{prop:skeFibr}(c) on p. \pageref{prop:skeFibr}, which also implies that $OE^\GG_\opvar=\carr{OE_\opvar}$). 
	
	We complete the square by taking a pullback of span $(IE_\opvar, OE_\opvar)$ and thus we have a functor \frar{\opvar^{\ovr{\arfun}}}{\Square}{\skecatgp} (which extends functor \frar{\opvar^\arfun}{\monicArrow}{\skecatgp} and) whose image is a pullback for any operation \opvar.  The sketches $I_\opvar, O_\opvar, K_\opvar, E_\opvar$ are called, resp. the {\em Input, Output, Overlap, {\em and} scopE} of operation $\opvar$.
	%
	Moreover, as the pullback of sketches in diagram (b) is based on the pullback of their carrier graphs, and the square (c) is a pullback too, we conclude that the entire square (c) is the image of the composed functor $$\Square\rTo^{\opvar^{\ovr{\arfun}}}\skecatgp\rTo^{\carr{.}}\GG.$$ Note that while diagram (c) is a pushout in \GG, diagram (b) may not be a pushout in \skecatgp\ if sketch $E_\opvar$ has constraints that do not occur into $I_\opvar$ nor $O_\opvar$. %
\end{myconstr}
The discussion above is summarized by the following.
\begin{myprop}[Extended Arity functor]
	\label{prop:extendedArity}
	Any operation signature \frar{\arfun}{\opsig}{\monicspacegp}
	%skecatgp^{\cdot\hookrightarrow\cdot}} 
	gives rise to a functor  \frar{\ovr{\arfun}}{\opsig}{\squarespacegp} 
	%{\skecatgpmonic^{\Square}} 
	whose image is a pullback of monics as shown in diagram \eqref{Square}(b), while the image of the composed functor 
	$$\Square\rTo^{\arfun(\opvar)}\skecatgp\rTo^{\carr{.}}\GG$$
	is a complementary pushout square in \GG\ (and hence is also a pullback) as shown in diagram \eqref{Square}(c). 
	\zd{all this is nice but the problem is that the proof of Prop. \ref{prop:atomquery} now needs to be revised, actually a new proof is to be found. }
\end{myprop}

%\footnote{We could formulate conditions say this by, first, considering \Square\ to be a sketch in the corresponding signature and requiring $\arfun(\opvar)$ to be a sketch morphism.}
%considering $[,\Square, \skecatgp]$ to be the set of all sketch morphisms.}

%For a symbol $\opvar\in\opsig$, the elements of the image category $\arfun(\opvar)(\Square)$ are named a shown in diagram \eqref{Square}(b). %(all arrows are monic due to condition a)). %  and name $X\in\sqobs$, we write $X_\opvar$ for the sketch $\arfun(\opvar)(X)$, and correspondingly $XY_\opvar$ for the  sketch morphism $\arfun(\opvar)(XY)$, $XY\in\sqarrs$; due to condition a), all these are monics. 
%

%Note that due to adhesiveness of \skecatgp\ and \GG, every pushout square $\arfun(\opvar)$ for an operation symbol $\opvar \in \opsig$ is not only a pushout in \skecatgp\ (resp. \GG)  but also a pullback in \skecatgp (resp. \GG). 

\begin{mydef}[IO vs. IE opperations]
	\label{def:optypes2}
	Operation $\opvar\in\opsig$ is called an {\em IO-operation} if the square in \eqref{Square}(c) is a pushout in \skecatgp. In this context, we will sometime call general operations as defined in \defref{opsig} {\em IE-operations}. 
\end{mydef}


\subsection{Syntax: the prism business}

Diagram \eqref{atomquerydiag} gives rise to a prism diagram  \eqref{queryPrism} built by a  diagram chasing described bewlo. %in Appendix \sectref{queryPrism}. 
\zd{Now proving this is a whole story if at all possible w/out further restrictions}
\begin{equation}
\label{eq:queryPrism}
\xymatrix{
	& & K_\opvar \ar@{>->}[dll]_{KI_\opvar} \ar@{>->}[dr]^{KO_\opvar} \ar@{->>}[ddd]^(0.6){b^K_q}|{\hole} & \\
	I_\opvar \ar@{>->}[dr]_{IE_\opvar} \ar[ddd]_{b^I_q} & & & O_\opvar  \ar@{>->}[dll]_(0.6){OE_\opvar} \ar@{->>}[ddd]^{b^O_q} \\
	& E_\opvar \ar[ddd]^(0.6){b^E_q} & & \\
	& & K_q\ar@{_{(}->}[dll]|{\hole}_(0.4){KI_q} \ar@{^{(}->}[dr]^{KO_q} & \\
	I_q \ar@{^{(}->}[dr]_{IE_q} & &  &O_q \ar@{_{(}->}[dll]^{OE_q} \\
	& E_q & & \\
}
\end{equation}
%\begin{lemma}[Atomic Query Arity]\label{lem:atomquery}	\normalsize
\begin{myprop}[Atomic query arity]
	\label{prop:atomqueryPrism}
	Every atomic query gives rise to a diagram 
	$$\frar{\bind(q)}{\Square}{(\skecatgp)^{\cdot\rightarrow\cdot}}$$
	in an arrow category whose objects are sketch moprhisms (\eg, $\bind(q)(I)=b^I_q$) and arrows are commutative squares  (\eg, $\bind(q)(IE)$ is the left-front square of the prism). 
	%Note that this arrow category has two obvious projections:
	% \frar{\bind^{\dom}(q)}{\Square}{\skecatgp} (the top square equal to $\arfun(op(q))$) and 
	%\frar{\bind^{\cod}(q)}{\Square}{\skecatgp} (the bottom square).
	%}
	%$\Square \to \skecatgp^{~\cdot\rightarrow\cdot}$ visualized by the prism diagram \eqref{queryPrism}, where the 
	The left-front, top and bottom faces of the prism are pushouts (see Appendix \sectref{queryPrism} for a proof) denoted by $Dom(\bind(q))$ and $Cod(\bind(q))$.
\end{myprop}
%\end{lemma}
\input{sections/proof-prizmLemma}

\subsection{Semantics}

\begin{mydef}[Deep semantics for operations]
	\label{def:deepSemantics}
	Let $\opsig$ be an operation signature over predicate signature \predsig. The {\em deep IO-semantics} of an operation $\opvar\in\opsig$ is given by a mapping
	\frar{\semm{\opvar}_{IO}}{\semm{I_\opvar}}{\semm{O_\opvar}}
	such that 
	\begin{equation}
	\label{eq:IOSemantics}
	PB_{KI_\opvar}(t_I) =t_K=PB_{ KO_\opvar}(\semm{\opvar}_{IO}(t_I))
	\end{equation}
	%$\compose{KI_\opvar}{t} =\compose{KO_\opvar}{\semm{\opvar}_{IO}(t) $ 
	for any valid model $t_I\in\semm{I_\opvar}$ (this equality means that the $K_\opvar$-part of the input data are not allowed to be changed). 
	
	The {\em deep IE-semantics} of an operation $\opvar\in \opsig$ is a mapping
	\frar{\semm{\opvar}_{IE}}{\semm{I_\opvar}}{\semm{E_\opvar}} %%\frar{\semm{\opvar}}{\semm{I_\opvar}}{\semm{E_\opvar}} 
	such that for any 
	$t_I\in\semm{I_\opvar}$, equality $t_I=PB_{IE_\opvar}(\semm{\opvar}_{IE}(t_I))$ holds (see diagram in \eqref{deep-ie-sem}) -- this requirement ensures that input data are not changed.
	\begin{equation}\label{eq:deep-ie-sem}
	%\[
	\xymatrix{
		% row 1
		\inputArity{\opvar} 
		\ar@{^{(}->}[r]^{IE_\opvar} 
		& \scopeArity{\opvar} 
		\\  % row 2
		A 	\ar[u]^{t_I}  \ar@{^{(}->}[r] 
		\ar@{}[ur]|(.2){\Large \urcorner} 
		& 
		\semm{\opvar}_{IE}(A) % A_E^\opvar 
		\ar[u]_{\semm{\opvar}_{IE}(t_I)} 
	}
	%\]
	\end{equation} 
	
\end{mydef}
\begin{mylem}[IO and IE semantics are equivalent]
	\label{lem:deepsem-io=ie}
	
	\begin{equation}
	\label{eq:vanKampenSemantics}
	\begin{tabular}{cc}
	\xymatrix @C=3em @R=2em{
		& K_A \ar@{_{(}->}[dl]_{KI_A} \ar@{^{(}->}[rr]^{KO_A} \ar[dd]^(0.7){t_K}|{\hole} &  & O_A \ar@{_{(}->}[dl]^{OE_A} \ar[dd]^{t_O=\semantics{\opvar}_{IO}(t_I)} \\ 
		A  \ar@{^{(}->}[rr]^(0.7){IE_A} \ar[dd]_{t_I} &  & E_A \ar[dd]_(0.7){t_E} &  \\ 
		& K_\opvar \ar@{_{(}->}[dl]_{KI_\opvar} \ar@{^{(}->}[rr]^(0.7){KO_\opvar}|{\hole}  &   & O_\opvar \ar@{_{(}->}[dl]^{OE_\opvar} \\
		I_\opvar \ar@{^{(}->}[rr]_{IE_\opvar} &  & E_\opvar
	}
	&
	\xymatrix @C=3em @R=2em{
		& K_A \ar@{_{(}->}[dl]_{h} \ar@{^{(}->}[rr]^{k} \ar[dd]^(0.7){t_K}|{\hole} &  & O_A \ar@{_{(}->}[dl]^{h^*} \ar[dd]^{t_O} \\ 
		A  \ar@{^{(}->}[rr]^(0.7){k^*} \ar[dd]_{t_I} &  & E_A \ar[dd]_(0.7){t_E=\semantics{\opvar}_{IE}(t_I)} &  \\ 
		& K_\opvar \ar@{_{(}->}[dl]_{KI_\opvar} \ar@{^{(}->}[rr]^(0.7){KO_\opvar}|{\hole}  &   & O_\opvar \ar@{_{(}->}[dl]^{OE_\opvar} \\
		I_\opvar \ar@{^{(}->}[rr]_{IE_\opvar} &  & E_\opvar
	}
	\\
	$t_K=\PB_{KI_\opvar}(t_I) = \PB_{KO_\opvar}(t_O)$ by \eqref{IOSemantics}
	& 
	$t_O=\PB_{OE_\opvar}(t_E)$
	\\
	$(OE_A, IE_A)=\PO(KI_A,KO_A)$
	&
	$t_K=\PB_{KE_\opvar}(t_E)$
	\\
	$t_E$ is the universal arrow of the upper PO
	& 
	\end{tabular}
	\end{equation}	
	``$\Rightarrow$''\par
	Consider the diagram in Equation~\eqref{vanKampenSemantics}.
	The bottom square is a pushout consisting of monos by definition, thus it has the VanKampen property.
	The rear left and rear right squares a pullbacks according to the definition in Equation~\eqref{IOSemantics}.
	Now, we construct the top square as pushout, which yields the universal arrow
	\frar{\semantics{\omega}_{IE}(t_I)}{A^+}{E_\omega}.
	Finally, because of the VanKampen property the two front squares become pullbacks, i.e. providing the necessary property for IE-semantics.\par
	``$\Leftarrow$'' \PAST{I think here might be a problem. We cannot use the VanKampen property in the opposite direction, i.e. to conclude that the rear squares are pullbacks when the front squares are.}
\end{mylem}

==> sections/subsec--genGra.tex <==
%\renewcommand{\HH}{\enma{H}}
\subsection{Generalized Graphs}\label{sec:genGraphs}
%The rationale  behind this terminology is due to arguably the most import representative: \emph{directed multigraphs}.
As our discussion in Sect.2 suggests, we need a very general notion of graphs as presheaves  \frar{G}{\II}{\setcat} for a suitable schema category $\II$. \zdmodd{In all our applications, graphs have \hical\ structure that allows their traversal from the top elements to the bottom. 
%our with the only restriction is an arbitrary but fixed finite category whose objects are called {\em cell types}, and for object $H\in\HH$, elements of set $G(H)$ are called $G$'s {\em cells of type $H$}. 
For example, ordinary directed multigraphs are given by schema $\II=\Graph$ with $\Ob{\Graph}=\{\nfont{Node},\nfont{Arrow}\}$ and two non-identity arrows \frar{\so,\ta}{\nfont{Arrow}}{\nfont{Node}} so that object \nfont{Arrow} is above \nfont{Node}
\shortlong{Other examples can be found in the TR.
}{(Below we will show other examples.)}
Hence, we require category \II\ to be \hical\ in the folloiwng sense.}{}{NoNoNo!!!} {-3}

\begin{mydef}[Graphs] \label{def:hgraph}
Let \II\ be a \caty. A {\em \II-graph} is a functor \frar{G}{\II}{\setcat}, \ie, a (co)presheaf over {\em schema} \II. We will normally refer to such functors as merely graphs, but if we want to stress their distinction from ordinary directed multigraphs (which are functors \frar{G}{\II_\graphind}{\setcat} over schema specified in \cref{eqdiag:schema4graphs} above or maybe \cref{eqdiag:schema4graphsCurved} below would be better ), we will refer to them as \II-graphs or, sometimes, as 'graphs' in single quotes. 
\zd{this is another version }
\begin{equation}\label{eqdiag:schema4graphsCurved}
\begin{tabular}{c}
	$	\xymatrix{
		\nfont{Node} 
		& \nfont{Arrow} \ar@/^4pt/[l]^{\ta}\ar@/_4pt/[l]_{\so}	
	} $
	\\
	Schema \Graph\ for ordinary (directed multi-)graphs
\end{tabular}
\end{equation}
\ActTR{% Act 23 version 
	For a graph $G$, we write $\Elem{G}$ for the set $\bigcup_{X\in\Ob{\II}}G(X)$. }
{ % the longer TR version with hierarchiers 
For a graph $G$, elements of set $G(H)$ with $H\in\II_n$ are called {\em n-cells (of type $H$)}, and if $\II_n$ is not a singleton, we say that $n$-cells are multi-sorted. We write $\Elem{G}$ for the set $\bigcup_{H\in\Ob{\II}}G(H)$. 
}
	The presheaf topos of all \II-graphs will be denoted by \GG, and we assume that throughout the paper the schema \II\ is arbitrary but fixed. A graph $G$ is {\em finite} if $\Elem{G}$ is finite.  All finite graphs form a (sub)category (of \GG) denoted by $\GGfin$. \zdzd{we can replace $\GGfin$ by $\GG_\mathsf{fin}$ to make it less sexy.}
\end{mydef}
\ActTR{}{We will try to depict 'graphs' as graphical objects. For example, if object $H\in \II$ has exactly two non-looping outgoing arrows, say, $x,y$, we will call them {\em source} and {\em target}, and depict each element $a\in G(H)$ as an arrow from element $a.G(x)$ to element $a.G(y)$. %If $I \in \cat{I}$ has no other outgoing morphisms than the identity $\identity{I} : I \to I$, we call elements $x \in G(I)$ \emph{nodes} otherwise \emph{edges} or \emph{arcs}.
%}
%\zdhll{If there exists a morphism $\arrow{I}{j}{J} \in \II$ and $J$ has outgoing non-identity morphisms we further call an element $x \in G(I)$ a \emph{hyperedge}.}{to be checked}{-7}
\zdzd{\textcolor{blue}{hm, most probably, to give the name 'graph' more intuitive sense, we need to pose some conditions on \II, say, require \II\ to be a rooted dag, whose root is called \Node, children are different sorts of 1-hyperesges, then we will have 2-hyper-edges, etc. Binary hyperedges (exactly two arrows to the parents) are called arrows. ...I guess having such a structure would be very useful for parsing, but maybe it's even necessary for parsing?? If so, then parsing would be a much nicer result. I once came to having some structure over \II\ when thinking about equations as a result of parsing.}}
} % the end of TR-Act24 diff
%\mkRemark{Presheaf notation}{rem:presheaf}
%\clearpage
\begin{myexa}[Fancy Graph with Hyperedges]
	\label{exa:samplepresheaf}%\zd{make the span-thing with arrow $\ta_1$ accurate}
	Assume $\II$ is the category in \cref{fig:fancyGraph}(a) (identities omitted), in which the stroked arrow \so\ from node \HEdge\ is a shorthand for a span, \ie, one more node $X_{\so\so}$ and two leg arrows $x_{\so\so}$ and $x'_{\so\so}$  from $X_{\so\so}$ into \HEdge\ and \Node\ resp.  \cref{fig:fancyGraph}(b) depicts a \II-graph given by the following functor $G : \II \to \setcat$. The value of $G$ for objects of \caty\ a) is this:  $G(\Node)=\{A,B,P,Q\}$, $G(\Edge)=\{f,g,i\}$, $G(\text{2-\Edge})=\{\alpha\}$, $G(\HEdge)=\{h\}$, and $G(X_{\so\so})=\{hA, hP\}$, while the value of $G$ on \II-arrows can be easily derived from image b), \eg, $G(x_{\so\so})(hA)=h$, $G(x'_{\so\so})(hA)=A$, $G(\ta_1)(h)=Q$, $G(\ta_2)(h)=g$ (\ie, tentacles with hollow circles instantiate span \so\so\ from \HEdge\ to \Node, tentacles with black circle instantiate arrow $\ta_2$) and so on. Elements instantiating objects \Edge\ and 2-\Edge\ are visualized by arrows as usual. 
\begin{figure}[h]
	\centering 
\begin{tabular}{cc}
\parbox{0.45\linewidth}{
			$\xymatrix @C=1em @R=3em {
				& \Node & \\
				\mathsf{HEdge}  
					%\ar@/^1.7pc/[ur]^{\ta_1}|{|}
					\ar@<0.6ex>[ur]^{\so\so} | {|}
					\ar@<-0.6ex>[ur]_{\ta_1} 
					%\ar@/_1.7pc/[ur]_{\ta_2} 
					\ar[rr]^{\ta_2}
				&&  \Edge \ar@<-0.5ex>[ul]_{\ta} \ar@<0.5ex>[ul]^{\so}  %\\
				&&  \text{2-\Edge} \ar@<-0.5ex>[ll]_{\ta} 
											\ar@<0.5ex>[ll]^{\so}
}$
} % end parbox
&
\parbox{0.45\linewidth}{\centering
				\includegraphics[width=0.55\linewidth]{pdfs/fancyGraph-2}
} % end parbox
\\
a) Metaschema \II\  for 'graphs'
& b) 	A sample `graph' $G$ instantiating \II
\end{tabular}
\caption{Example of a higher-order graph with a complex hyperedge
%\\ \zd{consider joining $\ta_{1,2}$ into a span, say,  $\ta_{12}$, then node $P$ is to be renamed into, say, $B$, while $B$ is to be renamed into, say, $P$, so that the hyperedge $h$ would include set $\{A,C\}$ at the filed name $\ta_{12}$. Then $Q$ is to be renamed into, say, $X$.}
}
\label{fig:fancyGraph}
\end{figure}
%%\begin{align*}
%%	G(\Node) =  &\{P, Q, A, B\}  
%%	&  	G(\so_{_\text{@2-\Edge}}) =  \alpha \mapsto f \\
%%	G(\Edge) = &\{f,g,i\}  %\text{~(three edges)~}
%%	& 	G(\ta_{_\text{@2-\Edge}})  = \alpha \mapsto g \\
%%	G(\text{2-\Edge}) =& \{\alpha\}  & G(\ta_1) =  m \mapsto A \\
%%	G(\mathsf{HEdge}) = & \{h\} & G(\ta_2) =  m \mapsto B \\
%%	G(\so_{_\text{@\Edge}}) = &\{f \mapsto A, g \mapsto A, i \mapsto Q \}& G(\ta_3) =  m \mapsto P  \\
%%	G(\ta_{_\text{@\Edge}}) =  & \{f \mapsto B, g \mapsto B, i \mapsto Q\} & G(\ta_4) =  m \mapsto Q \\
%%\end{align*}
%%%The example exemplifies different features graphical features. 
%Elements of $G(0)$ can be called nodes, elements of $G(1)$ and $G(2)$ can be visualized as arrows (since the respective object in $\II$ has exactly two outgoing non-identity morphisms.
%There is an edge between edges, $\alpha$,  and a hyperegde $n$ connecting four elements (``sources'' of the hyperedge) as shown (as the respective object in $\II$ has more than two outgoing non-identity morphisms).
%Lines connecting a hyperedge to its sources  will be called \emph{tentacles}.
%}
\end{myexa}

%\END 

==> sections/subsec--genGraphs-modified.tex <==
%\renewcommand{\HH}{\enma{H}}
\subsection{Generalized Graphs}\label{sec:genGraphs}
%The rationale  behind this terminology is due to arguably the most import representative: \emph{directed multigraphs}.
As our discussion in Sect.2 suggests, we need a very general notion of graphs as (co)presheaves  \frar{G}{\II}{\setcat} for a suitable category $\II$ called {\em metaschema}. \zdmodd{In all our applications, graphs have \hical\ structure that allows their traversal from the top elements to the bottom. 
%our with the only restriction is an arbitrary but fixed finite category whose objects are called {\em cell types}, and for object $H\in\HH$, elements of set $G(H)$ are called $G$'s {\em cells of type $H$}. 
For example, ordinary directed multigraphs are given by schema $\II=\Graph$ with $\Ob{\Graph}=\{\nfont{Node},\nfont{Arrow}\}$ and two non-identity arrows \frar{\so,\ta}{\nfont{Arrow}}{\nfont{Node}} so that object \nfont{Arrow} is above \nfont{Node}
\shortlong{Other examples can be found in the TR.
}{(Below we will show other examples.)}
Hence, we require category \II\ to be \hical\ in the folloiwng sense.}{}{NoNoNo!!!} {-3}

\begin{mydef}[Graphs]
	\label{def:hgraph}
	Let \II\ be a \caty. An {\em \II-graph} is a functor \frar{G}{\II}{\setcat}, \ie, a presheaf over {\em schema} \II. We will normally refer to such functors as merely graphs, but if we want to stress their distinction from ordinary directed multigraphs (which are functors \frar{G}{\II_\graph}{\setcat} over schema specified in \cref{eq:schema4graphs}), we will refer to them as \II-graphs or, sometimes, as 'graphs' in single quotes. 
%	\begin{equation}\label{eq:schema4graphs}
%	\begin{tabular}{c}
%	$	\xymatrix{
%		\nfont{Node} 
%		& \nfont{Arrow} \ar@/^4pt/[l]^{\ta}\ar@/_4pt/[l]_{\so}	
%	} $
%	\\
%	Schema \Graph\ for ordinary (directed multi-)graphs
%	\end{tabular}
%	\end{equation}
	For a graph \hgrarr, elements of set $G(H)$ with $H\in\II_n$ are called {\em n-cells (of type $H$)}, and if $\II_n$ is not a singleton, we say that $n$-cells are multi-sorted. We write $\Elem{G}$ for the set $\bigcup_{H\in\Ob{\II}}G(H)$. 
	
	The presheaf topos of all \II-graphs will be denoted by \GG, and we assume that throughout the paper the schema \II\ is arbitrary but fixed. A graph $G$ is {\em finite} if $\Elem{G}$ is finite.  All finite graphs form a (sub)category (of \GG) denoted by $\GGfin$. \zdzd{we can replace $\GGfin$ by $\GG_\mathsf{fin}$ to make it less sexy.}
\end{mydef}
We will try to depict 'graphs' as graphical objects. For example, if object $H\in \II$ has exactly two non-looping outgoing arrows, say, $x,y$, we will call them {\em source} and {\em target}, and depict each element $a\in G(H)$ as an arrow from element $a.G(x)$ to element $a.G(y)$. %If $I \in \cat{I}$ has no other outgoing morphisms than the identity $\identity{I} : I \to I$, we call elements $x \in G(I)$ \emph{nodes} otherwise \emph{edges} or \emph{arcs}.
%\zdhll{If there exists a morphism $\arrow{I}{j}{J} \in \II$ and $J$ has outgoing non-identity morphisms we further call an element $x \in G(I)$ a \emph{hyperedge}.}{to be checked}{-7}

\zdzd{hm, most probably, to give the name 'graph' more intuitive sense, we need to pose some conditions on \II, say, require \II\ to be a rooted dag, whose root is called \Node, children are different sorts of 1-hyperesges, then we will have 2-hyper-edges, etc. Binary hyperedges (exactly two arrows to the parents) are called arrows. ...I guess having such a structure would be very useful for parsing, but maybe it's even necessary for parsing?? If so, then parsing would be a much nicer result. I once came to having some structure over \II\ when thinking about equations as a result of parsing.}
%\mkRemark{Presheaf notation}{rem:presheaf}
\clearpage
\begin{myexa}[Fancy Graph with Hyperedges]
	\label{exa:samplepresheaf}%\zd{make the span-thing with arrow $\ta_1$ accurate}
	Assume $\II$ is the category in \cref{fig:fancyGraph}(a) (identities omitted), in which the stroked arrow \so\ from node \HEdge\ is a shorthand for a span, \ie, one more node $X_{\so\so}$ and two leg arrows $x_{\so\so}$ and $x'_{\so\so}$  from $X_{\so\so}$ into \HEdge\ and \Node\ resp.  \cref{fig:fancyGraph}(b) depicts a \II-graph given by the following functor $G : \II \to \setcat$. The value of $G$ for objects of \caty\ a) is this:  $G(\Node)=\{A,B,P,Q\}$, $G(\Edge)=\{f,g,i\}$, $G(\text{2-\Edge})=\{\alpha\}$, $G(\HEdge)=\{h\}$, and $G(X_{\so\so})=\{hA, hP\}$, while the value of $G$ on \II-arrows can be easily derived from image b), \eg, $G(x_{\so\so})(hA)=h$, $G(x'_{\so\so})(hA)=A$, $G(\ta_1)(h)=Q$, $G(\ta_2)(h)=g$ (\ie, tentacles with hollow circles instantiate span \so\so\ from \HEdge\ to \Node, tentacles with black circle instantiate arrow $\ta_2$) and so on. Elements instantiating objects \Edge\ and 2-\Edge\ are visualized by arrows as usual. 
\begin{figure}[h]
	\centering 
\begin{tabular}{cc}
\parbox{0.45\linewidth}{
			$\xymatrix @C=1em @R=3em {
				& \Node & \\
				\mathsf{HEdge}  
					%\ar@/^1.7pc/[ur]^{\ta_1}|{|}
					\ar@<0.6ex>[ur]^{\so\so} | {|}
					\ar@<-0.6ex>[ur]_{\ta_1} 
					%\ar@/_1.7pc/[ur]_{\ta_2} 
					\ar[rr]^{\ta_2}
				&&  \Edge \ar@<-0.5ex>[ul]_{\ta} \ar@<0.5ex>[ul]^{\so}  %\\
				&&  \text{2-\Edge} \ar@<-0.5ex>[ll]_{\ta} 
											\ar@<0.5ex>[ll]^{\so}
}$
} % end parbox
&
\parbox{0.45\linewidth}{\centering
				\includegraphics[width=0.55\linewidth]{pdfs/fancyGraph-2}
} % end parbox
\\
a) Metaschema \II\  for 'graphs'
& b) 	A sample `graph' $G$ instantiating \II
\end{tabular}
\caption{Example of a higher-order graph with a complex hyperedge
%\\ \zd{consider joining $\ta_{1,2}$ into a span, say,  $\ta_{12}$, then node $P$ is to be renamed into, say, $B$, while $B$ is to be renamed into, say, $P$, so that the hyperedge $h$ would include set $\{A,C\}$ at the filed name $\ta_{12}$. Then $Q$ is to be renamed into, say, $X$.}
}
\label{fig:fancyGraph}
\end{figure}
%%\begin{align*}
%%	G(\Node) =  &\{P, Q, A, B\}  
%%	&  	G(\so_{_\text{@2-\Edge}}) =  \alpha \mapsto f \\
%%	G(\Edge) = &\{f,g,i\}  %\text{~(three edges)~}
%%	& 	G(\ta_{_\text{@2-\Edge}})  = \alpha \mapsto g \\
%%	G(\text{2-\Edge}) =& \{\alpha\}  & G(\ta_1) =  m \mapsto A \\
%%	G(\mathsf{HEdge}) = & \{h\} & G(\ta_2) =  m \mapsto B \\
%%	G(\so_{_\text{@\Edge}}) = &\{f \mapsto A, g \mapsto A, i \mapsto Q \}& G(\ta_3) =  m \mapsto P  \\
%%	G(\ta_{_\text{@\Edge}}) =  & \{f \mapsto B, g \mapsto B, i \mapsto Q\} & G(\ta_4) =  m \mapsto Q \\
%%\end{align*}
%%%The example exemplifies different features graphical features. 
%Elements of $G(0)$ can be called nodes, elements of $G(1)$ and $G(2)$ can be visualized as arrows (since the respective object in $\II$ has exactly two outgoing non-identity morphisms.
%There is an edge between edges, $\alpha$,  and a hyperegde $n$ connecting four elements (``sources'' of the hyperedge) as shown (as the respective object in $\II$ has more than two outgoing non-identity morphisms).
%Lines connecting a hyperedge to its sources  will be called \emph{tentacles}.
%}
\end{myexa}

%\END 

==> sections/subsec--sign-as-profunctors.tex <==
\subsection{Signatures as profunctors/barrels}\label{sec:sign-as-profunctors}


Given a schema \II\ for graphs, a predicate signature over \II\ is a functor \frar{\arfun}{\predsig}{\oppCat{(\setcat^{\II})}} or 
\frar{\arfunop}{\predsigop}{{\setcat^{\II}}}. Currying gives us a profunctor
\begin{equation}\label{eq:arprofun}
	\frar{\arfunpro}{ \predsigop\times\II}{\setcat}.
\end{equation}
which maps a pair of objects $P\in\predsig$, $X\in\II$   to the set 
\begin{equation}\label{eq:wavyarr-ovr}
	\arfunpro(P,X )=\compr{\ovr{a}}{a\in P^\arfun(X)}
\end{equation}
where writing $\ovr{a}$ is a notational trick to show the change of the role of element $a$ from being an element of an arity shape to being a wavy (binding) arrow 
\frar{\ovr{a}}{P}{X}%
\footnote{with a more formal attitude, we can consider $\ovr{a}$ as a pair $(a,*)$ with * being some predefined token}. %note that arrows go from the second component of the pair to the first one). 
In the opposite direction, we write $\und{a}\in P^\arfun(X)$ for a given wavy arrow $a\in\arfunpro(P,X)$, thus,  
\begin{equation}\label{eq:wavyarr-und}
	P^\arfun(X) =\compr{\und{a}}{a\in\arfunpro(X,P)}
\end{equation}
and $\ovr{\und{a}}=a$ for any $a\in \arfunpro(X,P)\sqcup P^\arfun(X)$.
%\zd{Of course it's better to write this accurately as a canonic iso\mor\ between sets $P^\arfun(P)(X)$ and 		  	$\arfunpro(P,X)$  established by bijections \ovr{...\strut} and \und{...}. This is an instance of what I once called Lemma 2/Fact 2 (while Fact 1 is Groth. Equiv.), but it seems we don't need this general Fact 2 and the instance above is enough. }

%The collage construct below makes it all precise. 
It is known that any profunctor is equivalent to a cospan of functors 
\begin{equation}\label{eq:collcospan}
	%\predsig\hookrightarrow\pstarii\hookleftarrow\II	
	\collageHP
\end{equation}
whose apex is the {\em collage} category of the profunctor and legs are full embeddings \citebenabu. {\sc Add citation: 1) Distributors at Work by Jean B\'enabou June 2000 2) Joyal's CatLab Distributors and barrels.}

The collage \caty\ is defined as follows. $\Ob{\,\pstarii}=\Ob{\II}\sqcup\Ob{\predsig}$, and for a pair of objects $X,Y \in \Ob{\,\pstarii}$, %$P\in\predsig$, $X\in\II$, 
we set
\begin{equation}	\label{eq:collage}
\pstarii\,(X,Y) = 
	\begin{cases}
		\predsig(X,Y)  & \mbox{ if } X, Y\in\predsig \\
		\II(X,Y) &  \mbox{ if } X,Y\in\II \\
		{\arfunpro}(X,Y) & \mbox{ if } X\in\PP  \mbox{ and } Y\in\II  \\
		\varnothing & \mbox{ if } X \in\II \mbox{ and }  Y\in\PP 
	\end{cases}
\end{equation}
\zdmodd{Note that for category \pstarii, the usual notation for hom-sets is reversed and formula  $\iistarp(\_, P)$ denotes the set of arrows {\em from} $P$.}{}{see ZD-comment below in red}{-5} 
\\
\zd{In the previous version, the arrows were reversed b/c i first wrote the discrete \hical\ section 4.3 where layers are built from the left to the right (which is normal) but then aritywavy arrows go from the right to the left. To keep the arity-wavy arrows as written an odd decision to reverse the dir of arrows in hom-sets was taken. In the current version, hom-sets are normal, but the hierarchical sections is to be fixed.}
%\zdzd{I am not happy with this reversal but  So, maybe it's less painful to keep it as is.} 
\begin{wrapfigure}{r}{3.5cm}
	\vspace{-2ex}
	\centering
	\xymatrix @C=6em{
		X \ar@{<-}[r]^a %{\arfunpro(p,X)}
		& P \ar@{<-}[d]^{p}
		\\
		X' \ar@{<-}[u]_h 
		\ar@{<-}[r]^{a'=\arfunpro(h,p)(a)}
		& P' 
	}
\end{wrapfigure}
\noindent Arrow composition is given by functions $\arfunpro(h, \id)$ and $\arfunpro(\id,p)$ as shown in the inset figure, and its  associativity is ensured by the functoriality of \arfun. Arrows in $\arfunpro(X,Y)$ are sometimes called {\em formal} or {\em wavy}; in our context, they are exactly {\em binding} arrows we considered in the example above. 


It is easy to see that the collage category above is an instance of the following construct.
\begin{mydef}\label{def:formalSig}
	A {\em split} \hcaty\  is a pair $(H, m)$ with H\ a \hical\ \caty\ of height $N\ge 2$ and $m\in (0,N)$ a natural number. Objects of height less than $m$ (there is at least one) are called {\em cell types} or {\em graphical}; they and arrows between them form a full category $H_{[0,m)]}\subset H$. Objects of height more or equal to $m$ (there is at least one) are {\em predicate symbols} (logical elements); they and arrows between them form a full subcategory $\PPha\subset H$. Arrows from predicate symbols to cell types are called {\em wavy}.
	%	We will write an ha-signature  as a chain of categories
	%	$$\XPha\subset\PPha_0\subset\ldots\PPha_{N-1}$$
	%	(but note that the \Parl-height of, say, $\PParl_0$ elements is $m$).
\end{mydef}
\zd{It seesm all the hassle above is for saying that we have a barrel. Then all the hassle with hierarchical cats is also redundant: a signature is a profunctor, hence a barrel, hence the carrier category of pred symbols is divided into a schema for graphs, a pred signature as such, and a set fo arity arrows from predicates to graphical elements.  }
\begin{myprop}\label{prop:predsig:func=arless}
	The constructs of a predicate signature and a split \hcaty\ are naturally equivalent.
\end{myprop}
\begin{proof} Let $(H, \heifun, m)$ is a split \hcaty\ of height $N$. The intermediate $m$ generates  a functor %\frar{\hat m}{\overrightarrow{N}}{\overrightarrow{2}}, 
	\frar{\nfont{m}}{[0,N-1]}{[0,1]} whose composition with \heifun\ gives us a barrel \frar{\brl=\heifun\comp\nfont{m}}{H^\oppind}{[0,1]} and hence a profunctor \frar{\check \brl}{\HPha\times\PPha^\oppind}{\setcat} (see Joyal \cite{}); uncurrying the latter gives us a signature \frar{\arfun_{m}}{\PPha^\oppind}{\setcat^{\HPha}}.  
	%Note that arity \frar{X^{\arfun_{m}}}{\XPha}{\setcat} of an element $X$ is nothing but the hom-functor $H(P,\_)$ restricted to graphical elements. 
	The opposite transformation was considered above. Natural iso\mor\ of exponentiation and currying, and of profunctors and barrels, give us required natural equivalence. Thus, we can consider any split \hcaty\ as the collage \iistarp\ of a graphical schema $\II=H_{[0,m)}$ and a signature $\PP=H_{[m,N)}$ with arity $\arfun_m$ defined as above.
\end{proof}
 %The second (and final) step is given by the following result. 


==> sections/subsec-whyConstraintsIndexed.tex <==
\subsubsection{\thissecnum.3  Why constraints may need indexing.}
\label{sec:whyConstrIndexed}
%\begin{myexa}[Constraints in Software Engineering]
Consider Fig.~\ref{fig:constraintsSEExample}. 
It comprises a software specification for modeling the human resources information system.
It contains two classifiers \texttt{Employee} and \texttt{Department} with its respective attributes and there is a reference \texttt{manages} between both classifiers stating which employee manages which department.
From interviews with different domain experts, one may record two requirements \emph{Req1} and \emph{Req2}.
The first requirement is a rather fuzzy natural language formulation that every department should have a small managerial team. The second requirement states that every Department should have exactly one manager. The system designers implemented  REQ1 by declaring the multiplicity (constraint) for the \corring\ end of association $\nfont{manages}$ to be  [1..3], while REQ2 is implemented by a multiplicity [1..1]. Clearly, [1..1] implies [1..3] but system designers may prefer to keep both constraints for traceability and map REQ1 to [1..3] and REQ2 to [1..1].  
Later it may turn out that the implementation of REQ1 by [1..3] is ineffective and REQ1 is re-implemented with multiplicity [1..1]. Hence, the implementations (= predicates) of both requirements are actually identical, but for traceability and further maintenance, it makes sense to keep two different indexes  REQ1 and REQ2 mapped to the same constraint [1..1]. % to clearly separate the requirements and be able to react to change in requirements.
\begin{figure}
	\centering
	\includegraphics[width=0.5\linewidth]{figures/SimpleConstraint}
	\caption{Constraints in SE} 
	\label{fig:constraintsSEExample}
\end{figure}
%\end{myexa}


==> sections/subske-op.tex <==
\begin{includeLong}
\subsection{Some operations on sketch subobjects}
\begin{mydef}[Operations between subobject semi-lattices]
	\label{def:specialSketchMorphisms}
Let $\predsig$ be a predicate signature and $S \in \skecatgp$ a sketch.
There is a subobject functor 
\[
	\subskefun{S} : \subobjlattice{\carrier{S}} \to \subobjlattice{S}
\]
which adds to a subgraph $G \subseteq \carrier{S}$ all $S$-constraint that can be declared on $G$.
\zdhllno{It is defined via the right adjoint $\pbfunctorRightAdjoint{(id,\boldsymbol{!})}$ of the pullback functor $\arrow{\subobjlattice{S}}{\pbfunctor{(id,\boldsymbol{!})}}{\subobjlattice{\carrier{S}}}$, see Remark~\ref{rem:setTheory}.}{lets talk about this def!!}{-10}
Note that $\carrier{S}$ can be interpreted as a sketch without diagrams, thus there is a canonical sketch morphism $\arrow{\carrier{S}}{(id,\boldsymbol{!})}{S}$ in $\skecatgp$.\par

Furthermore, there is another functor 
\[
	\subsigfun{\predsig } : \skecatgp \to \subobjlattice{\predicateSig}
\]
which maps a $\predicateSig$-sketch $S$ to its effective predicate signature, i.e. those predicates from \predsig\ that are actually used in the sketch, $\subsigfun{\predicateSig}(S) \subseteq \predsig$.
It is defined as the image of $\labell$, i.e. $\subsigfun{\predicateSig}(S) = \image{\labell}$. Arrows in $\subobjlattice{\predsig}$ are inclusions and $\subsigfun{\predsig}$ is obviously a functor.

Finally, if $\PP'$ is a subsignature of \PP, \ie, $\carr{\PP'}\subset\carr{\PP}$ in \catcat, and $\frestr{\arfun'}{\PP}=\arfun$, then we have a forgetful functor \frar{\frestr{\_}{\PP'}}{\GG||\PP}{\GG||\PP'}. 
\end{mydef}
\end{includeLong}

\zd{It is very disappointing that nothing is said about sketch semantics}
\bigskip
\bfem{The rest of the page is intentionally empty .}

==> sections/tab-sig2.tex <==
 \begin{table}[h]
 	%\begin{wraptable}{R}{0.35\textwidth}
 	%\vspace{-1cm}
 	\caption{Complex conjunctive constraints $\phi$ over signature in \cref{tab:sign}
 	\\ \zd{[inverse] is incorrectly defined. A correct def is a) to define query $\dom(r)$ and then require 
 	\\ $[\subseteq_2](\dom(p), p.q)\wedge\subseteq_2](\dom(q), q.p)$. 
 	\\ But this def essentially uses queries \dom(.) and \_.\_ , so...? It's better to omit it here, and perhaps define it immediately in \cref{tab:sign}]}
 } \label{tab:signComplexConj}
 	\vspace{0.1cm} 
 	\centering
 	\begin{tabular}{|c|c|c|}
 		\hline
 		$\phi$'s name & Arity shape, $S_\phi$ & $\phi$'s logical structure, \skelogictxt{$\phi$}\mathstrut
 \\   [2.5pt]  \hline \hline%ROW 1
 [1] & 		
 \begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
 	E  %\ar[loop left, <-, "e", distance=2em, start anchor={[yshift=-1ex]west}, end
 	    %anchor={[yshift=1ex]west}]  
 	\ar[r,  "r "] % \ar[r, <-, shift right=0.75ex, "q" '] 
 	& F 
 \end{tikzcd}
   & $[1..*](r) \wedge [0..1](r)$
 \\ [5pt] \hline 
 		[inverse] & 
 		\begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
 			E \ar[loop left, <-, "e", distance=2em, start anchor={[yshift=-1ex]west}, end
 			         anchor={[yshift=1ex]west}]  
 			\ar[r, shift left=0.75ex, "p "] \ar[r, <-, shift right=0.75ex, "q" '] 
 			& F\ar[loop right, <-, "f", distance=2em, start anchor= 			
 			   {[yshift=1ex]east}, end anchor={[yshift=-1ex]east}]
 		\end{tikzcd}
 		& 
 		\mbox{$[\id](e)\wedge[\subseteq](p,q,e)\wedge [\id](f)\wedge[\subseteq](q,p,f)$}
 \\ \hline   % Row 3
         \bndRsrcX{1} \rule{0mm}{10mm}$_{\rule{0mm}{12mm}}$
  & 
  \begin{tikzcd}[row sep=5ex, column sep=7ex,cells={nodes={draw=black, %circle, 
  			                          outer sep=0pt,inner sep=.35ex}}]
  	\Resr_1 & \Owner \ar[l, "\owns_1" '] \ar[ld,"\gapnamegap{1}{\owns_2}{-1}" ', pos=0.75] \ar[d, "\owns_3"]
  	\\
  	\Resr_2 & \Resr_3
 \end{tikzcd}
 & $
 \mathrm{[or]}(\owns_1, \owns_2)\wedge [0..1](\owns_1) \wedge [0..1](\owns_3)
  $
  \\ \hline 
\end{tabular}
\end{table}


==> sections/tab-sig2bang.tex <==
 \begin{table}[h]
 	%\begin{wraptable}{R}{0.35\textwidth}
 	%\vspace{-1cm}
 	\caption{Complex conjunctive constraints $\phi$ over signature in \cref{tab:sign}} \label{tab:signComplex}
 	\vspace{0.1cm} 
 	\centering
 	\begin{tabular}{|c|c|c|}
 		\hline
 		$\phi$'s name & Arity shape, $S_\phi$ & $\phi$'s logical structure, \skelogictxt{$\phi$}\mathstrut
 \\    \hline \hline %ROW 1
 		[inverse] & 
 		\begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
 			E \ar[loop left, <-, "e", distance=2em, start anchor={[yshift=-1ex]west}, end
 			         anchor={[yshift=1ex]west}]  
 			\ar[r, shift left=0.75ex, "p "] \ar[r, <-, shift right=0.75ex, "q" '] 
 			& F\ar[loop right, <-, "f", distance=2em, start anchor= 			
 			   {[yshift=1ex]east}, end anchor={[yshift=-1ex]east}]
 		\end{tikzcd}
 		& 
 		\mbox{$[\id](e)\wedge[\subseteq](p,q,e)\wedge [\id](f)\wedge[\subseteq](q,p,f)$}
 \\ \hline   % Row 3
         [bndRsrc]$_1$ \rule{0mm}{10mm}$_{\rule{0mm}{12mm}}$
  & 
  \begin{tikzcd}[row sep=5ex, column sep=7ex,cells={nodes={draw=black, %circle, 
  			                          outer sep=0pt,inner sep=.35ex}}]
  	\Resr_1 & \Owner \ar[l, "\owns_1" '] \ar[ld,"\gapnamegap{1}{\owns_2}{-1}" ', pos=0.75] \ar[d, "\owns_3"]
  	\\
  	\Resr_2 & \Resr_3
 \end{tikzcd}
 & $
 \mathrm{[or]}(\owns_1, \owns_2)\wedge [0..1](\owns_1) \wedge [0..1](\owns_3)
  $
  \\ \hline 
\end{tabular}
\end{table}


==> sections/tab-sig3.tex <==

 
 \begin{table}[h]
 	%\begin{wraptable}{R}{0.35\textwidth}
 	%\vspace{-1cm}
 	\caption{Implicational  constraints $\phi$
 		\\ \zd{Row 3 is for future use!!}
 		\\ \zd{it makes sense to join tables \cref{tab:signComplexConj} and \cref{tab:signComplexConj}}
 		}
   \label{tab:signComplexImpl}
 	\vspace{0.1cm} 
 	\centering
 	\begin{tabular}{|c|c|c|}
 		\hline
 		$\phi$'s name & Arity shape, $S_\phi$ & $\phi$'s logical structure, \skelogictxt{$\phi$}\rule{0mm}{5mm}%{0mm}
 \\    \hline \hline %ROW 1 inv2inj
 	[inv2inj] & 
 		\begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
 			E \ar[loop left, <-, "e", distance=2em, start anchor={[yshift=-1ex]west}, end
 			anchor={[yshift=1ex]west}]  
 			\ar[r, shift left=0.75ex, "p "] \ar[r, <-, shift right=0.75ex, "q" '] 
 			& F\ar[loop right, <-, "f", distance=2em, start anchor= 			
 			{[yshift=1ex]east}, end anchor={[yshift=-1ex]east}]
 		\end{tikzcd}
 		& 
 		\mbox{$[\mathrm{inverse}](e,p,q,f)\Rightarrow [0..1](p) \wedge [0..1](q)$}
 \\	\hline  %\hline  % Row 2
         \bndRsrcX{2}\rule{0mm}{10mm}$_{\rule{0mm}{12mm}}$
  & 
  \begin{tikzcd}[row sep=5ex, column sep=7ex,cells={nodes={draw=black, %circle, 
  			                          outer sep=0pt,inner sep=.35ex}}]
  	\Resr_1 & \Owner \ar[l, "\owns_1" '] \ar[ld,"\gapnamegap{1}{\owns_2}{-1}" ', pos=0.75] \ar[d, "\owns_3"]
  	\\
  	\Resr_2 & \Resr_3
 \end{tikzcd}
 & $\text{[or]}(\owns_1,\owns_2)\Rightarrow [0..1](owns_3)
 $
\\ \hline
         [bndOr]$_2$ \rule{0mm}{10mm}$_{\rule{0mm}{12mm}}$
& 
\begin{tikzcd}[row sep=5ex, column sep=7ex,
	cells={nodes={%circle, 
			outer sep=0pt,inner sep=.35ex}}]
	\basenodeRect{\Resr$_1$} & \basenodeRect{\Owner} \ar[l, "\owns_1" '] 
	\ar[ld, derived, "\gapnamegap{0}{\owns_{1+2}}{-5}" ', description, pos=0.75] 
	\ar[d, "\owns_2"]
	\\
	\dernode{\Resr_{1+2}} \ar[r, derived, <-, "\owns_1'" ' ] 
                     	\ar[u, derived, <-, "\owns_2' " ]     
	& \basenodeRect{\Resr$_2$}
\end{tikzcd}
& $[0..2](\owns_1)\wedge [0..2](\owns_2) ,\owns_2) \wedge [0..2](\owns_{1+2})
$
\\ \hline
\end{tabular}
\end{table}


==> sections/tab-sign.tex <==
\begin{table}[h]
 %\begin{wraptable}{R}{0.35\textwidth}
 %\vspace{-1cm}
 \caption{Sample Constraints \label{tab:sign}}
 \vspace{0.1cm} 
 \centering
  \begin{tabular}{|c|c|c|}
   \hline
   Name, $c$ & Arity shape, $S_c$ & Semantics for $t\models c$ (in FOL)
   \\ \hline \hline %\row 0
  [1..*] & $\xymatrix{ % constraint [1..*] 
 	*+[o][F-]{A}\ar@{->}[r]^{r}_{\rule{0mm}{2mm}}  % |-*=0@{>}
 	%*+[o][F-]{A}\ar% |-*=0@{>}[r]^{r}_{\rule{0mm}{2mm}} 
 	& *+[o][F-]{B}}$
 &  $\forall a\exists h\; r^t(a,h,b)$ %\wedge  r^t(a,h_2,b_2) \Rightarrow  b_1=b_2$  
   \\   \hline  % row 1
 [0..1] & $\xymatrix{ % constraint [0..1]
 	*+[o][F-]{A}\ar@{->}[r]^{r}_{\rule{0mm}{2mm}}  % |-*=0@{>}
 	%*+[o][F-]{A}\ar% |-*=0@{>}[r]^{r}_{\rule{0mm}{2mm}} 
 & *+[o][F-]{B}}$
 &  $ r^t(a,h_1,b_1)\wedge  r^t(a,h_2,b_2) \Rightarrow  b_1=b_2$
 \\ \hline % row 1'
 [0..2] & $\xymatrix{ %% constraint [0..2]
 	*+[o][F-]{A}\ar@{->}[r]^{r}_{\rule{0mm}{2mm}}  % |-*=0@{>}
 	%*+[o][F-]{A}\ar% |-*=0@{>}[r]^{r}_{\rule{0mm}{2mm}} 
 	& *+[o][F-]{B}}$  %end diagram
 	&  % now its semantics
 $\begin{array}{l}
 	 r^t(a,h_1,b_1)\wedge  r^t(a,h_2,b_2) \wedge r^t(a,h_3,b_3) \\ 
 	 \Rightarrow  \quad b_1=b_2 \vee b_2=b_3\vee b_1=b_3
 	\end{array}$  % end semantics
  \\  \hline  % row 2
  [trans] & % begin diagram foir [trans]
  $ \begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
  A\ar[loop right, "r",  loop right, distance=2em, start anchor={[yshift=1ex]east}, end anchor={[yshift=-1ex]east}, %"\rule{0mm}{5mm}"
  ]
\end{tikzcd}$
    & $r^t(a_1,h_1,a_2) \wedge r^t(a_2,h_2,a_3) \Rightarrow \exists h\; r^t(a_1,h,a_3)$
\\  \hline % row 4 [or]
    [or] & $\xymatrix{*+[o][F-]{B_1} 
    	& *+[o][F-]{A}\ar@{->}[r]_{r_2}^{\rule{0mm}{2mm}}\ar@{->}[l]^{r_1} 
    	& *+[o][F-]{B_2} }$ 
    & $\forall a\in A^t\left( \exists h_1\, r_1^t(a,h_1,b_1) \vee \exists h_2\,r_2^t(a,h_2,b_2)\right)$
\\  \hline  % row 5 [id]
    [id] & % diagram for id
    $ \begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
    	A\ar[loop right, "r", loop right, distance=2em, start anchor={[yshift=1ex]east}, end anchor={[yshift=-1ex]east}, %"\rule{0mm}{5mm}"
    	]
    \end{tikzcd}$
    &  $r^t=\id{(A^t)}$ (that is, $\forall a\in A^t\exists!h\;r^t(a,h,a)$)
   \\  \hline  % row 3*
    [=$_2$] & $\xymatrix{ % diagram for [=_2]
    	*+[o][F-]{A}\ar@<.5ex>[r]^{r_1}_{\rule{0mm}{2mm}} 
    	                   \ar@<-.5ex>[r]_{r_2}_{\rule{0mm}{2mm}}
   	& *+[o][F-]{B}}$ % end diagram
    &  $r_1^t = r_2^t$ %$ \exists h_1\, r_1^t(a,h_1,b)\Leftrightarrow \exists h_2 r_2^t(a,h_2,b) $
       \\  \hline  % row 4
    $[=]$ & 
%    	$\xymatrix{ % diagram for [=_3]
%    	*+[o][F-]{A}\ar@{->}[r]_{r_1}\ar@/^1pc/@{->}[rr]^{r_3} 
%    	& *+[o][F-]{B}\ar@{->}[r]_{r_2} 
%    	& *+[o][F-]{C}
%    	}$  % end diagram for [=_3] 
% tikz diagram for [=_3]
$ \begin{tikzcd}[cells={nodes={draw=black, circle, outer sep=0pt,inner sep=.35ex}}]
A \ar[r, "r_1"'] & B\ar[r, "r_2"'] & C \ar[ll, <-, bend right=25, "r" ']
\end{tikzcd}$  % end tikz diagram  '
    & % semanrics for [=_3] 
    $r_1^t.r_2^t = r_3^t$ %(which abbreviates a FOL formula)
 %    $\begin{array}{c}
%    	\text{ Conjunction of $[\subseteq]$ above and the folloiwng condition: }
%    	\\
%    	r^t(a,h, c) \Rightarrow \exists h_1\,r_1^t(a,h_1,b) \wedge  \exists h_2\,r_2^t(b,h_2,c) 
%    \end{array}$
%    
\\  \hline  % row 5
$[\subseteq_2$] & $\xymatrix{ 
	*+[o][F-]{A}\ar@<.5ex>[r]^{r_1}_{\rule{0mm}{2mm}} 
	\ar@<-.5ex>[r]_{r_2}_{\rule{0mm}{2mm}}
& *+[o][F-]{B}}$
&  $r_1^t \subseteq r_2^t$ %$ \exists h_1\, r_1^t(a,h_1,b)\Leftrightarrow \exists h_2 r_2^t(a,h_2,b) $
\\  \hline  % row 6
 	$[\subseteq_3]$ & $\xymatrix{*+[o][F-]{A}\ar@{->}[r]_{r_1}\ar@/^1pc/@{->}[rr]^{r_3} & *+[o][F-]{B}\ar@{->}[r]_{r_2} & *+[o][F-]{C}}$ 
	& $\begin{array}{c}
		r_1^t.r_2^t \subseteq r_3^t   %\text{ (which abbreviates a FOL formula) }
	\end{array}$
\\  \hline  % row 7
	$[\supseteq_3]$ & $\xymatrix{*+[o][F-]{A}\ar@{->}[r]_{r_1}\ar@/^1pc/@{->}[rr]^{r_3} & *+[o][F-]{B}\ar@{->}[r]_{r_2} & *+[o][F-]{C}}$ 
	& $\begin{array}{c}
	r_1^t.r_2^t \supseteq r_3^t   %\text{ (which abbreviates a FOL formula) }
 \end{array}$
          \\    \hline  % end 
  \end{tabular}
 % \vspace{-0.8cm}
 %\end{wraptable}
\end{table}
